AGN and Star Formation feedback in the evolution of galaxy outflows

We conducted 3D-MHD simulations to investigate the feedback processes in the central 1kpc scale of galaxies hosting both active star formation (SF) and an AGN wind. Our simulations naturally generated a turbulent and clumpy interstellar medium driven by SF evolution. We found that the AGN wind duty cycle plays a crucial role in shaping the evolution of the outflows. This cycle consists of an active, a remnant and an inactive phase, lasting up to 1.5 Myr. The duration of the cycle increases with larger star formation rate (SFR) and smaller AGN wind power (tested for luminosities log L = 42-44 ergs per second and SFR=1-1000 solar masses per year. The feedback on SF, whether positive or negative, depends on various factors, including the AGN outflow opening angle, power, and phase of activity, as well as the initial SFR. The passage of the AGN wind enhances SF in a ring around it, resembling the structures observed in ULIRGs, and is stronger for larger AGN power or SFR. Also, a higher SFR enhances the mixing of interstellar matter with the AGN wind, resulting in a greater number of colder, denser structures with volume filling factors ~ 0.02 to 0.12 and velocities comparable to those observed in Seyferts and LINERs, but smaller than those observed in ULIRGs. The efficiency of the AGN wind in transporting mass to kiloparsec distances diminishes with increasing SFR. The mass loss rates range from 50 to 250 solar masses per year within the initial 2 Myr of evolution, which aligns with observed rates in nearby Seyferts and ULIRGs.

==> references.tex <==

@article{Fournier1901,
author={Fournier, Paul},
title={Not a Real Paper},
journal={ApJ},
fjournal={Astrophysical Journal},
volume=1,
pages={101-111},
year=1901,
}

@article{vanDijk1902,
author={{\VAN{Dijk}{Van}{van}} Dijk, Thomas},
title={An important paper},
journal={QJRAS},
fjournal={Quarterly Journal of the Royal Astronomial Society},
volume=2,
pages={202-207},
year=1902,
}

@article{deLaguarde1903,
author={{\VAN{Laguarde}{De}{de}} Laguarde, Anne},
title={Another Unreal Paper},
journal={Nat},
fjournal={Nature},
volume=3,
pages={303-304},
year=1903,
}

@article{delaGuarde1904,
author={{\VAN{Guarde}{De la}{de la}} Guarde, Simon},
title={A Last Unreal Paper},
journal={MNRAS},
fjournal={Monthly Notices of the Royal Astronomial Society},
volume=4,
pages={404-481},
year=1904,
}

@ARTICLE{Hussain_etal2023,
       author = {{Hussain}, Saqib and {Alves Batista}, Rafael and {de Gouveia Dal Pino}, Elisabete M. and {Dolag}, Klaus},
        title = "{The diffuse gamma-ray flux from clusters of galaxies}",
      journal = {Nature Communications},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = apr,
       volume = {14},
          eid = {2486},
        pages = {2486},
          doi = {10.1038/s41467-023-38226-w},
archivePrefix = {arXiv},
       eprint = {2203.01260},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023NatCo..14.2486H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Barai_dGDP2019,
       author = {{Barai}, Paramita and {de Gouveia Dal Pino}, Elisabete M.},
        title = "{Intermediate-mass black hole growth and feedback in dwarf galaxies at high redshifts}",
      journal = {\mnras},
     keywords = {black hole physics, hydrodynamics, galaxies: dwarf, galaxies: high-redshift, quasars: supermassive black holes, large-scale structure of Universe, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = aug,
       volume = {487},
       number = {4},
        pages = {5549-5563},
          doi = {10.1093/mnras/stz1616},
archivePrefix = {arXiv},
       eprint = {1807.04768},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.487.5549B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Crutcher1991,
abstract = {This paper presents a summary of all 27 available sensitive Zeeman measurements of magnetic Ðeld strengths in molecular clouds together with other relevant physical parameters. From these data input parameters to magnetic star formation theory are calculated, and predictions of theory are compared with observations. Results for this cloud sample are the following : (2) Internal motions are supersonic but approximately equal to the Alfve speed, which suggests that supersonic motions are likely MHD ?n waves. (2) The ratio of thermal to magnetic pressures b B0.04, implying that magnetic Ðelds are impor- p tant in the physics of molecular clouds. (3) The mass{\`{E}}to{\`{E}}magnetic {\~{N}}ux ratio is about twice critical, which suggests but does not require that static magnetic Ðelds alone are insufficient to support clouds against gravity. (4) Kinetic and magnetic energies are approximately equal, which suggests that static magnetic Ðelds and MHD waves are roughly equally important in cloud energetics. (5) Magnetic Ðeld strengths scale with gas densities as o BoPoi with iB0.47 ; this agrees with the prediction of ambipolar di†usion driven star formation, but this scaling may also be predicted simply by Alfve? nic motions. The measure- ments of magnetic Ðeld strengths in molecular clouds make it clear that magnetic Ðelds are a crucial component of the physics governing cloud evolution and star formation},
author = {Crutcher, Richard},
doi = {10.1049/ip-cds:20020365},
file = {:home/william/Documents/Papers/Crutcher{\_}1999{\_}ApJ{\_}520{\_}706.pdf:pdf},
issn = {13502409},
journal = {Astrophys. JOURNAL, 520706{\`{E}}713, 1991 August 1},
pages = {1--8},
title = {{MAGNETIC FIELDS IN MOLECULAR CLOUDS: OBSERVATIONS CONFRONT THEORY}},
volume = {520},
year = {1991}
}
@article{Lutz2019,
abstract = {We report new detections and limits from a NOEMA and ALMA CO(1-0) search for molecular outflows in 13 local galaxies with high far-infrared surface brightness, and combine these with local universe CO outflow results from the literature. CO line ratios and spatial outflow structure of our targets provide some constraints on the conversion steps from observables to physical quantities such as molecular mass outflow rates. Where available, ratios between outflow emission in higher J CO transitions and in CO(1-0) typically are consistent with excitation Ri1 . 1. For IRAS 13120-5453, however, R31 = 2.10 ± 0.29 indicates optically thin CO in the outflow. Like much of the outflow literature, we use $\alpha$CO(1−0)= 0.8, and we present arguments for using C=1 in deriving molecular mass outflow rates Mout = CMoutRoutvout . We compare the two main methods for molecular outflow detection: CO mm interferometry and Herschel OH-based spectroscopic outflow searches. For 26 sources studied with both methods, we find an 80{\%} agreement in detecting vout {\&} 150 km s−1 outflows, and non-matches can be plausibly ascribed to outflow geometry and signal-to-noise ratio. For the Gonz{\'{a}}lez-Alfonso et al. (2017) sample of 12 bright ultraluminous infrared galaxies (ULIRGs) with detailed OH-based outflow modeling, CO outflows are detected in all but one. Outflow masses, velocities, and sizes for these 11 sources agree well between the two methods, and modest remaining differences may relate to the different but overlapping regions sampled by CO emission and OH absorption. Outflow properties correlate better with active galactic nucleus (AGN) luminosity and with bolometric luminosity than with far-infrared surface brightness. The most massive outflows are found for systems with current AGN activity, but significant outflows in non-AGN systems must relate to star formation or to AGN activity in the recent past. We report scaling relations for the increase of outflow mass, rate, momentum rate, and kinetic power with bolometric luminosity. Short ∼ 106 yr flow times and some sources with resolved multiple outflow episodes support a role of intermittent driving, likely by AGN.},
author = {Lutz, D. and Sturm, E. and Janssen, A. and Veilleux, S. and Aalto, S. and Cicone, C. and Contursi, A. and Davies, R. I. and Feruglio, C. and Fischer, J. and Fluetsch, A. and Garcia-Burillo, S. and Genzel, R. and Gonz{\'{a}}lez-Alfonso, E. and Graci{\'{a}}-Carpio, J. and Herrera-Camus, R. and Maiolino, R. and Schruba, A. and Shimizu, T. and Sternberg, A. and Tacconi, L. J. and Wei{\ss}, A.},
file = {:home/william/Documents/Papers/aa36803-19.pdf:pdf},
issn = {23318422},
journal = {arXiv},
keywords = {Dynamics,Galaxies: ISM,Galaxies: active,Galaxies: kinematics},
pages = {1--35},
title = {{Molecular outflows in local galaxies: Method comparison and a role of intermittent AGN driving}},
volume = {134},
year = {2019}
}
@article{1977MNRAS.179..433B,
author = {Blandford, R.{\~{}}D. and Znajek, R.{\~{}}L.},
doi = {10.1093/mnras/179.3.433},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Blandford, Znajek - 1977 - Electromagnetic extraction of energy from Ken- black holes.pdf:pdf},
journal = {MNRAS},
keywords = {Active Galactic Nuclei,Astrophysics,Black Holes (Astronomy),Electromagnetic Fields,Electron-Positron Pairs,Energy Sources,Pair Production,Rotating Matter},
pages = {433--456},
title = {{Electromagnetic extraction of energy from Kerr black holes}},
volume = {179},
year = {1977}
}
@article{Klessen2015,
author = {Klessen, Ralf S. and Glover, Simon C.O.},
doi = {10.1007/978-3-662-47890-5_2},
file = {:home/william/Documents/Papers/[Klessen]-Physical Processes in the Interstellar.pdf:pdf},
isbn = {9783662478905},
journal = {Star Form. Galaxy Evol. Connect. Numer. Model. to Real. Saas-Fee Adv. Course 43. Swiss Soc. Astrophys. Astron.},
pages = {85--249},
title = {{Physical processes in the interstellar medium}},
year = {2015}
}
@article{Stacey2018,
abstract = {Determining the star-forming properties of radio-quiet quasars is important for understanding the co-evolution of star formation and black hole accretion. Here, we present the detection of the gravitationally-lensed radio-quiet quasars SDSS J1055+4628, SDSS J1313+5151 and SBS 1520+530 at 144 MHz that fall in the HETDEX Spring Field targeted in the LOFAR Two-metre Sky Survey (LoTSS) first full data release. We compare their radio and far-infrared luminosities relative to the radio-infrared correlation and find that their radio luminosities can be explained by star formation. The implied star formation rates derived from their radio and infrared luminosities are between 20 and 300 {\$}\backslashrm{\{}M{\_}{\{}\backslashodot{\}}{\~{}}yr{\^{}}{\{}-1{\}}{\}}{\$}. These detections represent the first study of gravitationally lensed sources with LOFAR, opening a new frequency window for investigating the star-forming properties of high-redshift quasars at radio wavelengths. We consider the implications for future data releases and estimate that many of the objects in our parent sample will be detected during LoTSS, significantly increasing the fraction of gravitationally lensed radio-quiet quasars with radio detections.},
archivePrefix = {arXiv},
arxivId = {1811.07932},
author = {Stacey, H. R. and McKean, J. P. and Jackson, N. J. and Best, P. N. and Rivera, G. Calistro and Callingham, J. R. and Duncan, K. J. and G{\"{u}}rkan, G. and Hardcastle, M. J. and Iacobelli, M. and Mechev, A. P. and Morabito, L. K. and Prandoni, I. and R{\"{o}}ttgering, H. J. A. and Sabater, J. and Shimwell, T. W. and Tasse, C. and Williams, W. L.},
doi = {10.1051/0004-6361/201833967},
eprint = {1811.07932},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Stacey et al. - 2018 - LoTSSHETDEX Disentangling star formation and AGN activity in gravitationally-lensed radio-quiet quasars.pdf:pdf},
issn = {14320746},
keywords = {evolution,galaxies,general,gravitational lensing,quasars,radio continuum,star-formation,strong},
pages = {1--10},
title = {{LoTSS/HETDEX: Disentangling star formation and AGN activity in gravitationally-lensed radio-quiet quasars}},
url = {http://arxiv.org/abs/1811.07932},
year = {2018}
}
@article{Mizuno2015,
abstract = {We have performed two-dimensional special-relativistic magnetohydrodynamic simulations of non-equilibrium over-pressured relativistic jets in cylindrical geometry. Multiple stationary recollimation shock and rarefaction structures are produced along the jet by the nonlinear interaction of shocks and rarefaction waves excited at the interface between the jet and the surrounding ambient medium. Although initially the jet is kinematically dominated, we have considered axial, toroidal, and helical magnetic fields to investigate the effects of different magnetic-field topologies and strengths on the recollimation structures. We find that an axial field introduces a larger effective gas pressure and leads to stronger recollimation shocks and rarefactions, resulting in larger flow variations. The jet boost grows quadratically with the initial magnetic field. On the other hand, a toroidal field leads to weaker recollimation shocks and rarefactions, significantly modifying the jet structure after the first recollimation rarefaction and shock. The jet boost decreases systematically. For a helical field, instead, the behavior depends on the magnetic pitch, with a phenomenology that ranges between the one seen for axial and toroidal magnetic fields, respectively. In general, however, a helical magnetic field yields a more complex shock and rarefaction substructure close to the inlet that significantly modifies the jet structure. The differences in shock structure resulting from different field configurations and strengths may have observable consequences for disturbances propagating through a stationary recollimation shock.},
archivePrefix = {arXiv},
arxivId = {1505.00933},
author = {Mizuno, Yosuke and G{\'{o}}mez, Jose L. and Nishikawa, Ken Ichi and Meli, Athina and Hardee, Philip E. and Rezzolla, Luciano},
doi = {10.1088/0004-637X/809/1/38},
eprint = {1505.00933},
file = {:home/william/Downloads/Mizuno{\_}2015{\_}ApJ{\_}809{\_}38.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {galaxies: jets,magnetohydrodynamics (MHD),methods: numerical,shock waves},
number = {1},
pages = {38},
publisher = {IOP Publishing},
title = {{Recollimation shocks in magnetized relativistic jets}},
url = {http://dx.doi.org/10.1088/0004-637X/809/1/38},
volume = {809},
year = {2015}
}
@article{Fujita2018,
abstract = {In models of galaxy formation, feedback driven both by supernova (SN) and active galactic nucleus is not efficient enough to quench star formation in massive galaxies.Models of smaller galaxies have suggested that cosmic rays (CRs) play a major role in expelling material from the star-forming regions by diffusing SN energy to the lower density outskirts. We therefore run gas dynamical simulations of galactic outflows from a galaxy contained in a halo with 5 × 1012 M⊙ that resembles a local ultraluminous galaxy, including both SN thermal energy and a treatment of CRs using the same diffusion approximation as Salem {\&} Bryan. We find that CR pressure drives a low-density bubble beyond the edge of the shell swept up by thermal pressure, but the main bubble driven by SN thermal pressure overtakes it later, which creates a large-scale biconical outflow. CRs diffusing into the disc are unable to entrain its gas in the outflows, yielding a mass-loading rate of only {\~{}}0.1 per cent with varied CR diffusion coefficients. We find no significant difference in mass-loading rates in SN-driven outflows with or without CR pressure. Our simulations strongly suggest that it is hard to drive a heavily mass-loaded outflow with CRs from a massive halo potential, although more distributed star formation could lead to a different result.},
archivePrefix = {arXiv},
arxivId = {1804.10302},
author = {Fujita, Akimi and Low, Mordecai Mark Mac},
doi = {10.1093/mnras/sty715},
eprint = {1804.10302},
file = {:home/william/Documents/Papers/sty715.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Cosmic rays,Galaxies: Evolution,Galaxies: Haloes,Galaxies: Kinematics and dynamics,Galaxies: Starburst},
number = {1},
pages = {531--538},
title = {{Cosmic ray driven outflows in an ultraluminous galaxy}},
volume = {477},
year = {2018}
}
@article{Taylor1960,
author = {Taylor, L S and Istroduction, I},
file = {:home/william/Documents/Papers/1-s2.0-0003491660901160-main.pdf:pdf},
pages = {377--392},
title = {{L. s. taylor}},
year = {1960}
}
@article{Ichimaru1977a,
author = {Ichimaru, S.},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Unknown - 1977 - No Title.pdf:pdf},
isbn = {0520231503},
journal = {Astron. Astrophys.},
pages = {840--855},
title = {{BIMODAL BEHAVIOR OF ACCRETION DISKS: THEORY AND APPLICATION TO CYGNUS X-l TRANSITIONS}},
volume = {214},
year = {1977}
}
@article{Ghisellini2014,
abstract = {Theoretical models for the production of relativistic jets from active galactic nuclei predict that jet power arises from the spin and mass of the central black hole, as well as the magnetic field near the event horizon. The physical mechanism mechanism underlying the contribution from the magnetic field is the torque exerted on the rotating black hole by the field amplified by the accreting material. If the squared magnetic field is proportional to the accretion rate, then there will be a correlation between jet power and accretion luminosity. There is evidence for such a correlation, but inadequate knowledge of the accretion luminosity of the limited and inhomogeneous used samples prevented a firm conclusion. Here we report an analysis of archival observations of a sample of blazars (quasars whose jets point towards Earth) that overcomes previous limitations. We find a clear correlation between jet power as measured through the gamma-ray luminosity, and accretion luminosity as measured by the broad emission lines, with the jet power dominating over the disk luminosity, in agreement with numerical simulations. This implies that the magnetic field threading the black hole horizon reaches the maximum value sustainable by the accreting matter.},
archivePrefix = {arXiv},
arxivId = {1411.5368},
author = {Ghisellini, G. and Tavecchio, F. and Maraschi, L. and Celotti, A. and Sbarrato, T.},
doi = {10.1038/nature13856},
eprint = {1411.5368},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ghisellini et al. - 2014 - The power of relativistic jets is larger than the luminosity of their accretion disks.pdf:pdf},
isbn = {0028-0836},
issn = {14764687},
journal = {Nature},
number = {7527},
pages = {376--378},
pmid = {25409827},
publisher = {Nature Publishing Group},
title = {{The power of relativistic jets is larger than the luminosity of their accretion disks}},
url = {http://dx.doi.org/10.1038/nature13856},
volume = {515},
year = {2014}
}
@article{Ryzhii2011,
abstract = {We study the characteristics of photogenerated electron-hole plasma in optically pumped graphene layers at elevated (room) temperatures when the interband and intraband processes of emission and absorption of optical phonons play a crucial role. The electron-hole plasma heating and cooling as well as the effect of nonequilibrium optical phonons are taken into account. The dependences of the quasi-Fermi energy and effective temperature of optically pumped graphene layers on the intensity of pumping radiation are calculated. The variation of the frequency dependences dynamic conductivity with increasing pumping intensity as well as the conditions when this conductivity becomes negative in a certain range of frequencies are considered. The effects under consideration can markedly influence the achievement of the negative dynamic conductivity in optically pumped graphene layers associated with the population inversion and, hence, lead to the in-depth understanding of the experimental results and the realization graphene-based terahertz and infrared lasers operating at room temperatures. {\textcopyright} 2011 The Japan Society of Applied Physics.},
archivePrefix = {arXiv},
arxivId = {1102.2026},
author = {Ryzhii, Victor and Ryzhii, Maxim and Mitin, Vladimir and Satou, Akira and Otsuji, Taiichi},
doi = {10.1143/JJAP.50.094001},
eprint = {1102.2026},
file = {:home/william/Documents/Papers/May.2b7e5baac08d15d6fa76a37b7f6cd10196f3.pdf:pdf},
issn = {00214922},
journal = {Jpn. J. Appl. Phys.},
number = {9 PART 1},
pages = {1--9},
title = {{Effect of heating and cooling of photogenerated electron-hole plasma in optically pumped graphene on population inversion}},
volume = {50},
year = {2011}
}
@article{Romero2018,
abstract = {Starbursts are galaxies undergoing massive episodes of star formation. The combined effect of stellar winds from hot stars and supernova explosions creates a high-temperature cavity in the nuclear region of these objects. The very hot gas expands adiabatically and escapes from the galaxy creating a superwind which sweeps matter from the galactic disk. The superwind region in the halo is filled with a multi-phase gas with hot, warm, cool, and relativistic components. The shocks associated with the superwind of starbursts and the turbulent gas region of the bubble inflated by them might accelerate cosmic rays up to high energies. In this work we calculate the cosmic ray production associated with the superwind using parameters that correspond to the nearby southern starburst galaxy NGC 253, which has been suggested as a potential accelerator of ultra-high energy cosmic rays. We evaluate the efficiency of both diffusive shock acceleration (DSA) and stochastic diffusive acceleration (SDA) in the superwind of NGC 253. We estimate the distribution of both hadrons and leptons and calculate the corresponding spectral energy distributions of photons. We find that the strong mass load of the superwind, recently determined through ALMA observations, strongly attenuates the efficiency of DSA in NGC 253, whereas SDA is constrained by the age of the starburst. We conclude that NGC 253 and similar starbursts can only accelerate iron nuclei beyond {\$}\backslashsim10{\^{}}{\{}18{\}}{\$} eV under very special conditions. If the central region of the galaxy harbors a starved supermassive black hole of {\$}\backslashsim10{\^{}}6{\$} {\$}M{\_}{\{}\backslashodot{\}}{\$}, as suggested by some recent observations, a contribution in the range {\$}10{\^{}}{\{}18{\}}-10{\^{}}{\{}19{\}}{\$} eV can be present for accretion rates {\$}\backslashdot{\{}m{\}}\backslashsim10{\^{}}{\{}-3{\}}{\$} in Eddington units. Only if very strong magnetic field amplification occurs close to the superwind shock energies of the order of 100 EeV might be achieved.},
archivePrefix = {arXiv},
arxivId = {1801.06483},
author = {Romero, Gustavo E. and M{\"{u}}ller, Ana Laura and Roth, Markus},
doi = {10.1051/0004-6361/201832666},
eprint = {1801.06483},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Romero, M{\"{u}}ller, Roth - 2018 - Particle acceleration in the superwinds of starburst galaxies.pdf:pdf},
issn = {14320746},
keywords = {acceleration of particles,galaxies,individual,non-thermal,radiation mechanisms,starburst},
title = {{Particle acceleration in the superwinds of starburst galaxies}},
url = {http://arxiv.org/abs/1801.06483},
volume = {57},
year = {2018}
}
@inproceedings{Sanders1996,
abstract = {At luminosities above 1011L⊙, infrared galaxies become the dominant population of extragalactic objects in the local Universe (z {\textless}0.5), being more numerous than optically selected starburst and Seyfert galaxies, and QSOs at comparable bolometric luminosity. Multiwavelength observations clearly show that the trigger for the intense IR emission is the strong interaction/merger of molecular gas-rich spirals, and that the bulk of the IR luminosity for all but the most luminous objects is due to dust heating from an intense starburst within giant molecular clouds (GMCs). At the highest luminosities (Lir {\textgreater} 1012L⊙), nearly all IR selected objects appear to be advanced mergers that are powered by both a circumnuclear starburst and AGN, both of which are fueled by an enormous concentration of molecular gas (∼ 1010 M⊙) that has been funneled into the merger nucleus. The intense circumnuclear starburst that accompanies the luminous IR phase may represent a primary stage in the formation of elliptical galaxy cores, the formation of globular clusters, and the metal enrichment of the intergalactic medium by gas and dust expelled from the nucleus due to the combined forces of supernova explosions and powerful stellar winds. {\textcopyright} Universidad Nacional Aut{\'{o}}noma de M{\'{e}}xico.},
author = {Sanders, D B},
booktitle = {Rev. Mex. Astron. y Astrofis. Ser. Conf.},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Sanders, Mirabel - 1996 - Luminous infrared galaxies.pdf:pdf},
issn = {14052059},
keywords = {Galaxies: starburst,Infrared: galaxies},
pages = {42--47},
title = {{Luminous infrared galaxies}},
volume = {6},
year = {1997}
}
@article{York,
author = {York, N E W},
file = {:home/william/Documents/Papers/CFL.paper.pdf:pdf},
journal = {New York},
title = {{AEC Computing and Applied Mathematics Center}}
}
@article{Zubovas2020,
abstract = {The properties of large-scale galactic outflows, such as their kinetic energy and momentum rates, correlate with the luminosity of the active galactic nucleus (AGN). This is well explained by the wind-driven outflow model, where a fraction of the AGN luminosity drives the outflow. However, significant departures from these correlations have been observed in a number of galaxies. This may happen because AGN luminosity varies on a much shorter time-scale (∼104-105 yr) than outflow properties do (∼106 yr). We investigate the effect of AGN luminosity variations on outflow properties using 1D numerical simulations. This effect can explain the very weak outflow in PDS 456: if its nucleus is currently much brighter than the long-term average luminosity, the outflow has not had time to react to this luminosity change. Conversely, the outflow in Mrk 231 is consistent with being driven by an almost continuous AGN, while IRAS F11119+3257 represents an intermediate case between the two. Considering a population of AGN, we find that very low momentum loading factors pout {\textless} LAGN/c should be seen in a significant fraction of objects - up to 15{\%} depending on the properties of AGN variability and galaxy gas fraction. The predicted distribution of loading factors is consistent with the available observational data. We discuss how this model might help constrain the duty cycles of AGN during the period of outflow inflation, implications for multiphase, and spatially distinct outflows, and suggest ways of improving AGN prescriptions in numerical simulations.},
archivePrefix = {arXiv},
arxivId = {2008.12492},
author = {Zubovas, Kastytis and Nardini, Emanuele},
doi = {10.1093/mnras/staa2652},
eprint = {2008.12492},
file = {:home/william/Documents/Papers/2008.12492.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {accretion, accretion discs,galaxies: active,quasars: general},
number = {3},
pages = {3633--3647},
title = {{Intermittent AGN episodes drive outflows with a large spread of observable loading factors}},
volume = {498},
year = {2020}
}
@article{1982MNRAS.199..883B,
author = {Blandford, R.{\~{}}D. and Payne, D.{\~{}}G.},
doi = {10.1093/mnras/199.4.883},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Blandford, Payne - 1982 - Hydromagnetic flows from accretion discs and the production of radio jets.pdf:pdf},
journal = {MNRAS},
keywords = {Angular Momentum,Astrophysics,Black Holes (Astronomy),Critical Point,Disks (Shapes),Energy Transfer,Magnetohydrodynamic Flow,Momentum Transfer,Radio Jets (Astronomy),Solar Corona,Stellar Mass Accretion},
pages = {883--903},
title = {{Hydromagnetic flows from accretion discs and the production of radio jets}},
volume = {199},
year = {1982}
}
@article{Walsh2016,
abstract = {? 2016. The American Astronomical Society. All rights reserved..The nearby lenticular galaxy NGC 1277 is thought to host one of the largest black holes known, however the black hole mass measurement is based on low spatial resolution spectroscopy. In this paper, we present Gemini Near-infrared Integral Field Spectrometer observations assisted by adaptive optics. We map out the galaxy's stellar kinematics within ?440 pc of the nucleus with an angular resolution that allows us to probe well within the region where the potential from the black hole dominates. We find that the stellar velocity dispersion rises dramatically, reaching ?550 km s-1 at the center. Through orbit-based, stellar-dynamical models we obtain a black hole mass of (4.9 1.6) 109 Mo (1? uncertainties). Although the black hole mass measurement is smaller by a factor of ?3 compared to previous claims based on large-scale kinematics, NGC 1277 does indeed contain one of the most massive black holes detected to date, and the black hole mass is an order of magnitude larger than expectations from the empirical relation between black hole mass and galaxy luminosity. Given the galaxy's similarities to the higher redshift (z ? 2) massive quiescent galaxies, NGC 1277 could be a relic, passively evolving since that period. A population of local analogs to the higher redshift quiescent galaxies that also contain over-massive black holes may suggest that black hole growth precedes that of the host galaxy.},
archivePrefix = {arXiv},
arxivId = {1511.04455},
author = {Walsh, Jonelle L and van den Bosch, Remco C. E. and Gebhardt, Karl and Yıldırım, Akın and Richstone, Douglas O and G{\"{u}}ltekin, Kayhan and Husemann, Bernd},
doi = {10.3847/0004-637X/817/1/2},
eprint = {1511.04455},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Walsh et al. - 2016 - A 5 × 10 9 M ⊙ BLACK HOLE IN NGC 1277 FROM ADAPTIVE OPTICS SPECTROSCOPY.pdf:pdf},
issn = {1538-4357},
journal = {Astrophys. J.},
keywords = {black hole physics,cd,elliptical and lenticular,galaxies,individual,kinematics and dynamics,machine-readable table,ngc 1277,nuclei,supporting material},
number = {1},
pages = {2},
title = {{A 5 × 10 9 M ⊙ BLACK HOLE IN NGC 1277 FROM ADAPTIVE OPTICS SPECTROSCOPY}},
url = {http://stacks.iop.org/0004-637X/817/i=1/a=2?key=crossref.1174e5897fa25119af02e653c091250e},
volume = {817},
year = {2016}
}
@article{Fragile2005,
abstract = {We present results from two-dimensional numerical simulations of the interactions between magnetized shocks and radiative clouds. Our primary goal is to characterize the dynamical evolution of the shocked clouds. We perform runs in both the strong and weak magnetic field limits and consider three different field orientations. For the geometries considered, we generally find that magnetic fields external to, but concentrated near, the surface of the cloud suppress the growth of destructive hydrodynamic instabilities. External fields also increase the compression of the cloud by effectively acting as a confinement mechanism driven by the interstellar flow and local field stretching. This can have a dramatic effect on both the efficiency of radiative cooling, which tends to increase with increasing magnetic field strength, and on the size and distribution of condensed cooled fragments. In contrast, fields acting predominately internally to the cloud tend to resist compression, thereby inhibiting cooling. We observe that, even at modest strengths, internal fields can completely suppress low-temperature cooling.},
author = {Fragile, P. Chris and Anninos, Peter and Gustafson, Kyle and Murray, Stephen D.},
doi = {10.1086/426313},
file = {:home/william/Documents/Papers/Fragile{\_}2005{\_}ApJ{\_}619{\_}327.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
number = {1},
pages = {327--339},
title = {{Magnetohydrodynamic Simulations of Shock Interactions with Radiative Clouds}},
volume = {619},
year = {2005}
}
@article{Hilfinger1987,
author = {Hilfinger, Andreas and Paulsson, Johan},
doi = {10.1038/325379c0},
file = {:home/william/Documents/Papers/geach2015.pdf:pdf},
issn = {00280836},
journal = {Nature},
number = {6103},
pages = {379},
title = {{When the wind blows}},
volume = {325},
year = {1987}
}
@article{Guo2012,
abstract = {The Fermi Gamma-ray Space Telescope reveals two large gamma-ray bubbles in the Galaxy, which extend about 50 degrees ({\~{}} 10 kpc) above and below the Galactic center (GC) and are symmetric about the Galactic plane. Using axisymmetric hydrodynamic simulations with a self-consistent treatment of the dynamical cosmic ray (CR) - gas interaction, we show that the bubbles can be created with a recent active galactic nucleus (AGN) jet activity about 1 - 3 Myr ago, which was active for a duration of {\~{}} 0.1 - 0.5 Myr. The bipolar jets were ejected into the Galactic halo along the rotation axis of the Galaxy. Near the GC, the jets must be moderately light with a typical density contrast 0.001 {\textless}{\~{}} $\backslash$eta {\textless}{\~{}} 0.1 relative to the ambient hot gas. The jets are energetically dominated by kinetic energy, and over-pressured with either CR or thermal pressure which induces lateral jet expansion, creating fat CR bubbles as observed. The sharp edges of the bubbles imply that CR diffusion across the bubble surface is strongly suppressed. The jet activity induces a strong shock, which heats and compresses the ambient gas in the Galactic halo, potentially explaining the ROSAT X-ray shell features surrounding the bubbles. The Fermi bubbles provide plausible evidence for a recent powerful AGN jet activity in our Galaxy, shedding new insights into the origin of the halo CR population and the channel through which massive black holes in disk galaxies release feedback energy during their growth.},
author = {Guo, Fulai and Mathews, William G.},
doi = {10.1088/0004-637X/756/2/181},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Guo, Mathews - 2012 - The Fermi bubbles. I. Possible evidence for recent AGN jet activity in the GALAXY.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {Galaxy: nucleus,cosmic rays,galaxies: active,galaxies: jets,gamma rays: galaxies},
number = {2},
title = {{The Fermi bubbles. I. Possible evidence for recent AGN jet activity in the GALAXY}},
volume = {756},
year = {2012}
}
@article{Dasyra2012,
abstract = {We present deep observations of the 12CO(1-0) and (3-2) lines in 4C12.50, carried out with the 30m telescope of the Institut de Radioastronomie Millimetrique. Our observations revealed the cold molecular gas component of a warm molecular gas outflow that was previously known from Spitzer Space Telescope data. The 12CO(3-2) profile indicates the presence of absorption at -950 km/s from systemic velocity with a central optical depth of 0.22. Its profile is similar to that of the HI absorption that was seen in radio data of this source. A potential detection of the (0-1) absorption enabled us to place an upper limit of 0.03 on its central optical depth, and to constrain the excitation temperature of the outflowing CO gas to {\textgreater}=65K assuming that the gas is thermalized. If the molecular clouds are fully obscuring their background millimeter continuum that is emitted by the radio core, the H2 column density is {\textgreater}=1.810 22 /cm 2. The outflow is then carrying an estimated cold H2 mass of at least 4.210 3 Msun along the nuclear line of sight. This mass will be even higher when integrated over several lines of sight, but if it were to exceed 310 9 Msun, the outflow would most likely be seen in emission. Since the ambient cold gas reservoir of 4C12.50 is 1.010 10 Msun, the outflowing-to-ambient mass ratio of the warm gas (37{\%}) could be elevated with respect to that of the cold gas.},
archivePrefix = {arXiv},
arxivId = {astro-ph.CO/1203.3452},
author = {Dasyra, KM and Combes, F},
doi = {10.1051/0004-6361/201219229},
eprint = {1203.3452},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Dasyra, Combes - 2012 - Cold and warm molecular gas in the outflow of 4C12. 50.pdf:pdf},
issn = {0004-6361},
journal = {arXiv Prepr. arXiv1203.3452},
keywords = {active,galaxies,ism,jets and outflows,kinematics and dynamics,line,nuclei,profiles},
pages = {1--5},
primaryClass = {astro-ph.CO},
title = {{Cold and warm molecular gas in the outflow of 4C12. 50}},
url = {http://arxiv.org/abs/1203.3452},
volume = {541},
year = {2012}
}
@article{1390,
author = {سعید, صاحبدل فر،},
file = {:home/william/Documents/Papers/1993A+A...273..318S.pdf:pdf},
pages = {368},
title = {{No Titleنانوکاتالیست ها کاربردنانوفناوری در کاتالیزگری}},
year = {1390}
}
@article{McWhirter1975,
abstract = {The density and temperature distribution of the solar corona is calculated assuming an energy balance between thermal conduction and radiated power loss with the primary heating of the corona by the dissipation of sound-waves propagated upwards from below the sun's surface. A sharp transition region is found and the calculated results are compared with observations. A detailed model atmosphere for the transition region and corona is derived using the Harvard Smithsonian Reference Atmosphere (for the chromosphere) as starting point.$\backslash$nHydrostatic equilibrium is assumed in the calculations but it is also shown that a pressure arises because of the sound waves which is of comparable magnitude to hydrostatic pressure. The inclusion of this pressure introduces difficulties that are discussed.},
author = {McWhirter, R. W. P. and Thonemann, P. C. and Wilson, R.},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/McWhirter, Thonemann, Wilson - 1975 - The heating of the solar corona. II - A model based on energy balance.pdf:pdf},
issn = {0004-6361},
journal = {Astron. Astrophys.},
pages = {63--73},
title = {{The heating of the solar corona. II - A model based on energy balance}},
url = {http://adsabs.harvard.edu/abs/1975A{\%}26A....40...63M{\%}5Cnhttp://adsabs.harvard.edu/cgi-bin/nph-data{\_}query?bibcode=1975A{\%}26A....40...63M{\&}link{\_}type=ARTICLE},
volume = {40},
year = {1975}
}
@article{Zheng2008,
abstract = {We carry out high-resolution FUSE spectroscopy of the nuclear region of NGC 1068. The first set of spectra was obtained with a 30" square aperture that collected all emission from the narrow-line region. The data reveal a strong broad O VI component of FWHM {\~{}}3500 km s-1 and two narrow O VI $\lambda$ $\lambda$1031, 1037 components of {\~{}}350 km s-1. The C III $\lambda$977 and N III $\lambda$991 emission lines in this spectrum can be fitted with a narrow component of FWHM {\~{}}1000 km s-1 and a broad one of {\~{}}2500 km s-1. Another set of seven spatially resolved spectra was made using a long slit of 1.25''×20'' at steps of {\~{}}1" along the axis of the emission-line cone. We find the following: (1) Major emission lines in the FUSE wavelength range consist of a broad and a narrow component. (2) There is a gradient in the velocity field for the narrow O VI component of {\~{}}200 km s-1 from {\~{}}2" southwest of the nucleus to {\~{}}4" northeast. A similar pattern is also observed with the broad O VI component, with a gradient of {\~{}}3000 km s-1. These are consistent with the HST STIS findings and suggest a biconical structure in which the velocity field is mainly radial outflow. (3) A major portion of the C III and N III line flux is produced in the compact core. They are therefore not effective temperature diagnostics for the conical region. (4) The best-fit UV continuum suggests virtually no reddening, and the He II I($\lambda$1640)/I($\lambda$1085) ratio suggests a consistently low extinction factor across the cone. At {\~{}}2" northeast of the nucleus there is a region characterized by (a) a strong Ly$\alpha$ flux but normal C IV flux, (b) a broad O VI line, and (c) a significantly enhanced C III flux. Based on observations made with the NASA-CNES-CSA Far Ultraviolet Spectroscopic Explorer (FUSE), which is operated for NASA by The Johns Hopkins University under NASA contract NAS5-32985, and observations with the NASA/ESA Hubble Space Telescope, obtained at the Space Telescope Science Institute, which is operated by the Association of Universities for Research in Astronomy, Inc., under NASA contract NAS5-26555.},
archivePrefix = {arXiv},
arxivId = {0806.4641},
author = {Zheng, Wei and Wang, Jun‐Xian and Kriss, Gerard A. and Sahnow, David and Allen, Mark and Dopita, Michael and Tsvetanov, Zlatan and Bicknell, Geoffrey},
doi = {10.1086/591547},
eprint = {0806.4641},
file = {:home/william/Documents/Papers/0806.4641.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
number = {2},
pages = {881--891},
title = {{Spatially Resolved Far‐Ultraviolet Spectroscopy of the Nuclear Region of NGC 1068}},
volume = {686},
year = {2008}
}
@article{Ruschel-Dutra2021,
abstract = {We analyse optical data cubes of the inner kiloparsec of 30 local (z ≤ 0.02) active galactic nucleus (AGN) hosts that our research group, AGNIFS, has collected over the past decade via observations with the integral field units of the Gemini Multi-Object Spectrographs. Spatial resolutions range between 50 and 300 pc and spectral coverage is from 4800 or 5600 to 7000 {\AA}, at velocity resolutions of ≈50 km s-1. We derive maps of the gas excitation and kinematics, and determine the AGN ionization axis - which has random orientation relative to the galaxy - and the kinematic major axes of the emitting gas. We find that rotation dominates the gas kinematics in most cases, but is disturbed by the presence of inflows and outflows. Outflows have been found in 21 nuclei, usually along the ionization axis. The gas velocity dispersion is traced by W80 (velocity width encompassing 80 per cent of the line flux), adopted as a tracer of outflows. In seven sources, W80 is enhanced perpendicularly to the ionization axis, indicating lateral expansion of the outflow. We have estimated mass-outflow rates ˙M and powers ˙E, finding median values of log, [˙M/(M⊙, yr-1)] = -2.1-1.0+1.6 and log, [˙E/(erg, s-1)] = 38.5-0.9+1.8, respectively. Both quantities show a mild correlation with the AGN luminosity (LAGN). ˙E is of the order of 0.01 LAGN for four sources, but much lower for the majority (nine) of the sources, with a median value of log, [˙E/LAGN] = -5.34-0.9+3.2, indicating that typical outflows in the local Universe are unlikely to significantly impact their host galaxy evolution.},
archivePrefix = {arXiv},
arxivId = {2107.07635},
author = {Ruschel-Dutra, D. and Storchi-Bergmann, T. and Schnorr-M{\"{u}}ller, A. and Riffel, R. A. and {Dall'agnol De Oliveira}, B. and Lena, D. and Robinson, A. and Nagar, N. and Elvis, M.},
doi = {10.1093/mnras/stab2058},
eprint = {2107.07635},
file = {:home/william/Documents/Papers/stab2058.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {galaxies: Seyfert,galaxies: active,galaxies: kinematics and dynamics,galaxies: nuclei},
number = {1},
pages = {74--89},
title = {{AGNIFS survey of local AGN: GMOS-IFU data and outflows in 30 sources}},
volume = {507},
year = {2021}
}
@article{Pino2005,
abstract = {We propose here that the large-scale superluminal ejections observed in the galactic microquasar GRS 1915+105 during radio flare events are produced by violent magnetic reconnection episodes in the corona just above the inner edge of the magnetized accretion disk that surrounds the central ∼10M ⊙ black hole. The process occurs when a large-scale magnetic field is established by a turbulent dynamo in the inner disk region with a ratio between the gas+radiation and the magnetic pressures $\beta$ ≃ 1, implying a magnetic field intensity of ∼7 × 108 G. During this process, substantial angular momentum is removed from the disk by the wind generated by the vertical magnetic flux therefore increasing the disk mass accretion to a value near (but below) the critical one (Ṁ ∼ 10 19 g s-1). Part of the magnetic energy released by reconnection heats the coronal gas (Tc ≲ 5 × 10 8 K) that produces a steep X-ray spectrum with luminosity L X ≃ 1039 erg s-1, consistent with observations. The remaining magnetic energy released goes to accelerate the particles to relativistic velocities ($\nu$ - $\nu$A - c, where $\nu$A is the Alfv{\'{e}}n speed) in the reconnection site through first-order Fermi processes. In this context, two possible mechanisms have been examined that produce power-law electron distributions N(E) ∝ E -$\alpha$E, with $\alpha$E = 5/2, 2, and corresponding synchrotron radio power-law spectra with spectral indices which are compatible with that observed during the flares (S$\nu$ ∝ $\nu$-0.75,-0.5). {\textcopyright} ESO 2005.},
author = {{De Gouveia Dal Pino}, E. M. and Lazarian, A},
doi = {10.1051/0004-6361:20042590},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Pino, Lazarian - 2005 - Production of the large scale superluminal ejections of the microquasar GRS 1915 105 by violent magnetic reconn.pdf:pdf},
issn = {00046361},
journal = {Astron. Astrophys.},
keywords = {Acceleration of particles,Accretion,Black hole physics,Magnetic fields,accretion disks},
number = {3},
pages = {845--853},
title = {{Production of the large scale superluminal ejections of the microquasar GRS 1915+105 by violent magnetic reconnection}},
volume = {441},
year = {2005}
}

@ARTICLE{Almeida2021,
       author = {{Ramos Almeida}, C. and {Bischetti}, M. and {Garc{\'\i}a-Burillo}, S. and {Alonso-Herrero}, A. and {Audibert}, A. and {Cicone}, C. and {Feruglio}, C. and {Tadhunter}, C.~N. and {Pierce}, J.~C.~S. and {Pereira-Santaella}, M. and {Bessiere}, P.~S.},
        title = "{The diverse cold molecular gas contents, morphologies, and kinematics of type-2 quasars as seen by ALMA}",
      journal = {\aap},
     keywords = {galaxies: active, galaxies: nuclei, quasars: general, galaxies: evolution, ISM: jets and outflows, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = feb,
       volume = {658},
          eid = {A155},
        pages = {A155},
          doi = {10.1051/0004-6361/202141906},
archivePrefix = {arXiv},
       eprint = {2111.13578},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A&A...658A.155R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Stepanovs2014,
abstract = {We present MHD simulations exploring the launching, acceleration, and collimation of jets and disk winds. The evolution of the disk structure is consistently taken into account. Extending our earlier studies, we now consider the self-generation of the magnetic field by an $\alpha$2$\Omega$ mean-field dynamo. The disk magnetization remains on a rather low level, which helps to evolve the simulations for T {\textgreater} 10, 000 dynamical time steps on a domain extending 1500 inner disk radii. We find the magnetic field of the inner disk to be similar to the commonly found open field structure, favoring magneto-centrifugal launching. The outer disk field is highly inclined and predominantly radial. Here, differential rotation induces a strong toroidal component, which plays a key role in outflow launching. These outflows from the outer disk are slower, denser, and less collimated. If the dynamo action is not quenched, magnetic flux is continuously generated, diffuses outward through the disk, and fills the entire disk. We have invented a toy model triggering a time-dependent mean-field dynamo. The duty cycles of this dynamo lead to episodic ejections on similar timescales. When the dynamo is suppressed as the magnetization falls below a critical value, the generation of the outflows and also accretion is inhibited. The general result is that we can steer episodic ejection and large-scale jet knots by a disk-intrinsic dynamo that is time-dependent and regenerates the jet-launching magnetic field.},
archivePrefix = {arXiv},
arxivId = {1409.7003},
author = {Stepanovs, Deniss and Fendt, Christian and Sheikhnezami, Somayeh},
doi = {10.1088/0004-637X/796/1/29},
eprint = {1409.7003},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Stepanovs, Fendt, Sheikhnezami - 2014 - Modelling mhd accretion-ejection - episodic ejections of jets triggered by a mean-field disk dyn.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {accretion,accretion disks - galaxies,jets - ISM,jets and outflows - magnetohydrodynamics (MHD) - s,mass-loss - stars,pre-main sequence},
number = {1},
title = {{Modeling MHD accretion-ejection: Episodic ejections of jets triggered by a mean-field disk dynamo}},
volume = {796},
year = {2014}
}
@article{Stone2008,
author = {Stone, James M and Gardiner, Thomas A and Teuben, Peter and Hawley, John F and Simon, Jacob B},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Stone et al. - 2008 - ATHENA A NEW CODE FOR ASTROPHYSICAL MHD.pdf:pdf},
title = {{ATHENA : A NEW CODE FOR ASTROPHYSICAL MHD}},
year = {2008}
}
@article{Tremblay2016,
abstract = {Supermassive black holes in galaxy centres can grow by the accretion of gas, liberating energy that might regulate star formation on galaxy-wide scales. The nature of the gaseous fuel reservoirs that power black hole growth is nevertheless largely unconstrained by observations, and is instead routinely simplified as a smooth, spherical inflow of very hot gas. Recent theory and simulations instead predict that accretion can be dominated by a stochastic, clumpy distribution of very cold molecular clouds - a departure from the "hot mode" accretion model - although unambiguous observational support for this prediction remains elusive. Here we report observations that reveal a cold, clumpy accretion flow towards a supermassive black hole fuel reservoir in the nucleus of the Abell 2597 Brightest Cluster Galaxy (BCG), a nearby (redshift z=0.0821) giant elliptical galaxy surrounded by a dense halo of hot plasma. Under the right conditions, thermal instabilities can precipitate from this hot gas, producing a rain of cold clouds that fall toward the galaxy's centre, sustaining star formation amid a kiloparsec-scale molecular nebula that inhabits its core. The observations show that these cold clouds also fuel black hole accretion, revealing "shadows" cast by the molecular clouds as they move inward at about 300 kilometres per second towards the active supermassive black hole in the galaxy centre, which serves as a bright backlight. Corroborating evidence from prior observations of warmer atomic gas at extremely high spatial resolution, along with simple arguments based on geometry and probability, indicate that these clouds are within the innermost hundred parsecs of the black hole, and falling closer towards it.},
archivePrefix = {arXiv},
arxivId = {arXiv:1606.02304v2},
author = {Tremblay, Grant R. and Oonk, J. B.Raymond and Combes, Fran{\c{c}}oise and Salom{\'{e}}, Philippe and O'Dea, Christopher P. and Baum, Stefi A. and Voit, G. Mark and Donahue, Megan and McNamara, Brian R. and Davis, Timothy A. and McDonald, Michael A. and Edge, Alastair C. and Clarke, Tracy E. and Galv{\'{a}}n-Madrid, Roberto and Bremer, Malcolm N. and Edwards, Louise O.V. and Fabian, Andrew C. and Hamer, Stephen and Li, Yuan and Maury, Ana{\"{e}}lle and Russell, Helen R. and Quillen, Alice C. and Urry, C. Megan and Sanders, Jeremy S. and Wise, Michael W.},
doi = {10.1038/nature17969},
eprint = {arXiv:1606.02304v2},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Tremblay et al. - 2016 - Cold, clumpy accretion onto an active supermassive black hole.pdf:pdf},
issn = {14764687},
journal = {Nature},
number = {7606},
pages = {218--221},
title = {{Cold, clumpy accretion onto an active supermassive black hole}},
volume = {534},
year = {2016}
}
@article{Imanishi2019,
abstract = {We present the results of our ALMA HCN J=3-2 and HCO+ J=3-2 line observations of a uniformly selected sample ({\textgreater}25) of nearby ultraluminous infrared galaxies (ULIRGs) at z {\textless} 0.15. The emission of these dense molecular gas tracers and continuum are spatially resolved in the majority of observed ULIRGs for the first time with achieved synthesized beam sizes of {\~{}}0.2 arcsec or {\~{}}500 pc. In most ULIRGs, the HCN-to-HCO+ J=3-2 flux ratios in the nuclear regions within the beam size are systematically higher than those in the spatially extended regions. The elevated nuclear HCN J=3-2 emission could be related to (a) luminous buried active galactic nuclei, (b) the high molecular gas density and temperature in ULIRG's nuclei, and/or (c) mechanical heating by spatially compact nuclear outflows. A small fraction of the observed ULIRGs display higher HCN-to-HCO+ J=3-2 flux ratios in localized off-nuclear regions than those of the nuclei, which may be due to mechanical heating by spatially extended outflows. The observed nearby ULIRGs are generally rich in dense ({\textgreater}10{\^{}}5 cm{\^{}}-3) molecular gas, with an estimated mass of {\textgreater}10{\^{}}9 Msun within the nuclear (a few kpc) regions, and dense gas can dominate the total molecular mass there. We find a low detection rate ({\textless}20{\%}) regarding the possible signature of a vibrationally excited (v2=1f) HCN J=3-2 emission line in the vicinity of the bright HCO+ J=3-2 line that may be due, in part, to the large molecular line widths of ULIRGs.},
archivePrefix = {arXiv},
arxivId = {1902.04124},
author = {Imanishi, Masatoshi and Nakanishi, Kouichiro and Izumi, Takuma},
doi = {10.3847/1538-4365/ab05b9},
eprint = {1902.04124},
file = {:home/william/Documents/Papers/1902.04124.pdf:pdf},
issn = {0067-0049},
journal = {Astrophys. J. Suppl. Ser.},
keywords = {Galaxies: Seyfert,Galaxies: active,Galaxies: nuclei,Galaxies: starburst,Quasars: general,Submillimeter: galaxies},
number = {2},
pages = {19},
title = {{ALMA Spatially Resolved Dense Molecular Gas Survey of Nearby Ultraluminous Infrared Galaxies}},
volume = {241},
year = {2019}
}
@article{2012ApJ...745L..34Z,
abstract = {It is widely suspected that active galactic nucleus (AGN) activity ultimately sweeps galaxies clear of their gas. We work out the observable properties required to achieve this. Large-scale AGN-driven outflows should have kinetic luminosities ∼$\eta$LEdd/2 ∼ 0.05LEdd and momentum rates ∼20LEdd/c, where LEdd is the Eddington luminosity of in which molecular species coexist with hot gas, which can persist after the central AGN has switched off. This the central black hole and $\eta$ ∼ 0.1 its radiative accretion efficiency. This creates an expanding two-phase medium picture predicts outflow velocities ∼1000–1500 km s−1 and mass outflow rates up to 4000 M? yr−1 on kpc scales, fixed mainly by the host galaxy velocity dispersion (or equivalently black hole mass). All these features agree with those of outflows observed in galaxies such as Mrk231. This strongly suggests that AGN activity is what sweeps galaxies clear of their gas on a dynamical timescale and makes them red and dead. We suggest future observational tests of this picture.},
archivePrefix = {arXiv},
arxivId = {1201.0866},
author = {Zubovas, K and King, A},
doi = {10.1088/2041-8205/745/2/L34},
eprint = {1201.0866},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Zubovas, King - 2012 - Clearing Out a Galaxy.pdf:pdf},
journal = {apjl},
keywords = {accretion,accretion disks,black hole physics,galaxies: evolution,quasars: general},
pages = {L34},
title = {{Clearing Out a Galaxy}},
volume = {745},
year = {2012}
}
@article{Hollenbach1989,
abstract = {The structure and emission-line spectra of fast (vs = 30-150 km s-1), steady interstellar shocks in molecular gas at densities n0 = 103-106 cm-3 are presented. The results are for J shocks, in which the shock front is treated as a discontinuity and ambipolar diffusion is negligible. The relative concentrations of H2, H, and H + entering the shock front are determined by the photoionizing precursor, for which a theory is developed. In almost the entire parameter space studied, the H2 is completely dissociated, either by the precursor field or by collisions in the shock, and then is reformed on grain surfaces over a column density {\~{}}1021-22 cm-2 down- stream. A chemical reaction network follows the chemistry of H, C, O, and, to a lesser extent, Si. The radiative cooling of the gas is partially offset by heating due to absorption of UV radiation from the hot gas near the shock front and due to the release of chemical energy by the formation of H2. The spectra of fast J shocks show the following features: (1) H2 emission is dominated by collisional excita- tion in the low-J rotational lines and by formation pumping in the high-J rotational lines and the vibrational lines; as a result, the H2 spectrum can mimic that of pumping by ultraviolet radiation. The intensity of the 1-0 S(l) line is less than 10-3 ergs cm-2 s{\_}1 sr-1, far less than in C shocks in dense gas and far less than inferred in many sources. (2) O i(63 /un) is proportional to the particle flux through the shock for n0vs {\textless} 1012 cm-2 s-1. O i(63 jum)/C ii(158 /mi) is a good discriminant between J shocks and photodissociation regions when the O i line is strong. The line to continuum ratios and the line profiles may also discriminate J shocks from photodissociation regions. (3) Ne n(12.8 /un) and Si n(35 /un) are good discriminants between J shocks and C shocks, since C shocks have very low ionic abundances. (4) S i(25 /un), C n(11.4 /un), Fe i(24 /un), Fe ii(26 /un), Fe n(35 /un), and Ni n(6.6 /un) are predicted in J shocks in dense (n0 {\textgreater} 105 cm-3) gas. (5) C i 29849, N i(1.04 /un), Fe n(1.3 /un), and Fe n(1.7 /un) are predicted to be strong near infrared emission lines. (6) Intensities of CO rotational lines, of the total intensity of OH and H20 rovibrational cooling, and of Ha, H{\ss}, Pa, P/?, Bra, Br{\ss}, and Bry are also given. These results have direct application to Herbig-Haro objects, winds from protostars, supernova remnants in molecular clouds, and H20 masers. The prime diagnostics for a J shock in the protostellar outflow source in the BN-KL region of Orion are the infrared hydrogen lines and the fine structure lines of ions such as Si+. Broad, intense O i(63 /¿m) emission is predicted to be the signature of supernova remnants “ buried ” in molec- ular clouds. The temperature plateau produced by H2 formation heating behind J shocks in dense gas (n0},
author = {Hollenbach, D. and McKee, C.},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Mckee - 1989 - No Title.pdf:pdf},
journal = {Apj},
keywords = {biologicamente ativos que s{\~{a}}o,dependentes das suas estruturas},
number = {Mm},
pages = {306--336},
title = {{Molecule formation and infrared emission in fast interestellar shocks: III results for J shocks in molecular clouds}},
volume = {342},
year = {1989}
}
@article{St-Onge2020,
abstract = {The turbulent amplification of cosmic magnetic fields depends upon the material properties of the host plasma. In many hot, dilute astrophysical systems, such as the intracluster medium (ICM) of galaxy clusters, the rarity of particle-particle collisions allows departures from local thermodynamic equilibrium. These departures - pressure anisotropies - exert anisotropic viscous stresses on the plasma motions that inhibit their ability to stretch magnetic-field lines. We present an extensive numerical study of the fluctuation dynamo in a weakly collisional plasma using magnetohydrodynamic (MHD) equations endowed with a field-parallel viscous (Braginskii) stress. When the stress is limited to values consistent with a pressure anisotropy regulated by firehose and mirror instabilities, the Braginskii-MHD dynamo largely resembles its MHD counterpart, particularly when the magnetic field is dynamically weak. If instead the parallel viscous stress is left unabated - a situation relevant to recent kinetic simulations of the fluctuation dynamo and, we argue, to the early stages of the dynamo in a magnetized ICM - the dynamo changes its character, amplifying the magnetic field while exhibiting many characteristics reminiscent of the saturated state of the large-Prandtl-number () MHD dynamo. We construct an analytic model for the Braginskii-MHD dynamo in this regime, which successfully matches simulated dynamo growth rates and magnetic-energy spectra. A prediction of this model, confirmed by our numerical simulations, is that a Braginskii-MHD plasma without pressure-anisotropy limiters will not support a dynamo if the ratio of perpendicular and parallel viscosities is too small. This ratio reflects the relative allowed rates of field-line stretching and mixing, the latter of which promotes resistive dissipation of the magnetic field. In all cases that do exhibit a viable dynamo, the generated magnetic field is organized into folds that persist into the saturated state and bias the chaotic flow to acquire a scale-dependent spectral anisotropy.},
archivePrefix = {arXiv},
arxivId = {2003.09760},
author = {St-Onge, D. A. and Kunz, M. W. and Squire, J. and Schekochihin, A. A.},
doi = {10.1017/S0022377820000860},
eprint = {2003.09760},
file = {:home/william/Documents/Papers/2003.09760.pdf:pdf},
issn = {14697807},
journal = {J. Plasma Phys.},
keywords = {astrophysical plasmas,plasma instabilities,plasma nonlinear phenomena},
title = {{Fluctuation dynamo in a weakly collisional plasma}},
year = {2020}
}
@article{Dadina2010,
abstract = {Context. The physical conditions of the gas forming the narrow-line regions (NLR) in active galactic nuclei (AGN) have been extensively studied in the optical band. Recently detailed X-ray studies have shown how the emission in the 0.1-2 keV band detected in Seyfert 2 galaxies is associated to gas lying close to or associated with the NLR. Aims. We take advantage of the spectacular extension (∼15") of the NLR in the type II Seyfert galaxy NGC 5252 and of the complementary characteristics of XMM-Newton and Chandra to investigate the physical conditions of the gas in this galaxy. Methods. The X-ray data from XMM-Newton are used to define the spectral properties of the ionising nuclear source. The Chandra data are used to trace the spatial characteristics of the soft X-ray emission. This information is then compared to the optical HST characteristics of the NLR in NGC 5252. Results. The X-ray spectrum of the nucleus of NGC 5252 is intrinsically flat ($\Gamma$∼1.4-1.5) and absorbed by neutral gas with a column density NH∼1022 cm -2. Below ∼1 keV a soft excess is detected. The high-resolution spectrum obtained with the XMM-Newton RGS shows emission lines in the 0.2-1.5 keV range which strongly indicate that the soft X-ray component is essentially due to ionised gas. Moreover, the soft X-ray emission is spatially resolved around the nucleus and well overlaps the images obtained in narrow optical bands centred around the [Oiii] emission line at 5007 {\AA}. The [Oiii]/soft-X flux ratios along the ionisation cones are basically constant. This indicates that the electron density does not significantly deviate from the r-2 law (constant ionisation parameter) moving outward from the nucleus. Conclusions. This result combined with previous optical studies suggests two plausible but different scenarios in the reconstruction of the last ∼30= 000 years of history of the central AGN. The most promising one is that the source is indeed a "quasar relic" with a steady and inefficient energy release from the accretion of matter onto the central super-massive black-hole. This scenario is suggested also by the flat nuclear X-ray spectrum that evokes an advection dominated accretion flow (ADAF) like emission mechanism. {\textcopyright} ESO, 2010.},
author = {Dadina, M. and Guainazzi, M. and Cappi, M. and Bianchi, S. and Vignali, C. and Malaguti, G. and Comastri, A.},
doi = {10.1051/0004-6361/200913727},
file = {:home/william/Documents/Papers/[Dadina, et l.]-X-ray imaging of the ionisation cones in NGC 5252.pdf:pdf},
issn = {00046361},
journal = {Astron. Astrophys.},
keywords = {Galaxies: active,X-ray: galaxies,galaxies: individual: NGC 5252,galaxies: seyfert},
number = {24},
pages = {1--8},
title = {{X-ray imaging of the ionisation cones in NGC 5252}},
volume = {516},
year = {2010}
}
@article{Yoshida2019,
abstract = {We performed deep spectropolarimetric observations of a prototypical starburst galaxy M82 with the Subaru Telescope in order to study the kinematics of the dust outflow. We obtained optical polarized emission-line spectra up to ∼4 kpc away from the nucleus of the galaxy along three position angles, 138◦, 150◦ and 179◦ within the conical outflowing wind (superwind). The H$\alpha$ emission line in the superwind is strongly polarized and the polarization pattern shows dust scattering of central light sources, being consistent with the previous works. The intensity weighted polarization degree of the H$\alpha$ line reaches ∼30{\%} at maximum. There are at least two light sources at the central region of the galaxy; one of which is located at the near- infrared nucleus and the other resides at one of the peaks of the 3 mm radio and molecular gas emission. The outer ({\textgreater} 1 kpc) dust is illuminated by the former, whereas the inner dust is scattering the light from the latter. We investigated as well the dust motion from the velocity field of the polarized H$\alpha$ emission line. The dust is accelerated outward on the northwest side of the nucleus. A simple bi-conical dust outflow model shows that the outflow velocity of the dust reaches {\textgreater} ∼ 300−450 km s−1 at ∼ 4 kpc from the nucleus, suggesting that some portion of the dust escapes from the gravitational potential of M82 into the intergalactic space. At some regions on the southeast side, in particular along the position angle of 138◦, the dust has radial velocity slower than the systemic velocity of the galaxy, apparently suggesting inflowing motion toward the nucleus. These components are spatially consistent with a part of the molecular gas stream, which is kinematically independent of the outflow gas, thus the apparent inflow motion of the dust reflects the streaming motion associated with the molecular gas stream.},
archivePrefix = {arXiv},
arxivId = {1711.00240},
author = {Yoshida, Michitoshi and Kawabata, Koji and Ohyama, Youichi and Itoh, Ryosuke and Hattori, Takashi},
doi = {10.1093/pasj/xxx000},
eprint = {1711.00240},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Yoshida et al. - 2019 - Spectropolarimetry of the superwind filamentsof the starburst galaxy M82 II kinematics of thedust surrounding th.pdf:pdf},
issn = {0004-6264},
keywords = {astronomical society of japan,c 2018,dust,galaxies,individual,interstellar,m82,nearby,starburst},
number = {1},
pages = {1--21},
title = {{Spectropolarimetry of the superwind filamentsof the starburst galaxy M82 II: kinematics of thedust surrounding the nuclear starburst}},
url = {http://arxiv.org/abs/1711.00240},
volume = {00},
year = {2019}
}

@article{MelioliDalPino2015ApJ...812...90M,
archivePrefix = {arXiv},
arxivId = {1509.00357},
author = {Melioli, C and {de Gouveia Dal Pino}, E.{\~{}}M.},
doi = {10.1088/0004-637X/812/2/90},
eprint = {1509.00357},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Melioli, Pino - 2015 - GAS OUTFLOWS in SEYFERT GALAXIES EFFECTS of STAR FORMATION VERSUS AGN FEEDBACK.pdf:pdf},
journal = {Apj},
keywords = {ISM: kinematics and dynamics,evolution,galaxies: ISM,galaxies: Seyfert,galaxies: active,galaxies: jets},
pages = {90},
title = {{Gas Outflows in Seyfert Galaxies: Effects of Star Formation versus AGN Feedback}},
volume = {812},
year = {2015}
}

@article{Melioli-dGDPino2015,
    archivePrefix = {arXiv},
    arxivId = {1509.00357},
    author = {MdGDP15},
    doi = {10.1088/0004-637X/812/2/90},
    eprint = {1509.00357},
    file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Melioli, Pino - 2015 - GAS OUTFLOWS in SEYFERT GALAXIES EFFECTS of STAR FORMATION VERSUS AGN FEEDBACK.pdf:pdf},
    journal = {Apj},
    keywords = {ISM: kinematics and dynamics,evolution,galaxies: ISM,galaxies: Seyfert,galaxies: active,galaxies: jets},
    pages = {90},
    title = {{Gas Outflows in Seyfert Galaxies: Effects of Star Formation versus AGN Feedback}},
    volume = {812},
    year = {2015}
}

@article{Park2018a,
abstract = {We study Faraday rotation in the jet of M87 inside the Bondi radius using eight Very Long Baseline Array data sets, one at 8 GHz, four at 5 GHz, and three at 2 GHz. We obtain Faraday rotation measures (RMs) measured across the bandwidth of each data set. We find that the magnitude of RM systematically decreases with increasing distance from the black hole from 5,000 to 200,000 Schwarzschild radii. The data, showing predominantly negative RM sign without significant difference of the RMs on the northern and southern jet edges, suggest that the spatial extent of the Faraday screen is much larger than the jet. We apply models of hot accretion flows, thought to be prevalent in active galactic nuclei having relatively low luminosity such as M87, and find that the decrease of RM is described well by a gas density profile {\$}\backslashrho \backslashpropto r{\^{}}{\{}-1{\}}{\$}. This behavior matches the theoretically expected signature of substantial winds, nonrelativistic un-collimated gas outflows from hot accretion flows, which is consistent with the results of various numerical simulations. The pressure profile inferred from the density profile is flat enough to collimate the jet, which can result in gradual acceleration of the jet in a magneto-hydrodynamical process. This picture is in good agreement with the observed gradual collimation and acceleration of the M87 jet inside the Bondi radius. The dominance of negative RMs suggests that jet and wind axis are misaligned such that the jet emission exposes only one side of the toroidal magnetic fields permeating the winds.},
archivePrefix = {arXiv},
arxivId = {1812.08386},
author = {Park, Jongho and Hada, Kazuhiro and Kino, Motoki and Nakamura, Masanori and Ro, Hyunwook and Trippe, Sascha},
doi = {10.3847/1538-4357/aaf9a9},
eprint = {1812.08386},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Park et al. - 2018 - Faraday rotation in the jet of M87 inside the Bondi radius indication of winds from hot accretion flows confining t.pdf:pdf},
issn = {15384357},
pages = {1--24},
title = {{Faraday rotation in the jet of M87 inside the Bondi radius: indication of winds from hot accretion flows confining the relativistic jet}},
url = {http://arxiv.org/abs/1812.08386},
year = {2018}
}

@article{Husemann2012,
abstract = {We present a detailed analysis of a large sample of 31 low-redshift, mostly radio-quiet type 1 quasi-stellar objects (QSOs) observed with integral field spectroscopy to study their extended emission-line regions (EELRs). We focus on the ionisation state of the gas, size and luminosity of extended narrow line regions (ENLRs), which corresponds to those parts of the EELR dominated by ionisation from the QSO, as well as the kinematics of the ionised gas. We detect EELRs around 19 of our 31 QSOs (61{\%}) after deblending the unresolved QSO emission and the extended host galaxy light in the integral field data with a new dedicated algorithm. Based on standard emission-line diagnostics we identify 13EELRs to be entirely ionised by the QSO radiation, 3 EELRs are composed of H ii regions and 3 EELRs display signatures of both ionisation mechanisms at different locations. The typical size of the ENLR is∼10 kpc at a median nuclear [O III] luminosity of log (L([Oiii])/[ergs-1])=42.7±0. 15. We show that the ENLR sizes are least a factor of ∼2 larger than determined with the Hubble Space Telescope, but are consistent with those of recently reported type 2 QSOs at matching [O III] luminosities. The ENLR of type 1 and type 2 QSOs therefore appear to follow the same size-luminosity relation. Furthermore, we show for the first time that the ENLR size is much better correlated with the QSO continuum luminosity than with the total/nuclear [O III] luminosity. We show that ENLR luminosity and radio luminosity are correlated, and argue that radio jets even in radio-quiet QSOs are important for shaping the properties of the ENLR. Strikingly, the kinematics of the ionised gas is quiescent and likely gravitationally driven in the majority of cases and we find only 3 objects with radial gas velocities exceeding {\textgreater}400 km s-1 in specific regions of the EELR that can be associate with radio jets. In general, these are significantly lower outflow velocities and detection rates compared to starburst galaxies or radio-loud QSOs. This represent a challenge for some theoretical feedback models in which luminous QSOs are expected to radiatively drive an outflow out to scales of the entire host galaxy. {\textcopyright} ESO, 2012.},
archivePrefix = {arXiv},
arxivId = {1210.0566},
author = {Husemann, B. and Wisotzki, L. and S{\'{a}}nchez, S. F. and Jahnke, K.},
doi = {10.1051/0004-6361/201220076},
eprint = {1210.0566},
file = {:home/william/Documents/Papers/[Husseman]-The properties of the extended warm ionised gas around.pdf:pdf},
issn = {00046361},
journal = {Astron. Astrophys.},
keywords = {Galaxies: ISM,Galaxies: active,Quasars: emission lines},
title = {{The properties of the extended warm ionised gas around low-redshift QSOs and the lack of extended high-velocity outflows}},
volume = {549},
year = {2012}
}
@article{Dashyan2018,
abstract = {Dwarf galaxy anomalies, such as their abundance and cusp-core problems, remain a prime challenge in our understanding of galaxy formation. The inclusion of baryonic physics could potentially solve these issues, but the efficiency of stellar feedback is still controversial. We analytically explore the possibility of feedback from active galactic nuclei (AGNs) in dwarf galaxies and compare AGN and supernova (SN) feedback. We assume the presence of an intermediate-mass black hole within low-mass galaxies and standard scaling relations between the relevant physical quantities. We model the propagation and properties of the outflow and explore the critical condition for global gas ejection. Performing the same calculation for SNe, we compare the ability of AGNs and SNe to drive gas out of galaxies. We find that a critical halo mass exists below which AGN feedback can remove gas from the host halo and that the critical halo mass for an AGN is greater than the equivalent for SNe in a significant part of the parameter space, suggesting that an AGN could provide an alternative and more successful source of negative feedback than SNe, even in the most massive dwarf galaxies.},
archivePrefix = {arXiv},
arxivId = {1710.05900},
author = {Dashyan, Gohar and Silk, Joseph and Mamon, Gary A and Dubois, Yohan and Hartwig, Tilman},
doi = {10.1093/MNRAS/STX2716},
eprint = {1710.05900},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Dashyan et al. - 2018 - AGN feedback in dwarf galaxies 1 I N T RO D U C T I O N.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Black hole physics -methods: analytical,Galaxies: active,Galaxies: dwarf,Galaxies: evolution,Galaxies: luminosity function,Mass function},
number = {4},
pages = {5698--5703},
title = {{AGN feedback in dwarf galaxies?}},
volume = {473},
year = {2018}
}
@article{Barai2018,
author = {Barai, Paramita and de Gouveia Dal Pino, Elisabete},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Barai, Gouveia, Pino - 2018 - Intermediate-Mass Black Holes in Dwarf Galaxies at High Redshifts.pdf:pdf},
number = {February},
title = {{Intermediate-Mass Black Holes in Dwarf Galaxies at High Redshifts}},
volume = {000},
year = {2018}
}
@article{Heywood2019,
abstract = {The Galactic Centre contains a supermassive black hole with a mass of four million Suns1 within an environment that differs markedly from that of the Galactic disk. Although the black hole is essentially quiescent in the broader context of active galactic nuclei, X-ray observations have provided evidence for energetic outbursts from its surroundings2. Also, although the levels of star formation in the Galactic Centre have been approximately constant over the past few hundred million years, there is evidence of increased short-duration bursts3, strongly influenced by the interaction of the black hole with the enhanced gas density present within the ring-like central molecular zone4 at Galactic longitude |l| {\textless} 0.7 degrees and latitude |b| {\textless} 0.2 degrees. The inner 200-parsec region is characterized by large amounts of warm molecular gas5, a high cosmic-ray ionization rate6, unusual gas chemistry, enhanced synchrotron emission7,8, and a multitude of radio-emitting magnetized filaments9, the origin of which has not been established. Here we report radio imaging that reveals a bipolar bubble structure, with an overall span of 1 degree by 3 degrees (140 parsecs × 430 parsecs), extending above and below the Galactic plane and apparently associated with the Galactic Centre. The structure is edge-brightened and bounded, with symmetry implying creation by an energetic event in the Galactic Centre. We estimate the age of the bubbles to be a few million years, with a total energy of 7 × 1052 ergs. We postulate that the progenitor event was a major contributor to the increased cosmic-ray density in the Galactic Centre, and is in turn the principal source of the relativistic particles required to power the synchrotron emission of the radio filaments within and in the vicinity of the bubble cavities.},
author = {Heywood, I. },
doi = {10.1038/s41586-019-1532-5},
file = {:home/william/Documents/Papers/s41586-019-1532-5.pdf:pdf},
isbn = {4158601915325},
issn = {14764687},
journal = {Nature},
number = {7773},
pages = {235--237},
pmid = {31511683},
title = {{Inflation of 430-parsec bipolar radio bubbles in the Galactic Centre by an energetic event}},
volume = {573},
year = {2019}
}
@article{Manuscript2018,
author = {Manuscript, Original},
doi = {00.0000/X000000000000000X},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Manuscript - 2018 - Fo r R iew On Fo r R iew On ly.pdf:pdf},
isbn = {1303270218},
keywords = {allergy,asthma and immunology research},
title = {{Fo r R iew On Fo r R iew On ly}},
year = {2018}
}
@article{Netzer1993,
abstract = {Broad absorption features are common in the X-ray spectrum of low-luminosity AGNs. The features have been modeled by leaky neutral absorbers or by highly ionized gas that completely occult the continuum source. Such models are incomplete since they do not take into account all the physical processes in the gas. In particular, no previous model included the X-ray emission by the ionized absorbing gas and the reflection of the continuum source radiation. The present work discusses the emission, absorption, and reflection properties of photoionized gases with emphasis on conditions thought to prevail in AGNs. It shows that such gas is likely to produce intense X-ray line and continuum radiation and to reflect a sizable fraction of the nonstellar continuum at all energies. If such gas is indeed responsible for the observed X-ray absorption, then absorption edges are much weaker than commonly assumed, and some residual X-ray continuum is likely to be observed even if the line of sight is completely blocked. Moreover, X-ray emission features may show up in sources not showing X-ray absorption. This has immense consequences for medium-resolution X-ray missions, such as BBXRT and Astro-D, and for the planned high-resolution experiments on board XMM and AXAF.},
author = {Netzer, Hagai},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Netzer - 1993 - Ionized Absorbers, ionized emitters, and the X-ray spectrum of AGN.pdf:pdf},
journal = {Apj},
pages = {594--601},
title = {{Ionized Absorbers, ionized emitters, and the X-ray spectrum of AGN}},
volume = {411},
year = {1993}
}
@article{Santoro2020,
abstract = {Active galactic nuclei (AGN) feedback operated by the expansion of radio jets can play a crucial role in driving gaseous outflows on galaxy scales. Galaxies hosting young radio AGN, whose jets are in the first phases of expansion through the surrounding interstellar medium (ISM), are the ideal targets to probe the energetic significance of this mechanism. In this paper, we characterise the warm ionised gas outflows in a sample of nine young radio sources from the 2Jy sample, combining X-shooter spectroscopy and Hubble Space Telescope (HST) imaging data. We find that the warm outflows have similar radial extents (∼0.06 – 2 kpc) as radio sources, consistent with the idea that ‘jet mode' AGN feedback is the dominant driver of the outflows detected in young radio galaxies. Exploiting the broad spectral coverage of the X-shooter data, we have used the ratios of trans-auroral emission lines of [S ii] and [O ii] to estimate the electron densities, finding that most of the outflows have gas densities (log(ne cm−3) ∼ 3 − 4.8), which we speculate could be the result of compression by jet-induced shocks. Combining our estimates of the emission-line luminosities, radii, and densities, we find that the kinetic powers of the warm outflows are a relatively small fraction of the energies available from the accretion of material onto the central supermassive black hole (SMBH), reflecting AGN feedback efficiencies below 1{\%} in most cases. Overall, the warm outflows detected in our sample are strikingly similar to those found in nearby ultraluminous infrared galaxies (ULIRGs), but more energetic and with a high feedback efficiencies on average than the general population of nearby AGN of similar bolometric luminosity; this is likely to reflect a high degree of coupling between the jets and the near-nuclear ISM in the early stages of radio source evolution.},
author = {Santoro, Francesco and Tadhunter, C. and Baron, D. and Morganti, R. and Holt, J.},
file = {:home/william/Documents/Papers/aa39077-20.pdf:pdf},
issn = {23318422},
journal = {arXiv},
keywords = {Galaxies: active, evolution, ISM,ISM: jets and outflows, evolution},
title = {{AGN-driven outflows and the AGN feedback efficiency in young radio galaxies}},
volume = {54},
year = {2020}
}
@article{Wylezalek2018,
abstract = {Different mechanisms can drive outflows in active galactic nuclei (AGNs), but it is often unclear which mechanism dominates, if any. To quantify the impact of AGN feedback on galaxy evolution, the driving mechanism of outflows must be better understood.},
author = {Wylezalek, Dominika and Morganti, Raffaella},
doi = {10.1038/s41550-018-0409-0},
file = {:home/william/Documents/Papers/wylezalek2018.pdf:pdf},
issn = {23973366},
journal = {Nat. Astron.},
number = {3},
pages = {181--182},
publisher = {Springer US},
title = {{Questions and challenges of what powers galactic outflows in active galactic nuclei}},
url = {http://dx.doi.org/10.1038/s41550-018-0409-0},
volume = {2},
year = {2018}
}
@article{Geral2018,
author = {Geral, Quadro},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Geral - 2018 - Proposta 5258681595890087.pdf:pdf},
title = {{Proposta 5258681595890087}},
volume = {1},
year = {2018}
}
@article{Knapen2018,
abstract = {We present the discovery of a small {\$}0.2{\^{}}{\{}\backslashprime\backslashprime{\}}{\$} (60 pc) radius kinematically decoupled core, as well as an outflow jet, in the archetypical AGN-starburst "composite" galaxy NGC 7130 from integral field data obtained with the adaptive optics-assisted MUSE-NFM instrument on the VLT. Correcting the already good natural seeing at the time of our science verification observations with the four-laser GALACSI AO system we reach an unprecedented spatial resolution of around {\$}0.15{\^{}}{\{}\backslashprime\backslashprime{\}}{\$}. We confirm the existence of star-forming knots arranged in an {\$}0.58{\^{}}{\{}\backslashprime\backslashprime{\}}{\$} (185 pc) radius ring around the nucleus, previously observed from UV and optical {\{}$\backslash$it Hubble Space Telescope{\}} and CO(6-5) ALMA imaging. We determine the position of the nucleus as the location of a peak in gas velocity dispersion. A plume of material extends towards the NE from the nucleus until at least the edge of our FOV at 2{\$}{\^{}}{\{}\backslashprime\backslashprime{\}}{\$} (640 pc) radius which we interpret as an outflow jet originating in the AGN. The plume is not visible morphologically, but is clearly characterised in our data by emission lines ratios characteristic of AGN emission, enhanced gas velocity dispersion, and distinct non-circular gas velocities. Its orientation is roughly perpendicular to line of nodes of the rotating host galaxy disk. An {\$}0.2{\^{}}{\{}\backslashprime\backslashprime{\}}{\$}-radius circumnuclear area of positive and negative velocities indicates a tiny inner disk, which can only be seen after combining the integral field spectroscopic capabilities of MUSE with adaptive optics.},
archivePrefix = {arXiv},
arxivId = {1812.00809},
author = {Knapen, J. H. and Comer{\'{o}}n, S. and Seidel, M. K.},
doi = {10.1051/0004-6361/201834669},
eprint = {1812.00809},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Knapen, Comer{\'{o}}n, Seidel - 2018 - MUSE-AO view of the starburst-AGN connection NGC 7130.pdf:pdf},
issn = {1432-0746},
keywords = {active,galaxies,individual,ism,jets,ngc 7130,nuclei},
pages = {1--6},
title = {{MUSE-AO view of the starburst-AGN connection: NGC 7130}},
url = {http://arxiv.org/abs/1812.00809},
year = {2018}
}
@article{Russell2018a,
abstract = {We present a new 300 ks Chandra observation of M87 that limits pileup to only a few per cent of photon events and maps the hot gas properties closer to the nucleus than has previously been possible. Within the supermassive black hole's gravitational sphere of influence, the hot gas is multiphase and spans temperatures from 0.2 to 1 keV. The radiative cooling time of the lowest temperature gas drops to only 0.1-0.5 Myr, which is comparable to its free fall time. Whilst the temperature structure is remarkably symmetric about the nucleus, the density gradient is steep in sectors to the N and S, with {\$}\backslashrho{\{}\backslashpropto{\}}r{\^{}}{\{}-1.5\backslashpm0.1{\}}{\$}, and significantly shallower along the jet axis to the E, where {\$}\backslashrho{\{}\backslashpropto{\}}r{\^{}}{\{}-0.93\backslashpm0.07{\}}{\$}. The density structure within the Bondi radius is therefore consistent with steady inflows perpendicular to the jet axis and an outflow directed E along the jet axis. By putting limits on the radial flow speed, we rule out Bondi accretion on the scale resolved at the Bondi radius. We show that deprojected spectra extracted within the Bondi radius can be equivalently fit with only a single cooling flow model, where gas cools from 1.5 keV down below 0.1 keV at a rate of 0.03 M{\$}{\_}{\{}\backslashodot{\}}{\$}/yr. For the alternative multi-temperature spectral fits, the emission measures for each temperature component are also consistent with a cooling flow model. The lowest temperature and most rapidly cooling gas in M87 is therefore located at the smallest radii at {\~{}}100 pc and may form a mini cooling flow. If this cooling gas has some angular momentum, it will feed into the cold gas disk around the nucleus, which has a radius of {\~{}}80 pc and therefore lies just inside the observed transition in the hot gas structure.},
author = {Russell, H. R. and Fabian, A. C. and McNamara, B. R. and Miller, J. M. and Nulsen, P. E.J. and Piotrowska, J. M. and Reynolds, C. S.},
doi = {10.1093/mnras/sty835},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Russell et al. - 2018 - The imprints of AGN feedback within a supermassive black hole's sphere of influence.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: Clusters: M87,Intergalactic medium,X-rays: Galaxies: Clusters},
number = {3},
pages = {3583--3599},
title = {{The imprints of AGN feedback within a supermassive black hole's sphere of influence}},
volume = {477},
year = {2018}
}
@article{Williams2016,
abstract = {We present the first wide area (19 deg2), deep (≈120-150 $\mu$Jy beam-1), high-resolution (5.6 × 7.4 arcsec) LOFAR High Band Antenna image of the Bo{\"{o}}tes field made at 130-169 MHz. This image is at least an order of magnitude deeper and 3-5 times higher in angular resolution than previously achieved for this field at low frequencies. The observations and data reduction, which includes full direction-dependent calibration, are described here. We present a radio source catalogue containing 6 276 sources detected over an area of 19 deg2, with a peak flux density threshold of 5$\sigma$. As the first thorough test of the facet calibration strategy, introduced by van Weeren et al., we investigate the flux and positional accuracy of the catalogue. We present differential source counts that reach an order of magnitude deeper in flux density than previously achieved at these low frequencies, and show flattening at 150-MHz flux densities below 10 mJy associated with the rise of the low flux density star-forming galaxies and radio-quiet AGN.},
archivePrefix = {arXiv},
arxivId = {1605.01531},
author = {Williams, W. L. and {Van Weeren}, R. J. and R{\"{o}}ttgering, H. J.A. and Best, P. and Dijkema, T. J. and {De Gasperin}, F. and Hardcastle, M. J. and Heald, G. and Prandoni, I. and Sabater, J. and Shimwell, T. W. and Tasse, C. and {Van Bemmel}, I. M. and Br{\"{u}}ggen, M. and Brunetti, G. and Conway, J. E. and En{\ss}lin, T. and Engels, D. and Falcke, H. and Ferrari, C. and Haverkorn, M. and Jackson, N. and Jarvis, M. J. and Kapi{\'{n}}ska, A. D. and Mahony, E. K. and Miley, G. K. and Morabito, L. K. and Morganti, R. and Orr{\'{u}}, E. and Retana-Montenegro, E. and Sridhar, S. S. and Toribio, M. C. and White, G. J. and Wise, M. W. and Zwart, J. T.L.},
doi = {10.1093/mnras/stw1056},
eprint = {1605.01531},
file = {:home/william/Documents/Papers/stw1056.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: active,Radio continuum: galaxies,Surveys,Techniques: interferometric},
number = {3},
pages = {2385--2412},
title = {{LOFAR 150-MHz observations of the Bo{\"{o}}tes field: Catalogue and source counts}},
volume = {460},
year = {2016}
}
@article{Marasco2020,
abstract = {We used MUSE adaptive optics data in narrow field mode to study the properties of the ionised gas in MR 2251-178 and PG 1126-041, two nearby (z0.06) bright quasars (QSOs) hosting sub-pc scale ultra-fast outflows (UFOs) detected in the X-ray band. We decomposed the optical emission from diffuse gas into a low- and a high-velocity components. The former is characterised by a clean, regular velocity field and a low (∼80 km s-1) velocity dispersion. It traces regularly rotating gas in PG 1126-041, while in MR 2251-178 it is possibly associated with tidal debris from a recent merger or flyby. The other component is found to be extended up to a few kpc from the nuclei, and shows a high (∼800 km s-1) velocity dispersion and a blue-shifted mean velocity, as is expected from outflows driven by active galactic nuclei (AGN). We estimate mass outflow rates up to a few Mpdbl yr-1 and kinetic efficiencies LKIN/LBOL between 1-4 × 10-4, in line with those of galaxies hosting AGN of similar luminosities. The momentum rates of these ionised outflows are comparable to those measured for the UFOs at sub-pc scales, which is consistent with a momentum-driven wind propagation. Pure energy-driven winds are excluded unless about 100× additional momentum is locked in massive molecular winds. In comparing the outflow properties of our sources with those of a small sample of well-studied QSOs hosting UFOs from the literature, we find that winds seem to systematically lie either in a momentum-driven or an energy-driven regime, indicating that these two theoretical models bracket the physics of AGN-driven winds very well.},
archivePrefix = {arXiv},
arxivId = {2009.11294},
author = {Marasco, A. and Cresci, G. and Nardini, E. and Mannucci, F. and Marconi, A. and Tozzi, P. and Tozzi, G. and Amiri, A. and Venturi, G. and Piconcelli, E. and Lanzuisi, G. and Tombesi, F. and Mingozzi, M. and Perna, M. and Carniani, S. and Brusa, M. and {DI Serego Alighieri}, S.},
doi = {10.1051/0004-6361/202038889},
eprint = {2009.11294},
file = {:home/william/Documents/Papers/2009.11294.pdf:pdf},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Galaxies: ISM,ISM: jets and outflows,Quasars: individual: MR 2251-178,Quasars: individual: PG 1126-041,Techniques: imaging spectroscopy},
pages = {1--18},
title = {{Galaxy-scale ionised winds driven by ultra-fast outflows in two nearby quasars}},
volume = {644},
year = {2020}
}
@article{Ji2017,
abstract = {Cold ({\$}T\backslashsim 10{\^{}}{\{}4{\}} \backslash \backslashmathrm{\{}K{\}}{\$}) gas is very commonly found in both galactic and cluster halos. There is no clear consensus on its origin. Such gas could be uplifted from the central galaxy by galactic or AGN winds. Alternatively, it could form in situ by thermal instability. Fragmentation into a multi-phase medium has previously been shown in hydrodynamic simulations to take place once {\$}t{\_}\backslashmathrm{\{}cool{\}}/t{\_}\backslashmathrm{\{}ff{\}}{\$}, the ratio of the cooling time to the free-fall time, falls below a threshold value. Here, we use 3D plane-parallel MHD simulations to investigate the influence of magnetic fields. We find that because magnetic tension suppresses buoyant oscillations of condensing gas, it destabilizes all scales below {\$}l{\_}\backslashmathrm{\{}A{\}}{\^{}}\backslashmathrm{\{}cool{\}} \backslashsim v{\_}\backslashmathrm{\{}A{\}} t{\_}\backslashmathrm{\{}cool{\}}{\$}, enhancing thermal instability. This effect is surprisingly independent of magnetic field orientation or cooling curve shape, and sets in even at very low magnetic field strengths. Magnetic fields critically modify both the amplitude and morphology of thermal instability, with {\$}\backslashdelta \backslashrho/\backslashrho \backslashpropto \backslashbeta{\^{}}{\{}-1/2{\}}{\$}, where {\$}\backslashbeta{\$} is the ratio of thermal to magnetic pressure. In galactic halos, magnetic fields can render gas throughout the entire halo thermally unstable, and may be an attractive explanation for the ubiquity of cold gas, even in the halos of passive, quenched galaxies.},
archivePrefix = {arXiv},
arxivId = {1710.00822},
author = {Ji, Suoqing and Oh, S. Peng and McCourt, Michael},
doi = {10.1093/mnras/sty293},
eprint = {1710.00822},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ji, Oh, McCourt - 2017 - The impact of magnetic fields on thermal instability.pdf:pdf},
issn = {0035-8711},
keywords = {clusters,evolution,galaxies,general,haloes},
number = {October},
pages = {1--16},
title = {{The impact of magnetic fields on thermal instability}},
url = {http://arxiv.org/abs/1710.00822},
volume = {16},
year = {2017}
}
@article{Figure,
author = {Figure, Supplementary},
doi = {10.15713/ins.mmj.3},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Figure - Unknown - No Title No Title{\_}2015(2).pdf:pdf},
isbn = {9789004310087},
number = {c},
pages = {1--4},
pmid = {29982528},
title = {{No Title No Title{\_}2015}}
}
@article{Husemann2018a,
abstract = {Feedback from active galactic nuclei (AGNs) remains controversial despite its wide acceptance as necessary to regulate massive galaxy growth. Consequently, we held a workshop in October 2017, at Leiden's Lorentz Center, to distinguish between the reality and myths of feedback.},
archivePrefix = {arXiv},
arxivId = {1802.10304},
author = {Husemann, Bernd and Harrison, Chris M.},
doi = {10.1038/s41550-018-0407-2},
eprint = {1802.10304},
file = {:home/william/Documents/Papers/husemann2018.pdf:pdf},
issn = {23973366},
journal = {Nat. Astron.},
number = {3},
pages = {196--197},
publisher = {Springer US},
title = {{Reality and myths of AGN feedback}},
url = {http://dx.doi.org/10.1038/s41550-018-0407-2},
volume = {2},
year = {2018}
}
@article{Sun2017,
abstract = {To study the impact of active galactic nuclei (AGN) feedback on the galactic ISM, we present Magellan long-slit spectroscopy of 12 luminous nearby type 2 AGN (L{\_}bol{\~{}}10{\^{}}{\{}45.0-46.5{\}} erg/s, z{\~{}}0.1). These objects are selected from a parent sample of spectroscopically identified AGN to have high [OIII]{\{}$\backslash$lambda{\}}5007 and WISE mid-IR luminosities and extended emission in the SDSS r-band images, suggesting the presence of extended [OIII]{\{}$\backslash$lambda{\}}5007 emission. We find spatially resolved [OIII] emission (2-35 kpc from the nucleus) in 8 out of 12 of these objects. Combined with samples of higher luminosity type 2 AGN, we confirm that the size of the narrow-line region (R{\_}NLR) scales with the mid-IR luminosity until the relation flattens at {\~{}}10 kpc. Nine out of 12 objects in our sample have regions with broad [OIII] linewidths (w{\_}80{\textgreater}600 km/s), indicating outflows. We define these regions as the kinematically-disturbed region (KDR). The size of the KDR (R{\_}KDR) is typically smaller than R{\_}NLR by few kpc but also correlates strongly with the AGN mid-IR luminosity. Given the unknown density in the gas, we derive a wide range in the energy efficiency {\{}$\backslash$eta{\}}=dot{\{}E{\}}/L{\_}bol=0.01{\%}-30{\%}. We find no evidence for an AGN luminosity threshold below which outflows are not launched. To explain the sizes, velocity profiles, and high occurrence rates of the outflows in the most luminous AGN, we propose a scenario in which energy-conserving outflows are driven by AGN episodes with {\~{}}10{\^{}}8-year durations. Within each episode the AGN flickers on shorter timescales, with a cadence of {\~{}}10{\^{}}6 year active phases separated by {\~{}}10{\^{}}7 years.},
archivePrefix = {arXiv},
arxivId = {1611.04469},
author = {Sun, Ai-Lei and Greene, Jenny E. and Zakamska, Nadia L.},
doi = {10.3847/1538-4357/835/2/222},
eprint = {1611.04469},
file = {:home/william/Documents/Papers/[Sun et al.]-Sizes and Kinematics of Extended Narrow-line Regions in Luminous Obscured AGN.pdf:pdf},
issn = {1538-4357},
journal = {Astrophys. J.},
keywords = {ISM: jets and outflows,active,emission lines,galaxies,galaxies: active,ism,jets and out fl,ows,quasars,quasars: emission lines,quasars: supermassive black holes,supermassive black holes},
number = {2},
pages = {222},
publisher = {IOP Publishing},
title = {{Sizes and Kinematics of Extended Narrow-line Regions in Luminous Obscured AGN Selected by Broadband Images}},
url = {http://dx.doi.org/10.3847/1538-4357/835/2/222},
volume = {835},
year = {2017}
}
@article{Hartwig2018,
abstract = {Galactic outflows, driven by active galactic nuclei (AGNs), play a crucial role in galaxy formation and in the self-regulated growth of supermassive black holes (BHs). AGN feedback couples to and affects gas, rather than stars, and in many, if not most, gas-rich galaxies cold gas is rotationally supported and settles in a disc.We present a 2Danalytical model forAGN-driven outflows in a gaseous disc and demonstrate the main improvements, compared to existing 1D solutions. We find significant differences for the outflow dynamics and wind efficiency. The outflow is energy-driven due to inefficient cooling up to a certain AGN luminosity ({\~{}}1043 erg s-1 in our fiducial model), above which the outflow remains momentum-driven in the disc up to galactic scales.We reproduce results of 3D simulations that gas is preferentially ejected perpendicular to the disc and find that the fraction of ejected interstellar medium is lower than in 1D models. The recovery time of gas in the disc, defined as the free-fall time from the radius to which the AGN pushes the ISM at most, is remarkably short, of the order 1Myr. This indicates that AGN-driven winds cannot suppress BH growth for long. Without the inclusion of supernova feedback, we find a scaling of the BH mass with the halo velocity dispersion of MBH ∝ $\sigma$4.8.},
archivePrefix = {arXiv},
arxivId = {1707.03826},
author = {Hartwig, Tilman and Volonteri, Marta and Dashyan, Gohar},
doi = {10.1093/MNRAS/STY229},
eprint = {1707.03826},
file = {:home/william/Documents/Papers/sty229.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Black hole physics,Galaxies: active,Methods: analytical,Quasars: general,Quasars: supermassive black holes},
number = {2},
pages = {2288--2307},
title = {{Active galactic nucleus outflows in galaxy discs}},
volume = {476},
year = {2018}
}
@article{Monroe1970,
abstract = {The problem of representing electromagnetic fields in an electron plasma subjected to large and rapid electron-density variations due to transient ionization processes is considered. The inherently nonlinear character of this problem, which arises in the Maxwell-Euler equations through the electron transport term ▽{\textperiodcentered}(nV), is retained under the assumption that temporal variations of the electron density n are of first order in magnitude while spatial variations in n are of second order. That is, we asume V{\textperiodcentered}▽n≪n▽{\textperiodcentered}V and consequently, ▽{\textperiodcentered}(nV) ≃n▽{\textperiodcentered}V, where V is the induced velocity field. With the aid of vector and scalar potentials, it is shown that, in this case, the set of ten coupled Maxwell-Euler equations describing a cold, isotropic, lossy, electron plasma with current and ionization sources can be reduced to a set of five integro-differential equations which are effectively decoupled. A method of solving these equations based on perturbation techniques is sketched for the case where the initial electron density is zero. {\textcopyright} 1970 The American Institute of Physics.},
author = {Monroe, Richard L.},
doi = {10.1063/1.1658713},
file = {:home/william/Documents/Papers/monroe1970.pdf:pdf},
issn = {00218979},
journal = {J. Appl. Phys.},
number = {2},
pages = {560--562},
title = {{Electromagnetic radiation in a time-varying plasma}},
volume = {41},
year = {1970}
}
@article{Baron2018c,
abstract = {Post starburst E+A galaxies show indications of a powerful starburst that was quenched abruptly. Their disturbed, bulge-dominated morphologies suggest that they are merger remnants. The more massive E+A galaxies are suggested to be quenched by AGN feedback, yet little is known about AGN-driven winds in this short-lived phase. We present spatially-resolved IFU spectroscopy by the Keck Cosmic Web Imager of SDSS J003443.68+251020.9, at z=0.118. The system consists of two galaxies, the larger of which is a post starburst E+A galaxy hosting an AGN. Our modelling suggests a 400 Myrs starburst, with a peak star formation rate of 120 Msun/yr. The observations reveal stationary and outflowing gas, photoionized by the central AGN. We detect gas outflows to a distance of 17 kpc from the central galaxy, far beyond the region of the stars (about 3 kpc), inside a conic structure with an opening angle of 70 degrees. We construct self-consistent photoionization and dynamical models for the different gas components and show that the gas outside the galaxy forms a continuous flow, with a mass outflow rate of about 24 Msun/yr. The gas mass in the flow, roughly {\$}10{\^{}}9{\$} Msun, is larger than the total gas mass within the galaxy, some of which is outflowing too. The continuity of the flow puts a lower limit of 60 Myrs on the duration of the AGN feedback. Such AGN are capable of removing, in a single episode, most of the gas from their host galaxies and expelling enriched material into the surrounding CGM.},
archivePrefix = {arXiv},
arxivId = {1804.03150},
author = {Baron, Dalya and Netzer, Hagai and Prochaska, J. Xavier and Cai, Zheng and Cantalupo, Sebastiano and Martin, D. Christopher and Matuszewski, Mateusz and Moore, Anna M. and Morrissey, Patrick and Neill, James D.},
doi = {10.1093/mnras/sty2113},
eprint = {1804.03150},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Baron et al. - 2018 - Direct evidence of AGN-feedback a post starburst galaxy stripped of its gas by AGN-driven winds(2).pdf:pdf},
issn = {0035-8711},
keywords = {1 i n t,active,evolution,galaxies,general,interactions,masses of su-,ro d u c,star formation,strong correlation between the,t i o n,the discovery of a},
pages = {3993--4016},
publisher = {Oxford University Press},
title = {{Direct evidence of AGN-feedback: a post starburst galaxy stripped of its gas by AGN-driven winds}},
url = {http://arxiv.org/abs/1804.03150{\%}0Ahttp://dx.doi.org/10.1093/mnras/sty2113},
volume = {4016},
year = {2018}
}
@article{Marshall2017a,
abstract = {We present radiative transfer models of deeply buried ultraluminous infrared galaxy (ULIRG) spectral energy distributions and use them to construct a three-dimensional diagram for diagnosing the nature of ULIRG nuclei. Our diagnostic is based upon the properties dominating mid-IR continua of low-redshift ULIRGs: continuum slope, PAH equivalent width, and silicate feature strength. We use our diagnostic to analyze archival Spitzer Space Telescope IRS spectra of ULIRGs and find that: (1) {\textgreater}75{\%} (in some cases 100{\%}) of the bolometric luminosities of the most deeply buried ULIRGs must be powered by a hidden active galactic nucleus; (2) the observed absence of deeply buried ULIRGs with large PAH equivalent widths is naturally explained by our models showing that deep absorption features are quickly "filled-in" by small quantities of unobscured PAH emission at the level of {\~{}}1{\%} the bolometric nuclear luminosity (e.g., as emitted by the host galaxy disk); and (3) an unobscured "keyhole" view through {\textless}{\~{}}10{\%} of the obscuring medium surrounding a deeply buried ULIRG is sufficient to make it appear nearly unobscured in the mid-IR. This modeling and analysis of deeply buried galaxy spectra also provides a powerful tool for interpreting the mid-IR spectra of high-redshift sources to be obtained with superb angular resolution using the James Webb Space Telescope.},
archivePrefix = {arXiv},
arxivId = {1708.04709},
author = {Marshall, J. A. and Elitzur, M. and Armus, L. and Diaz-Santos, T. and Charmandaris, V.},
doi = {10.3847/1538-4357/aabcc0},
eprint = {1708.04709},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Marshall et al. - 2017 - The Nature of Deeply Buried Ultraluminous Infrared Galaxies A Unified Model for Highly Obscured Dusty Galaxy Em.pdf:pdf},
issn = {1538-4357},
keywords = {active,galaxies,infrared,ism,starburst},
title = {{The Nature of Deeply Buried Ultraluminous Infrared Galaxies: A Unified Model for Highly Obscured Dusty Galaxy Emission}},
url = {http://arxiv.org/abs/1708.04709},
year = {2017}
}
@article{Page2012,
abstract = {The old, red stars that constitute the bulges of galaxies, and the massive black holes at their centres, are the relics of a period in cosmic history when galaxies formed stars at remarkable rates and active galactic nuclei (AGN) shone brightly as a result of accretion onto black holes. It is widely suspected, but unproved, that the tight correlation between the mass of the black hole and the mass of the stellar bulge results from the AGN quenching the surrounding star formation as it approaches its peak luminosity. X-rays trace emission from AGN unambiguously, whereas powerful star-forming galaxies are usually dust-obscured and are brightest at infrared and submillimetre wavelengths. Here we report submillimetre and X-ray observations that show that rapid star formation was common in the host galaxies of AGN when the Universe was 2-6 billion years old, but that the most vigorous star formation is not observed around black holes above an X-ray luminosity of 1044 ergs per second. This suppression of star formation in the host galaxy of a powerful AGN is a key prediction of models in which the AGN drives an outflow, expelling the interstellar medium of its host and transforming the galaxy's properties in a brief period of cosmic time. {\textcopyright} 2012 Macmillan Publishers Limited.},
archivePrefix = {arXiv},
arxivId = {1310.4147},
author = {Page, M. J. and Symeonidis, M. and Vieira, J. D. and Altieri, B. and Amblard, A. and Arumugam, V. and Aussel, H. and Babbedge, T. and Blain, A. and Bock, J. and Boselli, A. and Buat, V. and Castro-Rodr{\~{n}}guez, N. and Cava, A. and Chanial, P. and Clements, D. L. and Conley, A. and Conversi, L. and Cooray, A. and Dowell, C. D. and Dubois, E. N. and Dunlop, J. S. and Dwek, E. and Dye, S. and Eales, E. and Elbaz, D. and Farrah, D. and Fox, M. and Franceschini, A. and Gear, G. and Glenn, J. and Griffin, M. and Halpern, M. and Hatziminaoglou, E. and Ibar, E. and Isaak, K. and Lagache, G. and Lagache, G. and Levenson, L. and Lu, N. and Madden, S. and Maffei, B. and Mainetti, G. and Marchetti, L. and Nguyen, H. T. and O'halloran, B. and Oliver, S. J. and Omont, A. and Panuzzo, P. and Papageorgiou, A. and Pearson, C. P. and P{\'{e}}rez-Fournon, I. and Pohlen, M. and Rawlings, J. I. and Rigopoulou, D. and Riguccini, L. and Rizzo, D. and Rodighiero, G. and Roseboom, I. G. and Rowan-Robinson, M. and Portal, M. S{\'{a}}nchez and Schulz, B. and Scott, D. and Seymour, N. and Shupe, D. L. and Smith, A. J. and Stevens, J. A. and Trichas, M. and Tugwell, K. E. and Vaccari, M. and Valtchanov, I. and Viero, M. and Vigroux, L. and Wang, L. and Ward, R. and Wright, G. and Xu, C. K. and Zemcov, M.},
doi = {10.1038/nature11096},
eprint = {1310.4147},
file = {:home/william/Documents/Papers/page2012.pdf:pdf},
issn = {00280836},
journal = {Nature},
number = {7397},
pages = {213--216},
title = {{The suppression of star formation by powerful active galactic nuclei}},
volume = {485},
year = {2012}
}
@article{Tesileanu2008,
abstract = {Context. Time-dependent cooling processes are of paramount importance in the evolution of astrophysical gaseous nebulae and, in particular, when radiative shocks are present. Given the recent improvements in resolution of the observational data, simulating these processes in a more realistic manner in magnetohydrodynamic (MHD) codes will provide a unique tool for model discrimination. Aims. The present work introduces a necessary set of tools that can be used to model radiative astrophysical flows in the optically-thin plasma limit. We aim to provide reliable and accurate predictions of emission line ratios and radiative cooling losses in astrophysical simulations of shocked flows. Moreover, we discuss numerical implementation aspects to ease future improvements and implementation in other MHD numerical codes. Methods. The most important source of radiative cooling for our plasma conditions comes from the collisionally-excited line radiation. We evolve a chemical network, including 29 ion species, to compute the ionization balance in non-equilibrium conditions. The numerical methods are implemented in the PLUTO code for astrophysical fluid dynamics and particular attention has been devoted to resolve accuracy and efficiency issues arising from cooling timescales considerably shorter than the dynamical ones. Results. After a series of validations and tests, typical astrophysical setups are simulated in 1D and 2D, employing both the present cooling model and a simplified one. The influence of the cooling model on structure morphologies can become important, especially for emission line diagnostic purposes. Conclusions. The tests make us confident that the use of the presented detailed radiative cooling treatment will allow more accurate predictions in terms of emission line intensities and shock dynamics in various astrophysical setups.},
author = {Te¸sileanu, O Te¸sileanu and Mignone, A and Massaglia, S},
doi = {10.1051/0004-6361:200809461},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Te¸sileanu, Mignone, Massaglia - 2008 - Astrophysics Simulating radiative astrophysical flows with the PLUTO code a non-equilibrium, mu.pdf:pdf},
journal = {A{\&}A},
pages = {429--440},
title = {{Astrophysics Simulating radiative astrophysical flows with the PLUTO code: a non-equilibrium, multi-species cooling function}},
volume = {488},
year = {2008}
}
@article{ClavijoBohorquez2021,
author = {{Clavijo Boh{\'{o}}rquez}, William Eduard and {de Gouveia Dal Pino}, Elisabete Mar{\'{i}}a and Melioli, Clauidio},
file = {:home/william/Documents/Papers/output.pdf:pdf},
keywords = {active galaxies,galactic winds,holes,magneto-hydrodynamical simulations,star formation,super massive black},
title = {{FEEDBACK IN GALAXIES HOSTING AGN AND SF WINDS ...}},
year = {2021}
}
@article{Zovaro2018,
abstract = {We report the discovery of shocked molecular and ionized gas resulting from jet-driven feedback in the compact radio galaxy 4C 31.04 using near-IR imaging spectroscopy. 4C 31.04 is a ∼ 100 pc double-lobed Compact Steep Spectrum source believed to be a very young AGN. It is hosted by a giant elliptical with a ∼ 10 9 M multi-phase gaseous circumnuclear disc. We used high spatial resolution, adaptive optics-assisted Hand K-band integral field Gemini/NIFS observations to probe (1) the warm (∼ 10 3 K) molecular gas phase, traced by ro-vibrational transitions of H 2 , and (2), the warm ionized medium, traced by the [Fe ii] 1.644 µm line. The [Fe ii] emission traces shocked gas ejected from the disc plane by a jet-blown bubble 300 − 400 pc in diameter, whilst the H 2 emission traces shock-excited molecular gas in the interior ∼ 1 kpc of the circumnuclear disc. Hydrodynamical modelling shows that the apparent discrepancy between the extent of the shocked gas and the radio emission can occur when the brightest regions of the synchrotron-emitting plasma are temporarily halted by dense clumps, whilst less bright plasma can percolate through the porous ISM and form an energy-driven bubble that expands freely out of the disc plane. This bubble is filled with low surface-brightness plasma not visible in existing VLBI observations of 4C 31.04 due to insufficient sensitivity. Additional radial flows of jet plasma may percolate to ∼ kpc radii in the circumnuclear disc, driving shocks and accelerating clouds of gas, giving rise to the H 2 emission.},
archivePrefix = {arXiv},
arxivId = {1811.08971v1},
author = {Zovaro, Henry R M and Sharp, Robert and Nesvadba, Nicole P H and Bicknell, Geoffrey V and Mukherjee, Dipanjan and Wagner, Alexander Y and Groves, Brent and Krishna, Shreyam},
eprint = {1811.08971v1},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Zovaro et al. - 2018 - Jets blowing bubbles in the young radio galaxy 4C 31.04.pdf:pdf},
journal = {Mnras},
keywords = {04,4c 31,active,galaxies,individual,ism,jets,jets and outflows,kinematics and dynamics,nuclei},
number = {November},
pages = {1--18},
title = {{Jets blowing bubbles in the young radio galaxy 4C 31.04}},
volume = {000},
year = {2018}
}
@article{Tadhunter2021,
abstract = {Emission-line variability studies have the potential to provide key information about the structures of the near-nuclear outflow regions of AGN. Here we present a VLT/Xshooter spectrum of the nucleus of the ULIRG F01004-2237 that was taken in August 2018, about 8 yr after a major flare in its integrated optical emission. Compared with our WHT/ISIS spectrum from September 2015, the broad, red wings of the emission lines most closely associated with the flaring event, including HeII(4686), NIII(4100,4640) and HeI(5876), have substantially declined in flux. In contrast, the broad, blue wings that dominate the [OIII], [NeIII], [NeV] and [OI] forbidden lines have increased in flux by a factor 1.4 - 4.4 (depending on the line). Moreover, the [FeVII](6087) line is detected in the new spectrum for the first time. We interpret these results in terms of a light echo from the outflowing warm gas: the direct emission from the flaring event is continuing to fade, but due to light travel time effects we are only now observing the impact of the flare on the emission from the extended outflow region. Unless the outflow is confined to a small range of angles close to our line of sight, these observations imply that the outflow must be relatively compact (r{\textless}50 pc). In terms of the nature of the flare event, we speculate that the properties of the F01004-2237 flare may be the result of a tidal disruption event (TDE) occurring in an object with pre-existing AGN activity.},
archivePrefix = {arXiv},
arxivId = {2104.08317},
author = {Tadhunter, C. and Patel, M. and Mullaney, J.},
eprint = {2104.08317},
file = {:home/william/Documents/Papers/2104.08317.pdf:pdf},
keywords = {active,evolution,galaxies,starburst},
number = {April},
pages = {1--12},
title = {{A light echo from the warm outflow in the ULIRG F01004-2237 following a major flare in its optical continuum emission}},
url = {http://arxiv.org/abs/2104.08317},
volume = {12},
year = {2021}
}
@article{Munoz2022,
abstract = {Outflows play a major role in the evolution of galaxies. However, we do not have yet a complete picture of their properties (extension, geometry, orientation and clumpiness). For low-luminosity Active Galactic Nuclei (AGNs), in particular, low-ionisation nuclear emission line regions (LINERs), the rate of outflows and their properties are largely unknown. The main goal of this work is to create the largest, up-to-date atlas of ionised gas outflow candidates in a sample of 70 nearby LINERs. We use narrow-band, imaging data to analyse the morphological properties of the ionised gas nuclear emission of these galaxies and to identify signatures of extended emission with distinctive outflow-like morphologies. We obtained new imaging data from ALFOSC/NOT for 32 LINERs. We complemented it with HST archival data for 6 objects and with results from the literature for other 32 targets. We additionally obtained soft X-ray data from Chandra archive to compare with the ionised gas. The distribution of the ionised gas in these LINER shows that {\$}\backslashsim{\$}32{\%} have bubble-like emission, {\$}\backslashsim{\$}28{\%} show a 'Core-halo', unresolved emission, and {\$}\backslashsim{\$}21{\%} have a disky-like distribution. Dust lanes prevent a detailed classification for {\$}\backslashsim{\$}11{\%} of the sample ('Dusty'). If we account for the kinematical information, available for 60 galaxies, we end up with 48{\%} of the LINERs with detected outflows/inflows (50{\%} considering only kinematical information based on Integral Field Spectroscopy). Our results suggest that the incidence of outflows in LINERs may vary from 41{\%} up to 56{\%}, based on both the Halpha morphology and the kinematical information from the literature. The ionised gas is co-spatial with the soft X-ray emission for the majority of cases ({\$}\backslashsim{\$}60{\%}), so that they may have a common origin. We discuss the use of Halpha imaging for the pre-selection of candidates likely hosting ionised gas outflows.},
archivePrefix = {arXiv},
arxivId = {2201.05080},
author = {Mu{\~{n}}oz, Laura Hermosa and M{\'{a}}rquez, Isabel and Cazzoli, Sara and Masegosa, Josefa and Ag{\'{i}}s-Gonz{\'{a}}lez, Beatriz},
eprint = {2201.05080},
file = {:home/william/Documents/Papers/2201.05080.pdf:pdf},
keywords = {active,galaxies,kinematics and dynamics,nuclei,statistics,structure},
title = {{A search for ionised gas outflows in an Halpha imaging atlas of nearby LINERs}},
url = {http://arxiv.org/abs/2201.05080},
year = {2022}
}
@article{Mou2015a,
abstract = {In a previous work, we have shown that the formation of the Fermi bubbles can be due to the interaction between winds launched from the hot accretion flow in Sgr A* and the interstellar medium (ISM). In that work, we focus only on the morphology. In this paper we continue our study by calculating the gamma-ray radiation. Some cosmic ray protons (CRp) and electrons must be contained in the winds, which are likely formed by physical processes such as magnetic reconnection. We have performed MHD simulations to study the spatial distribution of CRp, considering the advection and diffusion of CRp in the presence of magnetic field. We find that a permeated zone is formed just outside of the contact discontinuity between winds and ISM, where the collisions between CRp and thermal nuclei mainly occur. The decay of neutral pions generated in the collisions, combined with the inverse Compton scattering of background soft photons by the secondary leptons generated in the collisions and primary CR electrons can well explain the observed gamma-ray spectral energy distribution. Other features such as the uniform surface brightness along the latitude and the boundary width of the bubbles are also explained. The advantage of this accretion wind model is that the adopted wind properties come from the detailed small scale MHD numerical simulation of accretion flows and the value of mass accretion rate has independent observational evidences. The success of the model suggests that we may seriously consider the possibility that cavities and bubbles observed in other contexts such as galaxy clusters may be formed by winds rather than jets.},
author = {Mou, Guobin and Yuan, Feng and Gan, Zhaoming and Sun, Mouyuan},
doi = {10.1088/0004-637X/811/1/37},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Mou et al. - 2015 - THE ACCRETION WIND MODEL of FERMI BUBBLES. II. RADIATION.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {Galaxy: nucleus,accretion accretion disks,black hole physics,galaxies: active,galaxies: jets},
number = {1},
pages = {37},
publisher = {IOP Publishing},
title = {{THE ACCRETION WIND MODEL of FERMI BUBBLES. II. RADIATION}},
url = {http://dx.doi.org/10.1088/0004-637X/811/1/37},
volume = {811},
year = {2015}
}
@article{Yang2018,
abstract = {Observations show that winds can be driven from the inner most region (inside 50 schwarschild radius) of a thin disk. It is interesting to study the winds launched from the inner most region. A hot corona above the black hole (BH) thin disk is irradiated by the disk. We perform two dimensional hydrodynamical simulations to study the winds driven by radiation force from the corona in the inner most regions. The hard X-ray spectrum from active galactic nuclei (AGNs) suggests that the corona temperature is about {\$}10{\^{}}9{\$} K, so that we mainly analyze the properties of winds (or outflows) from the {\$}10{\^{}}9{\$} K corona. The disk luminosity plays an important role in driving the outflows. The more luminous the disk, the stronger the outflows. Mass outflow rate ({\$}\backslashdot{\{}M{\}}{\_}{\{}\backslashrm out{\}}{\$}) at 90 schwarschild radius depends on disk luminosity, which can be described as {\$}\backslashdot{\{}M{\}}{\_}{\{}\backslashrm out{\}}\backslashpropto 10{\^{}}{\{}3.3 \backslashGamma{\}}{\$} ({\$}\backslashGamma{\$} is the ratio of the disk luminosity to the Eddington luminosity). In the case of high luminosity (e.g. {\$}\backslashGamma=0.75{\$}), the supersonic outflows with maximum speed {\$}1.0 \backslashtimes 10{\^{}}4{\$} Km s{\$}{\^{}}{\{}-1{\}}{\$} are launched at {\$}\backslashsim17{\^{}}{\{}o{\}}{\$} --{\$}30{\^{}}{\{}o{\}}{\$} and {\$}\backslashsim50{\^{}}{\{}o{\}}{\$} --{\$}80{\^{}}{\{}o{\}}{\$} away from the pole axis. The Bernoulli parameter keeps increasing with the outward propagation of outflows. The radiation force keeps accelerating the outflows when outflows move outward. Therefore, we can expect the outflows can escape from the BH gravity and go to galactic scale. The interaction between outflows and interstellar medium may be an important AGNs feedback process.},
archivePrefix = {arXiv},
arxivId = {1809.09778},
author = {Yang, Xiao-Hong and Bu, De-Fu and Li, Qi-Xiu},
eprint = {1809.09778},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Yang, Bu, Li - 2018 - Numerical simulations of winds driven by radiation force from the corona above a thin disk.pdf:pdf},
number = {2012},
title = {{Numerical simulations of winds driven by radiation force from the corona above a thin disk}},
url = {http://arxiv.org/abs/1809.09778},
year = {2018}
}
@article{Zubovas2016,
abstract = {Observations of massive outflows with detectable central active galactic nuclei (AGN) typically find them within radii ≲10 kpc. We show that this apparent size restriction is a natural result of AGN driving if this process injects total energy only of the order of the gas binding energy to the outflow, and the AGN varies over time ('flickers') as suggested in recent work. After the end of all AGN activity, the outflow continues to expand to larger radii, powered by the thermal expansion of the remnant-shocked AGN wind. We suggest that on average, outflows should be detected further from the nucleus in more massive galaxies. In massive gas-rich galaxies, these could be several tens of kpc in radius. We also consider the effect that pressure of such outflows has on a galaxy disc. In moderately gas-rich discs, with gas-to-baryon fraction {\textless}0.2, the outflow may induce star formation significant enough to be distinguished from quiescent by an apparently different normalization of the Kennicutt-Schmidt law. The star formation enhancement is probably stronger in the outskirts of galaxy discs, so coasting outflows might be detected by their effects upon the disc even after the driving AGN has shut off. We compare our results to the recent inference of inside-out quenching of star formation in galaxy discs.},
archivePrefix = {arXiv},
arxivId = {1607.07258},
author = {Zubovas, Kastytis and King, Andrew},
doi = {10.1093/mnras/stw1845},
eprint = {1607.07258},
file = {:home/william/Documents/Papers/stw1845.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Accretion,Accretion discs,Galaxies: evolution,ISM: evolution,Quasars: general,Stars: formation},
number = {4},
pages = {4055--4066},
title = {{The small observed scale of AGN-driven outflows, and inside-out disc quenching}},
volume = {462},
year = {2016}
}
@article{DeGouveiaDalPino2020,
abstract = {Large-scale, broad outflows are common in active galaxies. In systems where star formation coexists with an AGN, it is unclear yet the role that both play on driving the outflows. In this work we present three-dimensional radiative-cooling MHD simulations of the formation of these outflows, considering the feedback from both the AGN and supernovae-driven winds. We find that a large-opening-angle AGN wind develops fountain structures that make the expanding gas to fallback. Furthermore, it exhausts the gas near the nuclear region, extinguishing star formation and accretion within a few 100.000 yr, which establishes the duty cycle of these outflows. The AGN wind accounts for the highest speed features in the outflow with velocities around 10.000 km s-1 (as observed in UFOs), but these are not as cold and dense as required by observations of molecular outflows. The SNe-driven wind is the main responsible for the observed mass-loading of the outflows.},
archivePrefix = {arXiv},
arxivId = {1809.07588},
author = {{De Gouveia Dal Pino}, Elisabete M. and Clavijo-Boh{\'{o}}rquez, William and Melioli, Claudio},
doi = {10.1017/S174392131800604X},
eprint = {1809.07588},
file = {:home/william/Documents/Papers/1809.07588.pdf:pdf},
isbn = {0000000000000},
issn = {17439221},
journal = {Proc. Int. Astron. Union},
keywords = {Galaxy: active,Star Formation,Supernova},
number = {342},
pages = {229--233},
title = {{AGN and Star Formation Feedback in Galaxy Outflows}},
volume = {2},
year = {2020}
}
@article{Gabuzda2017a,
abstract = {This paper reviews observational evidence obtained to date about the overall structure of the magnetic fields in the jets of Active Galactic Nuclei (AGN). Because they are sensitive to the line-of-sight magnetic-field component, Faraday rotation observations of AGN jets provide an effective tool for searching for toroidal jet magnetic fields, whose line-of-sight component changes systematically across the jet. Transverse Faraday rotation measure (RM) gradients providing direct evidence for helical/toroidal magnetic fields have been reliably detected in nearly 40 AGN on parsec scales. Helical magnetic fields are believed to form due to the combined action of the rotation of the central black hole and accretion disk, and these observations demonstrate that at least some of this helical field survives to distances well beyond the Very Long Baseline Interferometry (VLBI) core. Observations of reversals in the direction of the transverse RM gradients in a number of AGN provide evidence for a "return" magnetic field forming a nested helical-field structure with oppositely directed azimuthal components in the inner and outer regions of the helical magnetic field. The collected data now provide firm evidence for a predominance of inward jet currents on parsec scales and outward currents on scales greater than a few tens of parsecs. This suggests a global pattern of magnetic fields and currents with an inward current near the jet axis and an outward current farther from the jet axis, with these currents closing in the accretion disk and far out in the radio lobes, forming a self-consistent set of fields and currents together with the implied nested helical-field structure.},
author = {Gabuzda, Denise},
doi = {10.3390/galaxies5010011},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Gabuzda - 2017 - The Origin and Structure of the Magnetic Fields and Currents of AGN Jets.pdf:pdf},
issn = {20754434},
journal = {Galaxies},
keywords = {Active galactic nuclei,Magnetic fields,Radio interferometry,Relativistic jets},
number = {1},
title = {{The origin and structure of the magnetic fields and currents of AGN jets}},
volume = {5},
year = {2017}
}
@article{Margalit2021,
abstract = {Pauli blocking of spontaneous emission is responsible for the stability of atoms. Higher electronic orbitals cannot decay to lower-lying states if they are already occupied -- this is Pauli blocking due to occupation of internal states. Pauli blocking also occurs when free atoms scatter light elastically (Rayleigh scattering) and the final external momentum states are already occupied. A suppression of the total rate of light scattering requires a quantum-degenerate Fermi gas with a Fermi energy larger than the photon recoil energy. This has been predicted more than 30 years ago, but never realized. Here we report the creation of a dense Fermi gas of ultracold lithium atoms and show that at low temperatures light scattering is suppressed. We also explore the suppression of inelastic light scattering when two colliding atoms emit light shifted in frequency.},
archivePrefix = {arXiv},
arxivId = {2103.06921},
author = {Margalit, Yair and Lu, Yu-Kun and Top, Furkan Cagri and Ketterle, Wolfgang},
doi = {10.1126/science.abi6153},
eprint = {2103.06921},
file = {:home/william/Documents/Papers/2103.06921.pdf:pdf},
issn = {0036-8075},
title = {{Pauli blocking of light scattering in degenerate fermions}},
url = {http://arxiv.org/abs/2103.06921},
year = {2021}
}
@article{Batcheldor2007,
abstract = {In order to identify the dominant nuclear outflow mechanisms in active galactic nuclei, we have undertaken deep, high-resolution observations of two compact radio sources (PKS 1549-79 and PKS 1345+12) with the Advanced Camera for Surveys (ACS) aboard the Hubble Space Telescope. Not only are these targets known to have powerful emission-line outflows, but they also contain all the potential drivers for the outflows: relativistic jets, quasar nuclei, and starbursts. ACS allows the compact nature ({\textless}0.15") of these radio sources to be optically resolved for the first time. Through comparison with existing radio maps, we have seen consistency in the nuclear position angles of both the optical emission-line and radio data. There is no evidence for biconical emission-line features on the large scale, and there is a divergence in the relative position angles of the optical and radio structure. This enables us to exclude starburst-driven outflows. However, we are unable to clearly distinguish between radiative AGN wind-driven outflows and outflows powered by relativistic radio jets. The small-scale biconical features, indicative of such mechanisms, could be below the resolution limit of ACS, especially if aligned close to the line of sight. In addition, there may be offsets between the radio and optical nuclei induced by heavy dust obscuration, nebular continuum, or scattered light from the AGN. Based on observations made with the NASA/ESA Hubble Space Telescope obtained at the Space Telescope Science Institute, which is operated by the Association of Universities for Research in Astronomy, Inc. under NASA contract NAS 5-26555. These observations are associated with program 10206.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0702498},
author = {Batcheldor, Dan and Tadhunter, Clive and Holt, Joanna and Morganti, Raffaella and O'Dea, Christopher P. and Axon, David J. and Koekemoer, Anton},
doi = {10.1086/515391},
eprint = {0702498},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Batcheldor et al. - 2007 - Dominant Nuclear Outflow Driving Mechanisms in Powerful Radio Galaxies.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
number = {1},
pages = {70--77},
primaryClass = {astro-ph},
title = {{Dominant Nuclear Outflow Driving Mechanisms in Powerful Radio Galaxies}},
url = {http://stacks.iop.org/0004-637X/661/i=1/a=70},
volume = {661},
year = {2007}
}
@article{Wang2020,
abstract = {It arises a puzzle in $\backslash$NGC$\backslash$, how to secularly maintain the counter-rotating disc from {\$}0.2{\$} to {\$}7\backslash,{\$}pc unambiguously detected by recent ALMA observations of molecular gas. Upon further analysis of disc dynamics, we find that the Kelvin-Helmholtz (KH) instability (KHI) results in an unavoidable catastrophe of the disc developed at the interface between the reversely rotating parts, and demonstrate that a close binary of supermassive black holes provides tidal torques as the unique external sources to prevent the disc from the KH catastrophe. We are led to the inescapable conclusion that there must be a binary black hole at the center of NGC 1068, to prevent it from the KH catastrophe. The binary is composed of black holes with a separation of {\$}0.1\backslash,{\$}pc from GRAVITY/VLTI observations, a total mass of {\$}1.3\backslashtimes 10{\^{}}{\{}7{\}}\backslash:M{\_}{\{}\backslashodot{\}}{\$} and a mass ratio of {\$}\backslashsim 0.3{\$} estimated from the angular momentum budge of the global system. The KHI gives rise to forming a gap without cold gas at the velocity interface which overlaps with the observed gap of hot and cold dust regions. Releases of kinematic energies from the KHI of the disc are in agreement with observed emissions in radio and {\$}\backslashgamma{\$}-rays. Such a binary is shrinking with a timescale much longer than the local Hubble time via gravitational waves, however, the KHI leads to an efficient annihilation of the orbital angular momentum and speed up merge of the binary, providing a new paradigm of solving the long term issue of "final parsec problem". Future observations of GRAVITY+/VLTI are expected to be able to spatially resolve the CB-SMBHs suggested in this paper.},
archivePrefix = {arXiv},
arxivId = {2005.01220},
author = {Wang, J. -M. and Songsheng, Y. -Y. and Li, Y. -R. and Du, P. and Zhe, Y.},
eprint = {2005.01220},
file = {:home/william/Documents/Papers/[Wang et al.]-Dynamical evidence of the sub-parsec counter-rotating disc for a.pdf:pdf},
keywords = {accretion,accretion discs,active,binary,black holes,galaxies},
number = {May},
title = {{Dynamical evidence of the sub-parsec counter-rotating disc for a close binary of supermassive black holes in the nucleus of NGC 1068}},
url = {http://arxiv.org/abs/2005.01220},
year = {2020}
}
@article{Mukherjee2016,
abstract = {We present the results of three dimensional relativistic hydrodynamic simulations of interaction of AGN jets with a dense turbulent two-phase interstellar medium, which would be typical of high redshift galaxies. We describe the effect of the jet on the evolution of the density of the turbulent ISM. The jet driven energy bubble affects the gas to distances up to several kiloparsecs from the injection region. The shocks resulting from such interactions create a multi-phase ISM and radial outflows. One of the striking result of this work is that low power jets (P{\_}jet {\textless} 10{\^{}}{\{}43{\}} erg/s) although less efficient in accelerating clouds, are trapped in the ISM for a longer time and hence affect the ISM over a larger volume. Jets of higher power drill through with relative ease. Although the relativistic jets launch strong outflows, there is little net mass ejection to very large distances, supporting a galactic fountain scenario for local feedback.},
archivePrefix = {arXiv},
arxivId = {1606.01143},
author = {Mukherjee, Dipanjan and Bicknell, Geoffrey V. and Sutherland, Ralph and Wagner, Alex},
doi = {10.1093/mnras/stw1368},
eprint = {1606.01143},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Mukherjee et al. - 2016 - Relativistic jet feedback in high-redshift galaxies - I. Dynamics.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: ISM,Galaxies: evolution,Galaxies: highredshift,Galaxies: jets,Hydrodynamics,Methods: numerical},
number = {1},
pages = {967--983},
title = {{Relativistic jet feedback in high-redshift galaxies - I. Dynamics}},
volume = {461},
year = {2016}
}
@article{Riffel2011a,
abstract = {We have mapped the stellar and gaseous kinematics, as well as the emission-line flux distributions and ratios, from the inner ≈450pc radius of the Seyfert 2 galaxy Mrk1157, using two-dimensional near-infrared J- and K l-band spectra obtained with the Gemini Near-Infrared Integral-Field Spectrograph instrument at a spatial resolution of ≈35pc and velocity resolution of ≈40kms -1. The stellar velocity field shows a rotation pattern, with a discrete S-shaped zero velocity curve - a signature of a nuclear bar. The presence of a bar is also supported by the residual map between the observed rotation field and a model of circular orbits in a Plummer potential. The stellar velocity dispersion ($\sigma$ *) map presents a partial ring of low-$\sigma$ * values (50-60kms -1) at 250pc from the nucleus surrounded by higher $\sigma$ * values from the galaxy bulge. We propose that this ring has origin in kinematically colder regions with recent star formation. The stellar velocity dispersion of the bulge (100kms -1) implies in a black hole mass of M BH= 8.3 +3.2- 2.2× 10 6M ⊙. Emission-line flux distributions are most extended along the position angle PA = 27°/153°, reaching at least 450pc from the nucleus and following the orientation observed in previous optical emission-line [Oiii] imaging and radio jets. The molecular hydrogen gas has an excitation temperature T exc≈ 2300K and its emission is dominated by thermal processes, mainly due to X-ray heating by the active nucleus, with a possible small contribution from shocks produced by the radio jet. The [Feii] excitation has a larger contribution from shocks produced by the radio jet, as evidenced by the line-ratio maps and velocity dispersion maps, which show spatial correlation with the radio structures. The coronal lines are resolved, extending up to ≈150pc and are also slightly more extended along PA = 27°/153°. The gaseous kinematics show two components: one due to the gas located in the galaxy plane, in similar rotation to that of the stars, and another in outflow, which is oriented close to the plane of the sky, thus extending to high latitudes, as the galaxy plane is inclined by ≈45° relative to the plane of the sky. The gas rotating in the plane dominates the H 2 and Pa$\beta$ emission, while the gas in outflow is observed predominantly in [Feii] emission. The [Feii] emission is originated in gas being pushed by the radio jet, which destroys dust grains, releasing Fe. From the outflow velocities and implied geometry, we estimate a mass-outflow rate of for the ionized gas and a kinetic power for the outflow of. The distinct flux distributions and kinematics of the H 2- and [Feii]-emitting gas, with the former more restricted to the plane of the galaxy and the latter tracing the outflows related to radio jets, are a common characteristic of six Seyfert galaxies (ESO428-G14, NGC4051, 7582 and4151, Mrk1066, and now Mrk1157) we have studied so far using similar two-dimensional observations and other two (Circinus and NGC2110) using long-slit observations. We conclude that the H 2 emission surrounding the nucleus in the galaxy plane is a tracer of the gas feeding to the active nucleus, while the [Feii] emission is a tracer of its feedback. {\textcopyright} 2011 The Authors Monthly Notices of the Royal Astronomical Society {\textcopyright} 2011 RAS.},
archivePrefix = {arXiv},
arxivId = {1107.2564},
author = {Riffel, Rogemar A. and Storchi-Bergmann, Thaisa},
doi = {10.1111/j.1365-2966.2011.19441.x},
eprint = {1107.2564},
file = {:home/william/Documents/Papers/mnras0417-2752.pdf:pdf},
issn = {00358711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: ISM,Galaxies: Seyfert,Galaxies: individual: Mrk1157,Galaxies: individual: NGC591,Galaxies: kinematics and dynamics,Infrared: galaxies},
number = {4},
pages = {2752--2769},
title = {{Feeding and feedback in the active nucleus of Mrk 1157 probed with the Gemini Near-Infrared Integral-Field Spectrograph}},
volume = {417},
year = {2011}
}
@article{Gabuzda,
abstract = {Long-lived, stable jets are observed in a wide variety of systems, from protostars, through Galactic compact objects to active galactic nuclei (AGN). Magnetic fields play a central role in launching, accelerating, and collimating the jets through various media. The termination of jets in molecular clouds or the interstellar medium deposits enormous amounts of mechanical energy and momentum, and their interactions with the external medium, as well, in many cases, as the radiation processes by which they are observed, are intimately connected with the magnetic fields they carry. This review focuses on the properties and structures of magnetic fields in long-lived jets, from their launch from rotating magnetized young stars, black holes, and their accretion discs, to termination and beyond. We compare the results of theory, numerical simulations, and observations of these diverse systems and address similarities and differences between relativistic and non-relativistic jets in protostellar versus AGN systems. On the observational side, we focus primarily on jets driven by AGN because of the strong observational constraints on their magnetic field properties, and we discuss the links between the physics of these jets on all scales. {\textcopyright} 2012 Springer Science+Business Media B.V.},
archivePrefix = {arXiv},
arxivId = {1205.2073},
author = {Pudritz, Ralph E. and Hardcastle, Martin J. and Gabuzda, Denise C},
doi = {10.1007/s11214-012-9895-z},
eprint = {1205.2073},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Gabuzda, May - Unknown - Magnetic Fields in Astrophysical Jets From Launch to Termination.pdf:pdf},
issn = {00386308},
journal = {Space Sci. Rev.},
keywords = {Jets,Magnetic fields,Polarization,Radio continuum: galaxies,X-rays: galaxies},
number = {1-4},
pages = {27--72},
title = {{Magnetic fields in astrophysical jets: From launch to termination}},
volume = {169},
year = {2012}
}
@article{2010A&A...521A..57T,
archivePrefix = {arXiv},
arxivId = {astro-ph.HE/1006.2858},
author = {Tombesi, F and Cappi, M and Reeves, J.{\~{}}N. and Palumbo, G.{\~{}}G.{\~{}}C. and Yaqoob, T and Braito, V and Dadina, M},
doi = {10.1051/0004-6361/200913440},
eprint = {1006.2858},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Tombesi et al. - 2010 - Evidence for ultra-fast outflows in radio-quiet AGNs I . Detection and statistical incidence of Fe K-shell absor.pdf:pdf},
journal = {aap},
keywords = {X-ray: galaxies,black hole physics,galaxies: Seyfert,line: identification},
pages = {A57},
primaryClass = {astro-ph.HE},
title = {{Evidence for ultra-fast outflows in radio-quiet AGNs. I. Detection and statistical incidence of Fe K-shell absorption lines}},
volume = {521},
year = {2010}
}

@ARTICLE{Netzer2015,
       author = {{Netzer}, Hagai},
        title = "{Revisiting the Unified Model of Active Galactic Nuclei}",
      journal = {\araa},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = aug,
       volume = {53},
        pages = {365-408},
          doi = {10.1146/annurev-astro-082214-122302},
archivePrefix = {arXiv},
       eprint = {1505.00811},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ARA&A..53..365N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Gnat2007,
abstract = {We present new computations of the equilibrium and non-equilibrium cooling efficiencies and ionization states for low-density radiatively cooling gas containing cosmic abundances of the elements H, He, C, N, O, Ne, Mg, Si, S, and Fe. We present results for gas temperatures between 1e4 and 1e8 K, assuming dust-free and optically thin conditions, and no external radiation. For non-equilibrium cooling we solve the coupled time-dependent ionization and energy loss equations for a radiating gas cooling from an initially hot, {\textgreater}5e6K equilibrium state, down to 1e4K. We present results for heavy element compositions ranging from 1e-3 to 2 times the elemental abundances in the Sun. We consider gas cooling at constant density (isochoric) and at constant pressure (isobaric). We calculate the critical column densities and temperatures at which radiatively cooling clouds make the dynamical transition from isobaric to isochoric evolution. We construct ion ratio diagnostics for the temperature and metallicity in radiatively cooling gas. We provide numerical estimates for the maximal cloud column densities for which the gas remains optically thin to the cooling radiation. We present our computational results in convenient on-line figures and tables (see http://wise-obs.tau.ac.il/{\~{}}orlyg/cooling/).},
archivePrefix = {arXiv},
arxivId = {astro-ph/0608181},
author = {Gnat, Orly and Sternberg, Amiel},
doi = {10.1086/509786},
eprint = {0608181},
file = {:home/william/Documents/Papers/Gnat{\_}2007{\_}ApJS{\_}168{\_}213.pdf:pdf},
issn = {0067-0049},
journal = {Astrophys. J. Suppl. Ser.},
number = {2},
pages = {213--230},
primaryClass = {astro-ph},
title = {{Time‐dependent Ionization in Radiatively Cooling Gas}},
volume = {168},
year = {2007}
}
@article{Leighly2016,
abstract = {Mrk 231 is a nearby quasar with an unusually red near-UV-to-optical continuum, generally explained as heavy reddening by dust (e.g., Leighly et al. 2014). Yan et al. 2015 proposed that Mrk{\~{}}231 is a milli-parsec black-hole binary with little intrinsic reddening. We show that if the observed FUV continuum is intrinsic, as assumed by Yan et al. 2015, it fails by a factor of about 100 in powering the observed strength of the near-infrared emission lines, and the thermal near and mid-infrared continuum. In contrast, the line and continuum strengths are typical for a reddened AGN spectral energy distribution. We find that the HeI*/Pbeta ratio is sensitive to the spectral energy distribution for a one-zone model. If this sensitivity is maintained in general broad-line region models, then this ratio may prove a useful diagnostic for heavily reddened quasars. Analysis of archival HST STIS and FOC data revealed evidence that the far-UV continuum emission is resolved on size scales of {\~{}}40 parsecs. The lack of broad absorption lines in the far-UV continuum might be explained if it were not coincident with the central engine. One possibility is that it is the central engine continuum reflected from the receding wind on the far side of the quasar.},
archivePrefix = {arXiv},
arxivId = {1604.03456},
author = {Leighly, Karen M. and Terndrup, Donald M. and Gallagher, Sarah C. and Lucy, Adrian B.},
doi = {10.3847/0004-637x/829/1/4},
eprint = {1604.03456},
file = {:home/william/Documents/Papers/Leighly{\_}2016{\_}ApJ{\_}829{\_}4.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
keywords = {accretion,accretion disks,accretion, accretion disks,emission lines,individual,mrk 231,quasars,quasars: emission lines,quasars: individual (Mrk 231),quasars: supermassive black holes,supermassive black holes},
number = {1},
pages = {4},
publisher = {IOP Publishing},
title = {{the Binary Black Hole Model for Mrk 231 Bites the Dust}},
url = {http://dx.doi.org/10.3847/0004-637X/829/1/4},
volume = {829},
year = {2016}
}
@article{Sturm2011,
abstract = {Mass outflows driven by stars and active galactic nuclei (AGNs) are a key element in many current models of galaxy evolution. They may produce the observed black-hole-galaxy mass relation and regulate and quench both star formation in the host galaxy and black hole accretion. However, observational evidence of such feedback processes through outflows of the bulk of the star-forming molecular gas is still scarce. Here we report the detection of massive molecular outflows, traced by the hydroxyl molecule (OH), in far-infrared spectra of ULIRGs obtained with Herschel-PACS as part of the SHINING key project. In some of these objects the (terminal) outflow velocities exceed 1000kms-1, and their outflow rates (up to 1200 M yr -1) are several times larger than their star formation rates. We compare the outflow signatures in different types of ULIRGs and in starburst galaxies to address the issue of the energy source (AGN or starburst) of these outflows. We report preliminary evidence that ULIRGs with a higher AGN luminosity (and higher AGN contribution to L IR) have higher terminal velocities and shorter gas depletion timescales. The outflows in the observed ULIRGs are able to expel the cold gas reservoirs from the centers of these objects within 106-108 years. {\textcopyright} 2011. The American Astronomical Society. All rights reserved.},
archivePrefix = {arXiv},
arxivId = {1105.1731},
author = {Sturm, E. and Gonzlez-Alfonso, E. and Veilleux, S. and Fischer, J. and Graci-Carpio, J. and Hailey-Dunsheath, S. and Contursi, A. and Poglitsch, A. and Sternberg, A. and Davies, R. and Genzel, R. and Lutz, D. and Tacconi, L. and Verma, A. and Maiolino, R. and {De Jong}, J. A.},
doi = {10.1088/2041-8205/733/1/L16},
eprint = {1105.1731},
file = {:home/william/Documents/Papers/1105.1731.pdf:pdf},
issn = {20418205},
journal = {Astrophys. J. Lett.},
keywords = {Galaxies: active,ISM: jets and outflows,galaxies: evolution,galaxies: starburst},
number = {1 PART 2},
pages = {1--14},
title = {{Massive molecular outflows and negative feedback in ULIRGs observed by herschel-pacs}},
volume = {733},
year = {2011}
}
@article{VanDenBosch2015,
abstract = {We have conducted an optical long-slit spectroscopic survey of 1022 galaxies using the 10m Hobby-Eberly Telescope (HET) at McDonald Observatory. The main goal of the HET Massive Galaxy Survey (HETMGS) is to find nearby galaxies that are suitable for black hole mass measurements. In order to measure accurately the black hole mass, one should kinematically resolve the region where the black hole dominates the gravitational potential. For most galaxies, this region is much less than an arcsecond. Thus, black hole masses are best measured in nearby galaxies with telescopes that obtain high-spatial resolution. The HETMGS focuses on those galaxies predicted to have the largest sphere-of-influence, based on published stellar velocity dispersions or the galaxy fundamental plane. To ensure coverage over galaxy types, the survey targets those galaxies across a face-on projection of the fundamental plane. We present the sample selection and resulting data products from the long-slit observations, including central stellar kinematics and emission line ratios. The full dataset, including spectra and resolved kinematics, is available online. Additionally, we show that the current crop of black hole masses are highly biased towards dense galaxies and that especially large disks and low dispersion galaxies are under-represented. This survey provides the necessary groundwork for future systematic black hole mass measurement campaigns.},
author = {{Van Den Bosch}, Remco C.E. and Gebhardt, Karl and G{\"{u}}ltekin, Kayhan and Yildirim, Akin and Walsh, Jonelle L.},
doi = {10.1088/0067-0049/218/1/10},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/van den Bosch et al. - 2015 - Hunting for Supermassive Black Holes in Nearby Galaxies With the Hobby-Eberly Telescope.pdf:pdf},
issn = {00670049},
journal = {Astrophys. Journal, Suppl. Ser.},
keywords = {catalogs,galaxies: elliptical and lenticular, cD,galaxies: spiral,galaxies: structure,quasars: supermassive black holes,surveys},
number = {1},
title = {{Hunting for Supermassive Black Holes in Nearby Galaxies With the Hobby-Eberly Telescope}},
volume = {218},
year = {2015}
}
@article{Chung2009,
abstract = {We present 12CO J=1--{\textgreater}0 observations of ultraluminous infrared galaxies (ULIRGs) obtained using the Redshift Search Receiver (RSR) on the 14-m telescope of the Five College Radio Astronomy Observatory. The RSR is a novel, dual-beam, dual-polarization receiver equipped with an ultra-wideband spectrometer backend that is being built as a facility receiver for the Large Millimeter Telescope. Our sample consists of 29 ULIRGs in the redshift range of 0.04-0.11, including 10 objects with no prior 12CO measurements. We have detected 27 systems (a detection rate of 93{\%}), including 9 ULIRGs that are detected in CO for the first time. Our study has increased the number of local ULIRGs with CO measurements by {\~{}}15{\%}. The CO line luminosity L'{\_}CO, correlates well with far-infrared luminosity L{\_}FIR, following the general trend of other local ULIRGs. However, compared to previous surveys we probe deeper into the low CO luminosity end of ULIRG population as a single study by including a number of CO faint objects in the sample. As a result, we find 1) a smoother transition between the ULIRG population and local QSOs in L{\_}FIR-L'{\_}CO ("star formation efficiency") space, and 2) a broader range of L{\_}FIR/L'{\_}CO flux ratio ({\~{}}60--1000 L{\_}sun/[K km/s/pc{\^{}}2]) than previously reported. In our new survey, we also have found a small number of ULIRGs with extreme L{\_}FIR/L'{\_}CO which had been known to be rare. The mid-IR color and radio-excess of 56 local ULIRGs as a function of FIR-to-CO flux ratio is examined and compared with those of spirals/starburst galaxies and low-z QSOs. In this paper, using a large sample of local ULIRGs we explore the origin of their current power source and potential evolution to QSOs.},
archivePrefix = {arXiv},
arxivId = {0906.2797},
author = {Chung, Aeree and Narayanan, Gopal and Yun, Min S. and Heyer, Mark and Erickson, Neal R.},
doi = {10.1088/0004-6256/138/3/858},
eprint = {0906.2797},
file = {:home/william/Documents/Papers/0906.2797.pdf:pdf},
issn = {0004-6256},
journal = {Astron. J.},
number = {3},
pages = {858--872},
title = {{ the Redshift Search Receiver Observations of 12 Co J = 1 → 0 in 29 Ultraluminous Infrared Galaxies }},
volume = {138},
year = {2009}
}
@article{Nielsen2016,
abstract = {The {\^{a}} €standard' model of cosmology is founded on the basis that the expansion rate of the universe is accelerating at present-As was inferred originally from the Hubble diagram of Type Ia supernovae. There exists now a much bigger database of supernovae so we can perform rigorous statistical tests to check whether these {\^{a}} €standardisable candles' indeed indicate cosmic acceleration. Taking account of the empirical procedure by which corrections are made to their absolute magnitudes to allow for the varying shape of the light curve and extinction by dust, we find, rather surprisingly, that the data are still quite consistent with a constant rate of expansion.},
archivePrefix = {arXiv},
arxivId = {1506.01354},
author = {Nielsen, J T and Guffanti, A and Sarkar, S},
doi = {10.1038/srep35596},
eprint = {1506.01354},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Nielsen, Guffanti, Sarkar - 1990 - Marginal evidence for cosmic acceleration from Type Ia supernovae.pdf:pdf},
issn = {20452322},
journal = {Sci. Rep.},
pages = {1--8},
publisher = {Nature Publishing Group},
title = {{Marginal evidence for cosmic acceleration from Type Ia supernovae}},
url = {http://dx.doi.org/10.1038/srep35596},
volume = {6},
year = {2016}
}
@article{Kaaret2017,
author = {Kaaret, Philip and Feng, Hua and Roberts, Timothy P},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Kaaret, Feng, Roberts - 2017 - Ultraluminous X-Ray Sources.pdf:pdf},
keywords = {accretion physics,black holes,galaxies,neutron stars,x-ray binaries,x-rays},
pages = {303--342},
title = {{Ultraluminous X-Ray Sources}},
year = {2017}
}
@article{Kraemer2015,
abstract = {We present a detailed, photoionization modeling analysis of XMM-Newton/Reflection Grating Spectrometer observations of the Seyfert 2 galaxy NGC 1068. The spectrum, previously analyzed by Kinkhabwala et al., reveals a myriad of soft X-ray emission lines, including those from H- and He-like carbon, nitrogen, oxygen, and neon, and M- and L-shell iron. As noted in the earlier analysis, based on the narrowness of the radiative recombination continua, the electron temperatures in the emission-line gas are consistent with photoionization, rather than collisional ionization. The strengths of the carbon and nitrogen emission lines, relative to those of oxygen, suggest unusual elemental abundances, which we attribute to the star formation history of the host galaxy. Overall, the emission lines are blueshifted with respect to systemic, with radial velocities ∼160 km s-1, similar to that of [O III] $\lambda$5007, and thus consistent with the kinematics and orientation of the optical emission-line gas and, hence, likely part of an active galactic nucleus driven outflow. We were able to achieve an acceptable fit to most of the strong emission lines with a two-component photoionization model, generated with cloudy. The two components have ionization parameters and column densities of logU = -0.05 and 1.22 and logNH = 20.85 and 21.2 and covering factors of 0.35 and 0.84, respectively. The total mass of the X-ray gas is roughly an order of magnitude greater than the mass of ionized gas determined from optical and near-IR spectroscopy, which indicates that it may be the dominant component of the narrow-line region. Furthermore, we suggest that the medium that produces the scattered/polarized optical emission in NGC 1068 possesses similar physical characteristics to those of the more highly ionized of the X-ray model components.},
archivePrefix = {arXiv},
arxivId = {1410.6799},
author = {Kraemer, S. B. and Sharma, N. and Turner, T. J. and George, Ian M. and {Michael Crenshaw}, D.},
doi = {10.1088/0004-637X/798/1/53},
eprint = {1410.6799},
file = {:home/william/Documents/Papers/1410.6799.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {Galaxies: Active,Galaxies: Individual (NGC 1068),Galaxies: Seyfert,X-rays: Galaxies},
number = {1},
pages = {1--32},
title = {{Physical conditions in the x-ray emission-line gas in NGC 1068}},
volume = {798},
year = {2015}
}
@article{Morganti2018,
abstract = {This review summarises what we have learnt in the last two decades based on H i 21 cm absorption observations about the cold interstellar medium (ISM) in the central regions of active galaxies and about the interplay between this gas and the active nucleus (AGN). H i absorption is a powerful tracer on all scales, from the parsec-scales close to the central black hole to structures of many tens of kpc tracing interactions and mergers of galaxies. Given the strong radio continuum emission often associated with the central activity, H i absorption observations can be used to study the H i near an active nucleus out to much higher redshifts than is possible using H i emission. In this way, H i absorption has been used to characterise in detail the general ISM in active galaxies, to trace the fuelling of radio-loud AGN, to study the feedback occurring between the energy released by the active nucleus and the ISM, and the impact of such interactions on the evolution of galaxies and of their AGN. In the last two decades, significant progress has been made in all these areas. It is now well established that many radio loud AGN are surrounded by small, regularly rotating gas disks that contain a significant fraction of H i. The structure of these disks has been traced down to parsec scales by very long baseline interferometry observations. Some groups of objects, and in particular young and recently restarted radio galaxies, appear to have a particularly high detection rate of H i. This is interesting in connection with the evolution of these AGN and their impact on the surrounding ISM. This is further confirmed by an important discovery, made thanks to technical upgrades of radio telescopes, namely the presence of fast, AGN-driven outflows of cold gas which give a direct view of the impact of the energy released by AGN on the evolution of galaxies (AGN feedback). In addition, evidence has been collected that clouds of cold gas can play a role in fuelling the nuclear activity. This review ends by briefly describing the upcoming large, blind H i absorption surveys planned for the new radio telescopes which will soon become operational. These surveys will allow to significantly expand existing work, but will also allow to explore new topics, in particular, the evolution of the cold ISM in AGN.},
archivePrefix = {arXiv},
arxivId = {1807.01475},
author = {Morganti, Raffaella and Oosterloo, Tom},
doi = {10.1007/s00159-018-0109-x},
eprint = {1807.01475},
file = {:home/william/Documents/Papers/Morganti-Oosterloo2018{\_}Article{\_}TheInterstellarAndCIrcumnuclea.pdf:pdf},
issn = {09354956},
journal = {Astron. Astrophys. Rev.},
keywords = {Galaxies: active,ISM: jets and outflow,Radio lines: galaxies},
number = {1},
pages = {1--59},
publisher = {Springer Berlin Heidelberg},
title = {{The interstellar and circumnuclear medium of active nuclei traced by HI 21 cm absorption}},
url = {https://doi.org/10.1007/s00159-018-0109-x},
volume = {26},
year = {2018}
}
@article{Jones2019,
abstract = {We report the discovery of a high-redshift, massive molecular outflow in the starburst galaxy SPT 0346-52 (z =5.656) via the detected absorption of high-excitation water transitions (H2O 42,3-41,4 and H2O 33,0-32,1) with the Atacama Large Millimeter/submillimeter Array (ALMA). The host galaxy is one of the most powerful starburst galaxies at high redshift (star formation rate; SFR ∼3600 M year-1), with an extremely compact (∼320 pc) star formation region and a SFR surface density (SFR~5500 M year-1 kpc-2) five times higher than "maximum"(i.e. Eddington-limited) starbursts, implying a highly transient phase. The estimated outflow rate is ∼500 M year-1, which is much lower than the SFR, implying that in this extreme starburst the outflow capabilities saturate and the outflow is no longer capable of regulating star formation, resulting in a runaway process in which star formation will use up all available gas in less than 30 Myr. Finally, while previous kinematic investigations of this source revealed possible evidence for an ongoing major merger, the coincidence of the hyper-compact starburst and high-excitation water absorption indicates that this is a single starburst galaxy surrounded by a disc.},
archivePrefix = {arXiv},
arxivId = {1911.09967},
author = {Jones, G. C. and Maiolino, R. and Caselli, P. and Carniani, S.},
doi = {10.1051/0004-6361/201936989},
eprint = {1911.09967},
file = {:home/william/Documents/Papers/aa36989-19.pdf:pdf},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Galaxies: high-redshift,Galaxies: starburst,ISM: jets and outflows},
pages = {1--7},
title = {{Detection of a high-redshift molecular outflow in a primeval hyperstarburst galaxy}},
volume = {632},
year = {2019}
}
@article{2013MNRAS.430.3235M,
archivePrefix = {arXiv},
arxivId = {1301.5005},
author = {Melioli, C and {de Gouveia Dal Pino}, E.{\~{}}M. and Geraissate, F.{\~{}}G.},
doi = {10.1093/mnras/stt126},
eprint = {1301.5005},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Melioli, de Gouveia Dal Pino, Geraissate - 2013 - Evolution of M82-like starburst winds revisited 3D radiative cooling hydrodynamical si.pdf:pdf},
journal = {MNRAS},
keywords = {ISM: abundances,ISM: bubbles,ISM: jets and outflows,galaxies: ISM,galaxies: kinematics and dynamics,galaxies: starburst},
pages = {3235--3248},
title = {{Evolution of M82-like starburst winds revisited: 3D radiative cooling hydrodynamical simulations}},
volume = {430},
year = {2013}
}
@article{Chen2020a,
abstract = {Large-scale outflows are generally considered as a possible evidence that active galactic nuclei (AGNs) can severely affect their host galaxies. Recently an ultraluminous IR galaxy (ULIRG) at {\$}z=0.49{\$}, AKARI J0916248+073034, was found to have a galaxy-scale [OIII] {\$}\backslashlambda{\$}5007 outflow with one of the highest energy-ejection rates at {\$}z{\textless}1.6{\$}. However, the central AGN activity estimated from its torus mid-IR (MIR) radiation is weak relative to the luminous [OIII] emission. In this work we report the first NuSTAR hard X-ray follow-up of this ULIRG to constrain its current AGN luminosity. The intrinsic 2-10 keV luminosity shows a 90{\%} upper-limit of {\$}3.0\backslashtimes10{\^{}}{\{}43{\}}{\$} erg s{\$}{\^{}}{\{}-1{\}}{\$} assuming Compton-thick obscuration ({\$}N{\_}{\{}\backslashrm H{\}}=1.5\backslashtimes10{\^{}}{\{}24{\}}{\$} cm{\$}{\^{}}{\{}-2{\}}{\$}), which is only 3.6{\%} of the luminosity expected from the extinction corrected [OIII] luminosity. With the NuSTAR observation, we succeed to identify that this ULIRG has a most extreme case of X-ray deficit among local ULIRGs. A possible scenario to explain the drastic declining in both of the corona (X-ray) and torus (MIR) is that the primary radiation from the AGN accretion disk is currently in a fading status, as a consequence of a powerful nuclear wind suggested by its powerful ionized outflow in the galaxy scale.},
archivePrefix = {arXiv},
arxivId = {2011.06914},
author = {Chen, Xiaoyang and Ichikawa, Kohei and Noda, Hirofumi and Kawamuro, Taiki and Kawaguchi, Toshihiro and Toba, Yoshiki and Akiyama, Masayuki},
doi = {10.3847/2041-8213/abca30},
eprint = {2011.06914},
file = {:home/william/Documents/Papers/2011.06914.pdf:pdf},
issn = {2041-8205},
journal = {Astrophys. J.},
keywords = {active galaxies,ulirg,x-ray agn},
number = {1},
pages = {L2},
title = {{NuSTAR Non-detection of a Faint Active Galactic Nucleus in an Ultraluminous Infrared Galaxy with Kpc-scale Fast Wind}},
volume = {905},
year = {2020}
}
@article{Cruz1999,
author = {Cruz, Santa},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Cruz - 1999 - ( 1999. The American Astronomical Society. All rights reserved. Printed in U.S.A.pdf:pdf},
number = {1994},
pages = {118--135},
title = {{( 1999. The American Astronomical Society. All rights reserved. Printed in U.S.A.}},
volume = {20},
year = {1999}
}
@article{Fukumura2017,
abstract = {We analyze a 900-ks stacked Chandra/HETG spectrum of NGC 3783 in the context of magnetically-driven accretion-disk wind models in an effort to provide tight constraints on the global conditions of the underlying absorbers. Motivated by the earlier measurements of its absorption measure distribution (AMD) indicating X-ray-absorbing ionic columns that decrease slowly with decreasing ionization parameter, we employ 2D magnetohydrodynamic (MHD) disk-wind models to describe the global outflow. We compute its photoionization structure along with the wind kinematic properties allowing us to further calculate in a self-consistent fashion the shapes of the major X-ray absorption lines. With the wind radial density profile determined by the AMD, the profiles of the ensemble of the observed absorption features are determined by the two global parameters of the MHD wind; i.e. disk inclination $\backslash$theta{\_}obs and wind density normalization n{\_}o. Considering the most significant absorption features in the ({\~{}}1.8A-20A) range, we show that the MHD-wind is best described by n(r){\~{}}6.9e11(r/ro){\^{}}-1.15 [cm{\^{}}-3] and $\backslash$theta{\_}obs=44deg. We argue that winds launched by X-ray heating, radiation pressure or even MHD winds but with steeper radial density profiles are strongly disfavored by data. Considering the properties of Fe K band absorption features (i.e. Fe xxv and Fe xxvi), while typically prominent in the AGN X-ray spectra, they appear to be weak in NGC 3783. For the specific parameters of our model obtained by fitting the AMD and the rest of absorption features, these features are found to be weak in agreement with observation.},
archivePrefix = {arXiv},
arxivId = {1712.08181},
author = {Fukumura, Keigo and Kazanas, Demosthenes and Shrader, Chris and Behar, Ehud and Tombesi, Francesco and Contopoulos, Ioannis},
doi = {10.3847/1538-4357/aaa3f6},
eprint = {1712.08181},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Fukumura et al. - 2017 - Magnetized Disk-Winds in NGC 3783.pdf:pdf},
isbn = {0112210201},
issn = {1538-4357},
journal = {Astrophys. J.},
keywords = {accretion,accretion disks,accretion,accretion disks,galaxies: individual (NG,galaxies,individual,magnetohydrodynamics,methods,mhd,ngc3783,numerical,seyfert},
number = {1},
pages = {40},
publisher = {IOP Publishing},
title = {{Magnetized Disk-Winds in NGC 3783}},
url = {http://arxiv.org/abs/1712.08181},
volume = {853},
year = {2017}
}
@article{Tan2021,
abstract = {Infrared quasi-stellar objects (IR QSOs) are a rare subpopulation selected from ultraluminous infrared galaxies (ULIRGs) and have been regarded as promising candidates of ULIRG-to-optical QSO transition objects. Here we present NOEMA observations of the CO(1-0) line and 3 mm continuum emission in an IR QSO IRAS F07599+6508 at {\$}z=0.1486{\$}, which has many properties in common with Mrk 231. The CO emission is found to be resolved with a major axis of {\$}\backslashsim{\$}6.1 kpc that is larger than the size of {\$}\backslashsim{\$}4.0 kpc derived for 3 mm continuum. We identify two faint CO features located at a projected distance of {\$}\backslashsim{\$}11.4 and 19.1 kpc from the galaxy nucleus, respectively, both of which are found to have counterparts in the optical and radio bands and may have a merger origin. A systematic velocity gradient is found in the CO main component, suggesting that the bulk of molecular gas is likely rotationally supported. Based on the radio-to-millimeter spectral energy distribution and IR data, we estimate that about 30{\$}\backslash{\%}{\$} of the flux at 3 mm arises from free-free emission and infer a free-free-derived star formation rate of 77 {\$}M{\_}\backslashodot\backslash {\{}\backslashrm yr{\^{}}{\{}-1{\}}{\}}{\$}, close to the IR estimate corrected for the AGN contribution. We find a high-velocity CO emission feature at the velocity range of about -1300 to -2000 km s{\$}{\^{}}{\{}-1{\}}{\$}. Additional deep CO observations are needed to confirm the presence of a possible very high-velocity CO extension of the OH outflow in this IR QSO.},
archivePrefix = {arXiv},
arxivId = {2104.01069},
author = {Tan, Qing-Hua and Gao, Yu and Daddi, Emanuele and Xia, Xiao-Yang and Hao, Cai-Na and Omont, Alain and Kohno, Kotaro},
eprint = {2104.01069},
file = {:home/william/Documents/Papers/2104.01069.pdf:pdf},
keywords = {ISM-galaxies,active-galaxies,evolution-galaxies,galaxies,molecules,starburst-ISM},
number = {2012},
title = {{Deep Observations of CO and Free-Free Emission in Ultraluminous Infrared QSO IRAS F07599+6508}},
url = {http://arxiv.org/abs/2104.01069},
year = {2021}
}
@article{Costa2015,
abstract = {Observations of the emission from spatially extended cold gas around bright high-redshift QSOs reveal surprisingly large velocity widths exceeding 2000 km s{\^{}}(-1), out to projected distances as large as 30 kpc. The high velocity widths have been interpreted as the signature of powerful AGN-driven outflows. Naively, these findings appear in tension with hydrodynamic models in which AGN-driven outflows are energy-driven and thus very hot with typical temperatures T = 10{\^{}}6-7 K. Using the moving-mesh code Arepo, we perform 'zoom-in' cosmological simulations of a z = 6 QSO and its environment, following black hole growth and feedback via energy-driven outflows. In the simulations, the QSO host galaxy is surrounded by a clumpy circum-galactic medium pre-enriched with metals due to supernovae-driven galactic outflows. As a result, part of the AGN-driven hot outflowing gas can cool radiatively, leading to large amounts ({\textgreater} 10{\^{}}9 M{\_}sun) of cold gas comoving with the hot bipolar outflow. This results in velocity widths of spatially extended cold gas similar to those observed. We caution, however, that gas inflows, random motions in the deep potential well of the QSO host galaxy and cooling of supernovae-driven winds contribute significantly to the large velocity width of the cold gas in the simulations, complicating the interpretation of observational data.},
author = {Costa, Tiago and Sijacki, Debora and Haehnelt, Martin G.},
doi = {10.1093/mnrasl/slu193},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Costa, Sijacki, Haehnelt - 2015 - Fast cold gas in hot AGN outflows.pdf:pdf},
issn = {17453933},
journal = {Mon. Not. R. Astron. Soc. Lett.},
keywords = {Cosmology: theory,Methods: numerical,Quasars: supermassive black holes},
number = {1},
pages = {L30--L34},
title = {{Fast cold gas in hot AGN outflows}},
volume = {448},
year = {2015}
}
@article{Carretti2013,
abstract = {The nucleus of the Milky Way is known to harbour regions of intense star formation activity as well as a super-massive black hole. Recent Fermi space telescope observations have revealed regions of $\backslash$gamma-ray emission reaching far above and below the Galactic Centre, the so-called Fermi bubbles. It is uncertain whether these were generated by nuclear star formation or by quasar-like outbursts of the central black hole and no information on the structures' magnetic field has been reported. Here we report on the detection of two giant, linearly-polarized radio Lobes, containing three ridge-like sub-structures, emanating from the Galactic Centre. The Lobes each extend {\~{}}60 deg, bear a close correspondence to the Fermi bubbles, are located in the Galactic bulge, and are permeated by strong magnetic fields of up to 15 $\backslash$mu G. Our data signal that the radio Lobes originate in a bi-conical, star-formation (rather than black hole) driven outflow from the Galaxy's central 200 pc that transports a massive magnetic energy of {\~{}}10{\^{}}55 erg into the Galactic halo. The ridges wind around this outflow and, we suggest, constitute a `phonographic' record of nuclear star formation activity over at least 10 Myr.},
author = {Carretti, Ettore and Crocker, Roland M. and Staveley-Smith, Lister and Haverkorn, Marijke and Purcell, Cormac and Gaensler, B. M. and Bernardi, Gianni and Kesteven, Michael J. and Poppi, Sergio},
doi = {10.1038/nature11734},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Carretti et al. - 2013 - Giant magnetized outflows from the centre of the Milky Way.pdf:pdf},
issn = {00280836},
journal = {Nature},
number = {7430},
pages = {66--69},
publisher = {Nature Publishing Group},
title = {{Giant magnetized outflows from the centre of the Milky Way}},
url = {http://dx.doi.org/10.1038/nature11734},
volume = {493},
year = {2013}
}

@ARTICLE{Schure2009,
       author = {{Schure}, K.~M. and {Kosenko}, D. and {Kaastra}, J.~S. and {Keppens}, R. and {Vink}, J.},
        title = "{A new radiative cooling curve based on an up-to-date plasma emission code}",
      journal = {\aap},
     keywords = {hydrodynamics, ISM: evolution, radiation mechanisms: thermal, Astrophysics - Galaxy Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2009,
        month = dec,
       volume = {508},
       number = {2},
        pages = {751-757},
          doi = {10.1051/0004-6361/200912495},
archivePrefix = {arXiv},
       eprint = {0909.5204},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A&A...508..751S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Komossa2015a,
abstract = {Aims: Radio-loud narrow-line type 1 galaxies provide us with a fresh look at the blazar phenomenon, the causes of radio loudness, and the physics of jet formation. We present a multi-wavelength study of the radio-loud narrow-line type 1 quasar RX J2314.9+2243, which exhibits some remarkable multi-wavelength properties. It is among the few radio-loud narrow-line type 1 galaxies, with a tentative $\gamma$-ray detection, is luminous in the infrared, and shows an exceptionally broad and blueshifted [OIII]$\lambda$5007 emission-line component.  Methods: In order to understand the nature of this source, we have obtained optical, UV, X-ray, and radio observations of RX J2314.9+2243.  Results: Its spectral energy distribution (SED) shows a broad hump extending between the IR and far-UV, a steep radio spectrum and flat X-ray spectrum. Its IR to far-UV SED is consistent with a scenario, in which synchrotron emission from a jet dominates the broadband emission, even though an absorption scenario cannot yet be fully excluded. The high blueshift of its very broad [OIII] component, 1260 km s-1, is consistent with a face-on view, with the jet (and outflow) pointing towards us. RX J2314.9+2243 likely represents an extreme case of AGN induced feedback in the local universe.  The optical spectrum (FITS format) is only available at the CDS via anonymous ftp to http://cdsarc.u-strasbg.fr (ftp://130.79.128.5) or via http://cdsarc.u-strasbg.fr/viz-bin/qcat?J/A+A/574/A121},
author = {Komossa, S. and Xu, Dawei and Fuhrmann, L. and Grupe, D. and Yao, S. and Fan, Z. and Myserlis, I. and Angelakis, E. and Karamanavis, V. and Yuan, W. and Zensus, J. A.},
doi = {10.1051/0004-6361/201424814},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Komossa et al. - 2015 - What powers the radio-loud narrow-line Seyfert 1 galaxy RX J2314.92243.pdf:pdf},
issn = {0004-6361},
journal = {Astron. Astrophys.},
keywords = {2243,9,active,evolution,galaxies,individual,rx j2314,seyfert},
pages = {A121},
title = {{What powers the radio-loud narrow-line Seyfert 1 galaxy RX J2314.9+2243?}},
url = {http://www.aanda.org/10.1051/0004-6361/201424814},
volume = {574},
year = {2015}
}
@article{Xu2015,
author = {Xu, Ye},
file = {:home/william/Documents/Papers/[Cunnigham(thesis)]-Molecular.Outflows.in.SF.regions.pdf:pdf},
number = {August},
title = {{Molecular spectra in massive star forming regions}},
year = {2015}
}
@article{Yang2017,
abstract = {The Fermi bubbles, two giant gamma-ray bubbles above and below the Galactic center (GC), are among the most important findings of the Fermi Gamma-ray Space Telescope. Because of the proximity, spatially resolved, multi-wavelength observations offer excellent opportunities to learn about the physical origin of the bubbles. One of the unique features of the observed bubbles is that their gamma-ray spectrum, including a high-energy cutoff at {\~{}}110 GeV and the overall shape of the spectrum, is nearly spatially uniform. The high-energy spectral cutoff is suggestive of a leptonic origin as it could be a signature of synchrotron and inverse-Compton (IC) cooling of cosmic-ray (CR) electrons; however, even for a leptonic model, it is not obvious why the spectrum should be spatially uniform. In this work, we investigate the formation of the Fermi bubble in the leptonic jet scenario using a newly implemented CRSPEC module in FLASH that allows us to track the evolution of CR spectrum on-the-fly during the simulations. We show that the high-energy cutoff is caused by fast synchrotron and IC cooling near the GC when the jets were first launched. After the jets propagate away from the GC, the dynamical timescale of the jets become the shortest among all relevant timescales, and therefore the spectrum is essentially advected with only mild cooling losses. This could explain why the bubble spectrum is nearly spatially uniform: the CRs from different parts of the bubbles as seen today all share the same origin near the GC at early stage of the bubble expansion. We find that the CR spatial and spectral distribution predicted by the leptonic jet model can simultaneously match the normalization, spectral shape, and high-energy cutoff of the observed gamma-ray spectrum and their spatial uniformity, suggesting that past AGN jet activity is a likely mechanism for the formation of the Fermi bubbles.},
archivePrefix = {arXiv},
arxivId = {1706.05025},
author = {Yang, H. -Y. K. and Ruszkowski, M.},
doi = {ARTN 2
10.3847/1538-4357/aa9434},
eprint = {1706.05025},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Yang, Ruszkowski - 2017 - The Spatially Uniform Spectrum of the Fermi Bubbles the Leptonic AGN Jet Scenario.pdf:pdf},
isbn = {0004-637x},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {cosmic rays,cosmic rays,Galaxy: nucleus,gamma rays: galaxies,m,galaxies,galaxy,gamma rays,magnetohydrodynamics,mhd,nucleus},
number = {1},
pages = {2},
publisher = {IOP Publishing},
title = {{The Spatially Uniform Spectrum of the Fermi Bubbles: the Leptonic AGN Jet Scenario}},
url = {http://arxiv.org/abs/1706.05025},
volume = {850},
year = {2017}
}
@article{DiMatteo2005,
abstract = {In the early Universe, while galaxies were still forming, black holes as massive as a billion solar masses powered quasars. Supermassive black holes are found at the centres of most galaxies today, where their masses are related to the velocity dispersions of stars in their host galaxies and hence to the mass of the central bulge of the galaxy. This suggests a link between the growth of the black holes and their host galaxies, which has indeed been assumed for a number of years. But the origin of the observed relation between black hole mass and stellar velocity dispersion, and its connection with the evolution of galaxies, have remained unclear. Here we report simulations that simultaneously follow star formation and the growth of black holes during galaxy-galaxy collisions. We find that, in addition to generating a burst of star formation, a merger leads to strong inflows that feed gas to the supermassive black hole and thereby power the quasar. The energy released by the quasar expels enough gas to quench both star formation and further black hole growth. This determines the lifetime of the quasar phase (approaching 100 million years) and explains the relationship between the black hole mass and the stellar velocity dispersion.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0502199},
author = {{Di Matteo}, Tiziana and Springel, Volker and Ilernquist, Lars},
doi = {10.1038/nature03335},
eprint = {0502199},
file = {:home/william/Documents/Papers/dimatteo2005.pdf:pdf},
issn = {00280836},
journal = {Nature},
number = {7026},
pages = {604--607},
primaryClass = {astro-ph},
title = {{Energy input from quasars regulates the growth and activity of black holes and their host galaxies}},
volume = {433},
year = {2005}
}
@article{Miralles-Caballero2011,
abstract = {We present a comprehensive characterization of the general properties (luminosity functions (LFs), mass, size, ages, etc.) of optically selected compact stellar objects (knots) in a representative sample of 32 low-z luminous and ultraluminous infrared galaxies ((U)LIRGs). It is important to understand the formation and evolution of these properties in such systems, which represent the most extreme cases of starbursts in the low-z universe. We have made use of high angular resolution Advanced Camera for Surveys images from the Hubble Space Telescope in F435W (B) and F814W (I) bands. The galaxies in the sample represent different interaction phases (first contact, pre-merger, merger, and post-merger) and cover a wide luminosity range (11.46 ≤ log (L IR/L) ≤ 12.54). With a median size of 32pc, most of the nearly 3000 knots detected consist of complexes of star clusters. Some of the knots (15{\%}) are so blue that their colors indicate a young (i.e., {\textless}30Myr) and almost extinction-free population. There is a clear correlation of the mass of these blue knots with their radius, where MR 1.91 0.14, similar to that found in complexes of clusters in M51 and in giant molecular clouds. This suggests that the star formation within the knots is proportional to the gas density at any given radius. This relation does not depend significantly on either the infrared luminosity of the system or the interaction phase. The star formation of all the knots is characterized by LFs of the knots with slopes close to 2. Nevertheless, we see a marginally significant indication that the LF evolves with the interaction process, becoming steeper from early to advanced merger phases. Due to size-of-sample effects we are probably sampling knots in ULIRGs that intrinsically more luminous (by a factor of about four) than in less luminous systems. They also have sizes and are likely to have masses characteristic of clumps in galaxies at z ≳ 1. Knots in post-mergers are on average (1.3-2 times) larger, more luminous (2 mag) in the I band, and 0.5mag redder than those in systems in earlier phases. Two scenarios are briefly discussed: (1) the likely presence of relatively high extinction in the most advanced mergers and (2) the dissolution of the less massive clusters and/or their coalescence into more massive, evolved superclusters. {\textcopyright} 2011. The American Astronomical Society. All rights reserved.},
archivePrefix = {arXiv},
arxivId = {0906.2797},
author = {Garc{\'{i}}a-Mar{\'{i}}n, M. and Colina, Luis and Arribas, Santiago and Miralles-Caballero, Daniel and Colina, Luis and Arribas, Santiago and Duc, Pierre Alain and Chung, Aeree and Narayanan, Gopal and Yun, Min S. and Heyer, Mark and Erickson, Neal R.},
doi = {10.1088/0004-6256/142/3/79},
eprint = {0906.2797},
file = {:home/william/Documents/Papers/aa12537-09.pdf:pdf;:home/william/Documents/Papers/Miralles-Caballero.pdf:pdf;:home/william/Documents/Papers/0906.2797.pdf:pdf},
issn = {00046361},
journal = {Astron. J.},
keywords = {Galaxies: fundamental parameters,Galaxies: interactions,Galaxies: structure,galaxies: evolution,galaxies: interactions,galaxies: photometry,galaxies: star clusters: general,galaxies: starburst},
number = {3},
pages = {858--872},
title = {{Integral field optical spectroscopy of a representative sample of ULIRGs}},
volume = {142},
year = {2009}
}
@article{Saturni2018,
abstract = {Star-forming galaxies at high redshift show anomalous values of infrared excess, which can be described only by extremizing the existing relations between the shape of their ultraviolet continuum emission and their infrared-to-ultraviolet luminosity ratio, or by constructing $\backslash$textit{\{}ad-hoc{\}} models of star formation and dust distribution. We present an alternative explanation, based on unveiled AGN activity, to the existence of such galaxies. In fact, the presence of a weak AGN configures as a natural scenario in order to explain the observed spectral properties of such high-{\$}z{\$} objects in terms of a continuum slope distribution rather than altered infrared excesses, due to the different shape of the AGN continuum emission with respect to quiescent galaxies. To this aim, we directly compare the infrared-to-ultraviolet properties of high-redshift galaxies to those of known categories of AGN (quasars and Seyferts). We also infer the characteristics of their possible X-ray emission. We find a strong similarity between the spectral shapes and luminosity ratios of AGN with the corresponding properties of such galaxies. In addition, we derive expected X-ray fluxes that are compatible with energetics from AGN activity. We conclude that a moderate AGN contribution to the UV emission of such high-{\$}z{\$} objects is a valid alternative to explain their spectral properties. Even the presence of an active nucleus in each source would not violate the expected quasar statistics. Furthermore, we suggest that the observed similarities between anomalous star-forming galaxies and quasars may provide a benchmark for future theoretical and observational studies on the galaxy population in the early Universe.},
archivePrefix = {arXiv},
arxivId = {1806.07423},
author = {Saturni, Francesco Gabriele and Mancini, Mattia and Pezzulli, Edwige and Tombesi, Francesco},
eprint = {1806.07423},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Saturni et al. - 2018 - Zombie or active An alternative explanation to the properties of star-forming galaxies at high redshift.pdf:pdf},
keywords = {active,galaxies,general,infrared,ism,photometry,quasars,ultraviolet},
pages = {1--13},
title = {{"Zombie" or active? An alternative explanation to the properties of star-forming galaxies at high redshift}},
url = {http://arxiv.org/abs/1806.07423},
volume = {131},
year = {2018}
}
@article{2011ApJ...742...44T,
archivePrefix = {arXiv},
arxivId = {astro-ph.HE/1109.2882},
author = {Tombesi, F and Cappi, M and Reeves, J.{\~{}}N. and Palumbo, G.{\~{}}G.{\~{}}C. and Braito, V and Dadina, M},
doi = {10.1088/0004-637X/742/1/44},
eprint = {1109.2882},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Tombesi et al. - 2011 - Evidence for Ultra-Fast Outflows in radio-quiet active galactic nuclei. II. Detailed photoionization modeling of.pdf:pdf},
journal = {Apj},
keywords = {X-rays: galaxies,black hole physics,galaxies: Seyfert,galaxies: active,line: identification,plasmas},
pages = {44},
primaryClass = {astro-ph.HE},
title = {{Evidence for Ultra-fast Outflows in Radio-quiet Active Galactic Nuclei. II. Detailed Photoionization Modeling of Fe K-shell Absorption Lines}},
volume = {742},
year = {2011}
}
@article{Lonsdale2006,
abstract = { At luminosities above {\~{}} 10 11 L ⊙ , infrared galaxies become the dominant population of extragalactic objects in the local Universe ( z {\textless} 0.5), being more numerous than optically selected starburst and Seyfert galaxies, and QSOs at comparable bolometric luminosity. At the highest luminosities, ultraluminous infrared galaxies (ULIGs: L ir {\textgreater} 10 12 L ⊙ ), outnumber optically selected QSOs by a factor of {\~{}} 1.5–2. All of the nearest ULIGs ( z {\textless}0.1) appear to be advanced mergers that are powered by both a circumnuclear starburst and AGN, both of which are fueled by an enormous concentration of molecular gas ({\~{}} 10 10 M ⊙ ) that has been funneled into the merger nucleus. ULIGs may represent a primary stage in the formation of massive black holes and elliptical galaxy cores. The intense circumnuclear starburst that accompanies the ULIG phase may also represent a primary stage in the formation of globular clusters, and the metal enrichment of the intergalactic medium by gas and dust expelled from the nucleus due to the combined forces of supernova explosions and powerful stellar winds. },
archivePrefix = {arXiv},
arxivId = {astro-ph/0603031},
author = {Sanders, D.B. and Surace, J.A. and Ishida, C.M.},
doi = {10.1017/s0074180900112859},
eprint = {0603031},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Lonsdale, Farrah, Smith - 2006 - Ultraluminous Infrared Galaxies.pdf:pdf},
issn = {0074-1809},
journal = {Symp. - Int. Astron. Union},
pages = {289--294},
primaryClass = {astro-ph},
title = {{Ultraluminous Infrared Galaxies}},
url = {http://arxiv.org/abs/astro-ph/0603031{\%}0Ahttp://dx.doi.org/10.1007/3-540-30313-8{\_}9},
volume = {186},
year = {1999}
}
@article{Feltre2017,
abstract = {Spectroscopic studies of active galactic nuclei (AGN) are powerful means of probing the physical properties of the ionized gas within them. In particular, near future observational facilities, such as the James Webb Space Telescope (JWST), will allow detailed statistical studies of rest-frame ultraviolet and optical spectral features of the very distant AGN with unprecedented accuracy. In this proceedings, we discuss the various ways of exploiting new dedicated photoionization models of the narrow-line emitting regions (NLR) of AGN for the interpretation of forthcoming revolutionary datasets.},
author = {Feltre, Anna and Charlot, Stephane and Mignoli, Marco and Bongiorno, Angela and Calura, Francesco and Chevallard, Jacopo and Curtis-Lake, Emma and Gilli, Roberto and Plat, Adele},
doi = {10.3389/fspas.2017.00032},
file = {:home/william/Documents/Papers/fspas-04-00032.pdf:pdf},
issn = {2296987X},
journal = {Front. Astron. Sp. Sci.},
keywords = {active galaxies,emission lines,spectral models,spectroscopy,ultraviolet},
number = {November},
pages = {1--5},
title = {{Ultraviolet/Optical Emission of the Ionized Gas in AGN: Diagnostics of the Ionizing Source and Gas Properties}},
volume = {4},
year = {2017}
}
@article{Malyshev2017,
abstract = {The Fermi bubbles are one of the most remarkable features in the gamma-ray sky revealed by the Fermi Large Area Telescope (LAT). The nature of the gamma-ray emission and the origin of the bubbles are still open questions. In this note, we will review some basic features of leptonic and hadronic modes of gamma-ray production. At the moment, gamma rays are our best method to study the bubbles, but in order to resolve the origin of the bubbles multi-wavelength and multi-messenger observations will be crucial.},
archivePrefix = {arXiv},
arxivId = {1704.02629},
author = {Malyshev, Dmitry},
doi = {10.1051/epjconf/201713603011},
eprint = {1704.02629},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Malyshev - 2017 - Fermi Bubbles an Elephant in the Gamma-ray Sky.pdf:pdf},
pages = {4--7},
title = {{Fermi Bubbles: an Elephant in the Gamma-ray Sky}},
url = {http://arxiv.org/abs/1704.02629{\%}0Ahttp://dx.doi.org/10.1051/epjconf/201713603011},
volume = {3011},
year = {2017}
}
@article{1996ApJ...462..563N,
author = {Navarro, J.{\~{}}F. and Frenk, C.{\~{}}S. and White, S.{\~{}}D.{\~{}}M.},
doi = {10.1086/177173},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Navarro, Frenk, White - 1996 - The Structure of Cold Dark Matter Halos.pdf:pdf},
journal = {Apj},
keywords = {COSMOLOGY: DARK MATTER,COSMOLOGY: THEORY,GALAXIES: HALOS,METHODS: NUMERICAL},
pages = {563},
title = {{The Structure of Cold Dark Matter Halos}},
volume = {462},
year = {1996}
}
@article{Shangguan2020,
abstract = {The molecular gas serves as a key probe of the complex interplay between black hole accretion and star formation in the host galaxies of active galactic nuclei (AGNs). We use CO(2–1) observations from a new ALMA survey, in conjunction with literature measurements, to investigate the molecular gas properties of a representative sample of 40 z {\textless} 0.3 Palomar-Green quasars, the largest and most sensitive study of molecular gas emission to date for nearby quasars. We find that the AGN luminosity correlates with both the CO luminosity and black hole mass, suggesting that AGN activity is loosely coupled to the cold gas reservoir of the host. The observed strong correlation between host galaxy total infrared luminosity and AGN luminosity arises from their common dependence on the molecular gas. We argue that the total infrared luminosity, at least for low-redshift quasars, can be used to derive reliable star formation rates for the host galaxy. The host galaxies of low-redshift quasars have molecular gas content similar to that of star-forming galaxies of comparable stellar mass. Moreover, they share similar gas kinematics, as evidenced by their CO Tully-Fisher relation and the absence of detectable molecular outflows down to sensitive limits. There is no sign that AGN feedback quenches star formation for the quasars in our sample. On the contrary, the abundant gas supply forms stars prodigiously, at a rate that places most of them above the star-forming main sequence and with an efficiency that rivals that of starburst systems.},
archivePrefix = {arXiv},
arxivId = {2007.11286},
author = {Shangguan, Jinyi and Ho, Luis C. and Bauer, Franz E. and Wang, Ran and Treister, Ezequiel},
doi = {10.3847/1538-4357/aba8a1},
eprint = {2007.11286},
file = {:home/william/Documents/Papers/Shangguan{\_}2020{\_}ApJ{\_}899{\_}112.pdf:pdf},
issn = {1538-4357},
journal = {arXiv},
keywords = {(Galaxies:) quasars: general,Galaxies: ISM,Galaxies: active,Galaxies: evolution,Galaxies: seyfert,Submillimeter: galaxies},
number = {2},
pages = {112},
publisher = {IOP Publishing},
title = {{AGN feedback and star formation of quasar host galaxies: Insights from the molecular gas}},
url = {http://dx.doi.org/10.3847/1538-4357/aba8a1},
volume = {899},
year = {2020}
}
@article{Ibanez-Mejia2015,
abstract = {Molecular cloud observations show that clouds have non-thermal velocity dispersions that scale with the cloud size as {\$}\backslashsigma\backslashpropto R{\^{}}{\{}1/2{\}}{\$} at constant surface density, and for varying surface density scale with both the cloud`s size and surface density, {\$}\backslashsigma{\^{}}2 \backslashpropto R \backslashSigma{\$}. The energy source driving these chaotic motions remains poorly understood. We describe the velocity dispersions observed in a cloud population formed in a kiloparsec-scale numerical simulation of a magnetized, supernova-driven, self-gravitating, interstellar medium, including diffuse heating and radiative cooling. We compare the relationships between velocity dispersion, size, and surface density measured in the simulated cloud population to those found in observations of Galactic molecular clouds. We find that external supernova explosions can not drive turbulent motions of the observed magnitudes within dense clouds. On the other hand, self-gravity also induces non-thermal motions as gravitationally bound clouds begin to collapse in our model, and by doing so their internal velocity dispersions recover the observed relations. Energy conservation suggests that the observed behavior is consistent with the kinetic energy being proportional to the gravitational energy. However, the clouds in our model show no sign of reaching a stable equilibrium state at any time, even for strongly magnetized clouds. We conclude that gravitationally bound molecular clouds are always in a state of gravitational collapse and their properties are a natural result of this chaotic collapse. In order to agree with observed star formation efficiencies, this process must be terminated by the early destruction of the clouds, presumably from internal stellar feedback.},
archivePrefix = {arXiv},
arxivId = {1511.05602},
author = {Ib{\'{a}}{\~{n}}ez-Mej{\'{i}}a, Juan C. and {Mac Low}, Mordecai-Mark and Klessen, Ralf S. and Baczynski, Christian},
doi = {10.3847/0004-637X/824/1/41},
eprint = {1511.05602},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ib{\'{a}}{\~{n}}ez-Mej{\'{i}}a et al. - 2015 - Gravitational contraction versus Supernova driving and the origin of the velocity dispersion-size relati.pdf:pdf},
issn = {1538-4357},
journal = {Astrophys. J.},
keywords = {ISM: clouds,ISM: kinematics and dynamics,ISM: structure,clouds,ism,kinematics and dynamics,magnetohydrodynamics,magnetohydrodynamics (MHD),mhd,structure,turbulence},
number = {1},
pages = {1--15},
publisher = {IOP Publishing},
title = {{Gravitational contraction versus Supernova driving and the origin of the velocity dispersion-size relation in molecular clouds}},
url = {http://arxiv.org/abs/1511.05602{\%}0Ahttp://dx.doi.org/10.3847/0004-637X/824/1/41},
volume = {824},
year = {2015}
}
@article{Goosmann2011,
abstract = {We model the expected X-ray polarization induced by complex reprocessing in the active nucleus of the Seyfert 2 galaxy NGC 1068. Recent analysis of infrared interferometry observations suggests that the ionized outflows ejected by the central engine are not aligned with the symmetry axis of the obscuring torus. This conclusion was obtained by extrapolating the apparent orientation of the narrow-line region to the inner parts of the ionization cones. We show that future measurements of the soft X-ray polarization vector unambiguously determine the orientation of the ionization cones. Furthermore, X-ray polarimetry across a broad photon energy range may independently verify the misalignment between the ionization cones and the axis of the torus. To model the expected polarization percentage and position angle, we apply the radiative transfer code stokes. Reprocessing of the primary X-ray radiation takes place in the accretion disc, the surrounding equatorial torus and the inclined, ionized outflows. We also examine additional equatorial scattering occurring in between the accretion disc and the inner surfaces of the torus. Radiative coupling between the different reprocessing components is computed coherently. The resulting polarization properties depend on the optical depth of the reprocessing regions and on the viewing angle of the observer. We show that even under unfavourable conditions the misalignment of the outflows with respect to the torus axis can be determined from a rotation of the polarization position angle between softer and harder X-rays. We argue that the misalignment of the outflows with respect to the torus axis in NGC 1068 may be constrained by a future X-ray mission if equipped with a broad-band polarimeter. {\textcopyright} 2011 The Authors Monthly Notices of the Royal Astronomical Society {\textcopyright} 2011 RAS.},
archivePrefix = {arXiv},
arxivId = {1012.4652},
author = {Goosmann, R. W. and Matt, G.},
doi = {10.1111/j.1365-2966.2011.18923.x},
eprint = {1012.4652},
file = {:home/william/Documents/Papers/1012.4652.pdf:pdf},
issn = {00358711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: Seyfert,Galaxies: individual: NGC 1068,Polarization,Radiative transfer,Techniques: polarimetric,X-rays: galaxies},
number = {4},
pages = {3119--3128},
title = {{Spotting the misaligned outflows in NGC 1068 using X-ray polarimetry}},
volume = {415},
year = {2011}
}
@article{Tombesi2013a,
abstract = {The existence of ionized X-ray absorbing layers of gas along the line of sight to the nuclei of Seyfert galaxies is a well established observational fact. This material is systematically outflowing and shows a large range in parameters. However, its actual nature and dynamics are still not clear. In order to gain insights into these important issues we performed a literature search for papers reporting the parameters of the soft X-ray warm absorbers (WAs) in 35 type 1 Seyferts and compared their properties to those of the ultra-fast outflows (UFOs) detected in the same sample. The fraction of sources with WAs is {\textgreater}60{\%}, consistent with previous studies. The fraction of sources with UFOs is {\textgreater}34{\%}, {\textgreater}67{\%} of which also show WAs. The large dynamic range obtained when considering all the absorbers together allows us, for the first time, to investigate general relations among them. In particular, we find significant correlations indicating that the closer the absorber is to the central black hole, the higher the ionization, column, outflow velocity and consequently the mechanical power. The absorbers continuously populate the whole parameter space, with the WAs and the UFOs lying always at the two ends of the distribution. This strongly suggest that these absorbers, often considered of different types, could actually represent parts of a single large-scale stratified outflow observed at different locations from the black hole. The observed parameters and correlations are consistent with both radiation pressure through Compton scattering and MHD processes contributing to the outflow acceleration, the latter playing a major role. Most of the absorbers, especially the UFOs, have a sufficiently high mechanical power to significantly contribute to AGN feedback.},
archivePrefix = {arXiv},
arxivId = {1212.4851},
author = {Tombesi, F and Cappi, M and Reeves, J N and Nemmen, R S and Braito, V and Gaspari, M and Reynolds, C S},
doi = {10.1093/mnras/sts692},
eprint = {1212.4851},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Tombesi et al. - 2013 - Unification of X-ray winds in Seyfert galaxies From ultra-fast outflows to warm absorbers.pdf:pdf},
issn = {00358711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Accretion,Black hole physics,Galaxies: Seyfert,Galaxies: active,X-rays: galaxies,accretion discs},
number = {2},
pages = {1102--1117},
title = {{Unification of X-ray winds in Seyfert galaxies: From ultra-fast outflows to warm absorbers}},
volume = {430},
year = {2013}
}
@article{Fluetsch2021,
abstract = {Galactic outflows are known to consist of several gas phases; however, the connection between these phases has been investigated little and only in a few objects. In this paper, we analyse Multi Unit Spectroscopic Explorer (MUSE)/Very Large Telescope (VLT) data of 26 local (U)LIRGs and study their ionized and neutral atomic phases. We also include objects from the literature to obtain a sample of 31 galaxies with spatially resolved multiphase outflow information. We find that the ionized phase of the outflows has on average an electron density three times higher than the disc (ne,disc ∼145 cm-3 versus ne,outflow ∼500 cm-3), suggesting that cloud compression in the outflow is more important than cloud dissipation. We find that the difference in extinction between outflow and disc correlates with the outflow gas mass. Together with the analysis of the outflow velocities, this suggests that at least some of the outflows are associated with the ejection of dusty clouds from the disc. This may support models where radiation pressure on dust contributes to driving galactic outflows. The presence of dust in outflows is relevant for potential formation of molecules inside them. We combine our data with millimetre data to investigate the molecular phase. We find that the molecular phase accounts for more than 60 per cent of the total mass outflow rate in most objects and this fraction is higher in active galactic nuclei (AGN)-dominated systems. The neutral atomic phase contributes of the order of 10 per cent, while the ionized phase is negligible. The ionized-to-molecular mass outflow rate declines slightly with AGN luminosity, although with a large scatter.},
archivePrefix = {arXiv},
arxivId = {2006.13232},
author = {Fluetsch, A. and Maiolino, R. and Carniani, S. and Arribas, S. and Belfiore, F. and Bellocchi, E. and Cazzoli, S. and Cicone, C. and Cresci, G. and Fabian, A. C. and Gallagher, R. and Ishibashi, W. and Mannucci, F. and Marconi, A. and Perna, M. and Sturm, E. and Venturi, G.},
doi = {10.1093/mnras/stab1666},
eprint = {2006.13232},
file = {:home/william/Documents/Papers/2006.13232.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {ISM: evolution,galaxies: ISM,galaxies: active,galaxies: evolution},
number = {4},
pages = {5753--5783},
title = {{Properties of the multiphase outflows in local (ultra)luminous infrared galaxies}},
volume = {505},
year = {2021}
}
@article{Strickland2009a,
abstract = {We measure the net energy efficiency of supernova (SN) and stellar wind feedback in the starburst galaxy M82 and the degree of mass loading of the hot gas piston driving its superwind by comparing a large suite of one and two-dimensional hydrodynamical models to a set of observational constraints derived from hard X-ray observations of the starburst region (the fluxes of the He$\alpha$ and Ly$\alpha$-like lines of S, Ar, Ca, and Fe, along with the total diffuse E = 2-8keV X-ray luminosity). These are the first direct measurements of the feedback efficiency and mass loading of SN-heated and enriched plasma in a starburst galaxy. We consider a broad range of plausible parameters for the M82 starburst, varying the age and mode of star formation, the starburst region size and geometry, and SN metal yields. Over all these varied input parameters all the models that satisfy the existing observational constraints have medium to high thermalization efficiencies (30{\%} ≤$\epsilon$ ≤ 100{\%}) and the volume-filling wind fluid that flows out of the starburst region is only mildly centrally mass loaded (1.0 ≤ $\beta$ ≤ 2.8). These results imply a temperature of the plasma within the starburst region in the range 30-80 million Kelvin, a mass-flow rate of the wind fluid out of the starburst region of and a terminal velocity of the wind in the range v ∞ = 1410 - 2240 km s-1 . This velocity is considerably larger than the escape velocity from M82 (v esc ≲ 460 km s-1 ) and the velocity of the H$\alpha$ emitting clumps and filaments within M82's wind (v H$\alpha$ 600 km s-1 ). Drawing on these results we provide a prescription for implementing starburst-driven superwinds in cosmological models of galaxy formation and evolution that more accurately represents the energetics of the hot metal-enriched phases than the existing recipes do. {\textcopyright} 2009. The American Astronomical Society. All rights reserved.},
archivePrefix = {arXiv},
arxivId = {0903.4175},
author = {Strickland, David K. and Heckman, Timothy M.},
doi = {10.1088/0004-637X/697/2/2030},
eprint = {0903.4175},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Strickland, Heckman - 2009 - Supernova feedback efficiency and mass loading in the starburst and galactic superwind exemplar M82.pdf:pdf},
isbn = {bibcode:2009ApJ...697.2030S},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {Galaxies: halos,Galaxies: individual (NGC 3034 (M82)),Galaxies: starburst,ISM: bubbles,Intergalactic medium,X-rays: galaxies},
number = {2},
pages = {2030--2056},
title = {{Supernova feedback efficiency and mass loading in the starburst and galactic superwind exemplar M82}},
volume = {697},
year = {2009}
}
@article{Su2010,
abstract = {Data from the Fermi-LAT reveal two large gamma-ray bubbles, extending 50 degrees above and below the Galactic center, with a width of about 40 degrees in longitude. The gamma-ray emission associated with these bubbles has a significantly harder spectrum (dN/dE {\~{}} E{\^{}}-2) than the IC emission from electrons in the Galactic disk, or the gamma-rays produced by decay of pions from proton-ISM collisions. There is no significant spatial variation in the spectrum or gamma-ray intensity within the bubbles, or between the north and south bubbles. The bubbles are spatially correlated with the hard-spectrum microwave excess known as the WMAP haze; the edges of the bubbles also line up with features in the ROSAT X-ray maps at 1.5-2 keV. We argue that these Galactic gamma-ray bubbles were most likely created by some large episode of energy injection in the Galactic center, such as past accretion events onto the central massive black hole, or a nuclear starburst in the last {\~{}}10 Myr. Dark matter annihilation/decay seems unlikely to generate all the features of the bubbles and the associated signals in WMAP and ROSAT; the bubbles must be understood in order to use measurements of the diffuse gamma-ray emission in the inner Galaxy as a probe of dark matter physics. Study of the origin and evolution of the bubbles also has the potential to improve our understanding of recent energetic events in the inner Galaxy and the high-latitude cosmic ray population.},
author = {Su, Meng and Slatyer, Tracy R. and Finkbeiner, Douglas P.},
doi = {10.1088/0004-637X/724/2/1044},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Su, Slatyer, Finkbeiner - 2010 - Giant gamma-ray bubbles from Fermi-LAT Active Galactic nucleus activity or bipolar Galactic wind.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {Galaxies: active,Galaxies: starburst,Gamma rays: diffuse background,Ism: jets and outflows},
number = {2},
pages = {1044--1082},
title = {{Giant gamma-ray bubbles from Fermi-LAT: Active Galactic nucleus activity or bipolar Galactic wind?}},
url = {http://stacks.iop.org/0004-637X/724/i=2/a=1044?key=crossref.5aa3963ec8c1c799c748f54d6037d4e5},
volume = {724},
year = {2010}
}
@article{Trebitsch2019,
archivePrefix = {arXiv},
arxivId = {1901.01261},
author = {Trebitsch, Maxime and Volonteri, Marta and Dubois, Yohan},
eprint = {1901.01261},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Trebitsch, Volonteri, Dubois - 2019 - Black hole obscuration and duty cycles mediated by AGN feedback in high redshift galaxies.pdf:pdf},
isbn = {1901.01261v1},
keywords = {ages,dark,first stars,formation,galaxies,high-redshift,nuclei,quasars,reionization,supermassive black holes},
number = {January},
pages = {1--13},
title = {{Black hole obscuration and duty cycles mediated by AGN feedback in high redshift galaxies}},
url = {https://arxiv.org/abs/1901.01261},
volume = {13},
year = {2019}
}
@article{doi:10.1146/annurev-astro-082214-122316,
author = {King, Andrew and Pounds, Ken},
doi = {10.1146/annurev-astro-082214-122316},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/King, Pounds - 2015 - Powerful Outflows and Feedback from Active Galactic Nuclei.pdf:pdf},
journal = {Annu. Rev. Astron. Astrophys.},
number = {1},
pages = {115--154},
title = {{Powerful Outflows and Feedback from Active Galactic Nuclei}},
url = {https://doi.org/10.1146/annurev-astro-082214-122316},
volume = {53},
year = {2015}
}
@article{Pudritz2003,
author = {Pudritz, Ralph E and Ouyed, Rachid and Fendt, Christian and Brandenburg, Axel},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Pudritz et al. - 2003 - DISK WINDS , JETS , AND OUTFLOWS.pdf:pdf},
title = {{DISK WINDS , JETS , AND OUTFLOWS :}},
year = {2003}
}
@article{Ricci2017,
abstract = {The majority of the accreting supermassive black holes in the Universe are obscured by large columns of gas and dust1,2,3. The location and evolution of this obscuring material have been the subject of intense research in the past decades4,5, and are still debated. A decrease in the covering factor of the circumnuclear material with increasing accretion rates has been found by studies across the electromagnetic spectrum1,6,7,8. The origin of this trend may be driven by the increase in the inner radius of the obscuring material with incident luminosity, which arises from the sublimation of dust9; by the gravitational potential of the black hole10; by radiative feedback11,12,13,14; or by the interplay between outflows and inflows15. However, the lack of a large, unbiased and complete sample of accreting black holes, with reliable information on gas column density, luminosity and mass, has left the main physical mechanism that regulates obscuration unclear. Here we report a systematic multi-wavelength survey of hard-X-ray-selected black holes that reveals that radiative feedback on dusty gas is the main physical mechanism that regulates the distribution of the circumnuclear material. Our results imply that the bulk of the obscuring dust and gas is located within a few to tens of parsecs of the accreting supermassive black hole (within the sphere of influence of the black hole), and that it can be swept away even at low radiative output rates. The main physical driver of the differences between obscured and unobscured accreting black holes is therefore their mass-normalized accretion rate.},
archivePrefix = {arXiv},
arxivId = {1709.09651},
author = {Ricci, Claudio and Trakhtenbrot, Benny and Koss, Michael J. and Ueda, Yoshihiro and Schawinski, Kevin and Oh, Kyuseok and Lamperti, Isabella and Mushotzky, Richard and Treister, Ezequiel and Ho, Luis C. and Weigel, Anna and Bauer, Franz E. and Paltani, Stephane and Fabian, Andrew C. and Xie, Yanxia and Gehrels, Neil},
doi = {10.1038/nature23906},
eprint = {1709.09651},
file = {:home/william/Documents/Papers/ricci2017.pdf:pdf},
issn = {14764687},
journal = {Nature},
number = {7673},
pages = {488--491},
publisher = {Nature Publishing Group},
title = {{The close environments of accreting massive black holes are shaped by radiative feedback}},
url = {http://dx.doi.org/10.1038/nature23906},
volume = {549},
year = {2017}
}
@article{Spacek2017a,
abstract = {Energetic feedback from active galactic nuclei (AGNs) is difficult to observe, but often used in simulations to resolve several outstanding issues in galaxy formation. Here we derive new constraints on AGN feedback by comparing observations and simulations of the thermal Sunyaev-Zel'dovich (tSZ) effect, which causes spectral distortions in the cosmic microwave background with signal strengths that are proportional to the total energy deposited into the medium surrounding large galaxies. We draw on observational results presented in Spacek et al. (2016, 2017) who used data from the South Pole Telescope (SPT) and Atacama Cosmology Telescope (ACT) to measure the tSZ signal from {\textgreater}= 10{\^{}}11 M{\_}Sun and {\textgreater}= 1 Gyr galaxies in the redshift ranges of z=0.5-1.0 (low-z) and z=1.0-1.5 (high-z). Using two large-scale cosmological hydrodynamical simulations, one with AGN feedback (Horizon-AGN) and one without (Horizon-NoAGN), we extract simulated tSZ measurements around a population of galaxies equivalent to those observed. We find that the Horizon-AGN results only differ from the SPT measurements at levels of 0.4 sigma at low-z and 0.5 sigma at high-z, but they differ from the ACT measurements at levels of 6.9 sigma at low-z and 14.6 sigma at high-z. The Horizon-NoAGN results provide a slightly worse fit to the SPT measurements at levels of 1.8 sigma at low-z and 0.6 sigma at high-z, but a drastically better match to the ACT measurements at levels of 0.8 sigma at low-z and 1.9 sigma at high-z. We conclude that, while the lower-mass ({\textless}{\~{}} 5 x 10{\^{}}11 M{\_}Sun) SPT results show a hint of AGN feedback energy, the higher-mass ({\textgreater}{\~{}} 5 x 10{\^{}}11 M{\_}Sun) ACT results show significantly less energy than predicted in the simulation including feedback, indicating that AGN feedback may be milder than often predicted.},
archivePrefix = {arXiv},
arxivId = {1711.05304},
author = {Spacek, Alexander and Richardson, Mark and Scannapieco, Evan},
doi = {10.3847/1538-4357/aada01},
eprint = {1711.05304},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Spacek, Richardson, Scannapieco - 2017 - Using Real and Simulated Measurements of the Thermal Sunyaev-Zel'dovich Effect to Constrain Mod.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {cosmic background radiation,cosmic background radiation,galaxies: evolution,in,evolution,galaxies,general,intergalactic medium,large-scale structure of,quasars,universe},
number = {2},
pages = {109},
pmid = {900},
publisher = {IOP Publishing},
title = {{Using Real and Simulated Measurements of the Thermal Sunyaev-Zel'dovich Effect to Constrain Models of AGN Feedback}},
url = {http://arxiv.org/abs/1711.05304},
volume = {865},
year = {2017}
}
@article{Wehrle2009,
author = {a.{\~{}}E. Wehrle and Zacharias, Norbert and Johnston, Kenneth and Boboltz, David and Fey, A.{\~{}}L. and Gaume, Ralph and Ojha, R and Meier, D.{\~{}}L. and Murphy, D.{\~{}}W. and Jones, D.{\~{}}L. and Unwin, S.{\~{}}C. and Piner, B.{\~{}}G.},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Wehrle et al. - 2009 - What is the Structure of Relativistic Jets in AGN on Scales of Light Days.pdf:pdf},
journal = {astro2010 Astron. Astrophys. Decad. Surv.},
pages = {310--+},
title = {{What is the Structure of Relativistic Jets in AGN on Scales of Light Days?}},
volume = {2010},
year = {2009}
}
@article{VanMarle2011,
abstract = {Energy loss through optically thin radiative cooling plays an important part in the evolution of astrophysical gas dynamics and should therefore be considered a necessary element in any numerical simulation. Although the addition of this physical process to the equations of hydrodynamics is straightforward, it does create numerical challenges that have to be overcome in order to ensure the physical correctness of the simulation. First, the cooling has to be treated (semi-)implicitly, owing to the discrepancies between the cooling timescale and the typical timesteps of the simulation. Secondly, because of its dependence on a tabulated cooling curve, the introduction of radiative cooling creates the necessity for an interpolation scheme. In particular, we will argue that the addition of radiative cooling to a numerical simulation creates the need for extremely high resolution, which can only be fully met through the use of adaptive mesh refinement. {\textcopyright} 2010 Elsevier Ltd.},
archivePrefix = {arXiv},
arxivId = {1011.2610},
author = {van Marle, Allard Jan and Keppens, Rony},
doi = {10.1016/j.compfluid.2010.10.022},
eprint = {1011.2610},
file = {:home/william/Documents/Papers/[van Marle, et al.]-Radiative cooling in numerical astrophysics$\backslash$: the need.pdf:pdf},
issn = {00457930},
journal = {Comput. Fluids},
keywords = {Circumstellar envelopes,Computational techniques: fluid dynamics,Radiative recombination,Radiative transfer in astrophysics,Stellar winds},
number = {1},
pages = {44--53},
title = {{Radiative cooling in numerical astrophysics: The need for adaptive mesh refinement}},
volume = {42},
year = {2011}
}
@article{Lakehal2016a,
abstract = {A simple elegant expression of nonadiabatic light wave evolution is necessary in order to have a deeper insight for complicated optical phenomena in light science as well as in everyday life. Light wave propagation in linear media which have time-dependent electromagnetic parameters is investigated by utilizing a quadratic invariant of the system. The time behavior of the nonadiabatic geometric phase of the waves that yield a cyclic nonadiabatic evolution is analyzed in detail. Various quantum properties of light waves in this situation, such as variances of electric and magnetic fields, uncertainty product, coherent and squeezed states, and their classical limits, are developed. For better understanding of our research, we applied our analysis in a particular case. The variances of the fields D and B are illustrated and their time behaviors are addressed. Equivalent results for the corresponding classical systems are deduced from the study of the time evolution of the appropriate coherent and squeezed states.},
author = {Lakehal, Halim and Maamache, Mustapha and Choi, Jeong Ryeol},
doi = {10.1038/srep19860},
file = {:home/william/Documents/Papers/may.srep19860.pdf:pdf},
issn = {20452322},
journal = {Sci. Rep.},
number = {December 2015},
pages = {1--10},
publisher = {Nature Publishing Group},
title = {{Novel quantum description for nonadiabatic evolution of light wave propagation in time-dependent linear media}},
url = {http://dx.doi.org/10.1038/srep19860},
volume = {6},
year = {2016}
}
@article{Orszag1992,
abstract = {A Comment on the Letter by J. Janszky and An. V. Vinogradov, Phys. Rev. Lett. 64, 2771 (1990). {\textcopyright} 1992 The American Physical Society.},
author = {Orszag, M. and Ram{\'{i}}rez, R. and Retamal, J. C. and Saavedra, C.},
doi = {10.1103/PhysRevLett.68.3815},
file = {:home/william/Documents/Papers/PhysRevA.45.6570.pdf:pdf},
issn = {00319007},
journal = {Phys. Rev. Lett.},
number = {25},
pages = {3815},
title = {{Superposition of coherent states and squeezing}},
volume = {68},
year = {1992}
}
@article{Baron2018d,
abstract = {Large scale outflows of different gas phases are ubiquitous in the host galaxies of active galactic nuclei (AGN). Despite their many differences, they share a common property - they all contain dust. The dust is carried with the outflow, heated by the AGN, and emits at infrared wavelengths. This paper shows that the infrared emission of this dust can be used to detect AGN outflows and derive their properties. We use a sample of about 4000 type II AGN and compare the infrared properties of systems that show spectroscopic signature of ionized gas outflows to systems that do not. We detect an additional mid-infrared emission component in galaxies with spectroscopically discovered winds, and attribute it to the dust in the outflow. This new component offers novel constraints on the outflow properties, such as its mean location and covering factor. We measure the location of the outflow for roughly 1700 systems, with the distribution showing a prominent peak around 500 pc, a tail that extends to large distances (10 kpc), and no objects with a location smaller than 50 pc. The covering factor of the wind shows a wide distribution which is centered around 0.1, with 24$\%$ (8$\%$) of the winds showing covering factors larger than 0.2 (0.5). The dust emission is not sensitive to various systematics affecting optically-selected outflows, and can be used to estimate the mass outflow rate in thousands of galaxies with only 1D spectra.},
archivePrefix = {arXiv},
arxivId = {1810.06562},
author = {Baron, Dalya and Netzer, Hagai},
doi = {10.1093/mnras/sty2935},
eprint = {1810.06562},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Baron, Netzer - 2018 - Discovering AGN-driven winds through their infrared emission I. General method and wind location.pdf:pdf},
keywords = {active,evolution,galaxies,general,interactions,star formation,supermassive black holes},
journal = {MNRAS},
number = {October},
title = {{Discovering AGN-driven winds through their infrared emission: I. General method and wind location}},
url = {http://arxiv.org/abs/1810.06562$\%$0Ahttp://dx.doi.org/10.1093/mnras/sty2935},
volume = {000},
year = {2018}
}

@article{Ozaki2009,
abstract = {We investigated the kinematic and excitation structure of the NGC 1068 narrow-line region (NLR). We obtained profiles of several emission lines ([O in] A 5007, H/$\beta$, [O I] A 6300, and [Fe VII] $\lambda$ 6087) at high-velocity resolution (R ̃ 7500-11000), and confirmed that they showed different profiles. These profiles are useful for understanding the NLR structure, since they cover a wide ionization-potential range. By comparing the results with a photoioniza-tion model, we found that: (1) blueshifted components at the center are very dense, (2) those in the northeast region have slightly lower densities than those in the center, and (3) the ionization parameters of the blueshifted components increase with increasing velocity with respect to the systemic velocity. We investigated the NLR structure in NGC 1068 based on these results. We show that both the observed velocity dependence of the ionization parameter and the gradually increasing velocity field can be reproduced by varying the ionizing continuum attenuation, assuming a hollowed biconical geometry and varying the column densities of outflowing clouds. {\textcopyright} 2009 Astronomical Society of Japan.},
archivePrefix = {arXiv},
arxivId = {0901.1704},
author = {Ozaki, Shinobu},
doi = {10.1093/pasj/61.2.259},
eprint = {0901.1704},
file = {:home/william/Documents/Papers/0901.1704.pdf:pdf},
issn = {00046264},
journal = {Publ. Astron. Soc. Japan},
keywords = {Galaxies: Seyfert,Galaxies: individual (NGC 1068),Galaxies: kinematics and dynamics},
number = {2},
pages = {259--274},
title = {{Kinematic and excitation structure of the NGC 1068 narrow-line region}},
volume = {61},
year = {2009}
}
@article{Ruffa2019,
abstract = {This is the first paper of a series exploring the multi-frequency properties of a sample of eleven nearby low excitation radio galaxies (LERGs) in the southern sky. We are conducting an extensive study of different galaxy components (stars, warm and cold gas, radio jets) with the aim of improving our understanding of the AGN fuelling/feedback cycle in LERGs. We present ALMA Band 6 {\$}{\^{}}{\{}12{\}}{\$}CO(2-1) and continuum observations of nine sources. Continuum emission from the radio cores was detected in all objects. Six sources also show mm emission from jets on kpc/sub-kpc scales. The jet structures are very similar at mm and cm wavelengths. We conclude that synchrotron emission associated with the radio jets dominates the continuum spectra up to 230 GHz. The {\$}{\^{}}{\{}12{\}}{\$}CO(2-1) line was detected in emission in six out of nine objects, with molecular gas masses ranging from {\$}2 \backslashtimes 10{\^{}}{\{}7{\}}{\$} to {\$}2 \backslashtimes 10{\^{}}{\{}10{\}}{\$} M{\$}{\_}{\{}\backslashrm \backslashodot{\}}{\$}. The CO detections show disc-like structures on scales from {\$}\backslashapprox{\$}0.2 to {\$}\backslashapprox{\$}10 kpc. In one case (NGC 3100) the CO disc presents some asymmetries and is disrupted in the direction of the northern radio jet, indicating a possible jet/disc interaction. In IC 4296, CO is detected in absorption against the radio core, as well as in emission. In four of the six galaxies with CO detections, the gas rotation axes are roughly parallel to the radio jets in projection; the remaining two cases show large misalignments. In those objects where optical imaging is available, dust and CO appear to be co-spatial.},
archivePrefix = {arXiv},
arxivId = {1901.07513},
author = {Ruffa, Ilaria and Prandoni, Isabella and Laing, Robert A. and Paladino, Rosita and Parma, Paola and de Ruiter, Hans and Mignano, Arturo and Davis, Timothy A. and Bureau, Martin and Warren, Joshua},
eprint = {1901.07513},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ruffa et al. - 2019 - The AGN fuellingfeedback cycle in nearby radio galaxies - I. ALMA observations and early results.pdf:pdf},
keywords = {active,cd,elliptical and lenticular,galaxies,ism,jets,nuclei},
number = {January},
pages = {1--25},
title = {{The AGN fuelling/feedback cycle in nearby radio galaxies - I. ALMA observations and early results}},
url = {http://arxiv.org/abs/1901.07513},
volume = {25},
year = {2019}
}
@article{Leao2008,
abstract = {Considering that the main source of turbulence in the ISM medium are the explosions of supernovae (SNe), we explore here the role of SN shock front interactions with clouds on the star formation triggering in presence and in absence of magnetic field.},
archivePrefix = {arXiv},
arxivId = {0810.5374},
author = {Le{\~{a}}o, M. R. M. and {de Gouveia Dal Pino}, E. M. and Falceta-Gon{\c{c}}alves, D. and Melioli, C. and Geraissate, F. G.},
doi = {10.1017/s1743921309030191},
eprint = {0810.5374},
file = {:home/william/Documents/Papers/0810.5374.pdf:pdf},
issn = {1743-9213},
journal = {Proc. Int. Astron. Union},
keywords = {clouds,from laboratory and stars,ism,magnetic fields,magnetics fields in the,star,star formation,supernova remnant,to appear in,to the primordial structure,universe ii},
number = {S259},
pages = {105--106},
title = {{Local star formation triggered by SN shocks in magnetized diffuse neutral clouds}},
volume = {4},
year = {2008}
}
@article{Tremblay2010,
abstract = {We present Hubble Space Telescope Advanced Camera for Surveys and STIS FUV/NUV/optical imaging of the radio galaxy 3C 236, whose relic ∼ 4 Mpc radio jet lobes and inner 2 kpc compact steep spectrum (CSS) radio source are evidence of multiple epochs of active galactic nucleus (AGN) activity. Consistent with previous results, our data confirm the presence of four bright knots of FUV emission in an arc along the edge of the inner circumnuclear dust disk in the galaxy's nucleus, as well as FUV emission cospatial with the nucleus itself. We interpret these to be sites of recent or ongoing star formation. We present photometry of these knots, as well as an estimate for the internal extinction in the source using line ratios from archival ground-based spectroscopy. We estimate the ages of the knots by comparing our extinction-corrected photometry with stellar population synthesis models. We find the four knots cospatial with the dusty disk to be young, of order ∼ 107 yr old. The FUV emission in the nucleus, to which we do not expect scattered light from the AGN to contribute significantly, is likely due to an episode of star formation triggered ∼ 109 yr ago. We argue that the young ∼ 107 yr old knots stem from an episode of star formation that was roughly coeval with the event resulting in reignition of radio activity, creating the CSS source. The ∼ 109 yr old stars in the nucleus may be associated with the previous epoch of radio activity that generated the 4 Mpc relic source, before being cut off by exhaustion or interruption. The ages of the knots, considered in the context of both the disturbed morphology of the nuclear dust and the double-double morphology of the "old" and "young" radio sources, present evidence for an AGN/starburst connection that is possibly episodic in nature. We suggest that the AGN fuel supply was interrupted for ∼ 107 yr due to a minor merger event and has now been restored. The resultant nonsteady flow of gas in the disk is likely responsible for both the new episode of infall-induced star formation and also the multiple epochs of radio activity. {\textcopyright} 2010. The American Astronomical Society. All rights reserved.},
author = {Tremblay, Grant R. and O'Dea, Christopher P. and Baum, Stefi A. and Koekemoer, Anton M. and Sparks, William B. and {De Bruyn}, Ger and Schoenmakers, Arno P.},
doi = {10.1088/0004-637X/715/1/172},
file = {:home/william/Documents/Papers/[Tremblay et al.]-EPISODIC STAR FORMATION COUPLED TO REIGNITION OF RADIO ACTIVITY IN 3C 236.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {Galaxies: active,Galaxies: individual (3C 236),Galaxies: jets,Galaxies: starburst},
number = {1},
pages = {172--185},
title = {{Episodic star formation coupled to reignition of radio activity in 3C 236}},
volume = {715},
year = {2010}
}
@article{Martizzi2016,
abstract = {We use local Cartesian simulations with a vertical gravitational potential to study how supernova (SN) feedback in stratified galactic discs drives turbulence and launches galactic winds. Our analysis includes three disc models with gas surface densities ranging from Milky Way-like galaxies to gas-rich ultraluminous infrared galaxies (ULIRGs), and two different SN driving schemes (random and correlated with local gas density). In order to isolate the physics of SN feedback, we do not include additional feedback processes. We find that, in these local box calculations, SN feedback excites relatively low mass-weighted gas turbulent velocity dispersions ≈3-7 km s-1 and low wind mass loading factors $\eta$ ≲ 1 in all the cases we study. The low turbulent velocities and wind mass loading factors predicted by our local box calculations are significantly below those suggested by observations of gas-rich and rapidly star-forming galaxies; they are also in tension with global simulations of disc galaxies regulated by stellar feedback. Using a combination of numerical tests and analytic arguments, we argue that local Cartesian boxes cannot predict the properties of galactic winds because they do not capture the correct global geometry and gravitational potential of galaxies. The wind mass loading factors are in fact not well defined in local simulations because they decline significantly with increasing box height. More physically realistic calculations (e.g. including a global galactic potential and disc rotation) will likely be needed to fully understand disc turbulence and galactic outflows, even for the idealized case of feedback by SNe alone.},
archivePrefix = {arXiv},
arxivId = {1601.03399},
author = {Martizzi, Davide and Fielding, Drummond and Faucher-Gigu{\`{e}}re, Claude Andr{\'{e}} and Quataert, Eliot},
doi = {10.1093/mnras/stw745},
eprint = {1601.03399},
file = {:home/william/Documents/Papers/1601.03399.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: ISM,Galaxies: evolution,Galaxies: formation,Galaxies: general,ISM: supernova remnants,Methods: numerical},
number = {3},
pages = {2311--2326},
title = {{Supernova feedback in a local vertically stratified medium: Interstellar turbulence and galactic winds}},
volume = {459},
year = {2016}
}
@article{Koudmani2018,
abstract = {The systematic analysis of optical large-scale surveys has revealed a population of dwarf galaxies hosting AGN, which have been confirmed by X-ray follow-up observations. Recently, the MaNGA survey identified six dwarf galaxies that appear to have an AGN that is preventing on-going star formation. It is therefore timely to study the physical properties of dwarf galaxies, in particular whether the presence of an AGN can affect their evolution. Using the moving mesh code AREPO, we have investigated different models of AGN activity, ranging from simple energy-driven spherical winds to collimated, mass-loaded, bipolar outflows in high resolution simulations of isolated dwarf galaxies hosting an active black hole. Our simulations also include a novel implementation of star formation and mechanical supernova (SN) feedback. We find that AGN outflows have a small but systematic effect on the central star formation rates (SFRs) for all set-ups explored, while substantial effects on the global SFR are only obtained with strong SNe and a sustained high-luminosity AGN with an isotropic wind. This suggests that AGN feedback in dwarf galaxies is unlikely to directly regulate their global SFRs. There is, however, a significant effect on outflow properties, which are notably enhanced by the AGN to much higher outflow temperatures and velocities, in agreement with kinematic signatures from the MaNGA survey. This indicates that AGN may play an indirect role in regulating the baryon cycle in dwarf galaxies by hindering cosmic gas inflows.},
archivePrefix = {arXiv},
arxivId = {1812.04629},
author = {Koudmani, Sophie and Sijacki, Debora and Bourne, Martin A. and Smith, Matthew C.},
doi = {10.1093/mnras/stz097},
eprint = {1812.04629},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Koudmani et al. - 2018 - Fast and energetic AGN-driven outflows in simulated dwarf galaxies.pdf:pdf},
keywords = {active,dwarf,formation,galaxies,methods,numerical},
number = {January},
title = {{Fast and energetic AGN-driven outflows in simulated dwarf galaxies}},
url = {http://arxiv.org/abs/1812.04629{\%}0Ahttp://dx.doi.org/10.1093/mnras/stz097},
volume = {000},
year = {2018}
}
@article{2005A&A...444L...9M,
author = {Morganti, R and Tadhunter, C.{\~{}}N. and Oosterloo, T.{\~{}}A.},
doi = {10.1051/0004-6361:200500197},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Morganti, Tadhunter, Oosterloo - 2005 - Fast neutral outflows in powerful radio galaxies a major source of feedback in massive galaxies.pdf:pdf},
journal = {aap},
keywords = {galaxies: ISM,galaxies: active},
pages = {L9--L13},
title = {{Fast neutral outflows in powerful radio galaxies: a major source of feedback in massive galaxies}},
volume = {444},
year = {2005}
}
@article{Costa2020a,
abstract = {We present a new implementation for active galactic nucleus (AGN) feedback through small-scale, ultrafast winds in the moving-mesh hydrodynamic code arepo. The wind is injected by prescribing mass, momentum, and energy fluxes across a spherical boundary centred on a supermassive black hole according to available constraints for accretion disc winds. After sweeping-up a mass equal to their own, small-scale winds thermalize, powering energy-driven outflows with dynamics, structure, and cooling properties in excellent agreement with those of analytic wind solutions. Momentum-driven solutions do not easily occur, because the Compton cooling radius is usually much smaller than the free-expansion radius of the small-scale winds. Through various convergence tests, we demonstrate that our implementation yields wind solutions, which are well converged down to the typical resolution achieved in cosmological simulations. We test our model in hydrodynamic simulations of isolated Milky Way-mass galaxies. Above a critical AGN luminosity, initially spherical, small-scale winds power bipolar, energy-driven superwinds that break out of the galactic nucleus, flowing at speeds gt 1000 $\backslash$rm km s-1 out to sim 10 $\backslash$rm kpc. These energy-driven outflows result in moderate, but long-term, reduction in star formation, which becomes more pronounced for higher AGN luminosities and faster small-scale winds. Suppression of star formation proceeds through a rapid mode that involves the removal of the highest density, nuclear gas, and through a slower mode that effectively halts halo gas accretion. Our new implementation makes it possible to model AGN-driven winds in a physically meaningful and validated way in simulations of galaxy evolution, the interstellar medium and black hole accretion flows.},
archivePrefix = {arXiv},
arxivId = {2006.05997},
author = {Costa, Tiago and Pakmor, R{\"{u}}diger and Springel, Volker},
doi = {10.1093/mnras/staa2321},
eprint = {2006.05997},
file = {:home/william/Documents/Papers/staa2321.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {galaxies: evolution,hydrodynamics,methods: numerical,quasars: supermassive black holes,shock waves},
number = {4},
pages = {5229--5255},
title = {{Powering galactic superwinds with small-scale AGN winds}},
volume = {497},
year = {2020}
}
@article{Dalgarno,
author = {Dalgarno, A. and McCray, R. A.},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Dalgarno, McCray - Unknown - Heating and ionization of HI regions.pdf:pdf},
title = {{Heating and ionization of HI regions}}
}
@misc{Krawczynski2013,
abstract = {In this paper we give a brief review of the astrophysics of active galactic nuclei (AGNs). After a general introduction motivating the study of AGNs, we discuss our present understanding of the inner workings of the central engines, most likely accreting black holes with masses between 106 and 1010 M ⊙. We highlight recent results concerning the jets (collimated outflows) of AGNs derived from X-ray observations (Chandra) of kpc-scale jets and $\gamma$-ray observations of AGNs (Fermi, Cherenkov telescopes) with jets closely aligned with the lines of sight (blazars), and discuss the interpretation of these observations. Subsequently, we summarize our knowledge about the cosmic history of AGN formation and evolution. We conclude with a description of upcoming observational opportunities. {\textcopyright} 2013 Higher Education Press and Springer-Verlag Berlin Heidelberg.},
archivePrefix = {arXiv},
arxivId = {1301.4179},
author = {Krawczynski, Henric and Treister, Ezequiel},
booktitle = {Front. Phys.},
doi = {10.1007/s11467-013-0310-3},
eprint = {1301.4179},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Krawczynski, Treister - 2013 - Active Galactic Nuclei – the Physics of Individual Sources and the Cosmic History of Formation and Evol.pdf:pdf},
issn = {20950462},
keywords = {active galactic nuclei (AGNs),black hole accretion,cosmological evolution,relativistic jets},
number = {6},
pages = {609--629},
title = {{Active galactic nuclei - the physics of individual sources and the cosmic history of formation and evolution}},
volume = {8},
year = {2013}
}
@article{Ishibashi2018,
abstract = {Galactic outflows are now commonly observed in starburst and active galactic nuclei (AGN) host galaxies. Yet, there is no clear consensus on their physical driving mechanism(s). We have previously shown that AGN radiative feedback, driven by radiation pressure on dust, can account for the observed dynamics and energetics of galactic outflows, provided that radiation trapping is taken into account. Here we generalise our model results by explicitly considering the temporal evolution of the central AGN luminosity, and the shell mass evolution in different ambient density distributions. In the case of fixed-mass shells, the high observed values of the momentum ratio ({\$}\backslashzeta = \backslashdot{\{}p{\}}/(L/c){\$}) and energy ratio ({\$}\backslashepsilon{\_}k = \backslashdot{\{}E{\}}{\_}{\{}k{\}}/L{\$}) may be attributed to either radiation trapping or AGN luminosity decay. In contrast, for expanding shells sweeping up mass from the surrounding environment, a decay in AGN luminosity cannot account for the observed high energetics, and radiation trapping is necessarily required. Indeed, strong radiation trapping, e.g. due to high dust-to-gas ratios, can considerably boost the outflow energetics. We obtain a distinct radial dependence for the outflow energetics ({\$}\backslashzeta(r){\$}, {\$}\backslashepsilon{\_}k(r){\$}) in the case of radiation trapping and luminosity decay, which may help discriminate between the two scenarios. In this framework, the recently discovered `fossil' outflows, with anomalously high values of the energetics, may be interpreted as relics of past AGN activity. The observed outflow properties may therefore provide useful constraints on the past history of AGN activity and/or the physical conditions of the outflow launch region.},
author = {Ishibashi, W. and Fabian, A. C.},
doi = {10.1093/mnras/sty2617},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ishibashi, Fabian - 2018 - Variations on a theme of AGN-driven outflows luminosity evolution and ambient density distribution.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Black hole physics,Galaxies: active,Galaxies: evolution},
number = {4},
pages = {4522--4531},
publisher = {Oxford University Press},
title = {{Variations on a theme of AGN-driven outflows: Luminosity evolution and ambient density distribution}},
volume = {481},
year = {2018}
}
@article{McMillan2017,
abstract = {We present mass models of the Milky Way created to fit observational constraints and to be consistent with expectations from theoretical modelling. The method used to create these models is that demonstrated in our previous study, and we improve on those models by adding gas discs to the potential, considering the effects of allowing the inner slope of the halo density profile to vary, and including new observations of maser sources in the Milky Way amongst the new constraints. We provide a best-fitting model, as well as estimates of the properties of the Milky Way. Under the assumptions in our main model, we find that the Sun is R0 = 8.20 ± 0.09 kpc from the Galactic Centre, with the circular speed at the Sun being v0 = 232.8 ± 3.0 kms-1; and that the Galaxy has a total stellar mass of (54.3 ± 5.7) × 109 M⊙, a total virial mass of (1.30 ± 0.30) × 1012M⊙ and a local dark-matter density of 0.40 ± 0.04 GeV cm-3, where the quoted uncertainties are statistical. These values are sensitive to our choice of priors and constraints. We investigate systematic uncertainties, which in some cases may be larger. For example, if we weaken our prior on R0, we find it to be 7.97 ± 0.15 kpc and that v0 = 226.8 ± 4.2 kms-1.We find that most of these properties, including the local dark-matter density, are remarkably insensitive to the assumed power-law density slope at the centre of the dark-matter halo. We find that it is unlikely that the local standard of rest differs significantly from that found under assumptions of axisymmetry. We have made code to compute the force from our potential, and to integrate orbits within it, publicly available.},
archivePrefix = {arXiv},
arxivId = {1608.00971},
author = {McMillan, Paul J.},
doi = {10.1093/mnras/stw2759},
eprint = {1608.00971},
file = {:home/william/Documents/Papers/[McMillan et al.]-The mass distribution and gravitational potential of the Milky Way.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxy: fundamental parameters,Galaxy: kinematics and dynamics,Galaxy: structure,Methods: statistical},
number = {1},
pages = {76--94},
title = {{The mass distribution and gravitational potential of the Milky Way}},
volume = {465},
year = {2017}
}
@article{Nardini2018,
abstract = {Powerful outflows with a broad range of properties (such as velocity, ionization, radial scale and mass-loss rate) represent a key feature of active galactic nuclei (AGN), even more so since they have been simultaneously revealed also in individual objects. Here we revisit in a simple analytical framework the recent remarkable cases of two ultraluminous infrared quasars, IRAS F11119+3257 and Mrk 231, which allow us to investigate the physical connection between multi-phase AGN outflows across the ladder of distance from the central supermassive black hole (SMBH). We argue that any major deviations from the standard outflow propagation models might encode unique information on the past SMBH accretion history, and briefly discuss how this could help address some controversial aspects of the current picture of AGN feedback.},
archivePrefix = {arXiv},
arxivId = {1805.00040},
author = {Nardini, Emanuele and Zubovas, Kastytis},
doi = {10.1093/mnras/sty1144},
eprint = {1805.00040},
file = {:home/william/Documents/Papers/sty1144.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: active,Galaxies: evolution,ISM: jets and outflows,Quasars: general,Quasars: individual: supermassive black holes},
number = {2},
pages = {2274--2280},
publisher = {Oxford University Press},
title = {{Multi-phase outflows as probes of AGN accretion history}},
volume = {478},
year = {2018}
}
@article{2000MNRAS.314..511S,
author = {Strickland, D.{\~{}}K. and Stevens, I.{\~{}}R.},
doi = {10.1046/j.1365-8711.2000.03391.x},
file = {:home/william/Documents/Papers/2000MNRAS.314..511S.pdf:pdf},
journal = {MNRAS},
keywords = {GALAXIES: INDIVIDUAL: M82,GALAXIES: STARBURST,ISM: BUBBLES,ISM: JETS AND OUTFLOWS,METHODS: NUMERICAL,X-RAYS: GALAXIES},
pages = {511--545},
title = {{Starburst-driven galactic winds - I. Energetics and intrinsic X-ray emission}},
volume = {314},
year = {2000}
}
@article{DeGouveiadalPino1995,
abstract = {After a summary of the observations of cosmic magnetic fields, I briefly discuss the status of dynamos, the use of electric circuits, the physics of magnetic explosions, the role of magnetic tension and our strongest magnet known, the radio pulsar. Finally I mention a few problem areas which may show a breakthrough in the near future. {\textcopyright} 1995.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0603065},
author = {{de Gouveia dal Pino}, Elisabete M},
doi = {10.1016/0921-4526(94)01048-6},
eprint = {0603065},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/de Gouveia dal Pino - 1995 - Cosmic magnetic fields.pdf:pdf},
isbn = {0735403759},
issn = {09214526},
journal = {Phys. B Phys. Condens. Matter},
keywords = {-b,-r,10,12,35,38,52,54,58,62,65,80,96,97,98,and in the early,bp,clusters of galaxies,cm,dq,eg,en,fs,galaxies,gz,hb,hg,interstellar medium,intracluster and inter-galactic medium,jets and accretion disks,kh,ld,magnetic fields in,mj,pacs,stars,universe},
number = {1-4},
pages = {306--315},
primaryClass = {astro-ph},
title = {{Cosmic magnetic fields}},
volume = {211},
year = {1995}
}
@article{Pereira-Santaella2018a,
abstract = {We present new CO(2-1) observations of three low-z (d ∼350 Mpc) ultra-luminous infrared galaxy (ULIRG) systems (six nuclei) observed with the Atacama large millimeter/submillimeter array (ALMA) at high spatial resolution (∼500 pc). We detect massive cold molecular gas outflows in five out of six nuclei (Mout ∼ (0.3-5) × 108 M⊙). These outflows are spatially resolved with deprojected effective radii between 250 pc and 1 kpc although high-velocity molecular gas is detected up to Rmax ∼ 0.5-1.8 kpc (1-6 kpc deprojected). The mass outflow rates are 12-400 M⊙ yr-1 and the inclination corrected average velocity of the outflowing gas is 350-550 km s-1 (vmax = 500-900 km s-1). The origin of these outflows can be explained by the strong nuclear starbursts although the contribution of an obscured active galactic nucleus cannot be completely ruled out. The position angle (PA) of the outflowing gas along the kinematic minor axis of the nuclear molecular disk suggests that the outflow axis is perpendicular to the disk for three of these outflows. Only in one case is the outflow PA clearly not along the kinematic minor axis, which might indicate a different outflow geometry. The outflow depletion times are 15-80 Myr. These are comparable to, although slightly shorter than, the star-formation (SF) depletion times (30-80 Myr). However, we estimate that only 15-30{\%} of the outflowing molecular gas will escape the gravitational potential of the nucleus. The majority of the outflowing gas will return to the disk after 5-10 Myr and become available to form new stars. Therefore, these outflows will not likely completely quench the nuclear starbursts. These star-forming powered molecular outflows would be consistent with being driven by radiation pressure from young stars (i.e., momentum-driven) only if the coupling between radiation and dust increases with increasing SF rates. This can be achieved if the dust optical depth is higher in objects with higher SF. This is the case in at least one of the studied objects. Alternatively, if the outflows are mainly driven by supernovae (SNe), the coupling efficiency between the interstellar medium and SNe must increase with increasing SF levels. The relatively small sizes ({\textless}1 kpc) and dynamical times ({\textless}3 Myr) of the cold molecular outflows suggests that molecular gas cannot survive longer in the outflow environment or that it cannot form efficiently beyond these distances or times. In addition, the ionized and hot molecular phases have been detected for several of these outflows, so this suggests that outflowing gas can experience phase changes and indicates that the outflowing gas is intrinsically multiphase, likely sharing similar kinematics, but different mass and, therefore, different energy and momentum contributions.},
archivePrefix = {arXiv},
arxivId = {1805.03667},
author = {Pereira-Santaella, M. and Colina, L. and Garc{\'{i}}a-Burillo, S. and Combes, F. and Emonts, B. and Aalto, S. and Alonso-Herrero, A. and Arribas, S. and Henkel, C. and Labiano, A. and Muller, S. and {Piqueras L{\'{o}}pez}, J. and Rigopoulou, D. and {Van Der Werf}, P.},
doi = {10.1051/0004-6361/201833089},
eprint = {1805.03667},
file = {:home/william/Documents/Papers/aa33089-18.pdf:pdf},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Galaxies: ISM,Galaxies: active,Galaxies: kinematics and dynamics,Galaxies: nuclei,Galaxies: starburst},
pages = {1--20},
title = {{Spatially resolved cold molecular outflows in ULIRGs}},
volume = {616},
year = {2018}
}
@article{Tombesi2015a,
abstract = {Powerful winds driven by active galactic nuclei are often thought to affect the evolution of both supermassive black holes and their host galaxies, quenching star formation and explaining the close relationship between black holes and galaxies. Recent observations of large-scale molecular outflows in ultraluminous infrared galaxies support this quasar-feedback idea, because they directly trace the gas from which stars form. Theoretical models suggest that these outflows originate as energy-conserving flows driven by fast accretion-disk winds. Proposed connections between large-scale molecular outflows and accretion-disk activity in ultraluminous galaxies were incomplete because no accretion-disk wind had been detected. Conversely, studies of powerful accretion-disk winds have until now focused only on X-ray observations of local Seyfert galaxies and a few higher-redshift quasars. Here we report observations of a powerful accretion-disk wind with a mildly relativistic velocity (a quarter that of light) in the X-ray spectrum of IRAS F11119+3257, a nearby (redshift 0.189) optically classified type 1 ultraluminous infrared galaxy hosting a powerful molecular outflow. The active galactic nucleus is responsible for about 80 per cent of the emission, with a quasar-like luminosity of 1.5 × 10(46) ergs per second. The energetics of these two types of wide-angle outflows is consistent with the energy-conserving mechanism that is the basis of the quasar feedback in active galactic nuclei that lack powerful radio jets (such jets are an alternative way to drive molecular outflows).},
archivePrefix = {arXiv},
arxivId = {1501.07664},
author = {Tombesi, F and Mel{\'{e}}ndez, M. and Veilleux, S and Reeves, J N and Gonz{\'{a}}lez-Alfonso, E. and Reynolds, C S},
doi = {10.1038/nature14261},
eprint = {1501.07664},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Tombesi et al. - 2015 - Wind from the black-hole accretion disk driving a molecular outflow in an active galaxy.pdf:pdf},
isbn = {9780874216561},
issn = {14764687},
journal = {Nature},
number = {7544},
pages = {436--438},
pmid = {25810204},
title = {{Wind from the black-hole accretion disk driving a molecular outflow in an active galaxy}},
volume = {519},
year = {2015}
}
@article{Tampo2020,
abstract = {We report photometric and spectroscopic observations and analysis of the 2019 superout- burst of TCP J21040470+4631129. This object showed a 9-mag superoutburst with early superhumps and ordinary superhumps, which are the features of WZ Sge-type dwarf novae. Five rebrightenings were observed after the main superoutburst. The spectra during the post- superoutburst stage showed the Balmer, He I and possible sodium doublet features. The mass ratio is derived as 0.0880(9) from the period of the superhump. During the third and fifth re- brightenings, growing superhumps and superoutbursts were observed, which have never been detected during a rebrightening phase among WZ Sge-type dwarf novae with multiple rebright- enings. To induce a superoutburst during the brightening phase, the accretion disk was needed to expand beyond the 3:1 resonance radius of the system again after the main superoutburst.These peculiar phenomena can be explained by the enhanced viscosity and large radius of the disk suggested by the higher luminosity and the presence of late-stage superhumps during the post-superoutburst stage, plus by more mass supply from the cool mass reservoir and/or from the secondary because of the enhanced mass transfer than those of other WZ Sge-type dwarf novae.},
archivePrefix = {arXiv},
arxivId = {arXiv:2004.10508v1},
author = {Tampo, Yusuke and Kojiguchi, Naoto and Isogai, Keisuke and Kato, Taichi and Kimura, Mariko and Wakamatsu, Yasuyuki and Nogami, Daisaku},
doi = {10.1093/pasj/xxx000},
eprint = {arXiv:2004.10508v1},
file = {:home/william/Documents/Papers/1901.05618.pdf:pdf},
journal = {Publ. Astron. Soc. Japan},
keywords = {accretion,accretion disks-stars: novae,cataclysmic variables-stars: dwarf novae-stars: in},
number = {0},
pages = {1--6},
title = {{First Detection of Two Superoutbursts during Rebrightening Phase of a WZ Sge-type Dwarf Nova: TCP J21040470+4631129}},
url = {http://www.aavso.org/data-download},
volume = {00},
year = {2020}
}
@article{Nakamura2004,
abstract = {Non-relativistic three-dimensional magnetohydrodynamic simulations of Poynting-flux-dominated (PFD) jets are presented. Our study focuses on the propagation of strongly magnetized hypersonic but sub-Alfv{\'{e}}nic flow (Cs2 {\textless}{\textless} Vjet2 {\textless} VA2) and the development of a current-driven (CD) kink instability. This instability may be responsible for the "wiggled" structures seen in VLBI-scale AGN jets. In the present paper we investigate the nonlinear behavior of PFD jets in a variety of external ambient magnetized gas distributions, including those with density, pressure, and temperature gradients. Our numerical results show that PFD jets can develop kink distortions in the trans-Alfv{\'{e}}nic flow case, even when the flow itself is still strongly magnetically dominated. In the nonlinear development of the instability, a non-axisymmetric mode grows on time scales of order the Alfv{\'{e}}n crossing time (in the jet frame) and proceeds to disrupt the kinematic and magnetic structure of the jet. Because of a large scale poloidal magnetic field in the ambient medium, the growth of surface modes (i.e., MHD Kelvin-Helmholtz instabilities) is suppressed. The CD kink mode (m = 1) grows faster than the other higher order modes (m {\textgreater} 1), driven in large part by the radial component of the Lorentz force.},
archivePrefix = {arXiv},
arxivId = {arXiv:astro-ph/0312055v1},
author = {Nakamura, M. and Meier, D. L.},
doi = {10.1063/1.1718472},
eprint = {0312055v1},
file = {:home/william/Documents/Papers/3-D{\_}Simulations{\_}of{\_}MHD{\_}Jets{\_}-{\_}The{\_}Stability{\_}Proble.pdf:pdf},
isbn = {0735401764},
issn = {15517616},
journal = {AIP Conf. Proc.},
number = {December 2003},
pages = {308--313},
primaryClass = {arXiv:astro-ph},
title = {{3-D simulations of MHD Jets - The stability problem}},
volume = {703},
year = {2004}
}
@article{Silpa2021,
abstract = {We present the results of a multi-frequency, multi-scale radio polarimetric study with the Very Large Array (VLA) of the Seyfert 1 galaxy and BALQSO, Mrk 231. We detect complex total and polarized intensity features in the source. Overall, the images indicate the presence of a broad, one-sided, curved outflow towards the south which consists of a weakly collimated jet with poloidal inferred magnetic fields, inside a broader magnetized “wind” or “sheath” component with toroidal inferred magnetic fields. The model of a kpc-scale weakly collimated jet/lobe in Mrk 231 is strengthened by its C-shaped morphology, steep spectral index throughout, complexities in the magnetic field structures, and the presence of self-similar structures observed on the 10-parsec-scale in the literature. The “wind” may comprise both nuclear starburst (close to the core) and AGN winds, where the latter maybe the primary contributor. Moving away from the core, the “wind” component may also comprise the outer layers (or “sheath”) of a broadened jet. The inferred value of the (weakly collimated) jet production efficiency, $\eta$jet ∼ 0.01 is consistent with the estimates in the literature. The composite jet and wind outflow in Mrk 231 appears to be low-power and matter-dominated, and oriented at a small angle to our line of sight.},
archivePrefix = {arXiv},
arxivId = {2107.09466},
author = {Silpa, S and Kharb, P and O'Dea, C P and Baum, S A and Sebastian, B and Mukherjee, D and Harrison, C M},
doi = {10.1093/mnras/stab2110},
eprint = {2107.09466},
file = {:home/william/Documents/Papers/2107.09466.pdf:pdf},
issn = {0035-8711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {galaxies,general,individual,mrk 231,polarimetric,quasars,radio continuum,techniques},
number = {July},
pages = {1--12},
title = {{AGN jets and winds in polarised light: The case of Mrk 231}},
volume = {12},
year = {2021}
}
@article{Nawaz2016a,
abstract = {We present three dimensional relativistic hydrodynamical simulations of a precessing jet interacting with the intracluster medium and compare the simulated jet structure with the observed structure of the Hydra A northern jet. For the simulations, we use jet parameters obtained in the parameter space study of the first paper in this series and probe different values for the precession period and precession angle. We find that for a precession period P = 1 Myr and a precession angle = 20 degree the model reproduces i) the curvature of the jet, ii) the correct number of bright knots within 20 kpc at approximately correct locations, and iii) the turbulent transition of the jet to a plume. The Mach number of the advancing bow shock = 1.85 is indicative of gentle cluster atmosphere heating during the early stages of the AGN's activity.},
author = {Nawaz, M. A. and Bicknell, G. V. and Wagner, A. Y. and Sutherland, R. S. and McNamara, B. R.},
doi = {10.1093/mnras/stw330},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Nawaz et al. - 2016 - Jet-intracluster medium interaction in hydra A - II. The effect of jet precession.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: active,Galaxies: clusters: individual: Hydra A,Galaxies: clusters: intracluster medium,Galaxies: jets},
number = {1},
pages = {802--815},
title = {{Jet-intracluster medium interaction in hydra A - II. The effect of jet precession}},
volume = {458},
year = {2016}
}
@article{Crenshaw2015,
abstract = {We present a detailed study of AGN feedback in the narrow-line region (NLR) of the Seyfert 1 galaxy NGC 4151. We illustrate the data and techniques needed to determine the mass outflow rate and kinetic luminosity of the outflowing ionized gas as a function of position in the NLR. We find that the mass outflow rate peaks at a value of 3 solar masses per year at a distance of 70 pc from the central supermassive black hole (SMBH), which is about 10 times the outflow rate coming from inside 13 pc, and 230 times the mass accretion rate inferred from the bolometric luminosity of NGC 4151. Thus, most of the outflow must arise from "in situ" acceleration of ambient gas throughout the NLR. The kinetic luminosity peaks at 90 pc and drops rapidly thereafter, indicating that most of the kinetic energy is deposited within about 100 pc from the SMBH. Both values exceed the mass outflow rate and kinetic luminosity determined for the UV/X-ray absorber outflows in NGC 4151, indicating the importance of NLR outflows in providing feedback on scales where circumnuclear star formation and bulge growth occur.},
archivePrefix = {arXiv},
arxivId = {1411.4507},
author = {Crenshaw, D. Michael and Fischer, Travis C. and Kraemer, Steven B. and Schmitt, Henrique R.},
doi = {10.1088/0004-637X/799/1/83},
eprint = {1411.4507},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Crenshaw et al. - 2015 - Feedback from mass outflows in nearby active galactic nuclei. II. Outflows in the narrow-line region of NGC 415.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {Galaxies: Seyfert,Galaxies: active,Galaxies: individual (NGC 4151),Galaxies: kinematics and dynamics},
number = {1},
pages = {1--6},
title = {{Feedback from mass outflows in nearby active galactic nuclei. II. Outflows in the narrow-line region of NGC 4151}},
volume = {799},
year = {2015}
}
@article{Duran2016,
abstract = {Relativistic jets in active galactic nuclei (AGN) convert as much as half of their energy into radiation. To explore the poorly understood processes that are responsible for this conversion, we carry out fully 3D magnetohydrodynamic (MHD) simulations of relativistic magnetized jets. Unlike the standard approach of injecting the jets at large radii, our simulated jets self-consistently form at the source and propagate and accelerate outward for several orders of magnitude in distance before they interact with the ambient medium. We find that this interaction can trigger strong energy dissipation of two kinds inside the jets, depending on the properties of the ambient medium. Those jets that form in a new outburst and drill a fresh hole through the ambient medium fall victim to a 3D magnetic kink instability and dissipate their energy primarily through magnetic reconnection in the current sheets formed by the instability. On the other hand, those jets that form during repeated cycles of AGN activity and escape through a pre-existing hole in the ambient medium maintain their stability and dissipate their energy primarily at MHD recollimation shocks. In both cases the dissipation region can be associated with a change in the density profile of the ambient gas. The Bondi radius in AGN jets serves as such a location.},
archivePrefix = {arXiv},
arxivId = {1612.06929},
author = {Duran, Rodolfo Barniol and Tchekhovskoy, Alexander and Giannios, Dimitrios},
doi = {10.1093/mnras/stx1165},
eprint = {1612.06929},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Duran, Tchekhovskoy, Giannios - 2016 - Three-dimensional Simulations of AGN Jets Magnetic Kink Instability versus Conical Shocks.pdf:pdf},
keywords = {active,galaxies,instabilities,jets,magnetic fields,mhd},
number = {June},
title = {{Three-dimensional Simulations of AGN Jets: Magnetic Kink Instability versus Conical Shocks}},
url = {http://arxiv.org/abs/1612.06929{\%}0Ahttp://dx.doi.org/10.1093/mnras/stx1165},
volume = {000},
year = {2016}
}
@article{Combes2017b,
abstract = {In the last decade, observations have accumulated on gas outflows in galaxies, and in particular massive molecular ones. The mass outflow rate is estimated between 1 and 5 times the star formation rate. For the highest maximal velocities, they are driven by AGN; these outflows are therefore a clear way to moderate or suppress star formation. Some of the most convincing examples at low redshift come from the radio mode, when the radio jets are inclined toward the galaxy plane, or expand in the hot intra-cluster medium, in cool core clusters. However, AGN feedback can also be positive in many occasions, and the net effect is difficult to evaluate. The quenching efficiency is discussed in view of recent observations.},
author = {Combes, Francoise},
doi = {10.3389/fspas.2017.00010},
file = {:home/william/Documents/Papers/fspas-04-00010.pdf:pdf},
issn = {2296987X},
journal = {Front. Astron. Sp. Sci.},
keywords = {active galaxy nuclei,black holes,galaxies,molecules,outflows},
number = {September},
pages = {1--5},
title = {{AGN Feedback and Its Quenching Efficiency}},
volume = {4},
year = {2017}
}
@article{Zhang2019,
abstract = {We calculate the spectrum of escaping cosmic rays (CRs) accelerated in the shocks produced by expanding galactic superbubbles powered by supernovae producing a continuous energy outflow in star-forming galaxies. We solve the generalized Kompaneets equations adapted to expansion in various external density profiles including exponential and power-law shapes, and take into account that escaping CRs are dominated by those around their maximum energies. We find that the escaping CR spectrum largely depends on the specific density profiles and power source properties, and the results are compared to and constrained by the observed CR spectrum. As a particular case we apply the results to the Milky Way's Fermi Bubbles, and find that the Fermi Bubbles' CRs in our model could explain the observed CR flux and spectrum around the second knee at {\$}10{\^{}}{\{}17{\}}{\$} eV. At the same time, our model can also explain the microwave haze observed by {\$}\backslashtextit{\{}WMAP{\}}{\$} and {\$}\backslashtextit{\{}Planck{\}}{\$}, as well as the {\$}\backslashsim{\$} 10 GeV gamma-rays observed by {\$}\backslashtextit{\{}Fermi{\}}{\$}-LAT.},
archivePrefix = {arXiv},
arxivId = {1904.02333},
author = {Zhang, Zhaowei and Murase, Kohta and M{\'{e}}sz{\'{a}}ros, Peter},
eprint = {1904.02333},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Zhang, Murase, M{\'{e}}sz{\'{a}}ros - 2019 - Cosmic Rays Escaping from Galactic Starburst-Driven Superbubbles and Application to the Fermi Bubbles.pdf:pdf},
keywords = {acceleration of particles,astroparticle physics,bubbles,cosmic rays,fermi bubbles,individual objects,ism,kinematics and dynamics},
number = {Kompaneets 1960},
pages = {1--16},
title = {{Cosmic Rays Escaping from Galactic Starburst-Driven Superbubbles and Application to the Fermi Bubbles}},
url = {http://arxiv.org/abs/1904.02333},
year = {2019}
}
@article{316,
author = {ربه, ابن عبد},
file = {:home/william/Documents/Papers/1999ASPC..187..115B.pdf:pdf},
pages = {400},
title = {{No Title العقد الفريد}},
year = {316}
}
@article{King2011,
abstract = {We discuss massive outflows in galaxy bulges, particularly the ones driven by accretion episodes where the central supermassive black hole reaches the Eddington limit. We show that the quasar radiation field Compton-cools the wind shock until this reaches distances {\~{}}1kpc from the black hole, but becomes too dilute to do this at larger radii. Radiative processes cannot cool the shocked gas within the flow time at any radius. Outflows are therefore momentum driven at small radii (as required to explain theM-$\sigma$ relation). At large radii, they are energy driven, contrary to recent claims. We solve analytically the motion of an energy-driven shell after the central source has turned off. This shows that the thermal energy in the shocked wind can drive further expansion for a time {\~{}}10 times longer than the active time of the central source. Outflows observed at large radii with no active central source probably result from an earlier short (few Myr) active phase of this source. {\textcopyright} 2011 The Authors Monthly Notices of the Royal Astronomical Society {\textcopyright} 2011 RAS.},
author = {King, A R and Zubovas, K and Power, C},
doi = {10.1111/j.1745-3933.2011.01067.x},
file = {:home/william/Documents/Papers/415-1-L6.pdf:pdf},
issn = {17453933},
journal = {Mon. Not. R. Astron. Soc. Lett.},
keywords = {Accretion,Black hole physics,Galaxies: evolution,Quasars: general,accretion discs},
number = {1},
pages = {6--10},
title = {{Large-scale outflows in galaxies}},
volume = {415},
year = {2011}
}
@article{Padovani2017,
abstract = {AGN are quite unique astronomical sources emitting over more than 20 orders of magnitude in frequency, with different electromagnetic bands providing windows on different sub-structures and their physics. They come in a large number of flavors only partially related to intrinsic differences. I highlight here the types of sources selected in different bands, the relevant selection effects and biases, and the underlying physical processes. I then look at the “big picture” by describing the most important parameters one needs to describe the variety of AGN classes and by discussing AGN at all frequencies in terms of their sky surface density. I conclude with a look at the most pressing open issues and the main new facilities, which will flood us with new data to tackle them.},
author = {Padovani, Paolo},
doi = {10.3389/fspas.2017.00035},
file = {:home/william/Documents/Papers/fspas-04-00035.pdf:pdf},
issn = {2296987X},
journal = {Front. Astron. Sp. Sci.},
keywords = {X-ray emission,active galactic nuclei,infrared emission,quasars,radio emission,supermassive black holes,$\gamma$-ray emission},
number = {November},
pages = {1--7},
title = {{Active Galactic Nuclei at All Wavelengths and from All Angles}},
volume = {4},
year = {2017}
}
@article{Scoville2000,
abstract = {We present near-infrared images obtained with the Hubble Space Telescope NICMOS camera for a sample of nine luminous [LIGs: LIR(8-1000 $\mu$m){\textgreater}=1011 Lsolar] and 15 ultraluminous (ULIGS: LIR{\textgreater}=1012 Lsolar) infrared galaxies. The sample includes representative systems classified as warm (f25$\mu$m/f60$\mu$m{\textgreater}0.2) and cold (f25$\mu$m/f60$\mu$m{\textless}=0.2) based on the mid-infrared colors and systems with nuclear emission lines classified as H II (i.e., starburst), QSO, Seyfert, and LINER. The morphologies of the sample galaxies are diverse and provide further support for the idea that they are created by the collision or interactions of spiral galaxies. Although no new nuclei are seen in the NICMOS images, the NICMOS images do reveal new spiral structures, bridges, and circumnuclear star clusters. The colors and the luminosities of the observed clusters are consistent with them being young (107-108 yr), formed as a result of galactic interactions, and having masses much greater than those of Galactic globular clusters. In NGC 6090 and VV 114, they are preferentially situated along the area of overlap of the two galactic disks. With the exception of IR 17208-0018, all of the ULIGs have at least one compact (2.2 $\mu$m FWHM{\textless}=200 pc) nucleus. Analysis of the near-infrared colors (i.e., m1.1-1.6 vs. m1.6-2.2) derived from 1.1" diameter apertures suggests that the warm galaxies have near-infrared colors consistent with QSO+hot dust emission and the cold galaxies, as a group, have near-infrared colors consistent with reddened starlight. In addition, the cold ULIG UGC 5101 (and possibly three others) have near-infrared colors suggesting additional active galactic nucleus-like near-infrared components in their nuclei. In a 2 kpc diameter aperture measurement, the global colors of all of the cold galaxies except UGC 5101 are consistent with starlight with a few magnitudes of visual extinction. The general dichotomy of the near-infrared properties of the warm and the cold galaxies are further supported by the light distributions: seven of the eight warm galaxies have unresolved nuclear emission that contributes significantly (i.e., {\textgreater}=30{\%}-40{\%}) to the total near-infrared luminosity. The smooth, more extended light observed in all of the galaxies is most likely composed of giant and supergiant stars, but evidence at longer wavelengths suggests that these stars contribute little to the high 8-1000 $\mu$m luminosity of these galaxies. Finally, light profiles of nine of the 24 systems were fitted well by an r1/4 law (and not so well by an exponential disk profile). Whether these star systems eventually become massive central bulges or giant elliptical galaxies will depend on how efficiently the present ISM is converted into stars.},
author = {Scoville, N. Z. and Evans, A. S. and Thompson, R. and Rieke, M. and Hines, D. C. and Low, F. J. and Dinshaw, N. and Surace, J. A. and Armus, L.},
doi = {10.1086/301248},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Coville - 2000 - Nicmos imaging of infrared-luminous galaxies n. z. s coville.pdf:pdf},
issn = {00046256},
journal = {Astron. J.},
keywords = {active {\`{e}} galaxies,galaxies,interactions {\`{e}} galaxies,ism {\`{e}} galaxies,starburst},
number = {3},
pages = {991--1061},
title = {{NICMOS Imaging of Infrared-Luminous Galaxies}},
volume = {119},
year = {2000}
}
@article{Voit2020,
abstract = {Star formation in the universe's most massive galaxies proceeds furiously early in time but then nearly ceases. Plenty of hot gas remains available but does not cool and condense into star-forming clouds. Active galactic nuclei (AGN) release enough energy to inhibit cooling of the hot gas, but energetic arguments alone do not explain why quenching of star formation is most effective in high-mass galaxies. In fact, optical observations show that quenching is more closely related to a galaxy's central stellar velocity dispersion ({\$}\backslashsigma{\_}v{\$}) than to any other characteristic. Here, we show that high {\$}\backslashsigma{\_}v{\$} is critical to quenching because a deep central potential well maximizes the efficacy of AGN feedback. In order to remain quenched, a galaxy must continually sweep out the gas ejected from its aging stars. Supernova heating can accomplish this task as long as the AGN sufficiently reduces the gas pressure of the surrounding circumgalactic medium (CGM). We find that CGM pressure acts as the control knob on a valve that regulates AGN feedback and suggest that feedback power self-adjusts so that it suffices to lift the CGM out of the galaxy's potential well. Supernova heating then drives a galactic outflow that remains homogeneous if {\$}\backslashsigma{\_}v \backslashgtrsim 240 \backslash, {\{}\backslashrm km \backslash, s{\^{}}{\{}-1{\}}{\}}{\$}. AGN feedback can effectively quench galaxies with a comparable velocity dispersion, but feedback in galaxies with a much lower velocity dispersion tends to result in convective circulation and accumulation of multiphase gas within the galaxy.},
archivePrefix = {arXiv},
arxivId = {2006.09381},
author = {Voit, G. M. and Bryan, G. L. and Prasad, D. and Frisbie, R. and Li, Y. and Donahue, M. and O'Shea, B. W. and Sun, M. and Werner, N.},
eprint = {2006.09381},
file = {:home/william/Documents/Papers/2006.09381.pdf:pdf},
keywords = {galaxies,halos,intergalactic medium,ism},
title = {{A Black-Hole Feedback Valve in Massive Galaxies}},
url = {http://arxiv.org/abs/2006.09381},
year = {2020}
}
@article{Zubovas2017,
author = {Zubovas, Kastytis},
doi = {10.1038/s41550-017-0093},
file = {:home/william/Documents/Papers/zubovas2017.pdf:pdf},
issn = {23973366},
journal = {Nat. Astron.},
number = {April},
pages = {1--2},
publisher = {Macmillan Publishers Limited},
title = {{Galaxy evolution: Let there be stars}},
url = {http://dx.doi.org/10.1038/s41550-017-0093},
volume = {1},
year = {2017}
}
@article{Tadhunter2014a,
abstract = {Massive outflows driven by active galactic nuclei are widely recognized to have a key role in the evolution of galaxies, by heating the ambient gas, expelling it from the nuclear regions, and thereby affecting the star-formation histories of the galaxy bulges. It has been proposed that the powerful jets of relativistic particles (such as electrons) launched by some active nuclei can both accelerate and heat the molecular gas, which often dominates the mass budgets of the outflows. Clear evidence for this mechanism, in the form of detailed associations between the molecular gas kinematics and features in the radio-emitting jets, has however been lacking. Here we report that the warm molecular hydrogen gas in the western radio lobe of the Seyfert galaxy IC 5063 is moving at high velocities-up to about 600 kilometres per second-relative to the galaxy disk. This suggests that the molecules have been accelerated by fast shocks driven into the interstellar medium by the expanding radio jets. These results demonstrate the general feasibility of accelerating molecular outflows in fast shocks driven by active nuclei.},
archivePrefix = {arXiv},
arxivId = {1407.1332},
author = {Tadhunter, C. and Morganti, R. and Rose, M. and Oonk, J. B.R. and Oosterloo, T.},
doi = {10.1038/nature13520},
eprint = {1407.1332},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Tadhunter et al. - 2014 - Jet acceleration of the fast molecular outflows in the Seyfert galaxy IC 5063.pdf:pdf},
isbn = {0028-0836},
issn = {14764687},
journal = {Nature},
number = {7510},
pages = {440--443},
pmid = {25043049},
publisher = {Nature Publishing Group},
title = {{Jet acceleration of the fast molecular outflows in the Seyfert galaxy IC 5063}},
url = {http://dx.doi.org/10.1038/nature13520},
volume = {511},
year = {2014}
}
@article{Lamastra2019,
abstract = {Several observations are revealing the widespread occurrence of mildly relativistic wide-angle AGN winds strongly interacting with the gas of their host galaxy. Such winds are potential cosmic-ray accelerators, as supported by gamma-ray observations of the nearby Seyfert galaxy NGC 1068 with the Fermi gamma-ray space telescope. The non-thermal emission produced by relativistic particles accelerated by the AGN-driven wind observed in the circum-nuclear molecular disk of such galaxy is invoked to produce the gamma-ray spectrum. The AGN wind model predicts a hard spectrum that extend in the very high energy band which differs significantly from those corresponding to other models discussed in the literature, like starburst or AGN jet. We present dedicated simulations of observations through the Cherenkov Telescope Array (CTA), the next-generation ground based gamma-ray observatory, of the very high energy spectrum of the Seyfert galaxy NGC 1068 assuming the AGN wind and the AGN jet models. We demonstrate that, considering 50 hours of observations, CTA can be effectively used to constrain the two different emission models, providing important insight into the physics governing the acceleration of particles in non-relativistic AGN-driven outflows. This analysis strongly motivates observations of Seyfert and starburst galaxies with CTA in order to test source population models of the extragalactic gamma-ray and neutrino backgrounds.},
archivePrefix = {arXiv},
arxivId = {1904.06918},
author = {Lamastra, Alessandra and Tavecchio, Fabrizio and Romano, Patrizia and Landoni, Marco and Vercellone, Stefano},
doi = {10.1016/j.astropartphys.2019.04.003},
eprint = {1904.06918},
file = {:home/william/Documents/Papers/1-s2.0-S0927650519300362-main.pdf:pdf},
issn = {09276505},
journal = {Astropart. Phys.},
keywords = {Galaxies,Gamma rays,Individual,NGC 1068,Seyfert},
pages = {16--23},
publisher = {Elsevier B.V.},
title = {{Unveiling the origin of the gamma-ray emission in NGC 1068 with the Cherenkov Telescope Array}},
url = {https://doi.org/10.1016/j.astropartphys.2019.04.003},
volume = {112},
year = {2019}
}
@article{Asahina2017a,
abstract = {{\textcopyright} 2017. The American Astronomical Society. All rights reserved. By performing three-dimensional magnetohydrodynamics simulations of subrelativistic jets and disk winds propagating into the magnetized inhomogeneous interstellar medium (ISM), we investigate the magnetic effects on the active galactic nucleus feedback. Our simulations reveal that the magnetic tension force promotes the acceleration of the dense gas clouds, since the magnetic field lines, which are initially straight, bend around the gas clouds. In the jet models, the velocity dispersion of the clouds increases with an increase in the initial magnetic fields. The increment of the kinetic energy of the clouds is proportional to the initial magnetic fields, implying that the magnetic tension force increases the energy conversion efficiency from the jet to the gas clouds. Through simulations of the mildly collimated disk wind and the funnel-shaped disk wind, we confirm that such an enhancement of the energy conversion efficiency via the magnetic fields appears even if the energy is injected via the disk winds. The enhancement of the acceleration of the dense part of the magnetized ISM via the magnetic tension force will occur wherever the magnetized inhomogeneous matter is blown away.},
author = {Asahina, Yuta and Nomura, Mariko and Ohsuga, Ken},
doi = {10.3847/1538-4357/aa6c5f},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Asahina, Nomura, Ohsuga - 2017 - Enhancement of Feedback Efficiency by Active Galactic Nucleus Outflows via the Magnetic Tension Force i.pdf:pdf},
issn = {1538-4357},
journal = {Astrophys. J.},
keywords = {ISM: clouds,ISM: jets and outflows,magnetohydrodyn,clouds,ism,jets and out fl,magnetohydrodynamics,mhd,ows,shock waves},
number = {1},
pages = {25},
publisher = {IOP Publishing},
title = {{Enhancement of Feedback Efficiency by Active Galactic Nucleus Outflows via the Magnetic Tension Force in the Inhomogeneous Interstellar Medium}},
url = {http://dx.doi.org/10.3847/1538-4357/aa6c5f},
volume = {840},
year = {2017}
}
@article{Banda-Barragan2018,
abstract = {We present a set of numerical experiments designed to systematically investigate how turbulence and magnetic fields influence the morphology, energetics, and dynamics of filaments produced in wind-cloud interactions. We cover 3D, magnetohydrodynamic systems of supersonic winds impacting clouds with turbulent density, velocity, and magnetic fields. We find that lognormal density distributions aid shock propagation through clouds, increasing their velocity dispersion and producing filaments with expanded cross-sections and highly magnetized knots and subfilaments. In self-consistently turbulent scenarios, the ratio of filament to initial cloud magnetic energy densities is {\~{}}1. The effect of Gaussian velocity fields is bound to the turbulence Mach number: Supersonic velocities trigger a rapid cloud expansion; subsonic velocities only have a minor impact. The role of turbulent magnetic fields depends on their tension and is similar to the effect of radiative losses: the stronger the magnetic field or the softer the gas equation of state, the greater the magnetic shielding at wind-filament interfaces and the suppression of Kelvin-Helmholtz instabilities. Overall, we show that including turbulence and magnetic fields is crucial to understanding cold gas entrainment in multiphase winds. While cloud porosity and supersonic turbulence enhance the acceleration of clouds, magnetic shielding protects them from ablation and causes Rayleigh-Taylor-driven subfilamentation. Wind-swept clouds in turbulent models reach distances {\~{}}15-20 times their core radius and acquire bulk speeds {\~{}}0.3-0.4 of the wind speed in one cloud-crushing time, which are three times larger than in non-turbulent models. In all simulations, the ratio of turbulent magnetic to kinetic energy densities asymptotes at {\~{}}0.1-0.4, and convergence of all relevant dynamical properties requires at least 64 cells per cloud radius.},
archivePrefix = {arXiv},
arxivId = {1706.06607},
author = {Banda-Barrag{\'{a}}n, W. E. and Federrath, C. and Crocker, R. M. and Bicknell, G. V.},
doi = {10.1093/mnras/stx2541},
eprint = {1706.06607},
file = {:home/william/Documents/Papers/stx2541.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: starburst,ISM: clouds,ISM: magnetic fields,MHD,Methods: numerical,Turbulence},
number = {3},
pages = {3454--3489},
title = {{Filament formation in wind-cloud interactions- II. Clouds with turbulent density, velocity, and magnetic fields}},
volume = {473},
year = {2018}
}
@article{Melioli2006,
abstract = {Recent observational studies of the age distribution of star clusters in nearby merging galaxies and starburst (SB) galaxies indicate a premature death of the young clusters. The fate of an evolving star cluster crucially depends of its gas content. This behaves like a glue that helps to keep the star system gravitationally bound. In SB systems where the rate of supemovae (SNe) explosions is elevated one should expect an efficient heating of the gas and its complete removal which could then favor the rapid dissociation of the evolving star clusters. Based on a contemporaneous study of the dynamical evolution of the interstellar gas in SB environments (Melioli {\&} de Gouveia Dal Pino 2004, A{\&}A, 424, 817) where it has been considered also the presence of dense clouds that may inhibit the heating efficiency of the interstellar gas by the SNe, we have here computed the timescales for gas removal from young clusters embedded in these systems and found that they are consistent with the very short timescales for cluster dissolution which are inferred from the observational studies above. Our results indicate that typical SB proto-clusters should start to disperse after less than 5 Myr. For a given total gas mass content, this result is nearly insensitive to the initial star formation efficiency. {\textcopyright} ESO 2006.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0511663},
author = {Melioli, C. and {De Gouveia Dal Pino}, E. M.},
doi = {10.1051/0004-6361:200500218},
eprint = {0511663},
file = {:home/william/Documents/Papers/0511663.pdf:pdf},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Stellar cluster: ISM, SNc,Stellar clusters: general},
number = {3},
primaryClass = {astro-ph},
title = {{ISM gas removal from starburst galaxies and the premature death of star clusters}},
volume = {445},
year = {2006}
}
@ARTICLE{Morganti2013,
       author = {{Morganti}, R. and {Frieswijk}, W. and {Oonk}, R.~J.~B. and {Oosterloo}, T. and {Tadhunter}, C.},
        title = "{Tracing the extreme interplay between radio jets and the ISM in IC 5063}",
      journal = {\aap},
     keywords = {galaxies: active, galaxies: individual: IC 5063, ISM: jets and outflows, radio lines: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = apr,
       volume = {552},
          eid = {L4},
        pages = {L4},
          doi = {10.1051/0004-6361/201220734},
archivePrefix = {arXiv},
       eprint = {1302.2236},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...552L...4M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Harrison2017,
abstract = {Supermassive black holes are found at the centres of massive galaxies. During the growth of these black holes they light up to become visible as active galactic nuclei (AGNs) and release extraordinary amounts of energy across the electromagnetic spectrum. This energy is widely believed to regulate the rate of star formation in the black holes' host galaxies via so-called AGN feedback. However, the details of how and when this occurs remain uncertain from both an observational and theoretical perspective. I review some of the theoretical motivation and observational results and discuss possible observational signatures of the impact of supermassive black hole growth on star formation.},
archivePrefix = {arXiv},
arxivId = {1703.06889},
author = {Harrison, C. M.},
doi = {10.1038/s41550-017-0165},
eprint = {1703.06889},
file = {:home/william/Documents/Papers/harrison2017.pdf:pdf},
issn = {23973366},
journal = {Nat. Astron.},
number = {July},
pages = {1--8},
publisher = {Macmillan Publishers Limited},
title = {{Impact of supermassive black hole growth on star formation}},
url = {http://dx.doi.org/10.1038/s41550-017-0165},
volume = {1},
year = {2017}
}
@article{OSullivan2007,
abstract = {Preliminary VLBA polarisation results on 6 ``blazars'' from 6.5-cm to 7-mm are presented here. Observing at several different wavelengths, separated by short and long intervals, enabled reliable information about the magnetic (B) field structure to be obtained and for the effect of Faraday Rotation to be determined and corrected. For all sources the magnitude of the core Rotation Measure (RM) derived from the shorter wavelength data was greater than that derived from the longer wavelength data, consistent with a higher electron density and/or B-field strength closer to the central engine. A transverse RM gradient was detected in the jet of 0954+658, providing evidence for the presence of a helical B-field surrounding the jet. The RM in the core region of 2200+420 (BL Lac) displays sign changes in different wavelength intervals (on different spatial scales); we suggest an explanation for this in terms of modest bends in a helical B-field surrounding the jet.},
archivePrefix = {arXiv},
arxivId = {0710.0128},
author = {O'Sullivan, Shane P. and Gabuzda, Denise C},
eprint = {0710.0128},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/O'Sullivan, Gabuzda - 2007 - Investigation of the Faraday Rotation Measure and Magnetic Field Structures of Several AGN Jets on Sub-Pars.pdf:pdf},
journal = {Astron. Soc. Pacific Conf. Ser.},
number = {July 2006},
pages = {5},
title = {{Investigation of the Faraday Rotation Measure and Magnetic Field Structures of Several AGN Jets on Sub-Parsec to Parsec Scales}},
url = {http://arxiv.org/abs/0710.0128},
volume = {386},
year = {2007}
}
@article{Dobler2012,
abstract = {The microwave "haze" was first discovered with the initial release of the full sky data from the Wilkinson Microwave Anisotropy Probe. It is diffuse emission towards the center of our Galaxy with spectral behavior that makes it difficult to categorize as any of the previously known emission mechanisms at those wavelengths. With now seven years of WMAP data publicly available, we have learned much about the nature of the haze, and with the release of data from the Fermi Gamma-Ray Space Telescope and the discovery of the gamma-ray haze/bubbles, we have had a spectacular confirmation of its existence at other wavelengths. As the WMAP mission winds down and the Planck mission prepares to release data, I take a last look at what WMAP has to tell us about the origin of this unique Galactic feature. Much like the gamma-rays, the microwave haze/bubbles is elongated in latitude with respect to longitude by a factor of roughly two, and at high latitudes, the microwave emission cuts off sharply above {\~{}}35 degrees (compared to {\~{}}50 degrees in the gammas). The hard spectrum of electrons required to generate the microwave synchrotron is consistent with that required to generate the gamma-ray emission via inverse Compton scattering, though it is likely that these signals result from distinct regions of the spectrum ({\~{}}10 GeV for the microwaves, {\~{}}1 TeV for the gammas). While there is no evidence for significant haze polarization in the 7-year WMAP data, I demonstrate explicitly that it is unlikely such a signal would be detectable above the noise.},
author = {Dobler, Gregory},
doi = {10.1088/0004-637X/750/1/17},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Dobler - 2012 - A last look at the microwave hazebubbles with WMAP.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {Galaxy: center,ISM: bubbles,ISM: structure,radio continuum: ISM},
number = {1},
title = {{A last look at the microwave haze/bubbles with WMAP}},
volume = {750},
year = {2012}
}

@article{Riffel2021a,
abstract = {The near-infrared spectra of active galactic nuclei (AGN) present emission lines of different atomic and molecular species. The mechanisms involved in the origin of these emission lines in AGN are still not fully understood. We use J- and K-band integral field spectra of six luminous ({\$}43.1\backslashlt \backslashlog L{\_}{\{}\backslashrm bol{\}}/({\{}\backslashrm erg\backslash, s{\^{}}{\{}-1{\}}{\}})\backslashlt 44.4{\$}) Seyfert galaxies (NGC 788, Mrk 607, NGC 3227, NGC 3516, NGC 5506, and NGC 5899) in the local Universe (0.0039 {\textless} z {\textless} 0.0136) to investigate the gas excitation within the inner 100–300 pc radius of the galaxies at spatial resolutions of a few tens of parsecs. In all galaxies, the H2 emission originates from thermal processes with excitation temperatures in the range 2400–5200 K. In the high-line ratio (HLR) region of the H2/Br$\gamma$ versus [Fe ii]/Pa$\beta$ diagnostic diagram, which includes 29 per cent of the spaxels, shocks are the main excitation mechanism, as indicated by the correlation between the line widths and line ratios. In the AGN region of the diagram (64 per cent of the spaxels) the H2 emission is due to the AGN radiation. The [Fe ii] emission is produced by a combination of photoionization by the AGN radiation and shocks in five galaxies and is dominated by photoionization in NGC 788. The [S ix]1.2523 $\mu$m coronal emission line is present in all galaxies, and its flux distributions are extended from 80 to 185 pc from the galaxy nuclei, except for NGC 5899, in which this line is detected only in the integrated spectrum.},
archivePrefix = {arXiv},
arxivId = {2103.08736},
author = {Riffel, Rogemar A and Bianchin, Marina and Riffel, Rog{\'{e}}rio and Storchi-Bergmann, Thaisa and Sch{\"{o}}nell, Astor J and Dahmer-Hahn, Luis Gabriel and Dametto, Natacha Z and Diniz, Marlon R},
doi = {10.1093/mnras/stab788},
eprint = {2103.08736},
file = {:home/william/Documents/Papers/2111.09130.pdf:pdf},
issn = {0035-8711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {active,galaxies,kinematics,nuclei,seyfert},
number = {4},
pages = {5161--5178},
title = {{Gemini NIFS survey of feeding and feedback in nearby active galaxies – IV. Excitation}},
volume = {503},
year = {2021}
}
@article{2005A&A...439..521M,
author = {Morganti, R and Oosterloo, T.{\~{}}A. and Tadhunter, C.{\~{}}N. and van Moorsel, G and Emonts, B},
doi = {10.1051/0004-6361:20053175},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Morganti et al. - 2005 - The location of the broad H i absorption in 3C 305 clear evidence for a jet-accelerated neutral outflow.pdf:pdf},
journal = {aap},
keywords = {galaxies: ISM,galaxies: active,galaxies: individual: 3C 305},
pages = {521--526},
title = {{The location of the broad H i absorption in 3C 305: clear evidence for a jet-accelerated neutral outflow}},
volume = {439},
year = {2005}
}
@article{Schawinski2006,
abstract = {Detailed high-resolution observations of the innermost regions of nearby galaxies have revealed the presence of supermassive black holes. These black holes may interact with their host galaxies by means of 'feedback' in the form of energy and material jets; this feedback affects the evolution of the host and gives rise to observed relations between the black hole and the host. Here we report observations of the ultraviolet emissions of massive early-type galaxies. We derive an empirical relation for a critical black-hole mass (as a function of velocity dispersion) above which the outflows from these black holes suppress star formation in their hosts by heating and expelling all available cold gas. Supermassive black holes are negligible in mass compared to their hosts but nevertheless seem to play a critical role in the star formation history of galaxies. {\textcopyright} 2006 Nature Publishing Group.},
author = {Schawinski, Kevin and Khochfar, Sadegh and Kaviraj, Sugata and Yi, Sukyoung K. and Boselli, Alessandro and Barlow, Tom and Conrow, Tim and Forster, Karl and Friedman, Peter G. and Martin, D. Chris and Morrissey, Patrick and Neff, Susan and Schiminovich, David and Seibert, Mark and Small, Todd and Wyder, Ted K. and Bianchi, Luciana and Donas, Jose and Heckman, Tim and Lee, Young Wook and Madore, Barry and Milliard, Bruno and Rich, R. Michael and Szalay, Alex},
doi = {10.1038/nature04934},
file = {:home/william/Documents/Papers/schawinski2006.pdf:pdf},
issn = {14764687},
journal = {Nature},
number = {7105},
pages = {888--891},
title = {{Suppression of star formation in early-type galaxies by feedback from supermassive black holes}},
volume = {442},
year = {2006}
}
@article{Eso,
author = {{\'{E}}s{\`{o}}, {\^{I}} {\`{E}} {\^{O}}g{\ss} {\^{I}} {\"{E}}{\o}r{\^{i}} and {\`{I}}q{\`{o}}, {\O} Ð {\`{U}}i{\"{i}} {\^{I}} and {\^{E}}a{\'{i}}, {\`{E}} {\'{E}} {\~{N}} {\^{E}}z{\^{e}}a{\`{e}} {\~{O}} and {\`{I}}, {\`{O}} {\'{U}} {\^{E}} {\`{I}} {\`{O}} {\O} {\`{O}} {\'{I}} {\^{E}}{\`{u}}a{\"{u}} {\'{I}} {\^{I}} {\"{E}}q{\`{u}}a{\'{i}} {\`{O}} {\"{U}} {\^{O}} and {\^{E}}a{\"{o}}g{\^{e}}a{\'{e}}, {\O} and {\'{I}}i{\^{a}}, {\^{I}} and {\"{O}}, {\"{E}} S {\^{I}} {\`{E}} {\"{I}} Ð {\`{E}} {\"{I}}q {\"{E}} S {\`{O}} {\O} {\'{U}}f{\"{e}}ð {\O} {\^{I}} {\"{E}} Ð {\'{I}} and {\`{U}}a{\'{i}}, Ð {\`{E}} {\'{E}}s{\"{e}}s{\^{i}} {\`{E}} {\`{I}} {\'{I}} {\"{U}} {\`{U}}{\^{e}}a{\`{e}} {\'{E}} and {\`{I}}, {\`{O}} {\"{U}} {\^{O}}},
file = {:home/william/Documents/Papers/1999pcim.conf...77E.pdf:pdf},
title = {{{\`{U}}A f e ¥ z ¢  s }}
}
@article{Blandford2001,
abstract = {Recent developments in the spectropolarimetric study of compact objects, specifically black holes (stellar and massive) and neutron stars are reviewed. The lectures are organized around five topics: disks, jets, outflows, neutron stars and black holes. They emphasize physical mechanisms and are intended to bridge the gap between the fundamentals of polarimetry and the phenomenology of observed cosmic sources of polarized radiation, as covered by the other lecturers. There has been considerable recent progress in spectropolarimetry from radio through optical frequencies and this is producing some unique diagnostics of the physical conditions around compact objects. It is argued that there is a great need to develop a correspondingly sensitive polarimetric capability at ultraviolet through gamma-ray energies.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0107228},
author = {Blandford, Roger and Agol, Eric and Broderick, Avery and Heyl, Jeremy and Koopmans, Leon and Lee, Hee-Won},
eprint = {0107228},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Blandford et al. - 2001 - Compact Objects and Accretion Disks.pdf:pdf},
primaryClass = {astro-ph},
title = {{Compact Objects and Accretion Disks}},
url = {http://arxiv.org/abs/astro-ph/0107228},
year = {2001}
}
@article{Field1965,
author = {Field, George B and Field, George B},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Field, Field - 1965 - THERMAL INSTABILITY George B. Field Princeton University Observatory Received June 4, 1964 revised March 30, 1965.pdf:pdf},
journal = {Astrophys. J.},
pages = {531--567},
title = {{THERMAL INSTABILITY George B. Field Princeton University Observatory Received June 4, 1964; revised March 30, 1965}},
year = {1965}
}
@article{Teng2009,
abstract = {We report the results from our analysis of Suzaku X-ray Imaging Spectrometer (XIS) (0.5-10 keV) and Hard X-ray Detector (HXD)/PIN (15-40 keV) observations of five well-known local ultraluminous infrared galaxies: IRAS F05189-2524, IRAS F08572 + 3915, Mrk 273, PKS 1345 + 12, and Arp 220. The XIS observations of F05189-2524 and Mrk 273 reveal strong iron lines consistent with Fe K$\alpha$ and changes in spectral shapes with respect to previous Chandra and XMM-Newton observations. Mrk 273 is also detected by the HXD/PIN at ∼ 1.8$\sigma$. For F05189-2524, modeling of the data from the different epochs suggests that the change in spectral shape is likely due to the central source switching off, leaving behind a residual reflection spectrum, or an increase in the absorbing column. An increase in the covering fraction of the absorber can describe the spectral variations seen in Mrk 273, although a reduction in the intrinsic active galactic nucleus (AGN) luminosity cannot be formally ruled out. The Suzaku spectra of Mrk 273 are well fitted by a ∼ 94{\%} covering fraction model with a column density of ∼ 1024 cm-2. The absorption-corrected log[L 2-10keV/L IR] ratio is consistent with those found in PG Quasars. The 0.5-10 keV spectrum of PKS 1345 + 12 and Arp 220 seem unchanged from previous observations and their hard X-ray emission is not convincingly detected by the HXD/PIN. The large column density derived from CO observations and the large equivalent width of an ionized Fe line in Arp 220 can be reconciled by an ionized reflection model. F08572 + 3915 is undetected in both the XIS and HXD/PIN, but the analysis of unpublished Chandra data provides a new measurement at low energies. {\textcopyright} 2009. The American Astronomical Society. All rights reserved.},
archivePrefix = {arXiv},
arxivId = {0809.2090},
author = {Teng, Stacy H. and Veilleux, Sylvain and Anabuki, Naohisa and Dermer, Charles D. and Gallo, Luigi C. and Nakagawa, Takao and Reynolds, Christopher S. and Sanders, D. B. and Terashima, Yuichi and Wilson, Andrew S.},
doi = {10.1088/0004-637X/691/1/261},
eprint = {0809.2090},
file = {:home/william/Documents/Papers/Teng{\_}2009{\_}ApJ{\_}691{\_}261.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {X-rays: galaxies,galaxies: active,galaxies: individual (IRAS F05189,galaxies: starburst},
number = {1},
pages = {261--276},
title = {{Suzaku observations of local ultraluminous infrared galaxies}},
volume = {691},
year = {2009}
}
@article{Tesileanu2008a,
abstract = {Context. Time-dependent cooling processes are of paramount importance in the evolution of astrophysical gaseous nebulae and, in particular, when radiative shocks are present. Given the recent improvements in resolution of the observational data, simulating these processes in a more realistic manner in magnetohydrodynamic (MHD) codes will provide a unique tool for model discrimination.Aims. The present work introduces a necessary set of tools that can be used to model radiative astrophysical flows in the optically-thin plasma limit. We aim to provide reliable and accurate predictions of emission line ratios and radiative cooling losses in astrophysical simulations of shocked flows. Moreover, we discuss numerical implementation aspects to ease future improvements and implementation in other MHD numerical codes.Methods. The most important source of radiative cooling for our plasma conditions comes from the collisionally-excited line radiation. We evolve a chemical network, including 29 ion species, to compute the ionization balance in non-equilibrium conditions. The numerical methods are implemented in the PLUTO code for astrophysical fluid dynamics and particular attention has been devoted to resolve accuracy and efficiency issues arising from cooling timescales considerably shorter than the dynamical ones.Results. After a series of validations and tests, typical astrophysical setups are simulated in 1D and 2D, employing both the present cooling model and a simplified one. The influence of the cooling model on structure morphologies can become important, especially for emission line diagnostic purposes.Conclusions. The tests make us confident that the use of the presented detailed radiative cooling treatment will allow more accurate predictions in terms of emission line intensities and shock dynamics in various astrophysical setups. {\textcopyright} 2008 ESO.},
archivePrefix = {arXiv},
arxivId = {0807.3657},
author = {Teşileanu, O. and Mignone, A. and Massaglia, S.},
doi = {10.1051/0004-6361:200809461},
eprint = {0807.3657},
file = {:home/william/Documents/Papers/0807.3657.pdf:pdf},
issn = {00046361},
journal = {Astron. Astrophys.},
keywords = {ISM: Herbig-Haro objects,ISM: jets and outflows,Line: formation,Magnetohydrodynamics (MHD),Methods: numerical,Radiation mechanisms: thermal},
number = {1},
pages = {429--440},
title = {{Simulating radiative astrophysical flows with the PLUTO code: A non-equilibrium, multi-species cooling function}},
volume = {488},
year = {2008}
}
@article{Ackermann2014,
abstract = {The Fermi bubbles are two large structures in the gamma-ray sky extending to 55° above and below the Galactic center. We analyze 50 months of Fermi Large Area Telescope data between 100 MeV and 500 GeV above 10° in Galactic latitude to derive the spectrum and morphology of the Fermi bubbles. We thoroughly explore the systematic uncertainties that arise when modeling the Galactic diffuse emission through two separate approaches. The gamma-ray spectrum is well described by either a log parabola or a power law with an exponential cutoff. We exclude a simple power law with more than 7$\sigma$ significance. The power law with an exponential cutoff has an index of 1.9 ± 0.2 and a cutoff energy of 110 ± 50 GeV. We find that the gamma-ray luminosity of the bubbles is erg s-1. We confirm a significant enhancement of gamma-ray emission in the southeastern part of the bubbles, but we do not find significant evidence for a jet. No significant variation of the spectrum across the bubbles is detected. The width of the boundary of the bubbles is estimated to be deg. Both inverse Compton (IC) models and hadronic models including IC emission from secondary leptons fit the gamma-ray data well. In the IC scenario, synchrotron emission from the same population of electrons can also explain the WMAP and Planck microwave haze with a magnetic field between 5 and 20 $\mu$G.},
author = {Ackermann, M. and Albert, A. and Atwood, W. B. and Baldini, L. and Ballet, J. and Barbiellini, G. and Bastieri, D. and Bellazzini, R. and Bissaldi, E. and Blandford, R. D. and Bloom, E. D. and Bottacini, E. and Brandt, T. J. and Bregeon, J. and Bruel, P. and Buehler, R. and Buson, S. and Caliandro, G. A. and Cameron, R. A. and Caragiulo, M. and Caraveo, P. A. and Cavazzuti, E. and Cecchi, C. and Charles, E. and Chekhtman, A. and Chiang, J. and Chiaro, G. and Ciprini, S. and Claus, R. and Cohen-Tanugi, J. and Conrad, J. and Cutini, S. and D'Ammando, F. and {De Angelis}, A. and {De Palma}, F. and Dermer, C. D. and Digel, S. W. and {Di Venere}, L. and {Do Couto E Silva}, E. and Drell, P. S. and Favuzzi, C. and Ferrara, E. C. and Focke, W. B. and Franckowiak, A. and Fukazawa, Y. and Funk, S. and Fusco, P. and Gargano, F. and Gasparrini, D. and Germani, S. and Giglietto, N. and Giordano, F. and Giroletti, M. and Godfrey, G. and Gomez-Vargas, G. A. and Grenier, I. A. and Guiriec, S. and Hadasch, D. and Harding, A. K. and Hays, E. and Hewitt, J. W. and Hou, X. and Jogler, T. and J{\'{o}}hannesson, G. and Johnson, A. S. and Johnson, W. N. and Kamae, T. and Kataoka, J. and Kn{\"{o}}dlseder, J. and Kocevski, D. and Kuss, M. and Larsson, S. and Latronico, L. and Longo, F. and Loparco, F. and Lovellette, M. N. and Lubrano, P. and Malyshev, D. and Manfreda, A. and Massaro, F. and Mayer, M. and Mazziotta, M. N. and McEnery, J. E. and Michelson, P. F. and Mitthumsiri, W. and Mizuno, T. and Monzani, M. E. and Morselli, A. and Moskalenko, I. V. and Murgia, S. and Nemmen, R. and Nuss, E. and Ohsugi, T. and Omodei, N. and Orienti, M. and Orlando, E. and Ormes, J. F. and Paneque, D. and Panetta, J. H.},
doi = {10.1088/0004-637X/793/1/64},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ackermann et al. - 2014 - The spectrum and morphology of the Fermi bubbles.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {Galaxy: general,Galaxy: halo,astroparticle physics,cosmic rays,gamma rays: diffuse background,methods: data analysis},
number = {1},
title = {{The spectrum and morphology of the Fermi bubbles}},
volume = {793},
year = {2014}
}
@article{Combes2009,
author = {Combes, F.},
doi = {10.1051/0004-6361/200912152},
file = {:home/william/Documents/Papers/[Combes]-Commentary on Tully and Fisher 1977 paper.pdf:pdf},
issn = {00046361},
journal = {Astron. Astrophys.},
number = {1},
pages = {119--120},
title = {{From distances to galaxy evolution and the dark matter problem}},
volume = {500},
year = {2009}
}
@article{Symeonidis2021,
abstract = {We investigate the balance of power between stars and AGN across cosmic history, based on the comparison between the infrared (IR) galaxy luminosity function (LF) and the IR AGN LF. The former corresponds to emission from dust heated by stars and AGN, whereas the latter includes emission from AGN-heated dust only. We find that at all redshifts (at least up to z ∼ 2.5), the high-luminosity tails of the two LFs converge, indicating that the most IR-luminous galaxies are AGN-powered. Our results shed light to the decades-old conundrum regarding the flatter high-luminosity slope seen in the IR galaxy LF compared to that in the UV and optical. We attribute this difference to the increasing fraction of AGN-dominated galaxies with increasing total IR luminosity (LIR). We partition the LIR−z parameter space into a star formation-dominated and an AGN-dominated region, finding that the most luminous galaxies at all epochs lie in the AGN-dominated region. This sets a potential ‘limit' to attainable star formation rates, casting doubt on the abundance of ‘extreme starbursts': if AGN did not exist, LIR {\textgreater} 1013 L⊙ galaxies would be significantly rarer than they currently are in our observable Universe. We also find that AGN affect the average dust temperatures (Tdust) of galaxies and hence the shape of the well-known LIR−Tdust relation. We propose that the reason why local ULIRGs are hotter than their high-redshift counterparts is because of a higher fraction of AGN-dominated galaxies amongst the former group.},
archivePrefix = {arXiv},
arxivId = {2102.11936},
author = {Symeonidis, M and Page, M J},
doi = {10.1093/mnras/stab598},
eprint = {2102.11936},
file = {:home/william/Documents/Papers/2102.11936.pdf:pdf},
issn = {0035-8711},
journal = {Mon. Not. R. Astron. Soc.},
number = {3},
pages = {3992--4007},
title = {{AGN and star formation across cosmic time}},
volume = {503},
year = {2021}
}
@article{Tadhunter2008,
abstract = {In the light of recent speculation that AGN have a major impact on the evolution of their host galaxies, I review the observational evidence for energetic outflows around AGN, concentrating in particular on the spatially resolved outflows around radioloud AGN. There is now substantial evidence that the large-scale radio jets have a major impact on the evolution of the hot and warm ISM in the surround galaxy haloes and clusters on a ˜5 - 500 kpc scale. However, although clear evidence for warm and cool outflows has also been found on the smaller ({\textless}5 kpc) scale of the NLR, these outflows are in general much less energetic than those driven by the radio jets on a larger scale. Indeed, the warm outflows detected in the NLR using both optical emission lines and narrow UV absorption line are generally less massive and energetic than those driven by extreme starbursts in ULIRGs. Apart from the radio jets, the only AGN-induced outflows that come close to matching the requirements of the galaxy evolution feedback models are those detected using the blueshifted X-ray absorption edge features.},
author = {Tadhunter, Clive},
file = {:home/william/Documents/Papers/2008MmSAI..79.1205T.pdf:pdf},
journal = {Mem SAIt},
keywords = {active,evolution,galaxies},
pages = {1205--1212},
title = {{The importance of sub-relativistic outflows in AGN host galaxies}},
url = {http://sait.oat.ts.astro.it/MmSAI/79/PDF/1205.pdf},
volume = {79},
year = {2008}
}
@article{Iwasawa2017,
abstract = {We present an X-ray study of the ultra-luminous infrared galaxy IRAS F00183-7111 (z = 0:327), using data obtained from NuSTAR, Chandra X-ray Observatory, Suzaku and XMM-Newton. The Chandra imaging shows that a point-like X-ray source is located at the nucleus of the galaxy at energies above 2 keV. However, the point source resolves into diffuse emission at lower energies, extending to the east, where the extranuclear [Oiii]$\lambda$5007 emission, presumably induced by a galactic-scale outflow, is present. The nuclear source is detected by NuSTAR up to the rest-frame 30 keV. The strong, high-ionization Fe K line, first seen by XMM-Newton, and subsequently by Suzaku and Chandra, is not detected in the NuSTAR data. The line flux appears to have been declining continuously between 2003 and 2016, while the continuum emission remained stable to within 30{\%}. Further observations are needed to confirm this. The X-ray continuum below 10 keV is characterised by a hard spectrum caused by cold absorption of NH {\~{}}1 × 1023 cm-2, compatible to that of the silicate absorption at 9.7 $\mu$m, and a broad absorption feature around 8 keV which we attribute to a high-ionization Fe K absorption edge. The latter is best described by a blueshifted, high-ionization (log ϵ {\~{}} 3) absorber with a column density of NH {\~{}} 1 × 1024 cm-2, similar to the X-ray high-velocity outflows observed in a number of active nuclei. No extra hard component, which would arise from a strongly absorbed (i.e. Compton-thick) source, is seen in the NuSTAR data. While a pure reflection scenario (with a totally hidden central source) is viable, direct emission from the central source of L2-10 keV ≈ 2 × 1044 erg s-1, behind layers of cold and hot absorbing gas may be an alternative explanation. In this case, the relative X-ray quietness (Lx/Lbol,AGN ≤ 6 × 10-3), the high-ionization Fe line, strong outflows inferred from various observations, and other similarities to the well-studied ULIRG/QSO Mrk 231 point that the central source in this ULIRG might be accreting close to the Eddington limit.},
archivePrefix = {arXiv},
arxivId = {1709.01708},
author = {Iwasawa, K. and Spoon, H. W.W. and Comastri, A. and Gilli, R. and Lanzuisi, G. and Piconcelli, E. and Vignali, C. and Brusa, M. and Puccetti, S.},
doi = {10.1051/0004-6361/201730950},
eprint = {1709.01708},
file = {:home/william/Documents/Papers/1709.01708.pdf:pdf},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Galaxies: active,Galaxies: individual: IRAS F00183, 7111,X-rays: galaxies},
pages = {1--9},
title = {{The active nucleus of the ULIRG IRAS F00183-7111 viewed by NuSTAR}},
volume = {606},
year = {2017}
}
@article{King2015a,
abstract = {Observational arguments suggest that the growth phases of the supermassive black holes in active galactic nuclei have a characteristic time-scale ˜105 yr. We show that this is the time-scale expected in the chaotic accretion picture of black hole feeding, because of the effect of self-gravity in limiting the mass of any accretion-disc feeding event.},
author = {King, Andrew and Nixon, Chris},
doi = {10.1093/mnrasl/slv098},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/King, Nixon - 2015 - AGN flickering and chaotic accretion.pdf:pdf},
issn = {17453933},
journal = {Mon. Not. R. Astron. Soc. Lett.},
keywords = {Accretion, accretion discs,Black hole physics,Galaxies: active,Galaxies: seyfert,Quasars: supermassive black holes,X-rays: galaxies},
number = {1},
pages = {L46--L47},
title = {{AGN flickering and chaotic accretion}},
volume = {453},
year = {2015}
}
@article{Revalski2021,
abstract = {Outflows of ionized gas driven by active galactic nuclei (AGN) may significantly impact the evolution of their host galaxies. However, determining the energetics of these outflows is difficult with spatially unresolved observations that are subject to strong global selection effects. We present part of an ongoing study using Hubble Space Telescope (HST) and Apache Point Observatory (APO) spectroscopy and imaging to derive spatially-resolved mass outflow rates and energetics for narrow line region (NLR) outflows in nearby AGN that are based on multi-component photoionization models to account for spatial variations in the gas ionization, density, abundances, and dust content. This expanded analysis adds Mrk 3, Mrk 78, and NGC 1068, doubling the sample in Revalski (2019). We find that the outflows contain total ionized gas masses of {\$}M \backslashapprox 10{\^{}}{\{}5.5{\}} - 10{\^{}}{\{}7.5{\}}{\$} {\$}M{\_}{\{}\backslashodot{\}}{\$} and reach peak velocities of {\$}v \backslashapprox 800 - 2000{\$} km s{\$}{\^{}}{\{}-1{\}}{\$}. The outflows reach maximum mass outflow rates of {\$}\backslashdot M{\_}{\{}out{\}} \backslashapprox 3 - 12{\$} {\$}M{\_}{\{}\backslashodot{\}}{\$} yr{\$}{\^{}}{\{}-1{\}}{\$} and encompass total kinetic energies of {\$}E \backslashapprox 10{\^{}}{\{}54{\}} - 10{\^{}}{\{}56{\}}{\$} erg. The outflows extend to radial distances of {\$}r \backslashapprox 0.1 - 3{\$} kpc from the nucleus, with the gas masses, outflow energetics, and radial extents positively correlated with AGN luminosity. The outflow rates are consistent with in-situ ionization and acceleration where gas is radiatively driven at multiple radii. These radial variations indicate that spatially-resolved observations are essential for localizing AGN feedback and determining the most accurate outflow parameters.},
archivePrefix = {arXiv},
arxivId = {2101.06270},
author = {Revalski, Mitchell and Meena, Beena and Martinez, Francisco and Polack, Garrett E. and Crenshaw, D. Michael and Kraemer, Steven B. and Collins, Nicholas R. and Fischer, Travis C. and Schmitt, Henrique R. and Schmidt, Judy and Maksym, W. Peter and Rafelski, Marc},
eprint = {2101.06270},
file = {:home/william/Documents/Papers/2101.06270.pdf:pdf},
keywords = {active,and dynamics,galaxies,individual,ism,jets and outflows,kinematics,mrk 3,mrk 78,ngc 1068,seyfert},
number = {5140},
title = {{Quantifying Feedback from Narrow Line Region Outflows in Nearby Active Galaxies -- III. Results for the Seyfert 2 Galaxies Markarian 3, Markarian 78, and NGC 1068}},
url = {http://arxiv.org/abs/2101.06270},
year = {2021}
}
@article{Lopez-Rodriguez2013a,
archivePrefix = {arXiv},
arxivId = {1302.6858},
author = {Lopez-Rodriguez, E. and Packham, C. and Young, S. and Elitzur, M. and Levenson, N. A. and Mason, R. E. and Almeida, C. Ramos and Alonso-Herrero, A. and Jones, T. J. and Perlman, E.},
doi = {10.5047/eps.2013.05.021},
eprint = {1302.6858},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Lopez-Rodriguez et al. - 2013 - New insights into the study of magnetic field in the clumpy torus of AGN using near-infrared polarimetry.pdf:pdf},
issn = {1343-8832},
journal = {Earth, Planets Sp.},
keywords = {agn,infrared,polarimetry,torus},
number = {10},
pages = {1117--1122},
title = {{New insights into the study of magnetic field in the clumpy torus of AGN using near-infrared polarimetry}},
url = {http://link.springer.com/10.5047/eps.2013.05.021},
volume = {65},
year = {2013}
}
@article{Zubovas2018,
abstract = {Massive large-scale AGN outflows are an important element of galaxy evolution, being a way through which the AGN can affect most of the host galaxy. However, outflows evolve on timescales much longer than typical AGN episode durations, therefore most AGN outflows are not observed simultaneously with the AGN episode that inflated them. It is therefore remarkable that rather tight correlations between outflow prop- erties and AGN luminosity exist. In this paper, I show that such correlations can be preserved during the fading phase of the AGN episode, provided that the AGN lumi- nosity evolves as a power law with exponent {\$}\backslashalpha{\_}{\{}\backslashrm d{\}} \backslashsim 1{\$} at late times. I also show that subsequent AGN episodes that illuminate an ongoing outflow are unlikely to produce outflow momentum or energy rates rising above the observed correlations. However, there may be many difficult-to-detect outflows with momentum and energy rates lower than expected from the current AGN luminosity. Detailed observations of AGN out- flow properties might help constrain the activity histories of typical and/or individual AGN.},
archivePrefix = {arXiv},
arxivId = {1710.01053},
author = {Zubovas, Kastytis},
doi = {10.1093/mnras/stx2569},
eprint = {1710.01053},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Zubovas - 2018 - Massive outflow properties suggest AGN fade slowly.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Accretion,Accretion discs,Galaxies: active,Galaxies: evolution,Quasars: general},
number = {3},
pages = {3525--3535},
title = {{Massive outflow properties suggest AGN fade slowly}},
volume = {473},
year = {2018}
}
@article{Veilleux2005,
abstract = {Galactic winds are the primary mechanism by which energy and metals are recycled in galaxies and are deposited into the intergalactic medium. New observations are revealing the ubiquity of this process, particularly at high redshift. We describe the physics behind these winds, discuss the observational evidence for them in nearby star-forming and active galaxies and in the high-redshift universe, and consider the implications of energetic winds for the formation and evolution of galaxies and the intergalactic medium. To inspire future research, we conclude with a set of observational and theoretical challenges. Copyright {\textcopyright} 2005 by Annual Reviews. All rights reserved.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0504435},
author = {Veilleux, Sylvain and Cecil, Gerald and Bland-Hawthorn, Joss},
doi = {10.1146/annurev.astro.43.072103.150610},
eprint = {0504435},
file = {:home/william/Documents/Papers/annurev.astro.43.072103.150610.pdf:pdf},
issn = {00664146},
journal = {Annu. Rev. Astron. Astrophys.},
keywords = {Evolution,Halos,Intergalactic medium,Kinematics and dynamics,Nuclei},
pages = {769--826},
primaryClass = {astro-ph},
title = {{Galactic winds}},
volume = {43},
year = {2005}
}
@article{Zhang2022,
abstract = {CSS J102913+404220 is a peculiar narrow line Seyfert 1 galaxy with an energetic nuclear optical outburst. We present a detailed analysis of its multi-wavelength photometric and spectroscopic observations covering a period of decade since outburst. We detect mid-infrared (MIR) flares delayed by about two months relative to the optical outburst, with an extremely high peak luminosity of log(L{\_}4.6um){\textgreater}44 erg/s. The MIR peak luminosity is at least an order of magnitude higher than any known supernovae explosions, suggesting the optical outburst might be due to a stellar tidal disruption event (TDE). We find late-time X-ray brightening by a factor of {\textgreater}30 with respect to what is observed about 100 days after the optical outburst peak, followed by a flux fading by a factor of {\~{}}4 within two weeks, making it one of Active Galactic Nuclei (AGNs) with extreme variability. Despite the dramatic X-ray variability, there are no coincident strong flux variations in optical, UV and MIR bands. This unusual variability behavior has been seen in other highly accreting AGNs and could be attributed to absorption variability. In this scenario, the decrease in the covering factor of absorber with accretion rate could cause the X-ray brightening, possibly induced by the TDE. Most strikingly, while the UV/optical continuum remains little changes with time, an evident enhancement in the flux of H{\_}alpha broad emission line is observed, about a decade after the nuclear optical outburst, which is an anomalous behavior never seen in any other AGNs. Such an H{\_}alpha anomaly could be explained by the replenishment of gas clouds and excitation within Broad Line Region (BLR) that originates, perhaps from the interaction of outflowing stellar debris with BLR. The results highlight the importance of late-time evolution of TDE that could affect the accreting properties of AGN, as suggested by recent simulations.},
archivePrefix = {arXiv},
arxivId = {2201.11048},
author = {Zhang, W. J. and Shu, X. W. and Sheng, Z. F. and Sun, L. M. and Dou, L. M. and Jiang, N. and Wang, J. G. and Hu, X. Y. and Wang, Y. B. and Wang, T. G.},
eprint = {2201.11048},
file = {:home/william/Documents/Papers/2201.11048.pdf:pdf},
keywords = {404220,accretion,accretion disks,active,css j102913,galaxies,individual,x-rays},
pages = {1--16},
title = {{Discovery of late-time X-ray flare and anomalous emission line enhancement after the nuclear optical outburst in a narrow-line Seyfert 1 Galaxy}},
url = {http://arxiv.org/abs/2201.11048},
year = {2022}
}
@article{Blumenthal.G.1970,
abstract = {Expressions are derived for the total energy loss and photon-production spectrum by the processes of Compton scatter- ing, bremsstrahlung, and synchrotron radiation from highly relativistic electrons. For Compton scattering, the general case, the Thomson limit, and the extreme Klein —Nishina limit are considered. Bremsstrahlung is treated for the cases where the electron is scattered by a pure Coulomb field and by an atom. For the latter case the effects of shielding are discussed extensively. The synchrotron spectrum is derived for an electron moving in a circular orbit perpendicular to the magnetic field and also for the general case where the electron's motion is helical. The total photon-production spec- trum is derived for each process when there is a power-law distribution of electron energies. The problems of the eBects of the three processes on the electron distribution itself are considered. It is shown that if the electron loses a small frac- tion of its energy in a single occurrence of a process, the electron distribution function satisfies a continuity equation which is a differential equation in energy space. For the more general case where the electron can Jose energy in discrete amounts (as in bremsstrahlung and extreme Klein —Nishina Compton losses), the electron distribution function satis6es an integro-differential equation. Some approximate solutions to this equation are derived for certain special cases.},
author = {{Blumenthal. G.}, Gould. J},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Blumenthal. G. - 1970 - Reviews of Modern Physics.pdf:pdf},
journal = {Rev. Mod. Phys.},
number = {2},
pages = {237--270},
title = {{Reviews of Modern Physics}},
volume = {42},
year = {1970}
}
@article{Krumholz2019a,
abstract = {Star-forming gas clouds are strongly magnetized, and their ionization fractions are high enough to place them close to the regime of ideal magnetohydrodyamics on all but the smallest size scales. In this review we discuss the effects of magnetic fields on the star formation rate (SFR) in these clouds, and on the mass spectrum of the fragments that are the outcome of the star formation process, the stellar initial mass function (IMF). Current numerical results suggest that magnetic fields by themselves are minor players in setting either the SFR or the IMF, changing star formation rates and median stellar masses only by factors of {\~{}}2−3 compared to non-magnetized flows. However, the indirect effects of magnetic fields, via their interaction with star formation feedback in the form of jets, photoionization, radiative heating, and supernovae, could have significantly larger effects. We explore evidence for this possibility in current simulations, and suggest avenues for future exploration, both in simulations and observations.},
archivePrefix = {arXiv},
arxivId = {1902.02557},
author = {Krumholz, Mark R. and Federrath, Christoph},
doi = {10.3389/fspas.2019.00007},
eprint = {1902.02557},
file = {:home/william/Documents/Papers/fspas-06-00007.pdf:pdf},
issn = {2296987X},
journal = {Front. Astron. Sp. Sci.},
keywords = {ISM: clouds,ISM: kinematics and dynamics,ISM: magnetic fields,galaxies: star formation,magnetohydrodynamics (MHD),stars: formation,turbulence},
number = {February},
pages = {1--28},
title = {{The Role of Magnetic Fields in Setting the Star Formation Rate and the Initial Mass Function}},
volume = {6},
year = {2019}
}
@article{Rupke2018,
abstract = {Galaxy-scale outflows of gas, or galactic winds (GWs), driven by energy from star formation are a pivotal mechanism for regulation of star formation in the current model of galaxy evolution. Observations of this phenomenon have proliferated through the wide application of old techniques on large samples of galaxies, the development of new methods, and advances in telescopes and instrumentation. I review the diverse portfolio of direct observations of stellar GWs since 2010. Maturing measurements of the ionized and neutral gas properties of nearby winds have been joined by exciting new probes of molecular gas and dust. Low-{\$}z{\$} techniques have been newly applied in large numbers at high {\$}z{\$}. The explosion of optical and near-infrared 3D imaging spectroscopy has revealed the complex, multiphase structure of nearby GWs. These observations point to stellar GWs being a common feature of rapidly star-forming galaxies throughout at least the second half of cosmic history, and suggest that scaling relationships between outflow and galaxy properties persist over this period. The simple model of a modest-velocity, biconical flow of multiphase gas and dust perpendicular to galaxy disks continues to be a robust descriptor of these flows.},
archivePrefix = {arXiv},
arxivId = {1812.05184},
author = {Rupke, David S. N.},
doi = {10.3390/galaxies6040138},
eprint = {1812.05184},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Rupke - 2018 - A Review of Recent Observations of Galactic Winds Driven by Star Formation.pdf:pdf},
keywords = {feedback,galactic winds,outflows,star formation},
title = {{A Review of Recent Observations of Galactic Winds Driven by Star Formation}},
url = {http://arxiv.org/abs/1812.05184{\%}0Ahttp://dx.doi.org/10.3390/galaxies6040138},
year = {2018}
}
@article{Desch1998,
abstract = {Key processes are examined in the heating and cooling of molecular gas
with emphasis on environments for water masers at the nuclei of
galaxies. The exchange of infrared radiation between the gas and dust
grains is evaluated in determining the cooling of the gas and in
determining the thermal coupling between the gas and the dust grains.
Calculations are performed for the transport of continuum radiation
through an optically thick slab to assess the temperatures of the dust
grains. The highly refined observational description of the subparsec
circumnuclear disk in the galaxy NGC 4258 serves as a focus. The viscous
dissipation that is inherent in an accretion disk is reconsidered as a
source of heat to create the masing environment. Based on our cooling
rates, the input of energy that is required to create the bulk of the
observed masing gas is evaluated and is found to be comparable in
magnitude (per unit surface area) to that generated by the viscous
dissipation. To be effective in actually creating the masing
environment, the distribution for the viscous dissipation of heat with
distance from the midplane of the disk must be quite different from the
distribution of the mass. Tentative evidence that this is plausible is
discussed. One consequence is the likely presence of a component of the
disk at the midplane that is colder and much more massive than the
masing gas. The recent interpretation that the inner disk of NGC 4258
may be advective is especially useful for this description, since the
viscous dissipation at the location of the masers tends to be enhanced.
A significant temperature difference between the gas and the grains,
which is necessary for masing, is found to result regardless of whether
the heating in these environments is provided by viscous dissipation or
by X-rays.},
author = {Desch, S. J. and Wallin, B. K. and Watson, W. D.},
doi = {10.1086/305391},
file = {:home/william/Documents/Papers/Radiative{\_}Cooling{\_}and{\_}Viscous{\_}Dissipation{\_}in{\_}Molec.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
number = {2},
pages = {775--785},
title = {{Radiative Cooling and Viscous Dissipation in Molecular Accretion Disks at the Nuclei of Galaxies}},
volume = {496},
year = {1998}
}
@article{Nielsen1998,
abstract = {This paper presents a general formulation of least-squares estimation using Lagrange multipliers. It is general in the sense that it takes into account the covariance matrix of all measured quantities and allows any known constraint to be imposed on the quantities being estimated. The technique may be used to estimate parameters of a calibration curve for a transducer taking into account the uncertainty and correlation coefficients of the measured stimuli and responses. It may also be used to adjust measured fundamental constants to a coherent set obeying the appropriate physical laws.},
author = {Nielsen, L.},
doi = {10.1088/0026-1394/35/2/6},
file = {:home/william/Documents/Papers/Least-squares{\_}estimation{\_}using{\_}Lagrange{\_}multiplier.pdf:pdf},
issn = {00261394},
journal = {Metrologia},
number = {2},
pages = {115--118},
title = {{Least-squares estimation using Lagrange multipliers}},
volume = {35},
year = {1998}
}
@article{Fabian2001,
abstract = {Although soft X-ray absorption features in AGNs were discovered almost ten years ago, the nature and location of the gas creating them has remained controversial. Guided by the results of recent high-resolution X-ray spectroscopy, we argue that these features are created in a multitemperature wind whose source of matter is photoionized evaporation from the inner edge of the obscuring torus often found surrounding an AGN. Photoionized evaporation in the presence of a copious mass source locks the ratio of ionizing intensity to pressure to a critical value. However, a broad range of temperatures can coexist in equilibrium for this value of the ratio of ionizing intensity to pressure. Consequently, the flow is expected to be strongly inhomogeneous in temperature. The inferred distance of this material from the source of ionizing radiation depends on how much matter exists at the highest obtainable temperature. This distance can be measured by monitoring how ionic column densities respond to changes in the ionizing continuum on timescales of days to years.},
archivePrefix = {arXiv},
arxivId = {astro-ph/9502006},
author = {Fabian, A. C. and Reynolds, C. S.},
doi = {10.1086/323442},
eprint = {9502006},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Fabian, Reynolds - 2001 - Warm Absorbers in Active Galactic Nuclei.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
keywords = {Galaxies: Seyfert,Galaxies: active,Galaxies: nuclei,Quasars: absorption lines,Ultraviolet: galaxies,X-rays: galaxies},
number = {2},
pages = {684--690},
primaryClass = {astro-ph},
title = {{Warm Absorbers in Active Galactic Nuclei}},
url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-0035841719{\&}partnerID=tZOtx3y1},
volume = {561},
year = {2001}
}
@article{Hansen2018,
abstract = {Radiative cooling plays a crucial role in the dynamics of many astrophysical flows, and is particularly important in the dense shocked gas within Herbig-Haro (HH) objects and stellar jets. Simulating cooling processes accurately is necessary to compare numerical simulations with existing and planned observations of HH objects, such as those from the Hubble Space Telescope and the James Webb Space Telescope. In this paper, we discuss a new, non-equilibrium cooling scheme we have implemented into the three-dimensional magnetohydrodynamic (MHD) code ASTROBEAR. The new cooling function includes ionization, recombination, and excitation of all the important atomic species that cool below 10 000 K. We tested the routine by comparing its predictions with those from the well-tested onedimensional Cox-Raymond shock code (Raymond 1979). The results show that ASTROBEAR accurately tracks the ionization fraction, temperature, and other MHD variables for all lowvelocity (≲90 km s-1) magnetized radiative shock waves. The new routine allows us to predict synthetic emission maps in all the bright forbidden and permitted lines observed in stellar jets, including H$\alpha$, [NII], [OI], and [S II]. We present an example as to how these synthetic maps facilitate a direct comparison with narrowband images of HH objects.},
archivePrefix = {arXiv},
arxivId = {1809.02207},
author = {Hansen, E. C. and Hartigan, P. and Frank, A. and Wright, A. and Raymond, J. C.},
doi = {10.1093/mnras/sty2471},
eprint = {1809.02207},
file = {:home/william/Documents/Papers/1809.02207.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {(ISM:) Herbig-Haro objects,(magnetohydrodynamics) MHD,ISM: jets and outflows,Line: formation,Methods: numerical,Radiation mechanisms: thermal},
number = {3},
pages = {3098--3107},
title = {{Simulating radiative magnetohydrodynamical flows with ASTROBEAR: Implementation and applications of non-equilibrium cooling}},
volume = {481},
year = {2018}
}
@article{Lunardini2015,
abstract = {The Fermi Bubbles have been imaged in sub-TeV gamma rays at Fermi-LAT, and, if their origin is hadronic, they might have been seen with low statistics in {\$}\backslashsim 0.1- 1{\$} PeV neutrinos at IceCube. We discuss the detectability of these objects at the new High Altitude Water Cherenkov (HAWC) gamma ray detector. HAWC will view the North Bubble for {\$}\backslashsim 2-3{\$} hours a day, and will map its spectrum at 0.1-100 TeV. For the hard primary proton spectrum required to explain five events at IceCube, a high significance detection at HAWC will be achieved in less than 30 days. The combination of results at HAWC and IceCube will substantiate the hadronic model, or constrain its spectral parameters.},
author = {Lunardini, Cecilia and Razzaque, Soebur and Yang, Lili},
doi = {10.1103/PhysRevD.92.021301},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Lunardini, Razzaque, Yang - 2015 - Multimessenger study of the Fermi bubbles Very high energy gamma rays and neutrinos.pdf:pdf},
issn = {15502368},
journal = {Phys. Rev. D - Part. Fields, Gravit. Cosmol.},
number = {2},
pages = {1--5},
title = {{Multimessenger study of the Fermi bubbles: Very high energy gamma rays and neutrinos}},
volume = {92},
year = {2015}
}
@article{Rose2018a,
abstract = {Although now routinely incorporated into hydrodynamic simulations of galaxy evolution, the true importance of the feedback effect of the outflows driven by active galactic nuclei (AGNs) remains uncertain from an observational perspective. This is due to a lack of accurate information on the densities, radial scales and level of dust extinction of the outflow regions. Here we use the unique capabilities of VLT/Xshooter to investigate the warm outflows in a representative sample of nine local (0.06 {\textless} z {\textless} 0.15) Ultraluminous Infrared Galaxies (ULIRGs) with AGNs and, for the first time, accurately quantify the key outflow properties. We find that the outflows are compact (0.06 {\textless} R[O III] {\textless} 1.2 kpc), significantly reddened (median E(B-V){\~{}}0.5magnitudes), and have relatively high electron densities (3.4 {\textless} log10 ne (cm-3) {\textless} 4.8). It is notable that the latter densities - obtained using trans-auroral [S II] and [O II] emission-line ratios - exceed those typically assumed for the warm, emission-line outflows in active galaxies, but are similar to those estimated for broad and narrow absorption line outflow systems detected in some type 1 AGN. Even if we make the most optimistic assumptions about the true (deprojected) outflow velocities, we find relatively modest mass outflow rates (0.07 {\textless} M? {\textless} 14 M⊙ yr-1) and kinetic powers measured as a fraction of the AGN bolometric luminosities (4 × 10-4 {\textless} E/LBOL {\textless} 0.8 per cent). Therefore, although warm, AGN-driven outflows have the potential to strongly affect the star formation histories in the inner bulge regions (r {\~{}} 1 kpc) of nearby ULIRGs, we lack evidence that they have a significant impact on the evolution of these rapidly evolving systems on larger scales.},
archivePrefix = {arXiv},
arxivId = {1710.06600},
author = {Rose, Marvin and Tadhunter, Clive and Almeida, Cristina Ramos and Zaur{\'{i}}n, Javier Rodr{\'{i}}guez and Santoro, Francesco and Spence, Robert},
doi = {10.1093/MNRAS/STX2590},
eprint = {1710.06600},
file = {:home/william/Documents/Papers/stx2590.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: active,Galaxies: interactions,Quasars: emission lines,Quasars: general},
number = {1},
pages = {128--156},
title = {{Quantifying the AGN-driven outflows in ULIRGs (QUADROS) - I: VLT/Xshooter observations of nine nearby objects}},
volume = {474},
year = {2018}
}
@article{Martinez-Tibaduiza2020,
abstract = {In this work we demonstrate new BCH-like relations involving the generators of the su(1,1), su(2) and so(2,1) Lie algebras. We use our results to obtain in a straightforward way the composition of an arbitrary number of elements of the corresponding Lie groups. In order to make a self-consistent check of our results, as a first application we recover the non-trivial composition law of two arbitrary squeezing operators. As a second application, we show how our results can be used to compute the time evolution operator of physical systems described by time-dependent hamiltonians given by linear combinations of the generators of the aforementioned Lie algebras.},
archivePrefix = {arXiv},
arxivId = {2005.09500},
author = {Mart{\'{i}}nez-Tibaduiza, D. and Arag{\~{a}}o, A. H. and Farina, C. and Zarro, C. A.D.},
doi = {10.1016/j.physleta.2020.126937},
eprint = {2005.09500},
file = {:home/william/Documents/Papers/New BCH-like relations of the su(1, 1), su(2) and so(2, 1) Lie algebras sublined.pdf:pdf},
issn = {03759601},
journal = {Phys. Lett. Sect. A Gen. At. Solid State Phys.},
keywords = {Baker-Campbell-Hausdorff relations,Lie Algebras,Squeezed States,Time-dependent hamiltonians},
number = {36},
pages = {126937},
publisher = {Elsevier B.V.},
title = {{New BCH-like relations of the su(1,1), su(2) and so(2,1) Lie algebras}},
url = {https://doi.org/10.1016/j.physleta.2020.126937},
volume = {384},
year = {2020}
}
@article{2011ApJ...737...26N,
archivePrefix = {arXiv},
arxivId = {1007.3505},
author = {Novak, G.{\~{}}S. and Ostriker, J.{\~{}}P. and Ciotti, L},
doi = {10.1088/0004-637X/737/1/26},
eprint = {1007.3505},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Novak, Ostriker, Ciotti - 2011 - Feedback from central black holes in elliptical galaxies Two-dimensional models compared to one-dimensi.pdf:pdf},
journal = {Apj},
keywords = {cD,galaxies: active,galaxies: elliptical and lenticular,galaxies: nuclei,quasars: general},
pages = {26},
title = {{Feedback from Central Black Holes in Elliptical Galaxies: Two-dimensional Models Compared to One-dimensional Models}},
volume = {737},
year = {2011}
}
@article{Zubovas2019,
abstract = {Warm absorbers are found in many AGN and consist of clouds moving at moderate radial velocities, showing complex ionization structures and having moderate to large column densities. Using 1D numerical calculations, we confirm earlier suggestions that the energy released by an AGN pushes the surrounding gas outward in a bubble until this reaches transparency. Typical AGN episode durations of {\$}5\backslashtimes 10{\^{}}4{\$} yr supply enough energy for this, except in very gas-rich and/or very compact galaxies, such as those in the early Universe. In those galaxies, the AGN might remain hidden for many periods of activity, hiding the black hole growth. The typical radii of {\$}0.1-1{\$} kpc, velocities of {\$}100-1000{\$} km s{\$}{\^{}}{\{}-1{\}}{\$} and resulting optical depths are consistent with observations of warm absorbers. The resulting structure is a natural outcome of outflows driven by AGN buried in an optically thick gas envelope, and has a total mass comparable to the final {\$}M -\backslashsigma{\$} mass the central supermassive black hole will eventually reach.These results suggest that AGN can feed very efficiently by agitating this surrounding dense material. This may not be easy to observe, as this gas is Compton thick along many sightlines. The infall may produce episodic star formation in the centre, building up nuclear star clusters simultaneously with the growth of the central black hole.},
archivePrefix = {arXiv},
arxivId = {1901.02224},
author = {Zubovas, Kastytis and King, Andrew},
eprint = {1901.02224},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Zubovas, King - 2019 - Warm absorbers supermassive black hole feeding, and Compton-thick AGN.pdf:pdf},
keywords = {accretion,accretion discs,evolution,general,ism,quasars},
number = {January},
pages = {1--9},
title = {{Warm absorbers: supermassive black hole feeding, and Compton-thick AGN}},
url = {http://arxiv.org/abs/1901.02224},
volume = {9},
year = {2019}
}
@article{Mhd,
author = {Mhd, Week Astrophysical and Magneto-, Week Radiation and Stone, Jim},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Mhd, Magneto-, Stone - Unknown - Numerical Methods Numerical Methods for Astrophysical Two lectures on Numerical Methods.pdf:pdf},
pages = {1--17},
title = {{Numerical Methods Numerical Methods for Astrophysical Two lectures on Numerical Methods}},
volume = {M}
}
@article{Bolatto2013,
abstract = {CO line emission represents the most accessible and widely used tracer of the molecular ISM. This renders the translation of observed CO intensity into total H2 gas mass critical to understanding star formation and the ISM in our Galaxy and beyond. We review the theoretical underpinning, techniques, and results of efforts to estimate this CO-to-H2 "conversion factor," XCO, in different environments. In the Milky Way disk, we recommend a conversion factor of cm-2 (K km s-1)-1 with ±30{\%} uncertainty. Studies of other "normal galaxies" return similar values in Milky Way-like disks, but with greater scatter and systematic uncertainty. Departures from this Galactic conversion factor are both observed and expected. Dust-based determinations, theoretical arguments, and scaling relations all suggest that XCO increases with decreasing metallicity, turning up sharply below metallicity ∼1/3-1/2 solar in a manner consistent with model predictions that identify shielding as a key parameter. Based on spectral line modeling and dust observations, XCO appears to drop in the central, bright regions of some but not all galaxies, often coincident with regions of bright CO emission and high stellar surface density. This lower XCO is also present in the overwhelmingly molecular ISM of starburst galaxies, where several lines of evidence point to a lower CO-to-H2 conversion factor. At high redshift, direct evidence regarding the conversion factor remains scarce; we review what is known based on dynamical modeling and other arguments. Copyright {\textcopyright}2013 by Annual Reviews. All rights reserved.},
archivePrefix = {arXiv},
arxivId = {1301.3498},
author = {Bolatto, Alberto D. and Wolfire, Mark and Leroy, Adam K.},
doi = {10.1146/annurev-astro-082812-140944},
eprint = {1301.3498},
file = {:home/william/Documents/Papers/bolatto2013.pdf:pdf},
issn = {00664146},
journal = {Annu. Rev. Astron. Astrophys.},
keywords = {Galaxies: ISM,ISM: general,ISM: molecules,Radio lines: ISM},
number = {June},
pages = {207--268},
title = {{The CO-to-H2 conversion factor}},
volume = {51},
year = {2013}
}
@article{Bicknell2018,
abstract = {We propose that Gigahertz Peak Spectrum (GPS) and Compact Steep Spectrum (CSS) radio sources are the signposts of relativistic jet feedback in evolving galaxies. Our simulations of relativistic jets interacting with a warm, inhomogeneous medium, utilizing cloud densities and velocity dispersions in the range derived from optical observations, show that free-free absorption can account for the {\~{}} GHz peak frequencies and low-frequency power laws inferred from the radio observations. These new computational models replace a power-law model for the free-free optical depth a more fundamental model involving disrupted log-normal distributions of warm gas. One feature of our new models is that at early stages, the low-frequency spectrum is steep but progressively flattens as a result of a broader distribution of optical depths, suggesting that the steep low-frequency spectra discovered by Callingham et al. may possibly be attributed to young sources. We also investigate the inverse correlation between peak frequency and size and find that the initial location on this correlation is determined by the average density of the warm ISM. The simulated sources track this correlation initially but eventually fall below it, indicating the need for a more extended ISM than presently modelled. GPS and CSS sources can potentially provide new insights into the phenomenon of AGN feedback since their peak frequencies and spectra are indicative of the density, turbulent structure, and distribution of gas in the host galaxy.},
archivePrefix = {arXiv},
arxivId = {1801.06518},
author = {Bicknell, Geoffrey V. and Mukherjee, Dipanjan and Wagner, Alexander Y. and Sutherland, Ralph S. and Nesvadba, Nicole P.H.},
doi = {10.1093/mnras/sty070},
eprint = {1801.06518},
file = {:home/william/Documents/Papers/sty070.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: evolution,ISM: jets and outflows,Radio continuum: galaxies},
number = {3},
pages = {3493--3501},
title = {{Relativistic jet feedback - II. Relationship to gigahertz peak spectrum and compact steep spectrum radio galaxies}},
volume = {475},
year = {2018}
}
@article{Sobacchi2018,
abstract = {In the paradigm of magnetic launching of astrophysical jets, instabilities in the magnetohydrodynamic (MHD) flow are a good candidate to convert the Poynting flux into the kinetic energy of the plasma. If the magnetized plasma fills the almost entire space, the jet is unstable to helical perturbations of its body. However, the growth rate of these modes is suppressed when the poloidal component of the magnetic field has a vanishing gradient, which may be the actual case for a realistic configuration. Here we show that, if the magnetized plasma is confined into a limited region by the pressure of some external medium, the velocity shear at the contact surface excites unstable modes which can affect a significant fraction of the jet's body. We find that when the Lorentz factor of the jet is $\Gamma$ {\~{}} 10 ($\Gamma$ {\~{}} 100), these perturbations typically develop after propagating along the jet for tens (hundreds) of jet's radii. Surface modes may therefore play an important role in converting the energy of the jet from the Poynting flux to the kinetic energy of the plasma, particularly in active galactic nuclei. The scaling of the dispersion relation with (i) the angular velocity of the field lines and (ii) the sound speed in the confining gas is discussed.},
archivePrefix = {arXiv},
arxivId = {1709.01103},
author = {Sobacchi, E. and Lyubarsky, Y E},
doi = {10.1093/mnras/stx2592},
eprint = {1709.01103},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Lyubarsky - 2018 - External Confinement and Surface Modes in Magnetised Force-Free Jets arXiv 1709 . 01103v2 astro-ph . HE 3 Oct 2017.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: jets,Instabilities,MHD},
number = {2},
pages = {2813--2821},
title = {{External confinement and surface modes in magnetized force-free jets}},
volume = {473},
year = {2018}
}
@article{Inoue2020,
abstract = {We report our high-resolution (0.03 arcsec to 0.07 arcsec) ALMA imaging of the quadruply lensed radio-loud quasar MG$\backslash$,J0414+0534 at redshift {\$}z=2.639{\$} in the continuum and the broad CO(11-10) line at {\$}\backslashsim 340\backslash,{\$}GHz. With the help of strong lensing magnification and ALMA's high-resolution, we succeeded in resolving the jet/dust and CO gas in the quasar host galaxy both extending up to {\$}\backslashsim 1\backslash,{\$}kpc, with a resolution of {\$}\backslashsim 50\backslash,{\$}pc for the first time. Both the continuum emission and the CO(11-10) line have a similar bimodal structure aligned with the quasar jets ({\$}\backslashsim 200\backslash,{\$}pc) observed by Very Long Baseline Interferometry (VLBI) at {\$}5\backslash,{\$}GHz and {\$}8.4\backslash,{\$}GHz. The CO gas in the vicinity of both the eastern and western jet components at the location of {\$}\backslashsim 80\backslash,{\$}pc from the quasar core are moving at high velocities up to {\$}\backslashpm 600\backslash,{\$}{\$}\backslashtextrm{\{}km{\}}\backslash,\backslashtextrm{\{}s{\}}{\^{}}{\{}-1{\}}{\$} relative to the core. The observed features show clear evidence of strong interaction between the jets and interstellar medium (ISM). High temperature and high density environments in the ISM of the quasar host galaxy, as suggested from CO line ratios, also support this result. The small scale of the jets, the jet-ISM interaction, and the continuum spectral energy distribution of this source indicate that we are watching the infancy stage of quasar radio activity.},
archivePrefix = {arXiv},
arxivId = {2003.01650},
author = {Inoue, Kaiki Taro and Matsushita, Satoki and Nakanishi, Kouichiro and Minezaki, Takeo},
doi = {10.3847/2041-8213/ab7b7e},
eprint = {2003.01650},
file = {:home/william/Documents/Papers/[Inoue et al.]-ALMA 50-parsec-resolution Imaging of Jet–ISM Interaction.pdf:pdf},
issn = {2041-8213},
journal = {Astrophys. J.},
keywords = {Radio loud quasars,Radio jets,Molecular clouds,Str},
number = {2},
pages = {L18},
publisher = {IOP Publishing},
title = {{ALMA 50-parsec-resolution Imaging of Jet–ISM Interaction in the Lensed Quasar MG J0414+0534}},
url = {http://dx.doi.org/10.3847/2041-8213/ab7b7e},
volume = {892},
year = {2020}
}
@article{Ruffa2021,
abstract = {This is the fourth paper of a series investigating the AGN fuelling/feedback processes in a sample of eleven nearby low-excitation radio galaxies (LERGs). In this paper we present follow-up Atacama Large Millimeter/submillimeter Array (ALMA) observations of one source, NGC 3100, targeting the 12CO(1-0), 12CO(3-2), HCO+(4-3), SiO(3-2) and HNCO(6-5) molecular transitions. 12CO(1-0) and 12CO(3-2) lines are nicely detected and complement our previous 12CO(2-1) data. By comparing the relative strength of these three CO transitions, we find extreme gas excitation conditions (i.e. Tex ≳ 50 K) in regions that are spatially correlated with the radio lobes, supporting the case for a jet-ISM interaction. An accurate study of the CO kinematics demonstrates that, although the bulk of the gas is regularly rotating, two distinct non-rotational kinematic components can be identified in the inner gas regions: one can be associated to inflow/outflow streaming motions induced by a two-armed spiral perturbation; the second one is consistent with a jet-induced outflow with vmax ≈ 200 km s−1 and {\$}\backslashdot{\{}M{\}}\backslashlesssim 0.12{\$} M⊙ yr−1. These values indicate that the jet-CO coupling ongoing in NGC 3100 is only mildly affecting the gas kinematics, as opposed to what expected from existing simulations and other observational studies of (sub-)kpc scale jet-cold gas interactions. HCO+(4-3) emission is tentatively detected in a small area adjacent to the base of the northern radio lobe, possibly tracing a region of jet-induced gas compression. The SiO(3-2) and HNCO(6-5) shock tracers are undetected: this - along with the tentative HCO+(4-3) detection - may be consistent with a deficiency of very dense (i.e. ncrit {\textgreater} 106 cm−3) cold gas in the central regions of NGC 3100.},
archivePrefix = {arXiv},
arxivId = {2112.00755},
author = {Ruffa, Ilaria and Prandoni, Isabella and Davis, Timothy A and Laing, Robert A and Paladino, Rosita and Casasola, Viviana and Parma, Paola and Bureau, Martin},
doi = {10.1093/mnras/stab3541},
eprint = {2112.00755},
file = {:home/william/Documents/Papers/2112.00755.pdf:pdf},
issn = {0035-8711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {active,cd,elliptical and lenticular,evolution,galaxies,ism,nuclei},
number = {December},
pages = {1--20},
title = {{The AGN fuelling/feedback cycle in nearby radio galaxies - IV. Molecular gas conditions and jet-ISM interaction in NGC 3100}},
volume = {20},
year = {2021}
}
@article{Miralles-Caballero2011,
abstract = {We present a comprehensive characterization of the general properties (luminosity functions (LFs), mass, size, ages, etc.) of optically selected compact stellar objects (knots) in a representative sample of 32 low-z luminous and ultraluminous infrared galaxies ((U)LIRGs). It is important to understand the formation and evolution of these properties in such systems, which represent the most extreme cases of starbursts in the low-z universe. We have made use of high angular resolution Advanced Camera for Surveys images from the Hubble Space Telescope in F435W (B) and F814W (I) bands. The galaxies in the sample represent different interaction phases (first contact, pre-merger, merger, and post-merger) and cover a wide luminosity range (11.46 ≤ log (L IR/L) ≤ 12.54). With a median size of 32pc, most of the nearly 3000 knots detected consist of complexes of star clusters. Some of the knots (15{\%}) are so blue that their colors indicate a young (i.e., {\textless}30Myr) and almost extinction-free population. There is a clear correlation of the mass of these blue knots with their radius, where MR 1.91 0.14, similar to that found in complexes of clusters in M51 and in giant molecular clouds. This suggests that the star formation within the knots is proportional to the gas density at any given radius. This relation does not depend significantly on either the infrared luminosity of the system or the interaction phase. The star formation of all the knots is characterized by LFs of the knots with slopes close to 2. Nevertheless, we see a marginally significant indication that the LF evolves with the interaction process, becoming steeper from early to advanced merger phases. Due to size-of-sample effects we are probably sampling knots in ULIRGs that intrinsically more luminous (by a factor of about four) than in less luminous systems. They also have sizes and are likely to have masses characteristic of clumps in galaxies at z ≳ 1. Knots in post-mergers are on average (1.3-2 times) larger, more luminous (2 mag) in the I band, and 0.5mag redder than those in systems in earlier phases. Two scenarios are briefly discussed: (1) the likely presence of relatively high extinction in the most advanced mergers and (2) the dissolution of the less massive clusters and/or their coalescence into more massive, evolved superclusters. {\textcopyright} 2011. The American Astronomical Society. All rights reserved.},
archivePrefix = {arXiv},
arxivId = {1107.1777},
author = {Miralles-Caballero, Daniel and Colina, Luis and Arribas, Santiago and Duc, Pierre Alain},
doi = {10.1088/0004-6256/142/3/79},
eprint = {1107.1777},
file = {:home/william/Documents/Papers/Miralles-Caballero.pdf:pdf},
issn = {00046256},
journal = {Astron. J.},
keywords = {galaxies: evolution,galaxies: interactions,galaxies: photometry,galaxies: star clusters: general,galaxies: starburst},
number = {3},
title = {{Characterization of optically selected star-forming knots in (U)LIRGs}},
volume = {142},
year = {2011}
}
@article{Heber2003,
abstract = {We discovered that HD 188112, a bright (V = $\backslash$magpt{\{}10{\}}{\{}2{\}}), nearby (80 pc) B-type star, is a unique subluminous B (sdB) star. SdB stars are usually identified with models of core helium burning Extreme Horizontal-Branch (EHB) stars of half a solar mass. A spectral analysis of the hydrogen and helium lines resulted in T{\_}eff = 21 500 +/- 500 K, log g = 5.66 +/- 0.05 placing the star below the EHB. HD 188112 was found to be radial velocity (RV) variable and the RV curve has been measured to be perfectly sinusoidal with a period of 0.606585 days and a semi-amplitude of 188.3 km s-1 indicating that it is a close binary system. From the atmospheric parameters and the Hipparcos parallax we conclude that the sdB star is of low mass (0.24 Msun). The mass of the sdB is too low to sustain core helium burning and it is now evolving into a helium core white dwarf. A lower limit to the mass of its unseen companion of 0.73 Msun is derived from the mass function. Because the companion does not contribute to the spectral energy distribution from the UV to the infrared it cannot be a main sequence star but must be a white dwarf (WD), a neutron star (NS) or a black hole. The system would qualify as pre-supernova Ia candidate (sdB+WD) if its total mass is above the Chandrasekhar limit (1.4 Msun), or as post-supernova (sdB+NS) if the companion mass is above that limit, requiring the inclination angle to be lower than 51deg or 48deg, respectively. Based on observations collected at the German-Spanish Astronomical Center (DSAZ), Calar Alto, operated by the Max-Planck-Institut f{\"{u}}r Astronomie, Heidelberg jointly with the Spanish National Commission for Astronomy. Based on observations collected at the European Southern Observatory (ESO proposal No. 65.H-0341(A) and 69.D-0016(A)).},
archivePrefix = {arXiv},
arxivId = {astro-ph/0304271},
author = {Heber, U and Edelmann, H and Lisker, T and Napiwotzki, R},
doi = {10.1051/0004-6361},
eprint = {0304271},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Heber et al. - 2003 - Letter to the Editor Astronomy.pdf:pdf},
isbn = {0009-8981 (Print)},
issn = {00098981},
journal = {Astron. Astrophys. Lett.},
keywords = {binaries,early-type,fundamental parameters,hd 188112,individual,spectroscopic,stars},
pages = {477--480},
pmid = {11432396},
primaryClass = {astro-ph},
title = {{Letter to the Editor Astronomy}},
volume = {480},
year = {2003}
}
@article{Cattaneo2009,
abstract = {Virtually all massive galaxies, including our own, host central black holes ranging in mass from millions to billions of solar masses. The growth of these black holes releases vast amounts of energy that powers quasars and other weaker active galactic nuclei. A tiny fraction of this energy, if absorbed by the host galaxy, could halt star formation by heating and ejecting ambient gas. A central question in galaxy evolution is the degree to which this process has caused the decline of star formation in large elliptical galaxies, which typically have little cold gas and few young stars, unlike spiral galaxies. {\textcopyright} 2009 Macmillan Publishers Limited. All rights reserved.},
author = {Cattaneo, A. and Faber, S. M. and Binney, J. and Dekel, A. and Kormendy, J. and Mushotzky, R. and Babul, A. and Best, P. N. and Br{\"{u}}ggen, M. and Fabian, A. C. and Frenk, C. S. and Khalatyan, A. and Netzer, H. and Mahdavi, A. and Silk, J. and Steinmetz, M. and Wisotzki, L.},
doi = {10.1038/nature08135},
file = {:home/william/Documents/Papers/cattaneo2009.pdf:pdf},
issn = {00280836},
journal = {Nature},
number = {7252},
pages = {213--219},
title = {{The role of black holes in galaxy formation and evolution}},
volume = {460},
year = {2009}
}
@article{Kraemer2017a,
abstract = {XMM-Newton and Suzaku spectra of AGN have revealed highly ionized gas, in the form of absorption lines from H-like and He-like Fe. Some of these absorbers, "Ultra Fast Outflows (UFOs)", have radial velocities of up to 0.25c. We have undertaken a detailed photo-ionization study of high-ionization Fe absorbers, both UFOs and non-UFOs, in a sample of AGN observed by XMM-Newton. We find that the heating and cooling processes in UFOs are Compton-dominated, unlike the non-UFOs. Both types are characterized by Force Multipliers on the order of unity, which suggests that they cannot be radiatively accelerated in sub-Eddington AGN, unless they were much less ionized at their point of origin. However, such highly ionized gas can be accelerated via a Magneto-Hydrodynamic (MHD) wind. We explore this possibility by applying a cold MHD flow model to the UFO in the well-studied Seyfert galaxy, NGC 4151. We find that the UFO can be accelerated along magnetic streamlines anchored in the accretion disk. In the process, we have been able to constrain the magnetic field strength and the magnetic pressure in the UFO and have determined that the system is not in magnetic/gravitational equipartition.Open questions include the variability of the UFOs and the apparent lack of non-UFOs in UFO sources.},
archivePrefix = {arXiv},
arxivId = {1711.07965},
author = {Kraemer, S. B. and Tombesi, F. and Bottorff, M. C.},
doi = {10.3847/1538-4357/aa9ce0},
eprint = {1711.07965},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Kraemer, Tombesi, Bottorff - 2017 - Physical Conditions in Ultra Fast Outflows in AGN.pdf:pdf},
issn = {1538-4357},
keywords = {accretion,accretion disks,active,galaxies,x-rays},
title = {{Physical Conditions in Ultra Fast Outflows in AGN}},
url = {http://arxiv.org/abs/1711.07965{\%}0Ahttp://dx.doi.org/10.3847/1538-4357/aa9ce0},
volume = {35},
year = {2017}
}
@article{Susanne2010,
abstract = {Supernova explosions are very violent events which transfer a significant amount of en-ergy to the interstellar medium (ISM) and are responsible for a large variety of physical processes. We will not discuss the actual explosion mechanisms here which are thought to be due to carbon deflagration of white dwarfs (type I) or the core collapse of massive stars (type II) but we will follow the dynamical evolution of the supernova remnant (SNR), i.e. the expanding cloud of hot gas in the ISM. This evolution can be divided into different phases according to the dominant physical processes, and simplified models can be made at least for the first stages, to get an idea of typical time scales, expansion velocities and sizes. Free Expansion Phase The shock wave created by the explosion moves outwards into the (more or less homo-geneous) interstellar gas at highly supersonic speed. During the first phase of the SNR evolution the surrounding ISM has no influence on the expansion of the shock wave, i.e. the pressure of the interstellar gas is negligible. Assuming that most of the supernova energy E SN (on the order of 10 44},
author = {Susanne, H},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Susanne - 2010 - Dynamical Evolution of Supernova Remnants Lecture Notes.pdf:pdf},
pages = {1--4},
title = {{Dynamical Evolution of Supernova Remnants Lecture Notes}},
year = {2010}
}
@article{Salome2016,
abstract = {NGC 5128 (Centaurus A) is one of the best example to study AGN-feedback in the local Universe. At 13.5 kpc from the galaxy, optical filaments with recent star formation are lying along the radio-jet direction. We used the Atacama Pathfinder EXperiment (APEX) to map the CO(2-1) emission all along the filaments structure. Molecular gas mass of (8.2 ± 0.5) × 107 M$\alpha$ was found over the 4.2 kpc-structure which represents about 3{\%} of the total gas mass of the NGC 5128 cold gas content. Two dusty mostly molecular structures are identified, following the optical filaments. The region corresponds to the crossing of the radio jet with the northern H i shell, coming from a past galaxy merger. One filament is located at the border of the H i shell, while the other is entirely molecular, and devoid of H i gas. The molecular mass is comparable to the H i mass in the shell, suggesting a scenario where the atomic gas was shocked and transformed in molecular clouds by the radio jet. Comparison with combined far-IR Herschel and UV GALEX estimation of star formation rates in the same regions leads to depletion times of more than 10 Gyr. The filaments are thus less efficient than discs in converting molecular gas into stars. Kinetic energy injection triggered by shocks all along the jet and gas interface is a possible process that appears to be consistent with MUSE line ratio diagnostics derived in a smaller region of the northern filaments. Whether the AGN is the sole origin of this energy input and what is the dominant (mechanical vs. radiative) mode for this process is however still to be investigated.},
author = {Salom{\'{e}}, Q. and Salom{\'{e}}, P. and Combes, F. and Hamer, S.},
doi = {10.1051/0004-6361/201628970},
file = {:home/william/Documents/Papers/[Salome et al.]-Star formation efficiency along the radio jet in Centaurus A.pdf:pdf},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Galaxies: evolution,Galaxies: individual: Centaurus A,Galaxies: interactions,Galaxies: star formation,Methods: data analysis,Radio lines: galaxies},
pages = {1--13},
title = {{Atomic-to-molecular gas phase transition triggered by the radio jet in Centaurus A}},
volume = {595},
year = {2016}
}
@article{Tombesi2012a,
abstract = {Using the results of a previous X-ray photo-ionization modelling of blue-shifted Fe K absorption lines on a sample of 42 local radio-quiet AGNs observed with XMM-Newton, in this letter we estimate the location and energetics of the associated ultra-fast outflows (UFOs). Due to significant uncertainties, we are essentially able to place only lower/upper limits. On average, their location is in the interval {\~{}}0.0003-0.03pc ({\~{}}10{\^{}}2-10{\^{}}4 r{\_}s) from the central black hole, consistent with what is expected for accretion disk winds/outflows. The mass outflow rates are constrained between {\~{}}0.01-1 M{\_}{\{}$\backslash$odot{\}} yr{\^{}}{\{}-1{\}}, corresponding to {\textgreater}5-10{\%} of the accretion rates. The average lower-upper limits on the mechanical power are log$\backslash$dot{\{}E{\}}{\_}K{\~{}}42.6-44.6 erg s{\^{}}{\{}-1{\}}. However, the minimum possible value of the ratio between the mechanical power and bolometric luminosity is constrained to be comparable or higher than the minimum required by simulations of feedback induced by winds/outflows. Therefore, this work demonstrates that UFOs are indeed capable to provide a significant contribution to the AGN cosmological feedback, in agreement with theoretical expectations and the recent observation of interactions between AGN outflows and the interstellar medium in several Seyferts galaxies.},
author = {Tombesi, F. and Cappi, M. and Reeves, J. N. and Braito, V.},
doi = {10.1111/j.1745-3933.2012.01221.x},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Tombesi et al. - 2012 - Evidence for ultrafast outflows in radio-quiet AGNs – III . Location and energetics.pdf:pdf},
isbn = {0306090201},
issn = {17453933},
journal = {Mon. Not. R. Astron. Soc. Lett.},
keywords = {Accretion,Accretion discs,Black hole physics,Galaxies: active,X-rays: galaxies},
number = {1},
title = {{Evidence for ultrafast outflows in radio-quiet AGNs - III. Location and energetics}},
volume = {422},
year = {2012}
}
@article{Ishibashi2015,
abstract = {Galaxy-scale outflows, which are thought to provide the link connecting the central black hole to its host galaxy, are now starting to be observed. However, the physical origin of the mechanism driving the observed outflows, whether due to energy-driving or radiation-driving, is still debated; and in some cases, it is not clear whether the central source is an active galactic nucleus (AGN) or a nuclear starburst. Here we study the role of radiation pressure on dust in driving galactic-scale AGN outflows, and analyse the dynamics of the outflowing shell as a function of the underlying physical parameters. We show that high-velocity outflows ({\$}\backslashgtrsim{\$}1000 km/s) with large momentum flux ({\$}\backslashgtrsim 10 L/c{\$}) can be obtained, by taking into account the effects of radiation trapping. In particular, the high observed values of the momentum boosts can be reproduced, provided that the shell is initially optically thick to the reprocessed infrared radiation. Alternatively, the inferred measurements of the momentum flux may be significantly biased by AGN variability. In this context, the observations of powerful outflows on kiloparsec scales, with no or weak signs of ongoing nuclear activity at the present time, could be re-interpreted as relics of past AGN episodes.},
archivePrefix = {arXiv},
arxivId = {1504.07393},
author = {Ishibashi, W. and Fabian, A. C.},
doi = {10.1093/mnras/stv944},
eprint = {1504.07393},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ishibashi, Fabian - 2015 - AGN feedback Galactic-scale outflows driven by radiation pressure on dust.pdf:pdf},
isbn = {bibcode:2015arXiv150407393I},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Black hole physics,Galaxies: active,Galaxies: evolution,Radiation: dynamics},
number = {1},
pages = {93--102},
title = {{AGN feedback: Galactic-scale outflows driven by radiation pressure on dust}},
volume = {451},
year = {2015}
}

@ARTICLE{Morganti2015,
       author = {{Morganti}, Raffaella and {Oosterloo}, Tom and {Oonk}, J.~B. Raymond and {Frieswijk}, Wilfred and {Tadhunter}, Clive},
        title = "{The fast molecular outflow in the Seyfert galaxy IC 5063 as seen by ALMA}",
      journal = {\aap},
     keywords = {galaxies: active, galaxies: individual: IC 5063, ISM: jets and outflows, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = aug,
       volume = {580},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/201525860},
archivePrefix = {arXiv},
       eprint = {1505.07190},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...580A...1M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{Gan2014a,
abstract = {Based on two-dimensional high-resolution hydrodynamic numerical simulation, we study the mechanical and radiative feedback effects from the central active galactic nucleus (AGN) on the cosmological evolution of an isolated elliptical galaxy. The inner boundary of the simulation domain is carefully chosen so that the fiducial Bondi radius is resolved and the accretion rate of the black hole is determined self-consistently. It is well known that when the accretion rates are high and low, the central AGNs will be in cold and hot accretion modes, which correspond to the radiative and kinetic feedback modes, respectively. The emitted spectrum from the hot accretion flows is harder than that from the cold accretion flows, which could result in a higher Compton temperature accompanied by a more efficient radiative heating, according to previous theoretical works. Such a difference of the Compton temperature between the two feedback modes, the focus of this study, has been neglected in previous works. Significant differences in the kinetic feedback mode are found as a result of the stronger Compton heating. More importantly, if we constrain models to correctly predict black hole growth and AGN duty cycle after cosmological evolution, we find that the favored model parameters are constrained: mechanical feedback efficiency diminishes with decreasing luminosity (the maximum efficiency being {\~{}}= 10-3.5), and X-ray Compton temperature increases with decreasing luminosity, although models with fixed mechanical efficiency and Compton temperature can be found that are satisfactory as well. We conclude that radiative feedback in the kinetic mode is much more important than previously thought.},
archivePrefix = {arXiv},
arxivId = {1403.0670},
author = {Gan, Zhaoming and Yuan, Feng and Ostriker, Jeremiah P and Ciotti, Luca and Novak, Gregory S},
doi = {10.1088/0004-637X/789/2/150},
eprint = {1403.0670},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Gan et al. - 2014 - Active galactic nucleus feedback in an isolated elliptical galaxy The effect of strong radiative feedback in the kin.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {accretion,accretion disks,black hole physics,cD,galaxies: active,galaxies: elliptical and lenticular,galaxies: evolution,galaxies: nuclei},
number = {2},
pages = {14},
title = {{Active galactic nucleus feedback in an isolated elliptical galaxy: The effect of strong radiative feedback in the kinetic mode}},
volume = {789},
year = {2014}
}
@article{Blandford2019a,
abstract = {The nuclei of most normal galaxies contain supermassive black holes, which can accrete gas through a disk and become active. These active galactic nuclei (AGNs) can form jets that are observed on scales from astronomical units to megaparsecs and from meter wavelengths to TeV energies. High-resolution radio imaging and multiwavelength/messenger campaigns are elucidating the conditions under which this happens. Evidence is presented that: □ Relativistic AGN jets are formed when the black hole spins and the the accretion disk is strongly magnetized, perhaps on account of gas accreting at high latitude beyond the black hole sphere of influence. □ AGN jets are collimated close to the black hole by magnetic stress associated with a disk wind. □ Higher-power jets can emerge from their galactic nuclei in a relativistic, supersonic, and proton-dominated state, and they terminate in strong, hot spot shocks; lower-power jets are degraded to buoyant plumes and bubbles. □ Jets may accelerate protons to EeV energies, which contribute to the cosmic ray spectrum and may initiate pair cascades that can efficiently radiate synchrotron $\gamma$-rays. □ Jets were far more common when the Universe was a few billion years old and black holes and massive galaxies were growing rapidly. □ Jets can have a major influence on their environments, stimulating and limiting the growth of galaxies. The observational prospects for securing our understanding of AGN jets are bright.},
archivePrefix = {arXiv},
arxivId = {1812.06025},
author = {Blandford, Roger and Meier, David and Readhead, Anthony},
doi = {10.1146/annurev-astro-081817-051948},
eprint = {1812.06025},
file = {:home/william/Documents/Papers/1812.06025.pdf:pdf},
issn = {00664146},
journal = {Annu. Rev. Astron. Astrophys.},
keywords = {active galactic nuclei,black holes,blazars,extragalactic radio sources,jets,$\gamma$-ray sources},
pages = {467--509},
title = {{Relativistic Jets from Active Galactic Nuclei}},
volume = {57},
year = {2019}
}
@article{Lehnert2009,
abstract = {We analyze the physical conditions in the interstellar gas of 11 actively star-forming galaxies at z2, based on integral-field spectroscopy from the ESO-VLT and Hubble Space Telescope/Near Infrared Camera and Multi-Object Spectrometer imaging. We concentrate on the high H$\alpha$ surface brightnesses, large line widths, line ratios, and the clumpy nature of these galaxies. We show that photoionization calculations and emission line diagnostics imply gas pressures and densities that are similar to the most intense nearby star-forming regions at z = 0 but over much larger scales (10-20 kpc). A relationship between surface brightness and velocity dispersion can be explained through simple energy injection arguments and a scaling set by nearby galaxies with no free parameters. The high velocity dispersions are a natural consequence of intense star formation thus regions of high velocity dispersion are not evidence for mass concentrations such as bulges or rings. External mechanisms such as cosmological gas accretion generally do not have enough energy to sustain the high velocity dispersions. In some cases, the high pressures and low gas metallicites may make it difficult to robustly distinguish between active galactic nucleus ionization cones and star formation, as we show for BzK-15504 at z = 2.38. We construct a picture where the early stages of galaxy evolution are driven by self-gravity which powers strong turbulence until the velocity dispersion is high. Then massive, dense, gas-rich clumps collapse, triggering star formation with high efficiencies and intensities as observed. At this stage, the intense star formation is likely self-regulated by the mechanical energy output of massive stars. {\textcopyright} 2009. The American Astronomical Society. All rights reserved.},
author = {Lehnert, M. D. and Nesvadba, N. P.H. and Tiran, L. Le and Matteo, P. Di and {Van Driel}, W. and Douglas, L. S. and Chemin, L. and Bournaud, F.},
doi = {10.1088/0004-637X/699/2/1660},
file = {:home/william/Documents/Papers/Lehnert{\_}2009{\_}ApJ{\_}699{\_}1660.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {Cosmology: observations,Galaxies: evolution,Galaxies: kinematics and dynamics,Infrared: galaxies},
number = {2},
pages = {1660--1678},
title = {{Physical conditions in the interstellar medium of intensely star-forming galaxies at redshift ∼ 2}},
volume = {699},
year = {2009}
}
@article{Draine2003,
abstract = {This review surveys the observed properties of interstellar dust grains: the wavelength-dependent extinction of starlight, including absorption features, from UV to IR; optical luminescence; IR emission; microwave emission; optical, UV, and X-ray scattering by dust; and polarization of starlight and of infrared emission. The relationship between presolar grains in meteorites and the interstellar grain population is discussed. Candidate grain materials and abundance constraints are considered. A dust model consisting of amorphous silicate grains, graphite grains, and PAHs is compared with observed emission and scattering. Some issues concerning evolution of interstellar dust are discussed.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0304489},
author = {Draine, B.T.},
doi = {10.1146/annurev.astro.41.011802.094840},
eprint = {0304489},
file = {:home/william/Documents/Papers/0304489.pdf:pdf},
issn = {0066-4146},
journal = {Annu. Rev. Astron. Astrophys.},
keywords = {infrared astronomy,interstellar grains,interstellar medium,light scattering},
number = {1},
pages = {241--289},
primaryClass = {astro-ph},
title = {{Interstellar Dust Grains}},
volume = {41},
year = {2003}
}
@article{Crocker2011,
abstract = {Recently evidence has emerged for enormous features in the gamma-ray sky observed by the Fermi-LAT instrument: bilateral `bubbles' of emission centered on the core of the Galaxy and extending to around 10 kpc above and below the Galactic plane. These structures are coincident with a non-thermal microwave `haze' found in WMAP data and an extended region of X-ray emission detected by ROSAT. The bubbles' gamma-ray emission is characterised by a hard and relatively uniform spectrum, relatively uniform intensity, and an overall luminosity {\~{}}4 x 10{\^{}}37 erg/s, around one order of magnitude larger than their microwave luminosity while more than order of magnitude less than their X-ray luminosity. Here we show that the bubbles are naturally explained as due to a population of relic cosmic ray protons and heavier ions injected by processes associated with extremely long timescale ({\textgreater}{\~{}}8 Gyr) and high areal density star-formation in the Galactic center.},
author = {Crocker, Roland M. and Aharonian, Felix},
doi = {10.1103/PhysRevLett.106.101102},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Crocker, Aharonian - 2011 - Fermi bubbles Giant, multibillion-year-old reservoirs of galactic center cosmic rays.pdf:pdf},
issn = {10797114},
journal = {Phys. Rev. Lett.},
number = {10},
pages = {1--4},
title = {{Fermi bubbles: Giant, multibillion-year-old reservoirs of galactic center cosmic rays}},
volume = {106},
year = {2011}
}
@article{Morganti2017c,
abstract = {Analytical and numerical galaxy-formation models indicate that active galactic nuclei (AGNs) likely play a prominent role in the formation and evolution of galaxies. However, quantifying this effect requires knowledge of how the nuclear activity proceeds throughout the life of a galaxy, whether it alternates with periods of quiescence and, if so, on what timescales these cycles occur. This topic has attracted growing interest, but making progress remains a challenging task. For optical and radio AGNs, a variety of techniques are used to perform a kind of 'archaeology' that traces the signatures of past nuclear activity. Here we summarize recent findings regarding the lifecycle of an AGN from optical and radio observations. The limited picture we have so far suggests that these cycles can range from long periods of 107-108 yr to shorter periods of 104-105 yr, even reaching extreme events on timescales of just a few years. Together with simulations, observational results regarding the multiple cycles of AGN activity help to create a complete picture of the AGN lifecycle.},
archivePrefix = {arXiv},
arxivId = {1709.01667},
author = {Morganti, Raffaella},
doi = {10.1038/s41550-017-0223-0},
eprint = {1709.01667},
file = {:home/william/Documents/Papers/[Morganti, Raffaela]arqueology of AGNs.pdf:pdf},
issn = {23973366},
journal = {Nat. Astron.},
number = {9},
pages = {596--605},
title = {{Archaeology of active galaxies across the electromagnetic spectrum}},
volume = {1},
year = {2017}
}
@article{DeBoer2014,
abstract = {The diffuse gamma-ray sky revealed 'Bubbles' of emission above and below the Galactic Plane symmetric around the centre of the Milky Way with a height of 10 kpc in both directions. At present there is no convincing explanation for the origin. To understand the role of the Galactic Centre (GC) one has to study the Bubble spectrum inside the disc, a region which has been excluded from previous analysis because of the large foreground. From a novel template fit, which allows a simultaneous determination of the signal and foreground in any direction, we find that bubble-like emission is not only found in the halo, but in the Galactic Plane as well with a width in latitude coinciding with the molecular clouds. The longitude distribution has a width corresponding to the Galactic Bar with an additional contribution from the Scutum-Centaurus arm. The energy spectrum of the Bubbles coincides with the predicted contribution from CRs trapped in sources (SCRs). Also the energetics fits well. Hence, we conclude that the bubble-like emission has a hadronic origin, which arises from SCRs and the Bubbles in the halo arise from hadronic interactions in advected gas. Evidence for advection is provided by the ROSAT X-rays from hot gas in the Bubble region.},
author = {{De Boer}, Wim and Weber, Markus},
doi = {10.1088/2041-8205/794/1/L17},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/De Boer, Weber - 2014 - Fermi bubbles and bubble-like emission from the galactic plane.pdf:pdf},
issn = {20418213},
journal = {Astrophys. J. Lett.},
keywords = {Galaxy: structure,acceleration of particles,gamma rays: ISM,gamma rays: diffuse background,methods: numerical,shock waves},
number = {1},
pages = {1--6},
title = {{Fermi bubbles and bubble-like emission from the galactic plane}},
volume = {794},
year = {2014}
}
@article{DeAvillez2004a,
abstract = {The role of matter circulation between the disk and halo in establishing the volume filling factors of the different ISM phases in the Galactic disk (|z| ≤ 250 pc) is investigated, using a modified version of the three-dimensional supernova-driven ISM model of Avillez (2000). We carried out adaptive mesh refinement simulations of the ISM with five supernova rates (in units of the Galactic value), $\sigma$/$\sigma$Gal = 1, 2, 4, 8 and 16 (corresponding to starburst conditions) using three finer level resolutions of 2.5, 1.25 and 0.625 pc, allowing us to understand how resolution would affect the volumes of gas phases in pressure equilibrium. We find that the volume filling factors of the different ISM phases depend sensitively on the existence of a duty cycle between the disk and halo acting as a pressure release valve for the hot (T {\textgreater} 105.5 K) phase in the disk. The amount of cold gas (defined as the gas with T {\textless} 103 K) picked up in the simulations varies from a value of 19{\%} for $\sigma$/$\sigma$Gal = 1 to ∼5{\%} for $\sigma$/$\sigma$Gal = 4 and ≤1{\%} for higher SN rates. Background heating prevents the cold gas from immediate collapse and thus ensures the stability of the cold gas phase. The mean occupation fraction of the hot phase varies from about 17{\%} for the Galactic SN rate to ∼28{\%}, for $\sigma$/$\sigma$Gal = 4, and to 44{\%} for $\sigma$/$\sigma$Gal = 16. Overall the filling factor of the hot gas does not increase much as we move towards higher SN rates, following a power law of fv,hot∝ ($\sigma$/$\sigma$Gal)0.363, Such a modest dependence on the SN rate is a consequence of the evacuation of the hot phase into the halo through the duty cycle. This leads to volume filling factors of the hot phase considerably smaller than those predicted in the three-phase model of McKee {\&} Ostriker (1977) even in the absence of magnetic fields.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0407034},
author = {{De Avillez}, M. A. and Breitschwerdt, D.},
doi = {10.1051/0004-6361:200400025},
eprint = {0407034},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/De Avillez, Breitschwerdt - 2004 - Volume filling factors of the ISM phases in star forming galaxies I. The role of the disk-halo intera.pdf:pdf},
issn = {00046361},
journal = {Astron. Astrophys.},
keywords = {Galaxies: Ism,Galaxies: Kinematics and dynamics,ISM: Structure},
number = {3},
pages = {899--911},
primaryClass = {astro-ph},
title = {{Volume filling factors of the ISM phases in star forming galaxies I. The role of the disk-halo interaction}},
volume = {425},
year = {2004}
}
@article{Silantev2009,
abstract = {We consider the integral light polarization from optically thick accretion disks. Basic mechanism is the multiple light scattering on free electrons (Milne's problem) in magnetized atmosphere. The Faraday rotation of the polarization plane changes both the value of integral polarization degree {\$}p{\$} and the position angle {\$}\backslashchi {\$}. Besides, the characteristic spectra of these values appear. We are testing the known relation between magnetic field of black hole at the horizon {\$}B{\_}{\{}BH{\}}{\$} and its mass {\$}M{\_}{\{}BH{\}}{\$}, and the usual power-law distribution inside the accretion disk. The formulae for {\$}p(\backslashlambda){\$} and {\$}\backslashchi(\backslashlambda){\$} depend on a number of parameters describing the particular dependence of magnetic field in accretion disk (the index of power-law distribution, the spin of the black hole, etc.). Comparison of our theoretical values of {\$}p{\$} and {\$}\backslashchi {\$} with observed polarization can help us to choice more realistic values of parameters if the accretion disk mechanism gives the main contribution to the observed integral polarization. The main content is connected with estimation of validity of the relation between {\$}B{\_}{\{}BH{\}}{\$} and {\$}M{\_}{\{}BH{\}}{\$}. We found for the AGN NGC 4258 that such procedure does not confirm the mentioned correlation between magnetic field and mass of black hole.},
archivePrefix = {arXiv},
arxivId = {0908.2725},
author = {Silant'ev, N. A. and Piotrovich, M Yu and Gnedin, Yu N and Natsvlishvili, T M},
eprint = {0908.2725},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Silant et al. - 2018 - THE BLACK HOLE MASS AND MAGNETIC FIELD CORRELATION IN AGN TESTING BY OPTICAL POLARIMETRY.pdf:pdf},
keywords = {accretion disks m edd,are the ordinary and,eddington accretion rates,polarization - magnetic fields,respec-},
title = {{The Black Hole Mass and Magnetic Field Correlation in AGN: Testing by Optical Polarimetry}},
url = {http://arxiv.org/abs/0908.2725},
year = {2009}
}
@article{Morganti2017b,
abstract = {The energy released by Active Galactic Nuclei (AGN) in the form of radiation, winds, or radio plasma jets, is known to impact on the surrounding interstellar medium. The result of these processes, known as AGN (negative) feedback, is suggested to prevent gas, in and around galaxies, from cooling, and to remove, or at least redistribute, gas by driving massive and fast outflows, hence playing a key role in galaxy evolution. Given its importance, a large effort is devoted by the astronomical community to trace the effects of AGN on the surrounding gaseous medium and to quantify their impact for different types of AGN. This review briefly summarizes some of the recent observational results obtained in different wavebands, tracing different phases of the gas. I also summarize the new insights they have brought, and the constraints they provide to numerical simulations of galaxy formation and evolution. The recent addition of deep observations of cold gas and, in particular, of cold molecular gas, has brought some interesting surprises and has expanded our understanding of AGN and AGN feedback.},
archivePrefix = {arXiv},
arxivId = {1712.05301},
author = {Morganti, Raffaella},
doi = {10.3389/fspas.2017.00042},
eprint = {1712.05301},
file = {:home/william/Documents/Papers/fspas-04-00042.pdf:pdf},
issn = {2296987X},
journal = {Front. Astron. Sp. Sci.},
keywords = {active galactic nuclei,extragalactic radio jets,interstellar medium,outflows,spectroscopy},
number = {November},
pages = {1--10},
title = {{The Many Routes to AGN Feedback}},
volume = {4},
year = {2017}
}
@article{Misawa2018,
abstract = {We search for velocity changes (i.e., acceleration/deceleration) of narrow absorption lines (NALs) that are intrinsic to the quasars, using spectra of 6 bright quasars that have been observed more than once with 8-10m class telescopes. While variations in line strength and profile are frequently reported (especially in broader absorption lines), definitive evidence for velocity shifts has not been found with only a few exceptions. Direct velocity shift measurements are valuable constraints on the acceleration mechanisms. In this study, we determine velocity shifts by comparing the absorption profiles of NALs at two epochs separated by more than 10 years in the observed frame, using the cross-correlation function method and we estimate the uncertainties using Monte Carlo simulations. We do not detect any significant shifts but we obtain 3{\$}\backslashsigma{\$} upper limits on the acceleration of intrinsic NALs (compared to intervening NALs in same quasars) of {\$}\backslashsim{\$}0.7 km s{\$}{\^{}}{\{}-1{\}}{\$} yr{\$}{\^{}}{\{}-1{\}}{\$} ({\$}\backslashsim{\$}0.002 cm s{\$}{\^{}}{\{}-2{\}}{\$}). We discuss possible scenarios for non-detection of NAL acceleration/deceleration and examine resulting constraints on the physical conditions in accretion disk wind.},
archivePrefix = {arXiv},
arxivId = {1809.07476},
author = {Misawa, Toru and Eracleous, Michael and Charlton, Jane C. and Kashikawa, Nobunari},
eprint = {1809.07476},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Misawa et al. - 2018 - Direct Measurement of Quasar Outflow Wind Acceleration.pdf:pdf},
title = {{Direct Measurement of Quasar Outflow Wind Acceleration}},
url = {http://arxiv.org/abs/1809.07476},
year = {2018}
}
@book{Netzer2006,
author = {Netzer, H},
doi = {10.1007/3-540-34621-X},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Netzer - 2006 - Active Galactic Nuclei Basic Physics and Main Components.pdf:pdf},
isbn = {354034621X},
pages = {1--38},
title = {{Active Galactic Nuclei : Basic Physics and Main Components}},
volume = {38},
year = {2006}
}
@article{Solano,
author = {Solano, C M D},
file = {:home/william/Documents/Papers/Plasma{\_}effects{\_}on{\_}quantum{\_}light.pdf:pdf},
pages = {3--4},
title = {{Plasma effects on quantum light}}
}
@article{2013ApJ...763L..18W,
archivePrefix = {arXiv},
arxivId = {1211.5851},
author = {Wagner, A.{\~{}}Y. and Umemura, M and Bicknell, G.{\~{}}V.},
doi = {10.1088/2041-8205/763/1/L18},
eprint = {1211.5851},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Wagner, Umemura, Bicknell - 2013 - Ultrafast outflows Galaxy-scale active galactic nucleus feedback.pdf:pdf},
journal = {Apjl},
keywords = {ISM: jets and outflows,galaxies: evolution,galaxies: formation,hydrodynamics,methods: numerical},
pages = {L18},
title = {{Ultrafast Outflows: Galaxy-scale Active Galactic Nucleus Feedback}},
volume = {763},
year = {2013}
}
@article{Juneau2021,
abstract = {There is growing evidence for physical influence between supermassive black holes and their host galaxies. We present a case study of nearby galaxy NGC 7582, for which we find evidence that galactic substructure plays an important role in affecting the collimation of ionized outflows as well as contributing to the heavy active galactic nucleus (AGN) obscuration. This result contrasts with a simple, small-scale AGN torus model, according to which AGN wind collimation may take place inside the torus itself, at subparsec scale. Using 3D spectroscopy with the MUSE instrument, we probe the kinematics of the stellar and ionized gas components as well as the ionization state of the gas from a combination of emission line ratios. We report for the first time a kinematically distinct core (KDC) in NGC 7582, on a scale of {\~{}}600pc. This KDC coincides spatially with dust lanes and starbursting complexes previously observed. We interpret it as a circumnuclear ring of stars and dusty, gas-rich material. We obtain a clear view of the outflowing cones over kpc scales, and demonstrate that they are predominantly photoionized by the central engine. We detect the back cone (behind the galaxy), and confirm previous results of a large nuclear obscuration of both the stellar continuum and HII regions. While we tentatively associate the presence of the KDC to a large-scale bar and/or a minor galaxy merger, we stress the importance of gaining a better understanding of the role of galaxy substructure in controlling the fueling, feedback and obscuration of AGN.},
archivePrefix = {arXiv},
arxivId = {2112.08380},
author = {Juneau, St{\'{e}}phanie and Goulding, Andy D. and Banfield, Julie and Bianchi, Stefano and Duc, Pierre-Alain and Ho, I-Ting and Dopita, Michael A. and {Scharw {\"{a}}chter}, Julia and Bauer, Franz E. and Groves, Brent and Alexander, David M. and Davies, Rebecca L. and Elbaz, David and Freeland, Emily and Hampton, Elise and Kewley, Lisa J. and Nikutta, Robert and Shastri, Prajval and Shu, Xinwen and Vogt, Fr{\'{e}}d{\'{e}}ric P. A. and Wang, Tao and Wong, O. Ivy and Woo, Jong-Hak},
eprint = {2112.08380},
file = {:home/william/Documents/Papers/2112.08380.pdf:pdf},
title = {{The Black Hole-Galaxy Connection: Interplay between Feedback, Obscuration, and Host Galaxy Substructure}},
url = {http://arxiv.org/abs/2112.08380},
year = {2021}
}
@article{Tombesi2017,
abstract = {We present a spectral analysis of a 200ks observation of the broad-line radio galaxy 3C120, performed with the high-energy transmission grating spectrometer on board the Chandra X-ray Observatory. We find (i) a neutral absorption component intrinsic to the source with a column density of N log 20.67 0.05 H =  cm −2 ; (ii) no evidence for a warm absorber (WA) with an upper limit on the column density of just N log 19.7 H {\textless} cm −2 , assuming the typical ionization parameter log$\xi$;2.5 erg s −1 cm; the WA may instead be replaced by (iii) a hot emitting gas with a temperature kT;0.7 keV observed as soft X-ray emission from ionized Fe L-shell lines, which may originate from a kiloparsec-scale shocked bubble inflated by the active galactic nucleus (AGN) wind or jet with a shock velocity of about 1000 km s −1 determined by the emission line width; (iv) a neutral Fe K$\alpha$ line and accompanying emission lines indicative of a Compton-thick cold reflector with a low reflection fraction R;0.2, suggesting a large opening angle of the torus; (v) a highly ionized Fe XXV emission feature indicative of photoionized gas with an ionization parameter log 3.75 0.38 0.27 x = -+ ergs −1 cm and a column density of N log 22 H {\textgreater} cm −2 localized within ∼2pc from the X-ray source; and (vi) possible signatures of a highly ionized disk wind. Together with previous evidence for intense molecular line emission, these results indicate that 3C120 is likely a late-state merger undergoing strong AGN feedback.},
archivePrefix = {arXiv},
arxivId = {1703.00516},
author = {Tombesi, F. and Mushotzky, R. F. and Reynolds, C. S. and Kallman, T. and Reeves, J. N. and Braito, V. and Ueda, Y. and Leutenegger, M. A. and Williams, B. J. and Stawarz, {\L}. and Cappi, M.},
doi = {10.3847/1538-4357/aa6342},
eprint = {1703.00516},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Tombesi et al. - 2017 - Feeding and Feedback in the Powerful Radio Galaxy 3C 120.pdf:pdf},
issn = {1538-4357},
journal = {Astrophys. J.},
keywords = {active,black hole physics,black hole physics,galaxies: active,line: identifi,galaxies,identi fi cation,line,x-rays},
number = {1},
pages = {16},
publisher = {IOP Publishing},
title = {{Feeding and Feedback in the Powerful Radio Galaxy 3C 120}},
url = {http://stacks.iop.org/0004-637X/838/i=1/a=16?key=crossref.5e349d2463f5a93d2b23c77642dabf8a},
volume = {838},
year = {2017}
}
@article{Melioli2006a,
abstract = {In the present study, considering the physical conditions that are relevant in interactions between supernova remnants (SNRs) and dense molecular clouds for triggering star formation we have built a diagram of SNR radius versus cloud density in which the constraints above delineate a shaded zone where star formation is allowed. We have also performed fully 3D radiatively cooling numerical simulations of the impact between SNRs and clouds under different initial conditions in order to follow the initial steps of these interactions. We determine the conditions that may lead either to cloud collapse and star formation or to complete cloud destruction and find that the numerical results are consistent with those of the SNR-cloud density diagram. Finally, we have applied the results above to the $\beta$ Pictoris stellar association which is composed of low-mass post-T Tauri stars with an age of 11 Myr. It has been recently suggested that its formation could have been triggered by the shock wave produced by an SN explosion localized at a distance of about 62 pc that may have occurred either in the Lower Centaurus Crux or in the Upper Centaurus Lupus which are both nearby older subgroups of that association (Ortega and co-workers). Using the results of the analysis above we have shown that the suggested origin for the young association at the proposed distance is plausible only for a very restricted range of initial conditions for the parent molecular cloud, that is, a cloud with a radius of the order of 10 pc and density of the order of 20 cm-3 and a temperature of the order of 50-100 K. {\textcopyright} 2006 RAS.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0608207},
author = {Melioli, C. and {De Gouveia Dal Pino}, E. M. and {De La Reza}, R. and Raga, A.},
doi = {10.1111/j.1365-2966.2006.11076.x},
eprint = {0608207},
file = {:home/william/Documents/Papers/mnras0373-0811.pdf:pdf},
issn = {00358711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {ISM: clouds,Stars: formation,Supernova remnants},
number = {2},
pages = {811--818},
primaryClass = {astro-ph},
title = {{Star formation triggered by SN explosions: An application to the stellar association of $\beta$ Pictoris}},
volume = {373},
year = {2006}
}
@article{Qiu2020,
abstract = { Aims. We investigate the physical and chemical conditions of molecular gas in the circumnuclear disk (CND) region of NGC 1068.  Methods. We carried out a spectral line survey with the IRAM 30 m telescope toward the center of NGC 1068 and mainly focused on the 2 mm band with a frequency coverage of 160.7–168.6 GHz and 176.5–184.3 GHz.  Results. Fifteen lines are detected in NGC 1068, eight of which are new detections for this galaxy. We derive the rotation temperatures and column densities of fourteen molecular species.  Conclusions. Based on the [HCO + (2 − 1)]/[HOC + (2 − 1)] ratio, we obtain a high ionization degree in the CND of NGC 1068. It is found that HC 3 N is concentrated in the east knot, while 13 CCH, CH 3 CN, SO, HOC + , CS, CH 3 CCH, and H 2 CO are concentrated in the west knot. Compared to the star-forming galaxies M 82 and NGC 253, the chemistry of NGC 1068 might be less strongly affected by the UV radiation field, and its kinetic temperature might be lower. },
archivePrefix = {arXiv},
arxivId = {2001.08697},
author = {Qiu, Jianjie and Zhang, Jiangshui and Zhang, Yong and Jia, Lanwei and Tang, Xindi},
doi = {10.1051/0004-6361/201935800},
eprint = {2001.08697},
file = {:home/william/Documents/Papers/[Qiu et al.]-2mm  spectroscopy observations toward the circumnuclear.pdf:pdf},
issn = {0004-6361},
journal = {Astron. Astrophys.},
keywords = {active,galaxies,individual,ism,molecules,ngc 1068,nuclei},
pages = {A125},
title = {{ $\lambda$ = 2 mm spectroscopy observations toward the circumnuclear disk of NGC 1068 }},
volume = {634},
year = {2020}
}
@article{Dobbs2011,
abstract = {We perform calculations of isolated disc galaxies to investigate how the properties of the interstellar medium (ISM), the nature of molecular clouds and the global star formation rate depend on the level of stellar feedback. We adopt a simple physical model, which includes a galactic potential, a standard cooling and heating prescription of the ISM and self-gravity of the gas. Stellar feedback is implemented by injecting energy into dense, gravitationally collapsing gas, but is independent of the Schmidt-Kennicutt relation. We obtain fractions of gas, and filling factors for different phases of the ISM in reasonable agreement with observations. Supernovae are found to be vital to reproduce the scaleheights of the different components of the ISM, and velocity dispersions. The giant molecular clouds (GMCs) formed in the simulations display mass spectra similar to the observations, their normalization depend on the level of feedback. We find {\~{}}40per cent of the clouds exhibit retrograde rotation, induced by cloud-cloud collisions. The star formation rates we obtain are in good agreement with the observed Schmidt-Kennicutt relation, and are not strongly depend on the star formation efficiency we assume, being largely self-regulated by the feedback. We also investigate the effect of spiral structure by comparing calculations with and without the spiral component of the potential. The main difference with a spiral potential is that more massive GMCs are able to accumulate in the spiral arms. Thus we are able to reproduce massive GMCs, and the spurs seen in many grand design galaxies, even with stellar feedback. The presence of the spiral potential does not have an explicit effect on the star formation rate, but can increase the star formation rate indirectly by enabling the formation of long-lived, strongly bound clouds. {\textcopyright} 2011 The Authors. Monthly Notices of the Royal Astronomical Society {\textcopyright} 2011 RAS.},
archivePrefix = {arXiv},
arxivId = {arXiv:1107.0154v1},
author = {Dobbs, C. L. and Burkert, A. and Pringle, J. E.},
doi = {10.1111/j.1365-2966.2011.19346.x},
eprint = {arXiv:1107.0154v1},
file = {:home/william/Documents/Papers/1107.0154.pdf:pdf},
issn = {00358711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: ISM,Hydrodynamics,ISM: clouds,ISM: evolution,ISM: kinematics and dynamics},
number = {2},
pages = {1318--1334},
title = {{The properties of the interstellar medium in disc galaxies with stellar feedback}},
volume = {417},
year = {2011}
}
@article{CacioppoJohnT.;Sandman1978,
abstract = {An analytical model of a prestressed concrete reactor vessel (PCRV) for LMFBR and the associated finite element com- puter code, involving an explicit time integration procedure, is described. The model is axisymmetric and includes simula- tions of the tensile cracking of concrete, the reinforcement, and a prestressing capability. The tensile cracking of concrete and the steel reinforcement are both modeled as continuously distr{\~{}}uted within the finite element. The stresses in the rein- forcement and concrete are computed separately and combined to give an overall stress state of the composite material. The reinformcement is assumed to be elastic, perfectly-plastic; the concrete is taken to be elastic, with tensile and com- pressive stress limits. Cracking of concrete is based on the criterion of maximum principal stress; a crack is assumed to form normal to the direction of the maximum principal stress. Attention is also given to the fact that cracks do not form instan- taneously, but develop gradually. Thus, after crack initiation the normal stress is reduced to zero gradually as a function of time. Residual shear resistance of cracks due to aggregate interlock is also taken into account. An existing crack is permitted to close. Prestressing of the PCRV is modeled by special structural members which represent an averaged prestressing layer equivalent to an axisymmetric shell. The internal prestressing members are superimposed over the reinforced concrete body of the PCRV; they are permitted to stretch and slide in a predetermined path, simulating the actual tendons. The validity of the code is examined by comparison with experimental data. Both static and dynamic data are com- pared with code predictions, and the agreement is satisfactory. A preliminary design has been developed for both pool and loop-type PCRVs. The code was applied to the analysis of these designs. This analysis reveals that the critical locations in such a design would be the head cover and the junction between the cover and the vessel wall and indicates the pattern of crack development. The results show that the development of a design adequate for current HCDA loads is quite feasible for pool-type or loop-type PCRVs.},
author = {{Cacioppo, John T.; Sandman}, Curt A.},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Unknown - 1978 - No Title.pdf:pdf},
isbn = {9789896540821},
number = {3},
pages = {377--389},
title = {{No 主観的健康感を中心とした在宅高齢者における 健康関連指標に関する共分散構造分析Title}},
volume = {2},
year = {1978}
}
@article{Cox2005,
abstract = {The interstellar medium in the vicinity of the Sun is arranged in large-scale structures of bubble walls, sheets, and filaments of warm gas, within which close to the midplane there are subsheets and filaments of cold dense material; the whole occupies roughly half the available volume and extends with decreasing mean density to at least a kiloparsec off the plane. The remainder of the volume is in bubble interiors, cavities, and tunnels of much lower density, with some but not all of those lower density regions hot enough to be observable via their X-ray emission. This entire system is pervaded by a rather strong and irregular magnetic field and cosmic rays, the pressures of which are confined by the weight of the interstellar gas, particularly that far from the plane where gravity is strong. Observations suggest that the cosmic rays and magnetic field have an even more extended vertical distribution than the warm gas, requiring either the weight of additional coronal material or magnetic tension to confine it to the disk. Adjusting one's perception of this medium to embrace the known aspects is difficult. After this adjustment, there are many problems to solve and prejudices to overcome - the weak role of thermal instability, the suppression of certain gravitational instabilities, the problem of determining the state in the low-density regions, the twin difficulties of not having too much OVI (O +5) and getting enough diffuse 3/4 keV X-ray emission, the possible importance of large old-barrel-shaped supernova remnants in clarifying matters, the possible role of dust evolution in adjusting the heating to make clouds stable, the factors influencing the magnitudes of the interstellar pressure and scale height - things that global models of the medium might examine to clarify some of these matters; attention to these details and more constitute the challenge of this subject. Copyright {\textcopyright} 2005 by Annual Reviews. All rights reserved.},
author = {Cox, Donald P.},
doi = {10.1146/annurev.astro.43.072103.150615},
file = {:home/william/Documents/Papers/cox2005.pdf:pdf},
issn = {00664146},
journal = {Annu. Rev. Astron. Astrophys.},
keywords = {Dust,Galaxies,Interstellar medium,Milky Way,Supernova remnants,X rays},
pages = {337--385},
title = {{The three-phase interstellar medium revisited}},
volume = {43},
year = {2005}
}
@article{Fluetsch2019,
abstract = {We study molecular outflows in a sample of 45 local galaxies, both star forming and active galactic nucleus (AGN), primarily by using CO data from the Atacama Large Millimeter/submillimeter Array (ALMA) archive and from the literature. For a subsample, we also compare the molecular outflow with the ionized and neutral atomic phases. We infer an empirical analytical function relating the outflow rate simultaneously to the star formation rate (SFR), L AGN, and galaxy stellar mass; this relation is much tighter than the relations with the individual quantities. The outflow kinetic power shows a larger scatter than in previous, more biased studies, spanning from 0.1 to 5 per cent of L AGN, while the momentum rate ranges from 1 to 30 times L AGN /c, indicating that these outflows can be both energy driven, but with a broad range of coupling efficiencies with the interstellar medium (ISM), and radiation pressure driven. For about 10 per cent of the objects, the outflow energetics significantly exceed the maximum theoretical values; we interpret these as 'fossil outflows' resulting from activity of a past strong AGN, which has now faded. We estimate that, in the stellar mass range probed here ({\textgreater} 10 10 ,M⊙), less than 5 per cent of the outflowing gas escapes the galaxy. The molecular gas depletion time associated with the outflow can be as short as a few million years in powerful AGN; however, the total gas (H 2 + Hi) depletion times are much longer. Altogether, our findings suggest that even AGN-driven outflows might be relatively ineffective in clearing galaxies of their entire gas content, although they are likely capable of clearing and quenching the central region.},
author = {Fluetsch, A. and Maiolino, R. and Carniani, S. and Marconi, A. and Cicone, C. and Bourne, M. A. and Costa, T. and Fabian, A. C. and Ishibashi, W. and Venturi, G.},
doi = {10.1093/mnras/sty3449},
file = {:home/william/Documents/Papers/sty3449.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {galaxies: ISM,galaxies: active,galaxies: evolution,galaxies: star formation,quasars: general},
number = {4},
pages = {4586--4614},
publisher = {Oxford University Press},
title = {{Cold molecular outflows in the local Universe and their feedback effect on galaxies}},
volume = {483},
year = {2019}
}
@article{Booth2013a,
abstract = {Energetic feedback from supernovae (SNe) and from active galactic nuclei (AGN) are both important processes that are thought to control how much gas is able to condense into galaxies and form stars. We show that although both AGN and SNe suppress star formation, they mutually weaken one another's effect by up to an order of magnitude in haloes in the mass range for which both feedback processes are efficient (). These results demonstrate the importance of the simultaneous, non-independent inclusion of these two processes in models of galaxy formation to estimate the total feedback strength. These results are of particular relevance to the interpretation of results from hydrodynamical simulations that model only one of the feedback processes, and also to those semi-analytic models that implicitly assume the effects of the two feedback processes to be independent.},
archivePrefix = {arXiv},
arxivId = {1203.3802},
author = {Booth, C. M. and Schaye, Joop},
doi = {10.1038/srep01738},
eprint = {1203.3802},
file = {:home/william/Documents/Papers/srep01738.pdf:pdf},
issn = {20452322},
journal = {Sci. Rep.},
pages = {1--5},
title = {{The interaction between feedback from active galactic nuclei and supernovae}},
volume = {3},
year = {2013}
}
@article{Zhang2020,
abstract = {The Fermi bubbles are two giant bubbles in gamma rays lying above and below the Galactic center (GC). Despite numerous studies on the bubbles, their origin and emission mechanism remain elusive. Here we use a suite of hydrodynamic simulations to study the scenario where the cosmic rays (CRs) in the bubbles are mainly accelerated at the forward shocks driven by a pair of opposing jets from Sgr A*. We find that an active galactic nucleus (AGN) jet event happened {\$}5-6{\$} Myr ago can naturally reproduce the bilobular morphology of the bubbles, and the postshock gas temperature in the bubbles is heated to {\$}\backslashsim0.4{\$} keV, consistent with recent X-ray observations. The forward shocks compress the hot halo gas, and at low latitudes, the compressed gas shows an X-shaped structure, naturally explaining the biconical X-ray structure in the ROSAT 1.5 keV map in both morphology and X-ray surface brightness. CR acceleration is most efficient in the head regions of the bubbles during the first 2 Myrs. The opposing jets release a total energy of {\$}\backslashsim 10{\^{}}{\{}55{\}}{\$} erg with an Eddington ratio of {\$}\backslashsim 10{\^{}}{\{}-3{\}}{\$}, which falls well in the range of the hot accretion flow mode for black holes. Our simulations further show that the forward shocks driven by spherical winds at the GC typically produce bubbles with much wider bases than observed, and could not reproduce the X-shaped X-ray structure at low latitudes. This suggests that starburst or AGN winds are unlikely the origin of the bubbles in the shock scenario.},
archivePrefix = {arXiv},
arxivId = {2003.03625},
author = {Zhang, Ruiyu and Guo, Fulai},
eprint = {2003.03625},
file = {:home/william/Documents/Papers/[Zhang]-SIMULATING THE FERMI BUBBLES AS FORWARD SHOCKS DRIVEN BY AGN JETS.pdf:pdf},
keywords = {active,cosmic rays,galaxies,galaxy,gamma rays,halo,jets},
title = {{Simulating the Fermi Bubbles as Forward Shocks driven by AGN Jets}},
url = {http://arxiv.org/abs/2003.03625},
year = {2020}
}
@article{Bon2018,
abstract = {Here we present a critical view of practical problems in the analysis of optical Fe II emission lines of Type 1 AGN spectra. Besides the very complex and unclear physical interpretation of the Fe II template shape, there are other issues that might affect the results of Fe II contribution as well (like the S/N, the AGN continuum component modelling, the complex shapes of other broad and narrow emission lines that are blending in the same part of the spectrum, the galactic host stellar component that could lead to mimicking of the Fe II template shape on some parts of spectrum, etc.). In this paper we concentrate particularly on the claims of possibility that in some objects Fe II could be strongly shifted to the red. We examine the effects in the fitting procedure that could artificially lead to such results.},
archivePrefix = {arXiv},
arxivId = {1812.05828},
author = {Bon, E. and Marziani, P. and Berton, M. and Bon, N. and Antonucci, R. and Gaskell, M. and Ferland, G.},
eprint = {1812.05828},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Bon et al. - 2018 - Fe II velocity shifts in optical spectra of type 1 AGN.pdf:pdf},
number = {April 2018},
pages = {0--7},
title = {{Fe II velocity shifts in optical spectra of type 1 AGN}},
url = {http://arxiv.org/abs/1812.05828},
year = {2018}
}
@misc{Silk2017,
abstract = {Could there be intermediate mass black holes in essentially all old dwarf galaxies? I argue that current observations of Active Galactic Nuclei in dwarfs allow such a radical hypothesis which provides early feedback and potentially provides a unifying explanation for many if not all of the apparent dwarf galaxy anomalies, such as the abundance, core-cusp,”too big to fail”, ultra-faint and baryon-fraction issues. I describe the supporting arguments, which are largely circumstantial in nature, and discuss a number of tests. There is no strong motivation for modifying the nature of cold dark matter in order to explain any of the dwarf galaxy”problems”.},
archivePrefix = {arXiv},
arxivId = {1703.08553},
author = {Silk, Joseph},
booktitle = {arXiv},
doi = {10.3847/2041-8213/aa67da},
eprint = {1703.08553},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Silk - 2017 - March 28, 2017 FEEDBACK BY MASSIVE BLACK HOLES IN DWARF GALAXIES.pdf:pdf},
issn = {23318422},
title = {{Feedback by massive black holes in dwarf galaxies}},
year = {2017}
}
@book{Madejski2016,
abstract = {This article reviews the recent observational results regarding $\gamma$ -ray emission from active galaxies. The most numerous discrete extragalactic $\gamma$ -ray sources are AGNs dominated by relativistic jets pointing in our direction (commonly known as blazars), and they are the main subject of the review. They are de-tected in all observable energy bands and are highly variable. The advent of the sensitive $\gamma$ -ray observations, afforded by the launch and continuing op-eration of the Fermi Gamma-ray Space Telescope and the AGILE Gamma-ray Imaging Detector, as well as by the deployment of current-generation Air Cerenkov Telescope arrays such as VERITAS, MAGIC, and HESS-II, con-tinually provides sensitive $\gamma$ -ray data over the energy range of ∼100 MeV to multi-TeV. Importantly, it has motivated simultaneous, monitoring obser-vations in other bands, resulting in unprecedented time-resolved broadband spectral coverage. After an introduction, in Sections 3, 4, and 5, we cover the current status and highlights of $\gamma$ -ray observations with (mainly) Fermi but also AGILE and put those in the context of broadband spectra in Sec-tion 6. We discuss the radiation processes operating in blazars in Section 7, and we discuss the content of their jets and the constraints on the loca-tion of the energy dissipation regions in, respectively, Sections 8 and 9. Sec-tion 10 covers the current ideas for particle acceleration processes in jets, and Section 11 discusses the coupling of the jet to the accretion disk in the host galaxy. Finally, Sections 12, 13, and 14 cover, respectively, the contribution of blazars to the diffuse $\gamma$ -ray background, the utility of blazars to study the extragalactic background light, and the insight they provide for study of populations of supermassive black holes early in the history of the Universe.},
author = {Madejski, Grzegorz (Greg) and Sikora, Marek},
booktitle = {Annu. Rev. Astron. Astrophys.},
doi = {10.1146/annurev-astro-081913-040044},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Madejski, Sikora - 2016 - Gamma-Ray Observations of Active Galactic Nuclei.pdf:pdf},
isbn = {0819130400},
issn = {0066-4146},
keywords = {agn jets,gamma-rays,supermassive black holes},
number = {1},
pages = {725--760},
title = {{Gamma-Ray Observations of Active Galactic Nuclei}},
url = {http://www.annualreviews.org/doi/10.1146/annurev-astro-081913-040044},
volume = {54},
year = {2016}
}
@article{Zhuang2020,
archivePrefix = {arXiv},
arxivId = {2007.11283},
author = {Zhuang, Ming-Yang and Ho, Luis C.},
doi = {10.3847/1538-4357/ab8f2e},
eprint = {2007.11283},
file = {:home/william/Documents/Papers/2007.11283.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {active,galaxies,ism,star formation},
number = {2},
pages = {108},
title = {{The Interplay between Star Formation and Black Hole Accretion in Nearby Active Galaxies}},
volume = {896},
year = {2020}
}
@article{Cielo2018,
abstract = {Feedback by Active Galactic Nuclei is often divided into quasar and radio mode, powered by radiation or radio jets, respectively. Both are fundamental in galaxy evolution, especially in late-type galaxies, as shown by cosmological simulations and observations of jet-ISM interactions in these systems. We compare AGN feedback by radiation and by collimated jets through a suite of simulations, in which a central AGN interacts with a clumpy, fractal galactic disc. We test AGN of {\$}10{\^{}}{\{}43{\}}{\$} and {\$}10{\^{}}{\{}46{\}}{\$} erg/s, considering jets perpendicular or parallel to the disc. Mechanical jets drive the more powerful outflows, exhibiting stronger mass and momentum coupling with the dense gas, while radiation heats and rarifies the gas more. Radiation and perpendicular jets evolve to be quite similar in outflow properties and effect on the cold ISM, while inclined jets interact more efficiently with all the disc gas, removing the densest {\$}20\backslash{\%}{\$} in {\$}20{\$} Myr, and thereby reducing the amount of cold gas available for star formation. All simulations show small-scale inflows of {\$}0.01-0.1{\$} M{\$}{\_}\backslashodot{\$}/yr, which can easily reach down to the Bondi radius of the central supermassive black hole (especially for radiation and perpendicular jets), implying that AGN modulate their own duty cycle in a feedback/feeding cycle.},
archivePrefix = {arXiv},
arxivId = {1712.03955},
author = {Cielo, Salvatore and Bieri, Rebekka and Volonteri, Marta and Wagner, Alexander Y and Dubois, Yohan},
doi = {10.1093/mnras/sty708},
eprint = {1712.03955},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Cielo et al. - 2018 - AGN feedback compared jets versus radiation 1 I N T RO D U C T I O N.pdf:pdf},
issn = {1365-2966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {galaxies,ism,jets,methods,numerical,quasars,radiative transfer},
pages = {1336--1355},
title = {{AGN Feedback Compared: Jets versus Radiation}},
volume = {1355},
year = {2018}
}
@article{Yang2012,
abstract = {The Fermi Gamma-Ray Space Telescope reveals two large bubbles in the Galaxy, which extend nearly symmetrically {\~{}}50° above and below the Galactic center. Using three-dimensional (3D) magnetohydrodynamic simulations that self-consistently include the dynamical interaction between cosmic rays (CRs) and thermal gas and anisotropic CR diffusion along the magnetic field lines, we show that the key characteristics of the observed gamma-ray bubbles and the spatially correlated X-ray features in the ROSAT 1.5 keV map can be successfully reproduced by recent jet activity from the central active galactic nucleus. We find that after taking into account the projection of the 3D bubbles onto the sky the physical heights of the bubbles can be much smaller than previously thought, greatly reducing the formation time of the bubbles to about a Myr. This relatively small bubble age is needed to reconcile the simulations with the upper limit of bubble ages estimated from the cooling time of high-energy electrons. No additional physical mechanisms are required to suppress large-scale hydrodynamic instabilities because the evolution time is too short for them to develop. The simulated CR bubbles are edge-brightened, which is consistent with the observed projected flat surface brightness distribution. Furthermore, we demonstrate that the sharp edges of the observed bubbles can be due to anisotropic CR diffusion along magnetic field lines that drape around the bubbles during their supersonic expansion, with suppressed perpendicular diffusion across the bubble surface. Possible causes of the slight bends of the Fermi bubbles to the west are also discussed.},
author = {Yang, H. Y.K. and Ruszkowski, M. and Ricker, P. M. and Zweibel, E. and Lee, D.},
doi = {10.1088/0004-637X/761/2/185},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Yang et al. - 2012 - The Fermi bubbles Supersonic active galactic nucleus jets with anisotropic cosmic-ray diffusion.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {Galaxy: nucleus,cosmic rays,diffusion,gamma rays: galaxies,magnetohydrodynamics (MHD),methods: numerical},
number = {2},
title = {{The Fermi bubbles: Supersonic active galactic nucleus jets with anisotropic cosmic-ray diffusion}},
volume = {761},
year = {2012}
}
@article{Ferrari1998,
abstract = {▪ Abstract Extragalactic jets were discovered and initially studied by radio astronomers in connection with extended radio sources. At present, the combination of jets and disks is considered the crucial element in unification models for all active galactic nuclei (AGNs). The acceleration and propagation conditions of jets, together with the aspect ratio of the disk/jet geometry with respect to the observer, shape the morphologies of AGNs. However, these phenomenological models are very complex from the physical and mathematical point of view, as they involve different elements of the theories of gravitation, fluid dynamics, and electrodynamics in a highly nonlinear combination and in conditions not easily reproducible in laboratory plasma or fluid experiments. In the last ten years, theorists have attacked the subject with advanced analytical and numerical methods, and some important results have already been established that confirm the global scenario, although we are still far from a complete physical...},
author = {Ferrari, Attilio},
doi = {10.1146/annurev.astro.36.1.539},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ferrari - 1998 - Modeling Extragalactic Jets.pdf:pdf},
issn = {0066-4146},
journal = {Annu. Rev. Astron. Astrophys.},
keywords = {astrophysical fluid dynamics,galactic nuclei,radio astronomy},
number = {1},
pages = {539--598},
title = {{Modeling Extragalactic Jets}},
url = {http://www.annualreviews.org/doi/10.1146/annurev.astro.36.1.539},
volume = {36},
year = {1998}
}
@article{Cresci2018,
abstract = {Galaxy-scale outflows powered by actively accreting supermassive black holes are routinely detected, and they have been associated both with suppression and triggering of star formation. Recent observational evidence and simulations are favouring a delayed mechanism that connects outflows and star formation},
archivePrefix = {arXiv},
arxivId = {1802.10305},
author = {Cresci, Giovanni and Maiolino, Roberto},
doi = {10.1038/s41550-018-0404-5},
eprint = {1802.10305},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Cresci, Maiolino - 2018 - Observing positive and negative AGN feedback.pdf:pdf},
issn = {23973366},
journal = {Nat. Astron.},
number = {3},
pages = {179--180},
title = {{Observing positive and negative AGN feedback}},
volume = {2},
year = {2018}
}
@article{Yang2014a,
abstract = {We analyze 60 months of all sky data from the Fermi-LAT. The Fermi Bubble structures discovered previously are clearly revealed by our analysis. With more data and, consequently, better statistics we can now divide each bubble into constant longitude slices to investigate their gross {\$}\backslashgamma{\$}-ray spectral morphology. While the detailed spectral behaviour of each slice derived within our analysis is somewhat dependent on the assumed background model, we find, robustly, a relative deficit of the flux at low energies (i.e., hardening) towards the top of the South Bubble. In neither Bubble does the spectrum soften with longitude. The morphology of the Fermi Bubbles is also revealed to be energy dependent: at high energies they are more extended. We conclude from the gamma-ray spectrum at high latitudes that a low energy break in the parent cosmic ray population is required in both leptonic and hadronic models. We briefly discuss possible leptonic and hadronic interpretation of this phenomenology.},
archivePrefix = {arXiv},
arxivId = {1402.0403},
author = {Yang, Rui-zhi and Aharonian, Felix and Crocker, Roland},
doi = {10.1051/0004-6361/201423562},
eprint = {1402.0403},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Yang, Aharonian, Crocker - 2014 - The Fermi Bubbles Revisited.pdf:pdf},
keywords = {cosmic rays,diffuse background,gamma rays,ism},
pages = {1--9},
title = {{The Fermi Bubbles Revisited}},
url = {http://arxiv.org/abs/1402.0403{\%}0Ahttp://dx.doi.org/10.1051/0004-6361/201423562},
year = {2014}
}
@article{Sternberg1989,
author = {Sternberg, A and Dalgarno, A},
file = {:home/william/Documents/Papers/[Sternberg, Dalgarno]-THE INFRARED RESPONSE OF MOLECULAR HYDROGEN GAS TO ULTRAVIOLET RADIATION$\backslash$:HIGH-DENSITY REGIONS.pdf:pdf},
journal = {ApJ},
pages = {197--233},
title = {{IR response of molecular H gas to UV radiation: high density regions}},
volume = {338},
year = {1989}
}
@ARTICLE{Veilleux2020,
       author = {{Veilleux}, Sylvain and {Maiolino}, Roberto and {Bolatto}, Alberto D. and {Aalto}, Susanne},
        title = "{Cool outflows in galaxies and their implications}",
      journal = {\aapr},
     keywords = {Galaxies: active, Evolution, Halo, Kinematics and dynamics, Starburst, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = apr,
       volume = {28},
       number = {1},
          eid = {2},
        pages = {2},
          doi = {10.1007/s00159-019-0121-9},
archivePrefix = {arXiv},
       eprint = {2002.07765},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&ARv..28....2V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Mukherjee2019,
archivePrefix = {arXiv},
arxivId = {arXiv:1812.08199v1},
author = {Mukherjee, Sagnick and Bhattacharjee, Anirban and Chatterjee, Suchetana and Newman, Jeffrey A. and Yan, Renbin},
doi = {10.3847/1538-4357/aaf9b7},
eprint = {arXiv:1812.08199v1},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Chatterjee et al. - 2019 - X-Ray Surface Brightness Profiles of Optically Selected Active Galactic Nuclei Comparison with X-Ray AGNs.pdf:pdf},
journal = {Astrophys. J.},
number = {1},
pages = {35},
title = {{X-Ray Surface Brightness Profiles of Optically Selected Active Galactic Nuclei: Comparison with X-Ray AGNs}},
volume = {872},
year = {2019}
}
@article{Matsushita1999,
abstract = {We investigated the physical properties of molecular gas in the nuclear region of M51 (Seyfert 2). We obtained an aperture synthesis 13 CO(J = 1 - 0) image using the Nobeyama Millimeter Array (NMA), and compared it with NMA 12 CO(J = 1 - 0) and HCN(J = 1 - 0) maps at similar spatial resolutions. Within a radius of 180 pc from the center, the 13 CO(1 - 0) integrated intensity was found to be 3 times weaker than that of HCN(1 - 0). Large-Velocity-Gradient (LVG) calculations suggest that the observed high HCN(1 -0)/ 13 CO(1 - 0) intensity ratio would arise from dense (n H2 ∼ 10 5 cm -3 ) and hot (T kin ≳ 300 K) molecular clouds in the nuclear molecular disk. We also observed in the 12 CO(1 - 0), (3 - 2), 13 CO(1 - 0), and (3 - 2) lines using the Nobeyama 45m and JCMT 15m telescopes. We detected weak 13 CO lines as well as strong 12 CO lines. The LVG calculations assuming a two-component model suggest that there is a large amount of low-density (n H2 ∼ 3 - 6 × 10 2 cm -3 ), low-temperature (T kin ∼ 20 - 50 K) gas, and a small amount of high-density (n H2 ≳ 10 4 cm -3 ), high-temperature (T kin ≳ 500 K) gas. The existence of the high-density and high-temperature component, although having a quite small beam filling factor, supports the aperture synthesis observation results mentioned above. Since this dense, hot gas is located in the nuclear molecular disk around the Active Galactic Nucleus (AGN), it may be heated by the strong X-ray radiation and/or by the shock induced by the radio jet. @1999 COSPAR. Published by Elsevier Science Ltd.},
author = {Matsushita, S. and Kohno, K. and Vila-Vilaro, B. and Tosaki, T. and Kawabe, R.},
doi = {10.1016/S0273-1177(99)00250-1},
file = {:home/william/Documents/Papers/1-s2.0-S0273117799002501-main.pdf:pdf},
isbn = {5049484748454},
issn = {02731177},
journal = {Adv. Sp. Res.},
number = {5-6},
pages = {1015--1018},
title = {{High-density and high-temperature molecular gas around the AGN in M51}},
volume = {23},
year = {1999}
}
@article{Strozzi2017,
abstract = {The effects of laser-plasma interactions (LPI) on the dynamics of inertial confinement fusion hohlraums are investigated via a new approach that self-consistently couples reduced LPI models into radiation-hydrodynamics numerical codes. The interplay between hydrodynamics and LPI - specifically stimulated Raman scatter and crossed-beam energy transfer (CBET) - mostly occurs via momentum and energy deposition into Langmuir and ion acoustic waves. This spatially redistributes energy coupling to the target, which affects the background plasma conditions and thus, modifies laser propagation. This model shows reduced CBET and significant laser energy depletion by Langmuir waves, which reduce the discrepancy between modeling and data from hohlraum experiments on wall x-ray emission and capsule implosion shape.},
author = {Strozzi, D. J. and Bailey, D. S. and Michel, P. and Divol, L. and Sepke, S. M. and Kerbel, G. D. and Thomas, C. A. and Ralph, J. E. and Moody, J. D. and Schneider, M. B.},
doi = {10.1103/PhysRevLett.118.025002},
file = {:home/william/Documents/Papers/PhysRevLett.118.025002.pdf:pdf},
issn = {10797114},
journal = {Phys. Rev. Lett.},
number = {2},
pages = {1--5},
pmid = {28128587},
title = {{Interplay of Laser-Plasma Interactions and Inertial Fusion Hydrodynamics}},
volume = {118},
year = {2017}
}
@article{Keel2021,
abstract = {We present a narrowband [O III] imaging survey of 111 AGN hosts and 17 merging-galaxy systems, in search of distant extended emission-line regions (EELRs) around AGN (either extant or faded). Our data reach deeper than detection from the broadband SDSS data, and cover a wider field than some early emission-line surveys used to study extended structure around AGN. Spectroscopic followup confirms two new distant AGN-ionized clouds, in the merging systems NGC 235 and NGC 5514, projected at 26 and 75 kpc from the nuclei (respectively). We also recover the previously-known region in NGC 7252. These results strengthen the connection between EELRs and tidal features; kinematically quiescent distant EELRs are virtually always photoionized tidal debris. We see them in {\~{}}10{\%} of the galaxies in our sample with tidal tails. Energy budgets suggest that the AGN in NGC 5514 has faded by {\textgreater}3 times during the extra light-travel time {\~{}}250,000 years from the nucleus to the cloud and then to the observer; strong shock emission in outflows masks the optical signature of the AGN. For NGC 235 our data are consistent with but do not unequivocally require variation over {\~{}}85,000 years. In addition to these very distant ionized clouds, luminous and extensive line emission within four galaxies - IC 1481, ESO 362-G08, NGC 5514, and NGC 7679. IC 1481 shows apparent ionization cones, a rare combination with its LINER AGN spectrum. In NGC 5514, we measure a 7-kpc shell expanding at {\~{}}370 km/s west of the nucleus.},
archivePrefix = {arXiv},
arxivId = {2112.07084},
author = {Keel, William C. and Moiseev, Alexei and Kozlova, D. V. and Ikhsanova, A. I and Oparin, D. V. and Uklein, R. I. and Smirnova, A. A. and Eselevich, M. V.},
doi = {10.1093/mnras/stab3656},
eprint = {2112.07084},
file = {:home/william/Documents/Papers/2112.07084.pdf:pdf},
keywords = {active,galaxies,interactions,seyfert},
number = {December},
pages = {1--20},
title = {{The TELPERION Survey for Distant [O III] Clouds around Luminous and Hibernating AGN}},
url = {http://arxiv.org/abs/2112.07084{\%}0Ahttp://dx.doi.org/10.1093/mnras/stab3656},
volume = {20},
year = {2021}
}
@article{Abeysekara2017,
abstract = {We present a search of very high energy gamma-ray emission from the Northern {\$}\backslashtextit{\{}Fermi{\}}{\$} Bubble region using data collected with the High Altitude Water Cherenkov (HAWC) gamma-ray observatory. The size of the data set is 290 days. No significant excess is observed in the Northern {\$}\backslashtextit{\{}Fermi{\}}{\$} Bubble region, hence upper limits above {\$}1\backslash,\backslashtext{\{}TeV{\}}{\$} are calculated. The upper limits are between {\$}3\backslashtimes 10{\^{}}{\{}-7{\}}\backslash,\backslashtext{\{}GeV{\}}\backslash, \backslashtext{\{}cm{\}}{\^{}}{\{}-2{\}}\backslash, \backslashtext{\{}s{\}}{\^{}}{\{}-1{\}}\backslash,\backslashtext{\{}sr{\}}{\^{}}{\{}-1{\}}{\$} and {\$}4\backslashtimes 10{\^{}}{\{}-8{\}}\backslash,\backslashtext{\{}GeV{\}}\backslash,\backslashtext{\{}cm{\}}{\^{}}{\{}-2{\}}\backslash,\backslashtext{\{}s{\}}{\^{}}{\{}-1{\}}\backslash,\backslashtext{\{}sr{\}}{\^{}}{\{}-1{\}}{\$}. The upper limits disfavor a proton injection spectrum that extends beyond {\$}100\backslash,\backslashtext{\{}TeV{\}}{\$} without being suppressed. They also disfavor a hadronic injection spectrum derived from neutrino measurements.},
archivePrefix = {arXiv},
arxivId = {1703.01344},
author = {Abeysekara, A. U. and Albert, A. and Alfaro, R. and Alvarez, C. and {\'{A}}lvarez, J. D. and Arceo, R. and Arteaga-Vel{\'{a}}zquez, J. C. and Solares, H. A. Ayala and Barber, A. S. and Bautista-Elivar, N. and Becerril, A. and Belmont-Moreno, E. and BenZvi, S. Y. and Berley, D. and Braun, J. and Brisbois, C. and Caballero-Mora, K. S. and Capistr{\'{a}}n, T. and Carrami{\~{n}}ana, A. and Casanova, S. and Castillo, M. and Cotti, U. and Cotzomi, J. and de Le{\'{o}}n, S. Couti{\~{n}}o and {De Le{\'{o}}n}, C. and {De la Fuente}, E. and Hernandez, R. Diaz and Dingus, B. L. and DuVernois, M. A. and D{\'{i}}az-V{\'{e}}lez, J. C. and Ellsworth, R. W. and Engel, K. and Fick, B. and Fiorino, D. W. and Fleischhack, H. and Fraija, N. and Garc{\'{i}}a-Gonz{\'{a}}lez, J. A. and Garfias, F. and Gerhardt, M. and Mu{\~{n}}oz, A. Gonz{\'{a}}lez and Gonz{\'{a}}lez, M. M. and Goodman, J. A. and Hampel-Arias, Z. and Harding, J. P. and Hernandez, S. and Hernandez-Almada, A. and Hinton, J. and Hona, B. and Hui, C. M. and H{\"{u}}ntemeyer, P. and Iriarte, A. and Jardin-Blicq, A. and Joshi, V. and Kaufmann, S. and Kieda, D. and Lara, A. and Lauer, R. J. and Lee, W. H. and Lennarz, D. and Vargas, H. Le{\'{o}}n and Linnemann, J. T. and Longinotti, A. L. and Raya, G. Luis and Luna-Garc{\'{i}}a, R. and L{\'{o}}pez-Coto, R. and Malone, K. and Marinelli, S. S. and Martinez, O. and Martinez-Castellanos, I. and Mart{\'{i}}nez-Castro, J. and Mart{\'{i}}nez-Huerta, H. and Matthews, J. A. and Miranda-Romagnoli, P. and Moreno, E. and Mostaf{\'{a}}, M. and Nellen, L. and Newbold, M. and Nisa, M. U. and Noriega-Papaqui, R. and Pelayo, R. and Pretz, J. and P{\'{e}}rez-P{\'{e}}rez, E. G. and Ren, Z. and Rho, C. D. and Rivi{\`{e}}re, C. and Rosa-Gonz{\'{a}}lez, D. and Rosenberg, M. and Ruiz-Velasco, E. and Salazar, H. and Greus, F. Salesa and Sandoval, A. and Schneider, M. and Schoorlemmer, H. and Sinnis, G. and Smith, A. J. and Springer, R. W. and Surajbali, P. and Taboada, I. and Tibolla, O. and Tollefson, K. and Torres, I. and Ukwatta, T. N. and Vianello, G. and Weisgarber, T. and Westerhoff, S. and Wisher, I. G. and Wood, J. and Yapici, T. and Yodh, G. B. and Zepeda, A. and Zhou, H.},
doi = {10.3847/1538-4357/aa751a},
eprint = {1703.01344},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Abeysekara et al. - 2017 - Search for Very High Energy Gamma Rays from the Northern {\$}textit{\{}Fermi{\}}{\$} Bubble Region with HAWC.pdf:pdf},
keywords = {astroparticle physics,diffuse background,galaxy,gamma rays,general,structure},
title = {{Search for Very High Energy Gamma Rays from the Northern {\$}\backslashtextit{\{}Fermi{\}}{\$} Bubble Region with HAWC}},
url = {http://arxiv.org/abs/1703.01344{\%}0Ahttp://dx.doi.org/10.3847/1538-4357/aa751a},
volume = {85},
year = {2017}
}
@article{Goyon2021,
abstract = {Slow and fast light, or large changes in the group velocity of light, have been observed in a range of optical media, but the fine optical control necessary to induce an observable effect has not been achieved in a plasma. Here, we describe how the ion-acoustic response in a fully ionized plasma can produce large and measurable changes in the group velocity of light. We show the first experimental demonstration of slow and fast light in a plasma, measuring group velocities between 0.12c and -0.34c.},
author = {Goyon, C. and Edwards, M. R. and Chapman, T. and Divol, L. and Lemos, N. and Williams, G. J. and Mariscal, D. A. and Turnbull, D. and Hansen, A. M. and Michel, P.},
doi = {10.1103/PhysRevLett.126.205001},
file = {:home/william/Documents/Papers/Slow and Fast Light in Plasma Using Optical Wave Mixing.pdf:pdf},
issn = {10797114},
journal = {Phys. Rev. Lett.},
keywords = {doi:10.1103/PhysRevLett.126.205001 url:https://doi},
number = {20},
pages = {205001},
pmid = {34110194},
publisher = {American Physical Society},
title = {{Slow and Fast Light in Plasma Using Optical Wave Mixing}},
url = {https://doi.org/10.1103/PhysRevLett.126.205001},
volume = {126},
year = {2021}
}
@article{Aalto2020,
abstract = {Submillimetre and millimetre observations are important in probing the properties of the molecular gas and dust around obscured active galactic nuclei (AGNs) and their feedback. With very high-resolution (0."02x0."03 (2x3 pc)) ALMA 345 GHz observations of CO 3-2, HCO{\$}{\^{}}+{\$} 4-3, HCN 4-3 {\$}\backslashnu{\_}2{\$}=1{\$}f{\$}, and continuum we have studied the molecular outflow and nucleus of the extremely radio-quiet lenticular galaxy NGC1377. The outflow is resolved, revealing a 150 pc long, clumpy, high-velocity, collimated molecular jet. The molecular emission is emerging from the spine of the jet with an average diameter of 3-7 pc. A narrow-angle, rotating molecular wind surrounds the jet and is enveloped by a larger-scale, slower CO-emitting structure. The jet and narrow wind are turbulent ({\$}\backslashsigma{\textgreater}{\$}40 kms{\$}{\^{}}{\{}-1{\}}{\$}) and have steep radial gas excitation gradients. The jet shows velocity reversals that we propose are caused by precession, or episodic directional changes. We suggest that an important process powering the outflow is magneto-centrifugal driving. In contrast, the large-scale CO-envelope may be a slow wind, or cocoon that stems from jet-wind interactions. An asymmetric, nuclear r{\$}\backslashsim{\$}2 pc and hot ({\textgreater}180 K) dust structure with a high molecular column density, N(H{\$}{\_}2{\$}){\$}\backslashsim1.8 \backslashtimes 10{\^{}}{\{}24{\}}{\$} cm{\$}{\^{}}{\{}-2{\}}{\$}, is detected in continuum and vibrationally excited HCN. Its luminosity is likely powered by a buried AGN. The mass of the supermassive black hole (SMBH) is estimated to {\$}\backslashsim9\backslashtimes10{\^{}}6{\$} M{\$}{\_}\backslashodot{\$} and the SMBH of NGC1377 appears to be at the end of an intense phase of accretion. The nuclear growth may be fuelled by low-angular momentum gas inflowing from gas ejected in the molecular jet and wind. Such a feedback-loop of cyclic accretion and outflows would be an effective process in growing the nuclear SMBH. This result invites new questions as to SMBH growth processes in obscured, dusty galaxies.},
archivePrefix = {arXiv},
arxivId = {2007.07824},
author = {Aalto, S. and Falstad, N. and Muller, S. and Wada, K. and Gallagher, J. S. and K{\"{o}}nig, S. and Sakamoto, K. and Vlemmings, W. and Ceccobello, C. and Dasyra, K. and Combes, F. and Garc{\'{i}}a-Burillo, S. and Oya, Y. and Mart{\'{i}}n, S. and van der Werf, P. and Evans, A. S. and Kotilainen, J.},
doi = {10.1051/0004-6361/202038282},
eprint = {2007.07824},
file = {:home/william/Documents/Papers/ALMA resolves the remarkable molecular jet and rotating wind in.pdf:pdf},
issn = {0004-6361},
journal = {Astron. Astrophys.},
keywords = {Galaxies: active,Galaxies: evolution,Galaxies: individual: NGC 1377,Galaxies: nuclei,ISM: jets and outflows,ISM: molecules},
month = {jul},
pages = {A104},
publisher = {EDP Sciences},
title = {{ALMA resolves the remarkable molecular jet and rotating wind in the extremely radio-quiet galaxy NGC 1377}},
url = {https://www.aanda.org/10.1051/0004-6361/202038282 http://arxiv.org/abs/2007.07824 http://dx.doi.org/10.1051/0004-6361/202038282},
volume = {640},
year = {2020}
}
@article{Das2007,
archivePrefix = {arXiv},
arxivId = {astro-ph/0611183},
author = {Das, V. and Crenshaw, D. M. and Kraemer, S. B.},
doi = {10.1086/510580},
eprint = {0611183},
file = {:home/william/Documents/Papers/0611183.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
number = {2},
pages = {699--708},
primaryClass = {astro-ph},
title = {{Dynamics of the Narrow‐Line Region in the Seyfert 2 Galaxy NGC 1068}},
volume = {656},
year = {2007}
}
@article{Dt1996,
abstract = {We now turn our attention to the last term, in which $\Gamma$ ≡ volumetric radiative heating rate [ erg cm −3 s −1 ] $\Lambda$ ≡ volumetric radiative cooling rate [ erg cm −3 s −1 ]. Unfortunately, due to a shortage of Greek letters, $\Gamma$ is also used to represent ionization rates. In this section of the course and notes, therefore, I will denote the radiative heating rate by H, and will reserve $\Gamma$ for ionization rates.},
author = {Dt, D},
file = {:home/william/Documents/Papers/notes8.pdf:pdf},
journal = {Weinb. al},
number = {8},
pages = {46--52},
title = {{8 Radiative Cooling and Heating}},
volume = {465},
year = {1996}
}
@article{Sartori2019,
abstract = {We present a numerical framework for the variability of active galactic nuclei (AGN), which links the variability of AGN over a broad range of timescales and luminosities to the observed properties of the AGN population as a whole, and particularly the Eddington ratio distribution function (ERDF). We have implemented our framework on GPU architecture, relying on previously published time series generating algorithms. After extensive tests that characterise several intrinsic and numerical aspects of the simulations, we describe some applications used for current and future time domain surveys and for the study of extremely variable sources (e.g., "changing look" or flaring AGN). Specifically, we define a simulation setup which reproduces the AGN variability observed in the PTF/iPTF survey, and use it to forward model longer light curves of the kind that may be observed within the LSST main survey. Thanks to our effcient implementations, these simulations are able to cover for example over 1 Myr with a roughly weekly cadence. We envision that this framework will become highly valuable to prepare for, and best exploit, data from upcoming time domain surveys, such as for example LSST.},
archivePrefix = {arXiv},
arxivId = {1909.06374},
author = {Sartori, Lia F. and Trakhtenbrot, Benny and Schawinski, Kevin and Caplar, Neven and Treister, Ezequiel and Zhang, Ce},
doi = {10.3847/1538-4357/ab3c55},
eprint = {1909.06374},
file = {:home/william/Documents/Papers/1909.06374.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {agn variability - quasars},
number = {2},
pages = {139},
title = {{A Forward Modeling Approach to AGN Variability--Method Description and Early Applications}},
volume = {883},
year = {2019}
}
@article{King2010a,
abstract = {I show that Eddington accretion episodes in active galactic nuclei (AGN)$\backslash$nare likely to produce winds with velocities v {\~{}} 0.1c and ionization$\backslash$nparameters up to {\{}{\$}\xi{\$}{\}} {\~{}} 10{\$}{\^{}}{\{}4{\}}{\$} (cgs), implying the presence of$\backslash$nresonance lines of helium- and hydrogen-like iron. These properties are$\backslash$ndirect consequences of momentum and mass conservation, respectively, and$\backslash$nagree with recent X-ray observations of fast outflows from AGN. Because$\backslash$nthe wind is significantly subluminal, it can persist long after the AGN$\backslash$nis observed to have become sub-Eddington. The wind creates a strong$\backslash$ncooling shock as it interacts with the interstellar medium of the host$\backslash$ngalaxy, and this cooling region may be observable in an inverse Compton$\backslash$ncontinuum and lower excitation emission lines associated with lower$\backslash$nvelocities. The shell of matter swept up by the (`momentum-driven')$\backslash$nshocked wind must propagate beyond the black hole's sphere of influence$\backslash$non a time-scale of {\$}\backslashlt{\$}{\~{}}3 {\{}$\backslash$times{\}} 10{\$}{\^{}}{\{}5{\}}{\$}yr. Outside this radius,$\backslash$nthe shell stalls unless the black hole mass has reached the value$\backslash$nM{\$}{\_}{\{}\sigma{\}}{\$} implied by the M-{\{}{\$}\sigma{\$}{\}} relation. If the wind shock$\backslash$ndid not cool, as suggested here, the resulting (`energy-driven') outflow$\backslash$nwould imply a far smaller supermassive black hole mass than actually$\backslash$nobserved. In galaxies with large bulges the black hole may grow somewhat$\backslash$nbeyond this value, suggesting that the observed M-{\{}{\$}\sigma{\$}{\}} relation may$\backslash$ncurve upwards at large M. Minor accretion events with small gas$\backslash$nfractions can produce galaxy-wide outflows with velocities significantly$\backslash$nexceeding {\{}{\$}\sigma{\$}{\}}, including fossil outflows in galaxies where there is$\backslash$nlittle current AGN activity. Some rare cases may reveal the$\backslash$nenergy-driven outflows which sweep gas out of the galaxy and establish$\backslash$nthe black hole-bulge mass relation. However, these require the quasar to$\backslash$nbe at the Eddington luminosity.$\backslash$n},
archivePrefix = {arXiv},
arxivId = {0911.1639},
author = {King, A. R.},
doi = {10.1111/j.1365-2966.2009.16013.x},
eprint = {0911.1639},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/King - 2010 - Black hole outflows.pdf:pdf},
issn = {00358711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Accretion, accretion discs,Black hole physics,Galaxies: active,Galaxies: formation},
number = {3},
pages = {1516--1522},
title = {{Black hole outflows}},
volume = {402},
year = {2010}
}
@article{2041-8205-719-2-L208,
author = {Wang, Junfeng and Fabbiano, Giuseppina and Risaliti, Guido and Elvis, Martin and Mundell, Carole G and Dumas, Gaelle and Schinnerer, Eva and Zezas, Andreas},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Wang et al. - 2010 - EXTENDED X-RAY EMISSION IN THE H i CAVITY OF NGC 4151 GALAXY-SCALE ACTIVE GALACTIC NUCLEUS FEEDBACK.pdf:pdf},
journal = {Astrophys. J. Lett.},
number = {2},
pages = {L208},
title = {{Extended X-ray Emission in the H I Cavity of NGC 4151: Galaxy-scale Active Galactic Nucleus Feedback?}},
url = {http://stacks.iop.org/2041-8205/719/i=2/a=L208},
volume = {719},
year = {2010}
}
@article{Unknownm,
author = {رسولی, چاپار},
file = {:home/william/Documents/Papers/26060769.pdf:pdf},
title = {{No Titleرساله ی دکتری دانشگاه شهید بهشتی}}
}
@article{Bieri2016,
abstract = {The quasar mode of Active Galactic Nuclei (AGN) in the high-redshift Universe is routinely observed in gas-rich galaxies together with large-scale AGN-driven winds. It is crucial to understand how photons emitted by the central AGN source couple to the ambient interstellar-medium to trigger large-scale outflows. By means of radiation-hydrodynamical simulations of idealised galactic discs, we study the coupling of photons with the multiphase galactic gas, and how it varies with gas cloud sizes, and the radiation bands included in the simulations, which are ultraviolet (UV), optical, and infrared (IR). We show how a quasar with a luminosity of {\$}10{\^{}}{\{}46{\}}{\$} erg/s can drive large-scale winds with velocities of {\$}10{\^{}}2-10{\^{}}3{\$} km/s and mass outflow rates around {\$}10{\^{}}3{\$} M{\$}{\_}\backslashodot{\$}/yr for times of order a few million years. Infrared radiation is necessary to efficiently transfer momentum to the gas via multi-scattering on dust in dense clouds. However, IR multi-scattering, despite being extremely important at early times, quickly declines as the central gas cloud expands and breaks up, allowing the radiation to escape through low gas density channels. The typical number of multi-scattering events for an IR photon is only about a quarter of the mean optical depth from the center of the cloud. Our models account for the observed outflow rates of {\$}\backslashsim{\$}500-1000 M{\$}{\_}\backslashodot{\$}/yr and high velocities of {\$}\backslashsim 10{\^{}}3{\$} km/s, favouring winds that are energy-driven via extremely fast nuclear outflows, interpreted here as being IR-radiatively-driven winds.},
archivePrefix = {arXiv},
arxivId = {1606.06281},
author = {Bieri, Rebekka and Dubois, Yohan and Rosdahl, Joakim and Wagner, Alexander Y. and Silk, Joseph and Mamon, Gary A.},
doi = {10.1093/mnras/stw2380},
eprint = {1606.06281},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Bieri et al. - 2016 - Outflows Driven by Quasars in High-Redshift Galaxies with Radiation Hydrodynamics.pdf:pdf},
keywords = {active,galaxies,high-redshift,ism,methods},
number = {June},
title = {{Outflows Driven by Quasars in High-Redshift Galaxies with Radiation Hydrodynamics}},
url = {http://arxiv.org/abs/1606.06281{\%}0Ahttp://dx.doi.org/10.1093/mnras/stw2380},
volume = {000},
year = {2016}
}
@article{Zhuravleva2019,
abstract = {Transport properties, such as viscosity and thermal conduction, of the hot intergalactic plasma in clusters of galaxies are largely unknown. Whereas for laboratory plasmas these characteristics are derived from the gas density and temperature1, such recipes can be fundamentally different for the intergalactic plasma2 owing to a low rate of particle collisions and a weak magnetic field3. In numerical simulations, these unknowns can often be avoided by modelling these plasmas as hydrodynamic fluids4–6, even though local, non-hydrodynamic features observed in clusters contradict this assumption7–9. Using deep Chandra observations of the Coma Cluster10,11, we probe gas fluctuations in intergalactic medium down to spatial scales where the transport processes should prominently manifest themselves—provided that hydrodynamic models12 with pure Coulomb collision rates are indeed adequate. We do not find evidence of such transport processes, implying that the effective isotropic viscosity is orders of magnitude smaller than naively expected. This indicates either an enhanced collision rate in the plasma due to particle scattering off microfluctuations caused by plasma instabilities2,13,14 or that the transport processes are anisotropic with respect to the local magnetic field15. This also means that numerical models with high Reynolds number appear more consistent with observations. Our results demonstrate that observations of turbulence in clusters16,17 are giving rise to a branch of astrophysics that can sharpen theoretical views on galactic plasmas.},
author = {Zhuravleva, I. and Churazov, E. and Schekochihin, A. A. and Allen, S. W. and Vikhlinin, A. and Werner, N.},
doi = {10.1038/s41550-019-0794-z},
file = {:home/william/Documents/Papers/10.1038@s41550-019-0794-z.pdf:pdf},
issn = {23973366},
journal = {Nat. Astron.},
number = {9},
pages = {832--837},
publisher = {Springer US},
title = {{Suppressed effective viscosity in the bulk intergalactic plasma}},
url = {http://dx.doi.org/10.1038/s41550-019-0794-z},
volume = {3},
year = {2019}
}
@article{Arav2020,
abstract = {The Hubble Space Telescope/Cosmic Origins Spectrograph (COS) has opened a new discovery space for studying quasar absorption outflows and their contribution to AGN feedback. Specifically, COS provides high-quality far-ultraviolet (FUV) spectra covering the diagnostic-rich 500-1050 Angstrom rest frame (hereafter, EUV500) of medium redshift objects. The quality and quantity of EUV500 diagnostic troughs allow us to probe the very high-ionization phase, which carries 90{\%} or more of the outflowing material, as well as to determine the distance of most outflows from the central source ({\$}R{\$}). The first objective is impossible to achieve with ground-based spectra, and {\$}R{\$} can be measured in only {\$}\backslashsim{\$}1{\%} of them. Here, we summarize the main results of the first dedicated survey of such outflows, including the following: 1) Measurements of the three most energetic outflows to date, which can be the main agents for AGN feedback processes in the environments of the host galaxies. 2) All the outflows have a very high-ionization component, similar to the one found in warm absorbers, which carries most of the outflow's kinetic luminosity. This finding suggests that all the high-ionization outflows observed from the ground also have a similar undetected very high-ionization component. 3) Of the 13 studied EUV500 outflows, 9 have {\$}100{\textless}R{\textless}2000{\$} parsecs, 2 have {\$}5{\textless}R{\textless}20{\$} parsecs, 1 has {\$}0.05{\textless}R{\textless}50{\$} parsecs, and in 1 case, {\$}R{\$} cannot be determined. 4) One of the outflows has the largest velocity shift (1550 km s{\$}{\^{}}{\{}-1{\}}{\$}) and acceleration (1.5 cm s{\$}{\^{}}{\{}-2{\}}{\$}) measured to date. This outflow is physically similar to the fast X-ray outflow detected in quasar PG 1211+143.},
archivePrefix = {arXiv},
arxivId = {2003.08688},
author = {Arav, Nahum and Xu, Xinfeng and Miller, Timothy and Kriss, Gerard A. and Plesha, Rachel},
doi = {10.3847/1538-4365/ab66af},
eprint = {2003.08688},
file = {:home/william/Documents/Papers/[Arav et al.]-HST-COS OBSERVATIONS OF QUASAR OUTFLOWS IN .pdf:pdf},
journal = {Astrophys. J. Suppl. Ser.},
keywords = {1646,absorption lines,active,galaxies,general,individual,jets and outflows,kinematics and dynamics,quasars,sdss j1042},
number = {2},
pages = {37},
title = {{ HST /COS Observations of Quasar Outflows in the 500–1050 {\AA} Rest Frame. I. The Most Energetic Outflows in the Universe and Other Discoveries }},
volume = {247},
year = {2020}
}
@article{Heywood2022,
abstract = { The inner ∼200 pc region of the Galaxy contains a 4 million M ⊙ supermassive black hole (SMBH), significant quantities of molecular gas, and star formation and cosmic-ray energy densities that are roughly two orders of magnitude higher than the corresponding levels in the Galactic disk. At a distance of only 8.2 kpc, the region presents astronomers with a unique opportunity to study a diverse range of energetic astrophysical phenomena, from stellar objects in extreme environments, to the SMBH and star-formation-driven feedback processes that are known to influence the evolution of galaxies as a whole. We present a new survey of the Galactic center conducted with the South African MeerKAT radio telescope. Radio imaging offers a view that is unaffected by the large quantities of dust that obscure the region at other wavelengths, and a scene of striking complexity is revealed. We produce total-intensity and spectral-index mosaics of the region from 20 pointings (144 hr on-target in total), covering 6.5 square degrees with an angular resolution of 4″ at a central frequency of 1.28 GHz. Many new features are revealed for the first time due to a combination of MeerKAT's high sensitivity, exceptional u , v -plane coverage, and geographical vantage point. We highlight some initial survey results, including new supernova remnant candidates, many new nonthermal filament complexes, and enhanced views of the Radio Arc bubble, Sagittarius A, and Sagittarius B regions. This project is a South African Radio Astronomy Observatory public legacy survey, and the image products are made available with this article. },
archivePrefix = {arXiv},
arxivId = {2201.10541},
author = {Heywood, I. },
doi = {10.3847/1538-4357/ac449a},
eprint = {2201.10541},
file = {:home/william/Documents/Papers/Heywood{\_}2022{\_}ApJ{\_}925{\_}165.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
keywords = {Galactic center,Galactic radio sources,Radio interferometry},
number = {2},
pages = {165},
publisher = {IOP Publishing},
title = {{The 1.28 GHz MeerKAT Galactic Center Mosaic}},
url = {http://arxiv.org/abs/2201.10541{\%}0Ahttp://dx.doi.org/10.3847/1538-4357/ac449a},
volume = {925},
year = {2022}
}
@article{Semenov2021,
abstract = {Observations of the {\$}\backslashgamma{\$}-ray emission around star clusters, isolated supernova remnants, and pulsar wind nebulae indicate that cosmic ray (CR) diffusion coefficient near the acceleration sites can be suppressed by a large factor compared to the Galaxy average. We explore the effects of such local suppression of CR diffusion on galaxy evolution using simulations of isolated disk galaxies with regular and high gas fractions. Our results show that while CR propagation with constant diffusivity can make gaseous disks more stable by increasing the midplane pressure, large-scale CR pressure gradients cannot prevent local fragmentation when the disk is unstable. In contrast, when CR diffusivity is suppressed in star-forming regions, accumulation of CRs in these regions results in strong local pressure gradients that prevent formation of massive gaseous clumps. As a result, the distribution of dense gas and star formation changes qualitatively: a globally unstable gaseous disk does not violently fragment into massive star-forming clumps but maintains a regular grand-design spiral structure. This effect regulates star formation and disk structure and is qualitatively different from and complementary to the global role of CRs in vertical hydrostatic support of the gaseous disk and in driving galactic winds.},
archivePrefix = {arXiv},
arxivId = {2012.01427},
author = {Semenov, Vadim A. and Kravtsov, Andrey V. and Caprioli, Damiano},
doi = {10.3847/1538-4357/abe2a6},
eprint = {2012.01427},
file = {:home/william/Documents/Papers/2012.01427.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
keywords = {cosmic rays,formation,galaxies,ism,kinematics and dynamics,methods,stars},
number = {2},
pages = {126},
title = {{Cosmic-Ray Diffusion Suppression in Star-forming Regions Inhibits Clump Formation in Gas-rich Galaxies}},
volume = {910},
year = {2021}
}
@article{Melioli2009b,
abstract = {The ejection of the gas out of the disk in late-type galaxies is related to star formation and is due mainly to Type II supernovae. In this paper we studied in detail the development of the Galactic fountains in order to understand their dynamical evolution and their influence in the redistribution of the freshly delivered metals over the disk. To this aim, we performed a number of 3D hydrodynamical radiative cooling simulations of the gas in the Milky Way where the whole Galaxy structure, the Galactic differential rotation and the supernovae explosions generated by a single OB association are considered. A typical fountain powered by 100 Type II supernovae may eject material up to {\$}\backslashsim 2{\$} kpc which than collapses back mostly in form of dense, cold clouds and filaments. The majority of the gas lifted up by the fountains falls back on the disk remaining within a radial distance {\$}\backslashDelta R=0.5{\$} kpc from the place where the fountain originated. This localized circulation of disk gas does not influence the radial chemical gradients on large scale, as required by the chemical models of the Milky Way which reproduce the metallicity distribution without invoking large fluxes of metals. Simulations of multiple fountains fuelled by Type II supernovae of different OB associations will be presented in a companion paper.},
author = {Melioli, C. and Brighenti, F. and D'Ercole, A. and {De Gouveia Dal Pino}, E. M.},
doi = {10.1111/j.1365-2966.2009.14725.x},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Melioli et al. - 2009 - Hydrodynamical simulations of Galactic fountains - II. Evolution of multiple fountains.pdf:pdf},
issn = {00358711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxy: disc,Galaxy: general,Hydrodynamics,ISM: bubbles,ISM: clouds,Methods: numerical},
number = {3},
pages = {1089--1105},
title = {{Hydrodynamical simulations of Galactic fountains - II. Evolution of multiple fountains}},
volume = {399},
year = {2009}
}
@article{Zubovas2014,
abstract = {It is usually assumed that outflows from luminous active galactic nuclei (AGN) are either in the energy-conserving (non-radiative) or in the momentum-conserving (radiative) regime. We show that in a non-spherical geometry the effects of both regimes may manifest at the same time, and that it is the momentum of the outflow that sets the MBH-$\sigma$ relation. Considering an initially elliptical distribution of gas in the host galaxy, we show that a non-radiative outflow opens up a wide 'escape route' over the paths of least resistance. Most of the outflow energy escapes in that direction. At the same time, in the directions of higher resistance, the ambient gas is affected mainly by the incident momentum from the outflow. Quenching SMBH growth requires quenching gas delivery along the paths of highest resistance, and therefore, it is the momentum of the outflow that limits the black hole growth. We present an analytical argument showing that such energy-conserving feedback bubbles driving leaky ambient shells will terminate SMBH growth once its mass reaches roughly the M$\sigma$ mass derived earlier by King for momentum-conserving AGN outflows. Our simulations also have potentially important implications for observations of AGN jet feedback and starburst galaxy feedback. The collimation of the wide angle AGN outflow away from the symmetry plane, as found in our simulations, indicates that credit for work done by such outflows may sometimes be mistakenly given to AGN jets or star formation feedback since wide angle $\nu$ {\~{}} 0.1c outflows are harder to observe and the phase when they are present may be short. {\textcopyright} 2014 The Authors Published by Oxford University Press on behalf of the Royal Astronomical Society.},
archivePrefix = {arXiv},
arxivId = {1403.3933},
author = {Zubovas, Kastytis and Nayakshin, Sergei},
doi = {10.1093/mnras/stu431},
eprint = {1403.3933},
file = {:home/william/Documents/Papers/MNRAS-2014-Zubovas-2625-35.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Accretion, accretion discs,Black hole physics,Galaxies: evolution,Quasars: general},
number = {3},
pages = {2625--2635},
title = {{Energy- and momentum-conserving AGN feedback outflows}},
volume = {440},
year = {2014}
}
@article{Garcia-Burillo2014,
abstract = {Aims. We investigate the fueling and the feedback of star formation and nuclear activity in NGC 1068, a nearby (D = 14 Mpc) Seyfert 2 barred galaxy, by analyzing the distribution and kinematics of the molecular gas in the disk. We aim to understand if and how gas accretion can self-regulate.Methods. We have used the Atacama Large Millimeter Array (ALMA) to map the emission of a set of dense molecular gas (n(H2) ' 1056 cm3) tracers (CO(3-2), CO(6-5), HCN(4-3), HCO+(4-3), and CS(7-6)) and their underlying continuum emission in the central r ∼ 2 kpc of NGC 1068 with spatial resolutions ∼0:3000:500 (∼20-35 pc for the assumed distance of D = 14 Mpc). Results. The sensitivity and spatial resolution of ALMA give an unprecedented detailed view of the distribution and kinematics of the dense molecular gas (n(H2) ≈ 1056cm3) in NGC 1068. Molecular line and dust continuum emissions are detected from a r ∼ 200 pc off-centered circumnuclear disk (CND), from the 2.6 kpc-diameter bar region, and from the r ∼ 1:3 kpc starburst (SB) ring. Most of the emission in HCO+, HCN, and CS stems from the CND. Molecular line ratios show dramatic order-of-magnitude changes inside the CND that are correlated with the UV/X-ray illumination by the active galactic nucleus (AGN), betraying ongoing feedback. We used the dust continuum fluxes measured by ALMA together with NIR/MIR data to constrain the properties of the putative torus using CLUMPY models and found a torus radius of 20+6 10 pc. The Fourier decomposition of the gas velocity field indicates that rotation is perturbed by an inward radial flow in the SB ring and the bar region. However, the gas kinematics from r ∼ 50 pc out to r ∼ 400 pc reveal a massive (Mmol ∼ 2:7+0:9 1:2 × 107 M) outflow in all molecular tracers. The tight correlation between the ionized gas outflow, the radio jet, and the occurrence of outward motions in the disk suggests that the outflow is AGN driven. Conclusions. The molecular outflow is likely launched when the ionization cone of the narrow line region sweeps the nuclear disk. The outflow rate estimated in the CND, dM=dt ∼ 63+21 37 M yr1, is an order of magnitude higher than the star formation rate at these radii, confirming that the outflow is AGN driven. The power of the AGN is able to account for the estimated momentum and kinetic luminosity of the outflow. The CND mass load rate of the CND outflow implies a very short gas depletion timescale of ≤1 Myr. The CND gas reservoir is likely replenished on longer timescales by efficient gas inflow from the outer disk. {\textcopyright} ESO 2014.},
archivePrefix = {arXiv},
arxivId = {1405.7706},
author = {Garc{\'{i}}a-Burillo, S. and Combes, F. and Usero, A. and Aalto, S. and Krips, M. and Viti, S. and Alonso-Herrero, A. and Hunt, L. K. and Schinnerer, E. and Baker, A. J. and Boone, F. and Casasola, V. and Colina, L. and Costagliola, F. and Eckart, A. and Fuente, A. and Henkel, C. and Labiano, A. and Mart{\'{i}}n, S. and M{\'{a}}rquez, I. and Muller, S. and Planesas, P. and {Ramos Almeida}, C. and Spaans, M. and Tacconi, L. J. and {Van Der Werf}, P. P.},
doi = {10.1051/0004-6361/201423843},
eprint = {1405.7706},
file = {:home/william/Documents/Papers/[Garcia-Burillo, Combes et al.]-Molecular line emission in NGC 1068 imaged with ALMA.pdf:pdf},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Galaxies: ISM,Galaxies: Seyfert,Galaxies: individual: NGC 1068,Galaxies: kinematics and dynamics,Galaxies: nuclei,Radio lines: galaxies},
pages = {1--24},
title = {{Molecular line emission in NGC 1068 imaged with ALMA : I. An AGN-driven outflow in the dense molecular gas}},
volume = {567},
year = {2014}
}
@article{Peretti2018,
abstract = {The high rate of star formation and supernova explosions of starburst galaxies make them interesting sources of high energy radiation. Depending upon the level of turbulence present in the their interstellar medium, the bulk of cosmic rays produced inside starburst galaxies may lose most of their energy before escaping, thereby making these sources behave as calorimeters, at least up to some maximum energy. Contrary to previous studies, here we investigate in detail the conditions under which cosmic ray confinement may be effective for electrons and nuclei and we study the implications of cosmic ray confinement in terms of multifrequency emission from starburst nuclei and production of high energy neutrinos. The general predictions are then specialized to three cases of active starbursts, namely M82, NGC253 and Arp220. Both primary and secondary electrons, as well as electron-positron pairs produced by gamma ray absorption inside starburst galaxies are taken into account. Electrons and positrons produced as secondary products of hadronic interactions are found to be responsible for most of the emission of leptonic origin. In particular, synchrotron emission of very high energy secondary electrons produces an extended emission of hard X-rays that represent a very interesting signature of hadronic process in starburst galaxies, potentially accessible to current and future observations in the X-ray band. A careful understanding of both the production and absorption of gamma rays in starburst galaxies is instrumental to the assessment of the role of these astrophysical sources as sources of high energy astrophysical neutrinos.},
archivePrefix = {arXiv},
arxivId = {1812.01996v1},
author = {Peretti, Enrico and Blasi, Pasquale and Aharonian, Felix and Morlino, Giovanni},
eprint = {1812.01996v1},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Peretti et al. - 2018 - Cosmic ray transport and radiative processes in nuclei of starburst galaxies.pdf:pdf},
journal = {Mnras},
keywords = {Confinement,Cosmic rays-,Starburst galaxy-},
number = {December},
pages = {1--14},
title = {{Cosmic ray transport and radiative processes in nuclei of starburst galaxies}},
url = {https://arxiv.org/pdf/1812.01996.pdf},
volume = {000},
year = {2018}
}
@article{Banda-Barragan2016b,
abstract = {Filamentary structures are ubiquitous in the interstellar medium, yet their formation, internal structure, and longevity have not been studied in detail. We report the results from a comprehensive numerical study that investigates the characteristics, formation, and evolution of filaments arising from magnetohydrodynamic interactions between supersonic winds and dense clouds. Here, we improve on previous simulations by utilizing sharper density contrasts and higher numerical resolutions. By following multiple density tracers, we find that material in the envelopes of the clouds is removed and deposited downstream to form filamentary tails, while the cores of the clouds serve as footpoints and late-stage outer layers of these tails. Aspect ratios ≳12, subsonic velocity dispersions {\~{}}0.1-0.3 of the wind sound speed, and magnetic field amplifications {\~{}}100 are found to be characteristic of these filaments. We also report the effects of different magnetic field strengths and orientations. The magnetic field strength regulates vorticity production: sinuous filamentary towers arise in non-magnetic environments, while strong magnetic fields inhibit small-scale perturbations at boundary layers making tails less turbulent. Magnetic field components aligned with the direction of the flow favour the formation of pressure-confined flux ropes inside the tails, whilst transverse components tend to form current sheets. Softening the equation of state to nearly isothermal leads to suppression of dynamical instabilities and further collimation of the tail. Towards the final stages of the evolution, we find that small cloudlets and distorted filaments survive the break-up of the clouds and become entrained in the winds, reaching velocities {\~{}}0.1 of the wind speed.},
archivePrefix = {arXiv},
arxivId = {1510.05356},
author = {Banda-Barrag{\'{a}}n, W. E. and Parkin, E. R. and Federrath, C. and Crocker, R. M. and Bicknel, G. V.},
doi = {10.1093/mnras/stv2405},
eprint = {1510.05356},
file = {:home/william/Documents/Papers/stv2405.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: starburst,ISM: clouds,ISM: magnetic fields,MHD- methods: numerical,Stars: winds, outflows},
number = {2},
pages = {1309--1333},
title = {{Filament formation in wind-cloud interactions - I. Spherical clouds in uniform magnetic fields}},
volume = {455},
year = {2016}
}
@article{GuimaraesM.&Silva1985,
abstract = {er than those in most current practice; and the use of a variable-size detector requires even larger sample areas but gives considerably better results. 1. M. Fuller and P. Griffiths, Anal. Chem. 50, 1906 (1978).},
author = {Lepp and McCray},
file = {:home/william/Documents/Papers/[Leep et al.]-Thermal Phases of Interestellar and Quasar gas.pdf:pdf},
journal = {日本鉄鋼協会 第 109 回(春季)講演大会},
keywords = {dorsiflexion - movement initiation,h-reflex - reciprocal inhibition,la inhibition - ankle},
number = {103},
pages = {1984},
title = {{Thermal Phases of the ISM and Quasar gas}},
volume = {11},
year = {1985}
}
@article{2005ApJ...618..569M,
author = {Murray, N and Quataert, E and Thompson, T.{\~{}}A.},
doi = {10.1086/426067},
file = {:home/william/Documents/Papers/Murray{\_}2005{\_}ApJ{\_}618{\_}569.pdf:pdf},
journal = {Apj},
keywords = {Galaxies: Formation,Galaxies: Fundamental Parameters,Galaxies: General,Galaxies: Intergalactic Medium,Galaxies: Starburst},
pages = {569--585},
title = {{On the Maximum Luminosity of Galaxies and Their Central Black Holes: Feedback from Momentum-driven Winds}},
volume = {618},
year = {2005}
}
@article{Navarro1996,
abstract = {We use N-body simulations to investigate the structure of dark halos in the standard Cold Dark Matter cosmogony. Halos are excised from simulations of cosmologically representative regions and are resimulated individually at high resolution. We study objects with masses ranging from those of dwarf galaxy halos to those of rich galaxy clusters. The spherically averaged density profiles of all our halos can be fit over two decades in radius by scaling a simple ``universal'' profile. The characteristic overdensity of a halo, or equivalently its concentration, correlates strongly with halo mass in a way which reflects the mass dependence of the epoch of halo formation. Halo profiles are approximately isothermal over a large range in radii, but are significantly shallower than {\$}r{\^{}}{\{}-2{\}}{\$} near the center and steeper than {\$}r{\^{}}{\{}-2{\}}{\$} near the virial radius. Matching the observed rotation curves of disk galaxies requires disk mass-to-light ratios to increase systematically with luminosity. Further, it suggests that the halos of bright galaxies depend only weakly on galaxy luminosity and have circular velocities significantly lower than the disk rotation speed. This may explain why luminosity and dynamics are uncorrelated in observed samples of binary galaxies and of satellite/spiral systems. For galaxy clusters, our halo models are consistent both with the presence of giant arcs and with the observed structure of the intracluster medium, and they suggest a simple explanation for the disparate estimates of cluster core radii found by previous authors. Our results also highlight two shortcomings of the CDM model. CDM halos are too concentrated to be consistent with the halo parameters inferred for dwarf irregulars, and the predicted abundance of galaxy halos is larger than the observed abundance of galaxies.},
archivePrefix = {arXiv},
arxivId = {astro-ph/9508025},
author = {Navarro, Julio F. and Frenk, Carlos S. and White, Simon D. M.},
doi = {10.1086/177173},
eprint = {9508025},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Navarro, Frenk, White - 1996 - The Structure of Cold Dark Matter Halos.pdf:pdf},
isbn = {0792339754},
issn = {0004-637X},
journal = {Astrophys. J.},
pages = {563},
pmid = {15003161},
primaryClass = {astro-ph},
title = {{The Structure of Cold Dark Matter Halos}},
url = {http://adsabs.harvard.edu/doi/10.1086/177173},
volume = {462},
year = {1996}
}
@article{Fay1967,
abstract = {Supernova explosions in a cloudy interstellar medium produce a three-component medium in which a large fraction of the volume is filled with hot, tenuous gas. In the disk of the galaxy the evolution of supernova remnants is altered by evaporation of cool clouds embedded in the hot medium. Radiative losses are enhanced by the resulting increase in density and by radiation from the conductive interfaces between clouds and hot gas. Mass balance (cloud evaporation rate = dense shell formation rate) and energy balance (supernova shock input = radiation loss) deter- mine the density and temperature of the hot medium with («, T) = (IO-2-5, 105-7) being repre- sentative values. Very small clouds will be rapidly evaporated or swept up. The outer edges of “standard” clouds ionized by the diffuse UV and soft X-ray backgrounds provide the warm ({\~{}}104 K) ionized and neutral components. A self-consistent model of the interstellar medium developed herein accounts for the observed pressure of interstellar clouds, the galactic soft X-ray background, the O vi absorption line observations, the ionization and heating of much of the interstellar medium, and the motions of the clouds. In the halo of the galaxy, where the clouds are relatively unimportant, we estimate («, T) = (IO-3-3, 106 0) below one pressure scale height. Energy input from halo supernovae is probably adequate to drive a galactic wind},
author = {{Christopher F. McKee} and {Jeremiah P. Ostriker}},
file = {:home/william/Documents/Papers/1977ApJ...218..148M.pdf:pdf},
journal = {Astrophys. Journal, 218148-169, 1977 Novemb. 15},
pages = {148--169},
title = {{A THEORY OF THE INTERSTELLAR MEDIUM: THREE COMPONENTS REGULATED BY SUPERNOVA EXPLOSIONS IN AN INHOMOGENEOUS SUBSTRATE}},
year = {1967}
}
@article{Emilia2021,
author = {Emilia, Regio},
file = {:home/william/Documents/Papers/Clavijo-Dal Pino-Melioli.pdf:pdf},
keywords = {active galaxies,galactic winds,holes,magneto-hydrodynamical simulations,star formation,super massive black},
title = {{FEEDBACK IN GALAXIES HOSTING AGN AND SF WINDS : THE EFFECTS OF THE AGN FLICKERING AND THE}},
year = {2021}
}
@article{Mertsch2017,
abstract = {The discovery of the Fermi bubbles---a huge bilobular structure seen in GeV gamma-rays above and below the Galactic center---implies the presence of a large reservoir of high energy particles at {\$}\backslashsim 10 \backslash, \backslashtext{\{}kpc{\}}{\$} from the disk. The absence of evidence for a strong shock coinciding with the edge of the bubbles, and constraints from multi-wavelength observations point towards stochastic acceleration by turbulence as a likely mechanism of acceleration. We have investigated the time-dependent acceleration of electrons in a large-scale outflow from the Galactic centre. For the first time, we present a detailed numerical solution of the particle kinetic equation that includes the acceleration, transport and relevant energy loss processes. We also take into account the addition of shock acceleration of electrons at the bubble's blast wave. Fitting to the observed spectrum and surface brightness distribution of the bubbles allows determining the transport coefficients, thereby shedding light on the origin of the Fermi bubbles.},
archivePrefix = {arXiv},
arxivId = {arXiv:1808.00330v1},
author = {Mertsch, Philipp and Petrosian, Vah{\'{e}}},
eprint = {arXiv:1808.00330v1},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Mertsch, Petrosian - 2017 - The Fermi bubbles from stochastic acceleration by turbulence in a galactic outflow.pdf:pdf},
issn = {18248039},
journal = {Proc. Sci.},
keywords = {acceleration of particles -,cosmic rays - ism,gamma rays,ism,jets and outflows -,shock waves - turbulence},
pages = {1--14},
title = {{The Fermi bubbles from stochastic acceleration by turbulence in a galactic outflow}},
year = {2017}
}
@article{Sullivan2008,
abstract = {We are using "broadband" (4.6 to 43 GHz) multi-frequency VLBA polarization observations of compact AGN to investigate the 3-D structure of their jet magnetic (B) fields. Observing at several frequencies, separated by short and long intervals, enables reliable determination of the distribution of Faraday Rotation, and thereby the intrinsic B field structure. Transverse Rotation Measure (RM) gradients were detected in the jets of 0954+658 and 1418+546, providing evidence for the presence of a helical B field surrounding the jet. The RM in the core regions of 2200+420 (BL Lac), 0954+658 and 1418+546 display different signs in different frequency-intervals (on different spatial scales); we suggest an explanation for this in terms of modest bends in a helical B field surrounding their jets. In future, polarization observations with a combination of VSOP-2 at 8, 22 and 43 GHz and ground arrays at frequencies with corresponding resolution will help map out the distributions of Faraday rotation, spectral index and the 3-D B field structure both across the jet and closer to the central engine, providing strong constraints for any jet B field models.},
archivePrefix = {arXiv},
arxivId = {0801.4897},
author = {O'Sullivan, Shane P. and Gabuzda, Denise C},
eprint = {0801.4897},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Sullivan, Gabuzda - 2008 - The Need For High Resolution In Studies Of The 3-D Magnetic Field Structure Of AGN Jets.pdf:pdf},
pages = {1--4},
title = {{The Need For High Resolution In Studies Of The 3-D Magnetic Field Structure Of AGN Jets}},
url = {http://arxiv.org/abs/0801.4897},
year = {2008}
}
@article{Rathjen2021,
abstract = {We present simulations of the multiphase interstellar medium (ISM) at solar neighbourhood conditions including thermal and non-thermal ISM processes, star cluster formation, and feedback from massive stars: stellar winds, hydrogen ionizing radiation computed with the novel treeray radiative transfer method, supernovae (SN), and the injection of cosmic rays (CR). N-body dynamics is computed with a 4th-order Hermite integrator. We systematically investigate the impact of stellar feedback on the self-gravitating ISM with magnetic fields, CR advection and diffusion, and non-equilibrium chemical evolution. SN-only feedback results in strongly clustered star formation with very high star cluster masses, a bi-modal distribution of the ambient SN densities, and low volume-filling factors (VFF) of warm gas, typically inconsistent with local conditions. Early radiative feedback prevents an initial starburst, reduces star cluster masses and outflow rates. Furthermore, star formation rate surface densities of {\$}\backslashSigma {\_}{\{}\backslashdot{\{}M{\}}{\_}\backslashstar {\}} = 1.4-5.9 \backslashtimes 10{\^{}}{\{}-3{\}}{\$}{\$}\backslashmathrm{\{}M{\}}{\_}\backslashodot \backslash, \backslashmathrm{\{}yr{\}}{\^{}}{\{}-1{\}}\backslash, \backslashmathrm{\{}kpc{\}}{\^{}}{\{}-2{\}}{\$}, VFFwarm = 60-80 per cent as well as thermal, kinetic, magnetic, and cosmic ray energy densities of the model including all feedback mechanisms agree well with observational constraints. On the short, 100 Myr, time-scales investigated here, CRs only have a moderate impact on star formation and the multiphase gas structure and result in cooler outflows, if present. Our models indicate that at low gas surface densities SN-only feedback only captures some characteristics of the star-forming ISM and outflows/inflows relevant for regulating star formation. Instead, star formation is regulated on star cluster scales by radiation and winds from massive stars in clusters, whose peak masses agree with solar neighbourhood estimates.},
archivePrefix = {arXiv},
arxivId = {2103.14128},
author = {Rathjen, Tim Eric and Naab, Thorsten and Girichidis, Philipp and Walch, Stefanie and W{\"{u}}nsch, Richard and Dinnbier, Franti{\v{s}}ek and Seifried, Daniel and Klessen, Ralf S. and Glover, Simon C.O.},
doi = {10.1093/mnras/stab900},
eprint = {2103.14128},
file = {:home/william/Documents/Papers/2103.14128.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {ISM: evolution,ISM: structure,cosmic rays,galaxies: ISM,galaxies: star formation,methods: numerical},
number = {1},
pages = {1039--1061},
title = {{SILCC VI - Multiphase ISM structure, stellar clustering, and outflows with supernovae, stellar winds, ionizing radiation, and cosmic rays}},
volume = {504},
year = {2021}
}
@article{Figureb,
author = {Hen{\'{o}}n, M},
doi = {10.15713/ins.mmj.3},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Figure - Unknown - No Title No Title{\_}2015.pdf:pdf},
isbn = {9789004310087},
journal = {A{\&}A},
number = {c},
pages = {1--4},
pmid = {29982528},
title = {{Vlasov Equation?}},
year = {1982}
}
@article{Harfst2006,
abstract = {We present a new particle code for modelling the evolution of galaxies. The code is based on a multi-phase description for the interstellar medium (ISM). We include star formation (SF), stellar feedback by massive stars and planetary nebulae, phase transitions, and interactions between gas clouds and ambient diffuse gas, namely condensation, evaporation, drag, and energy dissipation. The last is realised by radiative cooling and inelastic cloud-cloud collisions. We present new schemes for SF and stellar feedback that include a consistent calculation of the star-formation efficiency (SFE) based on ISM properties, as well as a detailed redistribution of the feedback energy into the different ISM phases. As a first test we show a model of the evolution of a present day Milky-Way-type galaxy. Though the model exhibits a quasi-stationary behaviour in global properties like mass fractions or surface densities, the evolution of the ISM is strongly variable locally depending on the local SF and stellar feedback. We start only with two distinct phases, but a three-phase ISM is formed soon and consists of cold molecular clouds, a warm gas disk, and a hot gaseous halo. Hot gas is also found in bubbles in the disk accompanied by type II supernovae explosions. The volume-filling factor of the hot gas in the disk is ∼35{\%}. The mass spectrum of the clouds follows a power-law with an index of $\alpha$ ≈-2. The star-formation rate (SFR) is ∼ 1.6 M⊙ yr-1 on average, decreasing slowly with time due to gas consumption. In order to maintain a constant SFR, gas replenishment, e.g. by infall, of the order 1 M⊙ yr-1 is required. Our model is in fair agreement with Kennicutt's (1998, ApJ, 498, 541) SF law including the cut-off at ∼10 M⊙ pc-2. Models with a constant SFE, i.e. no feedback on the SF, fail to reproduce Kennicutt's law. We performed a parameter study varying the particle resolution, feedback energy, cloud radius, SF time scale, and metallicity. In most these cases the evolution of the model galaxy was not significantly different to our reference model. Increasing the feedback energy by a factor of 4-5 lowers the SF rate by ∼0.5 M⊙ yr-1, while decreasing the metallicity by a factor of ∼100 increases the mass fraction of the hot gas from about 10{\%} to 30{\%}. {\textcopyright} ESO 2006.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0511775},
author = {Harfst, S. and Theis, Ch and Hensler, G.},
doi = {10.1051/0004-6361:20042190},
eprint = {0511775},
file = {:home/william/Documents/Papers/0511775.pdf:pdf},
issn = {00046361},
journal = {Astron. Astrophys.},
keywords = {Galaxies: ISM,Galaxies: kinematics and dynamics,Galaxy: evolution,ISM: evolution,Methods: N-body simulations},
number = {2},
pages = {509--518},
primaryClass = {astro-ph},
title = {{Modelling galaxies with a 3d multi-phase ISM}},
volume = {449},
year = {2006}
}
@article{King2021,
abstract = {The sample of dwarf galaxies with measured central black hole masses M and velocity dispersions $\sigma$ has recently doubled, and gives a close fit to the extrapolation of the M-$\sigma$ relation for more massive galaxies. We argue that this is difficult to reconcile with suggestions that the scaling relations between galaxies and their central black holes are simply a statistical consequence of assembly through repeated mergers. This predicts black hole masses significantly larger than those observed in dwarf galaxies unless the initial distribution of uncorrelated seed black hole and stellar masses is confined to much smaller masses than earlier assumed. It also predicts a noticeable flattening of the M-$\sigma$ relation for dwarfs, to M $\sigma$2 compared with the observed M $\sigma$4. In contrast black hole feedback predicts that black hole masses tend towards a universal M $\sigma$4 relation in all galaxies, and correctly gives the properties of powerful outflows recently observed in dwarf galaxies. These considerations emphasize once again that the fundamental physical black hole-galaxy scaling relation is between M and $\sigma$. The relation of M to the bulge mass Mb is acausal, and depends on the quite independent connection between Mb and $\sigma$ set by stellar feedback.},
archivePrefix = {arXiv},
arxivId = {2012.06258},
author = {King, Andrew and Nealon, Rebecca},
doi = {10.1093/mnrasl/slaa200},
eprint = {2012.06258},
file = {:home/william/Documents/Papers/2012.06258.pdf:pdf},
issn = {17453933},
journal = {Mon. Not. R. Astron. Soc. Lett.},
keywords = {X-rays: galaxies: dwarf,black hole physics,galaxies: Active,galaxies: Seyfert,quasars: general},
number = {1},
pages = {L1--L5},
title = {{Dwarf galaxies and the black hole scaling relations}},
volume = {502},
year = {2021}
}
@article{Plotnikov2018,
abstract = {Perpendicular relativistic ($\gamma$ 0= 10) shocks in magnetized pair plasmas are investigated using two-dimensional Particle-in-Cell simulations. A systematic survey, from unmagnetized to strongly magnetized shocks, is presented accurately capturing the transition from Weibelmediated to magnetic-reflection-shaped shocks. This transition is found to occur for upstream flow magnetizations 10-3 {\textless} $\sigma$ {\textless} 10-2 at which a strong perpendicular net current is observed in the precursor, driving the so-called current-filamentation instability. The global structure of the shock and shock formation time are discussed. The magnetohydrodynamics shock jump conditions are found in good agreement with the numerical results, except for 10-4 {\textless} $\sigma$ {\textless} 10-2 where a deviation up to 10 per cent is observed. The particle precursor length converges towards the Larmor radius of particles injected in the upstream magnetic field at intermediate magnetizations. For $\sigma$ {\textgreater} 10-2, it leaves place to a purely electromagnetic precursor following from the strong emission of electromagnetic waves at the shock front. Particle acceleration is found to be efficient in weakly magnetized perpendicular shocks in agreement with previous works, and is fully suppressed for $\sigma$ {\textgreater} 10-2. Diffusive shock acceleration is observed only in weakly magnetized shocks, while a dominant contribution of shock drift acceleration is evidenced at intermediate magnetizations. The spatial diffusion coefficients are extracted from the simulations allowing for a deeper insight into the self-consistent particle kinematics and scale with the square of the particle energy in weakly magnetized shocks. These results have implications for particle acceleration in the internal shocks of active galactic nucleus jets and in the termination shocks of pulsar wind nebulae.},
archivePrefix = {arXiv},
arxivId = {1712.02883},
author = {Plotnikov, Illya and Grassi, Anna and Grech, Mickael},
doi = {10.1093/MNRAS/STY979},
eprint = {1712.02883},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Grassi, Grech - 2018 - Perpendicular relativistic shocks in magnetized pair plasma Illya.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Acceleration of particles,Plasmas,Relativistic processes,Shock waves},
number = {4},
pages = {5238--5260},
title = {{Perpendicular relativistic shocks in magnetized pair plasma}},
volume = {477},
year = {2018}
}
@article{Kataoka2013a,
abstract = {We present Suzaku X-ray observations along two edge regions of the Fermi Bubbles, with eight {\~{}}20 ksec pointings across the northern part of the North Polar Spur (NPS) surrounding the north bubble and six across the southernmost edge of the south bubble. After removing compact X-ray features, diffuse X-ray emission is clearly detected and is well reproduced by a three-component spectral model consisting of unabsorbed thermal emission (temperature kT {\~{}}0.1 keV from the Local Bubble (LB), absorbed kT {\~{}}0.3 keV thermal emission related to the NPS and/or Galactic Halo (GH), and a power-law component at a level consistent with the cosmic X-ray background. The emission measure (EM) of the 0.3 keV plasma decreases by {\~{}}50{\%} toward the inner regions of the north-east bubble, with no accompanying temperature change. However, such a jump in the EM is not clearly seen in the south bubble data. While it is unclear if the NPS originates from a nearby supernova remnant or is related to previous activity within/around the Galactic Center, our Suzaku observations provide evidence suggestive of the latter scenario. In the latter framework, the presence of a large amount of neutral matter absorbing the X-ray emission as well as the existence of the kT {\~{}} 0.3 keV gas can be naturally interpreted as a weak shock driven by the bubbles' expansion in the surrounding medium, with velocity v{\_}exp {\~{}}300 km/s (corresponding to shock Mach number M {\~{}}1.5), compressing the GH gas to form the NPS feature. We also derived an upper limit for any non-thermal X-ray emission component associated with the bubbles and demonstrate, that in agreement with the findings above, the non-thermal pressure and energy estimated from a one-zone leptonic model of its broad-band spectrum, are in rough equilibrium with that of the surrounding thermal plasma.},
author = {Kataoka, J. and Tahara, M. and Totani, T. and Sofue, Y. and Stawarz and Takahashi, Y. and Takeuchi, Y. and Tsunemi, H. and Kimura, M. and Takei, Y. and Cheung, C. C. and Inoue, Y. and Nakamori, T.},
doi = {10.1088/0004-637X/779/1/57},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Kataoka et al. - 2013 - SUZAKU observations of the diffuse X-ray emission across the Fermi Bubbles' edges.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {Galaxy: center,Galaxy: halo,X-rays: ISM,acceleration of particles,cosmic rays},
number = {1},
title = {{SUZAKU observations of the diffuse X-ray emission across the Fermi Bubbles' edges}},
volume = {779},
year = {2013}
}
@article{Biernacki2017,
abstract = {We have recently improved our model of active galactic nucleus (AGN) by attaching the supermassive black hole (SMBH) to a massive nuclear star cluster (NSC). Here we study the effects of this new model in massive, gas-rich galaxies with several simulations of different feedback recipes with the hydrodynamics code RAMSES. These simulations are compared to a reference simulation without any feedback, in which the cooling halo gas is quickly consumed in a burst of star formation. In the presence of strong supernovae (SN) feedback, we observe the formation of a galactic fountain that regulates star formation over a longer period, but without halting it. If only AGN feedback is considered, as soon as the SMBH reaches a critical mass, strong outflows of hot gas are launched and prevent the cooling halo gas from reaching the disk, thus efficiently halting star formation, leading to the so-called "quenching". If both feedback mechanisms act in tandem, we observe a non-linear coupling, in the sense that the dense gas in the supernovae-powered galactic fountain is propelled by the hot outflow powered by the AGN at much larger radii than without AGN. We argue that these particular outflows are able to unbind dense gas from the galactic halo, thanks to the combined effect of SN and AGN feedback. We speculate that this mechanism occurs at the end of the fast growing phase of SMBH, and is at the origin of the dense molecular outflows observed in many massive high-redshift galaxies.},
archivePrefix = {arXiv},
arxivId = {1712.02794},
author = {Biernacki, Pawel and Teyssier, Romain},
doi = {10.1093/mnras/sty216},
eprint = {1712.02794},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Biernacki, Teyssier - 2017 - The combined effect of AGN and supernovae feedback in launching massive molecular outflows in high-redshift.pdf:pdf},
issn = {0035-8711},
keywords = {active,evolution,galaxies,methods,numerical,quasars,supermas-},
pages = {5688--5703},
title = {{The combined effect of AGN and supernovae feedback in launching massive molecular outflows in high-redshift galaxies}},
url = {http://arxiv.org/abs/1712.02794{\%}0Ahttp://dx.doi.org/10.1093/mnras/sty216},
volume = {5703},
year = {2017}
}
@article{Dawson1964,
abstract = {Calculations are presented which show that a laser pulse delivering powers of the order of 1010 W to a liquid or solid particle with dimensions of the order of 10-2 cm will produce a hot plasma with temperatures in the range of several hundred eV. To a large extent the plasma temperature is held down by its rapid expansion and cooling. This converts much of the energy supplied into ordered energy of expansion. This ordered expansion energy can amount to several keV per ion. If the expanding plasma can be caught in a magnetic field and its ordered motion converted to random motion this might be utilized as a means for filling controlled thermonuclear fusion devices with hot plasma. Further, it should also be possible to do many interesting plasma experiments on such plasmas.},
author = {Dawson, John M.},
doi = {10.1063/1.1711346},
file = {:home/william/Documents/Papers/dawson1964.pdf:pdf},
issn = {10706631},
journal = {Phys. Fluids},
number = {7},
pages = {981--987},
title = {{On the production of plasma by giant pulse lasers}},
volume = {7},
year = {1964}
}
@article{Chevalier1985,
abstract = {Galaxies with highly active star formation regions (starburst galaxies) are inferred to have high supernova rates in the region of activity. If most of the supernova energy input is thermalized, a strong wind is driven out of the active region. The authors present an analytical solution for the wind which is driven from a region of uniform mass and energy deposition. The solution is applied to M82 - the best observed case of a starburst galaxy.},
author = {Chevalier, R. A. and Clegg, A. W.},
doi = {10.1038/317044a0},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Chevalier, Clegg - 1985 - Wind from a starburst galaxy nucleus.pdf:pdf},
issn = {00280836},
journal = {Nature},
number = {6032},
pages = {44--45},
title = {{Wind from a starburst galaxy nucleus}},
volume = {317},
year = {1985}
}
@article{Juranova2022,
abstract = {Spectral-timing techniques have proven valuable in studying the interplay between the X-ray corona and the accretion disc in variable active galactic nuclei (AGN). Under certain conditions, photo-ionized outflows emerging from central AGN regions also play a role in the observable spectral-timing properties of the nuclear components. The variable ionizing flux causes the intervening gas to ionize or recombine, resulting in a time-dependent absorption spectrum. Understanding the spectral-timing properties of these outflows is critical for the determination of their role in the AGN environment, but also the correct interpretation of timing signatures of other AGN components. In this paper, we test the capabilities of the Athena X-IFU instrument in studying the spectral and spectral-timing properties of a black hole system displaying a variable outflow. We take the narrow-line Seyfert 1 IRAS 13224-3809 as a test case. Our findings show that while the non-linear response of the absorbing medium can result in complex behaviour of time lags, the resulting decrease in the coherence can be used to constrain gas density and distance to the central source. Ultimately, modelling the coherence spectra of AGN outflows may constitute a valuable tool in studying the physical properties of the outflowing gas.},
archivePrefix = {arXiv},
arxivId = {2201.02640},
author = {Jur{\'{a}}ňov{\'{a}}, A. and Costantini, E. and Uttley, P.},
eprint = {2201.02640},
file = {:home/william/Documents/Papers/2201.02640.pdf:pdf},
keywords = {absorption lines,galaxies,individual,iras 13224-3809,methods,numerical,quasars,seyfert},
number = {January},
pages = {1--11},
title = {{Spectral-timing of AGN ionized outflows with Athena}},
url = {http://arxiv.org/abs/2201.02640},
volume = {11},
year = {2022}
}
@article{Lykins2013,
abstract = {We discuss recent improvements in the calculation of the radiative cooling in both collisionally ionized and photoionized plasmas. We are extending the spectral simulation code CLOUDY so that as much as possible of the underlying atomic data are taken from external data bases, some created by others and some developed by the CLOUDY team. This paper focuses on recent changes in the treatment of many stages of ionization of iron, and discusses its extensions to other elements. The H- and He-like ions are treated in the isoelectronic approach described previously. Fe II is a special case treated with a large model atom. Here we focus on Fe III through Fe XXIV, ions which are important contributors to the radiative cooling of hot (T {\~{}} 105-107 K) plasmas and for X-ray spectroscopy. We use the Chianti atomic data base to greatly expand the number of transitions in the cooling function. Chianti only includes lines that have atomic data computed by sophisticated methods. This limits the line list to lower excitation, longer wavelength, transitions.We had previously included lines from the Opacity Project data base, which tends to include higher energy, shorter wavelength, transitions. These were combined with various forms of the 'g-bar' approximation, a highly approximate method of estimating collision rates. For several iron ions the two data bases are almost entirely complementary.We adopt a hybrid approach in which we use Chianti where possible, supplemented by lines from the Opacity Project for shorter wavelength transitions. The total cooling including the lightest 30 elements differs from some previous calculations by significant amounts. {\textcopyright} 2013 The Authors. Published by Oxford University Press on behalf of the Royal Astronomical Society.},
author = {Lykins, M. L. and Ferland, G. J. and Porter, Ryan L. and van Hoof, Peter A.M. and Williams, R. J.R. and Gnat, Orly},
doi = {10.1093/mnras/sts570},
file = {:home/william/Documents/Papers/sts570.pdf:pdf},
issn = {00358711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Atomic data-plasmas-methods,Numerical},
number = {4},
pages = {3133--3143},
title = {{Radiative cooling in collisionally ionized and photoionized plasmas}},
volume = {429},
year = {2013}
}
@article{Herold2019,
abstract = {The Fermi bubbles (FBs) are large gamma-ray emitting lobes extending up to {\$}55\backslashdeg{\$} in latitude above and below the Galactic center (GC). Although the FBs were discovered 8 years ago, their origin and the nature of the gamma-ray emission are still unresolved. Understanding the properties of the FBs near the Galactic plane may provide a clue to their origin. Previous analyses of the gamma-ray emission at the base of the FBs, what remains after subtraction of Galactic foregrounds, have shown an increased intensity compared to the FBs at high latitudes, a hard power-law spectrum without evidence of a cutoff up to approximately 1 TeV, and a displacement of the emission to negative longitudes relative to the GC. We analyze 9 years of Fermi Large Area Telescope data in order to study in more detail the gamma-ray emission at the base of the FBs, especially at energies above 10 GeV. We confirm that the gamma-ray emission at the base of the FBs is well described by a simple power law up to 1 TeV energies. The 95{\%} confidence lower limit on the cutoff energy is about 500 GeV. It has larger intensity than the FBs emission at high latitudes and is shifted to the west (negative longitudes) from the GC. If the emission at the base of the FBs is indeed connected to the high-latitude FBs, then the shift of the emission to negative longitudes disfavors models where the FBs are created by the supermassive black hole at the GC. We find that the gamma-ray spectrum can be explained either by gamma rays produced in hadronic interactions or by leptonic inverse Compton scattering. In the hadronic scenario, the emission at the base of the FBs can be explained either by several hundred supernova remnants (SNRs) near the Galactic center or by about 10 SNRs at a distance of {\~{}} 1 kpc. In the leptonic scenario, the necessary number of SNRs is a factor of a few larger than in the hadronic scenario. (abridged)},
archivePrefix = {arXiv},
arxivId = {1904.01454},
author = {Herold, Laura and Malyshev, Dmitry},
eprint = {1904.01454},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Herold, Malyshev - 2019 - Hard and bright gamma-ray emission at the base of the Fermi bubbles.pdf:pdf},
keywords = {center,galaxy,gamma rays,general,halo,ism,jets and outflows},
title = {{Hard and bright gamma-ray emission at the base of the Fermi bubbles}},
url = {http://arxiv.org/abs/1904.01454},
year = {2019}
}
@misc{Caraveo2020,
abstract = {High-energy photons are a powerful tool to understand the most violent phenomena in our Universe. However, detecting gamma-ray photons is a daunting task both owing to the overwhelming presence of cosmic rays and to the opacity of our atmosphere. Thus, direct detection of gamma-ray photons must be done in space, while instruments on the ground can see very high-energy photons through the secondary particles they produce in the atmosphere. Mastering space instruments as well as ground-based ones required decades of relentless efforts implying hardware and software developments as well as theoretical studies and extensive simulations. Space instruments, as well as ground-based ones, are now producing a steady flow of important results often in conjunction with observatories working at different wavelengths. Multi-messenger astronomy, which combines the electromagnetic channel with gravitational waves and neutrinos, is the newly born discipline to which high-energy gamma-ray detectors provide an essential contribution. Building instruments to continuously cover the gamma-ray sky is, thus, a priority for the astronomical community which is looking forward for the Cherenkov Telescope Array, a new generation ground based gamma-ray observatory designed to monitor, to study and to unveil the mysteries hidden in the very high energy sky.},
author = {Caraveo, Patrizia A},
booktitle = {Riv. del Nuovo Cim.},
doi = {10.1007/s40766-020-00006-3},
file = {:home/william/Documents/Papers/Caraveo2020{\_}Article{\_}TheGoldenAgeOfHigh-energyGamma.pdf:pdf},
issn = {18269850},
keywords = {Cherenkov telescopes,Gamma-ray astronomy,Gamma-ray missions,Gamma-ray sources,Multi-messenger astronomy},
number = {6},
pages = {281--318},
publisher = {Springer Berlin Heidelberg},
title = {{The golden age of high-energy gamma-ray astronomy: the Cherenkov Telescope Array in the multimessenger era}},
url = {https://doi.org/10.1007/s40766-020-00006-3},
volume = {43},
year = {2020}
}
@article{Rees1984,
author = {Rees, Martin J},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Rees - 1984 - Black hole models for active galactic nuclei.pdf:pdf},
pages = {471--506},
title = {{Black hole models for active galactic nuclei}},
year = {1984}
}
@article{Prieto2017a,
abstract = {By using cosmological hydrodynamical simulations we study the effect of supernova (SN) and active galactic nuclei (AGN) feedback on the mass transport of gas on to galactic nuclei and the black hole (BH) growth down to redshift z{\~{}}6. We study the BH growth in relation with the mass transport processes associated with gravity and pressure torques, and how they are modified by feedback. Cosmological gas funelled through cold flows reaches the galactic outer region close to free-fall. Then torques associated to pressure triggered by gas turbulent motions produced in the circum-galactic medium by shocks and explosions from SNe are the main source of mass transport beyond the central {\~{}} 100 pc. Due to high concentrations of mass in the central galactic region, gravitational torques tend to be more important at high redshift. The combined effect of almost free-falling material and both gravity and pressure torques produces a mass accretion rate of order {\~{}} 1 M{\_}sun/yr at {\~{}} pc scales. In the absence of SN feedback, AGN feedback alone does not affect significantly either star formation or BH growth until the BH reaches a sufficiently high mass of {\$}\backslashsim 10{\^{}}6{\$} M{\_}sun to self-regulate. SN feedback alone, instead, decreases both stellar and BH growth. Finally, SN and AGN feedback in tandem efficiently quench the BH growth, while star formation remains at the levels set by SN feedback alone due to the small final BH mass, {\~{}} few 10{\^{}}5 M{\_}sun. SNe create a more rarefied and hot environment where energy injection from the central AGN can accelerate the gas further.},
archivePrefix = {arXiv},
arxivId = {1701.06172},
author = {Prieto, Joaquin and Escala, Andres and Volonteri, Marta and Dubois, Yohan},
doi = {10.3847/1538-4357/aa5be5},
eprint = {1701.06172},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Prieto et al. - 2017 - How AGN and SNe feedback affect mass transport and black hole growth in high redshift galaxies.pdf:pdf},
issn = {1538-4357},
journal = {Astrophys. J.},
keywords = {formation,galaxies,galaxies: formation,large-scale structure of the,large-scale structure of the universe,quasars,quasars: supermassive black holes,stars,stars: formation,supermassive black holes,turbulence,universe},
number = {2},
pages = {1--13},
publisher = {IOP Publishing},
title = {{How AGN and SNe feedback affect mass transport and black hole growth in high redshift galaxies}},
url = {http://arxiv.org/abs/1701.06172{\%}0Ahttp://dx.doi.org/10.3847/1538-4357/aa5be5},
volume = {836},
year = {2017}
}
@article{Mukherjee2018a,
abstract = {We study the interactions of a relativistic jet with a dense turbulent gaseous disk of radius {\$}\backslashsim 2{\$} kpc. We have performed a suite of simulations with different mean density, jet power and orientation. Our results show that: A) the relativistic jet couples strongly with the gas in the inner kpc, creating a cavity and launching outflows. B) The high pressure bubble inflated by the jet and its back-flow compresses the disk at the outer edges, driving inflows within the disk. C) Jets inclined towards the disk couple more strongly with the disk and launch sub-relativistic, wide-angle outflows along the minor axis. D) Shocks driven directly by the jet and the jet-driven energy bubble raise the velocity dispersion throughout the disk by several times its initial value. E) Compression by the jet-driven shocks can enhance the star formation rate in the disk, especially in a ring-like geometry close to the axis. However, enhanced turbulent dispersion in the disk also leads to quenching of star formation. Whether positive or negative feedback dominates depends on jet power, ISM density, jet orientation with respect to the disc, and the time-scale under consideration. Qualitatively, our simulations compare favourably with kinematic and morphological signatures of several observed galaxies such as NGC 1052, NGC 3079, 3C 326 and 3C 293.},
archivePrefix = {arXiv},
arxivId = {1803.08305},
author = {Mukherjee, Dipanjan and Bicknell, Geoffrey V. and Wagner, Alexander Y. and Sutherland, Ralph S. and Silk, Joseph},
doi = {10.1093/mnras/sty1776},
eprint = {1803.08305},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Mukherjee et al. - 2018 - Relativistic jet feedback - III. Feedback on gas discs.pdf:pdf},
issn = {0035-8711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: evolution,Galaxies: highredshift,Galaxies: ism,Galaxies: jets,Hydrodynamics,Methods: numerical},
month = {oct},
number = {4},
pages = {5544--5566},
publisher = {Oxford University Press},
title = {{Relativistic jet feedback – III. Feedback on gas discs}},
url = {https://academic.oup.com/mnras/article/479/4/5544/5049320},
volume = {479},
year = {2018}
}
@article{LIMAetal.1982,
author = {LIMA et al.},
doi = {10.1016/S0197-0186(13)00110-1},
file = {:home/william/Documents/Papers/[Soltan]-Masses of Quasares.pdf:pdf},
number = {1981},
pages = {p.173--203},
title = {{No 主観的健康感を中心とした在宅高齢者における 健康関連指標に関する共分散構造分析Title}},
year = {1982}
}
@article{Balestra2005,
abstract = {We present a 23 ks XMM-Newton observation of the Ultraluminous Infrared Galaxy (ULIRG) Mrk 273. The hard X-ray spectrum can be modeled by a highly absorbed (∼7 × 1023 cm-2) power law plus an Fe Ka emission line. The iron line (detected at more than 99{\%} c.l.) is broad ($\sigma$ = 0.26-0.17+0.37 keV), suggesting possible superposition of a neutral iron line at 6.4 keV, and a blend of ionized iron lines from Fe XXV and Fe XXVI. Given the relatively short exposure, the three line components cannot be individually resolved with high statistical significance: the neutral component is detected at∼2.5$\sigma$ and the Fe XXV line at ∼2$\sigma$ c.l., while for the Fe XXVI line we can only estimate an upper limit. The broad band spectrum requires, in addition to a highly absorbed power law, at least three collisionally ionized plasma components, which may be associated with star-forming regions. The temperatures of the three plasmas are about 0.3, 0.8 and 6 keV, where the highest of the three is sufficient to produce ionized iron emission lines. An alternative interpretation for the origin of the soft emission might also be reflection off photoionized gas, as has been observed in a number of nearby Compton-thick Seyfert 2 galaxies (e.g. NGC 1068, Circinus, Mrk 3, NGC 4945). A hot gas, photoionized by the primary, continuum can also produce ionized iron lines. Unfortunately, given the limited statistics and the lack of high resolution spectroscopy, it is not possible to distinguish between the two models investigated. We further compare the XMM-Newton findings with the Chandra data obtaining consistent spectral results. The absorption-corrected hard X-ray luminosity of Mrk 273 is L 2-10kev ∼ 7 × 1042 erg s-1, corresponding to ∼0.2{\%} of the far-IR luminosity, similar to typical values found in pure starbursts. The thermal contribution to the soft X-ray luminosity is approximately 0.2-0.7 × 1042 ergs-1, comparable to those found in NGC 6240 and other starburst-dominated ULIRGs. We also analyze the XMM-Newton spectrum of Mrk 273x, an unabsorbed Seyfert 2 galaxy at redshift z = 0.458, which lies in the field of view of Mrk 273. {\textcopyright} ESO 2005.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0507321},
author = {Balestra, I. and Boller, Th and Gallo, L. and Lutz, D. and Hess, S.},
doi = {10.1051/0004-6361:20053558},
eprint = {0507321},
file = {:home/william/Documents/Papers/aa3558-05.pdf:pdf},
issn = {00046361},
journal = {Astron. Astrophys.},
keywords = {Galaxies: Seyfert,Galaxies: individual: Mrk 273,Galaxies: individual: Mrk 273x,X-rays: galaxies},
number = {2},
pages = {469--478},
primaryClass = {astro-ph},
title = {{XMM-Newton spectral properties of the ultraluminous IRAS galaxy Mrk 273}},
volume = {442},
year = {2005}
}
@article{Lonsdale2006a,
author = {Lonsdale, C J and Farrah, D and Smith, H E},
file = {:home/william/Documents/Papers/ultraluminous-infrared-galaxies.pdf:pdf},
journal = {Astrophys. Updat.},
title = {{Chap.9 Ultraluminous Infrared Galaxies}},
year = {2006}
}
@article{Pino2012,
abstract = {The formation of protostellar disks out of molecular cloud cores is still not fully understood. Under ideal MHD conditions, the removal of angular momentum from the disk progenitor by the typically embedded magnetic field may prevent the formation of a rotationally supported disk during the main protostellar accretion phase of low-mass stars. This has been known as the magnetic braking problem and the most investigated mechanism to alleviate this problem and help remove the excess of magnetic flux during the star formation process, the so-called ambipolar diffusion (AD), has been shown to be not sufficient to weaken the magnetic braking at least at this stage of the disk formation. In this work, motivated by recent progress in the understanding of magnetic reconnection in turbulent environments, we appeal to the diffusion of magnetic field mediated by magnetic reconnection as an alternative mechanism for removing magnetic flux. We investigate numerically this mechanism during the later phases of the protostellar disk formation and show its high efficiency. By means of fully three-dimensional MHD simulations, we show that the diffusivity arising from turbulent magnetic reconnection is able to transport magnetic flux to the outskirts of the disk progenitor at timescales compatible with the collapse, allowing the formation of a rotationally supported disk around the protostar of dimensions 100AU, with a nearly Keplerian profile in the early accretion phase. Since MHD turbulence is expected to be present in protostellar disks, this is a natural mechanism for removing magnetic flux excess and allowing the formation of these disks. This mechanism dismisses the necessity of postulating a hypothetical increase of the ohmic resistivity as discussed in the literature. Together with our earlier work which showed that magnetic flux removal from molecular cloud cores is very efficient, this work calls for reconsidering the relative role of AD in the processes of star and planet formation. {\textcopyright} 2012. The American Astronomical Society. All rights reserved.},
author = {Santos-Lima, R. and {De Gouveia Dal Pino}, E. M. and Lazarian, A},
doi = {10.1088/0004-637X/747/1/21},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Pino, Lazarian - 2012 - THE ROLE OF TURBULENT MAGNETIC RECONNECTION IN THE FORMATION OF.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {ISM: magnetic fields,accretion,accretion disks,diffusion,magnetohydrodynamics (MHD),stars: formation,turbulence},
number = {1},
title = {{The role of turbulent magnetic reconnection in the formation of rotationally supported protostellar disks}},
volume = {747},
year = {2012}
}
@article{BrianYu2020a,
abstract = {Outflows from starburst galaxies can be driven by thermal pressure, radiation, and cosmic rays. We present an analytic phenomenological model that accounts for these contributions simultaneously to investigate their effects on the hydrodynamical properties of outflows. We assess the impact of energy injection, wind opacity, magnetic field strength, and the mass of the host galaxy on flow velocity, temperature, density, and pressure profiles. For an M82-like wind, a thermally dominated driving mechanism is found to deliver the fastest and hottest wind. Radiation-driven winds in typical starburst-galaxy configurations are unable to attain the higher flow velocities and temperatures associated with thermal and cosmic ray-driven systems, leading to higher wind densities which would be more susceptible to cooling and fragmentation at lower altitudes. High opacity winds are more sensitive to radiative driving, but terminal flow velocities are still lower than those achieved by other driving mechanisms at realistic opacities. We demonstrate that variations in the outflow magnetic field can influence its coupling with cosmic rays, where stronger fields enable greater streaming but less driving near the base of the flow, instead with cosmic rays redirecting their driving impact to higher altitudes. The gravitational potential is less important in M82-like wind configurations, and substantial variations in the flow profiles only emerge at high altitude in massive haloes. This model offers a more generalized approach to examine the large-scale hydrodynamical properties for a wide variety of starburst galaxies.},
archivePrefix = {arXiv},
arxivId = {2001.04384},
author = {{Brian Yu}, B. P. and Owen, Ellis R. and Wu, Kinwah and Ferreras, Ignacio},
doi = {10.1093/mnras/staa021},
eprint = {2001.04384},
file = {:home/william/Documents/Papers/staa021.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Cosmic rays,Galaxies: Starburst,Hydrodynamics,ISM: Jets and outflows},
number = {3},
pages = {3179--3193},
publisher = {Oxford University Press},
title = {{A hydrodynamical study of outflows in starburst galaxies with different driving mechanisms}},
volume = {3193},
year = {2020}
}
@article{Oda2018,
abstract = {We report the broadband X-ray spectra of the ultra-luminous infrared galaxy (ULIRG) UGC 5101 in the 0.25-100 keV band observed with Swift/Burst Alert Telescope (BAT), NuSTAR, Suzaku, XMM-Newton, and Chandra. A Compton-thick AGN obscured with a hydrogen column density of {\$}\backslashapprox 1.3\backslashtimes10{\^{}}{\{}24{\}}{\$} cm{\$}{\^{}}{\{}-2{\}}{\$} is detected above 10 keV. A spectral fit with a numerical torus model favors a large half opening angle of the torus, {\$}{\textgreater}41{\$} degrees, suggesting that the covering fraction of material heavily obscuring the X-ray source is moderate. The intrinsic 2-10 keV luminosity is determined to be {\$}\backslashapprox 1.4\backslashtimes 10{\^{}}{\{}43{\}}{\$} erg s{\$}{\^{}}{\{}-1{\}}{\$}, which is {\$}\backslashapprox{\$}2.5 times larger than the previous estimate using only data below 10 keV with a simple spectral model. We find that UGC 5101 shows the ratio between the [O IV] 26 {\$}\backslashmu{\$}m line and 2-10 keV luminosities similar to those of normal Seyfert galaxies, along with other ULIRGs observed with NuSTAR, indicating that a significant portion of local ULIRGs are not really "X-ray faint" with respect to the flux of forbidden lines originating from the narrow line region (NLR). We propose a possible scenario that (1) the AGN in UGC 5101 is surrounded not only by Compton-thick matter located close to the equatorial plane but also by Compton-thin ({\$}N{\_}\backslashmathrm{\{}H{\}} \backslashsim 10{\^{}}{\{}21{\}}{\$} cm{\$}{\^{}}{\{}-2{\}}{\$}) matter in the torus-hole region and (2) it is accreting at a high Eddington rate with a steep UV to X-ray spectral energy distribution. Nevertheless, we argue that AGNs in many ULIRGs do not look extraordinary (i.e., extremely X-ray faint), as suggested by recent works, compared with normal Seyferts.},
archivePrefix = {arXiv},
arxivId = {1612.07450},
author = {Oda, Saeko and Tanimoto, Atsushi and Ueda, Yoshihiro and Imanishi, Masatoshi and Terashima, Yuichi and Ricci, Claudio},
doi = {10.3847/1538-4357/835/2/179},
eprint = {1612.07450},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Oda et al. - 2018 - Shedding light on the compton-thick active galactic nucleus in the ultra-luminous infrared galaxy ugc 5101 with broa.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
number = {2},
pages = {179},
title = {{Shedding Light on the Compton-thick Active Galactic Nucleus in the Ultraluminous Infrared Galaxy UGC 5101 with Broadband X-Ray Spectroscopy}},
volume = {835},
year = {2017}
}

@ARTICLE{Pereira-Santaella2021,
       author = {{Pereira-Santaella}, M. and {Colina}, L. and {Garc{\'\i}a-Burillo}, S. and {Lamperti}, I. and {Gonz{\'a}lez-Alfonso}, E. and {Perna}, M. and {Arribas}, S. and {Alonso-Herrero}, A. and {Aalto}, S. and {Combes}, F. and {Labiano}, A. and {Piqueras-L{\'o}pez}, J. and {Rigopoulou}, D. and {van der Werf}, P.},
        title = "{Physics of ULIRGs with MUSE and ALMA: The PUMA project. II. Are local ULIRGs powered by AGN? The subkiloparsec view of the 220 GHz continuum}",
      journal = {\aap},
     keywords = {galaxies: evolution, galaxies: interactions, galaxies: nuclei, infrared: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = jul,
       volume = {651},
          eid = {A42},
        pages = {A42},
          doi = {10.1051/0004-6361/202140955},
archivePrefix = {arXiv},
       eprint = {2104.08238},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...651A..42P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Ibanez-Mejia2017,
abstract = {In order to understand the origin of observed molecular cloud properties, it is critical to understand how clouds interact with their environments during their formation, growth, and collapse. It has been suggested that accretion-driven turbulence can maintain clouds in a highly turbulent state, preventing runaway collapse, and explaining the observed non-thermal velocity dispersions. We present 3D, AMR, MHD simulations of a kiloparsec-scale, stratified, supernova-driven, self-gravitating, interstellar medium, including diffuse heating and radiative cooling. These simulations model the formation and evolution of a molecular cloud population in the turbulent interstellar medium. We use zoom-in techniques to focus on the dynamics of the mass accretion and its history for individual molecular clouds. We find that mass accretion onto molecular clouds proceeds as a combination of turbulent and near free-fall accretion of a gravitationally bound envelope. Nearby supernova explosions have a dual role, compressing the envelope, boosting accreted mass, but also disrupting parts of the envelope and eroding mass from the cloud's surface. It appears that the inflow rate of kinetic energy onto clouds from supernova explosions is insufficient to explain the net rate of charge of the cloud kinetic energy. In the absence of self-consistent star formation, conversion of gravitational potential into kinetic energy during contraction seems to be the main driver of non-thermal motions within clouds. We conclude that although clouds interact strongly with their environments, bound clouds are always in a state of gravitational contraction, close to runaway, and their properties are a natural result of this collapse.},
archivePrefix = {arXiv},
arxivId = {1705.01779},
author = {Ib{\'{a}}{\~{n}}ez-Mej{\'{i}}a, Juan C. and {Mac Low}, Mordecai-Mark and Klessen, Ralf S. and Baczynski, Christian},
doi = {10.3847/1538-4357/aa93fe},
eprint = {1705.01779},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ib{\'{a}}{\~{n}}ez-Mej{\'{i}}a et al. - 2017 - Feeding vs. Falling The growth and collapse of molecular clouds in a turbulent interstellar medium.pdf:pdf},
issn = {1538-4357},
keywords = {keywords},
title = {{Feeding vs. Falling: The growth and collapse of molecular clouds in a turbulent interstellar medium}},
url = {http://arxiv.org/abs/1705.01779},
year = {2017}
}
@article{Bloch1974,
author = {Bloch, Robert and Tess, Bee},
file = {:home/william/Documents/Papers/1974ApJ...192..597D.pdf:pdf},
pages = {11--30},
title = {{No 主観的健康感を中心とした在宅高齢者における 健康関連指標に関する共分散構造分析Title}},
volume = {1},
year = {1974}
}
@article{Kennicutt2012,
abstract = {We review progress over the past decade in observations of large-scale star formation, with a focus on the interface between extragalactic and Galactic studies. Methods of measuring gas contents and star-formation rates are discussed, and updated prescriptions for calculating star-formation rates are provided. We review relations between star formation and gas on scales ranging from entire galaxies to individual molecular clouds. Copyright {\textcopyright} 2012 by Annual Reviews.},
archivePrefix = {arXiv},
arxivId = {1204.3552},
author = {Kennicutt, Robert C. and Evans, Neal J.},
doi = {10.1146/annurev-astro-081811-125610},
eprint = {1204.3552},
file = {:home/william/Documents/Papers/annurev-astro-081811-125610.pdf:pdf},
issn = {00664146},
journal = {Annu. Rev. Astron. Astrophys.},
keywords = {clouds,evolution,interstellar medium (ISM),molecules},
pages = {531--608},
title = {{Star formation in the milky way and nearby galaxies}},
volume = {50},
year = {2012}
}
@article{Yang2013,
abstract = {The origin of the Fermi bubbles and the microwave haze is yet to be determined. To disentangle different models requires detailed comparisons between theoretical predictions and multi-wavelength observations. Our previous simulations have demonstrated that the primary features of the Fermi bubbles could be successfully reproduced by recent jet activity from the central active galactic nucleus (AGN). In this work, we generate gamma-ray and microwave maps and spectra based on the simulated properties of cosmic rays (CRs) and magnetic fields in order to examine whether the observed bubble and haze emission could be explained by leptons contained in the AGN jets. We also investigate the model predictions of the polarization properties of the Fermi bubbles. We find that: (1) The same population of leptons can simultaneously explain the bubble and haze emission given that the magnetic fields within the bubbles are very close to the exponentially distributed ambient field, which can be explained by mixing in of the ambient field followed by turbulent field amplification; (2) The centrally peaked microwave profile suggests CR replenishment, which is consistent with the presence of a more recent second jet event; (3) The bubble interior exhibits a high degree of polarization because of ordered radial magnetic field lines stretched by elongated vortices behind the shocks; highly-polarized signals could also be observed inside the draping layer; (4) Enhancement of rotation measures could exist within the shock-compressed layer because of increased gas density and more amplified and ordered magnetic fields. We discuss the possibility that the deficient haze emission at b{\textless}-35 degrees is due to the suppression of magnetic fields, which is consistent with the existence of lower-energy CRs causing the polarized emission at 2.3 GHz. Possible AGN jet composition in the leptonic scenario is also discussed.},
author = {Yang, H. Y. K and Ruszkowski, M. and Zweibel, E.},
doi = {10.1093/mnras/stt1772},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Yang, Ruszkowski, Zweibel - 2013 - The Fermi bubbles Gamma-ray, microwave and polarization signatures of leptonic AGN jets.pdf:pdf},
issn = {00358711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Cosmic rays,Galaxy: Nucleus,Gamma-rays: Galaxies,Mhdmethods: Numerical,Radio continuum: Galaxies},
number = {3},
pages = {2734--2746},
title = {{The Fermi bubbles: Gamma-ray, microwave and polarization signatures of leptonic AGN jets}},
volume = {436},
year = {2013}
}
@article{Gupta2017,
abstract = {We reviewed multi-wavelength blazars variability and detection of quasi-periodic oscillations on intra-day timescales. The variability timescale from few minutes to up to less than a days is commonly known as intra-day variability. These fast variations are extremely useful to constrain the size of emitting region, black hole mass estimation, etc. It is noticed that in general blazars show intra-day variability in the complete electromagnetic spectrum. But some class of blazars either do not show or show very little intra-day variability in a specific band of electromagnetic spectrum. Blazars show rarely quasi-periodic oscillations in time series data in optical and X-ray bands. Other properties and emission mechanism of blazars are also briefly discussed.},
archivePrefix = {arXiv},
arxivId = {1712.02516},
author = {Gupta, Alok C.},
doi = {10.3390/galaxies6010001},
eprint = {1712.02516},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Gupta - 2017 - Multi-wavelength Intra-day Variability and Quasi-periodic Oscillation in Blazars.pdf:pdf},
keywords = {cosmic rays,dust,galactic winds,interstellar medium,magnetohydrodynamics,radiation hydrodynamics,radiative transfer,starbursts,supernovae},
pages = {1--47},
title = {{Multi-wavelength Intra-day Variability and Quasi-periodic Oscillation in Blazars}},
url = {http://arxiv.org/abs/1712.02516{\%}0Ahttp://dx.doi.org/10.3390/galaxies6010001},
year = {2017}
}
@article{Pate2020,
abstract = {The Casimir force was predicted in 1948 as a force arising between macroscopic bodies from the zero-point energy. At finite temperatures it has been shown that a thermal Casimir force exists due to thermal rather than zero-point energy and there are a growing number of experiments that characterise the effect at a range of temperatures and distances. Additionally, in the rapidly evolving field of cavity optomechanics there is an endeavor to manipulate phonons and enhance coherence. We demonstrate a new way to achieve this through the first observation of Casimir spring and dilution in macroscopic optomechanics, by coupling a metallic SiN membrane to a photonic re-entrant cavity. The attraction of the spatially-localised Casimir spring mimics a non-contacting boundary condition giving rise to increased strain and acoustic coherence through dissipation dilution. This work invents a new way to manipulate phonons via thermal photons leading to ``in situ'' reconfigurable mechanical states, to reduce loss mechanisms and to create new types of acoustic non-linearity -- all at room temperature.},
archivePrefix = {arXiv},
arxivId = {2004.05983},
author = {Pate, Jacob M. and Goryachev, Maxim and Chiao, Raymond Y. and Sharping, Jay E. and Tobar, Michael Edmund},
doi = {10.1038/s41567-020-0975-9},
eprint = {2004.05983},
file = {:home/william/Documents/Papers/10.1038s41567-020-0975-9.pdf:pdf;:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Pate et al. - 2020 - Casimir spring and dilution in macroscopic cavity optomechanics.pdf:pdf},
issn = {17452481},
journal = {Nat. Phys.},
publisher = {Springer US},
title = {{Casimir spring and dilution in macroscopic cavity optomechanics}},
url = {http://arxiv.org/abs/2004.05983},
year = {2020}
}
@article{Prakash2019,
abstract = {We report the discovery of a mid-infrared variable AGN which is hosted by an ultraluminous infrared galaxy (ULIRG) candidate in the Sloan Stripe 82 field. WISE J030654.88+010833.6 is a red, extended galaxy, which we estimate to be at a photometric redshift of 0.28 ≤ z ≤ 0.31, based on its optical and near-infrared spectral energy distribution (SED). The factor of two variability over 8 years seen in the WISE 3.4 and 4.6 µm wavelength channels is not clearly correlated with optical variability in archival data. Based on our estimation of the physical parameters of the host galaxy, J030654.88+010833.6 is possibly a composite AGN/starburst ULIRG in a phase where high star formation ∼ 70 M☉ year−1 is occurring. Our estimate of the black hole mass to stellar mass ratio also appears to be consistent with that of broad line AGN in the local universe. The long-term variability of J030654.88+010833.6 as seen in the WISE W1 and W2 light curves is likely due to variations in the accretion rate, with the energy being reprocessed by dust in the vicinity of the AGN.},
archivePrefix = {arXiv},
arxivId = {1908.04280},
author = {Prakash, Abhishek and Chary, Ranga Ram and Helou, George and Faisst, Andreas and Graham, Matthew J. and Masci, Frank J. and Shupe, David L. and Lee, Bomee},
doi = {10.3847/1538-4357/ab3b0b},
eprint = {1908.04280},
file = {:home/william/Documents/Papers/Prakash{\_}2019{\_}ApJ{\_}883{\_}154.pdf:pdf},
issn = {23318422},
journal = {arXiv},
keywords = {AGN,Catalogs,Galaxy,Light curve,Miscellaneous,SED,Surveys},
number = {2},
pages = {154},
publisher = {IOP Publishing},
title = {{A flaring AGN in a ULIRG candidate in stripe 82}},
url = {http://dx.doi.org/10.3847/1538-4357/ab3b0b},
volume = {883},
year = {2019}
}
@article{Davis2020,
author = {Davis, Shane and Tchekhovskoy, Alexander},
doi = {10.1146/annurev-astro-081817-051905},
file = {:home/william/Documents/Papers/10.1146annurev-astro-081817-051905.pdf:pdf},
issn = {1545-4282},
journal = {Annu. Rev. Astron. Astrophys.},
keywords = {black hole physics,general relativity,radiation transport},
number = {1},
pages = {407--439},
title = {{Magnetohydrodynamic Simulations of Active Galactic Nucleus Disks and Jets}},
volume = {58},
year = {2020}
}
@article{Evans2010,
abstract = {We present initial results from a new 440-ks Chandra HETG GTO observation of the canonical Seyfert 2 galaxy NGC 1068. The proximity of NGC 1068, together with Chandra's superb spatial and spectral resolution, allow an unprecedented view of its nucleus and circumnuclear NLR. We perform the first spatially resolved high-resolution X-ray spectroscopy of the 'ionization cone' in any AGN, and use the sensitive line diagnostics offered by the HETG to measure the ionization state, density, and temperature at discrete points along the ionized NLR. We argue that the NLR takes the form of outflowing photoionized gas, rather than gas that has been collisionally ionized by the small-scale radio jet in NGC 1068. We investigate evidence for any velocity gradients in the outflow, and describe our next steps in modeling the spatially resolved spectra as a function of distance from the nucleus. {\textcopyright} 2010 American Institute of Physics.},
archivePrefix = {arXiv},
arxivId = {arXiv:0910.3023v2},
author = {Evans, D. A. and Ogle, P. M. and Marshall, H. L. and Nowak, M. A. and Bianchi, S. and Guainazzi, M. and Dewey, D. and Schulz, N. S. and Noble, M. S. and Houck, J. and Canizares, C. R.},
doi = {10.1063/1.3475282},
eprint = {arXiv:0910.3023v2},
file = {:home/william/Documents/Papers/0910.3023.pdf:pdf},
isbn = {9780735407954},
issn = {0094243X},
journal = {AIP Conf. Proc.},
keywords = {X-rays: galaxies,galaxies: active,galaxies: individual (NGC 1068)},
pages = {425--428},
title = {{Spatially resolved Chandra HETG spectroscopy of the NLR ionization cone in NGC 1068}},
volume = {1248},
year = {2010}
}
@article{Melioli2008,
abstract = {The ejection of the gas out of the disk in late-type galaxies is related to star formation and is due mainly to Type II supernovae. In this paper we studied in detail the development of the Galactic fountains in order to understand their dynamical evolution and their influence in the redistribution of the freshly delivered metals over the disk. To this aim, we performed a number of 3D hydrodynamical radiative cooling simulations of the gas in the Milky Way where the whole Galaxy structure, the Galactic differential rotation and the supernovae explosions generated by a single OB association are considered. A typical fountain powered by 100 Type II supernovae may eject material up to {\$}\backslashsim 2{\$} kpc which than collapses back mostly in form of dense, cold clouds and filaments. The majority of the gas lifted up by the fountains falls back on the disk remaining within a radial distance {\$}\backslashDelta R=0.5{\$} kpc from the place where the fountain originated. This localized circulation of disk gas does not influence the radial chemical gradients on large scale, as required by the chemical models of the Milky Way which reproduce the metallicity distribution without invoking large fluxes of metals. Simulations of multiple fountains fuelled by Type II supernovae of different OB associations will be presented in a companion paper.},
archivePrefix = {arXiv},
arxivId = {0805.1138},
author = {Melioli, C. and Brighenti, F. and D'Ercole, A. and {De Gouveia Dal Pino}, E. M.},
doi = {10.1111/j.1365-2966.2008.13446.x},
eprint = {0805.1138},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Melioli et al. - 2008 - Hydrodynamical simulations of Galactic fountains - I. Evolution of single fountains.pdf:pdf},
issn = {00358711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxy: disc,Galaxy: general,Hydrodynamics,ISM: bubbles,ISM: clouds,Methods: numerical},
number = {2},
pages = {573--586},
title = {{Hydrodynamical simulations of Galactic fountains - I. Evolution of single fountains}},
volume = {388},
year = {2008}
}
@article{Katz1996,
abstract = {We study a family of "classical" orthogonal polynomials which satisfy (apart from a 3-term recurrence relation) an eigenvalue problem with a differential operator of Dunkl-type. These polynomials can be obtained from the little {\$}q{\$}-Jacobi polynomials in the limit {\$}q=-1{\$}. We also show that these polynomials provide a nontrivial realization of the Askey-Wilson algebra for {\$}q=-1{\$}.},
archivePrefix = {arXiv},
arxivId = {1011.1669},
author = {Vinet, Luc and Zhedanov, Alexei},
doi = {10.1088/1751-8113/44/8/085201},
eprint = {1011.1669},
file = {:home/william/Documents/Papers/1996ApJS..105...19K.pdf:pdf},
isbn = {9788578110796},
issn = {1751-8113},
journal = {J. Phys. A Math. Theor.},
keywords = {cosmology: theory — dark matter — galaxies: format},
month = {feb},
number = {8},
pages = {085201},
pmid = {25246403},
title = {{A ‘missing' family of classical orthogonal polynomials}},
url = {http://arxiv.org/abs/1011.1669 http://dx.doi.org/10.1088/1751-8113/44/8/085201 http://www.ncbi.nlm.nih.gov/pubmed/25246403 http://www.pubmedcentral.nih.gov/articlerender.fcgi?artid=PMC4249520 https://iopscience.iop.org/article/10.1088/1751-8113/44/8/08520},
volume = {44},
year = {2011}
}
@article{Falstad2021,
abstract = {Some luminous and ultraluminous infrared galaxies (LIRGs and ULIRGs) host extremely compact and dusty nuclei. The intense infrared radiation arising from warm dust in these sources is prone to excite vibrational levels of molecules such as HCN. This results in emission from the rotational transitions of vibrationally excited HCN (HCN-vib), with the brightest emission found in compact obscured nuclei (CONs). We aim to establish how common CONs are in the local Universe, and whether their prevalence depends on the luminosity or other properties of the host galaxy. We have conducted an Atacama Large Millimeter/submillimeter Array (ALMA) survey of the rotational J=3-2 transition of HCN-vib in a sample of 46 far-infrared luminous galaxies. Compact obscured nuclei are identified in 38 percent of ULIRGs, 21 percent of LIRGs, and 0 percent of lower luminosity galaxies. We find no dependence on the inclination of the host galaxy, but strong evidence of lower IRAS 25 to 60 {\{}$\backslash$mu{\}}m flux density ratios (f25/f60) in CONs compared to the rest of the sample. Furthermore, we find that CONs have stronger silicate features (s9.7{\{}$\backslash$mu{\}}m) but similar PAH equivalent widths (EQW6.2{\{}$\backslash$mu{\}}m) compared to other galaxies. In the local Universe, CONs are primarily found in (U)LIRGs. High resolution continuum observations of the individual nuclei are required to determine if the CON phenomenon is related to the inclinations of the nuclear disks. The lower f25/f60 ratios in CONs as well as the results for the mid-infrared diagnostics investigated are consistent with large dust columns shifting the nuclear radiation to longer wavelengths, making the mid- and far-infrared "photospheres" significantly cooler than the interior regions. To assess the importance of CONs in the context of galaxy evolution, it is necessary to extend this study to higher redshifts where (U)LIRGs are more common.},
archivePrefix = {arXiv},
arxivId = {2102.13563},
author = {Falstad, N. and Aalto, S. and K{\"{o}}nig, S. and Onishi, K. and Muller, S. and Gorski, M. and Sato, M. and Stanley, F. and Combes, F. and Gonz{\'{a}}lez-Alfonso, E. and Mangum, J. G. and Evans, A. S. and Barcos-Mu{\~{n}}oz, L. and Privon, G. C. and Linden, S. T. and D{\'{i}}az-Santos, T. and Mart{\'{i}}n, S. and Sakamoto, K. and Harada, N.},
doi = {10.1051/0004-6361/202039291},
eprint = {2102.13563},
file = {:home/william/Documents/Papers/2102.13563.pdf:pdf},
issn = {0004-6361},
journal = {Astron. Astrophys.},
keywords = {evolution,galaxies,ism,jets and outflows,molecules,nuclei},
pages = {1--16},
title = {{CON-quest. Searching for the most obscured galaxy nuclei}},
year = {2021}
}
@techreport{Berkhuijsen1998,
abstract = {A compilation of data on the volume filling factor f{\_}v of the warm ionized medium as a funcion of the local electron density indicates that approxmately the filling factor is proportional to the inverse of the electron density over 4 decades. This result is exprected for a fractal ISM.},
author = {Berkhuijsen, Elly M.},
file = {:home/william/Documents/Papers/1998LNP...506..301B.pdf:pdf},
pages = {4},
title = {{The Volume Filling Factor of the WIM}},
year = {1998}
}
@article{Tibaduiza2020,
abstract = {Using operator ordering techniques based on Baker-Campbell-Hausdorff (BCH) relations of the su(1,1) Lie algebra and a time-splitting approach, we present an alternative method of solving the dynamics of a time-dependent quantum harmonic oscillator for any initial state. We find an iterative analytical solution given by simple recurrence relations that are very well suited for numerical calculations. We use our solution to reproduce and analyse some results from the literature to prove the usefulness of our method. We also discuss the efficiency in squeezing by comparing the parametric resonance modulation with the so-called Janszky-Adam scheme.},
archivePrefix = {arXiv},
arxivId = {1908.11006},
author = {Tibaduiza, Daniel M. and Pires, Luis and Rego, Andreson L.C. and Szilard, Daniela and Zarro, Carlos and Farina, Carlos},
doi = {10.1088/1402-4896/abb254},
eprint = {1908.11006},
file = {:home/william/Documents/Papers/Efficient algebraic solution for a timedependent quantum harmonic oscillator.pdf:pdf},
issn = {14024896},
journal = {Phys. Scr.},
keywords = {algebraic methods,squeezed states,time-dependent harmonic oscillator},
number = {10},
pages = {105102},
publisher = {IOP Publishing},
title = {{Efficient algebraic solution for a time-dependent quantum harmonic oscillator}},
url = {http://dx.doi.org/10.1088/1402-4896/abb254},
volume = {95},
year = {2020}
}
@article{Bordoloi2016a,
abstract = {We report new observations from a systematic, spectroscopic, ultraviolet absorption-line survey that maps the spatial and kinematic properties of the high-velocity gas in the Galactic Center region. We examine the hypothesis that this gas traces the biconical nuclear outflow. We use ultraviolet spectra of 47 background QSOs and halo stars projected inside and outside the northern Fermi Bubble from the Hubble Space Telescope to study the incidence of high velocity absorption around it. We use five lines of sight inside the northern Fermi Bubble to constrain the velocity and column densities of outflowing gas traced by O I, Al II, C II, C IV, Si II, Si III, Si IV and other species. All five lines of sight inside the northern Fermi Bubble exhibit blueshifted high velocity absorption components, whereas only 9 out of the 42 lines of sight outside the northern Fermi Bubble exhibit blueshifted high velocity absorption components. The observed outflow velocity profile decreases with Galactic latitude and radial distance (R) from the Galactic Center. The observed blueshifted velocities change from {\$}v{\_}{\{}GSR{\}}{\$}=-265 km/s at R{\~{}}2.3 kpc to {\$}v{\_}{\{}GSR{\}}{\$}=-91 km/s at R{\~{}}6.5 kpc. We derive the metallicity of the entrained gas along the 1H1613-097 sightline, which passes through the center of the northern Fermi Bubble, finding [O/H] {\$}\backslashgtrsim -0.54 \backslashpm 0.15{\$}. A simple kinematic model tuned to match the observed absorption component velocities along the five lines of sight inside the Bubble, constrains the outflow velocities to {\~{}}1000{\$}-{\$}1300 km/s, and the age of the outflow to be {\~{}} 6{\$}-{\$}9 Myr. We estimate a minimum mass outflow rate for the nuclear outflow to be {\$}\backslashgtrsim{\$} 0.2 {\$}\backslashrm{\{} M{\_}{\{}\backslashodot{\}}\backslash; yr{\^{}}{\{}-1{\}}{\}}{\$}. Combining the age and mass outflow rates, we determine a minimum mass of total UV absorbing cool gas entrained in the Fermi Bubbles to be {\$}\backslashgtrsim \backslashrm{\{} 2 \backslashtimes 10{\^{}}{\{}6{\}} M{\_}{\{}\backslashodot{\}}{\}}{\$}.},
archivePrefix = {arXiv},
arxivId = {1612.01578},
author = {Bordoloi, Rongmon and Fox, Andrew J. and Lockman, Felix J. and Wakker, Bart P. and Jenkins, Edward B. and Savage, Blair D. and Hernandez, Svea and Tumlinson, Jason and Bland-Hawthorn, Joss and Kim, Tae-Sun},
doi = {10.3847/1538-4357/834/2/191},
eprint = {1612.01578},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Bordoloi et al. - 2016 - MAPPING THE NUCLEAR OUTFLOW OF THE MILKY WAY STUDYING THE KINEMATICS AND SPATIAL EXTENT OF THE NORTHERN FERMI B.pdf:pdf},
issn = {1538-4357},
journal = {Astrophys. J.},
keywords = {Galaxy: center,Galaxy: evolution,Galaxy: halo,ISM: jets and outflows,ISM: kinematics and dynamics,absorption lines,center,dynamics,evolution,galaxy,halo,ism,jets and out fl,kinematics and,ows,quasars,quasars: absorption lines},
number = {2},
pages = {1--21},
publisher = {IOP Publishing},
title = {{MAPPING THE NUCLEAR OUTFLOW OF THE MILKY WAY: STUDYING THE KINEMATICS AND SPATIAL EXTENT OF THE NORTHERN FERMI BUBBLE}},
url = {http://arxiv.org/abs/1612.01578{\%}0Ahttp://dx.doi.org/10.3847/1538-4357/834/2/191},
volume = {834},
year = {2016}
}
@article{Adhikari2018,
abstract = {The Absorption Measure Distribution (AMD) in the X-ray outflows of Seyfert galaxies describes the distribution of absorbing column density as a function of ionization parameter. Up to now, AMD has been measured only for seven objects with high resolution X-ray data that contain absorption lines from ionized heavy elements. Even though the amount of known AMDs is not large, they display universal broad shape with the existence of one prominent dip, for which the absorbing column drops by around two orders of magnitude. In this paper, we used the photoionization modelling to explain the overall AMD shape in observed active galactic nuclei (AGN). In particular, we show that the AMD shape depends both on: the spectral energy distribution (SED) of radiation which enters the outflow, and the density of the warm absorber (WA). Our best AMD model that closely reproduces the observed AMD shape is the one obtained with the gas density of WA of the order of {\$}10{\^{}}{\{}12{\}}{\$} cm{\$}{\^{}}{\{}-3{\}}{\$}, irradiated by the SED with Opt/UV luminosity 100 times higher than the X-ray luminosity. When the cloud density is high enough, free-free heating dominates the entire absorber, and only one instability zone occurs, which is in agreement with observations.},
archivePrefix = {arXiv},
arxivId = {1812.05154},
author = {Adhikari, T. P. and R{\'{o}}{\.{z}}a{\'{n}}ska, A. and Hryniewicz, K. and Czerny, B. and Behar, E.},
eprint = {1812.05154},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Adhikari et al. - 2018 - What shapes the Absorption Measure Distribution in AGN outflows.pdf:pdf},
keywords = {absorption lines,active - methods,galaxies,numerical - radiative transfer},
pages = {1--11},
title = {{What shapes the Absorption Measure Distribution in AGN outflows}},
url = {http://arxiv.org/abs/1812.05154},
year = {2018}
}
@article{Bustard2016,
abstract = {We present a versatile family of model galactic outflows including non-uniform mass and energy source distributions, a gravitational potential from an extended mass source, and radiative losses. The model easily produces steady-state wind solutions for a range of mass-loading factors, energy-loading factors, galaxy mass and galaxy radius. We find that, with radiative losses included, highly mass-loaded winds must be driven at high central temperatures, whereas low mass-loaded winds can be driven at low temperatures just above the peak of the cooling curve, meaning radiative losses can drastically affect the wind solution even for low mass-loading factors. By including radiative losses, we are able to show that subsonic flows can be ignored as a possible mechanism for expelling mass and energy from a galaxy compared to the more efficient transonic solutions. Specifically, the transonic solutions with low mass-loading and high energy-loading are the most efficient. Our model also produces low-temperature, high-velocity winds that could explain the prevalence of low-temperature material in observed outflows. Finally, we show that our model, unlike the well-known Chevalier {\&} Clegg (1985) model, can reproduce the observed linear relationship between wind X-ray luminosity and star formation rate (SFR) over a large range of SFR from {\$}1-1000{\$} M{\$}{\_}{\{}\backslashodot{\}}{\$}/yr assuming the wind mass-loading factor is higher for low-mass, and hence, low-SFR galaxies. We also constrain the allowed mass-loading factors that can fit the observed X-ray luminosity vs. SFR trend, further suggesting an inverse relationship between mass-loading and SFR as explored in advanced numerical simulations.},
archivePrefix = {arXiv},
arxivId = {arXiv:1509.07130v2},
author = {Bustard, Chad and Zweibel, Ellen G. and D'Onghia, Elena},
doi = {10.3847/0004-637x/819/1/29},
eprint = {arXiv:1509.07130v2},
file = {:home/william/Documents/Papers/1509.07130.pdf:pdf},
issn = {1538-4357},
journal = {Astrophys. J.},
number = {1},
pages = {29},
title = {{a Versatile Family of Galactic Wind Models}},
volume = {819},
year = {2016}
}
@article{Zensus1997,
abstract = {Observations of parsec-scale radio jets associated with active galactic nuclei are reviewed, with a particular emphasis on high-luminosity core-dominated sources where the most detailed information on individual objects exists. Extensive imaging surveys with very long baseline interferometry (VLBI) have made possible a morphologic classification of compact radio sources and systematic studies of the statistics of apparent (often faster-than-light) motions found in an increasing number of sources. VLBI monitoring studies at centimeter and millimeter wavelengths, enhanced by spectral and polarization imaging, of representative types of AGN can discriminate detailed physical models. The observations are especially discussed in light of the variant of the relativistic beaming model that explains kinematic, spectral, and polarization properties of parsec-scale jets through shocks in an underlying continuous jet flow.},
author = {Zensus, J Anton},
doi = {10.1146/annurev.astro.35.1.607},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Zensus - 1997 - PARSEC-SCALE JETS IN EXTRAGALACTIC RADIO.pdf:pdf},
issn = {00664146},
journal = {Annu. Rev. Astron. Astrophys.},
keywords = {Compact radio sources,Jet models,Radio jets,Radio source morphology,Superluminal motion,VLBI jets},
number = {1},
pages = {607--636},
title = {{Parsec-scale jets in extragalactic radio sources}},
volume = {35},
year = {1997}
}
@article{Zhu2017,
abstract = {We implement and test the exact time integration method proposed by Townsend for gas cooling in cosmological hydrodynamic simulations. The errors using this time integrator for the internal energy are limited by the resolution of the cooling tables and are insensitive to the size of the time-step, improving accuracy relative to explicit or implicit schemes when the cooling time is short. We compare results with different time integrators for gas cooling in cosmological hydrodynamic simulations.We find that the temperature of the gas in filaments before accreting into dark matter haloes to form stars, obtained with the exact cooling integration, lies close to the equilibrium where radiative cooling balances heating from the ultraviolet background. For comparison, the gas temperature without the exact integrator shows substantial deviations from the equilibrium relation. Galaxy stellar masses with the exact cooling technique agree reasonably well, but are systematically lower than the results obtained by the other integration schemes, reducing the need for feedback to suppress star formation. Our implementation of the exact cooling technique is provided and can be easily incorporated into any hydrodynamic code.},
author = {Zhu, Qirong and Smith, Britton and Hernquist, Lars},
doi = {10.1093/mnras/stx1346},
file = {:home/william/Documents/Papers/stx1346.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: evolution,Galaxies: formation,Methods: numerical},
number = {1},
pages = {1017--1025},
title = {{Gas cooling in hydrodynamic simulations with an exact time integration scheme}},
volume = {470},
year = {2017}
}
@article{Federrath2012,
abstract = {We derive and compare six theoretical models for the star formation rate (SFR) - the Krumholz {\&} McKee (KM), Padoan {\&} Nordlund (PN), and Hennebelle {\&} Chabrier (HC) models, and three multi-freefall versions of these, suggested by HC - all based on integrals over the log-normal distribution of turbulent gas. We extend all theories to include magnetic fields, and show that the SFR depends on four basic parameters: (1) virial parameter alpha{\_}vir; (2) sonic Mach number M; (3) turbulent forcing parameter b, which is a measure for the fraction of energy driven in compressive modes; and (4) plasma beta=2(M{\_}A/M){\^{}}2 with the Alfven Mach number M{\_}A. We compare all six theories with MHD simulations, covering cloud masses of 300 to 4x10{\^{}}6 solar masses and Mach numbers M = 3 to 50 and M{\_}A = 1 to infinity, with solenoidal (b=1/3), mixed (b=0.4) and compressive turbulent (b=1) forcings. We find that the SFR increases by a factor of four between M=5 and 50 for compressive forcing and alpha{\_}vir{\~{}}1. Comparing forcing parameters, we see that the SFR is more than 10x higher with compressive than solenoidal forcing for Mach 10 simulations. The SFR and fragmentation are both reduced by a factor of two in strongly magnetized, trans-Alfvenic turbulence compared to hydrodynamic turbulence. All simulations are fit simultaneously by the multi-freefall KM and multi-freefall PN theories within a factor of two over two orders of magnitude in SFR. The simulated SFRs cover the range and correlation of SFR column density with gas column density observed in Galactic clouds, and agree well for star formation efficiencies SFE = 1{\%} to 10{\%} and local efficiencies epsilon = 0.3 to 0.7 due to feedback. We conclude that the SFR is primarily controlled by interstellar turbulence, with a secondary effect coming from magnetic fields.},
author = {Federrath, Christoph and Klessen, Ralf S.},
doi = {10.1088/0004-637X/761/2/156},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Federrath, Klessen - 2012 - The star formation rate of turbulent magnetized clouds Comparing theory, simulations, and observations.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {ISM: clouds,ISM: kinematics and dynamics,ISM: structure,magnetohydrodynamics (MHD),stars: formation,turbulence},
number = {2},
title = {{The star formation rate of turbulent magnetized clouds: Comparing theory, simulations, and observations}},
volume = {761},
year = {2012}
}
@article{Mukherjee2018c,
abstract = {The interstellar medium of the radio galaxy IC 5063 is highly perturbed by an AGN jet expanding in the gaseous disc of the galaxy. We model this interaction with rela-tivistic hydrodynamic simulations and multiphase initial conditions for the interstellar medium and compare the results with recent observations. As the jets flood through the inter-cloud channels of the disc, they ablate, accelerate, and disperse clouds to ve-locities exceeding 400 km s −1 . Clouds are also destroyed or displaced in bulk from the central regions of the galaxy. Our models with jet powers of 10 44 erg s −1 and 10 45 erg s −1 are capable of reproducing many of the features seen in the position-velocity diagram published in Morganti et al. (2015) and confirm the notion that the jet is responsible for the strongly perturbed gas dynamics seen in the ionized, neutral, and molecular gas phases. In our simulations, we also see strong venting of the jet plasma perpen-dicular to the disc, which entrains clumps and diffuse filaments into the halo of the galaxy. Our simulations are the first 3D hydrodynamic simulations of the jet and ISM of IC 5063.},
archivePrefix = {arXiv},
arxivId = {1801.06875},
author = {Mukherjee, Dipanjan and Wagner, Alexander Y. and Bicknell, Geoffrey V. and Morganti, Raffaella and Oosterloo, Tom and Nesvadba, Nicole and Sutherland, Ralph S.},
doi = {10.1093/mnras/sty067},
eprint = {1801.06875},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Mukherjee et al. - 2018 - The jet-ISM interactions in IC 5063.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: Jets,Hydrodynamics,Methods: numerical,galaxies: ISM},
number = {1},
pages = {80--95},
title = {{The jet-ISM interactions in IC 5063}},
volume = {476},
year = {2018}
}
@article{Chan2018,
abstract = {We present the first results of cosmic ray (CR) feedback implemented in the Feedback In Realistic Environments (FIRE) simulations. We investigate CR feedback in non-cosmological simulations of dwarf, sub-{\$}L\backslashstar{\$} starburst, and {\$}L\backslashstar{\$} galaxies with different propagation models, including advection, isotropic and anisotropic diffusion, and streaming along field lines with different transport coefficients. We simulate CR diffusion and streaming simultaneously in galaxies with high resolution, using a newly-developed two moment method. We forward-model and compare to observations of {\$}\backslashgamma{\$}-ray emission from nearby and starburst galaxies. We reproduce the {\$}\backslashgamma{\$}-ray observations with constant isotropic diffusion coefficients {\$}\backslashkappa \backslashsim 3\backslashtimes 10{\^{}}{\{}28-29{\}}\backslash,{\{}\backslashrm cm{\^{}}{\{}2{\}}\backslash,s{\^{}}{\{}-1{\}}{\}}{\$}. Advection-only and streaming-only models (even allowing for super-Alfvenic streaming speeds) produce order-of-magnitude too large {\$}\backslashgamma{\$}-ray luminosities in dwarf and {\$}L\backslashstar{\$} galaxies. We show that in models that match the {\$}\backslashgamma{\$}-ray observations, most CRs escape low-gas-density galaxies (e.g.$\backslash$ dwarfs) before significant collisional losses, while starburst galaxies are CR proton calorimeters. While adiabatic losses can be significant, they occur only after CRs escape galaxies, so they are only of secondary importance for {\$}\backslashgamma{\$}-ray emissivities. Models where CRs are "trapped" in the star-forming disk have lower star formation efficiency, but these models are ruled out by {\$}\backslashgamma{\$}-ray observations. For models with constant {\$}\backslashkappa{\$} that match the {\$}\backslashgamma{\$}-ray observations, CRs form extended halos with scale heights of several kpc to several tens of kpc.},
archivePrefix = {arXiv},
arxivId = {1812.10496},
author = {Chan, T. K. and Keres, D. and Hopkins, P. F. and Quataert, E. and Su, K. -Y. and Hayward, C. C. and Faucher-Giguere, C. -A.},
eprint = {1812.10496},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Chan et al. - 2018 - Cosmic ray feedback in the FIRE simulations constraining cosmic ray propagation with GeV gamma ray emission.pdf:pdf},
keywords = {evolution,galaxies,kinematics and dynamics},
number = {December},
title = {{Cosmic ray feedback in the FIRE simulations: constraining cosmic ray propagation with GeV gamma ray emission}},
url = {http://arxiv.org/abs/1812.10496},
volume = {000},
year = {2018}
}
@article{Event2021,
abstract = {Event Horizon Telescope (EHT) observations at 230 GHz have now imaged polarized emission around the supermassive black hole in M87 on event-horizon scales. This polarized synchrotron radiation probes the structure of magnetic fields and the plasma properties near the black hole. Here we compare the resolved polarization structure observed by the EHT, along with simultaneous unresolved observations with the Atacama Large Millimeter/submillimeter Array, to expectations from theoretical models. The low fractional linear polarization in the resolved image suggests that the polarization is scrambled on scales smaller than the EHT beam, which we attribute to Faraday rotation internal to the emission region. We estimate the average density n e ∼ 10 4–7 cm −3 , magnetic field strength B ∼ 1–30 G, and electron temperature T e ∼ (1–12) × 10 10 K of the radiating plasma in a simple one-zone emission model. We show that the net azimuthal linear polarization pattern may result from organized, poloidal magnetic fields in the emission region. In a quantitative comparison with a large library of simulated polarimetric images from general relativistic magnetohydrodynamic (GRMHD) simulations, we identify a subset of physical models that can explain critical features of the polarimetric EHT observations while producing a relativistic jet of sufficient power. The consistent GRMHD models are all of magnetically arrested accretion disks, where near-horizon magnetic fields are dynamically important. We use the models to infer a mass accretion rate onto the black hole in M87 of (3–20) × 10 −4 M ⊙ yr −1 .},
author = {Akiyama, Kazunori and Algaba, Juan Carlos and Alberdi, Antxon and Alef, Walter and Anantua, Richard and Asada, Keiichi and Azulay, Rebecca and Baczko, Anne-Kathrin and Ball, David and Balokovi{\'{c}}, Mislav and Barrett, John and Benson, Bradford A. and Bintley, Dan and Blackburn, Lindy and Blundell, Raymond and Boland, Wilfred and Bouman, Katherine L. and Bower, Geoffrey C. and Boyce, Hope and Bremer, Michael and Brinkerink, Christiaan D. and Brissenden, Roger and Britzen, Silke and Broderick, Avery E. and Broguiere, Dominique and Bronzwaer, Thomas and Byun, Do-Young and Carlstrom, John E. and Chael, Andrew and Chan, Chi-kwan and Chatterjee, Shami and Chatterjee, Koushik and Chen, Ming-Tang and Chen, Yongjun and Chesler, Paul M. and Cho, Ilje and Christian, Pierre and Conway, John E. and Cordes, James M. and Crawford, Thomas M. and Crew, Geoffrey B. and Cruz-Osorio, Alejandro and Cui, Yuzhu and Davelaar, Jordy and {De Laurentis}, Mariafelicia and Deane, Roger and Dempsey, Jessica and Desvignes, Gregory and Dexter, Jason and Doeleman, Sheperd S. and Eatough, Ralph P. and Falcke, Heino and Farah, Joseph and Fish, Vincent L. and Fomalont, Ed and Ford, H. Alyson and Fraga-Encinas, Raquel and Friberg, Per and Fromm, Christian M. and Fuentes, Antonio and Galison, Peter and Gammie, Charles F. and Garc{\'{i}}a, Roberto and Gelles, Zachary and Gentaz, Olivier and Georgiev, Boris and Goddi, Ciriaco and Gold, Roman and G{\'{o}}mez, Jos{\'{e}} L. and G{\'{o}}mez-Ruiz, Arturo I. and Gu, Minfeng and Gurwell, Mark and Hada, Kazuhiro and Haggard, Daryl and Hecht, Michael H. and Hesper, Ronald and Himwich, Elizabeth and Ho, Luis C. and Ho, Paul and Honma, Mareki and Huang, Chih-Wei L. and Huang, Lei and Hughes, David H. and Ikeda, Shiro and Inoue, Makoto and Issaoun, Sara and James, David J. and Jannuzi, Buell T. and Janssen, Michael and Jeter, Britton and Jiang, Wu and Jimenez-Rosales, Alejandra and Johnson, Michael D. and Jorstad, Svetlana and Jung, Taehyun and Karami, Mansour and Karuppusamy, Ramesh and Kawashima, Tomohisa and Keating, Garrett K. and Kettenis, Mark and Kim, Dong-Jin and Kim, Jae-Young and Kim, Jongsoo and Kim, Junhan and Kino, Motoki and Koay, Jun Yi and Kofuji, Yutaro and Koch, Patrick M. and Koyama, Shoko and Kramer, Michael and Kramer, Carsten and Krichbaum, Thomas P. and Kuo, Cheng-Yu and Lauer, Tod R. and Lee, Sang-Sung and Levis, Aviad and Li, Yan-Rong and Li, Zhiyuan and Lindqvist, Michael and Lico, Rocco and Lindahl, Greg and Liu, Jun and Liu, Kuo and Liuzzo, Elisabetta and Lo, Wen-Ping and Lobanov, Andrei P. and Loinard, Laurent and Lonsdale, Colin and Lu, Ru-Sen and MacDonald, Nicholas R. and Mao, Jirong and Marchili, Nicola and Markoff, Sera and Marrone, Daniel P. and Marscher, Alan P. and Mart{\'{i}}-Vidal, Iv{\'{a}}n and Matsushita, Satoki and Matthews, Lynn D. and Medeiros, Lia and Menten, Karl M. and Mizuno, Izumi and Mizuno, Yosuke and Moran, James M. and Moriyama, Kotaro and Moscibrodzka, Monika and M{\"{u}}ller, Cornelia and Musoke, Gibwa and Mej{\'{i}}as, Alejandro Mus and Michalik, Daniel and Nadolski, Andrew and Nagai, Hiroshi and Nagar, Neil M. and Nakamura, Masanori and Narayan, Ramesh and Narayanan, Gopal and Natarajan, Iniyan and Nathanail, Antonios and Neilsen, Joey and Neri, Roberto and Ni, Chunchong and Noutsos, Aristeidis and Nowak, Michael A. and Okino, Hiroki and Olivares, H{\'{e}}ctor and Ortiz-Le{\'{o}}n, Gisela N. and Oyama, Tomoaki and {\"{O}}zel, Feryal and Palumbo, Daniel C. M. and Park, Jongho and Patel, Nimesh and Pen, Ue-Li and Pesce, Dominic W. and Pi{\'{e}}tu, Vincent and Plambeck, Richard and PopStefanija, Aleksandar and Porth, Oliver and P{\"{o}}tzl, Felix M. and Prather, Ben and Preciado-L{\'{o}}pez, Jorge A. and Psaltis, Dimitrios and Pu, Hung-Yi and Ramakrishnan, Venkatessh and Rao, Ramprasad and Rawlings, Mark G. and Raymond, Alexander W. and Rezzolla, Luciano and Ricarte, Angelo and Ripperda, Bart and Roelofs, Freek and Rogers, Alan and Ros, Eduardo and Rose, Mel and Roshanineshat, Arash and Rottmann, Helge and Roy, Alan L. and Ruszczyk, Chet and Rygl, Kazi L. J. and S{\'{a}}nchez, Salvador and S{\'{a}}nchez-Arguelles, David and Sasada, Mahito and Savolainen, Tuomas and Schloerb, F. Peter and Schuster, Karl-Friedrich and Shao, Lijing and Shen, Zhiqiang and Small, Des and Sohn, Bong Won and SooHoo, Jason and Sun, He and Tazaki, Fumie and Tetarenko, Alexandra J. and Tiede, Paul and Tilanus, Remo P. J. and Titus, Michael and Toma, Kenji and Torne, Pablo and Trent, Tyler and Traianou, Efthalia and Trippe, Sascha and van Bemmel, Ilse and van Langevelde, Huib Jan and van Rossum, Daniel R. and Wagner, Jan and Ward-Thompson, Derek and Wardle, John and Weintroub, Jonathan and Wex, Norbert and Wharton, Robert and Wielgus, Maciek and Wong, George N. and Wu, Qingwen and Yoon, Doosoo and Young, Andr{\'{e}} and Young, Ken and Younsi, Ziri and Yuan, Feng and Yuan, Ye-Fei and Zensus, J. Anton and Zhao, Guang-Yao and Zhao, Shan-Shan},
doi = {10.3847/2041-8213/abe4de},
file = {:home/william/Documents/Papers/Akiyama{\_}2021{\_}ApJL{\_}910{\_}L13.pdf:pdf},
issn = {2041-8205},
journal = {Astrophys. J. Lett.},
number = {1},
pages = {L13},
title = {{First M87 Event Horizon Telescope Results. VIII. Magnetic Field Structure near The Event Horizon}},
volume = {910},
year = {2021}
}
@article{Wasiewicz2011,
author = {Wasiewicz, P. and Hryniewicz, K. and Gajewski, P.},
doi = {10.1117/12.905591},
file = {:home/william/Documents/Papers/sqlquasars.pdf:pdf},
isbn = {9780819485823},
issn = {0277786X},
journal = {Photonics Appl. Astron. Commun. Ind. High-Energy Phys. Exp. 2011},
number = {June 2011},
pages = {80080W},
title = {{Astronomical spectral database of active galactic nuclei}},
volume = {8008},
year = {2011}
}
@article{Yusef-Zadeh2019,
abstract = {Radio, X-ray, and infrared observations of the inner few hundred parsecs of the Galactic Centre have highlighted two characteristics of the interstellar medium. The cosmic-ray ionization rate derived from molecular ions such as H{\$}-3{\$} is at least two to three orders of magnitude higher than in the Galactic disc. The other is bipolar X-ray and radio emission away from the Galactic plane. These features are consistent with a scenario in which high cosmic-ray pressure drives large-scale winds away from the Galactic plane. The interaction of such a wind with stellar wind bubbles may explain the energetic non-thermal radio filaments found throughout the Galactic Centre. Some of the implications of this scenario is the removal of gas driven by outflowing winds, acting as a feedback to reduce the star formation rate in the central molecular zone (CMZ), and the distortion of azimuthal magnetic field lines in the CMZ to vertical direction away from the plane. The combined effects of the wind and the vertical magnetic field can explain why most magnetized filaments run perpendicular to the galactic plane. This proposed picture suggests our Milky Way nucleus has recently experienced starburst or black hole activity, as recent radio and X-ray observations indicate.},
archivePrefix = {arXiv},
arxivId = {1909.07409},
author = {Yusef-Zadeh, F. and Wardle, M.},
doi = {10.1093/mnrasl/slz134},
eprint = {1909.07409},
file = {:home/william/Documents/Papers/slz134.pdf:pdf},
issn = {17453933},
journal = {Mon. Not. R. Astron. Soc. Lett.},
keywords = {Galaxy: Centre,accretion,accretion discs,black hole physics},
number = {1},
pages = {L1--L5},
publisher = {Oxford University Press},
title = {{Cosmic-ray-driven outflow from the Galactic Centre and the origin of magnetized radio filaments}},
volume = {490},
year = {2019}
}
@article{Cazzoli2017,
abstract = {The starburst-AGN coexistence in local (U)LIRGs makes these galaxies excellent laboratories for the study of stellar and AGN outflows and feedback. Outflows regulate star formation and AGN activity, redistributing gas, dust and metals over large scales in the interstellar and intergalactic media (negative feedback) being also considered to be able to undergo vigorous star formation (positive feedback). In this contribution, I will summarize the results from a search for outflows in a sample of nearby 38 local (U)LIRG systems observed with VIMOS/VLT integral field unit. For two galaxies of the sample I will detail the outflow properties and discuss the observational evidence for negative and positive outflow-feedback. The assessment of both negative and positive feedback effects represent a novel approach toward a comprehensive understanding of the impact of outflow feedback in the galaxy evolution.},
author = {Cazzoli, Sara},
doi = {10.3389/fspas.2017.00062},
file = {:home/william/Documents/Papers/fspas-04-00062.pdf:pdf},
issn = {2296987X},
journal = {Front. Astron. Sp. Sci.},
keywords = {ISM: jets and outflows,ISM: kinematics and dynamics,evolution,feedback,galaxies: starburst,techniques: spectroscopic},
number = {December},
pages = {1--5},
title = {{Negative and Positive Outflow-Feedback in Nearby (U)LIRGs}},
volume = {4},
year = {2017}
}
@article{Pino2020,
author = {Pino, De Gouveia Dal},
file = {:home/william/Documents/Papers/[Dal Pino]-SF-GALXIES.pdf:pdf},
title = {{SB galaxies CTA Bete review}},
volume = {d},
year = {2020}
}
@article{Riffel2020,
abstract = {The role of feedback from active galactic nuclei (AGNs) in the evolution of galaxies is still not fully understood, mostly due to the lack of observational constraints in the multiphase gas kinematics on the 10-100 pc scales. We have used the Gemini Near-Infrared Integral Field Spectrograph (NIFS) to map the molecular and ionized gas kinematics in the inner 900 × 900 pc2 of the Seyfert galaxy NGC 1275 at a spatial resolution of ∼70 pc. From the fitting of the CO absorption bandheads in the K band, we derive a stellar velocity dispersion of 265 ± 26 kms-1, which implies a black hole mass of MSMBH = 1.1+-0..5 × 109 M},
archivePrefix = {arXiv},
arxivId = {2006.15198},
author = {Riffel, Rogemar A. and Storchi-Bergmann, Thaisa and Zakamska, Nadia L. and Riffel, Rog{\'{e}}rio},
doi = {10.1093/mnras/staa1922},
eprint = {2006.15198},
file = {:home/william/Documents/Papers/staa1922.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: active,Galaxies: individual (NGC 1275),Galaxies: kinematics and dynamics},
number = {4},
pages = {4857--4873},
title = {{Ionized and hot molecular outflows in the inner 500 pc of NGC1275}},
volume = {496},
year = {2020}
}
@misc{Pellegrini2018,
abstract = {A recent determination of the relationships between the X-ray luminosity of the ISM (LX) and the stellar and total mass, for a sample of nearby early-type galaxies (ETGs), is used to investigate the origin of the hot gas, via a comparison with the results of hydrodynamical simulations of the ISM evolution for a large set of isolated ETGs. After the epoch of major galaxy formation (after z ' 2), the ISM is replenished by stellar mass losses and SN ejecta, at the rate predicted by stellar evolution, and is depleted by star formation; it is heated by the thermalization of stellar motions, SNe explosions and the mechanical (from winds) and radiative AGN feedback. The models agree well with the observed relations, even for the largely different LX values at the same mass, thanks to the sensitivity of the gas flow to many galaxy properties; this holds for models including AGN feedback, and those without. Therefore, the mass input from the stellar population is able to account for a major part of the observed LX; and AGN feedback, while very important to maintain massive ETGs in a time-averaged quasi-steady state, keeping low star formation and the black hole mass, does not dramatically alter the gas content originating in stellar recycled material. These conclusions are based on theoretical predictions for the stellar population contributions in mass and energy, and on a self-consistent modeling of AGN feedback.},
archivePrefix = {arXiv},
arxivId = {1802.02005},
author = {Pellegrini, Silvia and Ciotti, Luca and Negri, Andrea and Ostriker, Jeremiah P.},
booktitle = {arXiv},
doi = {10.3847/1538-4357/aaae07},
eprint = {1802.02005},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Negri - 2018 - Agn feedback and the origin and fate of the hot gas in early-type galaxies.pdf:pdf},
issn = {23318422},
keywords = {CD,Galaxies: elliptical and lenticular,Galaxies: evolution,Galaxies: kinematics and dynamics,Quasars: supermassive black holes,X-rays: ISM,X-rays: galaxies},
title = {{AGN feedback and the origin and fate of the hot gas in early-type galaxies}},
year = {2018}
}
@article{Maiolino2017,
abstract = {Recent observations have revealed massive galactic molecular outflows that may have the physical conditions (high gas densities) required to form stars. Indeed, several recent models predict that such massive outflows may ignite star formation within the outflow itself. This star-formation mode, in which stars form with high radial velocities, could contribute to the morphological evolution of galaxies, to the evolution in size and velocity dispersion of the spheroidal component of galaxies, and would contribute to the population of high-velocity stars, which could even escape the galaxy. Such star formation could provide in situ chemical enrichment of the circumgalactic and intergalactic medium (through supernova explosions of young stars on large orbits), and some models also predict it to contribute substantially to the star-formation rate observed in distant galaxies. Although there exists observational evidence for star formation triggered by outflows or jets into their host galaxy, as a consequence of gas compression, evidence for star formation occurring within galactic outflows is still missing. Here we report spectroscopic observations that unambiguously reveal star formation occurring in a galactic outflow at a redshift of 0.0448. The inferred star-formation rate in the outflow is larger than 15 solar masses per year. Star formation may also be occurring in other galactic outflows, but may have been missed by previous observations owing to the lack of adequate diagnostics.},
archivePrefix = {arXiv},
arxivId = {1703.08587},
author = {Maiolino, R. and Russell, H. R. and Fabian, A. C. and Carniani, S. and Gallagher, R. and Cazzoli, S. and Arribas, S. and Belfiore, F. and Bellocchi, E. and Colina, L. and Cresci, G. and Ishibashi, W. and Marconi, A. and Mannucci, F. and Oliva, E. and Sturm, E.},
doi = {10.1038/nature21677},
eprint = {1703.08587},
file = {:home/william/Documents/Papers/maiolino2017.pdf:pdf},
issn = {14764687},
journal = {Nature},
number = {7649},
pages = {202--206},
publisher = {Nature Publishing Group},
title = {{Star formation inside a galactic outflow}},
url = {http://dx.doi.org/10.1038/natur21677},
volume = {544},
year = {2017}
}
@article{Netzer2018,
abstract = {The topics covered in this summary review reflect the major areas discussed in the Padova meeting, in April 2017. They are divided into general categories: those areas where large progress has been made leading to a real new understanding (what we are doing “right”), and those where we are still in the dark (what we are doing “wrong”). The division reflects the status of the field as well as my subjective opinion.},
author = {Netzer, Hagai},
doi = {10.3389/fspas.2018.00010},
file = {:home/william/Documents/Papers/fspas-05-00010.pdf:pdf},
issn = {2296987X},
journal = {Front. Astron. Sp. Sci.},
keywords = {AGN-feedback,accretion disks,black holes,cosmology,host galaxies,reverberation mapping,star formation},
number = {May},
pages = {1--5},
title = {{Meeting Summary: A 2017 View of Active Galactic Nuclei}},
volume = {5},
year = {2018}
}
@article{Frazer2019,
abstract = {Numerical models of gas inflow towards a supermassive black hole (SMBH) show that star formation may occur in such an environment through the growth of a gravitationally unstable gas disc. We consider the effect of nuclear activity on such a scenario. We present the first three-dimensional grid-based radiative hydrodynamic simulations of direct collisions between infalling gas streams and a 4 × 106 M☉ SMBH, using ray-tracing to incorporate radiation consistent with an active galactic nucleus (AGN). We assume inflow masses of ≈105 M☉ and explore radiation fields of 10 per cent and 100 per cent of the Eddington luminosity (Ledd). We follow our models to the point of central gas disc formation preceding star formation and use the Toomre Q parameter (QT) to test for gravitational instability. We find that radiation pressure from UV photons inhibits inflow. Yet, for weak radiation fields, a central disc forms on time-scales similar to that of models without feedback. Average densities of {\textgreater}108 cm−3 limit photoheating to the disc surface allowing for QT ≈ 1. For strong radiation fields, the disc forms more gradually resulting in lower surface densities and larger QT values. Mass accretion rates in our models are consistent with 1-60 per cent of the Eddington limit, thus we conclude that it is unlikely that radiative feedback from AGN activity would inhibit circumnuclear star formation arising from a massive inflow event.},
archivePrefix = {arXiv},
arxivId = {1907.11534},
author = {Frazer, Christopher C. and Heitsch, Fabian},
doi = {10.1093/mnras/stz2083},
eprint = {1907.11534},
file = {:home/william/Documents/Papers/stz2083.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxy: centre,Hydrodynamics,Radiative transfer,Stars: formation},
number = {1},
pages = {52--77},
publisher = {Oxford University Press},
title = {{Gas inflow and star formation near supermassive black holes: The role of nuclear activity}},
volume = {489},
year = {2019}
}
@article{Nawaz2014,
abstract = {We present the first stage of an investigation of the interactions of the jets in the radio galaxy Hydra A with the intracluster medium. We consider the jet kinetic power, the galaxy and cluster atmosphere and the inner structure of the radio source. Analysing radio observations of the inner lobes of Hydra A by Taylor et al. we confirm the jet power estimates ˜1045 erg s-1 derived by Wise et al. from dynamical analysis of the X-ray cavities. With this result and a model for the galaxy halo, we explore the jet-intracluster medium interactions occurring on a scale of 10 kpc using two-dimensional, axisymmetric, relativistic pure hydrodynamic simulations. A key feature is that we identify the three bright knots in the northern jet as biconical reconfinement shocks, which result when an overpressured jet starts to come into equilibrium with the galactic atmosphere. Through an extensive parameter space study we deduce that the jet velocity is approximately 0.8c at a distance 0.5 kpc from the black hole. The combined constraints of jet power, the observed jet radius profile along the jet and the estimated jet pressure and jet velocity imply a value of the jet density parameter chi ≈ 13 for the northern jet. We show that for a jet beta = 0.8 and theta = 42$\backslash$,{\^{}}{\{}$\backslash$circ{\}}, an intrinsic asymmetry in the emissivity of the northern and southern jet is required for a consistent brightness ratio ≈7 estimated from the 6-cm Very Large Array image of Hydra A.},
archivePrefix = {arXiv},
arxivId = {arXiv:1408.4512v1},
author = {Nawaz, M. A. and Wagner, A. Y. and Bicknell, G. V. and Sutherland, R. S. and McNamara, B. R.},
doi = {10.1093/mnras/stu1563},
eprint = {arXiv:1408.4512v1},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Nawaz et al. - 2014 - Jet-intracluster medium interaction in Hydra A - I. Estimates of jet velocity from inner knots.pdf:pdf},
isbn = {doi:10.1093/mnras/stu1563},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: Active,Galaxies: Clusters: Intracluster medium,Galaxies: Jets},
number = {2},
pages = {1600--1614},
title = {{Jet-intracluster medium interaction in Hydra A - I. Estimates of jet velocity from inner knots}},
volume = {444},
year = {2014}
}
@article{Imanishi2018,
abstract = {We present the results of our ALMA observations of eleven (ultra)luminous infrared galaxies ((U)LIRGs) at J=4-3 of HCN, HCO+, HNC and J=3-2 of HNC. This is an extension of our previously published HCN and HCO+ J=3-2 observations to multiple rotational J-transitions of multiple molecules, to investigate how molecular emission line flux ratios vary at different J-transitions. We confirm that ULIRGs that contain or may contain luminous obscured AGNs tend to show higher HCN-to-HCO+ flux ratios than starburst galaxies, both at J=4-3 and J=3-2. For selected HCN-flux-enhanced AGN-important ULIRGs, our isotopologue H13CN, H13CO+, and HN13C J=3-2 line observations suggest a higher abundance of HCN than HCO+ and HNC, which is interpreted to be primarily responsible for the elevated HCN flux in AGN-important galaxies. For such sources, the intrinsic HCN-to-HCO+ flux ratios after line opacity correction will be higher than the observed ratios, making the separation between AGNs and starbursts even larger. The signature of the vibrationally excited (v2=1f) HCN J=4-3 emission line is seen in one ULIRG, IRAS 12112-0305 NE. P Cygni profiles are detected in the HCO+ J=4-3 and J=3-2 lines toward IRAS 15250+3609, with an estimated molecular outflow rate of {\~{}}250-750 Mo/year. The SiO J=6-5 line also exhibits a P Cygni profile in IRAS 12112+0305 NE, suggesting the presence of shocked outflow activity. Shock tracers are detected in many sources, suggesting ubiquitous shock activity in the nearby ULIRG population.},
archivePrefix = {arXiv},
arxivId = {1803.02408},
author = {Imanishi, Masatoshi and Nakanishi, Kouichiro and Izumi, Takuma},
doi = {10.3847/1538-4357/aab42f},
eprint = {1803.02408},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Imanishi, Nakanishi, Izumi - 2018 - ALMA Multiple-Transition Observations of High Density Molecular Tracers in Ultraluminous Infrared Ga.pdf:pdf},
issn = {1538-4357},
number = {1},
title = {{ALMA Multiple-Transition Observations of High Density Molecular Tracers in Ultraluminous Infrared Galaxies}},
url = {http://arxiv.org/abs/1803.02408},
year = {2018}
}
@article{Bing2019,
abstract = {Negative feedback from accretion on to supermassive black holes (SMBHs), that is to remove gas and suppress star formation in galaxies, has been widely suggested. However, for Seyfert galaxies which harbour less active, moderately accreting SMBHs in the local Universe, the feedback capability of their black hole activity is elusive. We present spatially resolved H $\alpha$ measurements to trace ongoing star formation in Seyfert galaxies and compare their specific star formation rate with a sample of star-forming galaxies whose global galaxy properties are controlled to be the same as the Seyferts. From the comparison, we find that the star formation rates within central kpc of Seyfert galaxies are mildly suppressed as compared to the matched normal star-forming galaxies. This suggests that the feedback of moderate SMBH accretion could, to some extent, regulate the ongoing star formation in these intermediate to late type galaxies under secular evolution.},
archivePrefix = {arXiv},
arxivId = {1810.00365},
author = {Bing, Longji and Shi, Yong and Chen, Yanmei and S{\'{a}}nchez, Sebasti{\'{a}}n F. and Maiolino, Roberto and Riffel, Rog{\'{e}}rio and Riffel, Rogemar A. and Wylezalek, Dominika and Bizyaev, Dmitry and Pan, Kaike and Drory, Niv},
doi = {10.1093/mnras/sty2662},
eprint = {1810.00365},
file = {:home/william/Documents/Papers/001089990.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: Seyfert,Galaxies: active,Galaxies: evolution,Galaxies: star formation},
number = {1},
pages = {194--205},
title = {{Mildly suppressed star formation in central regions of MaNGA Seyfert galaxies}},
volume = {482},
year = {2019}
}
@article{Riffel2009a,
abstract = {We analyse two-dimensional near-infrared K-band spectra from the inner 660 × 315pc{\textless}SUP{\textgreater}2{\textless}/SUP{\textgreater} of the Seyfert galaxy NGC7582 obtained with the Gemini near-infrared spectrograph integral field unit at a spatial resolution of {\~{}}50pc and spectral resolving power R {\~{}} 5900. The nucleus harbours an unresolved source well reproduced by a blackbody of temperature T {\~{}} 1050K, which we attribute to emission by circumnuclear dust located closer than 25pc from the nucleus, with a total mass of {\~{}}3 ×10{\textless}SUP{\textgreater}-3{\textless}/SUP{\textgreater}M{\textless}SUB{\textgreater}solar{\textless}/SUB{\textgreater}. Surrounding the nucleus, we observe a ring of active star formation, apparently in the Galactic plane, with a radius of {\~{}}190pc, an age of {\~{}}5Myr and a total mass of ionized gas of {\~{}}3 × 10{\textless}SUP{\textgreater}6{\textless}/SUP{\textgreater}M{\textless}SUB{\textgreater}solar{\textless}/SUB{\textgreater}. The radiation of the young stars in the ring accounts for at least 80 per cent of the ionization observed in the Brgamma emitting gas, the remaining being due to the radiation emitted by the active nucleus. The stellar kinematics was derived using the CO absorption band at 2.29mum and reveals: (i) a distorted rotation pattern in the radial velocity field with kinematic centre apparently displaced from the nuclear source by a few tens of parsec; (ii) a high-velocity dispersion in the bulge of sigma{\textless}SUB{\textgreater}*{\textless}/SUB{\textgreater} = 170kms{\textless}SUP{\textgreater}-1{\textless}/SUP{\textgreater} and (iii) a partial ring of sigma{\textless}SUB{\textgreater}*{\textless}/SUB{\textgreater} = 50kms{\textless}SUP{\textgreater}-1{\textless}/SUP{\textgreater}, located close to the Brgamma emitting ring, but displaced by {\~{}}50pc towards the nucleus, interpreted as due to stars formed from cold gas in a previous burst of star formation. The kinematics of the ionized gas shows a similar rotation pattern to that of the stars, plus a blueshifted component with velocities {\textgreater}=100kms{\textless}SUP{\textgreater}-1{\textless}/SUP{\textgreater} interpreted as due to an outflow along the ionization cone, which was partially covered by our observations. The mass outflow rate in the ionized gas was estimated as , which is one order of magnitude larger than the accretion rate to the active galactic nuclei (AGN), indicating that the outflowing gas does not originate in the AGN, but is instead the circumnuclear gas from the host galaxy being pushed away by a nuclear outflow. The flux distribution and kinematics of the hot molecular gas, traced by the H{\textless}SUB{\textgreater}2{\textless}/SUB{\textgreater}lambda2.22mum emission line, suggest most of this gas is in the Galactic plane. An excess blueshift along PA {\~{}} -70°, where a nuclear bar has been observed, can be interpreted as an inflow towards the nucleus. We thus conclude that the H{\textless}SUB{\textgreater}2{\textless}/SUB{\textgreater} kinematics traces the feeding of the AGN, while the ionized gas kinematics traces its feedback via the outflows. An AGN-starburst connection in the nucleus of NGC7582 is supported by the ratio between the mass accretion rate and the star formation rate in the circumnuclear region of {\~{}}0.26 per cent, which is close to the expected relation between the mass of the supermassive black holes and that of the host galaxy bulge in galaxies (the Magorrian relation).},
author = {Riffel, Rogemar A. and Storchi-Bergmann, Thaisa and Dors, Oli L. and Winge, Cl{\'{a}}udia},
doi = {10.1111/j.1365-2966.2008.14250.x},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Riffel et al. - 2009 - AGN-starburst connection in NGC 7582 Gemini near-infrared spectrograph integral field unit observations.pdf:pdf},
issn = {00358711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: Seyfert,Galaxies: individual: NGC 7582,Galaxies: kinematics and dynamics,Galaxies: starburst,Infrared: galaxies},
number = {3},
pages = {783--797},
title = {{AGN-starburst connection in NGC 7582: Gemini near-infrared spectrograph integral field unit observations}},
volume = {393},
year = {2009}
}
@article{Piran2005,
abstract = {Gamma-ray bursts ͑GRB's͒, short and intense pulses of low-energy ␥ rays, have fascinated astronomers and astrophysicists since their unexpected discovery in the late sixties. During the last decade, several space missions—BATSE ͑Burst and Transient Source Experiment͒ on the Compton Gamma-Ray Observatory, BeppoSAX and now HETE II ͑High-Energy Transient Explorer͒— together with ground-based optical, infrared, and radio observatories have revolutionized our understanding of GRB's, showing that they are cosmological, that they are accompanied by long-lasting afterglows, and that they are associated with core-collapse supernovae. At the same time a theoretical understanding has emerged in the form of the fireball internal-external shocks model. According to this model GRB's are produced when the kinetic energy of an ultrarelativistic flow is dissipated in internal collisions. The afterglow arises when the flow is slowed down by shocks with the surrounding circumburst matter. This model has had numerous successful predictions, like the predictions of the afterglow itself, of jet breaks in the afterglow light curve, and of the optical flash that accompanies the GRB's. This review focuses on the current theoretical understanding of the physical processes believed to take place in GRB's.},
author = {Piran, Tsvi},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Piran - 2005 - The Physics of Gamma-Ray Bursts.pdf:pdf},
number = {OCTOBER 2004},
title = {{The Physics of Gamma-Ray Bursts}},
volume = {76},
year = {2005}
}
@article{1996ApJ...462..563N,
author = {Navarro, J.{\~{}}F. and Frenk, C.{\~{}}S. and White, S.{\~{}}D.{\~{}}M.},
doi = {10.1086/177173},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Navarro, Frenk, White - 1996 - The Structure of Cold Dark Matter Halos.pdf:pdf},
journal = {Apj},
keywords = {COSMOLOGY: DARK MATTER,COSMOLOGY: THEORY,GALAXIES: HALOS,METHODS: NUMERICAL},
pages = {563},
title = {{The Structure of Cold Dark Matter Halos}},
volume = {462},
year = {1996}
}
@article{Parker1963,
abstract = {Kinematical hydromagnetic theory applications to low solar photosphere},
author = {Parker, E.N.},
doi = {10.1086/147663},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Parker - 1963 - Kinematical Hydromagnetic Theory and its Application to the Low Solar Photosphere.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
pages = {552},
title = {{Kinematical Hydromagnetic Theory and its Application to the Low Solar Photosphere.}},
url = {http://adsabs.harvard.edu/doi/10.1086/147663{\%}5Cnhttp://adsabs.harvard.edu/full/1963ApJ...138..552P},
volume = {138},
year = {1963}
}
@article{LaRosa2004,
author = {LaRosa, T. N. and Nord, Michael E. and Joseph, T. and Lazio, W. and Kassim, Namir E.},
doi = {10.1086/383233},
file = {:home/william/Documents/Papers/LaRosa{\_}2004{\_}ApJ{\_}607{\_}302.pdf:pdf;:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/LaRosa et al. - 2004 - New Nonthermal Filaments at the Galactic Center Are They Tracing a Globally Ordered Magnetic Field.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
number = {1},
pages = {302--308},
title = {{New Nonthermal Filaments at the Galactic Center: Are They Tracing a Globally Ordered Magnetic Field?}},
volume = {607},
year = {2004}
}
@article{Turner1998,
author = {Turner, T. J. and George, I. M. and Nandra, K. and Mushotzky, R. F.},
doi = {10.1086/305117},
file = {:home/william/Documents/Papers/9708231.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
number = {1},
pages = {91--101},
title = {{ ASCA Observations of Type 2 Seyfert Galaxies. III. Orientation and X‐Ray Absorption }},
volume = {493},
year = {1998}
}
@article{Townsend2009,
abstract = {A new scheme for incorporating radiative cooling in hydrodynamical codes is presented, centered around exact integration of the governing semidiscrete cooling equation. Using benchmark calculations based on the cooling downstream of a radiative shock, I demonstrate that the new scheme outperforms traditional explicit and implicit approaches in terms of accuracy, while remaining competitive in terms of execution speed. {\textcopyright} 2009. The American Astronomical Society. All rights reserved.},
archivePrefix = {arXiv},
arxivId = {0901.3146},
author = {Townsend, R. H.D.},
doi = {10.1088/0067-0049/181/2/391},
eprint = {0901.3146},
file = {:home/william/Documents/Papers/Townsend{\_}2009{\_}ApJS{\_}181{\_}391.pdf:pdf},
issn = {00670049},
journal = {Astrophys. Journal, Suppl. Ser. Ser.},
keywords = {Hydrodynamics,Methods: Numerical,Radiation mechanisms: Thermal,Shock waves},
number = {2},
pages = {391--397},
title = {{An exact integration scheme for radiative cooling in hydrodynamical simulations}},
volume = {181},
year = {2009}
}
@article{Raga2000,
archivePrefix = {arXiv},
arxivId = {1011.1669},
author = {Raga, A.{\~{}}C.},
doi = {10.1088/1751-8113/44/8/085201},
eprint = {1011.1669},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Raga - 2000 - A new, 3D adaptative grid code for astrophysical and geophysical gasdynamics.pdf:pdf},
isbn = {9781935117643},
issn = {1751-8113},
journal = {Rev. Mex. Astron. y Astrof{\'{i}}sica},
month = {feb},
pages = {6776},
pmid = {29982528},
title = {{A new, 3D adaptative grid code for astrophysical and geophysical gasdynamics}},
url = {http://arxiv.org/abs/1011.1669 http://dx.doi.org/10.1088/1751-8113/44/8/085201 http://stacks.iop.org/1751-8121/44/i=8/a=085201?key=crossref.abc74c979a75846b3de48a5587bf708f},
volume = {36},
year = {2000}
}
@article{Corey1987a,
abstract = {Weinstein S, Ponseti IV: Congenital dislocation of the hip. 1979; 61:119},
author = {Corey, E. J. and Su, Wei-guo},
file = {:home/william/Documents/Papers/1987MNRAS.228..973T.pdf:pdf},
journal = {Tetrahedron Lett.},
number = {44},
pages = {5241--5244},
title = {{No 主観的健康感を中心とした在宅高齢者における 健康関連指標に関する共分散構造分析Title}},
volume = {28},
year = {1987}
}
@article{Coppola2011,
abstract = {Cooling of primordial gas plays a crucial role in the birth of the first structures in our Universe. Due to the low fractional abundance of molecular species at high redshifts, spontaneous emission rather than collisions represents the most efficient way to cool the pristine plasma. In the present work, radiative cooling functions are evaluated for the diatomic species HD, HD+, HeH+, LiH and LiH+. Cooling functions for the triatomic ions H+3 and H2D+ are also considered. Analytic fits as functions of temperature are provided. {\textcopyright} 2011 The Authors Monthly Notices of the Royal Astronomical Society {\textcopyright} 2011 RAS.},
author = {Coppola, C. M. and Lodi, L. and Tennyson, J.},
doi = {10.1111/j.1365-2966.2011.18723.x},
file = {:home/william/Documents/Papers/mnras0415-0487.pdf:pdf},
issn = {00358711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Early Universe,Molecular processes},
number = {1},
pages = {487--493},
title = {{Radiative cooling functions for primordial molecules}},
volume = {415},
year = {2011}
}
@article{Li2018,
abstract = {Understanding how galaxies maintain the inefficiency of star formation with physically self-consistent models is a central problem for galaxy evolution. Although numerous theoretical models by invoking different feedback processes have been proposed in recent decades, the debate still exists. By means of high-resolution two-dimensional hydrodynamical simulations, we study the three feedback (stellar wind heating, SNe feedback, and AGN feedback) effects in suppressing star formation activities on the cosmological evolution of early-type galaxies with different stellar masses. The availability of gas sources for star formation comes exclusively from the mass losses of dying low-mass stars for most of our models. We find that SNe feedback can keep star formation at a significantly low level for low mass galaxies for a cosmological evolution time. For the high mass elliptical galaxies, AGN feedback can efficiently offset the radiative cooling and thus plays a dominate role in regulating the star formation activities. Such a suppression of star formation is extremely efficient in the inner region of the galaxies. As expected, AGB heating cannot balance the cooling losses in the whole galaxies and hence cannot account for the suppression for both cases. The hot plasma X-ray temperature {\$}T{\_}{\{}\backslashrm X{\}}{\$} can be in agreement with the observed data with the inclusion of effective feedback processes. We further find that X-ray luminosity {\$}L{\_}{\{}\backslashrm X{\}}{\$} for the hot gas in our effective feedback models is consistent with the observed values. These results thus suggest that we can use {\$}T{\_}{\{}\backslashrm X{\}}{\$} and {\$}L{\_}{\{}\backslashrm X{\}}{\$} to probe the role of different feedback processes. The inclusion of additional gas sources can make the mass scale between SNe and AGN feedback dominating in suppressing star formation decrease to an observationally inferred value of a few {\$}10{\^{}}{\{}10{\}}{\~{}}M{\_}{\{}\backslashodot{\}}{\$}.},
archivePrefix = {arXiv},
arxivId = {1803.01444},
author = {Li, Ya-Ping and Yuan, Feng and Mo, Houjun and Yoon, Doosoo and Gan, Zhao-Ming and Ho, Luis C. and Wang, Bo and Ostriker, Jeremiah P. and Ciotti, Luca},
eprint = {1803.01444},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Li et al. - 2018 - Stellar and AGN feedback in isolated early-type galaxies the role in regulating star formation and ISM properties.pdf:pdf},
number = {2016},
pages = {1--19},
title = {{Stellar and AGN feedback in isolated early-type galaxies: the role in regulating star formation and ISM properties}},
url = {http://arxiv.org/abs/1803.01444},
year = {2018}
}
@article{Binney2004,
abstract = {Evidence is summarized which suggests that when a protogalaxy collapses, a fraction f of its gas fails to heat to the virial temperature, where f is large for haloes less massive than the value M * associated with L * galaxies. Stars and galaxies form only from the cool gas fraction. Hot gas is ejected from low-mass systems as in conventional semi-analytic models of galaxy formation. In high-mass systems it is retained but does not cool and form stars. Instead it builds up as a largely inert atmosphere, in which cooling is inhibited by an episodically active galactic nucleus. Cold gas frequently falls into galactic haloes. In the absence of a dense atmosphere of virial-temperature gas it builds up on nearly circular orbits and can be observed in the 21-cm line of H I. When there is a sufficiently dense hot atmosphere, cold infalling gas tends to be ablated and absorbed by the hot atmosphere before it can form stars. The picture nicely explains away the surfeit of high-luminosity galaxies that has recently plagued semi-analytic models of galaxy formation, replacing them by systems of moderate luminosity from old stars and large X-ray luminosities from hot gas.},
author = {Binney, James},
doi = {10.1111/j.1365-2966.2004.07277.x},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Binney - 2004 - On the origin of the galaxy luminosity function.pdf:pdf},
journal = {Mon. Not. R. Astron. Soc},
keywords = {formation,galaxies},
pages = {1093--1096},
title = {{On the origin of the galaxy luminosity function}},
url = {https://oup.silverchair-cdn.com/oup/backfile/Content{\_}public/Journal/mnras/347/4/10.1111/j.1365-2966.2004.07277.x/2/347-4-1093.pdf?Expires=1490625615{\&}Signature=ZpJHnIgqnanHD-YoifckSOhMTuAn2LzJd6HYAem{~}DPYw5ATG7b8bfLNKEmC6{~}52T57Z4t7SYRCKqmuxRtL0Im9G29Wa9HS9y},
volume = {347},
year = {2004}
}
@article{Circosta2019,
author = {Circosta, Chiara},
file = {:home/william/Documents/Papers/Circosta{\_}Chiara.pdf:pdf},
title = {{A multi-wavelength study of the interstellar medium in active galactic nuclei at cosmic noon}},
year = {2019}
}
@article{Cielo2017a,
abstract = {Jets from Active Galactic Nuclei (AGN) inflate large cavities in the hot gas environment around galaxies and galaxy clusters. The large-scale gas circulation promoted within such cavities by the jet itself gives rise to backflows that propagate back to the center of the jet-cocoon system, spanning all the physical scales relevant for the AGN. Using an Adaptive Mesh Refinement code, we study these backflows through a series of numerical experiments, aiming at understanding how their global properties depend on jet parameters. We are able to characterize their mass flux down to a scale of a few kiloparsecs to about {\$}0.5\backslash,\backslashmathrm{\{}M{\_}\backslashodot/y{\}}{\$}for as long as {\$}15{\$} or {\$}20{\$} Myr, depending on jet power. We find that backflows are both spatially coherent and temporally textbf{\{}intermittent{\}}, independently of jet power in the range {\$}10{\^{}}{\{}43-45{\}}{\$} erg/s. Using the mass flux thus measured, we model analytically the effect of backflows on the central accretion region, where a Magnetically Arrested Disk lies at the center of a thin circumnuclear disk. Backflow accretion onto the disk modifies its density profile, producing a flat core and tail. We use this analytic model to predict how accretion beyond the BH magnetopause is modified, and thus how the jet power is temporally modulated. Under the assumption that the magnetic flux stays frozen in the accreting matter, and that the jets are always launched via the Blandford-Znajek (1977) mechanism, we find that backflows are capable of boosting the jet power up to tenfold during relatively short time episodes (a few Myr).},
archivePrefix = {arXiv},
arxivId = {1701.07825},
author = {Cielo, S. and Antonuccio-Delogu, V. and Silk, J. and Romeo, A. D.},
doi = {10.1093/mnras/stx403},
eprint = {1701.07825},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Cielo et al. - 2017 - Backflows by AGN jets Global properties and influence on SMBH accretion.pdf:pdf},
keywords = {1 i n t,active,bac k f l,d ag n j,e t,g y a n,galaxies,h o l o,jets,l at i o,m o r p,methods,n,numerical,ow,r e g u,ro d u c,s e l f,t i o n},
pages = {4526--4539},
title = {{Backflows by AGN jets: Global properties and influence on SMBH accretion}},
url = {http://arxiv.org/abs/1701.07825{\%}0Ahttp://dx.doi.org/10.1093/mnras/stx403},
volume = {4539},
year = {2017}
}
@article{Fox2015a,
abstract = {Giant lobes of plasma extend ≈55° above and below the Galactic center, glowing in emission from gamma rays (the Fermi Bubbles) to microwaves and polarized radio waves. We use ultraviolet absorption-line spectra from the Hubble Space Telescope to constrain the velocity of the outflowing gas within these regions, targeting the quasar PDS 456 (l, b = 10.°4, +11.°2). This sightline passes through a clear biconical structure seen in hard X-ray and gamma-ray emission near the base of the northern Fermi Bubble. We report two high-velocity metal absorption components, at v LSR = –235 and +250 km s–1, which cannot be explained by co-rotating gas in the Galactic disk or halo. Their velocities are suggestive of an origin on the front and back side of an expanding biconical outflow emanating from the Galactic center. We develop simple kinematic biconical outflow models that can explain the observed profiles with an outflow velocity of gsim900 km s–1 and a full opening angle of ≈110° (matching the X-ray bicone). This indicates Galactic center activity over the last ≈2.5-4.0 Myr, in line with age estimates of the Fermi Bubbles. The observations illustrate the use of UV spectroscopy to probe the properties of swept-up gas venting into the Fermi Bubbles. Based on observations taken under program 13448 of the NASA/ESA Hubble Space Telescope, obtained at the Space Telescope Science Institute, which is operated by the Association of Universities for Research in Astronomy, Inc., under NASA contract NAS 5-26555, and under program 14B-299 of the NRAO Green Bank Telescope, which is a facility of the National Science Foundation operated under cooperative agreement by Associated Universities, Inc.},
author = {Fox, Andrew J. and Bordoloi, Rongmon and Savage, Blair D. and Lockman, Felix J. and Jenkins, Edward B. and Wakker, Bart P. and Bland-Hawthorn, Joss and Hernandez, Svea and Kim, Tae Sun and Benjamin, Robert A. and Bowen, David V. and Tumlinson, Jason},
doi = {10.1088/2041-8205/799/1/L7},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Fox et al. - 2015 - PROBING the Fermi bubbles in ultraviolet absorption A spectroscopic signature of the milky way's biconical nuclear o.pdf:pdf},
issn = {20418213},
journal = {Astrophys. J. Lett.},
keywords = {Galaxy: center,Galaxy: evolution,Galaxy: halo,ISM: jets and outflows,ISM: kinematics and dynamics},
number = {1},
title = {{PROBING the Fermi bubbles in ultraviolet absorption: A spectroscopic signature of the milky way's biconical nuclear outflow}},
volume = {799},
year = {2015}
}
@article{Vermot2019,
abstract = {Aims. We characterise the properties of stars, dust, and gas and their spatial distribution in the central region of the Seyfert 2 galaxy NGC 1068. Method. Our study is based on near-infrared (YJH, 0.95-1.650 $\mu$m, R = 350) long-slit spectroscopy observations of the central region of NGC 1068 with a 0.4″ spatial resolution. We decomposed the observed continuum emission into three components: hot dust, stars, and scattered light from the central engine. We measured their contributions at various distances from the nucleus. We also measured fluxes and Doppler shifts for the emission lines in our spectrum to probe the physical conditions of the narrow line region. Results. Dust and stars are the main sources of continuum emission, but scattered light from the central engine has also been detected in the very central region. Together, these three components reproduce the observed continuum well. The dust emission is compatible with a 830 K blackbody. It has only been detected in the very central region and is not spatially resolved. The stellar content is ubiquitous. It harbours a 250 pc cusp centred around the nucleus, over-imposed on a young stellar background. The spectrum of the cusp is consistent with a 120 Myr old single stellar population. Finally, the emission lines exhibit a significant Doppler shift that is consistent with a radial outflow from the nucleus in a biconical structure. The [Fe II] behaviour strongly differs from other lines, indicating that it arises from a different structure.},
archivePrefix = {arXiv},
arxivId = {1905.09208},
author = {Vermot, Pierre and Cl{\'{e}}net, Yann and Gratadour, Damien},
doi = {10.1051/0004-6361/201935715},
eprint = {1905.09208},
file = {:home/william/Documents/Papers/1905.09208.pdf:pdf},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Galaxies: Seyfert,Galaxies: active,Galaxies: individual: NGC 1068,Galaxies: stellar content,Infrared: galaxies,Techniques: spectroscopic},
number = {35715},
pages = {1--12},
title = {{New insights on the central stellar population and gas outflow in NGC 1068 from YJH spectroscopy with SPHERE/VLT}},
volume = {629},
year = {2019}
}
@article{May2017,
abstract = {We present an analysis of the Seyfert 2 galaxyNGC1068 of archive data from the Spectrograph for INtegral Field Observations in the Near Infrared (SINFONI)-Very Large Telescope, in the HK bands with pixel scales of 0.1 (data set 1-DS1) and 0.025 (DS2) arcsec. The data are revisited with a sophisticated data treatment, such as the differential atmospheric refraction correction and the application of a Butterworth filtering and deconvolution. The gain in the process is quantified by a significant improvement in the Strehl ratio and it shows that an unprecedented high spatial resolution is achieved. For DS1, a detailed study of the H2, [FeII] and [Si VI] emission lines reveals a three-phase gas morphology: (1) the low-velocity [Fe II] emission representing the glowingwall of an hourglass structure, (2) the high-velocity compact blobs of low and high ionization emissions filling the hourglass volume and (3) the distribution of H2 molecular gas defines the thick and irregular walls of a bubble surrounding a cavity. Both the hourglass and the molecular emissions have an asymmetry caused by the fragmentation of the north-eastern molecular wall, closest to the active galactic nucleus, resulting in highvelocity compact blobs of ionized gas outside the bubble. The south-western part of the bubble is excavated by the jet, where the blobs remain confined and are blown along the bubble's inner boundary. We propose that those blobs are driven by a hot 'secondary wind' coming from the spot where the jet interacts and injects its energy in the molecular gas. The combination of a primary wind launched by the central source and the secondary wind is what we call a two-stage outflow. For DS2, we detected a [Si VI] outflow nearly coplanar to the maser disc and orthogonal to the CO outflow found by a previous study. Such unexpected scenario is interpreted as the interaction between the central radiation field and a two-phase gas density torus.},
archivePrefix = {arXiv},
arxivId = {2007.07932},
author = {May, D. and Steiner, J. E.},
doi = {10.1093/mnras/stx886},
eprint = {2007.07932},
file = {:home/william/Documents/Papers/2007.07932.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {(ngc 1068)-galaxies,Individual,Kinematics and dynamics-galaxies,Nuclei,Spectroscopic-galaxies,Techniques},
number = {1},
pages = {994--1025},
title = {{A two-stage outflow in ngc 1068}},
volume = {469},
year = {2017}
}
@article{Schmidt1966,
author = {Schmidt, Maarten},
doi = {10.1086/148854},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Schmidt - 1966 - Lifetimes of Extragalactic Radio Sources.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
pages = {7},
title = {{Lifetimes of Extragalactic Radio Sources}},
url = {http://adsabs.harvard.edu/doi/10.1086/148854},
volume = {146},
year = {1966}
}
@article{Cheng2015a,
abstract = {We analyse the origin of the gamma-ray flux from the Fermi Bubbles (FBs) in the framework of the hadronic model in which gamma-rays are produced by collisions of relativistic protons with the protons of background plasma in the Galactic halo. It is assumed in this model that the observed radio emission from the FBs is due to synchrotron radiation of secondary electrons produced by {\$}pp{\$} collisions. However, if these electrons loose their energy by the synchrotron and inverse-Compton, the spectrum of secondary electrons is too soft, and an additional arbitrary component of primary electrons is necessary in order to reproduce the radio data. Thus, a mixture of the hadronic and leptonic models is required for the observed radio flux. It was shown that if the spectrum of primary electrons is {\$}\backslashpropto E{\_}e{\^{}}{\{}-2{\}}{\$}, the permitted range of the magnetic field strength is within 2 - 7 {\$}\backslashmu{\$}G region. The fraction of gamma-rays produced by {\$}pp{\$} collisions can reach about 80{\%} of the total gamma-ray flux from the FBs. If magnetic field is {\textless}2 {\$}\backslashmu{\$}G or {\textgreater}7 {\$}\backslashmu{\$}G the model is unable to reproduce the data. Alternatively, the electrons in the FBs may lose their energy by adiabatic energy losses if there is a strong plasma outflow in the GC. Then, the pure hadronic model is able to reproduce characteristics of the radio and gamma-ray flux from the FBs. However, in this case the required magnetic field strength in the FBs and the power of CR sources are much higher than those followed from observations.},
author = {Cheng, K. S. and Chernyshov, D. O. and Dogiel, V. A. and Ko, C. M.},
doi = {10.1088/0004-637X/799/1/112},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Cheng et al. - 2015 - Multi-wavelength emission from the fermi bubble. II. Secondary electrons and the hadronic model of the bubble.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {Galaxy: center,acceleration of particles,gamma rays: ISM},
number = {1},
title = {{Multi-wavelength emission from the fermi bubble. II. Secondary electrons and the hadronic model of the bubble}},
volume = {799},
year = {2015}
}
@article{Lamastra2016,
abstract = {We compute the non-thermal emissions produced by relativistic particles accelerated by the shocks driven by the active galactic nucleus (AGN) in NGC 1068, and we compare the model predictions with the observed $\gamma$-ray and radio spectra. The former is produced by pion decay, inverse Compton scattering, and bremsstrahlung, while the latter is produced by synchrotron radiation. We derive the $\gamma$-ray and radio emissions by assuming the standard acceleration theory, and we discuss how our results compare with those corresponding to other commonly assumed sources of $\gamma$-ray and radio emissions, like supernova remnants (SNR) or AGN jets. We find that the AGN-driven shocks observed in the circumnuclear molecular disk of NGC 1068 provide a contribution to the $\gamma$-ray emission comparable to that provided by the starburst activity when standard particle acceleration efficiencies are assumed, while the shocks can yield the whole $\gamma$-ray emission only when the parameters describing the acceleration efficiency and the proton coupling with the molecular gas are tuned to values larger than those assumed in standard, SNR-driven shocks. We discuss the range of acceleration efficiencies (for protons and electrons) and of proton calorimetric fractions required to account for the observed $\gamma$-ray emission in the AGN outflow model. We further compare the neutrino flux expected in our model with constraints from current experiments, and we provide predictions for the detections by the upcoming KM3NeT neutrino telescope. This analysis strongly motivates observations of NGC 1068 at ≳ TeV energies with current and future Cherenkov telescopes in order to gain insight into the nature of the $\gamma$-rays source.},
archivePrefix = {arXiv},
arxivId = {1609.09664},
author = {Lamastra, A. and Fiore, F. and Guetta, D. and Antonelli, L. A. and Colafrancesco, S. and Menci, N. and Puccetti, S. and Stamerra, A. and Zappacosta, L.},
doi = {10.1051/0004-6361/201628667},
eprint = {1609.09664},
file = {:home/william/Documents/Papers/1609.09664.pdf:pdf},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Galaxies: Seyfert,Galaxies: individual: NGC 1068,Gamma rays: galaxies,Radiation mechanisms: general},
number = {Ic},
pages = {1--12},
title = {{Galactic outflow driven by the active nucleus and the origin of the gamma-ray emission in NGC 1068}},
volume = {596},
year = {2016}
}
@article{Fiore2017,
abstract = {Feedback from accreting SMBHs is often identified as the main mechanism responsible for regulating star-formation in AGN host galaxies. However, the relationships between AGN activity, radiation, winds, and star-formation are complex and still far from being understood. We study scaling relations between AGN properties, host galaxy properties and AGN winds. We then evaluate the wind mean impact on the global star-formation history, taking into account the short AGN duty cycle with respect to that of star-formation. We first collect AGN wind observations for 94 AGN with detected massive winds at sub-pc to kpc spatial scales. We then fold AGN wind scaling relations with AGN luminosity functions, to evaluate the average AGN wind mass-loading factor as a function of cosmic time. We find strong correlations between the AGN molecular and ionised wind mass outflow rates and the AGN bolometric luminosity. The power law scaling is steeper for ionised winds (slope 1.29+/-0.38) than for molecular winds (0.76+/-0.06), meaning that the two rates converge at high bolometric luminosities. The molecular gas depletion timescale and the molecular gas fraction of galaxies hosting powerful AGN winds are 3-10 times shorter and smaller than those of main-sequence galaxies with similar SFR, stellar mass and redshift. These findings suggest that, at high AGN bolometric luminosity, the reduced molecular gas fraction may be due to the destruction of molecules by the wind, leading to a larger fraction of gas in the atomic ionised phase. The AGN wind mass-loading factor {\$}\backslasheta=\backslashdot M{\_}{\{}OF{\}}/SFR{\$} is systematically higher than that of starburst driven winds. Our analysis shows that AGN winds are, on average, powerful enough to clean galaxies from their molecular gas only in massive systems at z{\textless}=2, i.e. a strong form of co-evolution between SMBHs and galaxies appears to break down for the least massive galaxies.},
archivePrefix = {arXiv},
arxivId = {1702.04507},
author = {Fiore, F. and Feruglio, C. and Shankar, F. and Bischetti, M. and Bongiorno, A. and Brusa, M. and Carniani, S. and Cicone, C. and Duras, F. and Lamastra, A. and Mainieri, V. and Marconi, A. and Menci, N. and Maiolino, R. and Piconcelli, E. and Vietri, G. and Zappacosta, L.},
doi = {10.1051/0004-6361/201629478},
eprint = {1702.04507},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Fiore et al. - 2017 - AGN wind scaling relations and the co-evolution of black holes and galaxies.pdf:pdf},
keywords = {active,evolution,galaxies,general,quasars},
pages = {1--21},
title = {{AGN wind scaling relations and the co-evolution of black holes and galaxies}},
url = {http://arxiv.org/abs/1702.04507{\%}0Ahttp://dx.doi.org/10.1051/0004-6361/201629478},
volume = {143},
year = {2017}
}
@article{U2018,
abstract = {The role of feedback in triggering or quenching star formation and hence driving galaxy evolution can be directly studied with high resolution integral field observations. The manifestation of feedback in shocks is particularly important to examine in galaxy mergers, where violent interactions of gas takes place in the interstellar medium during the course of the galactic collision. As part of our effort to systematically study the local population of luminous infrared galaxies within the Great Observatories All-Sky LIRG Survey, we undertook the Keck OSIRIS AO LIRG Analysis observing campaign to study the gas dynamics in the inner kiloparsec regions of these systems at spatial scales of a few 10s of parsecs. With high-resolution near-infrared adaptive optics-assisted integral-field observations taken with OSIRIS on the Keck Telescopes, we employ near-infrared diagnostics such as Brg and the ro-vibrationally excited H2 lines to quantify the nuclear star formation rate and identify feedback associated with shocked molecular gas seen in 21 nearby luminous infrared galaxies. Shocked molecular gas is preferentially found in the ultraluminous infrared systems, but may also be triggered at a lower luminosity, earlier merging stage. On circumnuclear scales, AGN have a strong effect on heating the surrounding molecular gas, though their coupling is not simply driven by AGN strength but rather is complicated by orientation, dust shielding, density, and other factors. We find that the nuclear star formation correlates with merger class and diminishing projected nuclear separations. These trends are largely consistent with the picture of merger-induced starbursts within the center of galaxy mergers.},
archivePrefix = {arXiv},
arxivId = {1811.09281},
author = {U, Vivian and Medling, Anne M. and Inami, Hanae and Armus, Lee and D{\'{i}}az-Santos, Tanio and Charmandaris, Vassilis and Howell, Justin and Stierwalt, Sabrina and Privon, George C. and Linden, Sean T. and Sanders, David B. and Max, Claire E. and Evans, Aaron S. and Barcos-Mu{\~{n}}oz, Loreto and Chiang, Charleston W. K. and Appleton, Phil and Canalizo, Gabriela and Fazio, Giovanni and Iwasawa, Kazushi and Larson, Kirsten and Mazzarella, Joseph and Murphy, Eric and Rich, Jeffrey and Surace, Jason},
doi = {10.3847/1538-4357/aaf1c2},
eprint = {1811.09281},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/U et al. - 2018 - Keck OSIRIS AO LIRG Analysis Feedback in the Nuclei of Luminous Infrared Galaxies.pdf:pdf},
keywords = {2008,2010,2011,active,allen et al,and others,e,farage et al,g,galaxies,however,iii,interactions,nuclei,rich et al,such optical-},
title = {{Keck OSIRIS AO LIRG Analysis: Feedback in the Nuclei of Luminous Infrared Galaxies}},
url = {http://arxiv.org/abs/1811.09281{\%}0Ahttp://dx.doi.org/10.3847/1538-4357/aaf1c2},
year = {2018}
}
@article{Ishibashi2018a,
abstract = {The increasing observational evidence of galactic outflows is considered as a sign of active galactic nucleus (AGN) feedback in action. However, the physical mechanism responsible for driving the observed outflows remains unclear, and whether it is due to momentum, energy, or radiation is still a matter of debate. The observed outflow energetics, in particular the large measured values of the momentum ratio ({\$}\backslashdot{\{}p{\}}/(L/c) \backslashsim 10{\$}) and energy ratio ({\$}\backslashdot{\{}E{\}}{\_}k/L \backslashsim 0.05{\$}), seems to favour the energy-driving mechanism; and most observational works have focused their comparison with wind energy-driven models. Here we show that AGN radiation pressure on dust can adequately reproduce the observed outflow energetics (mass outflow rate, momentum flux, and kinetic power), as well as the scalings with luminosity, provided that the effects of radiation trapping are properly taken into account. In particular, we predict a sub-linear scaling for the mass outflow rate ({\$}\backslashdot{\{}M{\}} \backslashpropto L{\^{}}{\{}1/2{\}}{\$}) and a super-linear scaling for the kinetic power ({\$}\backslashdot{\{}E{\}}{\_}k \backslashpropto L{\^{}}{\{}3/2{\}}{\$}), in agreement with the observational scaling relations reported in the most recent compilation of AGN outflow data. We conclude that AGN radiative feedback can account for the global outflow energetics, at least equally well as the wind energy-driving mechanism, and therefore both physical models should be considered in the interpretation of future AGN outflow observations.},
archivePrefix = {arXiv},
arxivId = {1801.09700},
author = {Ishibashi, W. and Fabian, A. C. and Maiolino, R.},
doi = {10.1093/mnras/sty236},
eprint = {1801.09700},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ishibashi, Fabian, Maiolino - 2018 - The energetics of AGN radiation pressure-driven outflows.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Black hole physics,Galaxies: Active,Galaxies: Evolution},
number = {1},
pages = {512--519},
title = {{The energetics of AGN radiation pressure-driven outflows}},
volume = {476},
year = {2018}
}
@article{Harrison2014,
abstract = {We present integral field unit (IFU) observations covering the [O III]4959,5007 and H-Beta emission lines of sixteen z{\textless}0.2 type 2 active galactic nuclei (AGN). Our targets are selected from a well-constrained parent sample of 24,000 AGN so that we can place our observations into the context of the overall AGN population. Our targets are radio-quiet with star formation rates ({\textless}{\~{}}[10-100] Msol/yr) that are consistent with normal star-forming galaxies. We decouple the kinematics of galaxy dynamics and mergers from outflows. We find high-velocity ionised gas (velocity widths of 600-1500 km/s and maximum velocities of {\textless}=1700 km/s) with observed spatial extents of {\textgreater}{\~{}}(6-16) kpc in all targets and observe signatures of spherical outflows and bi-polar superbubbles. We show that our targets are representative of z{\textless}0.2, luminous (i.e., L([O III]) {\textgreater} 5x10{\^{}}41 erg/s) type 2 AGN and that ionised outflows are not only common but also in {\textgreater}=70{\%} (3 sigma confidence) of cases, they are extended over kiloparsec scales. Our study demonstrates that galaxy-wide energetic outflows are not confined to the most extreme star-forming galaxies or radio-luminous AGN; however, there may be a higher incidence of the most extreme outflow velocities in quasars hosted in ultra-luminous infrared galaxies. Both star formation and AGN activity appear to be energetically viable to drive the outflows and we find no definitive evidence that favours one process over the other. Although highly uncertain, we derive mass outflow rates (typically {\~{}}10x the SFRs), kinetic energies ({\~{}}0.5-10{\%} of L[AGN]) and momentum rates (typically {\textgreater}{\~{}}10-20x L[AGN]/c) consistent with theoretical models that predict AGN-driven outflows play a significant role in shaping the evolution of galaxies.},
author = {Harrison, C. M. and Alexander, D. M. and Mullaney, J. R. and Swinbank, A. M.},
doi = {10.1093/mnras/stu515},
file = {:home/william/Documents/Papers/[Harrison. C. et al]-Kiloparsec-scale outflows are prevalent among luminous AGN-outflows and feedback in the context of the overall AGN population.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: active,Galaxies: evolution,Galaxies: kinematics and dynamics,Quasars: emission lines},
number = {4},
pages = {3306--3347},
title = {{Kiloparsec-scale outflows are prevalent among luminous AGN: Outflows and feedback in the context of the overall AGN population}},
volume = {441},
year = {2014}
}
@article{King2005,
abstract = {Recent observations of young galaxies at redshifts z {\~{}} 3 have revealed simultaneous AGN and starburst activity, as well as galaxy-wide superwinds. I show that there is probably a close connection between these phenomena by extending an earlier treatment of the M BH -$\sigma$ relation. As the black hole grows, an outflow drives a shell into the surrounding gas. This stalls after a dynamical time at a size determined by the hole's current mass and thereafter grows on the Salpeter timescale. The gas trapped inside this bubble cools, forms stars, and is recycled as accretion and outflow. The consequent high metallicity agrees with that commonly observed in AGN accretion. Once the hole reaches a critical mass, this region attains a size such that the gas can no longer cool efficiently. The resulting energy-driven flow expels the remaining gas as a superwind, fixing both the M BH -$\sigma$ relation and the total stellar bulge mass at values in good agreement with observations. Black hole growth thus produces starbursts and ultimately a superwind.},
author = {King, Andrew},
doi = {10.1086/499430},
file = {:home/william/Documents/Papers/[KIng]-THE AGN–STARBURST CONNECTION, GALACTIC SUPERWINDS.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
number = {2},
pages = {L121--L123},
title = {{ The AGN-Starburst Connection, Galactic Superwinds, and M BH -$\sigma$ }},
volume = {635},
year = {2005}
}
@article{Paynter2021,
abstract = {If gamma-ray bursts are at cosmological distances, they must be gravitationally lensed occasionally1,2. The detection of lensed images with millisecond-to-second time delays provides evidence for intermediate-mass black holes, a population that has been difficult to observe. Several studies have searched for these delays in gamma-ray burst light curves, which would indicate an intervening gravitational lens3–6. Among the {\~{}}104 gamma-ray bursts observed, there have been a handful of claimed lensing detections7, but none have been statistically robust. Here we present a Bayesian analysis identifying gravitational lensing in the light curve of GRB 950830. The inferred lens mass Ml depends on the unknown lens redshift zl, and is given by (1+zl)Ml=5.5−0.9+1.7×104M⊙ (90{\%} credibility), which we interpret as evidence for an intermediate-mass black hole. The most probable configuration, with a lens redshift zl ≈ 1 and a gamma-ray burst redshift zs ≈ 2, yields a present-day number density of about 2.3−1.6+4.9×103Mpc−3 (90{\%} credibility) with a dimensionless energy density $\Omega$IMBH≈4.6−3.3+9.8×10−4. The false alarm probability for this detection is {\~{}}0.6{\%} with trial factors. While it is possible that GRB 950830 was lensed by a globular cluster, it is unlikely as we infer a cosmic density inconsistent with predictions for globular clusters $\Omega$GC ≈ 8 × 10−6 at 99.8{\%} credibility. If a significant intermediate-mass black hole population exists, it could provide the seeds for the growth of supermassive black holes in the early Universe.},
archivePrefix = {arXiv},
arxivId = {2103.15414},
author = {Paynter, James and Webster, Rachel and Thrane, Eric},
doi = {10.1038/s41550-021-01307-1},
eprint = {2103.15414},
file = {:home/william/Documents/Papers/s41550-021-01307-1.pdf:pdf},
issn = {23973366},
journal = {Nat. Astron.},
number = {6},
pages = {560--568},
publisher = {Springer US},
title = {{Evidence for an intermediate-mass black hole from a gravitationally lensed gamma-ray burst}},
url = {http://dx.doi.org/10.1038/s41550-021-01307-1},
volume = {5},
year = {2021}
}
@article{Florez2020a,
abstract = {We investigate the relation between AGN and star formation (SF) activity at {\$}0.5 {\textless} z {\textless} 3{\$} by analyzing 898 galaxies with X-ray luminous AGN ({\$}L{\_}X {\textgreater} 10{\^{}}{\{}44{\}}{\$} erg s{\$}{\^{}}{\{}-1{\}}{\$}) and a large comparison sample of {\$}\backslashsim 320,000{\$} galaxies without X-ray luminous AGN. Our samples are selected from a large (11.8 deg{\$}{\^{}}2{\$}) area in Stripe 82 that has multi-wavelength (X-ray to far-IR) data. The enormous comoving volume ({\$}\backslashsim 0.3{\$} Gpc{\$}{\^{}}3{\$}) at {\$}0.5 {\textless} z {\textless} 3{\$} minimizes the effects of cosmic variance and captures a large number of massive galaxies ({\$}\backslashsim 30,000{\$} galaxies with {\$}M{\_}* {\textgreater} 10{\^{}}{\{}11{\}} \backslash M{\_}{\{}\backslashodot{\}}{\$}) and X-ray luminous AGN. While many galaxy studies discard AGN hosts, we fit the SED of galaxies with and without X-ray luminous AGN with Code Investigating GALaxy Emission (CIGALE) and include AGN emission templates. We find that without this inclusion, stellar masses and star formation rates (SFRs) in AGN host galaxies can be overestimated, on average, by factors of up to {\$}\backslashsim 5{\$} and {\$}\backslashsim 10{\$}, respectively. The average SFR of galaxies with X-ray luminous AGN is higher by a factor of {\$}\backslashsim 3{\$} to {\$}10{\$} compared to galaxies without X-ray luminous AGN at fixed stellar mass and redshift, suggesting that high SFRs and high AGN X-ray luminosities may be fueled by common mechanisms. The vast majority ({\$}{\textgreater} 95 \backslash{\%}{\$}) of galaxies with X-ray luminous AGN at {\$}z=0.5-3{\$} do not show quenched SF: this suggests that if AGN feedback quenches SF, the associated quenching process takes a significant time to act and the quenched phase sets in after the highly luminous phases of AGN activity.},
archivePrefix = {arXiv},
arxivId = {2007.12170},
author = {Florez, J. and Jogee, S. and Sherman, S. and Stevans, M. L. and Finkelstein, S. L. and Papovich, C. and Kawinwanichakij, L. and Ciardullo, R. and Gronwall, C. and Urry, C. M. and Kirkpatrick, A. and LaMassa, S. M. and Ananna, T. T. and Wold, I.},
eprint = {2007.12170},
file = {:home/william/Documents/Papers/2007.12170.pdf:pdf},
keywords = {evolution,galaxies,general,star formation},
number = {July},
pages = {1--24},
title = {{Exploring AGN and Star Formation Activity of Massive Galaxies at Cosmic Noon}},
url = {http://arxiv.org/abs/2007.12170},
volume = {24},
year = {2020}
}
@article{Abdalla2020,
abstract = {The Cherenkov Telescope Array (CTA), the new-generation ground-based observatory for $\gamma$-ray astronomy, provides unique capabilities to address significant open questions in astrophysics, cosmology, and fundamental physics. We study some of the salient areas of $\gamma$-ray cosmology that can be explored as part of the Key Science Projects of CTA, through simulated observations of active galactic nuclei (AGN) and of their relativistic jets. Observations of AGN with CTA will enable a measurement of $\gamma$-ray absorption on the extragalactic background light with a statistical uncertainty below 15{\%} up to a redshift z = 2 and to constrain or detect $\gamma$-ray halos up to intergalactic-magnetic-field strengths of at least 0.3 pG. Extragalactic observations with CTA also show promising potential to probe physics beyond the Standard Model. The best limits on Lorentz invariance violation from $\gamma$-ray astronomy will be improved by a factor of at least two to three. CTA will also probe the parameter space in which axion-like particles could constitute a significant fraction, if not all, of dark matter. We conclude on the synergies between CTA and other upcoming facilities that will foster the growth of $\gamma$-ray cosmology.},
archivePrefix = {arXiv},
arxivId = {2010.01349},
author = {Abdalla, H. and Abe, H. and Acero, F. and Acharyya, A. and Adam, R. and Agudo, I. and Aguirre-Santaella, A. and Alfaro, R. and Alfaro, J. and Alispach, C. and Aloisio, R. and Batista, R. Alves and Amati, L. and Amato, E. and Ambrosi, G. and Ang{\"{u}}ner, E. O. and Araudo, A. and Armstrong, T. and Arqueros, F. and Arrabito, L. and Asano, K. and Ascas{\'{i}}bar, Y. and Ashley, M. and Backes, M. and Balazs, C. and Balbo, M. and Balmaverde, B. and Larriva, A. Baquero and Martins, V. Barbosa and Barkov, M. and Baroncelli, L. and de Almeida, U. Barres and Barrio, J. A. and Batista, P. and Becerra, J. and Becherini, Y. and Beck, G. and Tjus, J. Becker and Belmont, R. and Benbow, W. and Bernardini, E. and Berti, A. and Berton, M. and Bertucci, B. and Beshley, V. and Bi, B. and Biasuzzi, B. and Biland, A. and Bissaldi, E. and Biteau, J. and Blanch, O. and Bocchino, F. and Boisson, C. and Bolmont, J. and Bonanno, G. and Arbeletche, L. Bonneau and Bonnoli, G. and Bordas, P. and Bottacini, E. and B{\"{o}}ttcher, M. and Bozhilov, V. and Bregeon, J. and Brill, A. and Brown, A. M. and Bruno, P. and Bruno, A. and Bulgarelli, A. and Burton, M. and Buscemi, M. and Caccianiga, A. and Cameron, R. and Capasso, M. and Caprai, M. and Caproni, A. and Capuzzo-Dolcetta, R. and Caraveo, P. and Carosi, R. and Carosi, A. and Casanova, S. and Cascone, E. and Cauz, D. and Cerny, K. and Cerruti, M. and Chadwick, P. and Chaty, S. and Chen, A. and Chernyakova, M. and Chiaro, G. and Chiavassa, A. and Chytka, L. and Conforti, V. and Conte, F. and Contreras, J. L. and Coronado-Blazquez, J. and Cortina, J. and Costa, A. and Costantini, H. and Covino, S. and Cristofari, P. and Cuevas, O. and D'Ammando, F. and Daniel, M. K. and Davies, J. and Dazzi, F. and de Angelis, A. and de Lavergne, M. de Bony and de Caprio, V. and dos Anjos, R. de C{\'{a}}ssia and Pino, E. M.de Gouveia Dal and de Lotto, B. and de Martino, D. and de Naurois, M. and Wilhelmi, E. de O{\~{n}}a and de Palma, F. and de Souza, V. and Delgado, C. and Ceca, R. Della and della Volpe, D. and Depaoli, D. and {Di Girolamo}, T. and {Di Pierro}, F. and D{\'{i}}az, C. and D{\'{i}}az-Bahamondes, C. and Diebold, S. and Djannati-Ata{\"{i}}, A. and Dmytriiev, A. and Dom{\'{i}}nguez, A. and Donini, A. and Dorner, D. and Doro, M. and Dournaux, J. and Dwarkadas, V. V. and Ebr, J. and Eckner, C. and Einecke, S. and Ekoume, T. R.N. and Els{\"{a}}sser, D. and Emery, G. and Evoli, C. and Fairbairn, M. and Falceta-Goncalves, D. and Fegan, S. and Feng, Q. and Ferrand, G. and Fiandrini, E. and Fiasson, A. and Fioretti, V. and Foffano, L. and Fonseca, M. V. and Font, L. and Fontaine, G. and Franco, F. J. and Coromina, L. Freixas and Fukami, S. and Fukazawa, Y. and Fukui, Y. and Gaggero, D. and Galanti, G. and Gammaldi, V. and Garcia, E. and Garczarczyk, M. and Gascon, D. and Gaug, M. and Gent, A. and Ghalumyan, A. and Ghirlanda, G. and Gianotti, F. and Giarrusso, M. and Giavitto, G. and Giglietto, N. and Giordano, F. and Glicenstein, J. and Goldoni, P. and Gonz{\'{a}}lez, J. M. and Gourgouliatos, K. and Grabarczyk, T. and Grandi, P. and Granot, J. and Grasso, D. and Green, J. and Grube, J. and Gueta, O. and Gunji, S. and Halim, A. and Harvey, M. and Collado, T. Hassan and Hayashi, K. and Heller, M. and Cadena, S. Hern{\'{a}}ndez and Hervet, O. and Hinton, J. and Hiroshima, N. and Hnatyk, B. and Hnatyk, R. and Hoffmann, D. and Hofmann, W. and Holder, J. and Horan, D. and H{\"{o}}randel, J. and Horvath, P. and Hovatta, T. and Hrabovsky, M. and Hrupec, D. and Hughes, G. and H{\"{u}}tten, M. and Iarlori, M. and Inada, T. and Inoue, S. and Insolia, A. and Ionica, M. and Iori, M. and Jacquemont, M. and Jamrozy, M. and Janecek, P. and Mart{\'{i}}nez, I. Jim{\'{e}}nez and Jin, W. and Jung-Richardt, I. and Jurysek, J. and Kaaret, P. and Karas, V. and Karkar, S. and Kawanaka, N. and Kerszberg, D. and Kh{\'{e}}lifi, B. and Kissmann, R. and Kn{\"{o}}dlseder, J. and Kobayashi, Y. and Kohri, K. and Komin, N. and Kong, A. and Kosack, K. and Kubo, H. and la Palombara, N. and Lamanna, G. and Lang, R. G. and Lapington, J. and Laporte, P. and Lemoine-Goumard, M. and Lenain, J. and Leone, F. and Leto, G. and Leuschner, F. and Lindfors, E. and Lloyd, S. and Lohse, T. and Lombardi, S. and Longo, F. and Lopez, A. and L{\'{o}}pez, M. and L{\'{o}}pez-Coto, R. and Loporchio, S. and Lucarelli, F. and Luque-Escamilla, P. L. and Lyard, E. and Maggio, C. and Majczyna, A. and Makariev, M. and Mallamaci, M. and Mandat, D. and Maneva, G. and Manganaro, M. and Manic{\`{o}}, G. and Marcowith, A. and Marculewicz, M. and Markoff, S. and Marquez, P. and Mart{\'{i}}, J. and Martinez, O. and Mart{\'{i}}nez, M. and Mart{\'{i}}nez, G. and Mart{\'{i}}nez-Huerta, H. and Maurin, G. and Mazin, D. and Mbarubucyeye, J. D. and Miranda, D. Medina and Meyer, M. and Micanovic, S. and Miener, T. and Minev, M. and Miranda, J. M. and Mitchell, A. and Mizuno, T. and Mode, B. and Moderski, R. and Mohrmann, L. and Molina, E. and Montaruli, T. and Moralejo, A. and Merino, J. Morales and Morcuende-Parrilla, D. and Morselli, A. and Mukherjee, R. and Mundell, C. and Murach, T. and Muraishi, H. and Nagai, A. and Nakamori, T. and Nemmen, R. and Niemiec, J. and Nieto, D. and Nievas, M. and Niko{\l}ajuk, M. and Nishijima, K. and Noda, K. and Nosek, D. and Nozaki, S. and O'Brien, P. and Ohira, Y. and Ohishi, M. and Oka, T. and Ong, R. A. and Orienti, M. and Orito, R. and Orlandini, M. and Orlando, E. and Osborne, J. P. and Ostrowski, M. and Oya, I. and Pagliaro, A. and Palatka, M. and Paneque, D. and Pantaleo, F. R. and Paredes, J. M. and Parmiggiani, N. and Patricelli, B. and Pavleti{\'{c}}, L. and Pe'er, A. and Pech, M. and Pecimotika, M. and Peresano, M. and Persic, M. and Petruk, O. and Pfrang, K. and Piatteli, P. and Pietropaolo, E. and Pillera, R. and Pilszyk, B. and Pimentel, D. and Pintore, F. and Pita, S. and Pohl, M. and Poireau, V. and Polo, M. and Prado, R. R. and Prast, J. and Principe, G. and Produit, N. and Prokoph, H. and Prouza, M. and Przybilski, H. and Pueschel, E. and P{\"{u}}hlhofer, G. and Pumo, M. L. and Punch, M. and Queiroz, F. and Quirrenbach, A. and Rando, R. and Razzaque, S. and Rebert, E. and Recchia, S. and Reichherzer, P. and Reimer, O. and Reimer, A. and Renier, Y. and Reposeur, T. and Rhode, W. and Ribeiro, D. and Rib{\'{o}}, M. and Richtler, T. and Rico, J. and Rieger, F. and Rizi, V. and Rodriguez, J. and Fernandez, G. Rodriguez and Ramirez, J. C.Rodriguez and V{\'{a}}zquez, J. J.Rodr{\'{i}}guez and Romano, P. and Romeo, G. and Roncadelli, M. and Rosado, J. and de Leon, A. Rosales and Rowell, G. and Rudak, B. and Rujopakarn, W. and Russo, F. and Sadeh, I. and Saha, L. and Saito, T. and Greus, F. Salesa and Sanchez, D. and S{\'{a}}nchez-Conde, M. and Sangiorgi, P. and Sano, H. and Santander, M. and Santos, E. M. and Sanuy, A. and Sarkar, S. and Saturni, F. G. and Sawangwit, U. and Scherer, A. and Schleicher, B. and Schovanek, P. and Schussler, F. and Schwanke, U. and Sciacca, E. and Scuderi, S. and Arroyo, M. Seglar and Sergijenko, O. and Servillat, M. and Seweryn, K. and Shalchi, A. and Sharma, P. and Shellard, R. C. and Siejkowski, H. and Sinha, A. and Sliusar, V. and Slowikowska, A. and Sokolenko, A. and Sol, H. and Specovius, A. and Spencer, S. and Spiga, D. and Stamerra, A. and Stani{\v{c}}, S. and Starling, R. and Stolarczyk, T. and Straumann, U. and Stri{\v{s}}kovi{\'{c}}, J. and Suda, Y. and {\'{S}}wierk, P. and Tagliaferri, G. and Takahashi, H. and Takahashi, M. and Tavecchio, F. and Taylor, L. and Tejedor, L. A. and Temnikov, P. and Terrier, R. and Terzic, T. and Testa, V. and Tian, W. and Tibaldo, L. and Tonev, D. and Torres, D. F. and Torresi, E. and Tosti, L. and Tothill, N. and Tovmassian, G. and Travnicek, P. and Truzzi, S. and Tuossenel, F. and Umana, G. and Vacula, M. and Vagelli, V. and Valentino, M. and Vallage, B. and Vallania, P. and van Eldik, C. and Varner, G. S. and Vassiliev, V. and Acosta, M. V{\'{a}}zquez and Vecchi, M. and Veh, J. and Vercellone, S. and Vergani, S. and Verguilov, V. and Vettolani, G. P. and Viana, A. and Vigorito, C. F. and Vitale, V. and Vorobiov, S. and Vovk, I. and Vuillaume, T. and Wagner, S. J. and Walter, R. and Watson, J. and White, M. and White, R. and Wiemann, R. and Wierzcholska, A. and Will, M. and Williams, D. A. and Wischnewski, R. and Wolter, A. and Yamazaki, R. and Yanagita, S. and Yang, L. and Yoshikoshi, T. and Zacharias, M. and Zaharijas, G. and Zaric, D. and Zavrtanik, M. and Zavrtanik, D. and Zech, A. and Zechlin, H. and Zhdanov, V. I. and {\v{Z}}ivec, M.},
eprint = {2010.01349},
file = {:home/william/Documents/Papers/2010.01349.pdf:pdf},
issn = {23318422},
journal = {arXiv},
title = {{Sensitivity of the Cherenkov Telescope Array for probing cosmology and fundamental physics with gamma-ray propagation}},
year = {2020}
}
@article{Marti2015a,
abstract = {An overview of grid-based numerical methods used in relativistic hydrodynamics (RHD) and magnetohydrodynamics (RMHD) is presented. Special emphasis is put on a comprehensive review of the application of high-resolution shock-capturing methods. Results of a set of demanding test bench simulations obtained with different numerical methods are compared in an attempt to assess the present capabilities and limits of the various numerical strategies. Applications to three astrophysical phenomena are briefly discussed to motivate the need for and to demonstrate the success of RHD and RMHD simulations in their understanding. The review further provides FORTRAN programs to compute the exact solution of the Riemann problem in RMHD, and to simulate 1D RMHD flows in Cartesian coordinates.},
author = {Mart{\'{i}}, Jos{\'{e}} Mar{\'{i}}a and M{\"{u}}ller, Ewald},
doi = {10.1007/lrca-2015-3},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Mart{\'{i}}, M{\"{u}}ller - 2015 - Grid-based Methods in Relativistic Hydrodynamics and Magnetohydrodynamics.pdf:pdf},
issn = {2367-3621},
journal = {Living Rev. Comput. Astrophys.},
keywords = {c the author,relativistic hydrodynamics,relativistic magnetohydrodynamics,rhd,rmhd,s,this article is distributed,under a},
number = {1},
title = {{Grid-based Methods in Relativistic Hydrodynamics and Magnetohydrodynamics}},
volume = {1},
year = {2015}
}
@article{Mou2014a,
abstract = {A pair of giant gamma-ray bubbles have been revealed by the {\{}$\backslash$it Fermi{\}} LAT. In this paper we investigate their formation mechanism. Observations have indicated that the activity of the supermassive black hole located at the Galactic center, Sgr A*, was much stronger than the present time. Specifically, one possibility is that while Sgr A* was also in the hot accretion regime, the accretion rate should be {\$}10{\^{}}3-10{\^{}}4{\$} times higher during the past {\$}\backslashsim 10{\^{}}7{\$} yr. On the other hand, recent MHD numerical simulations of hot accretion flows have unambiguously shown the existence of strong winds and obtained their properties. Based on these knowledge, by performing three-dimensional hydrodynamical simulations, we show in this paper that the Fermi bubbles could be inflated by winds launched from the ``past' hot accretion flow in Sgr A*. In our model, the active phase of Sgr A* is required to last for about 10 million years and it was quenched no more than 0.2 million years ago. The Central Molecular Zone (CMZ) is included and it collimates the wind orientation towards the Galactic poles. Viscosity suppresses the Rayleigh-Taylor and Kelvin-Helmholtz instabilities and results in the smoothness of the bubble edge. The main observational features of the bubbles can be well explained. Specifically, the {\{}$\backslash$it ROSAT{\}} X-ray features are interpreted by the shocked interstellar medium and the interaction region between winds and CMZ gas. The thermal pressure and temperature obtained in our model are in good consistency with the recent {\{}$\backslash$it Suzaku{\}} observations.},
author = {Mou, Guobin and Yuan, Feng and Bu, Defu and Sun, Mouyuan and Su, Meng},
doi = {10.1088/0004-637X/790/2/109},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Mou et al. - 2014 - Fermi bubbles inflated by winds launched from the hot accretion flow in sgr a.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {Galaxy: nucleus,accretion, accretion disks,black hole physics,galaxies: active,galaxies: jets},
number = {2},
title = {{Fermi bubbles inflated by winds launched from the hot accretion flow in sgr a*}},
volume = {790},
year = {2014}
}
@article{Gowardhan2018b,
abstract = {We report molecular gas observations of IRAS 20100-4156 and IRAS 03158+4227, two local ultraluminous infrared galaxies (ULIRGs) hosting some of the fastest and most massive molecular outflows known. Using ALMA and PdBI observations, we spatially resolve the CO(1-0) emission from the outflowing molecular gas in both and find maximum outflow velocities of {\$} v{\_}{\{}\backslashrm max{\}} \backslashsim 1600{\$} and {\$}\backslashsim 1700{\$} km/s for IRAS 20100-4156 and IRAS 03158+4227, respectively. We find total gas mass outflow rates of {\$}\backslashdot M{\_}{\{}\backslashrm OF{\}} \backslashsim 670{\$} and {\$}\backslashsim 350{\$} Msun/yr, respectively, corresponding to molecular gas depletion timescales {\$}\backslashtau{\^{}}{\{}\backslashrm dep{\}}{\_}{\{}\backslashrm OF{\}} \backslashsim 11{\$} and {\$}\backslashsim 16{\$} Myr. This is nearly 3 times shorter than the depletion timescales implied by star formation, {\$}\backslashtau{\^{}}{\{}\backslashrm dep{\}}{\_}{\{}\backslashrm SFR{\}} \backslashsim 33{\$} and {\$}\backslashsim 46{\$} Myr, respectively. To determine the outflow driving mechanism, we compare the starburst ({\$}L{\_}{\{}*{\}}{\$}) and AGN ({\$}L{\_}{\{}\backslashrm AGN{\}}{\$}) luminosities to the outflowing energy and momentum fluxes, using mid-infrared spectral decomposition to discern {\$}L{\_}{\{}\backslashrm AGN{\}}{\$}. Comparison to other molecular outflows in ULIRGs reveals that outflow properties correlate similarly with {\$}L{\_}{\{}*{\}}{\$} and {\$}L{\_}{\{}\backslashrm IR{\}}{\$} as with {\$}L{\_}{\{}\backslashrm AGN{\}}{\$}, indicating that AGN luminosity alone may not be a good tracer of feedback strength and that a combination of AGN and starburst activity may be driving the most powerful molecular outflows. We also detect the OH 1.667 GHz maser line from both sources and demonstrate its utility in detecting molecular outflows.},
archivePrefix = {arXiv},
arxivId = {1804.03147},
author = {Gowardhan, Avani and Spoon, Henrik and Riechers, Dominik A. and Gonz{\'{a}}lez-Alfonso, Eduardo and Farrah, Duncan and Fischer, Jacqueline and Darling, Jeremy and Fergulio, Chiara and Afonso, Jose and Bizzocchi, Luca},
doi = {10.3847/1538-4357/aabccc},
eprint = {1804.03147},
file = {:home/william/Documents/Papers/Gowardhan{\_}2018{\_}ApJ{\_}859{\_}35.pdf:pdf},
issn = {1538-4357},
journal = {Astrophys. J.},
keywords = {active,evolution,galaxies,galaxies: active,galaxies: evolution,galaxies: sta,interferometric,ism,jets and out fl,molecules,ows,starburst,techniques},
number = {1},
pages = {35},
publisher = {IOP Publishing},
title = {{The Dual Role of Starbursts and Active Galactic Nuclei in Driving Extreme Molecular Outflows}},
url = {http://dx.doi.org/10.3847/1538-4357/aabccc},
volume = {859},
year = {2018}
}
@article{Avery2022,
abstract = {This paper investigates the neutral gas phase of galactic winds via the Na I D{\$}\backslashlambda\backslashlambda 5890,5895{\$}{\{}$\backslash$AA{\}} feature within {\$}z \backslashsim 0.04{\$} MaNGA galaxies, and directly compares their incidence and strength to the ionized winds detected within the same parent sample. We find evidence for neutral outflows in 127 galaxies ({\$}\backslashsim 5{\$} per cent of the analysed line-emitting sample). Na I D winds are preferentially seen in galaxies with dustier central regions and both wind phases are more often found in systems with elevated SFR surface densities, especially when there has been a recent upturn in the star formation activity according to the SFR{\$}{\_}{\{}5Myr{\}}{\$}/SFR{\$}{\_}{\{}800Myr{\}}{\$} parameter. We find the ionized outflow kinematics to be in line with what we measure in the neutral phase. This demonstrates that, despite their small contributions to the total outflow mass budget, there is value to collecting empirical measurements of the ionized wind phase to provide information on the bulk motion in the outflow. Depending on dust corrections applied to the ionized gas diagnostics, the neutral phase has {\$}\backslashsim 1.2 - 1.8{\$} dex higher mass outflow rates ({\$}\backslashdot{\{}M{\}}{\_}{\{}out{\}}{\$}), on average, compared to the ionized phase. We quantify scaling relations between {\$}\backslashdot{\{}M{\}}{\_}{\{}out{\}}{\$} and the strengths of the physical wind drivers (SFR, {\$}L{\_}{\{}AGN{\}}{\$}). Using a radial-azimuthal stacking method, and by considering inclination dependencies, we find results consistent with biconical outflows orthogonal to the disk plane. Our work complements other multi-phase outflow studies in the literature which consider smaller samples, more extreme objects, or proceed via stacking of larger samples.},
archivePrefix = {arXiv},
arxivId = {2201.08079},
author = {Avery, Charlotte and Wuyts, Stijn and Schreiber, Natascha M. F{\"{o}}rster and Villforth, Carolin and Bertemes, Caroline and Hamer, Stephen L. and Sharma, Raman and Toshikawa, Jun and Zhang, Junkai},
eprint = {2201.08079},
file = {:home/william/Documents/Papers/2201.08079.pdf:pdf},
keywords = {evolution,galaxies,ism,jets and outflows,kinematics and dynamics},
number = {January},
pages = {1--14},
title = {{Cool outflows in MaNGA: a systematic study and comparison to the warm phase}},
url = {http://arxiv.org/abs/2201.08079},
volume = {14},
year = {2022}
}
@article{1390a,
abstract = {New results from th Pierre Auger Observatory could narrow the search for the origin of ultrahigh-energy cosmic rays},
author = {{Soebur Razzaque}},
file = {:home/william/Documents/Papers/UHeCR-SBs.pdf:pdf},
pages = {145},
title = {{The Anatomy of Ultrahigh-Energy Cosmic Rays}},
volume = {13},
year = {2020}
}
@article{Costa2020,
abstract = {We present a new implementation for active galactic nucleus (AGN) feedback through small-scale, ultra-fast winds in the moving-mesh hydrodynamic code AREPO. The wind is injected by prescribing mass, momentum and energy fluxes across a spherical boundary centred on a supermassive black hole according to available constraints for accretion disc winds. After sweeping-up a mass equal to their own, small-scale winds thermalise, powering energy-driven outflows with dynamics, structure and cooling properties in excellent agreement with those of analytic wind solutions. Momentum-driven solutions do not easily occur, because the Compton cooling radius is usually much smaller than the free-expansion radius of the small-scale winds. Through various convergence tests, we demonstrate that our implementation yields wind solutions which are well converged down to the typical resolution achieved in cosmological simulations. We test our model in hydrodynamic simulations of isolated Milky Way - mass galaxies. Above a critical AGN luminosity, initially spherical, small-scale winds power bipolar, energy-driven super-winds that break out of the galactic nucleus, flowing at speeds {\$}{\textgreater} 1000 \backslashrm \backslash, km \backslash, s{\^{}}{\{}-1{\}}{\$} out to {\$}\backslashsim 10 \backslash, \backslashrm kpc{\$}. These energy-driven outflows result in moderate, but long-term, reduction in star formation, which becomes more pronounced for higher AGN luminosities and faster small-scale winds. Suppression of star formation proceeds through a rapid mode that involves the removal of the highest-density, nuclear gas and through a slower mode that effectively halts halo gas accretion. Our new implementation makes it possible to model AGN-driven winds in a physically meaningful and validated way in simulations of galaxy evolution, the interstellar medium and black hole accretion flows.},
archivePrefix = {arXiv},
arxivId = {2006.05997},
author = {Costa, Tiago and Pakmor, R{\"{u}}diger and Springel, Volker},
eprint = {2006.05997},
file = {:home/william/Documents/Papers/2006.05997.pdf:pdf},
keywords = {evolution,galaxies,hydrodynamics,methods,numerical,quasars,shock waves,supermassive black holes},
number = {June},
pages = {1--29},
title = {{Powering galactic super-winds with small-scale AGN winds}},
url = {http://arxiv.org/abs/2006.05997},
volume = {29},
year = {2020}
}
@article{KennicuttJr.1998,
abstract = {Measurements of H-alpha, HI, and CO distributions in 61 normal spiral galaxies are combined with published far-infrared and CO observations of 36 infrared-selected starburst galaxies, in order to study the form of the global star formation law, over the full range of gas densities and star formation rates (SFRs) observed in galaxies. The disk-averaged SFRs and gas densities for the combined sample are well represented by a Schmidt law with index N = 1.4+-0.15. The Schmidt law provides a surprisingly tight parametrization of the global star formation law, extending over several orders of magnitude in SFR and gas density. An alternative formulation of the star formation law, in which the SFR is presumed to scale with the ratio of the gas density to the average orbital timescale, also fits the data very well. Both descriptions provide potentially useful "recipes" for modelling the SFR in numerical simulations of galaxy formation and evolution.},
archivePrefix = {arXiv},
arxivId = {astro-ph/9712213},
author = {{Kennicutt, Jr.}, Robert C.},
doi = {10.1086/305588},
eprint = {9712213},
file = {:home/william/Documents/Papers/Kennicutt,{\_}Jr.{\_}1998{\_}ApJ{\_}498{\_}541.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
number = {2},
pages = {541--552},
primaryClass = {astro-ph},
title = {{The Global Schmidt Law in Star‐forming Galaxies}},
volume = {498},
year = {1998}
}
@article{Morganti2021a,
abstract = {Ranging from a few pc to hundreds of kpc in size, radio jets have, during their evolution, an impact on their gaseous environment on a large range of scales. While their effect on larger scales is well established, it is now becoming clear that they can also strongly affect the interstellar medium (ISM) inside the host galaxy. Particularly important is the initial phase ((Formula presented.) years) of the evolution of the radio jet, when they expand into the inner few kpc of the host galaxy. Here we report on results obtained for a representative group of young radio galaxies using the cold molecular gas as a tracer of jet-ISM interactions. The sensitivity and high spatial resolution of ALMA and NOEMA are ideal to study the details of this process. In many objects, we find massive molecular outflows driven by the plasma jet, even in low-power radio sources. However, the observed outflows are limited to the circumnuclear regions and only a small fraction of the ISM is leaving the galaxy. Beyond this region, the impact of the jet seems to change. Fast outflows are replaced by a milder expansion driven by the expanding cocoon created by the jet-ISM interaction, resulting in dispersing and heating the ISM. These findings are in line with predictions from simulations of jets interacting with a clumpy medium and suggest a more complex view of the impact of AGN than presently implemented in cosmological simulations.},
archivePrefix = {arXiv},
arxivId = {2201.04157},
author = {Morganti, Raffaella and Oosterloo, Tom and Murthy, Suma and Tadhunter, Clive},
doi = {10.1002/asna.20210037},
eprint = {2201.04157},
file = {:home/william/Documents/Papers/2201.04157.pdf:pdf},
issn = {15213994},
journal = {Astron. Nachrichten},
keywords = {1 impact of,active,from small to large,galaxies,ism,jets and outflow,radio jets,radio lines,scales,young},
number = {9-10},
pages = {1135--1139},
title = {{The impact of young radio jets traced by cold molecular gas}},
volume = {342},
year = {2021a}
}
@article{1975PASJ...27..533M,
author = {Miyamoto, M and Nagai, R},
file = {:home/william/Documents/Papers/1975PASJ...27..533M.pdf:pdf},
journal = {pasj},
keywords = {Astronomical Models,Density Distribution,Functions (Mathematics),Galactic Structure,Globular Clusters,Gravitational Effects,Mass Distribution,Mathematical Models,Milky Way Galaxy,Potential Theory,Three Dimensional Models},
pages = {533--543},
title = {{Three-dimensional models for the distribution of mass in galaxies}},
volume = {27},
year = {1975}
}
@inproceedings{DeGouveiaDalPino2005,
abstract = {Highly collimated supersonic jets and less collimated outflows are observed to emerge from a wide variety of astrophysical objects. They are seen in young stellar objects (YSOs), proto-planetary nebulae, compact objects (like galactic black holes or microquasars, and X-ray binary stars), and in the nuclei of active galaxies (AGNs). Despite their different physical scales (in size, velocity, and amount of energy transported), they have strong morphological similarities. What physics do they share? These systems are either hydrodynamic or magnetohydrodynamic (MHD) in nature and are, as such, governed by non-linear equations. While theoretical models helped us to understand the basic physics of these objects, numerical simulations have been allowing us to go beyond the one-dimensional, steady-state approach extracting vital information. In this lecture, the formation, structure, and evolution of the jets are reviewed with the help of observational information, MHD and purely hydrodynamical modeling, and numerical simulations. Possible applications of the models particularly to YSOs and AGN jets are addressed. {\textcopyright} 2005 COSPAR. Published by Elsevier Ltd. All rights reserved.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0406319},
author = {{De Gouveia Dal Pino}, Elisabete M.},
booktitle = {Adv. Sp. Res.},
doi = {10.1016/j.asr.2005.03.145},
eprint = {0406319},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/De Gouveia Dal Pino - 2005 - Astrophysical jets and outflows.pdf:pdf},
issn = {02731177},
keywords = {Accretion disks,Active galactic nuclei,Astrophysical jets,Astrophysics,Black holes,Microquasars,Young stellar objects},
number = {5},
pages = {908--924},
primaryClass = {astro-ph},
title = {{Astrophysical jets and outflows}},
volume = {35},
year = {2005}
}
@article{May2020,
abstract = {We report near-infrared integral field spectroscopic observations of the active galactic nucleus NGC 4151 with archive data from the NIFS-Gemini North Telescope. We have selected best-seeing observations (≲0.3 arcsec) that, allied to our methodology of image processing techniques, show structures with spatial resolution comparable to those of the HST. The intricate outflow of NGC 4151 is revisited in light of the results found for NGC 1068, in a previous work, and a very similar dynamic is found: the low-velocity [Fe ii] emission depicts the glowing walls of an hourglass structure, while the high-velocity gas fills its volume. From this finding, we show that the misalignment between the jet and the NLR is not a projection effect, as previously thought. A molecular outflow is detected for the first time in this galaxy and, just like in NGC 1068, the transition between the molecular and the ionized gas phases comes from the fragmentation of molecular cavity walls into bullets of ionized gas exposed to the central source. Furthermore, it is suggestive that the same geometrical dichotomy between the cones seen in NGC 1068 is found here, with one side, where the cavity is disrupted by the AGN, being more extended than the other. Finally, a new spatial correlation between the high-velocity [Fe ii] and the soft X-ray emission of [Ne ix] is found, which is unexpected given the difference between their ionization potentials.},
archivePrefix = {arXiv},
arxivId = {2007.07374},
author = {May, D. and Steiner, J. E. and Menezes, R. B. and Williams, D R A and Wang, J.},
doi = {10.1093/mnras/staa1545},
eprint = {2007.07374},
file = {:home/william/Documents/Papers/2007.07374.pdf:pdf},
issn = {0035-8711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: Seyfert,Galaxies: individual: (NGC 4151),ISM,ISM: jets and outflows,ISM: kinematics and dynamics,Nuclei,Techniques: spectroscopic},
month = {aug},
number = {2},
pages = {1488--1516},
title = {{The nuclear architecture of NGC 4151: on the path toward a universal outflow mechanism in light of NGC 1068}},
url = {https://academic.oup.com/mnras/article/496/2/1488/5851281},
volume = {496},
year = {2020}
}
@article{Veilleux2017,
abstract = {In Tombesi et al. (2015), we reported the first direct evidence for a quasar accretion disk wind driving a massive molecular outflow. The target was F11119+3257, an ultraluminous infrared galaxy (ULIRG) with unambiguous type-1 quasar optical broad emission lines. The energetics of the accretion disk wind and molecular outflow were found to be consistent with the predictions of quasar feedback models where the molecular outflow is driven by a hot energy-conserving bubble inflated by the inner quasar accretion disk wind. However, this conclusion was uncertain because the energetics were estimated from the optically thick OH 119 um transition profile observed with Herschel. Here, we independently confirm the presence of the molecular outflow in F11119+3257, based on the detection of broad wings in the CO(1-0) profile derived from ALMA observations. The broad CO(1-0) line emission appears to be spatially extended on a scale of at least {\~{}}7 kpc from the center. Mass outflow rate, momentum flux, and mechanical power of (80-200) R{\_}7{\^{}}{\{}-1{\}} M{\_}sun/yr, (1.5-3.0) R{\_}7{\^{}}{\{}-1{\}} L{\_}AGN/c, and (0.15-0.40){\%} R{\_}7{\^{}}{\{}-1{\}} L{\_}AGN are inferred from these data, assuming a CO-to-H{\_}2 conversion factor appropriate for a ULIRG (R{\_}7 is the radius of the outflow normalized to 7 kpc and L{\_}AGN is the AGN luminosity). These rates are time-averaged over a flow time scale of 7x10{\^{}}6 yrs. They are similar to the OH-based rates time-averaged over a flow time scale of 4x10{\^{}}5 yrs, but about a factor 4 smaller than the local ("instantaneous"; {\textless}10{\^{}}5 yrs) OH-based estimates cited in Tombesi et al. The implications of these new results are discussed in the context of time-variable quasar-mode feedback and galaxy evolution. The need for an energy-conserving bubble to explain the molecular outflow is also re-examined.},
archivePrefix = {arXiv},
arxivId = {1706.00443},
author = {Veilleux, S. and Bolatto, A. and Tombesi, F. and Melendez, M. and Sturm, E. and Gonzalez-Alfonso, E. and Fischer, J. and Rupke, D. S. N.},
doi = {10.3847/1538-4357/aa767d},
eprint = {1706.00443},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Veilleux et al. - 2017 - Quasar Feedback in the Ultraluminous Infrared Galaxy F111193257 Connecting the Accretion Disk Wind with the Lar.pdf:pdf},
issn = {1538-4357},
journal = {Astrophys. J.},
keywords = {3257,active,evolution,f11119,galaxies,galaxies: active,galaxies: evolution,ISM: jets and,general,individual,ism,jets and out fl,ows,quasars},
number = {1},
pages = {18},
publisher = {IOP Publishing},
title = {{Quasar Feedback in the Ultraluminous Infrared Galaxy F11119+3257: Connecting the Accretion Disk Wind with the Large-Scale Molecular Outflow}},
url = {http://arxiv.org/abs/1706.00443{\%}0Ahttp://dx.doi.org/10.3847/1538-4357/aa767d},
volume = {843},
year = {2017}
}
@article{Tully1977,
abstract = {• גרינבלט, י. (2012). ענף הקיווי: תמונת מצב 2012, עלון הנוטע שה“מ, מחוז צפון, משרד החקלאות.},
author = {Tully, R. Brent and Fisher, J. Richard},
file = {:home/william/Documents/Papers/[Tully, Fisher]-A New Method to Determine Distance to Galaxies.pdf:pdf},
journal = {Astron. Astrophys.},
pages = {661--673},
title = {{A New Method of Determining Distances to Galaxies}},
volume = {54},
year = {1977}
}
@article{Bell1978,
abstract = {It is shown that charged particles can be accelerated to high energies in astrophysical shock fronts. Fast particles are prevented from streaming away upstream of a shock front by scattering off Alfven waves which they themselves generate. This scattering confines the particles to the region around the shock and results in first-order Fermi acceleration due to the particles crossing the shock many times. The consequent energy spectrum is a power law with an index close to that observed for galactic cosmic rays. The discussion relates to particles which are already relativistic, and their initial acceleration from thermal energies is not considered.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Bell, A. R.},
doi = {10.1093/mnras/182.3.443},
eprint = {arXiv:1011.1669v3},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Bell - 1978 - The acceleration of cosmic rays in shock fronts - II.pdf:pdf},
isbn = {9780874216561},
issn = {0035-8711},
journal = {Mon. Not. R. Astron. Soc.},
number = {3},
pages = {443--455},
pmid = {25052830},
title = {{The acceleration of cosmic rays in shock fronts - II}},
url = {https://academic.oup.com/mnras/article-lookup/doi/10.1093/mnras/182.3.443},
volume = {182},
year = {1978}
}
@article{Yang2021,
abstract = {In radio-loud active galactic nuclei (AGNs), ultra-fast outflows (UFOs) were detected at the inclination angle of ∼10°–70° away from jets. Except for the inclination angle of UFOs, the UFOs in radio-loud AGNs have similar properties to that in radio-quiet AGNs. The UFOs with such low inclination cannot be explained in the line-force mechanism. The magnetic-driving mechanism is suggested to explain the UFOs based on a self-similar solution with radiative transfer calculations. However, the energetics of self-similar solution need to be further confirmed based on numerical simulations. To understand the formation and acceleration of UFOs in radio-loud AGNs, this paper presents a model of the disk winds driven by both line force and magnetic field and implements numerical simulations. Initially, a magnetic field is set to 10 times stronger than the gas pressures at the disk surface. Simulation results imply that the disk winds driven by both line force and magnetic field could describe the properties of UFOs in radio-loud AGNs. Pure magnetohydrodynamics (MHDs) simulation is also implemented. When the initial conditions are the same, the hybrid models of magnetic fields and line force are more helpful to form UFOs than the pure MHD models. It is worth studying the case of a stronger magnetic field to confirm this result.},
archivePrefix = {arXiv},
arxivId = {2110.10954},
author = {Yang, Xiao-Hong},
doi = {10.3847/1538-4357/ac3236},
eprint = {2110.10954},
file = {:home/william/Documents/Papers/Yang{\_}2021{\_}ApJ{\_}922{\_}262.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
keywords = {Supermassive black holes,Radio active galactic nuc},
number = {2},
pages = {262},
publisher = {IOP Publishing},
title = {{Magnetohydrodynamic Winds Driven by Line Force from the Standard Thin Disk around Supermassive Black Holes: II. A Possible Model for Ultra-fast Outflows in Radio-loud AGNs}},
url = {http://dx.doi.org/10.3847/1538-4357/ac3236},
volume = {922},
year = {2021}
}
@article{Ponti2019,
abstract = {Evidence has mounted in recent decades that outflows of matter and energy from the central few parsecs of our Galaxy have shaped the observed structure of the Milky Way on a variety of larger scales1. On scales of 15 parsecs, the Galactic Centre has bipolar lobes that can be seen in both the X-ray and radio parts of the spectrum2,3, indicating broadly collimated outflows from the centre, directed perpendicular to the Galactic plane. On larger scales, approaching the size of the Galaxy itself, $\gamma$-ray observations have revealed the so-called ‘Fermi bubble' features4, implying that our Galactic Centre has had a period of active energy release leading to the production of relativistic particles that now populate huge cavities on both sides of the Galactic plane. The X-ray maps from the ROSAT all-sky survey show that the edges of these cavities close to the Galactic plane are bright in X-rays4–6. At intermediate scales (about 150 parsecs), radio astronomers have observed the Galactic Centre lobe, an apparent bubble of emission seen only at positive Galactic latitudes7,8, but again indicative of energy injection from near the Galactic Centre. Here we report prominent X-ray structures on these intermediate scales (hundreds of parsecs) above and below the plane, which appear to connect the Galactic Centre region to the Fermi bubbles. We propose that these structures, which we term the Galactic Centre ‘chimneys', constitute exhaust channels through which energy and mass, injected by a quasi-continuous train of episodic events at the Galactic Centre, are transported from the central few parsecs to the base of the Fermi bubbles4.},
author = {Ponti, G. and Hofmann, F. and Churazov, E. and Morris, M. R. and Haberl, F. and Nandra, K. and Terrier, R. and Clavel, M. and Goldwurm, A.},
doi = {10.1038/s41586-019-1009-6},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ponti et al. - 2019 - An X-ray chimney extending hundreds of parsecs above and below the Galactic Centre.pdf:pdf},
issn = {14764687},
journal = {Nature},
number = {7748},
pages = {347--350},
publisher = {Springer US},
title = {{An X-ray chimney extending hundreds of parsecs above and below the Galactic Centre}},
url = {http://dx.doi.org/10.1038/s41586-019-1009-6},
volume = {567},
year = {2019}
}
@article{Woo2020,
abstract = {We investigate the connection between ionized gas outflows and star formation activity using a large sample of type 1 and 2 AGNs with far-IR detections or star formation rate (SFR) estimates. The strength of ionized gas outflows, measured by the velocity dispersion and velocity shift of the [O iii] emission line, clearly shows a correlation with SFR. The connection between specific star formation rate (sSFR) and [O iii] gas velocity dispersion indicates that AGNs with stronger outflows are hosted by galaxies with higher SFR. Compared to star-forming galaxies in the main sequence, both type 1 and type 2 AGNs show sSFR similar to that of non-AGN galaxies, indicating no instantaneous AGN feedback, while sSFR is higher (lower) for AGNs with stronger (weaker) outflows than that of main sequence galaxies. These results are consistent with a delayed AGN feedback scenario. However, it is also possible that a decease/increase of gas fraction may cause the correlation without AGN feedback. Subject headings: galaxies: active — galaxies: kinematics and dynamics},
archivePrefix = {arXiv},
arxivId = {2008.04919},
author = {Woo, Jong Hak and Son, Donghoon and Rakshit, Suvendu},
doi = {10.3847/1538-4357/abad97},
eprint = {2008.04919},
file = {:home/william/Documents/Papers/Woo{\_}2020{\_}ApJ{\_}901{\_}66.pdf:pdf},
issn = {15384357},
journal = {arXiv},
title = {{The correlation of outflow kinematics with star formation rate - Gas outflows in AGNs. VI}},
volume = {66},
year = {2020}
}
@article{Cheung2016,
abstract = {Quiescent galaxies with little or no ongoing star formation dominate the galaxy population above {\$}M{\_}{\{}*{\}}\backslashsim 2 \backslashtimes 10{\^{}}{\{}10{\}}{\~{}}M{\_}{\{}\backslashodot{\}}{\$}, where their numbers have increased by a factor of {\$}\backslashsim25{\$} since {\$}z\backslashsim2{\$}. Once star formation is initially shut down, perhaps during the quasar phase of rapid accretion onto a supermassive black hole, an unknown mechanism must remove or heat subsequently accreted gas from stellar mass loss or mergers that would otherwise cool to form stars. Energy output from a black hole accreting at a low rate has been proposed, but observational evidence for this in the form of expanding hot gas shells is indirect and limited to radio galaxies at the centers of clusters, which are too rare to explain the vast majority of the quiescent population. Here we report bisymmetric emission features co-aligned with strong ionized gas velocity gradients from which we infer the presence of centrally-driven winds in typical quiescent galaxies that host low-luminosity active nuclei. These galaxies are surprisingly common, accounting for as much as {\$}10\backslash{\%}{\$} of the population at {\$}M{\_}* \backslashsim 2 \backslashtimes 10{\^{}}{\{}10{\}}{\~{}} M{\_}{\{}\backslashodot{\}}{\$}. In a prototypical example, we calculate that the energy input from the galaxy's low-level active nucleus is capable of driving the observed wind, which contains sufficient mechanical energy to heat ambient, cooler gas (also detected) and thereby suppress star formation.},
archivePrefix = {arXiv},
arxivId = {1605.07626},
author = {Cheung, Edmond and Bundy, Kevin and Cappellari, Michele and Peirani, S{\'{e}}bastien and Rujopakarn, Wiphu and Westfall, Kyle and Yan, Renbin and Bershady, Matthew and Greene, Jenny E and Heckman, Timothy M and Drory, Niv and Law, David R and Masters, Karen L and Thomas, Daniel and Wake, David A and Weijmans, Anne Marie and Rubin, Kate and Belfiore, Francesco and Vulcani, Benedetta and Chen, Yan Mei and Zhang, Kai and Gelfand, Joseph D. and Bizyaev, Dmitry and Roman-Lopes, A. and Schneider, Donald P.},
doi = {10.1038/nature18006},
eprint = {1605.07626},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Cheung et al. - 2016 - Suppressing star formation in quiescent galaxies with supermassive black hole winds.pdf:pdf},
isbn = {1476-4687 (Electronic)$\backslash$r0028-0836 (Linking)},
issn = {14764687},
journal = {Nature},
number = {7604},
pages = {504--508},
pmid = {27225122},
publisher = {Nature Publishing Group},
title = {{Suppressing star formation in quiescent galaxies with supermassive black hole winds}},
url = {http://dx.doi.org/10.1038/nature18006},
volume = {533},
year = {2016}
}
@article{Young1991,
author = {Young, J. S. and Scoville, N. Z.},
doi = {10.1146/annurev.aa.29.090191.003053},
file = {:home/william/Documents/Papers/annurev.aa.29.090191.003053.pdf:pdf},
issn = {00664146},
journal = {Annu. Rev. Astron. Astrophys.},
keywords = {Galaxy evolution,Hubble sequence,Interstellar medium,Star formation},
number = {1},
pages = {581--625},
title = {{Molecular gas in galaxies}},
volume = {29},
year = {1991}
}
@article{Batista2021,
abstract = {One of the most promising ways to probe intergalactic magnetic fields (IGMFs) is through gamma rays produced in electromagnetic cascades initiated by high-energy gamma rays or cosmic rays in the intergalactic space. Because the charged component of the cascade is sensitive to magnetic fields, gamma-ray observations of distant objects such as blazars can be used to constrain IGMF properties. Ground-based and space-borne gamma-ray telescopes deliver spectral, temporal, and angular information of high-energy gamma-ray sources, which carries imprints of the intervening magnetic fields. This provides insights into the nature of the processes that led to the creation of the first magnetic fields and into the phenomena that impacted their evolution. Here we provide a detailed description of how gamma-ray observations can be used to probe cosmic magnetism. We review the current status of this topic and discuss the prospects for measuring IGMFs with the next generation of gamma-ray observatories.},
archivePrefix = {arXiv},
arxivId = {2105.12020},
author = {Batista, Rafael Alves and Saveliev, Andrey},
eprint = {2105.12020},
file = {:home/william/Documents/Papers/2105.12020.pdf:pdf},
keywords = {electromagnetic cascades,high-energy gamma rays,intergalactic magnetic fields},
pages = {1--55},
title = {{The Gamma-Ray Window to Intergalactic Magnetism}},
url = {http://arxiv.org/abs/2105.12020},
year = {2021}
}
@article{1995ApJ...438...62W,
author = {Wilson, A.{\~{}}S. and Colbert, E.{\~{}}J.{\~{}}M.},
doi = {10.1086/175054},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Wilson, Colbert - 1995 - The difference between radio-loud and radio-quiet active galaxies.pdf:pdf},
journal = {Apj},
keywords = {Active Galactic Nuclei,Black Holes (Astronomy),Cosmology,Interacting Galaxies,Luminosity,Quasars,Radio Astronomy,Radio Jets (Astronomy)},
pages = {62--71},
title = {{The difference between radio-loud and radio-quiet active galaxies}},
volume = {438},
year = {1995}
}
@article{Abbett2012,
abstract = {We present a series of numerical simulations ofthe quiet–Sun plasma threaded by magnetic fields that extend from the upper convection zone into the low corona.We discuss an efficient, simplified approximationto thephysics of optically thick radiative transport through the surface layers, and investigate the effects of convective turbulence on the magnetic structure of the Sun's atmosphere in an initially unipolar (open field) region. We find that the net Poynting flux below the surface is on average directed toward the interior, while in the photosphere and chromosphere the net flow of electromagnetic energy is outward into the solar corona. Overturning convective motions between these layers driven by rapid radiative cooling appears to be the source of energy for the oppositely directed fluxes of electromagnetic energy.},
archivePrefix = {arXiv},
arxivId = {arXiv:1102.1035v1},
author = {Abbett, W. P. and Fisher, G. H.},
doi = {10.1007/s11207-011-9817-3},
eprint = {arXiv:1102.1035v1},
file = {:home/william/Documents/Papers/1102.1035.pdf:pdf},
isbn = {9781461437611},
journal = {Sol. Flare Magn. Fields Plasmas},
keywords = {Convection,Corona,Magnetic fields,Photosphere,Radiative transfer},
number = {February 2011},
pages = {3--20},
title = {{Radiative coolingin MHD models of the quiet sun convection zone and corona}},
year = {2012}
}
@article{Jarvis2020,
abstract = {We use a sample of powerful z ≈ 0.1 type 2 quasars ('obscured'; log [LAGN/erg s-1] ≳ 45), which host kpc-scale ionized outflows and jets, to identify possible signatures of AGN feedback on the total molecular gas reservoirs of their host galaxies. Specifically, we present Atacama Pathfinder EXperiment (APEX) observations of the CO(2-1) transition for nine sources and the CO(6-5) for a subset of three. We find that the majority of our sample reside in starburst galaxies (average specific star formation rates-sSFR-of 1.7 Gyr-1), with the seven CO-detected quasars also having large molecular gas reservoirs (average Mgas = 1.3 × 1010 M⊙), even though we had no pre-selection on the star formation or molecular gas properties. Despite the presence of quasars and outflows, we find that the molecular gas fractions (Mgas/M* = 0.1-1.2) and depletion times (Mgas/SFR = 0.16-0.95 Gyr) are consistent with those expected for the overall galaxy population with matched stellar masses and sSFRs. Furthermore, for at least two of the three targets with the required measurements, the CO(6-5)/CO(2-1) emission-line ratios are consistent with star formation dominating the CO excitation over this range of transitions. The targets in our study represent a gas-rich phase of galaxy evolution with simultaneously high levels of star formation and nuclear activity; furthermore, the jets and outflows do not have an immediate appreciable impact on the global molecular gas reservoirs.},
archivePrefix = {arXiv},
arxivId = {2007.10351},
author = {Jarvis, M. E. and Harrison, C. M. and Mainieri, V. and {Calistro Rivera}, G. and Jethwa, P. and Zhang, Z. Y. and Alexander, D. M. and Circosta, C. and Costa, T. and {De Breuck}, C. and Kakkad, D. and Kharb, P. and Lansbury, G. B. and Thomson, A. P.},
doi = {10.1093/mnras/staa2196},
eprint = {2007.10351},
file = {:home/william/Documents/Papers/2007.10351.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {ISM: Jets and outflows,ISM: Molecules,galaxies: Active,galaxies: Evolution,galaxies: General,galaxies: ISM},
number = {2},
pages = {1560--1575},
title = {{High molecular gas content and star formation rates in local galaxies that host quasars, outflows, and jets}},
volume = {498},
year = {2020}
}
@article{2014A&ARv..22...73F,
archivePrefix = {arXiv},
arxivId = {astro-ph.HE/1407.7615},
author = {Falomo, R and Pian, E and Treves, A},
doi = {10.1007/s00159-014-0073-z},
eprint = {1407.7615},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Falomo, Pian, Treves - 2014 - An optical view of BL Lacertae objects.pdf:pdf},
keywords = {BL Lacertae objects: general,Galaxies: active,Galaxies: jets,Galaxies: nuclei,Quasars: supermassive black holes,Radiation mechanisms: non-thermal},
pages = {73},
primaryClass = {astro-ph.HE},
title = {{An optical view of BL Lacertae objects}},
volume = {22},
year = {2014}
}
@article{Grissom2014,
abstract = {The electron scattering optical depth constraints on reionization suggest that there may be other sources that contribute to the ionization of hydrogen aside from observable star forming galaxies. Often the calculated value of the electron scattering optical depth, $\tau$es, falls below the measurements derived from observations of the cosmic microwave background, or an assumption about non-observable sources must be made in order to reach agreement. Here, we calculate the hydrogen ionization fraction as a function of redshift and the electron scattering optical depth from both galaxies and active galactic nuclei (AGN) factoring in the secondary collisional ionizations from the AGN X-ray emission. In this paper we use the most current determination of the evolving hard X-ray luminosity function and extrapolate its evolution beyond z = 6. The AGN spectral energy distributions include both UV and X-ray ionizing photons. To search for the largest possible effect, all AGNs are assumed to have $\lambda$Edd = 1.0 and to be completely unobscured. The results show that AGNs produce a perturbative effect on the reionization of hydrogen and they remain in agreement with current constraints. Our calculations find the epoch of reionization still ends at z ≈ 6 and only increases the electron scattering optical depth by {\~{}}2.3{\%} under ideal conditions. This can only be moderately increased by assuming a constant black hole mass of MBH = 105 M{\^{a}}{\v{S}}™. As a result, we conclude that there is a need for other sources beyond observable galaxies and AGNs that contribute to the reionization of hydrogen at z {\textgreater} 6. {\textcopyright} 2014 ESO.},
author = {Grissom, R. L. and Ballantyne, D. R. and Wise, J. H.},
doi = {10.1051/0004-6361/201322637},
file = {:home/william/Documents/Papers/aa22637-13.pdf:pdf},
issn = {00046361},
journal = {Astron. Astrophys.},
keywords = {Dark ages reionization first stars,Galaxies: active,Galaxies: evolution,Quasars: general},
pages = {1--5},
title = {{On the contribution of active galactic nuclei to reionization}},
volume = {561},
year = {2014}
}
@article{Pierce1992,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Pierce, Michael J and {R. Brent Tully}},
eprint = {arXiv:1011.1669v3},
file = {:home/william/Documents/Papers/[Pierce and Tully]-Luminosity-Line width  Relations and the intergalactic  Distance Scale. I.Absolute Calibration.pdf:pdf},
journal = {J. Chem. Inf. Model.},
keywords = {icle},
pages = {47--55},
title = {{Luminosity-Line width Relations and the Extragalatic Distance Scale. I. Absolute Calibration}},
volume = {387},
year = {1992}
}
@article{Abbott2016,
abstract = {On September 14, 2015 at 09:50:45 UTC the two detectors of the Laser Interferometer Gravitational-Wave Observatory simultaneously observed a transient gravitational-wave signal. The signal sweeps upwards in frequency from 35 to 250 Hz with a peak gravitational-wave strain of 1.0×10−21. It matches the waveform predicted by general relativity for the inspiral and merger of a pair of black holes and the ringdown of the resulting single black hole. The signal was observed with a matched-filter signal-to-noise ratio of 24 and a false alarm rate estimated to be less than 1 event per 203 000 years, equivalent to a significance greater than 5.1$\sigma$. The source lies at a luminosity distance of 410+160−180 Mpc corresponding to a redshift z=0.09+0.03−0.04. In the source frame, the initial black hole masses are 36+5−4M⊙ and 29+4−4M⊙, and the final black hole mass is 62+4−4M⊙, with 3.0+0.5−0.5M⊙c2 radiated in gravitational waves. All uncertainties define 90{\%} credible intervals. These observations demonstrate the existence of binary stellar-mass black hole systems. This is the first direct detection of gravitational waves and the first observation of a binary black hole merger.},
author = {Abbott, B. P. and Abbott, R. and Abbott, T. D. and Abernathy, M. R. and Acernese, F. and Ackley, K. and Adams, C. and Adams, T. and Addesso, P. and Adhikari, R. X. and Adya, V. B. and Affeldt, C. and Agathos, M. and Agatsuma, K. and Aggarwal, N. and Aguiar, O. D. and Aiello, L. and Ain, A. and Ajith, P. and Allen, B. and Allocca, A. and Altin, P. A. and Anderson, S. B. and Anderson, W. G. and Arai, K. and Arain, M. A. and Araya, M. C. and Arceneaux, C. C. and Areeda, J. S. and Arnaud, N. and Arun, K. G. and Ascenzi, S. and Ashton, G. and Ast, M. and Aston, S. M. and Astone, P. and Aufmuth, P. and Aulbert, C. and Babak, S. and Bacon, P. and Bader, M. K.M. and Baker, P. T. and Baldaccini, F. and Ballardin, G. and Ballmer, S. W. and Barayoga, J. C. and Barclay, S. E. and Barish, B. C. and Barker, D. and Barone, F. and Barr, B. and Barsotti, L. and Barsuglia, M. and Barta, D. and Bartlett, J. and Barton, M. A. and Bartos, I. and Bassiri, R. and Basti, A. and Batch, J. C. and Baune, C. and Bavigadda, V. and Bazzan, M. and Behnke, B. and Bejger, M. and Belczynski, C. and Bell, A. S. and Bell, C. J. and Berger, B. K. and Bergman, J. and Bergmann, G. and Berry, C. P.L. and Bersanetti, D. and Bertolini, A. and Betzwieser, J. and Bhagwat, S. and Bhandare, R. and Bilenko, I. A. and Billingsley, G. and Birch, J. and Birney, R. and Birnholtz, O. and Biscans, S. and Bisht, A. and Bitossi, M. and Biwer, C. and Bizouard, M. A. and Blackburn, J. K. and Blair, C. D. and Blair, D. G. and Blair, R. M. and Bloemen, S. and Bock, O. and Bodiya, T. P. and Boer, M. and Bogaert, G. and Bogan, C. and Bohe, A. and Bojtos, P. and Bond, C. and Bondu, F. and Bonnand, R. and Boom, B. A. and Bork, R. and Boschi, V. and Bose, S. and Bouffanais, Y. and Bozzi, A. and Bradaschia, C. and Brady, P. R. and Braginsky, V. B. and Branchesi, M. and Brau, J. E. and Briant, T. and Brillet, A. and Brinkmann, M. and Brisson, V. and Brockill, P. and Brooks, A. F. and Brown, D. A. and Brown, D. D. and Brown, N. M. and Buchanan, C. C. and Buikema, A. and Bulik, T. and Bulten, H. J. and Buonanno, A. and Buskulic, D. and Buy, C. and Byer, R. L. and Cabero, M. and Cadonati, L. and Cagnoli, G. and Cahillane, C. and Bustillo, J. Calder{\'{o}}n and Callister, T. and Calloni, E. and Camp, J. B. and Cannon, K. C. and Cao, J. and Capano, C. D. and Capocasa, E. and Carbognani, F. and Caride, S. and Diaz, J. Casanueva and Casentini, C. and Caudill, S. and Cavagli{\`{a}}, M. and Cavalier, F. and Cavalieri, R. and Cella, G. and Cepeda, C. B. and Baiardi, L. Cerboni and Cerretani, G. and Cesarini, E. and Chakraborty, R. and Chalermsongsak, T. and Chamberlin, S. J. and Chan, M. and Chao, S. and Charlton, P. and Chassande-Mottin, E. and Chen, H. Y. and Chen, Y. and Cheng, C. and Chincarini, A. and Chiummo, A. and Cho, H. S. and Cho, M. and Chow, J. H. and Christensen, N. and Chu, Q. and Chua, S. and Chung, S. and Ciani, G. and Clara, F. and Clark, J. A. and Cleva, F. and Coccia, E. and Cohadon, P. F. and Colla, A. and Collette, C. G. and Cominsky, L. and Constancio, M. and Conte, A. and Conti, L. and Cook, D. and Corbitt, T. R. and Cornish, N. and Corsi, A. and Cortese, S. and Costa, C. A. and Coughlin, M. W. and Coughlin, S. B. and Coulon, J. P. and Countryman, S. T. and Couvares, P. and Cowan, E. E. and Coward, D. M. and Cowart, M. J. and Coyne, D. C. and Coyne, R. and Craig, K. and Creighton, J. D.E. and Creighton, T. D. and Cripe, J. and Crowder, S. G. and Cruise, A. M. and Cumming, A. and Cunningham, L. and Cuoco, E. and Canton, T. Dal and Danilishin, S. L. and D'Antonio, S. and Danzmann, K. and Darman, N. S. and {Da Silva Costa}, C. F. and Dattilo, V. and Dave, I. and Daveloza, H. P. and Davier, M. and Davies, G. S. and Daw, E. J. and Day, R. and De, S. and Debra, D. and Debreczeni, G. and Degallaix, J. and {De Laurentis}, M. and Del{\'{e}}glise, S. and {Del Pozzo}, W. and Denker, T. and Dent, T. and Dereli, H. and Dergachev, V. and Derosa, R. T. and {De Rosa}, R. and Desalvo, R. and Dhurandhar, S. and D{\'{i}}az, M. C. and {Di Fiore}, L. and {Di Giovanni}, M. and {Di Lieto}, A. and {Di Pace}, S. and {Di Palma}, I. and {Di Virgilio}, A. and Dojcinoski, G. and Dolique, V. and Donovan, F. and Dooley, K. L. and Doravari, S. and Douglas, R. and Downes, T. P. and Drago, M. and Drever, R. W.P. and Driggers, J. C. and Du, Z. and Ducrot, M. and Dwyer, S. E. and Edo, T. B. and Edwards, M. C. and Effler, A. and Eggenstein, H. B. and Ehrens, P. and Eichholz, J. and Eikenberry, S. S. and Engels, W. and Essick, R. C. and Etzel, T. and Evans, M. and Evans, T. M. and Everett, R. and Factourovich, M. and Fafone, V. and Fair, H. and Fairhurst, S. and Fan, X. and Fang, Q. and Farinon, S. and Farr, B. and Farr, W. M. and Favata, M. and Fays, M. and Fehrmann, H. and Fejer, M. M. and Feldbaum, D. and Ferrante, I. and Ferreira, E. C. and Ferrini, F. and Fidecaro, F. and Finn, L. S. and Fiori, I. and Fiorucci, D. and Fisher, R. P. and Flaminio, R. and Fletcher, M. and Fong, H. and Fournier, J. D. and Franco, S. and Frasca, S. and Frasconi, F. and Frede, M. and Frei, Z. and Freise, A. and Frey, R. and Frey, V. and Fricke, T. T. and Fritschel, P. and Frolov, V. V. and Fulda, P. and Fyffe, M. and Gabbard, H. A.G. and Gair, J. R. and Gammaitoni, L. and Gaonkar, S. G. and Garufi, F. and Gatto, A. and Gaur, G. and Gehrels, N. and Gemme, G. and Gendre, B. and Genin, E. and Gennai, A. and George, J. and Gergely, L. and Germain, V. and Ghosh, Abhirup and Ghosh, Archisman and Ghosh, S. and Giaime, J. A. and Giardina, K. D. and Giazotto, A. and Gill, K. and Glaefke, A. and Gleason, J. R. and Goetz, E. and Goetz, R. and Gondan, L. and Gonz{\'{a}}lez, G. and Castro, J. M.Gonzalez and Gopakumar, A. and Gordon, N. A. and Gorodetsky, M. L. and Gossan, S. E. and Gosselin, M. and Gouaty, R. and Graef, C. and Graff, P. B. and Granata, M. and Grant, A. and Gras, S. and Gray, C. and Greco, G. and Green, A. C. and Greenhalgh, R. J.S. and Groot, P. and Grote, H. and Grunewald, S. and Guidi, G. M. and Guo, X. and Gupta, A. and Gupta, M. K. and Gushwa, K. E. and Gustafson, E. K. and Gustafson, R. and Hacker, J. J. and Hall, B. R. and Hall, E. D. and Hammond, G. and Haney, M. and Hanke, M. M. and Hanks, J. and Hanna, C. and Hannam, M. D. and Hanson, J. and Hardwick, T. and Harms, J. and Harry, G. M. and Harry, I. W. and Hart, M. J. and Hartman, M. T. and Haster, C. J. and Haughian, K. and Healy, J. and Heefner, J. and Heidmann, A. and Heintze, M. C. and Heinzel, G. and Heitmann, H. and Hello, P. and Hemming, G. and Hendry, M. and Heng, I. S. and Hennig, J. and Heptonstall, A. W. and Heurs, M. and Hild, S. and Hoak, D. and Hodge, K. A. and Hofman, D. and Hollitt, S. E. and Holt, K. and Holz, D. E. and Hopkins, P. and Hosken, D. J. and Hough, J. and Houston, E. A. and Howell, E. J. and Hu, Y. M. and Huang, S. and Huerta, E. A. and Huet, D. and Hughey, B. and Husa, S. and Huttner, S. H. and Huynh-Dinh, T. and Idrisy, A. and Indik, N. and Ingram, D. R. and Inta, R. and Isa, H. N. and Isac, J. M. and Isi, M. and Islas, G. and Isogai, T. and Iyer, B. R. and Izumi, K. and Jacobson, M. B. and Jacqmin, T. and Jang, H. and Jani, K. and Jaranowski, P. and Jawahar, S. and Jim{\'{e}}nez-Forteza, F. and Johnson, W. W. and Johnson-Mcdaniel, N. K. and Jones, D. I. and Jones, R. and Jonker, R. J.G. and Ju, L. and Haris, K. and Kalaghatgi, C. V. and Kalogera, V. and Kandhasamy, S. and Kang, G. and Kanner, J. B. and Karki, S. and Kasprzack, M. and Katsavounidis, E. and Katzman, W. and Kaufer, S. and Kaur, T. and Kawabe, K. and Kawazoe, F. and K{\'{e}}f{\'{e}}lian, F. and Kehl, M. S. and Keitel, D. and Kelley, D. B. and Kells, W. and Kennedy, R. and Keppel, D. G. and Key, J. S. and Khalaidovski, A. and Khalili, F. Y. and Khan, I. and Khan, S. and Khan, Z. and Khazanov, E. A. and Kijbunchoo, N. and Kim, C. and Kim, J. and Kim, K. and Kim, Nam Gyu and Kim, Namjun and Kim, Y. M. and King, E. J. and King, P. J. and Kinzel, D. L. and Kissel, J. S. and Kleybolte, L. and Klimenko, S. and Koehlenbeck, S. M. and Kokeyama, K. and Koley, S. and Kondrashov, V. and Kontos, A. and Koranda, S. and Korobko, M. and Korth, W. Z. and Kowalska, I. and Kozak, D. B. and Kringel, V. and Krishnan, B. and Kr{\'{o}}lak, A. and Krueger, C. and Kuehn, G. and Kumar, P. and Kumar, R. and Kuo, L. and Kutynia, A. and Kwee, P. and Lackey, B. D. and Landry, M. and Lange, J. and Lantz, B. and Lasky, P. D. and Lazzarini, A. and Lazzaro, C. and Leaci, P. and Leavey, S. and Lebigot, E. O. and Lee, C. H. and Lee, H. K. and Lee, H. M. and Lee, K. and Lenon, A. and Leonardi, M. and Leong, J. R. and Leroy, N. and Letendre, N. and Levin, Y. and Levine, B. M. and Li, T. G.F. and Libson, A. and Littenberg, T. B. and Lockerbie, N. A. and Logue, J. and Lombardi, A. L. and London, L. T. and Lord, J. E. and Lorenzini, M. and Loriette, V. and Lormand, M. and Losurdo, G. and Lough, J. D. and Lousto, C. O. and Lovelace, G. and L{\"{u}}ck, H. and Lundgren, A. P. and Luo, J. and Lynch, R. and Ma, Y. and Macdonald, T. and Machenschalk, B. and Macinnis, M. and Macleod, D. M. and Maga{\~{n}}a-Sandoval, F. and Magee, R. M. and Mageswaran, M. and Majorana, E. and Maksimovic, I. and Malvezzi, V. and Man, N. and Mandel, I. and Mandic, V. and Mangano, V. and Mansell, G. L. and Manske, M. and Mantovani, M. and Marchesoni, F. and Marion, F. and M{\'{a}}rka, S. and M{\'{a}}rka, Z. and Markosyan, A. S. and Maros, E. and Martelli, F. and Martellini, L. and Martin, I. W. and Martin, R. M. and Martynov, D. V. and Marx, J. N. and Mason, K. and Masserot, A. and Massinger, T. J. and Masso-Reid, M. and Matichard, F. and Matone, L. and Mavalvala, N. and Mazumder, N. and Mazzolo, G. and McCarthy, R. and McClelland, D. E. and McCormick, S. and McGuire, S. C. and McIntyre, G. and McIver, J. and McManus, D. J. and McWilliams, S. T. and Meacher, D. and Meadors, G. D. and Meidam, J. and Melatos, A. and Mendell, G. and Mendoza-Gandara, D. and Mercer, R. A. and Merilh, E. and Merzougui, M. and Meshkov, S. and Messenger, C. and Messick, C. and Meyers, P. M. and Mezzani, F. and Miao, H. and Michel, C. and Middleton, H. and Mikhailov, E. E. and Milano, L. and Miller, J. and Millhouse, M. and Minenkov, Y. and Ming, J. and Mirshekari, S. and Mishra, C. and Mitra, S. and Mitrofanov, V. P. and Mitselmakher, G. and Mittleman, R. and Moggi, A. and Mohan, M. and Mohapatra, S. R.P. and Montani, M. and Moore, B. C. and Moore, C. J. and Moraru, D. and Moreno, G. and Morriss, S. R. and Mossavi, K. and Mours, B. and Mow-Lowry, C. M. and Mueller, C. L. and Mueller, G. and Muir, A. W. and Mukherjee, Arunava and Mukherjee, D. and Mukherjee, S. and Mukund, N. and Mullavey, A. and Munch, J. and Murphy, D. J. and Murray, P. G. and Mytidis, A. and Nardecchia, I. and Naticchioni, L. and Nayak, R. K. and Necula, V. and Nedkova, K. and Nelemans, G. and Neri, M. and Neunzert, A. and Newton, G. and Nguyen, T. T. and Nielsen, A. B. and Nissanke, S. and Nitz, A. and Nocera, F. and Nolting, D. and Normandin, M. E.N. and Nuttall, L. K. and Oberling, J. and Ochsner, E. and O'Dell, J. and Oelker, E. and Ogin, G. H. and Oh, J. J. and Oh, S. H. and Ohme, F. and Oliver, M. and Oppermann, P. and Oram, Richard J. and O'Reilly, B. and O'Shaughnessy, R. and Ott, C. D. and Ottaway, D. J. and Ottens, R. S. and Overmier, H. and Owen, B. J. and Pai, A. and Pai, S. A. and Palamos, J. R. and Palashov, O. and Palomba, C. and Pal-Singh, A. and Pan, H. and Pan, Y. and Pankow, C. and Pannarale, F. and Pant, B. C. and Paoletti, F. and Paoli, A. and Papa, M. A. and Paris, H. R. and Parker, W. and Pascucci, D. and Pasqualetti, A. and Passaquieti, R. and Passuello, D. and Patricelli, B. and Patrick, Z. and Pearlstone, B. L. and Pedraza, M. and Pedurand, R. and Pekowsky, L. and Pele, A. and Penn, S. and Perreca, A. and Pfeiffer, H. P. and Phelps, M. and Piccinni, O. and Pichot, M. and Pickenpack, M. and Piergiovanni, F. and Pierro, V. and Pillant, G. and Pinard, L. and Pinto, I. M. and Pitkin, M. and Poeld, J. H. and Poggiani, R. and Popolizio, P. and Post, A. and Powell, J. and Prasad, J. and Predoi, V. and Premachandra, S. S. and Prestegard, T. and Price, L. R. and Prijatelj, M. and Principe, M. and Privitera, S. and Prix, R. and Prodi, G. A. and Prokhorov, L. and Puncken, O. and Punturo, M. and Puppo, P. and P{\"{u}}rrer, M. and Qi, H. and Qin, J. and Quetschke, V. and Quintero, E. A. and Quitzow-James, R. and Raab, F. J. and Rabeling, D. S. and Radkins, H. and Raffai, P. and Raja, S. and Rakhmanov, M. and Ramet, C. R. and Rapagnani, P. and Raymond, V. and Razzano, M. and Re, V. and Read, J. and Reed, C. M. and Regimbau, T. and Rei, L. and Reid, S. and Reitze, D. H. and Rew, H. and Reyes, S. D. and Ricci, F. and Riles, K. and Robertson, N. A. and Robie, R. and Robinet, F. and Rocchi, A. and Rolland, L. and Rollins, J. G. and Roma, V. J. and Romano, J. D. and Romano, R. and Romanov, G. and Romie, J. H. and Rosi{\'{n}}ska, D. and Rowan, S. and R{\"{u}}diger, A. and Ruggi, P. and Ryan, K. and Sachdev, S. and Sadecki, T. and Sadeghian, L. and Salconi, L. and Saleem, M. and Salemi, F. and Samajdar, A. and Sammut, L. and Sampson, L. M. and Sanchez, E. J. and Sandberg, V. and Sandeen, B. and Sanders, G. H. and Sanders, J. R. and Sassolas, B. and Sathyaprakash, B. S. and Saulson, P. R. and Sauter, O. and Savage, R. L. and Sawadsky, A. and Schale, P. and Schilling, R. and Schmidt, J. and Schmidt, P. and Schnabel, R. and Schofield, R. M.S. and Sch{\"{o}}nbeck, A. and Schreiber, E. and Schuette, D. and Schutz, B. F. and Scott, J. and Scott, S. M. and Sellers, D. and Sengupta, A. S. and Sentenac, D. and Sequino, V. and Sergeev, A. and Serna, G. and Setyawati, Y. and Sevigny, A. and Shaddock, D. A. and Shaffer, T. and Shah, S. and Shahriar, M. S. and Shaltev, M. and Shao, Z. and Shapiro, B. and Shawhan, P. and Sheperd, A. and Shoemaker, D. H. and Shoemaker, D. M. and Siellez, K. and Siemens, X. and Sigg, D. and Silva, A. D. and Simakov, D. and Singer, A. and Singer, L. P. and Singh, A. and Singh, R. and Singhal, A. and Sintes, A. M. and Slagmolen, B. J.J. and Smith, J. R. and Smith, M. R. and Smith, N. D. and Smith, R. J.E. and Son, E. J. and Sorazu, B. and Sorrentino, F. and Souradeep, T. and Srivastava, A. K. and Staley, A. and Steinke, M. and Steinlechner, J. and Steinlechner, S. and Steinmeyer, D. and Stephens, B. C. and Stevenson, S. P. and Stone, R. and Strain, K. A. and Straniero, N. and Stratta, G. and Strauss, N. A. and Strigin, S. and Sturani, R. and Stuver, A. L. and Summerscales, T. Z. and Sun, L. and Sutton, P. J. and Swinkels, B. L. and Szczepa{\'{n}}czyk, M. J. and Tacca, M. and Talukder, D. and Tanner, D. B. and T{\'{a}}pai, M. and Tarabrin, S. P. and Taracchini, A. and Taylor, R. and Theeg, T. and Thirugnanasambandam, M. P. and Thomas, E. G. and Thomas, M. and Thomas, P. and Thorne, K. A. and Thorne, K. S. and Thrane, E. and Tiwari, S. and Tiwari, V. and Tokmakov, K. V. and Tomlinson, C. and Tonelli, M. and Torres, C. V. and Torrie, C. I. and T{\"{o}}yr{\"{a}}, D. and Travasso, F. and Traylor, G. and Trifir{\`{o}}, D. and Tringali, M. C. and Trozzo, L. and Tse, M. and Turconi, M. and Tuyenbayev, D. and Ugolini, D. and Unnikrishnan, C. S. and Urban, A. L. and Usman, S. A. and Vahlbruch, H. and Vajente, G. and Valdes, G. and Vallisneri, M. and {Van Bakel}, N. and {Van Beuzekom}, M. and {Van Den Brand}, J. F.J. and {Van Den Broeck}, C. and Vander-Hyde, D. C. and {Van Der Schaaf}, L. and {Van Heijningen}, J. V. and {Van Veggel}, A. A. and Vardaro, M. and Vass, S. and Vas{\'{u}}th, M. and Vaulin, R. and Vecchio, A. and Vedovato, G. and Veitch, J. and Veitch, P. J. and Venkateswara, K. and Verkindt, D. and Vetrano, F. and Vicer{\'{e}}, A. and Vinciguerra, S. and Vine, D. J. and Vinet, J. Y. and Vitale, S. and Vo, T. and Vocca, H. and Vorvick, C. and Voss, D. and Vousden, W. D. and Vyatchanin, S. P. and Wade, A. R. and Wade, L. E. and Wade, M. and Waldman, S. J. and Walker, M. and Wallace, L. and Walsh, S. and Wang, G. and Wang, H. and Wang, M. and Wang, X. and Wang, Y. and Ward, H. and Ward, R. L. and Warner, J. and Was, M. and Weaver, B. and Wei, L. W. and Weinert, M. and Weinstein, A. J. and Weiss, R. and Welborn, T. and Wen, L. and We{\ss}els, P. and Westphal, T. and Wette, K. and Whelan, J. T. and Whitcomb, S. E. and White, D. J. and Whiting, B. F. and Wiesner, K. and Wilkinson, C. and Willems, P. A. and Williams, L. and Williams, R. D. and Williamson, A. R. and Willis, J. L. and Willke, B. and Wimmer, M. H. and Winkelmann, L. and Winkler, W. and Wipf, C. C. and Wiseman, A. G. and Wittel, H. and Woan, G. and Worden, J. and Wright, J. L. and Wu, G. and Yablon, J. and Yakushin, I. and Yam, W. and Yamamoto, H. and Yancey, C. C. and Yap, M. J. and Yu, H. and Yvert, M. and Zadro{\.{z}}ny, A. and Zangrando, L. and Zanolin, M. and Zendri, J. P. and Zevin, M. and Zhang, F. and Zhang, L. and Zhang, M. and Zhang, Y. and Zhao, C. and Zhou, M. and Zhou, Z. and Zhu, X. J. and Zucker, M. E. and Zuraw, S. E. and Zweizig, J.},
doi = {10.1103/PhysRevLett.116.061102},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Wu et al. - 2011 - The theoretical basis of oil-coal co-processing and process optimization.pdf:pdf},
issn = {10797114},
journal = {Phys. Rev. Lett.},
number = {6},
pages = {1--16},
title = {{Observation of gravitational waves from a binary black hole merger}},
volume = {116},
year = {2016}
}
@article{Yesuf2020,
abstract = {Active galactic nucleus (AGN) feedback is expected to impact the amount of cold gas in galaxies by driving strong galactic winds, by preventing external gas inflows, or by changing the thermodynamical state of the gas. We use molecular gas mass estimates based on dust absorption (H{\$}\backslashalpha{\$}/H{\$}\backslashbeta{\$}) to study gas content of large samples of type 2 AGN host galaxies in comparison with inactive galaxies. Using sparse principal component and clustering analysis, we analyze a suite of stellar and structural parameters of {\$}\backslashsim 27,100{\$} face-on, central galaxies at redshift {\$}z = 0.02-0.15{\$} and with stellar mass {\$}M{\_}\backslashstar \backslashapprox 10{\^{}}{\{}10{\}}-2\backslashtimes 10{\^{}}{\{}11{\}}\backslash,M{\_}\backslashodot{\$}. We identify four galaxy groups of similar mass and morphology (mass surface density, velocity dispersion, concentration, and S$\backslash$'{\{}e{\}}rsic index) that can be evolutionarily linked through a lifecycle wherein gas content mediates their star formation rate (SFR) and level of AGN activity. Galaxies first consume their gas mostly through bursty star formation, then enter into a transition phase of intermediate gas richness in which star formation and AGNs coexist, before settling into retirement as gas-poor, quiescent systems with residual levels of AGN activity (LINERs). Strongly accreting black holes (Seyferts) live in gas-rich, star-forming hosts, but neither their gas reservoir nor their ability to form stars seem to be impacted $\backslash$emph{\{}instantaneously{\}} (timescales {\$}\backslashlesssim 0.5{\$}$\backslash$,Gyr) by AGN feedback. Our results are inconsistent with AGN feedback models that predict that central, bulge-dominated, Seyfert-like AGNs in massive galaxies have significantly lower molecular gas fractions compared to inactive galaxies of similar mass, morphology, and SFR.},
archivePrefix = {arXiv},
arxivId = {2007.12026},
author = {Yesuf, Hassen M. and Ho, Luis C.},
eprint = {2007.12026},
file = {:home/william/Documents/Papers/2007.12026.pdf:pdf},
keywords = {dust,evolution,galaxies,ism,molecules,nuclei,seyfert,star formation},
title = {{Gas Content Regulates the Lifecycle of Star Formation and Black Hole Accretion in Galaxies}},
url = {http://arxiv.org/abs/2007.12026},
year = {2020}
}
@article{Herrera-Camus2020,
abstract = {Aims. Our aim is to search for and characterize inflows and outflows of molecular gas in four ultraluminous infrared galaxies (ULIRGs; LIR {\textgreater} 1012LO ) at z ∼ 0.2-0.3 and one distant quasi-stellar object (QSO) at z = 6.13. Methods. We used Herschel/PACS and ALMA Band 7 observations of the hydroxyl molecule (OH) line at rest-frame wavelength 119 $\mu$m, which in absorption can provide unambiguous evidence of inflows or outflows of molecular gas in nuclear regions of galaxies. Our study contributes to doubling the number of OH 119 $\mu$m observations of luminous systems at z ∼ 0.2-0.3, and pushes the search for molecular outflows based on the OH 119 $\mu$m transition to z ∼ 6. Results. We detect OH 119 $\mu$m high-velocity absorption wings in three of the four ULIRGs. In two cases, IRAS F20036-1547 and IRAS F13352+6402, the blueshifted absorption profiles indicate the presence of powerful and fast (∼200-500 km s-1) molecular gas outflows. Consistent with an inside-out quenching scenario, these outflows are depleting the central reservoir of star-forming molecular gas at a rate similar to that of intense star formation activity. For the starburst-dominated system IRAS 10091+4704, we detect an inverted P Cygni profile that is unique among ULIRGs and indicates the presence of a fast (∼400 km s-1) inflow of molecular gas at a rate of ∼100 MO yr-1 towards the central region. Finally, we tentatively detect (∼3$\sigma$) the OH 119 $\mu$m doublet in absorption in the z = 6.13 QSO ULAS J131911+095051. The OH 119 $\mu$m feature is blueshifted with a median velocity that suggests the presence of a molecular outflow, although characterized by a modest molecular mass loss rate of ∼200 MO yr-1. This value is comparable to the small mass outflow rates found in the stacking of the [C » II] spectra of other z ∼ 6 QSOs and suggests that ejective feedback in this phase of the evolution of ULAS J131911+095051 has subsided.},
archivePrefix = {arXiv},
arxivId = {1912.05548},
author = {Herrera-Camus, R. and Sturm, E. and Graci{\'{a}}-Carpio, J. and Veilleux, S. and Shimizu, T. and Lutz, D. and Stone, M. and Gonz{\'{a}}lez-Alfonso, E. and Davies, R. and Fischer, J. and Genzel, R. and Maiolino, R. and Sternberg, A. and Tacconi, L. and Verma, A.},
doi = {10.1051/0004-6361/201937109},
eprint = {1912.05548},
file = {:home/william/Documents/Papers/1912.05548.pdf:pdf},
isbn = {1342270673},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Galaxies: active,Galaxies: evolution,Galaxies: high-redshift,Quasars: absorption lines},
pages = {1--9},
title = {{Molecular gas inflows and outflows in ultraluminous infrared galaxies at z ∼0.2 and one QSO at z = 6.1}},
volume = {633},
year = {2020}
}
@article{Dekel2019,
abstract = {We address a simple model where the Kennicutt-Schmidt (KS) relation between the macroscopic densities of star formation rate (SFR, $\rho$sfr) and gas (n) in galactic discs emerges from self-regulation of the SFR via supernova feedback. It arises from the physics of supernova bubbles, insensitive to the microscopic SFR recipe and not explicitly dependent on gravity. The key is that the filling factor of SFR-suppressed supernova bubbles self-regulates to a constant, f ∼ 0.5. Expressing the bubble fading radius and time in terms of n, the filling factor is f ∝ S n−s with s = 1.5, where S is the supernova rate density. A constant f thus refers to $\rho$sfr ∝ n1.5, with a density-independent SFR efficiency per free-fall time ∼0.01. The self-regulation to f ∼ 0.5 and the convergence to a KS relation independent of the local SFR recipe are demonstrated in cosmological and isolated-galaxy simulations using different codes and recipes. In parallel, the spherical analysis of bubble evolution is generalized to clustered supernovae, analytically and via simulations, yielding s = 1.5 ± 0.5. An analysis of photoionized bubbles about presupernova stars yields a range of KS slopes but the KS relation is dominated by the supernova bubbles. Superbubble blowouts may lead to an alternative self-regulation by outflows and recycling. While the model is oversimplified, its simplicity and validity in the simulations may argue that it captures the origin of the KS relation.},
archivePrefix = {arXiv},
arxivId = {1903.00962},
author = {Dekel, Avishai and Sarkar, Kartick C. and Jiang, Fangzhou and Bournaud, Frederic and Krumholz, Mark R. and Ceverino, Daniel and Primack, Joel R.},
doi = {10.1093/mnras/stz1919},
eprint = {1903.00962},
file = {:home/william/Documents/Papers/stz1919.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: ISM,Galaxies: evolution,Galaxies: formation,Stars: formation,Supernovae: general},
number = {4},
pages = {4753--4778},
publisher = {Oxford University Press},
title = {{The global star formation law by supernova feedback}},
volume = {488},
year = {2019}
}
@article{Cielo2017,
abstract = {Feedback by Active Galactic Nuclei is often divided into quasar and radio mode, powered by radiation or radio jets, respectively. Both are fundamental in galaxy evolution, especially in late-type galaxies, as shown by cosmological simulations and observations of jet-ISM interactions in these systems. We compare AGN feedback by radiation and by collimated jets through a suite of simulations, in which a central AGN interacts with a clumpy, fractal galactic disc. We test AGN of {\$}10{\^{}}{\{}43{\}}{\$} and {\$}10{\^{}}{\{}46{\}}{\$} erg/s, considering jets perpendicular or parallel to the disc. Mechanical jets drive the more powerful outflows, exhibiting stronger mass and momentum coupling with the dense gas, while radiation heats and rarefies the gas more. Radiation and perpendicular jets evolve to be quite similar in outflow properties and effect on the cold ISM, while inclined jets interact more efficiently with all the disc gas, removing the densest {\$}20\backslash{\%}{\$} in {\$}20{\$} Myr, and thereby reducing the amount of cold gas available for star formation. All simulations show small-scale inflows of {\$}0.01-0.1{\$} M{\$}{\_}\backslashodot{\$}/yr, which can easily reach down to the Bondi radius of the central supermassive black hole (especially for radiation and perpendicular jets), implying that AGN modulate their own duty cycle in a feedback/feeding cycle.},
archivePrefix = {arXiv},
arxivId = {1712.03955},
author = {Cielo, S. and Bieri, R. and Volonteri, M. and Wagner, A. and Dubois, Y.},
doi = {10.1093/mnras/sty708},
eprint = {1712.03955},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Cielo et al. - 2017 - AGN Feedback Compared Jets versus Radiation.pdf:pdf},
issn = {1365-2966},
keywords = {active,galaxies,high-redshift,ism,methods},
journal = {MNRAS},
number = {December},
title = {{AGN Feedback Compared: Jets versus Radiation}},
url = {http://arxiv.org/abs/1712.03955{\%}0Ahttp://dx.doi.org/10.1093/mnras/sty708},
volume = {000},
year = {2017}
}
@article{Koudmani2019,
abstract = {The systematic analysis of optical large-scale surveys has revealed a population of dwarf galaxies hosting active galactic nuclei (AGN), which have been confirmed by X-ray followup observations. Recently, the MaNGA survey identified six dwarf galaxies that appear to have an AGN that is preventing on-going star formation. It is therefore timely to study the physical properties of dwarf galaxies, in particular whether the presence of an AGN can affect their evolution. Using the moving mesh code AREPO, we have investigated different models of AGN activity, ranging from simple energy-driven spherical winds to collimated, mass-loaded, bipolar outflows in high-resolution simulations of isolated dwarf galaxies hosting an active black hole. Our simulations also include a novel implementation of star formation and mechanical supernova (SN) feedback. We find that AGN outflows have a small but systematic effect on the central star formation rates (SFRs) for all set-ups explored, while substantial effects on the global SFR are only obtained with strong SNe and a sustained high-luminosity AGN with an isotropic wind. This suggests that AGN feedback in dwarf galaxies is unlikely to directly regulate their global SFRs. There is, however, a significant effect on outflow properties, which are notably enhanced by the AGN to much higher outflow temperatures and velocities, in agreement with kinematic signatures from the MaNGA survey. This indicates that AGN may play an indirect role in regulating the baryon cycle in dwarf galaxies by hindering cosmic gas inflows.},
archivePrefix = {arXiv},
arxivId = {1812.04629},
author = {Koudmani, Sophie and Sijacki, Debora and Bourne, Martin A. and Smith, Matthew C.},
doi = {10.1093/mnras/stz097},
eprint = {1812.04629},
file = {:home/william/Documents/Papers/stz097.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: active,Galaxies: dwarf,Galaxies: formation,Methods: numerical},
number = {2},
pages = {2047--2066},
publisher = {Oxford University Press},
title = {{Fast and energetic AGN-driven outflows in simulated dwarf galaxies}},
volume = {484},
year = {2019}
}
@article{Ko2019,
abstract = {Processes of dissipation of energy released during capture and disruption stars by Galactic central Black hole. This process should periodically happen in the Galactic center and affect Galactic center environment as well as Galactic halo. Routine star disruptions by the central supermassive black hole BH provide enough cumulative energy to form the Fermi Bubbles. A single star of super-Eddington eruption provide an subsonic outflow gas whose total energy is about {\$}10{\^{}}{\{}52{\}}{\$} erg. The average rate of disruption events is expected to be {\$}10{\^{}}{\{}-4{\}}-10{\^{}}{\{}-5{\}}{\$}yr{\$}{\^{}}{\{}-1{\}}{\$} that provides the average power of energy release in the GC {\$}\backslashdot{\{}W{\}}\backslashsim 3\backslashtimes 10{\^{}}{\{}41{\}}{\$} erg s{\$}{\^{}}{\{}-1{\}}{\$}, just needed to support Fermi Bubbles in the halo. In the exponential atmosphere the energy from the GC propagates perpendicular to the Galactic plane and provides symmetric features in the halo.},
archivePrefix = {arXiv},
arxivId = {1904.03958},
author = {Ko, C. M. and Chernyshov, D. O. and Cheng, H. and Dai, L. and Dogiel, V. A.},
eprint = {1904.03958},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Ko et al. - 2019 - Formation of Fermi Bubbles by Tidal Disruption Events at Galactic Center.pdf:pdf},
keywords = {clouds,cosmic rays,gamma rays,ism,mhd,non-thermal,radiation mechanisms,scattering,turbulence},
title = {{Formation of Fermi Bubbles by Tidal Disruption Events at Galactic Center}},
url = {http://arxiv.org/abs/1904.03958},
volume = {1},
year = {2019}
}
@article{Luminet2003,
abstract = {The current 'standard model' of cosmology posits an infinite flat universe forever expanding under the pressure of dark energy. First-year data from the Wilkinson Microwave Anisotropy Probe (WMAP) confirm this model to spectacular precision on all but the largest scales. Temperature correlations across the microwave sky match expectations on angular scales narrower than 60° but, contrary to predictions, vanish on scales wider than 60°. Several explanations have been proposed. One natural approach questions the underlying geometry of space-namely, its curvature and topology. In an infinite flat space, waves from the Big Bang would fill the universe on all length scales. The observed lack of temperature correlations on scales beyond 60° means that the broadest waves are missing, perhaps because space itself is not big enough to support them. Here we present a simple geometrical model of a finite space-the Poincar{\'{e}} dodecahedral space-which accounts for WMAP's observations with no fine-tuning required. The predicted density is $\Omega$ 0 ≈ 1.013 {\textgreater} 1, and the model also predicts temperature correlations in matching circles on the sky.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0310253},
author = {Luminet, Jean Pierre and Weeks, Jeffrey R. and Riazuelo, Alain and Lehoucq, Roland and Uzan, Jean Philippe},
doi = {10.1038/nature01944},
eprint = {0310253},
file = {:home/william/Documents/Papers/83950 593..640 {\_} Enhanced Reader.pdf:pdf},
issn = {00280836},
journal = {Nature},
number = {6958},
pages = {593--595},
primaryClass = {astro-ph},
title = {{Dodecahedral space topology as an explanation for weak wide-angle temperature correlations in the cosmic microwave background}},
volume = {425},
year = {2003}
}
@article{Yang2018b,
abstract = {The Fermi bubbles, two giant structures above and below the Galactic center (GC), are among the most important discoveries of the Fermi Gamma-ray Space Telescope. Studying their physical origin has been providing valuable insights into cosmic-ray transport, the Galactic magnetic field, and past activity at the GC in the Milky Way galaxy. Despite their importance, the formation mechanism of the bubbles is still elusive. Over the past few years there have been numerous efforts, both observational and theoretical, to uncover the nature of the bubbles. In this article, we present an overview of the current status of our understanding of the bubbles' origin, and discuss possible future directions that will help to distinguish different scenarios of bubble formation.},
archivePrefix = {arXiv},
arxivId = {1802.03890},
author = {Yang, H. -Y. K. and Ruszkowski, M. and Zweibel, E. G.},
doi = {10.3390/galaxies6010029},
eprint = {1802.03890},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Yang, Ruszkowski, Zweibel - 2018 - Unveiling the Origin of the Fermi Bubbles.pdf:pdf},
issn = {20754434},
keywords = {cosmic rays,galaxy,gamma rays},
pages = {1--9},
title = {{Unveiling the Origin of the Fermi Bubbles}},
url = {http://arxiv.org/abs/1802.03890{\%}0Ahttp://dx.doi.org/10.3390/galaxies6010029},
year = {2018}
}
@article{Hayashi2021,
abstract = {We present the results of our multifrequency observations for 10 ultraluminous infrared galaxies (ULIRGs) made by the Karl G. Jansky Very Large Array at 1.4, 5.5, 9.0, and 14.0 GHz. Our sample is selected from ULIRGs whose active galactic nuclei (AGNs) are not found at optical wavelengths (∼70 per cent of the total ULIRGs), but whose presence is suggested by mid-infrared or submillimetre observations ({\textgreater}50 per cent of the non-AGN ULIRGs at optical wavelengths). The statistical properties of the targets are similar to those of the entire ULIRG sample, which implies that ULIRGs have common radiative processes regardless of the presence of optical AGNs, and thus AGNs might equally contribute to the radio emission of every ULIRG. Although their spectra are mainly explained by starbursts and/or merger activity, some individual sources suggest contributions from AGNs. IRAS 00188-0856, whose optical morphology is not disturbed, shows a large non-thermal fraction and a spectral break at high frequency, which can be explained by synchrotron ageing of non-thermal plasma emitted from AGNs. In addition, we find 100-kpc-scale extended emission associated with IRAS 01004-2237. The two-sided morphology and absence of extended X-ray emission suggest that this system is not induced by a merger in a cluster but originates from AGN activity.},
archivePrefix = {arXiv},
arxivId = {2101.12058},
author = {Hayashi, Takayuki J. and Hagiwara, Yoshiaki and Imanishi, Masatoshi},
doi = {10.1093/mnras/stab1084},
eprint = {2101.12058},
file = {:home/william/Documents/Papers/2101.12058.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {galaxies: active,galaxies: nuclei,radio continuum: galaxies,techniques: interferometric},
number = {2},
pages = {2675--2686},
title = {{Radio properties of 10 nearby ultraluminous infrared galaxies with signatures of luminous buried active galactic nuclei}},
url = {http://arxiv.org/abs/2101.12058},
volume = {504},
year = {2021}
}

@article{Morganti2013b,
abstract = {High-resolution (0.5 arcsec) CO(2-1) observations performed with the Atacama Large Millimetre/submillimetre Array have been used to trace the kinematics of the molecular gas in the Seyfert 2 galaxy{\{}IC{\~{}}5063{\}}. Although one of the most radio-loud Seyfert galaxy, IC{\~{}}5063 is a relatively weak radio source (P{\_}1.4GHz = 3 x 10{\^{}}23 W Hz{\^{}}-1). The data reveal that the kinematics of the gas is very complex. A fast outflow of molecular gas extends along the entire radio jet ({\~{}} 1 kpc), with the highest outflow velocities about 0.5 kpc from the nucleus, at the location of the brighter hot-spot in the W lobe. All the observed characteristics can be described by a scenario of a radio plasma jet expanding into a clumpy medium, interacting directly with the clouds and inflating a cocoon that drives a lateral outflow into the interstellar medium. This suggests that most of the observed cold molecular outflow is due to fast cooling of the gas after the passage of a shock and that it is the end product of the cooling process.},
archivePrefix = {arXiv},
arxivId = {1504.04694},
author = {Morganti, Raffaella and Fogasy, Judit and Paragi, Zsolt and Oosterloo, Tom and Orienti, Monica},
doi = {10.1126/science.1240436},
eprint = {1504.04694},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Morganti et al. - 2013 - Radio jets clearing the way through a galaxy Watching feedback in action.pdf:pdf},
isbn = {0036-8075},
issn = {10959203},
journal = {Science (80-. ).},
number = {6150},
pages = {1082--1085},
pmid = {24009387},
title = {{Radio jets clearing the way through a galaxy: Watching feedback in action}},
volume = {341},
year = {2013}
}
@article{Kaaret2022,
abstract = {Chandra observations of the nearby, candidate Lyman-continuum (LyC) emitting galaxy Tol 0440-381 show brightening of an X-ray source by at least a factor of 4 to a luminosity of 1.6E40 erg/s over 3.8{\~{}}days. The X-ray emission likely arises from either a low-luminosity AGN or an ultraluminous X-ray source. The properties of the X-ray source are similar to those found in Haro 11 and Tololo 1247-232, the only other LyC-emitting galaxies that have been resolved in X-rays. All three galaxies host luminous, variable, and hard spectrum X-ray sources that are likely accretion-powered. Accretion onto compact objects produces powerful outflows and ionizing radiation that could help enable LyC escape.},
archivePrefix = {arXiv},
arxivId = {2201.03138},
author = {Kaaret, P. and Bluem, J. and Prestwich, A. H.},
doi = {10.1093/mnrasl/slab127},
eprint = {2201.03138},
file = {:home/william/Documents/Papers/2201.03138.pdf:pdf},
keywords = {binaries,galaxies,individual,star formation,tol 0440-381,x-rays},
number = {January},
pages = {1--5},
title = {{Rapid turn-on of a luminous X-ray source in the candidate Lyman continuum emitting galaxy Tol 0440-381}},
url = {http://arxiv.org/abs/2201.03138{\%}0Ahttp://dx.doi.org/10.1093/mnrasl/slab127},
volume = {5},
year = {2022}
}
@article{Edgar2004,
abstract = {If a point mass moves through a uniform gas cloud, at what rate does it accrete material? This is the question studied by Bondi, Hoyle and Lyttleton. This paper draws together the work performed in this area since the problem was first studied. Time has shown that, despite the simplifications made, Bondi, Hoyle and Lyttleton made quite accurate predictions for the accretion rate. Bondi- Hoyle-Lyttleton accretion has found application in many fields of astronomy, and these are also discussed. {\textcopyright} 2004 Elsevier B.V. All rights reserved.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0406166},
author = {Edgar, Richard},
doi = {10.1016/j.newar.2004.06.001},
eprint = {0406166},
file = {:home/william/Documents/Papers/[Edgar R,.]-A Review of Bondi–Hoyle–Lyttleton.pdf:pdf},
issn = {13876473},
journal = {New Astron. Rev.},
keywords = {Accretion},
number = {10},
pages = {843--859},
primaryClass = {astro-ph},
title = {{A review of Bondi-Hoyle-Lyttleton accretion}},
volume = {48},
year = {2004}
}
@article{Graur2015,
abstract = {Using a method to discover and classify supernovae (SNe) in galaxy spectra, we detect 91 Type Ia SNe (SNe Ia) and 16 Type II SNe (SNe II) among {\~{}}740 000 galaxies of all types and {\~{}}215 000 star-forming galaxies without active galactic nuclei, respectively, in Data Release 9 of the Sloan Digital Sky Survey. Of these SNe, 15 SNe Ia and eight SNe II are new discoveries reported here for the first time. We use our SN samples to measure SN rates per unit mass as a function of galaxy stellar mass, star-formation rate (SFR), and specific SFR (sSFR), as derived by the MPA-JHU Galspec pipeline. We show that correlations between SN Ia and SN II rates per unit mass and galaxy stellar mass, SFR, and sSFR can be explained by a combination of the respective SN delay-time distributions (the distributions of times that elapse between the formation of a stellar population and all ensuing SNe), the ages of the surveyed galaxies, the redshifts at which they are observed, and their star formation histories. This model was first suggested by Kistler et al. for the SN Ia rate-mass correlation, but is expanded here to SNe II and to correlations with galaxy SFR and sSFR. Finally, we measure a volumetric SN II rate at redshift 0.075 of RII, V = 0.621-0.154+0.197 (stat)-0.063+0.024 (sys) × 10-4 yr-1 Mpc-3. Assuming that SNe IIP and IIL account for 60 per cent of all core-collapse (CC) SNe, the CC SN rate is RCC, V = 1.04-0.26+0.33 (stat)-0.11+0.04 (sys) × 10-4 yr-1 Mpc-3.},
archivePrefix = {arXiv},
arxivId = {1412.7991},
author = {Graur, Or and Bianco, Federica B. and Modjaz, Maryam},
doi = {10.1093/mnras/stv713},
eprint = {1412.7991},
file = {:home/william/Documents/Papers/1412.7991.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Methods: observational,Supernovae: general,Surveys},
number = {1},
pages = {905--925},
title = {{A unified explanation for the supernova rate-galaxy mass dependence based on supernovae detected in Sloan galaxy spectra}},
volume = {450},
year = {2015}
}
@article{McGaugh2012,
abstract = {The baryonic Tully-Fisher relation (BTFR) is an empirical relation between baryonic mass and rotation velocity in disk galaxies. It provides tests of galaxy formation models in $\Lambda$CDM and of alternative theories like modified Newtonian dynamics (MOND). Observations of gas-rich galaxies provide a measure of the slope and normalization of the BTFR that is more accurate (if less precise) than that provided by star-dominated spirals, as their masses are insensitive to the details of stellar population modeling. Recent independent data for such galaxies are consistent with M b = AV 4f with A = 47 6 M km -4 s 4. This is equivalent to MOND with a 0 = 1.3 0.3 s -2. The scatter in the data is consistent with being due entirely to observational uncertainties. It is unclear why the physics of galaxy formation in $\Lambda$CDM happens to pick out the relation predicted by MOND. We introduce a feedback efficacy parameter to relate halo properties to those of the galaxies they host. correlates with star formation rate and gas fraction in the sense that galaxies that have experienced the least star formation have been most impacted by feedback. {\textcopyright} 2012. The American Astronomical Society. All rights reserved.},
archivePrefix = {arXiv},
arxivId = {1107.2934},
author = {McGaugh, Stacy S.},
doi = {10.1088/0004-6256/143/2/40},
eprint = {1107.2934},
file = {:home/william/Documents/Papers/[McGaugh]-The Baryonic Tully-Fisher Relation of Gas-rich Galaxies as a Test of $\Lambda$CDM and MOND.pdf:pdf},
issn = {00046256},
journal = {Astron. J.},
keywords = {galaxies: dwarf,galaxies: irregular,galaxies: kinematics and dynamics,galaxies: spiral},
number = {2},
title = {{The baryonic tully-fisher relation of gas-rich galaxies as a test of $\Lambda$cDM and MOND}},
volume = {143},
year = {2012}
}
@article{PaulM.Muchinsky2012,
abstract = {Predicting the binding mode of flexible polypeptides to proteins is an important task that falls outside the domain of applicability of most small molecule and protein−protein docking tools. Here, we test the small molecule flexible ligand docking program Glide on a set of 19 non-$\alpha$-helical peptides and systematically improve pose prediction accuracy by enhancing Glide sampling for flexible polypeptides. In addition, scoring of the poses was improved by post-processing with physics-based implicit solvent MM- GBSA calculations. Using the best RMSD among the top 10 scoring poses as a metric, the success rate (RMSD ≤ 2.0 {\AA} for the interface backbone atoms) increased from 21{\%} with default Glide SP settings to 58{\%} with the enhanced peptide sampling and scoring protocol in the case of redocking to the native protein structure. This approaches the accuracy of the recently developed Rosetta FlexPepDock method (63{\%} success for these 19 peptides) while being over 100 times faster. Cross-docking was performed for a subset of cases where an unbound receptor structure was available, and in that case, 40{\%} of peptides were docked successfully. We analyze the results and find that the optimized polypeptide protocol is most accurate for extended peptides of limited size and number of formal charges, defining a domain of applicability for this approach.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Hollenbach, D.},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
file = {:home/william/Documents/Papers/1979ApJS...41..555H.pdf:pdf},
isbn = {9788578110796},
issn = {1098-6596},
journal = {Astrophys. J.},
keywords = {icle},
number = {9},
pages = {1689--1699},
pmid = {25246403},
title = {{MOLECULE FORMATION AND INFRARED EMISSION IN FAST INTERESTELLAR SHOCK. I-PHYSICAL PROCESSES}},
volume = {53},
year = {1979}
}
@article{Chen2020,
abstract = {Large-scale outflows are generally considered as a possible evidence that active galactic nuclei (AGNs) can severely affect their host galaxies. Recently an ultraluminous IR galaxy (ULIRG) at z = 0.49, AKARI J0916248+073034, was found to have a galaxy-scale [Oiii] $\lambda$5007 outflow with one of the highest energy-ejection rates at z {\textless} 1.6. However, the central AGN activity estimated from its torus mid-IR (MIR) radiation is weak relative to the luminous [Oiii] emission. In this work we report the first NuSTAR hard X-ray follow-up of this ULIRG to constrain its current AGN luminosity. The intrinsic 2–10 keV luminosity shows a 90{\%} upper-limit of 3.0 × 1043 erg s−1 assuming Compton-thick obscuration (NH = 1.5 × 1024 cm−2), which is only 3.6{\%} of the luminosity expected from the extinction corrected [Oiii] luminosity. With the NuSTAR observation, we succeed to identify that this ULIRG has a most extreme case of X-ray deficit among local ULIRGs. A possible scenario to explain the drastic declining in both of the corona (X-ray) and torus (MIR) is that the primary radiation from the AGN accretion disk is currently in a fading status, as a consequence of a powerful nuclear wind suggested by its powerful ionized outflow in the galaxy scale.},
archivePrefix = {arXiv},
arxivId = {2011.06914},
author = {Chen, Xiaoyang and Ichikawa, Kohei and Noda, Hirofumi and Kawamuro, Taiki and Kawaguchi, Toshihiro and Toba, Yoshiki and Akiyama, Masayuki},
doi = {10.3847/2041-8213/abca30},
eprint = {2011.06914},
file = {:home/william/Documents/Papers/Chen{\_}2020{\_}ApJL{\_}905{\_}L2.pdf:pdf},
issn = {23318422},
journal = {arXiv},
keywords = {Active galaxies,ULIRG,X-ray AGN},
number = {1},
pages = {L2},
publisher = {IOP Publishing},
title = {{NuSTAR Non-detection of a faint active galactic nucleus in an ultraluminous IR galaxy with Kpc-scale fast wind}},
url = {http://dx.doi.org/10.3847/2041-8213/abca30},
volume = {905},
year = {2020}
}
@article{Lopez-Rodriguez2019,
abstract = {We report the first detection of galactic spiral structure by means of thermal emission from magnetically aligned dust grains. Our 89 µm polarimetric imaging of NGC 1068 with the High-resolution Airborne Wideband Camera/Polarimeter (HAWC+) on NASAs Stratospheric Observatory for Infrared Astronomy (SOFIA) also sheds light on magnetic field structure in the vicinity of the galaxys inner-bar and active galactic nucleus (AGN). We find correlations between the 89 µm magnetic field vectors and other tracers of spiral arms, and a symmetric polarization pattern as a function of the azimuthal angle arising from the projection and inclination of the disk field component in the plane of the sky. The observations can be fit with a logarithmic spiral model with pitch angle of 16.9−+22..78◦ and a disk inclination of 48 ± 2◦. We infer that the bulk of the interstellar medium from which the polarized dust emission originates is threaded by a magnetic field that closely follows the spiral arms. Inside the central starburst disk ({\textless} 1.6 kpc), the degree of polarization is found to be lower than for far-infrared sources in the Milky Way, and has minima at the locations of most intense star formation near the outer ends of the inner-bar. Inside the starburst ring, the field direction deviates from the model, becoming more radial along the leading edges of the inner-bar. The polarized flux and dust temperature peak ∼ 3 − 600 NE of the AGN at the location of a bow shock between the AGN outflow and the surrounding interstellar medium, but the AGN itself is weakly polarized ({\textless} 1{\%}) at both 53 and 89 µm.},
archivePrefix = {arXiv},
arxivId = {1907.06648},
author = {Lopez-Rodriguez, Enrique and Dowell, C. Darren and Jones, Terry J. and Harper, Doyal A. and Berthoud, Marc and Chuss, David and Dale, Daniel A. and Guerra, Jordan A. and Hamilton, Ryan T. and Looney, Leslie W. and Michail, Joseph M. and Nikutta, Robert and Novak, Giles and Santos, Fabio P. and Sheth, Kartik and Siah, Javad and Staguhn, Johannes and Stephens, Ian W. and Tassis, Konstantinos and Trinh, Christopher Q. and Ward-Thompson, Derek and Werner, Michael and Wollack, Edward J. and Zweibel, Ellen G.},
doi = {10.3847/1538-4357/ab5849},
eprint = {1907.06648},
file = {:home/william/Documents/Papers/1907.06648.pdf:pdf},
issn = {23318422},
journal = {arXiv},
keywords = {Galaxies - techniques,Individual (NGC 1068) - galaxies,Infrared,Magnetic fields,Polarimetric - galaxies},
title = {{SOFIA/HAWC+ traces the magnetic fields in NGC 1068}},
year = {2019}
}
@article{Correa2019,
abstract = {Ultra-Luminous Infrared Galaxies (ULIRGs) are the most luminous objects in the infrared sky. With infrared luminosities exceeding 1012 solar luminosities, ULIRGs contain strong star formation regions which could power hadronic acceleration. Moreover, a significant fraction of ULIRGs have been found to host Active Galactic Nuclei, which could also be a source of hadronic acceleration. Furthermore, such high infrared luminosities indicate that large amounts of dust are present in these objects. In the presence of hadronic acceleration, this dust not only represents an excellent target for high-energy neutrino production through the pp-channel, but it could also attenuate a significant fraction of the gamma rays that are produced in this process. This could relieve the apparent tension between the diffuse IceCube neutrino flux and the diffuse gamma-ray flux measured by Fermi-LAT. We present our source selection criteria and IceCube sensitivities in view of a search for high-energy neutrinos from these so far unexplored objects.},
archivePrefix = {arXiv},
arxivId = {1908.05137},
author = {Correa, Pablo and {De Vries}, Krijn D. and {Van Eijndhoven}, Nick},
doi = {10.22323/1.358.0860},
eprint = {1908.05137},
file = {:home/william/Documents/Papers/1908.05137.pdf:pdf},
issn = {23318422},
journal = {arXiv},
title = {{Investigation of Ultra-Luminous Infrared Galaxies as obscured high-energy neutrino source candidates}},
year = {2019}
}
@article{Longinotti2018,
abstract = {We report on the coexistence of powerful gas outflows observed in millimeter and X-ray data of the Radio-Loud Narrow Line Seyfert 1 Galaxy IRAS 17020+4544. Thanks to the large collecting power of the Large Millimeter Telescope, a prominent line arising from the 12CO(1-0) transition was revealed in recent observations of this source. The complex profile is composed by a narrow double-peak line and a broad wing. While the double-peak structure may be arising in a disk of molecular material, the broad wing is interpreted as the signature of a massive outflow of molecular gas with an approximate bulk velocity of -660 km/s. This molecular wind is likely associated to a multi-component X-ray Ultra-Fast Outflow with velocities reaching up to {\~{}}0.1c and column densities in the range 10{\^{}}{\{}21-23.9{\}} cm{\^{}}-2 that was reported in the source prior to the LMT observations. The momentum load estimated in the two gas phases indicates that within the observational uncertainties the outflow is consistent with being propagating through the galaxy and sweeping up the gas while conserving its energy. This scenario, which has been often postulated as a viable mechanism of how AGN feedback takes place, has so far been observed only in ULIRGs sources. IRAS 17020+4544 with bolometric and infrared luminosity respectively of 5X10{\^{}}{\{}44{\}} erg/s and 1.05X10{\^{}}{\{}11{\}} L{\_}sun appears to be an example of AGN feedback in a NLSy1 Galaxy (a low power AGN). New proprietary multi-wavelength data recently obtained on this source will allow us to corroborate the proposed hypothesis.},
archivePrefix = {arXiv},
arxivId = {1810.01941},
author = {Longinotti, A. L. and Vega, O. and Krongold, Y. and Aretxaga, I. and Yun, M. and Chavushyan, V. and Feruglio, C. and Gomez-Ruiz, A. and Monta{\~{n}}a, A. and Leon-Tavares, J. and Olguın-Iglesias, A. and Giroletti, M. and Guainazzi, M. and Kotilainen, J. and Panessa, F. and Zapata, L. A. and Cruz-Gonzalez, I. and Pati{\~{n}}o-Alvarez, V. M. and Rosa-Gonzalez, D. and Carrami{\~{n}}ana, A. and Carrasco, L. and Costantini, E. and Dultzin, D. and Guichard, J. and Puerari, I. and Santos-Lleo, M.},
eprint = {1810.01941},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Longinotti et al. - 2018 - Early Science with the Large Millimeter Telescope an energy-driven wind revealed by massive molecular and fas.pdf:pdf},
pages = {1--9},
title = {{Early Science with the Large Millimeter Telescope: an energy-driven wind revealed by massive molecular and fast X-ray outflows in the Seyfert Galaxy IRAS 17020+4544}},
url = {http://arxiv.org/abs/1810.01941},
year = {2018}
}
@article{Riffel2021,
abstract = {We present maps for the electron temperature in the inner kpc of three luminous Seyfert galaxies: Mrk 79, Mrk 348, and Mrk 607 obtained from Gemini Multi-Object Spectrograph-integral field unit observations at spatial resolutions of ∼110–280 pc. We study the distributions of electron temperature in active galaxies and find temperatures varying in the range from ∼8000 to {\textgreater} 30 000 K. Shocks due to gas outflows play an important role in the observed temperature distributions of Mrk 79 and Mrk 348, while standard photoionization models reproduce the derived temperature values for Mrk 607. In Mrk 79 and Mrk 348, we find direct evidence for shock ionization with overall orientation orthogonal to the ionization axis, where shocks can be easily observed as the active galactic nuclei radiation field is shielded by the nuclear dusty torus. This also indicates that even when the ionization cones are narrow, the shocks can be much wider angle.},
archivePrefix = {arXiv},
arxivId = {2012.02013},
author = {Riffel, R. A. and Dors, O. L. and Armah, M. and Storchi-Bergmann, T. and Feltre, A. and H{\"{a}}gele, G. F. and Cardaci, M. V. and Ruschel-Dutra, D. and Krabbe, A. C. and P{\'{e}}rez-Montero, E. and Zakamska, N. L. and Freitas, I. C.},
doi = {10.1093/mnrasl/slaa194},
eprint = {2012.02013},
file = {:home/william/Documents/Papers/2021MNRAS.501L..54R.pdf:pdf},
issn = {17453933},
journal = {Mon. Not. R. Astron. Soc. Lett.},
keywords = {Galaxies: ISM,Galaxies: Seyfert,Galaxies: abundances,Galaxies: active},
number = {1},
pages = {L54--L59},
title = {{Chemical abundances in Seyfert galaxies – V. The discovery of shocked emission outside the AGN ionization axis}},
volume = {501},
year = {2021}
}
@article{Sutherland2017,
abstract = {In this paper we treat the pre-ionisation problem in shocks over the velocity range {\$}10 {\textless} v{\_}{\{}\backslashrm s{\}} {\textless} 1500{\$}$\backslash$,km/s in a self-consistent manner. We identify four distinct classes of solution controlled by the value of the shock precursor parameter, {\$}\backslashPsi = {\{}\backslashcal Q{\}}/v{\_}s{\$}, where {\$}{\{}\backslashcal Q{\}}{\$} is the ionization parameter of the UV photons escaping upstream. This parameter determines both the temperature and the degree of ionisation of the gas entering the shock. In increasing velocity the shock solution regimes are cold neutral precursors ({\$}v{\_}s \backslashlesssim 40{\$}$\backslash$,km/s), warm neutral precursors ({\$}40 \backslashlesssim v{\_}s \backslashlesssim 75{\$}$\backslash$,km/s), warm partly-ionized precursors ({\$}75 \backslashlesssim v{\_}s \backslashlesssim 120{\$}$\backslash$,km/s), and fast shocks in which the pre-shock gas is in photoionisation equilibrium, and is fully ionized. The main effect of a magnetic field is to push these velocity ranges to higher values, and to limit the post-shock compression. In order to facilitate comparison with observations of shocks, we provide a number of convenient scaling relationships for parameters such as post-shock temperature, compression factors, cooling lengths, and H{\$}\backslashbeta{\$} and X-ray luminosity.},
archivePrefix = {arXiv},
arxivId = {1702.07453},
author = {Sutherland, Ralph S. and Dopita, Michael A.},
doi = {10.3847/1538-4365/aa6541},
eprint = {1702.07453},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Sutherland, Dopita - 2017 - Effects of Pre-ionisation in Radiative Shocks I Self-Consistent Models.pdf:pdf},
issn = {1538-4365},
journal = {Astrophys. J. Suppl. Ser.},
keywords = {atomic data,atomic data,atomic processes,radiative transfer,sh,atomic processes,machine-readable tables,radiative transfer,shock waves,supporting material},
number = {2},
pages = {34},
publisher = {IOP Publishing},
title = {{Effects of Pre-ionisation in Radiative Shocks I: Self-Consistent Models}},
url = {http://arxiv.org/abs/1702.07453{\%}0Ahttp://dx.doi.org/10.3847/1538-4365/aa6541},
volume = {229},
year = {2017}
}
@article{Pereira-Santaella2020,
abstract = {We used high-spatial resolution (70 pc; 0{\$} {\{}{\{}\backslashoverset{\{}\backslashprime\backslashprime{\}}{\{}.{\}}{\}}{\}} {\$}3) CO multi-transition (J = 1-0, 2-1, 4-3, and 6-5) ALMA data to study the physical conditions and kinematics of the cold molecular outflow in the local luminous infrared galaxy (LIRG) ESO 320-G030 (d = 48 Mpc, LIR/L = 1011.3). ESO 320-G030 is a double-barred isolated spiral, but its compact and obscured nuclear starburst (SFR ∼15 M yr-1; AV ∼40 mag) resembles those of ultra-luminous infrared galaxies (LIR/L {\textgreater} 1012). In the outflow, the CO(1-0)/CO(2-1) ratio is enhanced with respect to the rest of the galaxy and the CO(4-3) transition is undetected. This indicates that the outflowing molecular gas is less excited than the molecular gas in the nuclear starburst (i.e., outflow launching site) and in the galaxy disk. Non-local thermodynamic equilibrium radiative transfer modeling reveals that the properties of the molecular clouds in the outflow differ from those of the nuclear and disk clouds: The kinetic temperature is lower (Tkin ∼ 9 K) in the outflow, and the outflowing clouds have lower column densities. Assuming a 10-4 CO abundance, the large internal velocity gradients, 60-45+250 km s-1 pc-1, imply that the outflowing molecular clouds are not bound by self-gravity. All this suggests that the life-cycle (formation, collapse, dissipation) of the galaxy disk molecular clouds might differ from that of the outflowing molecular clouds which might not be able to form stars. The low kinetic temperature of the molecular outflow remains constant at radial distances between 0.3 and 1.7 kpc. This indicates that the heating by the hotter ionized outflow phase is not efficient and may favor the survival of the molecular gas phase in the outflow. The spatially resolved velocity structure of the outflow shows a 0.8 km s-1 pc-1 velocity gradient between 190 pc and 560 pc and then a constant maximum outflow velocity of about 700-800 km s-1 up to 1.7 kpc. This could be compatible with a pure gravitational evolution of the outflow, which would require coupled variations of the mass outflow rate and the outflow launching velocity distribution. Alternatively, a combination of ram pressure acceleration and cloud evaporation could explain the observed kinematics and the total size of the cold molecular phase of the outflow.},
archivePrefix = {arXiv},
arxivId = {2009.08481},
author = {Pereira-Santaella, M. and Colina, L. and Garc{\'{i}}a-Burillo, S. and Gonz{\'{a}}lez-Alfonso, E. and Alonso-Herrero, A. and Arribas, S. and Cazzoli, S. and Piqueras-L{\'{o}}pez, J. and Rigopoulou, D. and Usero, A.},
doi = {10.1051/0004-6361/202038838},
eprint = {2009.08481},
file = {:home/william/Documents/Papers/2009.08481.pdf:pdf},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Galaxies: ISM,Galaxies: nuclei,ISM: molecules,Infrared: galaxies},
title = {{Excitation and acceleration of molecular outflows in LIRGs: The extended ESO 320-G030 outflow on 200-pc scales}},
volume = {643},
year = {2020}
}
@article{Choi2014,
abstract = {Quantum dynamics of light waves traveling through a time-varying turbulent plasma is investigated via the SU(1,1) Lie algebraic approach. Plasma oscillations that accompany time-dependence of electromagnetic parameters of the plasma are considered. In particular, we assume that the conductivity of plasma involves a sinusoidally varying term in addition to a constant one. Regarding the time behavior of electromagnetic parameters in media, the light fields are modeled as a modified CK (Caldirola-Kanai) oscillator that is more complex than the standard CK oscillator. Diverse quantum properties of the system are analyzed under the consideration of time-dependent characteristics of electromagnetic parameters. Quantum energy of the light waves is derived and compared with the counterpart classical energy. Gaussian wave packet of the field whose probability density oscillates with time like that of classical states is constructed through a choice of suitable initial condition and its quantum behavior is investigated in detail. Our development presented here provides a useful way for analyzing time behavior of quantized light in complex plasma.},
author = {Choi, Jeong Ryeol},
doi = {10.1038/srep06880},
file = {:home/william/Documents/Papers/may.srep06880.pdf:pdf},
issn = {20452322},
journal = {Sci. Rep.},
pages = {1--7},
title = {{A novel method for analyzing complicated quantum behaviors of light waves in oscillating turbulent plasma}},
volume = {4},
year = {2014}
}
@article{Harrison2018a,
abstract = {It is the twentieth anniversary of the publication of the seminal papers by Magorrian et al. and Silk {\&} Rees which, along with other related work, ignited an explosion of publications connecting active galactic nuclei (AGN)-driven outflows to galaxy evolution. With a surge in observations of AGN outflows, studies are attempting to directly test AGN feedback models using the outflow properties. With a focus on outflows traced by optical and CO emission lines, we discuss significant challenges which greatly complicate this task from both an observational and theoretical perspective. We highlight observational uncertainties involved, and the assumptions required, when deriving kinetic coupling efficiencies (i.e., outflow kinetic power as a fraction of AGN luminosity) from typical observations. Based on recent models we demonstrate that extreme caution should taken when comparing observationally-derived kinetic coupling efficiencies to coupling efficiencies from fiducial feedback models.},
archivePrefix = {arXiv},
arxivId = {1802.10306},
author = {Harrison, C. M. and Costa, T. and Tadhunter, C. N. and Fl{\"{u}}tsch, A. and Kakkad, D. and Perna, M. and Vietri, G.},
doi = {10.1038/s41550-018-0403-6},
eprint = {1802.10306},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Harrison et al. - 2018 - AGN outflows and feedback twenty years on.pdf:pdf},
issn = {23973366},
journal = {Nat. Astron.},
number = {3},
pages = {198--205},
title = {{AGN outflows and feedback twenty years on}},
volume = {2},
year = {2018}
}
@article{Drzazga2011,
abstract = {Aims. Violent gravitational interactions can change the morphologies of galaxies and, by means of merging, transform them into elliptical galaxies. We aim to investigate how they affect the evolution of galactic magnetic fields. Methods. We selected 16 systems of interacting galaxies with available VLA archive radio data at 4.86 and 1.4 GHz and compared their radio emission and estimated magnetic field strengths with their star-forming activity, far-infrared emission, and the stage of tidal interaction. Results. The estimated mean of total magnetic field strength for our sample of interacting galaxies is 14 ± 5 $\mu$G, which is larger than for the non-interacting objects. The field regularity (of 0.27 ± 0.09) is lower than in typical spirals and indicates enhanced production of random magnetic fields in the interacting objects. We find a general evolution of magnetic fields: for weak interactions the strength of magnetic field is almost constant (10−15 $\mu$G) as interaction advances, then it increases up to 2×, peaks at the nuclear coalescence (25 $\mu$G), and decreases again, down to 5−6 $\mu$G, for the post-merger remnants. The main production of magnetic fields in colliding galaxies thus terminates somewhere close to the nuclear coalescence, after which magnetic field diffuses. The magnetic field strength for whole galaxies is weakly affected by the star formation rate (SFR), while the dependence is higher for galactic centres. We show that the morphological distortions visible in the radio total and polarized emission do not depend statistically on the global or local SFRs, while they do increase (especially in the polarization) with the advance of interaction. The constructed radio-far-infrared relations for interacting and non-interacting galaxies display a similar balance between the generation of cosmic rays, magnetic fields, and the production of the thermal energy and dust radiation. Conclusions. The regular magnetic fields are much more sensitive to morphological distortions induced by tidal interactions than are the random fields. As a result the polarized emission could be yet another indicator of an ongoing merging process. The found evolution of magnetic field with advancing interaction would definitely imply a stronger effect of magnetic fields on the galaxy surroundings in the earlier cosmological epochs. The process of strong gravitational interactions can efficiently magnetize the merger's surroundings, having a similar magnetizing effect on intergalactic medium as supernova explosions or galactic winds. If interacting galaxies generate some ultra-high energy cosmic rays (UHECRs), the disk or magnetized outflows can deflect them (up to 23 •), and make an association of the observed UHECRs with the sites of their origin very uncertain.},
author = {Drzazga, R T and Chy˙, K T and Jurusik, W and Wi{\'{o}}rkiewicz, K},
file = {:home/william/Documents/Papers/aa16092-10.pdf:pdf},
journal = {a{\&}a},
keywords = {galaxies,general – galaxies,interactions – radio continuum,magnetic fields – galaxies},
title = {{Magnetic field evolution in interacting galaxies}},
url = {https://www.aanda.org/articles/aa/pdf/2011/09/aa16092-10.pdf},
volume = {533},
year = {2011}
}
@incollection{Peterson2006,
abstract = {Reverberation mapping is a proven technique that is used to measure the size of the broad emission-line region and central black hole mass in active galactic nuclei. More ambitious reverberation mapping programs that are well within the capabilities of Hubble Space Telescope could allow us to determine the nature and flow of line-emitting gas in active nuclei and to assess accurately the systematic uncertainties in reverberation-based black hole mass measurements.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0407538},
author = {Peterson, B. M. and Horne, K.},
booktitle = {Planets to Cosmol. Essent. Sci. Final Years Hubble Sp. Telesc.},
doi = {10.1017/CBO9780511536328.009},
eprint = {0407538},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Peterson, Horne - 2006 - Reverberation mapping of active galactic nuclei.pdf:pdf},
isbn = {9780511536328},
issn = {0004-6280},
pages = {89--98},
pmid = {15003161},
primaryClass = {astro-ph},
title = {{Reverberation mapping of active galactic nuclei}},
volume = {9780521847},
year = {2006}
}
@article{Schawinski2015,
abstract = {We present an observational constraint for the typical active galactic nucleus (AGN) phase lifetime. The argument is based on the time lag between an AGN central engine switching on and becoming visible in X-rays, and the time the AGN then requires to photoionize a large fraction of the host galaxy. Based on the typical light travel time across massive galaxies, and the observed fraction of X-ray-selected AGN without AGN-photoionized narrow lines, we estimate that the AGN phase typically lasts {\~{}}105 yr. This lifetime is short compared to the total growth time of 107-109 yr estimated from e.g. the Soltan argument and implies that black holes grow via many such short bursts and that AGN therefore 'flicker' on and off. We discuss some consequences of this flickering behaviour for AGN feedback and the analogy of X-ray binaries and AGN lifecycles.},
archivePrefix = {arXiv},
arxivId = {1505.06733},
author = {Schawinski, Kevin and Koss, Michael and Berney, Simon and Sartori, Lia F.},
doi = {10.1093/mnras/stv1136},
eprint = {1505.06733},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Schawinski et al. - 2015 - Active galactic nuclei flicker An observational estimate of the duration of black hole growth phases of {\~{}}105.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: Seyfert,Galaxies: active,Quasars: general},
number = {3},
pages = {2517--2523},
title = {{Active galactic nuclei flicker: An observational estimate of the duration of black hole growth phases of {\~{}}10⁵ yr}},
volume = {451},
year = {2015}
}
@article{Pogge2011,
author = {Pogge, Richard W},
file = {:home/william/Documents/Papers/Intro.pdf:pdf},
journal = {Osu Ast871},
pages = {1--25},
title = {{Ch. 1 - Introduction to the Interstellar Medium}},
url = {http://www.astronomy.ohio-state.edu/{~}pogge/Ast871/Notes/Intro.pdf{\%}5Cnpapers2://publication/uuid/0A47944A-0ACC-4021-B7A0-641FA416EC18},
year = {2011}
}
@article{Morganti2021,
abstract = {We present an update of our ongoing project to characterise the impact of radio jets on the interstellar medium (ISM). This is done by tracing the distribution, kinematics and excitation of the molecular gas at high spatial resolution using ALMA. The radio active galactic nuclei (AGN) studied are in the interesting phase of having a recently born radio jet. In this stage, the plasma jets can have the largest impact on the ISM, as also predicted by state-of-the-art simulations. The two targets we present have quite different ages, allowing us to get snapshots of the effects of radio jets as they grow and evolve. Interestingly, both also host powerful quasar emission, making them ideal for studying the full impact of AGN. The largest mass outflow rate of molecular gas is found in a radio galaxy () hosting a newly born radio jet still in the early phase of emerging from an obscuring cocoon of gas and dust. Although the molecular mass outflow rate is high (few hundred), the outflow is limited to the inner few hundred pc region. In a second object (), the jet is larger (a few kpc) and is in a more advanced evolutionary phase. In this object, the distribution of the molecular gas is reminiscent of what is seen, on larger scales, in cool-core clusters hosting radio galaxies. Interestingly, gas deviating from quiescent kinematics (possibly indicating an outflow) is not very prominent, limited only to the very inner region, and has a low mass outflow rate. Instead, on kpc scales, the radio lobes appear associated with depressions in the distribution of the molecular gas. This suggests that the lobes have broken out from the dense nuclear region. However, the AGN does not appear to be able, at present, to stop the star formation observed in this galaxy. These results support the idea that the effects of the radio source start in the very first phases by producing outflows which, however, tend to be limited to the kpc region. After that, the effects turn into producing large-scale bubbles which could, in the long term, prevent the surrounding gas from cooling. Thus, our results provide a way to characterise the effect of radio jets in different phases of their evolution and in different environments, bridging the studies done for radio galaxies in clusters.},
archivePrefix = {arXiv},
arxivId = {2005.04765},
author = {Morganti, Raffaella and Oosterloo, Tom and Tadhunter, Clive N.},
doi = {10.1017/S1743921320001775},
eprint = {2005.04765},
file = {:home/william/Documents/Papers/2109.13516.pdf:pdf},
issn = {17439221},
journal = {Proc. Int. Astron. Union},
keywords = {ISM: jets and outflows,galaxies: active,galaxies: jets,radio continuum: galaxies},
pages = {243--248},
title = {{Taking snapshots of the jet-ISM interplay with ALMA}},
volume = {359},
year = {2021}
}

@article{2002A&A...392..267R,
author = {Raga, A.{\~{}}C. and {de Gouveia Dal Pino}, E.{\~{}}M. and Noriega-Crespo, A and Mininni, P.{\~{}}D. and Vel{\'{a}}zquez, P.{\~{}}F.},
doi = {10.1051/0004-6361:20020851},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Raga et al. - 2002 - Jetcloud collision, 3D gasdynamic simulations of HH 110.pdf:pdf},
journal = {aap},
keywords = {ISM: Herbig-Haro objects,ISM: individual (HH 110),ISM: jets and outflows,ISM: kinematics and dynamics,shock waves},
pages = {267--276},
title = {{Jet/cloud collision, 3D gasdynamic simulations of HH 110}},
volume = {392},
year = {2002}
}
@article{Yoon2019,
abstract = {In AGN feedback study, it is crucial to precisely determine the accretion rate of AGN and properly adopt the AGN physics, since they determine the AGN radiation and wind outputs. One key feature of such an AGN physics is that, depending on the value of the accretion rate, accretion is divided into two modes, namely hot and cold, corresponding to below and above {\$}2\backslash{\%} L{\_}{\{}\backslashrm Edd{\}}{\$} respectively. In this paper we investigate the role of the hot mode by performing hydrodynamical numerical simulations of AGN feedback in an isolated elliptical galaxy. We have run two test models. In one model, we always adopt the cold mode accretion physics no matter what value the accretion rate is; in another model, we turn off the AGN outputs once the accretion is in the hot mode. We have calculated the AGN light curves, black hole growth, star formation, and AGN energy duty-cycle and compared the results of these two models with the model in which the two modes are correctly taken into account. Important differences are found. For example, if we would adopt only the cold mode, compared to the model considering both modes, the AGN luminosity would become significantly smaller, the total mass of newly formed stars would become two orders of magnitude smaller, and the fraction of energy ejected within the high accretion regime (i.e., {\$}L{\_}{\{}\backslashrm BH{\}} {\textgreater} 2\backslash{\%} L{\_}{\{}\backslashrm Edd{\}}{\$}) would be very small ({\$}\backslashll 10{\^{}}{\{}-3{\}}{\$}), inconsistent with observations. These results strongly indicate the importance of hot mode feedback, which is because the time fraction of being in this mode is very large. We have also investigated the roles of wind and radiation in the hot mode and found that usually wind is more important than radiation; but, depending on the problem, radiation also cannot be neglected.},
archivePrefix = {arXiv},
arxivId = {1901.07570},
author = {Yoon, Doosoo and Yuan, Feng and Ostriker, Jeremiah P. and Ciotti, Luca},
eprint = {1901.07570},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Yoon et al. - 2019 - On the Role of Hot Feedback Mode in Active Galactic Nuclei Feedback in an Elliptical Galaxy.pdf:pdf},
keywords = {accretion,accretion disks - black,active - galaxies,evolution -,hole physics - galaxies},
title = {{On the Role of Hot Feedback Mode in Active Galactic Nuclei Feedback in an Elliptical Galaxy}},
url = {http://arxiv.org/abs/1901.07570},
year = {2019}
}
@article{Orienti2017,
author = {Orienti, Monica},
doi = {10.1164/rccm.200806-848OC},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/King et al. - 2017 - Fo r R iew On Fo r R iew On ly.pdf:pdf},
isbn = {9781509037582},
journal = {Proocedings, Perseus in Sicily},
pages = {1--60},
title = {{Extragalactic relativistic jets}},
year = {2017}
}
@article{Marchiolli1997,
abstract = {We begin by revisiting the so-called Caldirola-Kanai Hamiltonian and discuss its inherent ambiguity: does it represent a dissipative harmonic oscillator (HO) subject to a friction force, or does it describe an HO with a time-dependent mass (TDM)? Although classically both descriptions do coexist, in the quantum domain the solution of the Schr{\"{o}}dinger equation (or Heisenberg equations of motion) with a TDM does not present inconsistencies, however, the dissipative Hamiltonian shows violation of the Heisenberg uncertainty principle. This violation is avoided by introducing a stochastic force in the equations of motion, which will take care of the fluctuations due to the environment. Once the distinction between the dissipative and amplifying Hamiltonian is made clear, we consider the problem of the quantum TDM HO subject to dissipation, showing that both phenomena may be merged and described by a single Hamiltonian, the amplifying-dissipative Hamiltonian. We obtain the solutions of the Heisenberg equations of motion for the canonical momentum and position; next, we specialize on the weak damping limit and analyse the effects of the amplifying-dissipative process on the mean values of the physical variables.},
author = {Marchiolli, Marcelo A. and Mizrahi, Salomon S.},
doi = {10.1088/0305-4470/30/8/011},
file = {:home/william/Documents/Papers/marchiolli1997.pdf:pdf},
issn = {03054470},
journal = {J. Phys. A. Math. Gen.},
number = {8},
pages = {2619--2635},
title = {{Dissipative mass-accreting quantum oscillator}},
volume = {30},
year = {1997}
}
@article{Wagner2011,
abstract = {Over cosmic time, galaxies grow through the hierarchical merging of smaller galaxies. However, the bright region of the galaxy luminosity function is incompatible with the simplest version of hierarchical merging, and it is believed that feedback from the central black hole in the host galaxies reduces the number of bright galaxies and regulates the co-evolution of the black hole and host galaxy. Numerous simulations of galaxy evolution have attempted to include the physical effects of such feedback with a resolution usually exceeding a kiloparsec. However, interactions between jets and the interstellar medium involve processes occurring on less than kiloparsec scales. In order to further the understanding of processes occurring on such scales, we present a suite of simulations of relativistic jets interacting with a fractal two-phase interstellar medium with a resolution of two parsecs and a largest scale of one kiloparsec. The transfer of energy and momentum to the interstellar medium is considerable, and we find that jets with powers in the range of 10 43-1046 erg s-1 can inhibit star formation through the dispersal of dense gas in the galaxy core. We determine the effectiveness of this process as a function of the ratio of the jet power to the Eddington luminosity of the black hole, the pressure of the interstellar medium, and the porosity of the dense gas. {\textcopyright} 2011. The American Astronomical Society.},
archivePrefix = {arXiv},
arxivId = {astro-ph.CO/1012.1092},
author = {Wagner, A. Y. and Bicknell, G. V.},
doi = {10.1088/0004-637X/728/1/29},
eprint = {1012.1092},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Wagner, Bicknell - 2011 - Relativistic jet feedback in evolving galaxies.pdf:pdf},
isbn = {0004-637X},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {Galaxies: evolution,Galaxies: formation,Galaxies: jets,Hydrodynamics,ISM: jets and outflows,Methods: numerical},
number = {1},
primaryClass = {astro-ph.CO},
title = {{Relativistic jet feedback in evolving galaxies}},
volume = {728},
year = {2011}
}
@article{Deconto-Machado2022,
abstract = {We analyse the kinematics of 170 AGN host galaxies as compared to those of a matched control sample of non-active galaxies from the MaNGA survey in order to characterise and estimate the extents of the Narrow Line Region (NLR) and of the kinematically disturbed region (KDR) by the AGN. We define the observed NLR radius as the farthest distance from the nucleus within which both [Oiii]/H$\backslash$beta and [Nii]/H$\backslash$alpha ratios fall in the AGN region of the BPT diagram and the H$\backslash$alpha equivalent width is required to be larger than 3.0$\backslash$AA. The extent of the KDR is defined as the distance from the nucleus within which the AGN hosts galaxies shows a more disturbed gas kinematics than the control galaxies. The kinematics derived from the [Oiii] line profiles reveal that, on average, the most luminous AGN (L[Oiii] {\textgreater} 3.8 * 10{\^{}}40 erg s{\^{}}-1) possess higher residual difference between the gaseous and stellar velocities and velocities dispersion than their control galaxies. Spatially resolved NLR's and KDR's were found in 55 and 46 AGN host galaxies, with corrected radii 0.2 {\textless} r{\_}KDR,c {\textless} 2.3 kpc and 0.4 {\textless} r{\_}NLR,c {\textless} 10.1 kpc, with a relation between the two given by log r{\_}KDR,c = (0.53$\backslash$pm0.12) log r{\_}NLR,c + (1.07$\backslash$pm0.22), respectively. The extension of the KDR corresponds to about 30 per cent of that of the NLR. Assuming that the KDR is due to an AGN outflow, we have estimated ionised gas mass outflow rates that range between 10{\^{}}-5 and $\backslash$approx 1 Myr{\^{}}-1, and kinetic powers that range from 10{\^{}}34 to 10{\^{}}40 erg s{\^{}}-1. Comparing the power of the AGN ionised outflows with the AGN luminosities, they are always below the 0.05 L{\_}AGN model threshold for having an important feedback effect on their respective host galaxies. The mass outflow rates (and power) of our AGN sample correlate with their luminosities, populating the lowest AGN luminosity range of the correlations previously found for more powerful sources.},
archivePrefix = {arXiv},
arxivId = {2201.01690},
author = {Deconto-Machado, A. and Riffel, R. A. and Ilha, G. S. and Rembold, S. B. and Storchi-Bergmann, T. and Riffel, R. and Schimoia, J. S. and Schneider, D. P. and Bizyaev, D. and Feng, S. and Wylezalek, D. and da Costa, L. N. and do Nascimento, J. C. and Maia, M. A. G.},
doi = {10.1051/0004-6361/202140613},
eprint = {2201.01690},
file = {:home/william/Documents/Papers/2201.01690.pdf:pdf},
issn = {0004-6361},
keywords = {active,galaxies,general,kinematics and dynamics},
title = {{Ionised Gas Kinematics in MaNGA AGN. Extents of the Narrow Line and Kinematically Disturbed regions}},
url = {http://arxiv.org/abs/2201.01690},
year = {2022}
}
@article{Bruggen2002,
abstract = {Hot, X-ray-emitting plasma permeates clusters of galaxies. The X-ray surface brightness often shows a peak near the centre of the duster that is coincident with a drop in the entropy of the gas. This has been taken as evidence for a 'cooling flow', where the gas cools by radiating away its energy, and then falls to the centre. Searches for this cool gas have revealed significantly less than predicted, indicating that the mass deposition rate is much lower than expected. Most clusters with cooling flows, however, also host an active galactic nucleus at their centres. These active galactic nuclei can inflate large bubbles of hot plasma that subsequently rise through the cluster 'atmosphere', thus stirring the cooling gas and adding energy. Here we report highly resolved hydrodynamic simulations which show that buoyant bubbles increase the cooling time in the inner regions of clusters and significantly reduce the deposition of cold gas.},
author = {Br{\"{u}}ggen, Marcus and Kaiser, Christian R.},
doi = {10.1038/nature00857},
file = {:home/william/Documents/Papers/10.1038@nature00857.pdf:pdf},
issn = {00280836},
journal = {Nature},
number = {6895},
pages = {301--303},
title = {{Hot bubbles from active galactic nuclei as a heat source in cooling-flow clusters}},
volume = {418},
year = {2002}
}
@article{Baron2020a,
abstract = {Post-starburst E+A galaxies are systems that hosted a powerful starburst that was quenched abruptly. Simulations suggest that these systems provide the missing link between major merger ULIRGs and red and dead ellipticals, where AGN feedback is responsible for the expulsion or destruction of the molecular gas. However, many details remain unresolved and little is known about AGN-driven winds in this short-lived phase. We present spatially resolved IFU spectroscopy with MUSE/VLT of SDSS J124754.95-033738.6, a post-starburst E+A galaxy with a recent starburst that started 70 Myr ago and ended 30 Myr ago, with a peak SFR of {\$}\backslashsim 150\backslash, \backslashmathrm{\{}M{\_}{\{}\backslashodot {\}}\backslash,yr{\^{}}{\{} -1{\}}{\}}{\$}. We detect disturbed gas throughout the entire field of view, suggesting triggering by a minor merger. We detect fast-moving multiphased gas clouds, embedded in a double-cone face-on outflow, which are traced by ionized emission lines and neutral NaID emission and absorption lines. We find remarkable similarities between the kinematics, spatial extents, and line luminosities of the ionized and neutral gas phases, and propose a model in which they are part of the same outflowing clouds, which are exposed to both stellar and AGN radiation. Our photoionization model provides consistent ionized line ratios, NaID absorption optical depths and EWs, and dust reddening. Using the model, we estimate, for the first time, the neutral-to-ionized gas mass ratio (about 20), the sodium neutral fraction, and the size of the outflowing clouds. This is one of the best ever observed direct connections between the neutral and ionized outflow phases in AGN.},
archivePrefix = {arXiv},
arxivId = {2004.04749},
author = {Baron, Dalya and Netzer, Hagai and Davies, Ric I and {Xavier Prochaska}, J},
doi = {10.1093/mnras/staa1018},
eprint = {2004.04749},
file = {:home/william/Documents/Papers/staa1018.pdf:pdf},
issn = {0035-8711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {1 i n t,active,correlations between the masses,evolution,galaxies,general,interactions,of super,ro d u c,star formation,t i o n,the discovery of strong},
number = {4},
pages = {5396--5420},
publisher = {Oxford University Press},
title = {{Multiphase outflows in post-starburst E+A galaxies - II. A direct connection between the neutral and ionized outflow phases}},
volume = {494},
year = {2020}
}
@article{Miyoshi2005,
abstract = {A new multi-state Harten-Lax-van Leer (HLL) approximate Riemann solver for the ideal magnetohydrodynamic (MHD) equations is developed based on the assumption that the normal velocity is constant over the Riemann fan. This assumption is same as that used in the HLLC ("C" denotes Contact) approximate Riemann solver for the Euler equations. From the assumption, it is naturally derived that the Riemann fan should consist of four intermediate states for Bx≠ 0, whereas the number of the intermediate states is reduced to two when Bx= 0. Since the intermediate states satisfied with all jump conditions in this approximate Riemann system are analytically obtained, the multi-state HLL Riemann solver can be constructed straightforwardly. It is shown that this solver can exactly resolve isolated discontinuities formed in the MHD system, and hence named as HLLD Riemann solver. (Here, "D" stands for Discontinuities.) It is also analytically proved that the HLLD Riemann solver is positively conservative like the HLLC Riemann solver. Indeed, the HLLD Riemann solver corresponds to the HLLC Riemann solver when the magnetic field vanishes. Numerical tests demonstrate that the HLLD Riemann solver is more robust and efficient than the linearized Riemann solver, and its resolution is equally good. It indicates that the HLLD solver must be useful in practical applications for the ideal MHD equations. {\textcopyright} 2005 Elsevier Inc. All rights reserved.},
archivePrefix = {arXiv},
arxivId = {0501557},
author = {Miyoshi, Takahiro and Kusano, Kanya},
doi = {10.1016/j.jcp.2005.02.017},
eprint = {0501557},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Miyoshi, Kusano - 2005 - A multi-state HLL approximate Riemann solver for ideal magnetohydrodynamics.pdf:pdf},
isbn = {0021-9991},
issn = {00219991},
journal = {J. Comput. Phys.},
keywords = {Approximate Riemann solver,HLL,HLLC,HLLD,Magnetohydrodynamics,Positivity},
number = {1},
pages = {315--344},
title = {{A multi-state HLL approximate Riemann solver for ideal magnetohydrodynamics}},
volume = {208},
year = {2005}
}
@article{Soc2018,
author = {Soc, R},
doi = {00.0000/X000000000000000X},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Soc - 2018 - Fo r R iew On Fo r R iew On ly.pdf:pdf},
isbn = {0000000000000},
keywords = {cd,elliptical and lenticular,galaxies,hydrodynam-,ics,ism,nuclei,stellar dynamics},
title = {{Fo r R iew On Fo r R iew On ly}},
year = {2018}
}
@article{Belan2013,
abstract = {Context. In this paper we study the propagation of hypersonic hydrodynamic jets (Mach number {\textgreater}5) in a laboratory vessel and make comparisons with numerical simulations of axially symmetric flows with the same initial and boundary conditions. The astrophysical context is that of the jets originating around young stellar objects (YSOs). Aims. In order to gain a deeper insight into the phenomenology of YSO jets, we performed a set of experiments and numerical simulations of hypersonic jets in the range of Mach numbers from 10 to 20 and for jet-to-ambient density ratios from 0.85 to 5.4, using different gas species and observing jet lengths of the order of 150 initial radii or more. Exploiting the scalability of the hydrodynamic equations, we intend to reproduce the YSO jet behaviour with respect to jet velocity and elapsed times. In addition, we can make comparisons between the simulated, the experimental, and the observed morphologies. Methods. In the experiments the gas pressure and temperature are increased by a fast, quasi-isentropic compression by means of a piston system operating on a time scale of tens of milliseconds, while the gas density is visualized and measured by means of an electron beam system. We used the PLUTO software for the numerical solution of mixed hyperbolic/parabolic conservation laws targeting high Mach number flows in astrophysical fluid dynamics. We considered axisymmetric initial conditions and carried out numerical simulations in cylindrical geometry. The code has a modular flexible structure whereby different numerical algorithms can be separately combined to solve systems of conservation laws using the finite volume or finite difference approach based on Godunov-type schemes. Results. The agreement between experiments and numerical simulations is fairly good in most of the comparisons. The resulting scaled flow velocities and elapsed times are close to the ones shown by observations. The morphologies of the density distributions agree with the observed ones as well. Conclusions. The laboratory and the simulated hypersonic jets are all pressure matched, i.e. their axial regions are almost isentropic at the nozzle exit. They maintain their collimation for long distances in terms of the initial jet radii, without including magnetic confinement effects. This yields a qualitatively good agreement with the observed YSO jet morphologies. It remains to be seen what happens when non-axially symmetric perturbations of the flow are imposed at the nozzle, both in the experiment and in the simulation. {\textcopyright} ESO, 2013.},
author = {Belan, M. and Massaglia, S. and Tordella, D. and Mirzaei, M. and {De Ponte}, S.},
doi = {10.1051/0004-6361/201321040},
file = {:home/william/Documents/Papers/hyperjets.pdf:pdf},
issn = {00046361},
journal = {Astron. Astrophys.},
keywords = {Herbig-Haro objects,Hydrodynamics,ISM: jets and outflows,Shock waves,Stars: winds,outflows},
number = {June 2014},
title = {{The hydrodynamics of astrophysical jets: Scaled experiments and numerical simulations}},
volume = {554},
year = {2013}
}
@article{Nguyen2021,
abstract = {Cool clouds are expected to be destroyed and incorporated into hot supernova-driven galactic winds. The mass-loading of a wind by the cool medium modifies the bulk velocity, temperature, density, entropy, and abundance profiles of the hot phase relative to an un-mass-loaded outflow. We provide general equations and limits for this physics that can be used to infer the rate of cool gas entrainment from X-ray observations, accounting for non-spherical expansion. In general, mass-loading flattens the density and temperature profiles, decreases the velocity and increases the entropy if the Mach number is above a critical value. We first apply this model to a recent high-resolution galactic outflow simulation where the mass-loading can be directly inferred. We show that the temperature, entropy, and composition profiles are well-matched, providing evidence that this physics sets the bulk hot gas profiles. We then model the diffuse X-ray emission from the local starburst M82. The non-spherical (more cylindrical) outflow geometry is directly taken from the observed X-ray surface brightness profile. These models imply a total mass-loading rate that is about equal to that injected in the starburst, {\$}\backslashsimeq 10{\$} M{\$}{\_}\backslashodot{\$} yr{\$}{\^{}}{\{}-1{\}}{\$}, and they predict an asymptotic hot wind velocity of {\$}\backslashsim 1000\backslash,{\{}\backslashrm km \backslash s{\^{}}{\{}-1{\}}{\}}{\$} that is {\$}\backslashsim1.5-2{\$} times smaller than previous predictions. We also show how the observed entropy profile can be used to constrain the outflow velocity, making predictions for future missions like XRISM. We argue that the observed X-ray limb-brightening may be explained by mass-loading at the outflow's edges.},
archivePrefix = {arXiv},
arxivId = {2108.07343},
author = {Nguyen, Dustin D. and Thompson, Todd A.},
eprint = {2108.07343},
file = {:home/william/Documents/Papers/2108.07343.pdf:pdf},
keywords = {evolution,formation,galaxies,starburst,x-rays},
number = {August},
title = {{Mass-Loading and Non-Spherical Divergence in Hot Galactic Winds: Implications for X-ray Observations}},
url = {http://arxiv.org/abs/2108.07343},
volume = {000},
year = {2021}
}
@article{2012ApJ...757..136W,
archivePrefix = {arXiv},
arxivId = {1205.0542},
author = {Wagner, A.{\~{}}Y. and Bicknell, G.{\~{}}V. and Umemura, M},
doi = {10.1088/0004-637X/757/2/136},
eprint = {1205.0542},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Wagner, Bicknell, Umemura - 2012 - Driving outflows with relativistic jets and the dependence of active galactic nucleus feedback effici.pdf:pdf},
journal = {Apj},
keywords = {ISM: jets and outflows,galaxies: evolution,galaxies: formation,galaxies: jets,hydrodynamics,methods: numerical},
pages = {136},
title = {{Driving Outflows with Relativistic Jets and the Dependence of Active Galactic Nucleus Feedback Efficiency on Interstellar Medium Inhomogeneity}},
volume = {757},
year = {2012}
}
@article{.1375,
abstract = {Cosmetic products are generally formulated as emulsions, ointments, solutions or powders containing active ingredients. According to EU legislation, a cosmetic product is "any substance or preparation intended to be placed in contact with the various external parts of the human body with a view exclusively or mainly to cleaning, perfuming them, changing their appearance, and/or correcting body odors and/or protecting them or keeping them in good conditions". However, science advancement in both active carriers and ingredients has streamlined the process through which many cosmetic products by their delivery systems can induce modifications on the skin physiology. This is the reason why Reed and Kligman redefined these products as "cosmeceuticals", which refers to the combination of cosmetics and pharmaceuticals. Until recently, the term of cosmeceuticals has not had legal significance. The so-called cosmeceuticals, in fact, may induce modifications on the skin physiology, modifying, for example, transepidermal water loss, keratinocytes cohesion and turnover, modulating the inflammatory cascade, and/or altering the surface microbiota by the activity of the preservatives content. For these reasons, they are claimed to have medical or drug-like benefits. Naturally, their effectiveness on minor skin disorders or mild skin abnormalities has to be shown by in vitro and in vivo studies. On the other hand, their formulations contain emulsifiers, preservatives, and other chemicals which, by their cumulative use, may provoke side effects, such as allergic and/or sensitization phenomena. Moreover, many ingredients and packaging for such products are not biodegradable. In this study, we would like to introduce an innovative category of cosmeceuticals made by biodegradable nonwoven tissues. These cosmeceutical tissues, produced through the use of natural fibers, may bind different active ingredients and therefore become effective as antibacterial, anti-inflammatory, sun-protective, whitening, or anti-aging products, depending on the ingredient(s) used. Differently from the usual cosmetics, they do not contain preservatives, emulsifiers, colors, and other chemicals. They can be applied as dried tissue on wet skin, remaining in loco for around 30 min, slowly releasing the active ingredients entrapped into the fibers. It is interesting to underline that the tissue, acting as a carrier, has its own effectiveness via chitin and lignin polymers with an antibacterial and anti-inflammatory activity. When hydrolyzed by the human microbiota enzymes, they give rise to ingredients used as cell nourishment or energy. This paper will review part of the scientific research results, supporting this new category of biodegradable cosmetic products known as facial mask sheets.},
author = {{كريستينا، رود. كوكورس}},
file = {:home/william/Documents/Papers/1982MitAG..57..207D.pdf:pdf},
title = {{آموزش مهارت هاي ورزشي (راهنمايي مربيان)". ترجمة محمدتقي اقدسي، چاپ اول، دانشگاه تبريزNo Title}},
year = {1375}
}
@article{Fragile2004,
abstract = {Accumulating observational evidence for a number of radio galaxies suggests an association between their jets and regions of active star formation. The standard picture is that shocks generated by the jet propagate through an inhomogeneous medium and trigger the collapse of overdense clouds, which then become active star-forming regions. In this contribution, we report on recent hydrodynamic simulations of radiative shock-cloud interactions using two different cooling models: an equilibrium cooling-curve model assuming solar metallicities and a non-equilibrium chemistry model appropriate for primordial gas clouds. We consider a range of initial cloud densities and shock speeds in order to quantify the role of cooling in the evolution. Our results indicate that for moderate cloud densities ({\textgreater}1 cm{\^{}}{\{}-3{\}}) and shock Mach numbers ({\textless}20), cooling processes can be highly efficient and result in more than 50{\%} of the initial cloud mass cooling to below 100 K. We also use our results to estimate the final H{\_}2 mass fraction for the simulations that use the non-equilibrium chemistry package. This is an important measurement, since H{\_}2 is the dominant coolant for a primordial gas cloud. We find peak H{\_}2 mass fractions of {\textgreater}0.01 and total H{\_}2 mass fractions of {\textgreater}10{\^{}}{\{}-5{\}} for the cloud gas. Finally, we compare our results with the observations of jet-induced star formation in ``Minkowski's Object.'' We conclude that its morphology, star formation rate ({\~{}} 0.3M{\_}solar/yr) and stellar mass ({\~{}} 1.2 x 10{\^{}}7 M{\_}solar) can be explained by the interaction of a 90,000 km/s jet with an ensemble of moderately dense ({\~{}} 10 cm{\^{}}{\{}-3{\}}), warm (10{\^{}}4 K) intergalactic clouds in the vicinity of its associated radio galaxy at the center of the galaxy cluster.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0311298},
author = {Fragile, P. Chris and Murray, Stephen D. and Anninos, Peter and van Breugel, Wil},
doi = {10.1086/381726},
eprint = {0311298},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Fragile et al. - 2004 - Radiative Shock–induced Collapse of Intergalactic Clouds.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
number = {1},
pages = {74--87},
primaryClass = {astro-ph},
title = {{Radiative Shock–induced Collapse of Intergalactic Clouds}},
url = {http://stacks.iop.org/0004-637X/604/i=1/a=74},
volume = {604},
year = {2004}
}
@article{Teng2015,
abstract = {We present a Nuclear Spectroscopic Telescope Array (NuSTAR), Chandra, and XMM-Newton survey of nine of the nearest ultraluminous infrared galaxies (ULIRGs). The unprecedented sensitivity of NuSTAR at energies above 10 keV enables spectral modeling with far better precision than was previously possible. Six of the nine sources observed were detected sufficiently well by NuSTAR to model in detail their broadband X-ray spectra, and recover the levels of obscuration and intrinsic X-ray luminosities. Only one source (IRAS 13120-5453) has a spectrum consistent with a Compton-thick active galactic nucleus (AGN), but we cannot rule out that a second source (Arp 220) harbors an extremely highly obscured AGN as well. Variability in column density (reduction by a factor of a few compared to older observations) is seen in IRAS 05189-2524 and Mrk 273, altering the classification of these borderline sources from Compton-thick to Compton-thin. The ULIRGs in our sample have surprisingly low observed fluxes in high-energy ({\textgreater}10 keV) X-rays, especially compared to their bolometric luminosities. They have lower ratios of unabsorbed 2-10 keV to bolometric luminosity, and unabsorbed 2-10 keV to mid-IR [O iv] line luminosity than do Seyfert 1 galaxies. We identify IRAS 08572+3915 as another candidate intrinsically X-ray weak source, similar to Mrk 231. We speculate that the X-ray weakness of IRAS 08572+3915 is related to its powerful outflow observed at other wavelengths.},
archivePrefix = {arXiv},
arxivId = {1510.04453},
author = {Teng, Stacy H. and Rigby, Jane R. and Stern, Daniel and Ptak, Andrew and Alexander, D. M. and Bauer, Franz E. and Boggs, Stephen E. and Brandt, W. Niel and Christensen, Finn E. and Comastri, Andrea and Craig, William W. and Farrah, Duncan and Gandhi, Poshak and Hailey, Charles J. and Harrison, Fiona A. and Hickox, Ryan C. and Koss, Michael and Luo, Bin and Treister, Ezequiel and Zhang, William W.},
doi = {10.1088/0004-637X/814/1/56},
eprint = {1510.04453},
file = {:home/william/Documents/Papers/Teng{\_}2015{\_}ApJ{\_}814{\_}56.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {X-rays: galaxies,galaxies: active},
number = {1},
pages = {56},
publisher = {IOP Publishing},
title = {{A NuSTAR survey of nearby ultraluminous infrared galaxies}},
url = {http://dx.doi.org/10.1088/0004-637X/814/1/56},
volume = {814},
year = {2015}
}
@article{ArcaSedda2020,
abstract = {The detection of gravitational waves emitted during a neutron star–black hole merger and the associated electromagnetic counterpart will provide a wealth of information about stellar evolution nuclear matter, and general relativity. While the theoretical framework about neutron star–black hole binaries formed in isolation is well established, the picture is loosely constrained for those forming via dynamical interactions. Here, we use N-body simulations to show that mergers forming in globular and nuclear clusters could display distinctive marks compared to isolated mergers, namely larger masses, heavier black holes, and the tendency to have no associated electromagnetic counterpart. These features could represent a useful tool to interpreting forthcoming observations. In the local Universe, gravitational waves emitted from dynamical mergers could be unraveled by detectors sensitive in the decihertz frequency band, while those occurring at the distance range of Andromeda and the Virgo Cluster could be accessible to lower-frequency detectors like LISA.},
archivePrefix = {arXiv},
arxivId = {2003.02279},
author = {{Arca Sedda}, Manuel},
doi = {10.1038/s42005-020-0310-x},
eprint = {2003.02279},
file = {:home/william/Documents/Papers/s42005-020-0310-x.pdf:pdf},
isbn = {4200502003},
issn = {23993650},
journal = {Commun. Phys.},
number = {1},
pages = {1--10},
publisher = {Springer US},
title = {{Dissecting the properties of neutron star–black hole mergers originating in dense star clusters}},
url = {http://dx.doi.org/10.1038/s42005-020-0310-x},
volume = {3},
year = {2020}
}
@article{Sutherland2007,
abstract = {We present three-dimensional simulations of the interaction of a light hypersonic jet with an inhomogeneous thermal and turbulently supported disk in an elliptical galaxy. These simulations are applicable to the GPS/CSS phase of extragalactic radio sources. The interstellar medium in these simulations consists of a conventional hot (T{\~{}}107 K) component together with a warm (T{\~{}}104 K) turbulently supported disk whose local density is described by a lognormal density distribution and whose spatial structure is realized from a fractal power law. We model the jet as a light, supersonic nonrelativistic flow with parameters selected to be consistent with a relativistic jet with kinetic power just above the FR1/FR2 break. We identify four generic phases in the evolution of such a jet with the inhomogeneous interstellar medium: (1) an initial ``flood and channel'' phase, where progress is characterized by high-pressure gas finding changing weak points in the ISM, flowing through channels that form and reform over time; (2) a spherical, energy-driven bubble phase, where the bubble is larger than the disk scale, but the jet remains fully disrupted close to the nucleus; (3) a subsequent, rapid, jet break-out phase where the jet breaks free of the last obstructing dense clouds, becomes collimated once more, and pierces the spherical bubble; and (4) a classical phase, where the jet propagates in a momentum-dominated fashion similar to jets in single-component hot halos, leading to the classical jet-cocoon-bow shock structure. Mass transport in the simulations is investigated, and we propose a model for the morphology and component proper motions in the well-studied compact symmetric object 4C 31.04.},
author = {Sutherland, Ralph S. and Bicknell, Geoffrey V.},
doi = {10.1086/520640},
file = {:home/william/Documents/Papers/Sutherland{\_}2007{\_}ApJS{\_}173{\_}37.pdf:pdf},
issn = {0067-0049},
journal = {Astrophys. J. Suppl. Ser.},
number = {1},
pages = {37--69},
title = {{Interactions of a Light Hypersonic Jet with a Nonuniform Interstellar Medium}},
volume = {173},
year = {2007}
}
@article{Voit2015,
abstract = {The Universe's largest galaxies reside at the centres of galaxy clusters and are embedded in hot gas that, if left undisturbed, would cool quickly and create many more new stars than are actually observed. Cooling can be regulated by feedback from accretion of cooling gas onto the central black hole, but requires an accretion rate finely tuned to the thermodynamic state of the hot gas. Theoretical models in which cold clouds precipitate out of the hot gas via thermal instability and accrete onto the black hole exhibit the necessary tuning. Recent observational evidence shows that the abundance of cold gas in the centres of clusters increases rapidly near the predicted threshold for instability. Here we report observations showing that this precipitation threshold extends over a large range in cluster radius, cluster mass and cosmic time. We incorporate the precipitation threshold into a framework of theoretical models for the thermodynamic state of hot gas in galaxy clusters. According to that framework, precipitation regulates star formation in some giant galaxies, while thermal conduction prevents star formation in others if it can compensate for radiative cooling and shut off precipitation.},
archivePrefix = {arXiv},
arxivId = {1409.1598},
author = {Voit, G. M. and Donahue, M. and Bryan, G. L. and McDonald, M.},
doi = {10.1038/nature14167},
eprint = {1409.1598},
file = {:home/william/Documents/Papers/voit2015.pdf:pdf},
issn = {14764687},
journal = {Nature},
number = {7542},
pages = {203--206},
publisher = {Nature Publishing Group},
title = {{Regulation of star formation in giant galaxies by precipitation, feedback and conduction}},
url = {http://dx.doi.org/10.1038/nature14167},
volume = {519},
year = {2015}
}
@article{Jones2018,
abstract = {We present Far-Infrared polarimetry observations of M82 at 53 and {\$}154{\~{}}\backslashmu \backslashrm{\{}m{\}}{\$} and NGC 253 at {\$}89{\~{}}\backslashmu \backslashrm{\{}m{\}}{\$}, which were taken with HAWC+ in polarimetry mode on the Stratospheric Observatory for Infrared Astronomy (SOFIA). The polarization of M82 at {\$}53{\~{}}\backslashmu \backslashrm{\{}m{\}}{\$} clearly shows a magnetic field geometry perpendicular to the disk in the hot dust emission. For M82 the polarization at {\$}154{\~{}}\backslashmu \backslashrm{\{}m{\}}{\$} shows a combination of field geometry perpendicular to the disk in the nuclear region, but closer to parallel to the disk away from the nucleus. The fractional polarization at {\$}53{\~{}}\backslashmu \backslashrm{\{}m{\}}{\$} {\$}(154{\~{}}\backslashmu \backslashrm{\{}m{\}}){\$} ranges from 7{\%} (3{\%}) off nucleus to 0.5{\%} (0.3{\%}) near the nucleus. A simple interpretation of the observations of M82 invokes a massive polar outflow, dragging the field along, from a region {\$}\backslashsim 700{\$}{\~{}}pc in diameter that has entrained some of the gas and dust, creating a vertical field geometry seen mostly in the hotter {\$}(53{\~{}}\backslashmu \backslashrm{\{}m{\}}){\$} dust emission. This outflow sits within a larger disk with a more typical planar geometry that more strongly contributes to the cooler {\$}(154{\~{}}\backslashmu \backslashrm{\{}m{\}}){\$} dust emission. For NGC 253, the polarization at {\$}89{\~{}}\backslashmu \backslashrm{\{}m{\}}{\$} is dominated by a planar geometry in the tilted disk, with weak indication of a vertical geometry above and below the plane from the nucleus. The polarization observations of NGC 253 at {\$}53{\~{}}\backslashmu \backslashrm{\{}m{\}}{\$} were of insufficient S/N for detailed analysis.},
archivePrefix = {arXiv},
arxivId = {1812.06816},
author = {Jones, Terry Jay and Dowell, C. Darren and Rodriguez, Enrique Lopez and Zweibel, Ellen G. and Berthoud, Marc and Chuss, David T. and Goldsmith, Paul F. and Hamilton, Ryan T. and Hanany, Shaul and Harper, Doyal A. and Lazarian, 7 Alex and Looney, Leslie W. and Michail, Joseph M. and Morris, Mark R. and Novak, Giles and Santos, Fabio P. and Sheth, Kartik and Stacey, Gordon J. and Staguhn, Johannes and Stephens, Ian W. and Tassis, Konstantinos and Trinh, Christopher Q. and Volpert, C. G. and Werner, Michael and Wollack, Edward J.},
doi = {10.3847/2041-8213/aaf8b9},
eprint = {1812.06816},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Jones et al. - 2018 - SOFIA Far Infrared Imaging Polarimetry of M82 and NGC 253 Exploring the Super-Galactic Wind.pdf:pdf},
issn = {2041-8213},
title = {{SOFIA Far Infrared Imaging Polarimetry of M82 and NGC 253: Exploring the Super-Galactic Wind}},
url = {http://arxiv.org/abs/1812.06816},
year = {2018}
}
@article{Lutz2020,
abstract = {We report new detections and limits from a NOEMA and ALMA CO(1-0) search for molecular outflows in 13 local galaxies with high far-infrared surface brightness, and combine these with local universe CO outflow results from the literature. The CO line ratios and spatial outflow structure of our targets provide some constraints on the conversion steps from observables to physical quantities such as molecular mass outflow rates. Where available, ratios between outflow emission in higher J CO transitions and in CO(1-0) are typically consistent with excitation Ri1-1. However, for IRAS 13120-5453, R31 = 2.10 ± 0.29 indicates optically thin CO in the outflow. Like much of the outflow literature, we use $\alpha$CO(1?- 0) = 0.8, and we present arguments for using C = 1 in deriving molecular mass outflow rates ° out = CMoutvout/Rout. We compare the two main methods for molecular outflow detection: CO millimeter interferometry and Herschel OH-based spectroscopic outflow searches. For 26 sources studied with both methods, we find an 80{\%} agreement in detecting vout 150 km s-1 outflows, and non-matches can be plausibly ascribed to outflow geometry and signal-to-noise ratio. For a published sample of 12 bright ultraluminous infrared galaxies with detailed OH-based outflow modeling, CO outflows are detected in all but one. Outflow masses, velocities, and sizes for these 11 sources agree well between the two methods, and modest remaining differences may relate to the different but overlapping regions sampled by CO emission and OH absorption. Outflow properties correlate better with active galactic nucleus (AGN) luminosity and with bolometric luminosity than with far-infrared surface brightness. The most massive outflows are found for systems with current AGN activity, but significant outflows in nonAGN systems must relate to star formation or to AGN activity in the recent past. We report scaling relations for the increase of outflow mass, rate, momentum rate, and kinetic power with bolometric luminosity. Short flow times of ∼106 yr and some sources with resolved multiple outflow episodes support a role of intermittent driving, likely by AGNs.},
archivePrefix = {arXiv},
arxivId = {1911.05608},
author = {Lutz, D. and Sturm, E. and Janssen, A. and Veilleux, S. and Aalto, S. and Cicone, C. and Contursi, A. and Davies, R. I. and Feruglio, C. and Fischer, J. and Fluetsch, A. and Garcia-Burillo, S. and Genzel, R. and Gonz{\'{a}}lez-Alfonso, E. and Graci{\'{a}}-Carpio, J. and Herrera-Camus, R. and Maiolino, R. and Schruba, A. and Shimizu, T. and Sternberg, A. and Tacconi, L. J. and Wei{\ss}, A.},
doi = {10.1051/0004-6361/201936803},
eprint = {1911.05608},
file = {:home/william/Documents/Papers/1911.05608.pdf:pdf},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Galaxies: ISM,Galaxies: active,Galaxies: kinematics and dynamics},
number = {36803},
pages = {1--37},
title = {{Molecular outflows in local galaxies: Method comparison and a role of intermittent AGN driving}},
volume = {633},
year = {2020}
}
@article{Fukumura2010a,
abstract = {We present the two-dimensional ionization structure of self-similar magnetohydrodynamic winds off accretion disks around and irradiated by a central X-ray point source. On the basis of earlier observational clues and theoretical arguments, we focus our attention on a subset of these winds, namely those with radial density dependence n(r) ∝ 1/r (r is the spherical radial coordinate). We employ the photoionization code XSTAR to compute the ionic abundances of a large number of ions of different elements and then compile their line-of-sight (LOS) absorption columns. We focus our attention on the distribution of the column density of the various ions as a function of the ionization parameter $\xi$ (or equivalently r) and the angle $\theta$ . Particular attention is paid to the absorption mea-sure distribution (AMD), namely their hydrogen-equivalent column per logarithmic $\xi$ interval, dN H /dlog $\xi$ , which provides a measure of the winds' radial density profiles. For the chosen density profile n(r) ∝ 1/r, the AMD is found to be independent of $\xi$ , in good agreement with its behavior inferred from the X-ray spectra of several active galactic nuclei (AGNs). For the specific wind structure and X-ray spectrum, we also compute detailed absorption line profiles for a number of ions to obtain their LOS velocities, v ∼ 100–300 km s −1 (at log $\xi$ ∼ 2–3) for Fe xvii and v ∼ 1000–4000 km s −1 (at log $\xi$ ∼ 4–5) for Fe xxv, in good agreement with the observation. Our models describe the X-ray absorption properties of these winds with only two parameters, namely the mass-accretion rate ˙ m and the LOS angle $\theta$ . The probability of obscuration of the X-ray ionizing source in these winds decreases with increasing ˙ m and increases steeply with the LOS inclination angle $\theta$ . As such, we concur with previous authors that these wind configurations, viewed globally, incorporate all the requisite properties of the parsec scale " torii " invoked in AGN unification schemes. We indicate that a combination of the AMD and absorption line profile observations can uniquely determine these model parameters and their bearing on AGN population demographics.},
archivePrefix = {arXiv},
arxivId = {0910.3001},
author = {Fukumura, Keigo and Kazanas, Demosthenes and Contopoulos, Ioannis and Behar, Ehud},
doi = {10.1088/0004-637X/715/1/636},
eprint = {0910.3001},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Fukumura et al. - 2010 - Magnetohydrodynamic accretion disk winds as X-ray absorbers in active galactic nuclei.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {Accretion,Accretion disks,Galaxies: active,Methods: numerical,Quasars: absorption lines,X-rays: galaxies},
number = {1},
pages = {636--650},
title = {{Magnetohydrodynamic accretion disk winds as X-ray absorbers in active galactic nuclei}},
volume = {715},
year = {2010}
}
@misc{Yin2004,
abstract = {A sequential injection system which consists of a syringe pump, a selector valve, a multi-port valve, a gas-liquid separator and a solenoid valve for the determination of arsenic by hydride generation atomic absorption spectrometry using tetrahydroborate as reductant was developed. The reduction time of sample with tetrahydoborate has increased by keeping the reactant in gas-liquid separator by using the solenoid valve. Various parameters affecting the performance of the sequential injection system were optimized, including reaction-time, carrier gas flow, sample volume, tetrahydroborate volume and concentration. Established sequential injection hydride generation technique was simple and automated operation. A sample throughput of 112/h was achieved with 400 $\mu$L samples with a precision of 2.0{\%} RSD at 4 $\mu$g/L As (n = 10) and a detection limit of 0.09 $\mu$g/L. Good agreement with the certified values was obtained for the determination of arsenic in standard reference materials.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Nathan, Andrew J. and Scobell, Andrew},
booktitle = {Foreign Aff.},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Yin, Zhang, Wang - 2004 - Sequential injection analysis system for the determination of arsenic by hydride generation atomic absorption.pdf:pdf},
isbn = {9788578110796},
issn = {00157120},
keywords = {Arsenic,Hydride generation atomic absorption spectrometry,Sequential injection},
number = {5},
pages = {1365--1367},
pmid = {25246403},
title = {{How China sees America}},
volume = {91},
year = {2012}
}
@article{VanEldik2015a,
abstract = {Abstract During the last decades, increasingly precise astronomical observations of the Galactic Centre (GC) region at radio, infrared, and X-ray wavelengths laid the foundations to a detailed understanding of the high energy astroparticle physics of this most remarkable location in the Galaxy. Recently, observations of this region in high energy (HE, 10 MeV-100 GeV) and very high energy (VHE, {\textgreater} 100 GeV) $\gamma$-rays added important insights to the emerging picture of the Galactic nucleus as a most violent and active region where acceleration of particles to very high energies - possibly up to a PeV - and their transport can be studied in great detail. Moreover, the inner Galaxy is believed to host large concentrations of dark matter (DM), and is therefore one of the prime targets for the indirect search for $\gamma$-rays from annihilating or decaying dark matter particles. In this article, the current understanding of the $\gamma$-ray emission emanating from the GC is summarised and the results of recent DM searches in HE and VHE $\gamma$-rays are reviewed.},
author = {{Van Eldik}, Christopher},
doi = {10.1016/j.astropartphys.2015.05.002},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Van Eldik - 2015 - Gamma rays from the Galactic Centre region A review.pdf:pdf},
issn = {09276505},
journal = {Astropart. Phys.},
keywords = {Dark matter: annihilation,Dark matter: indirect detection,Galaxy: centre,Galaxy: star formation,Gamma rays: observations},
pages = {45--70},
publisher = {Elsevier Ltd.},
title = {{Gamma rays from the Galactic Centre region: A review}},
url = {http://dx.doi.org/10.1016/j.astropartphys.2015.05.002},
volume = {71},
year = {2015}
}
@article{Maiti1981,
abstract = {The paper presents a study of the observations and theory which are relevant to the presently popular behef that the solar-flare phenomenon is a direct consequence of the annihilation of magnetic fields on the sun. There is very little in the observations to support such views. A systematic study of the known theoretical mechanisms for the diffusion, reconnection, and annihilation of magnetic fields is presented. The mechanisms discussed are Joule dissipation, ambipolar diffusion, and various forms of Sweet's mechanism. It is shown that Sweet's mechanism is much more effective in a highly compressible medium if the merging magnetic fields are exactly antiparallel. None of the known mechanisms are sufficiently rapid to account for the solar flare from the annihilation of magnetic fields. Errors and omissions in earlier discussions of the problem are cited. Since no possible energy source other than magnetic fields has yet been developed, the question of field annihilation remains both open and pressing. The possibilities of runaway electrons and hydrodynamic instability, as means for hastening magnetic- field annihilation, are considered. It is shown that there is no reason to expect runaway electrons and no effective instability unless the fields are exactly antiparallel. The observational and theoretical difficulties with the hypothesis of magnetic-field annihilation sug- gest that other alternatives for the flare must be explored. I.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Parker, E.N.},
doi = {10.1128/AAC.03728-14},
eprint = {arXiv:1011.1669v3},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Parker - 1962 - No Title.pdf:pdf},
isbn = {9788578110796},
issn = {10986596},
journal = {Apjs},
keywords = {icle},
pages = {177--211},
pmid = {25246403},
title = {{THE SOLAR-FLARE PHENOMENON AND THE THEORY OF RECONNECTION AND ANNIHILATION OF MAGNETIC FIELDS}},
year = {1962}
}
@article{Perna2020,
abstract = {Context. Arp220 is the nearest and prototypical ultra-luminous infrared galaxy; it shows evidence of pc-scale molecular outflows in its nuclear regions and strongly perturbed ionised gas kinematics on kpc scales. It is therefore an ideal system for investigating outflow mechanisms and feedback phenomena in detail. Aims. We investigate the feedback effects on the Arp220 interstellar medium (ISM), deriving a detailed picture of the atomic gas in terms of physical and kinematic properties, with a spatial resolution that had never before been obtained (0.56″, i.e. ∼210 pc). Methods. We use optical integral-field spectroscopic observations from VLT/MUSE-AO to obtain spatially resolved stellar and gas kinematics, for both ionised ([N II]$\lambda$6583) and neutral (Na ID$\lambda$ $\lambda$589196) components; we also derive dust attenuation, electron density, ionisation conditions, and hydrogen column density maps to characterise the ISM properties. Results. Arp220 kinematics reveal the presence of a disturbed kpc-scale disc in the innermost nuclear regions as well as highly perturbed multi-phase (neutral and ionised) gas along the minor axis of the disc, which we interpret as a galactic-scale outflow emerging from the Arp220 eastern nucleus. This outflow involves velocities up to ∼1000 km s-1 at galactocentric distances of ≈5 kpc; it has a mass rate of ∼50 M- yr-1 and kinetic and momentum power of ∼1043 erg s-1 and ∼1035 dyne, respectively. The inferred energetics do not allow us to distinguish the origin of the outflows, namely whether they are active galactic nucleus- or starburst-driven. We also present evidence for enhanced star formation at the edges of - and within - the outflow, with a star-formation rate SFR ∼5 M- yr-1 (i.e. ∼2{\%} of the total SFR). Conclusions. Our findings suggest the presence of powerful winds in Arp220: They might be capable of heating or removing large amounts of gas from the host ("negative feedback") but could also be responsible for triggering star formation ("positive feedback").},
archivePrefix = {arXiv},
arxivId = {2009.03353},
author = {Perna, M. and Arribas, S. and Catal{\'{a}}n-Torrecilla, C. and Colina, L. and Bellocchi, E. and Fluetsch, A. and Maiolino, R. and Cazzoli, S. and {Hern{\'{a}}n Caballero}, A. and {Pereira Santaella}, M. and {Piqueras L{\'{o}}pez}, J. and {Rodr{\'{i}}guez Del Pino}, B.},
doi = {10.1051/0004-6361/202038328},
eprint = {2009.03353},
file = {:home/william/Documents/Papers/2009.03353.pdf:pdf},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Galaxies: ISM,Galaxies: active,Galaxies: individual: Arp 220,Galaxies: starburst},
title = {{MUSE view of Arp220: Kpc-scale multi-phase outflow and evidence for positive feedback}},
volume = {643},
year = {2020}
}
@article{Perna2021,
abstract = {Context. Ultraluminous infrared galaxies (ULIRGs) are characterised by extreme starburst (SB) and active galactic nucleus (AGN) activity, and are therefore ideal laboratories for studying the outflow phenomena and their feedback effects. We have recently started a project called Physics of ULIRGs with MUSE and ALMA (PUMA), which is a survey of 25 nearby (z {\textless} 0.165) ULIRGs observed with the integral field spectrograph MUSE and the interferometer ALMA. This sample includes systems with both AGN and SB nuclear activity in the pre- and post-coalescence phases of major mergers. Aims. The main goals of the project are (i) to study the prevalence of (ionised, neutral, and molecular) outflows as a function of the galaxy properties, (ii) to constrain the driving mechanisms of the outflows (e.g. distinguish between SB and AGN winds), and (iii) to identify and characterise feedback effects on the host galaxy. In this first paper, we present details on the sample selection, MUSE observations, and data reduction, and derive first high-level data products. Methods. MUSE data cubes were analysed to study the dynamical status of each of the 21 ULIRGs observed so far, taking the stellar kinematics and the morphological properties inferred from MUSE narrow-band images into account. We also located the ULIRG nuclei, taking advantage of near-infrared (HST) and millimeter (ALMA) data, and studied their optical spectra to infer (i) the ionisation state through standard optical line ratio diagnostics, and (ii) outflows in both atomic ionised ([O III], H$\alpha$) and neutral (Na ID) gas. Results. We show that the morphological and stellar kinematic classifications are consistent: post-coalescence systems are more likely associated with ordered motions, while interacting (binary) systems are dominated by non-ordered and streaming motions. We also find broad and asymmetric [O III] and Na ID profiles in almost all nuclear spectra, with line widths in the range [300 - 2000] km s-1, possibly associated with AGN- and SB-driven winds. This result reinforces previous findings that indicated that outflows are ubiquitous during the pre- and post-coalescence phases of major mergers.},
archivePrefix = {arXiv},
arxivId = {2011.11676},
author = {Perna, M. and Arribas, S. and {Pereira Santaella}, M. and Colina, L. and Bellocchi, E. and Catal{\'{a}}n-Torrecilla, C. and Cazzoli, S. and {Crespo G{\'{o}}mez}, A. and Maiolino, R. and {Piqueras L{\'{o}}pez}, J. and {Rodr{\'{i}}guez Del Pino}, B.},
doi = {10.1051/0004-6361/202039702},
eprint = {2011.11676},
file = {:home/william/Documents/Papers/2011.11676.pdf:pdf},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Galaxies: ISM,Galaxies: active,Galaxies: interactions,Galaxies: starburst},
number = {39702},
title = {{Physics of ULIRGs with MUSE and ALMA: The PUMA project: I. Properties of the survey and first MUSE data results}},
volume = {646},
year = {2021}
}
@article{Dugan2017,
abstract = {To investigate the differences in mechanical feedback from radio-loud and radio-quiet Active Galactic Nuclei (AGN) on the host galaxy, we perform 3D AMR hydrodynamic simulations of wide angle, radio-quiet winds with different inclinations on a single, massive, gas-rich disk galaxy at a redshift of 2-3. We compare our results to hydrodynamic simulations of the same galaxy but with a jet. The jet has an inclination of 0 degrees (perpendicular to the galactic plane), and the winds have inclinations of 0, 45, and 90 degrees. We analyze the impact on the host's gas, star formation, and circum-galactic medium. We find that jet feedback is energy-driven and wind feedback is momentum-driven. In all the simulations, the jet or wind creates a cavity mostly devoid of dense gas in the nuclear region where star formation is then quenched, but we find strong positive feedback in all the simulations at radii greater than 3 kpc. All four simulations have similar SFRs and stellar velocities with large radial and vertical components. However, the wind at an inclination of 90 degrees creates the highest density regions through ram pressure and generates the highest rates of star formation due to its ongoing strong interaction with the dense gas of the galactic plane. With increased wind inclination, we find greater asymmetry in gas distribution and resulting star formation. Our model generates an expanding ring of triggered star formation with typical velocity of order 1/3 of the circular velocity, superimposed on the older stellar population. This should result in a potentially detectable blue asymmetry in stellar absorption features at kpc scales.},
archivePrefix = {arXiv},
arxivId = {1608.01370},
author = {Dugan, Zachary and Gaibler, V. and Silk, J.},
doi = {10.3847/1538-4357/aa7566},
eprint = {1608.01370},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Dugan, Gaibler, Silk - 2017 - Feedback by AGN Jets and Wide-Angle Winds on a Galactic Scale.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
keywords = {Galaxy: formation,galaxies: active,galaxies: evolution,galaxies: jets,galaxies: star formation},
number = {1},
pages = {37},
publisher = {IOP Publishing},
title = {{Feedback by AGN Jets and Wide-Angle Winds on a Galactic Scale}},
url = {http://arxiv.org/abs/1608.01370{\%}0Ahttp://dx.doi.org/10.3847/1538-4357/aa7566},
volume = {844},
year = {2017}
}
@article{Melioli2004,
abstract = {The interstellar medium heated by supernova explosions (SN) may acquire$\backslash$nan expansion velocity larger than the escape velocity and leave the$\backslash$ngalaxy through a supersonic wind. Galactic winds are effectively$\backslash$nobserved in many local starburst galaxies (Lehnert {\&} Heckman 1996). The$\backslash$nSN ejecta are transported out of the galaxies by such winds which must$\backslash$naffect the chemical evolution of the galaxies. The effectiveness of the$\backslash$nprocesses mentioned above depends on the heating efficiency (HE) of the$\backslash$nSNs, i.e., the ratio between the kinetic plus internal energy density of$\backslash$nthe ambient gas and the SN energy density. In a starburst region,$\backslash$nseveral SN explosions occur at a large rate inside a relatively small$\backslash$nvolume. If the successive generations of SN remnants (SNRs) interact$\backslash$nwith each other very fast, then a superbubble of high temperature and$\backslash$nlow density will rapidly develop, before a significant increase of the$\backslash$nambient gas density that could lead to substantial losses of energy by$\backslash$nradiation. In this case, it is common to assume a value for HE of the$\backslash$norder of unity, since most of the available energy of the SNs will be$\backslash$ntransferred to the ambient gas in the form of kinetic and internal$\backslash$nenergy, instead of being radiated away. However this assumption fails to$\backslash$nreproduce both the chemical and dynamical characteristics of most$\backslash$nstarburst (SB) galaxies. In order to solve this paradigm, we have$\backslash$nconstructed a simple semi-analytical model, considering the essential$\backslash$ningredients of a SB environment, i.e., a three-phase medium composed by$\backslash$nhot diffuse gas, SNRs and clouds, which is able to qualitatively trace$\backslash$nthe thermalisation history of the ISM in a SB region and determine the$\backslash$nHE evolution (Melioli, de Gouveia Dal Pino, {\&} D'Ercole, A{\&}A, 2003,$\backslash$nsubmitted). Our study has also been accompanied by fully 3-D radiative$\backslash$ncooling, hydrodynamical simulations of SNR-SNR and SNR-clouds$\backslash$ninteractions (see Melioli, de Gouveia Dal Pino, {\&} Raga 2003, in$\backslash$npreparation).},
author = {Melioli, C and {E. M. de Gouveia Dal Pino}},
doi = {10.1051/0004-6361:20035750},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Melioli, E. M. de Gouveia Dal Pino - 2004 - Evolution of the ISM of starburst galaxies The SN heating efficiency.pdf:pdf},
isbn = {1-58381-166-4},
issn = {0004-6361},
journal = {Astron. Astrophys.},
keywords = {bubbles,galaxies,ism,starburst,supernova remnants},
number = {3},
pages = {817--831},
title = {{Evolution of the ISM of starburst galaxies: The SN heating efficiency}},
url = {http://www.aanda.org/10.1051/0004-6361:20035750},
volume = {424},
year = {2004}
}
@article{Riffel2011,
abstract = {We present stellar and gaseous kinematics of the inner ≈350-pc radius of the Seyfert galaxy Mrk1066 derived from J and Kl bands data obtained with the Gemini's Near-Infrared Integral Field Spectrograph (NIFS) at a spatial resolution of ≈35pc. The stellar velocity field is dominated by rotation in the galaxy plane but shows an S-shape distortion along the galaxy minor axis which seems to be due to an oval structure seen in an optical continuum image. Along this oval, between 170 and 280pc from the nucleus we find a partial ring of low $\sigma$* (≈50kms-1) attributed to an intermediate-age stellar population. The velocity dispersion of the stellar bulge ($\sigma$*≈ 90kms-1) implies a supermassive black hole mass of ≈5.4 × 106M⊙. From measurements of the emission-line fluxes and profiles ([Pii]$\lambda$ 1.1886$\mu$m, [Feii]$\lambda$ 1.2570$\mu$m, Pa$\beta$ and H2$\lambda$ 2.1218$\mu$m), we have constructed maps for the gas centroid velocity, velocity dispersion as well as channel maps. The velocity fields for all emission lines are dominated by a similar rotation pattern to that observed for the stars, but are distorted by the presence of two structures: (i) a compact rotating disc with radius r≈ 70pc; (ii) outflows along the radio jet which is oriented approximately along the galaxy major axis. The compact rotating disc is more conspicuous in the H2 emitting gas, which presents the smallest $\sigma$ values (≤70kms-1) and most clear rotation pattern, supporting a location in the galaxy plane. We estimate a gas mass for the disc of ∼107M⊙. The H2 kinematics further suggests that the nuclear disc is being fed by gas coming from the outer regions. The outflow is more conspicuous in the [Feii] emitting gas, which presents the highest $\sigma$ values (up to 150kms-1) and the highest blue and redshifts of up to 500kms-1, while the highest stellar rotation velocity is only ≈130kms-1. We estimate a mass-outflow rate in ionized gas of ≈6 × 10-2M⊙yr-1. The derived kinematics for the emitting gas is similar to that observed in previous studies supporting that the H2 is a tracer of the active galactic nucleus feeding and the [Feii] of its feedback. {\textcopyright} 2010 The Authors. Journal compilation {\textcopyright} 2010 RAS.},
author = {Riffel, Rogemar A. and Storchi-Bergmann, Thaisa},
doi = {10.1111/j.1365-2966.2010.17721.x},
file = {:home/william/Documents/Papers/mnras0411-0469.pdf:pdf},
issn = {00358711},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Galaxies: ISM,Galaxies: Seyfert,Galaxies: individual: Mrk1066,Galaxies: kinematics and dynamics,Infrared: galaxies},
number = {1},
pages = {469--486},
title = {{Compact molecular disc and ionized gas outflows within 350pc of the active nucleus of Mrk1066}},
volume = {411},
year = {2011}
}
@article{Crocker2015a,
abstract = {The Galactic Center's giant outflows are manifest in three different, non-thermal phenomena: i) the hard-spectrum, $\backslash$gamma-ray `Fermi Bubbles' emanating from the nucleus and extending to |b| {\~{}} 50 degrees; ii) the hard-spectrum, total-intensity microwave ({\~{}} 20-40 GHz) `Haze' extending to |b| {\~{}} 35 degrees in the lower reaches of the Fermi Bubbles; and iii) the steep spectrum, polarized, `S-PASS' radio ({\~{}} 2-20 GHz) Lobes that envelop the Bubbles and extend to |b| {\~{}} 60 degrees. We find that the nuclear outflows inflate a genuine bubble in each Galactic hemisphere that has the classical structure, working outwards, of reverse shock, contact discontinuity, and forward shock. Expanding into the finite pressure of the halo and given appreciable cooling and gravitational losses, the contact discontinuity of each bubble is now expanding only very slowly. We find observational signatures in both hemispheres of giant, reverse shocks at heights of {\~{}} 1 kpc above the nucleus; their presence ultimately explains all three of the non-thermal phenomena mentioned above. Synchrotron emission from shock-reaccelerated cosmic-ray electrons explains the spectrum, morphology, and vertical extent of the microwave Haze and the polarized radio Lobes. Collisions between shock-reaccelerated hadrons and denser gas in cooling condensations that form inside the contact discontinuity account for most of the Bubbles' $\backslash$gamma-ray emissivity.},
archivePrefix = {arXiv},
arxivId = {arXiv:1412.7510v2},
author = {Crocker, Roland M. and Bicknell, Geoffrey V. and Taylor, Andrew M. and Carretti, Ettore},
doi = {10.1088/0004-637X/808/2/107},
eprint = {arXiv:1412.7510v2},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Crocker et al. - 2015 - A UNIFIED MODEL of the FERMI BUBBLES, MICROWAVE HAZE, and POLARIZED RADIO LOBES REVERSE SHOCKS in the GALACTIC C.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {cosmic rays,gamma rays: diffuse background},
number = {2},
pages = {1--68},
title = {{A UNIFIED MODEL of the FERMI BUBBLES, MICROWAVE HAZE, and POLARIZED RADIO LOBES: REVERSE SHOCKS in the GALACTIC CENTER'S GIANT OUTFLOWS}},
volume = {808},
year = {2015}
}
@article{Feynman1982,
author = {Feynman, Richard P.},
doi = {10.1007/BF02650179},
file = {:home/william/Documents/Papers/Feynman1982{\_}Article{\_}SimulatingPhysicsWithComputers.pdf:pdf},
issn = {00207748},
journal = {Int. J. Theor. Phys.},
number = {6-7},
pages = {467--488},
title = {{Simulating physics with computers}},
volume = {21},
year = {1982}
}
@article{Garcia-Burillo2015,
abstract = {Context. Galaxy evolution scenarios predict that the feedback of star formation and nuclear activity (AGN) can drive the transformation of gas-rich spiral mergers into (ultra) luminous infrared galaxies and, eventually, lead to the build-up of QSO/elliptical hosts. Aims. We study the role that star formation and AGN feedback have in launching and maintaining the molecular outflows in two starburst-dominated advanced mergers, NGC 1614 (DL = 66 Mpc) and IRAS 17208-0014 (DL = 181 Mpc), by analyzing the distribution and kinematics of their molecular gas reservoirs. Both galaxies present evidence of outflows in other phases of their ISM. Methods. We used the Plateau de Bure interferometer (PdBI) to image the CO(10) and CO(21) line emissions in NGC 1614 and IRAS 17208-0014, respectively, with high spatial resolution (0: 0051: 002). The velocity fields of the gas were analyzed and modeled to find the evidence of molecular outflows in these sources and characterize the mass, momentum, and energy of these components. Results. While most (95{\%}) of the CO emission stems from spatially resolved (23 kpc-diameter) rotating disks, we also detect in both mergers the emission from high-velocity line wings that extend up to -500-700 km s1, well beyond the estimated virial range associated with rotation and turbulence. The kinematic major axis of the line-wing emission is tilted by 90 in NGC 1614 and by 180 in IRAS 17208-0014 relative to the major axes of their respective rotating disks. These results can be explained by the existence of non-coplanar molecular outflows in both systems: the outflow axis is nearly perpendicular to the rotating disk in NGC 1614, but it is tilted relative to the angular momentum axis of the rotating disk in IRAS 17208-0014. Conclusions. In stark contrast to NGC 1614, where star formation alone can drive its molecular outflow, the mass, energy, and momentum budget requirements of the molecular outflow in IRAS 17208-0014 can be best accounted for by the existence of a so far undetected (hidden) AGN of LAGN71011 L The geometry of the molecular outflow in IRAS 17208-0014 suggests that the outflow is launched by a non-coplanar disk that may be associated with a buried AGN in the western nucleus.},
archivePrefix = {arXiv},
arxivId = {1505.04705},
author = {Garc{\'{i}}a-Burillo, S. and Combes, F. and Usero, A. and Aalto, S. and Colina, L. and Alonso-Herrero, A. and Hunt, L. K. and Arribas, S. and Costagliola, F. and Labiano, A. and Neri, R. and Pereira-Santaella, M. and Tacconi, L. J. and {Van Der Werf}, P. P.},
doi = {10.1051/0004-6361/201526133},
eprint = {1505.04705},
file = {:home/william/Documents/Papers/aa26133-15.pdf:pdf},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Galaxies: ISM,Galaxies: individual: IRAS 17208-0014,Galaxies: individual: NGC1614,Galaxies: kinematics and dynamics,Galaxies: nuclei,Galaxies: starburst},
pages = {1--21},
title = {{High-resolution imaging of the molecular outflows in two mergers: IRAS 17208-0014 and NGC 1614}},
volume = {580},
year = {2015}
}
@article{Smith2019b,
abstract = {We present new XMM-Newton and NuSTAR observations of the galaxy merger IRAS F05189-2524 which is classified as an ultra-luminous infrared galaxy (ULIRG) and optical Seyfert 2 at z = 0.0426. We test a variety of spectral models which yields a best-fit consisting of an absorbed power law with emission and absorption features in the Fe K band. Remarkably, we find evidence for a blueshifted Fe K absorption feature at E = 7.8 keV (rest-frame) which implies an ultra-fast outflow (UFO) with vout = 0.11 ± 0.01c. We calculate that the UFO in IRAS F05189-2524 has a mass outflow rate of M out {\&} 1.0 M☉ yr−1, a kinetic power of E K {\&} 8{\%} LAGN, and a momentum rate (or force) of Pout {\&} 1.4 LAGN/c. Comparing the energetics of the UFO to the observed multi-phase outflows at kiloparsec scales yields an efficiency factor of f ∼ 0.05 for an energy-driven outflow. Given the uncertainties, however, we cannot exclude the possibility of a momentum-driven outflow. Comparing IRAS F05189-2524 with nine other objects with observed UFOs and large-scale galactic outflows suggests that there is a range of efficiency factors for the coupling of the energetics of the nuclear and galaxy-scale outflows that likely depend on specific physical conditions in each object.},
archivePrefix = {arXiv},
arxivId = {1910.14583},
author = {Smith, Robyn N. and Tombesi, Francesco and Veilleux, Sylvain and Lohfink, Anne M. and Luminari, Alfredo},
doi = {10.3847/1538-4357/ab4ef8},
eprint = {1910.14583},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Smith et al. - 2019 - Discovery of an X-ray quasar wind driving the cold gas outflow in the ultraluminous infrared galaxy IRAS F05189-25.pdf:pdf},
isbn = {0790580101},
issn = {23318422},
journal = {arXiv},
keywords = {Galaxies: active,Galaxies: individual (IRAS F05189-2524),Quasars: absorption lines,X-rays: galaxies},
title = {{Discovery of an X-ray quasar wind driving the cold gas outflow in the ultraluminous infrared galaxy IRAS F05189-2524}},
volume = {69},
year = {2019}
}
@article{Nokhrina2017,
abstract = {The effect of a mass-loading of the magnetohydrodynamic (MHD) flow in a relativistic jet from active galactic nuclei (AGN) due to {\$}\backslashgamma\backslashgamma\backslashrightarrow e{\^{}}+e{\^{}}-{\$} conversion is considered analytically. We argue that the effects of charge average separation due to specific initial pairs' motion lead to partial magnetic and electric fields screening or enhancement. The effect of the fields screening has not been considered earlier. The pairs with the center-of-mass moving faster or slower than the bulk plasma flow create a surface charge and a current which either screen or enhance both electric and magnetic fields in a pair creation domain. This impacts the bulk flow motion, which either accelerates or decelerates. The pairs with the center-of-mass moving with exactly the drift velocity does not induce the fields disturbance. In this case the flow decelerates due to pure mass-loading. For these different cases the Lorentz factor of the loaded outflow is calculated as a function of loading pairs number density. The effect may be important on sub-parsec to parsec scales due to conversion of TeV jet radiation on soft infra-red to ultra-violet external isotropic photon field. This leads to an outer shell acceleration. The conversion of MeV jet radiation on larger scales may account for the flow deceleration due to pure mass-loading. The proposed mechanism may be a source of internal shocks and instabilities in the pair creation region.},
archivePrefix = {arXiv},
arxivId = {1705.02581},
author = {Nokhrina, E. E. and Beskin, V. S.},
doi = {10.1093/mnras/stx1144},
eprint = {1705.02581},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Nokhrina, Beskin - 2017 - On the acceleration and deceleration of relativistic jets in active galactic nuclei - II. Mass-loading.pdf:pdf},
keywords = {active,galaxies,general,jets,non-thermal,quasars,radiation mechanisms,radio continuum},
number = {May},
title = {{On the acceleration and deceleration of relativistic jets in active galactic nuclei - II. Mass-loading}},
url = {http://arxiv.org/abs/1705.02581{\%}0Ahttp://dx.doi.org/10.1093/mnras/stx1144},
year = {2017}
}
@article{Fukumura2018,
author = {Fukumura, Keigo and Kazanas, Demosthenes and Shrader, Chris and Behar, Ehud and Tombesi, Francesco and Contopoulos, Ioannis},
doi = {10.3847/2041-8213/aadd10},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Fukumura et al. - 2018 - Variable Nature of Magnetically Driven Ultra-fast Out fl ows.pdf:pdf},
issn = {2041-8213},
journal = {Astrophys. J. Lett.},
keywords = {absorption lines,accretion,accretion disks,accretion,accretion disks,galaxies: individual (PD,galaxies,individual,magnetohydrodynamics,methods,mhd,numerical,pds 456,quasars},
number = {2},
pages = {L27},
publisher = {IOP Publishing},
title = {{Variable Nature of Magnetically Driven Ultra-fast Out fl ows}},
url = {http://dx.doi.org/10.3847/2041-8213/aadd10},
volume = {864},
year = {2018}
}
@article{Creasey2013,
abstract = {Feedback from supernovae is an essential aspect of galaxy formation. In order to improve subgrid models of feedback, we perform a series of numerical experiments to investigate how supernova explosions shape the interstellar medium (ISM) in a disc galaxy and power a galactic wind. We use the FLASH hydrodynamic code to model a simplified ISM, including gravity, hydrodynamics, radiative cooling above 104 K and star formation that reproduces the Kennicutt-Schmidt relation. By simulating a small patch of the ISM in a tall box perpendicular to the disc, we obtain subparsec resolution allowing us to resolve individual supernova events. The hot interiors of supernova explosions combine into larger bubbles that sweep-up the initially hydrostatic ISM into a dense, warm cloudy medium, enveloped by a much hotter and tenuous medium, all phases in near pressure equilibrium. The unbound hot phase develops into an outflow with wind speed increasing with distance as it accelerates from the disc. We follow the launch region of the galactic wind, where hot gas entrains and ablates warm ISM clouds leading to significantly increased mass loading of the flow, although we do not follow this material as it interacts with the galactic halo. We run a large grid of simulations in which we vary gas surface density, gas fraction and star formation rate in order to investigate the dependencies of the mass loading, $\beta$ = Mwind/ M. In the cases with the most effective outflows, we observe $\beta$ = 4; however, in other cases we find $\beta$ {\textgreater} 1. We find that outflows are more efficient in discs with lower surface densities or gas fractions. A simple model in which the warm cloudy medium is the barrier that limits the expansion of the blast wave reproduces the scaling of outflow properties with disc parameters at high star formation rates.We extend the scaling relations derived from an ISM patch to infer an effective mass loading for a galaxy with an exponential disc, finding that the mass loading depends on circular velocity as $\beta$ V -a d with a {\~{}} 2.5 for a model which fits the Tully- Fisher relation. Such a scaling is often assumed in phenomenological models of galactic winds in order to reproduce the flat faint end slope of the mass function. Our normalization is in approximate agreement with observed estimates of the mass loading for the Milky Way. The scaling we find sets the investigation of galaxy winds on a new footing, providing a physically motivated subgrid description of winds that can be implemented in cosmological hydrodynamic simulations and phenomenological models. {\textcopyright} 2013 The Authors Published by Oxford University Press on behalf of the Royal Astronomical Society.},
archivePrefix = {arXiv},
arxivId = {1211.1395},
author = {Creasey, Peter and Theuns, Tom and Bower, Richard G},
doi = {10.1093/mnras/sts439},
eprint = {1211.1395},
file = {:home/william/Documents/Papers/sts439.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Formation-galaxies,Galaxies,Hydrodynamics-methods,ISM,Numerical},
number = {3},
pages = {1922--1948},
title = {{How supernova explosions power galactic winds}},
volume = {429},
year = {2013}
}
@article{Lino2018,
abstract = {The Deep Convective Clouds and Chemistry (DC3) field campaign provided a unique set of observations to further investigate the role lightning and lightning-generated nitrogen oxides (LNOx) have on the composition of the upper troposphere. With the Weather Research and Forecasting model coupled with Chemistry (WRF-Chem), a cloud-resolved simulation of the 29-30 May 2012 severe supercell system investigated 18 flash rate parameterization schemes (FRPSs), the mean LNOx production per flash, and the transport and distribution of other trace gases. Most of the observed storm's meteorological and chemical conditions were well represented when the model included convective damping and lightning data assimilation techniques. Newly-developed FRPSs based on DC3 radar observations and Lightning Mapping Array (LMA) data are implemented in the model, along with previously developed schemes from the literature. The schemes are based on relationships between lightning and various kinematic, structural, and microphysical thunderstorm characteristics available in the model. The results suggest the simulated graupel and snow/ice hydrometeors require scaling factors to more closely represent proxy observations. The model flash rates generated over the simulation period are compared with LMA observations. Thirteen FRPSs overpredicted flashes by {\textgreater} 100{\%}. Generally, FRPSs based on storm kinematics and structure (particularly updraft volume) perform slightly better than schemes based on hydrometeors. However, the upward cloud ice flux FRPS best represents the observed lightning. The 10 WRF-Chem simulations included one run with no LNOx and nine runs with different LNOx production scenarios. The simulated CO and O3 are within 1{\%} and 3{\%} of aircraft observations, respectively, when compared with one model layer lower, which suggests the model slightly underestimates the convective transport. A LNOx production scenario of 82 moles per flash best represents the observed NOx mixing ratios in anvil outflow when combined with the observed flash channel vertical profiles and intracloud to cloud-to-ground ratios. This estimate is smaller than the mean 250 moles NO per flash suggested for a typical thunderstorm, but within the lower end of the estimated range (33-660 moles per flash). Analysis of the convective outflow using observations made 12-24 hours downwind indicates the mean daytime photochemical O3 production rate is about 1.6 ppbv per hour.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Korde-Nayak, Vaishali},
doi = {10.15713/ins.mmj.3},
eprint = {arXiv:1011.1669v3},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Lino et al. - 2018 - Development of high-strength microalloyed coiled rebar.pdf:pdf},
isbn = {9781935117643},
issn = {15470423},
journal = {MMJ - A J. by MIMER Med. Coll. Pune, India},
number = {1},
pages = {1--14},
pmid = {29982528},
title = {{Why is India the world's stillbirth capital: causes and solutions?}},
volume = {1},
year = {2017}
}
@article{Tanner2022,
abstract = {Using a series of 3D relativistic hydrodynamical simulations of active galactic nuclei (AGN) we investigate how AGN power, a clumpy ISM structure, and AGN jet angle with respect to the galactic disk affect the morphology and content of the resulting galactic outflow. For low power AGN across three orders of magnitude of AGN luminosities ({\$}10{\^{}}{\{}41{\}}-10{\^{}}{\{}43{\}}{\$} erg s{\$}{\^{}}{\{}-1{\}}{\$}) our simulations did not show significant changes to either the morphology or total mass of the outflow. Changing the angle of the AGN jet with respect to the galaxy did show small changes in the total outflow mass of a factor of 2-3. Jets perpendicular to the galactic disk were created hot single phase outflows, while jets close to parallel with the disk created the outflows were multi-phase with equal parts warm and hot, and significant cold gas. Overall The final morphology of low power AGN outflows depends primarily on how the jet impacts and interacts with large, dense clouds in the clumpy ISM. These clouds can disrupt, deflect, split, or suppress the jet preventing it from leaving the galactic disk as a coherent structure. But for simulations with AGN luminosities {\$}{\textgreater} 10{\^{}}{\{}44{\}}{\$} erg s{\$}{\^{}}{\{}-1{\}}{\$} the ISM played a minor role in determining the morphology of the outflow with an undisrupted jet leaving the disk. The final morphology of AGN outflows is different for low power AGNs vs. high power AGNs with the final morphology of low power AGN outflows dependent on the ISM structure within the first kpc surrounding the AGN.},
archivePrefix = {arXiv},
arxivId = {2201.08360},
author = {Tanner, Ryan and Weaver, Kimberly},
eprint = {2201.08360},
file = {:home/william/Documents/Papers/2201.08360.pdf:pdf},
keywords = {agn,galaxies,kinematics and dynamics,outflows},
title = {{Simulations of AGN Driven Galactic Outflow Morphology and Content}},
url = {http://arxiv.org/abs/2201.08360},
year = {2022}
}
@article{Muller-Sanchez2011,
abstract = {As part of an extensive study of the physical properties of active galactic nuclei (AGNs) we report high spatial resolution near-IR integral-field spectroscopy of the narrow-line region (NLR) and coronal-line region (CLR) of seven Seyfert galaxies. These measurements elucidate for the first time the two-dimensional spatial distribution and kinematics of the recombination line Br$\gamma$ and high-ionization lines [Si VI], [Al IX], and [Ca VIII] on scales {\textless}300pc from the AGN. The observations reveal kinematic signatures of rotation and outflow in the NLR and CLR. The spatially resolved kinematics can be modeled as a combination of an outflow bicone and a rotating disk coincident with the molecular gas. High-excitation emission is seen in both components, suggesting it is leaking out of a clumpy torus. While NGC1068 (Seyfert2) is viewed nearly edge-on, intermediate-type Seyferts are viewed at intermediate angles, consistent with unified schemes. A correlation between the outflow velocity and the molecular gas mass in r {\textless} 30pc indicates that the accumulation of gas around the AGN increases the collimation and velocity of the outflow. The outflow rate is 2-3 orders of magnitude greater than the accretion rate, implying that the outflow is mass loaded by the surrounding interstellar medium (ISM). In half of the observed AGNs, the kinetic power of the outflow is of the order of the power required by two-stage feedback models to be thermally coupled to the ISM and to match the MBH-$\sigma$* relation. In these objects, the radio jet is clearly interacting with the ISM, indicative of a link between jet power and outflow power. {\textcopyright} 2011 The American Astronomical Society. All rights reserved.},
archivePrefix = {arXiv},
arxivId = {arXiv:1107.3140v1},
author = {M{\"{u}}ller-S{\'{a}}nchez, F. and Prieto, M. A. and Hicks, E. K.S. and Vives-Arias, H. and Davies, R. I. and Malkan, M. and Tacconi, L. J. and Genzel, R.},
doi = {10.1088/0004-637X/739/2/69},
eprint = {arXiv:1107.3140v1},
file = {:home/william/Documents/Papers/1107.3140.pdf:pdf},
issn = {15384357},
journal = {Astrophys. J.},
keywords = {galaxies: Seyfert,galaxies: active,galaxies: kinematics and dynamics,galaxies: nuclei,infrared: galaxies,line: profiles},
number = {2},
title = {{Outflows from active galactic nuclei: Kinematics of the narrow-line and coronal-line regions in Seyfert galaxies}},
volume = {739},
year = {2011}
}
@article{Pina2021,
abstract = {We present new HI interferometric observations of the gas-rich ultra-diffuse galaxy AGC 114905, which previous work, based on low-resolution data, identified as an outlier of the baryonic Tully-Fisher relation. The new observations, at a spatial resolution {\$}\backslashsim 2.5{\$} times higher than before, reveal a regular HI disc rotating at about 23 km/s. Our kinematic parameters, recovered with a robust 3D kinematic modelling fitting technique, show that the flat part of the rotation curve is reached. Intriguingly, the rotation curve can be explained almost entirely by the baryonic mass distribution alone. We show that a standard cold dark matter halo that follows the concentration-halo mass relation fails to reproduce the amplitude of the rotation curve by a large margin. Only a halo with an extremely (and arguably unfeasible) low concentration reaches agreement with the data. We also find that the rotation curve of AGC 114905 deviates strongly from the predictions of Modified Newtonian dynamics. The inclination of the galaxy, which is measured independently from our modelling, remains the largest uncertainty in our analysis, but the associated errors are not large enough to reconcile the galaxy with the expectations of cold dark matter or Modified Newtonian dynamics.},
archivePrefix = {arXiv},
arxivId = {2112.00017},
author = {Pi{\~{n}}a, Pavel E. Mancera and Fraternali, Filippo and Oosterloo, Tom and Adams, Elizabeth A. K. and Oman, Kyle A. and Leisman, Lukas},
eprint = {2112.00017},
file = {:home/william/Documents/Papers/2112.00017.pdf:pdf},
keywords = {cosmology,dark matter,dwarfs,galaxies,irregular,kinematics and dynamics},
number = {December},
pages = {1--12},
title = {{No need for dark matter: resolved kinematics of the ultra-diffuse galaxy AGC 114905}},
url = {http://arxiv.org/abs/2112.00017},
volume = {12},
year = {2021}
}
@article{Li2020,
abstract = {We explore the survival of cool clouds in multiphase circumgalactic media. We revisit the 'cloud-crushing problem' in a large survey of simulations including radiative cooling, self-shielding, self-gravity, magnetic fields, and anisotropic Braginskii conduction and viscosity (with saturation). We explore a wide range of parameters including cloud size, velocity, ambient temperature and density, and a variety of magnetic field configurations and cloud turbulence. We find that realistic magnetic fields and turbulence have weaker effects on cloud survival; the most important physics is radiative cooling and conduction. Self-gravity and self-shielding are important for clouds that are initially Jeans-unstable, but largely irrelevant otherwise. Non-self-gravitating, realistically magnetized clouds separate into four regimes: (1) at low column densities, clouds evaporate rapidly via conduction; (2) a 'failed pressure confinement' regime, where the ambient hot gas cools too rapidly to provide pressure confinement for the cloud; (3) an 'infinitely long-lived' regime, in which the cloud lifetime becomes longer than the cooling time of gas swept up in the leading bow shock, so the cloud begins to accrete and grow; and (4) a 'classical cloud destruction' regime, where clouds are eventually destroyed by instabilities. In the final regime, the cloud lifetime can exceed the naive cloud-crushing time owing to conduction-induced compression. However, small and/or slow-moving clouds can also evaporate more rapidly than the cloud-crushing time. We develop simple analytic models that explain the simulated cloud destruction times in this regime.},
archivePrefix = {arXiv},
arxivId = {1909.02632},
author = {Li, Zhihui and Hopkins, Philip F. and Squire, Jonathan and Hummels, Cameron},
doi = {10.1093/mnras/stz3567},
eprint = {1909.02632},
file = {:home/william/Documents/Papers/stz3567.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {Dynamics,Galaxies: evolution,Galaxies: haloes,Galaxies: kinematics,ISM: clouds,ISM: structure},
number = {2},
pages = {1841--1854},
publisher = {Oxford University Press},
title = {{On the survival of cool clouds in the circumgalactic medium}},
volume = {492},
year = {2020}
}
@article{DeGouveiadalPino1993,
abstract = {We present the first results of fully 3D simulations of supersonic, radiatively cooling jets using the smoothed particle hydrodynamics technique (SPH). Our results qualitatively agree with the 2D simulations of Blondin et al. (1990), although the removal of the axisymmetry has resulted in relevant structural differences, especially at the jet head where a cold shell is formed from the condensation of shock-heated material. In particular, we found that the shell is not only dynamically unstable but also may undergo oscillations in density, which are attributed to global thermal instabilities. These effects may have important consequences on the dynamics and emission pattern of the observed HH objects associated to young stellar jets. We discuss the implications of our results in the interpretation of the observed properties of the stellar jets and HH objects. We also compare the structure of radiative cooling and adiabatic 3D jets.},
author = {{de Gouveia dal Pino}, Elisabete M and Benz, Willy},
doi = {10.1086/172785},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/de Gouveia dal Pino, Benz - 1993 - Three-dimensional simulations of protostellar jets.pdf:pdf},
issn = {15384357 0004637X},
journal = {Astrophys. J.},
pages = {686},
title = {{Three-dimensional simulations of protostellar jets}},
url = {http://adsabs.harvard.edu/cgi-bin/nph-data{\_}query?bibcode=1993ApJ...410..686D{\&}link{\_}type=ABSTRACT{\%}5Cnpapers2://publication/doi/10.1086/172785},
volume = {410},
year = {1993}
}
@article{Fabian2012,
abstract = {Radiation, winds and jets from the active nucleus of a massive galaxy can interact with its interstellar medium leading to ejection or heating of the gas. This can terminate star formation in the galaxy and stifle accretion onto the black hole. Such Active Galactic Nucleus (AGN) feedback can account for the observed proportionality between central black hole and host galaxy mass. Direct observational evidence for the radiative or quasar mode of feedback, which occurs when the AGN is very luminous, has been difficult to obtain but is accumulating from a few exceptional objects. Feedback from the kinetic or radio mode, which uses the mechanical energy of radio-emitting jets often seen when the AGN is operating at a lower level, is common in massive elliptical galaxies. This mode is well observed directly through X-ray observations of the central galaxies of cool core clusters in the form of bubbles in the hot surrounding medium. The energy flow, which is roughly continuous, heats the hot intracluster gas and reduces radiative cooling and subsequent star formation by an order of magnitude. Feedback appears to maintain a long-lived heating/cooling balance. Powerful, jetted radio outbursts may represent a further mode of energy feedback which affect the cores of groups and subclusters. New telescopes and instruments from the radio to X-ray bands will come into operation over the next few years and lead to a rapid expansion in observational data on all modes of AGN feedback.},
archivePrefix = {arXiv},
arxivId = {1204.4114},
author = {Fabian, A. C.},
doi = {10.1146/annurev-astro-081811-125521},
eprint = {1204.4114},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Fabian - 2012 - Observational Evidence of AGN Feedback.pdf:pdf},
issn = {0066-4146},
keywords = {'1111,black holes,galaxies,galaxy clusters,galaxy evolution,jets,outflows,radio},
mendeley-tags = {'1111},
title = {{Observational Evidence of AGN Feedback}},
url = {http://arxiv.org/abs/1204.4114{\%}0Ahttp://dx.doi.org/10.1146/annurev-astro-081811-125521},
year = {2012}
}
@article{Tomisaka1986,
abstract = {The evolution of a superbubble driven by sequential explosions of supernovae in an OB association is studied. The authors especially focus on the effect of the plane-stratified gas distribution in the direction perpendicular to the galactic disk. It is shown that the superbubble asymmetrically expands with respect to the parallel and perpendicular directions to the disk. In the case that the density on the disk plane, n0, is ≡1 cm-3, it is found that the cooled shell surrounds the hot cavity like an egg shape. On the other hand, in a low-density disk with n0 ≡ 0.1 cm-3, a cooled wall is formed only on the disk plane side of the bubble and the hot gas flows up to the halo region. This corresponds to the H I worms pointed out by Heiles (1984). The authors can show that the hot gas which is pushed up maintains the galactic hot gaseous halo.},
author = {Tomisaka, Kohji and Ikeuchi, Satoru},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Tomisaka, Ikeuchi - 1986 - Evolution of superbubble driven by sequential supernova explosions in a plane-stratified gas distribution.pdf:pdf},
journal = {Astron. Soc. Japan},
keywords = {B STARS,DENSITY DISTRIBUTION,GALACTIC EVOLUTION,GALACTIC STRUCTURE,GAS DENSITY,GRAVITATIONAL COLLAPSE,O STARS,STELLAR MASS EJECTION,STRATA,supernova remnants},
pages = {697},
title = {{Evolution of superbubble driven by sequential supernova explosions in a plane-stratified gas distribution}},
url = {http://adsabs.harvard.edu/cgi-bin/nph-data{\_}query?bibcode=1986PASJ...38..697T{\&}link{\_}type=ABSTRACT},
volume = {38},
year = {1986}
}
@article{Boltzmann,
author = {Boltzmann, Maxwell and Taylor, The},
file = {:home/william/Documents/Papers/MCon3.pdf:pdf},
number = {10},
pages = {3--4},
title = {{1 Conductivity{\_}Al.pdf}}
}
@article{Jaffe1983,
abstract = {The present analytic formula for spherical galaxy three-dimensional light distribution yields a fit with measured brightnesses which compares favorably with existing models, despite its simplicity. Surface brightness, gravitational potential and projected velocity dispersion can be straightforwardly computed by means of the formula, whose asymptotic behavior for large and small radii is sufficiently simple to invite speculative physical interpretations.},
author = {Jaffe, W},
doi = {10.1093/mnras/202.4.995},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Jaffe - 1983 - A simple model for the distribution of light in spherical galaxies.pdf:pdf},
issn = {0035-8711},
journal = {R. Astron. Soc.},
keywords = {ASTRONOMICAL MODELS,BRIGHTNESS DISTRIBUTION,GALACTIC RADIATION,GRAVITATIONAL FIELDS,LIGHT EMISSION,SURFACE PROPERTIES},
pages = {995},
title = {{A simple model for the distribution of light in spherical galaxies}},
url = {http://adsabs.harvard.edu/cgi-bin/nph-data{\_}query?bibcode=1983MNRAS.202..995J{\&}link{\_}type=ABSTRACT},
volume = {202},
year = {1983}
}
@article{Yang2018c,
abstract = {The origin of sub-TeV gamma rays detected by the Fermi-Large Area Telescope (LAT) from the Fermi Bubbles (FBs) at the Galactic center is still uncertain. In a hadronic model, acceleration of protons and/or nuclei and their subsequent interactions with gas in the bubble volume can produce the observed gamma rays. Recently the High Altitude Water Cherenkov (HAWC) observatory reported an absence of gamma-ray excess from the Northern FB at {\$}b\backslashgtrsim 6{\^{}}\backslashcirc{\$} Galactic latitude, which resulted in flux upper limits in the energy range of {\$}1.2-126{\$} TeV. These upper limits are consistent with the gamma-ray spectrum measured by Fermi-LAT at {\$}|b|\backslashge 10{\^{}}\backslashcirc{\$}, where an exponential cutoff at energies {\$}\backslashgtrsim 100{\$} GeV is evident. However, the FB gamma-ray spectrum at {\$}|b|\backslashle 10{\^{}}\backslashcirc{\$}, without showing any sign of cutoff up to around 1 TeV in the latest tentative results, remains unconstrained. The upcoming Cherenkov Telescope Array (CTA) will perform a Galactic center survey with unprecedented sensitivity in the energy between 20 GeV and 300 TeV. In this work, we perform both morphological and classic on/off analyses with planned CTA deep central and extended survey and estimate the sensitivity of CTA to the FB hadronic gamma-ray flux models that best fit the spectrum at {\$}|b|\backslashle 10{\^{}}\backslashcirc{\$} and whose counterpart neutrino flux model best fits the optimistic neutrino spectrum from IceCube Neutrino Observatory. We also perform sensitivity analysis with a future ground-based Cherenkov detector the Large High Altitude Air Shower Observatory (LHAASO). We find that CTA will be able to discover or constrain the FB gamma-ray flux at {\$}|b|\backslashle 10{\^{}}\backslashcirc{\$} in the {\$}\backslashapprox{\$} 200 GeV - 100 TeV range with planned observation strategy, while LHAASO may constrain emission in the {\$}\backslashapprox 100{\$} GeV - 100 TeV range if {\$}\backslashlesssim 10\backslash{\%}{\$} systematic uncertainties can be achieved.},
archivePrefix = {arXiv},
arxivId = {1811.10970},
author = {Yang, Lili and Razzaque, Soebur},
eprint = {1811.10970},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Yang, Razzaque - 2018 - Constraints on very high energy gamma-ray emission from the Fermi Bubbles with future ground-based experi.{\_}soebur-co:{\_}soebur-co},
number = {2},
pages = {1--9},
title = {{Constraints on very high energy gamma-ray emission from the Fermi Bubbles with future ground-based experiments}},
url = {http://arxiv.org/abs/1811.10970},
year = {2018}
}
@article{Bu2019,
archivePrefix = {arXiv},
arxivId = {1901.00972},
author = {Bu, De-Fu and Yang, Xiao-Hong},
eprint = {1901.00972},
file = {:home/william/.local/share/data/Mendeley Ltd./Mendeley Desktop/Downloaded/Bu, Yang - 2019 - Quenching black hole accretion by active galactic nuclei feedback.pdf:pdf},
title = {{Quenching black hole accretion by active galactic nuclei feedback}},
url = {https://arxiv.org/abs/1901.00972},
year = {2019}
}
@article{Schnorr-Muller2021,
abstract = {We characterized the kinematics, morphology, and stellar population (SP) properties of a sample of massive compact quiescent galaxies (MCGs, 10 ≲, log M∗/Modot, ≲, 11 and re ∼ 1-3 kpc) in the MaNGA Survey, with the goal of constraining their formation, assembly history, and assessing their relation with non-compact quiescent galaxies. We compared their properties with those of a control sample of median-sized quiescent galaxies (re ∼ 4-8 kpc) with similar effective velocity dispersions. MCGs have elevated rotational support, as evidenced by a strong anticorrelation between the Gauss-Hermite moment h3 and V/$\sigma$. In contrast, 30 per cent of control sample galaxies (CSGs) are slow rotators, and fast-rotating CSGs generally show a weak h3-V/$\sigma$ anticorrelation. MCGs and CSGs have similar ages, but MCGs are more metal-rich and $\alpha$-enhanced. Both MCGs and CSGs have shallow negative metallicity gradients and flat [$\alpha$/Fe] gradients. On average, MCGs and CSGs have flat age gradients, but CSGs have a significantly larger dispersion of gradient values. The kinematics and SP properties of MCGs suggest that they experienced highly dissipative gas-rich events, such as mergers, followed by an intense, short, and centrally concentrated burst of star formation, between 4 and 10 Gyr ago (z ∼0.4-2), and had a quiet accretion history since then. This sequence of events might be analogous to, although less extreme than, the compaction events that formed compact quiescent galaxies at z ∼ 2. The small sizes of MCGs, and the high efficiency and short duration of their last star formation episode suggest that they are descendants of compact post-starburst galaxies.},
archivePrefix = {arXiv},
arxivId = {2104.12737},
author = {Schnorr-M{\"{u}}ller, A. and Trevisan, M and Riffel, R and Chies-Santos, A. L. and Furlanetto, C and Ricci, T V and Lohmann, F S and Flores-Freitas, R. and Mallmann, N D and Alamo-Mart{\'{i}}nez, K. A.},
doi = {10.1093/mnras/stab2116},
eprint = {2104.12737},
file = {:home/william/Documents/Papers/stab2116.pdf:pdf},
issn = {13652966},
journal = {Mon. Not. R. Astron. Soc.},
keywords = {cD,galaxies: elliptical and lenticular,galaxies: evolution,galaxies: kinematics and dynamics,galaxies: statistics,galaxies: stellar content},
number = {1},
pages = {300--317},
title = {{The puzzling origin of massive compact galaxies in MaNGA}},
volume = {507},
year = {2021}
}


@book{ToroEleuterio1999,
  title     = "Riemann Solvers and Numerical Methods for Fluid Dynamics",
  author    = "Toro, Eleuterio",
  year      = "2009",
  publisher = "Springer-Verlag Berlin Heidelberg",
  doi      = {10.1007/b79761}
}


@article{Liu1998,
abstract = {Second order accurate (first order at extrema) cell averaged based approximations extending the Lax-Friedrichs central scheme, using component-wise rather than field-by-field limiting, have been found to give surprisingly good results for a wide class of problems involving shocks (see H. Nessyahu and E. Tadmor,J. Comput. Phys.87, 408, 1990). The advantages of component-wise limiting compared to its counterpart, field-by-field limiting, are apparent: (1) No complete set of eigenvectors is needed and hence weakly hyperbolic systems can be solved. (2) Component-wise limiting is faster than field-by-field limiting. (3) The programming is much simpler, especially for complicated coupled systems of many equations. However, these methods are based on cell-averages in a staggered grid and are thus a bit complicated to extend to multiple dimensions. Moreover the staggering causes slight difficulties at the boundaries. In this work we modify and extend this component-wise central differencing based procedure in two directions: (1) Point values, rather than cell averages are used, thus removing the need for staggered grids, and also making the extension to multi-dimensions quite simple. We use TVD Runge-Kutta time discretizations to update the solution. (2) A new type of decision process, which follows the general ENO philosophy is introduced and used. This procedure enables us to extend our method to a third order component-wise central ENO scheme, which apparently works well and is quite simple to implement in multi-dimensions. Additionally, our numerical viscosity is governed by the local magnitude of the maximum eigenvalue of the Jacobian, thus reducing the smearing in the numerical results. We found a speed up of a factor of 2 in each space dimension, on a SGIO2workstation, over methods based on field-by-field decomposition limiting. The new decision process leads to new, "convex" ENO schemes which, we believe, are of interest in a more general setting. Our numerical results show the value of these new methods. {\textcopyright} 1998 Academic Press.},
author = {Liu, Xu Dong and Osher, Stanley},
doi = {10.1006/jcph.1998.5937},
file = {:home/william/Documents/Papers/1-s2.0-S002199919895937X-main.pdf:pdf},
issn = {00219991},
journal = {J. Comput. Phys.},
number = {2},
pages = {304--330},
title = {{Convex ENO High Order Multi-dimensional Schemes without Field by Field Decomposition or Staggered Grids}},
volume = {142},
year = {1998}
}


@ARTICLE{1998A&A...331L...1S,
       author = {{Silk}, Joseph and {Rees}, Martin J.},
        title = "{Quasars and galaxy formation}",
      journal = {\aap},
     keywords = {GALAXY FORMATION: SUPERMASSIVE BLACK HOLES, QUASARS: OUTFLOWS, Astrophysics},
         year = 1998,
        month = mar,
       volume = {331},
        pages = {L1-L4},
archivePrefix = {arXiv},
       eprint = {astro-ph/9801013},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998A&A...331L...1S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{SilkRees1998,
       author = {{Silk}, Joseph and {Rees}, Martin J.},
        title = "{Quasars and galaxy formation}",
      journal = {\aap},
     keywords = {GALAXY FORMATION: SUPERMASSIVE BLACK HOLES, QUASARS: OUTFLOWS, Astrophysics},
         year = 1998,
        month = mar,
       volume = {331},
        pages = {L1-L4},
archivePrefix = {arXiv},
       eprint = {astro-ph/9801013},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998A&A...331L...1S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Falceta-Goncalves2010,
       author = {{Falceta-Gon{\c{c}}alves}, D. and {Caproni}, A. and {Abraham}, Z. and {Teixeira}, D.~M. and {de Gouveia Dal Pino}, E.~M.},
        title = "{Precessing Jets and X-ray Bubbles from NGC 1275 (3C 84) in the Perseus Galaxy Cluster: A View from Three-dimensional Numerical Simulations}",
      journal = {\apjl},
     keywords = {galaxies: clusters: individual: Perseus, galaxies: jets, methods: numerical, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2010,
        month = apr,
       volume = {713},
       number = {1},
        pages = {L74-L78},
          doi = {10.1088/2041-8205/713/1/L74},
archivePrefix = {arXiv},
       eprint = {1003.2406},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...713L..74F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{McNamara_2012,
	doi = {10.1088/1367-2630/14/5/055023},
	url = {https://doi.org/10.1088/1367-2630/14/5/055023},
	year = 2012,
	month = {may},
	publisher = {{IOP} Publishing},
	volume = {14},
	number = {5},
	pages = {055023},
	author = {B R McNamara and P E J Nulsen},
	title = {Mechanical feedback from active galactic nuclei in galaxies, groups and clusters},
	journal = {New Journal of Physics},
	abstract = {The radiative cooling timescales at the centers of hot atmospheres surrounding elliptical galaxies, groups and clusters are much shorter than their ages. Therefore, hot atmospheres are expected to cool and to form stars. Cold gas and star formation are observed in central cluster galaxies but at levels below those expected from an unimpeded cooling flow. X-ray observations have shown that wholesale cooling is being offset by mechanical heating from radio active galactic nuclei. Feedback is widely considered to be an important and perhaps unavoidable consequence of the evolution of galaxies and supermassive black holes. We show that cooling x-ray atmospheres and the ensuing star formation and nuclear activity are probably coupled to a self-regulated feedback loop. While the energetics are now reasonably well understood, other aspects of feedback are not. We highlight the problems of atmospheric heating and transport processes, accretion, and nuclear activity, and we discuss the potential role of black hole spin. We discuss x-ray imagery showing that the chemical elements produced by central galaxies are being dispersed on large scales by outflows launched from the vicinity of supermassive black holes. Finally, we comment on the growing evidence for mechanical heating of distant cluster atmospheres by radio jets and its potential consequences for the excess entropy in hot halos and a possible decline in the number of distant cooling flows.}
	}
	
@article{Nesvadbaetal2011,
    author = {{Nesvadba, N. P. H.} and {Boulanger, F.} and {Lehnert, M. D.} and {Guillard, P.}	and {Salome, P.}},
    title = {Dense gas without star formation: the kpc-sized turbulent molecular disk in 3C~N},
    DOI= "10.1051/0004-6361/201118018",
    url= "https://doi.org/10.1051/0004-6361/201118018",
    journal = {A\&A},
    year = 2011,
    volume = 536,
    pages = "L5",
    month = "",
}


@article{Nesvadba2010.521,
	author = {{Nesvadba, N. P. H.} and {Boulanger, F.} and {Salom\'e, P.} and {Guillard, P.} and {Lehnert, M. D.} and {Ogle, P.} and {Appleton, P.} and {Falgarone, E.} and {Pineau des Forets, G.}},
	title = {Energetics of the molecular gas in the H2 luminous radio galaxy 3C~326: Evidence for negative AGN feedback*},
	DOI= "10.1051/0004-6361/200913333",
	url= "https://doi.org/10.1051/0004-6361/200913333",
	journal = {A\&A},
	year = 2010,
	volume = 521,
	pages = "A65",
	month = "",
}



@article{Wylezalek2016.461,
    author = {Wylezalek, Dominika and Zakamska, Nadia L.},
    title = "{Evidence of suppression of star formation by quasar-driven winds in gas-rich host galaxies at z<1?}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {461},
    number = {4},
    pages = {3724-3739},
    year = {2016},
    month = {06},
    abstract = "{Feedback from active galactic nuclei (AGN) is widely considered to be the main driver in regulating the growth of massive galaxies through heating or driving gas out of the galaxy, preventing further increase in stellar mass. Observational proof for this scenario has, however, been scarce. We have assembled a sample of 132 radio-quiet type-2 and red AGN at 0.1 \\&lt; z \\&lt; 1. We measure the kinematics of the AGN-ionized gas, the host galaxies’ stellar masses and star formation rates (SFRs) and investigate the relationships between AGN luminosities, specific star formation rates (sSFRs) and outflow strengths W90 – the 90 per cent velocity width of the [O iii]λ5007Å line power and a proxy for the AGN-driven outflow speed. Outflow strength is independent of sSFR for AGN selected on their mid-IR luminosity, in agreement with previous work demonstrating that star formation is not sufficient to produce the observed ionized gas outflows which have to be powered by AGN activity. More importantly, we find a negative correlation between W90 and sSFR in the AGN hosts with the highest SFRs, i.e. with the highest gas content, where presumably the coupling of the AGN-driven wind to the gas is strongest. This implies that AGN with strong outflow signatures are hosted in galaxies that are more ‘quenched’ than galaxies with weaker outflow signatures. Despite the galaxies’ high SFRs, we demonstrate that the outflows are not star formation driven but indeed due to AGN powering. This observation is consistent with the AGN having a net suppression, ‘negative’ impact, through feedback on the galaxies’ star formation history.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/stw1557},
    url = {https://doi.org/10.1093/mnras/stw1557},
    eprint = {https://academic.oup.com/mnras/article-pdf/461/4/3724/8110626/stw1557.pdf},
}



@article{harrison2020proc, 
         title={Establishing the impact of powerful AGN on their host galaxies}, 
         volume={15}, 
         DOI={10.1017/S1743921320001696}, 
         number={S359}, 
         journal={Proceedings of the International Astronomical Union}, publisher={Cambridge University Press}, 
         author={Harrison, C. M. and Molyneux, S. J. and Scholtz, J. and Jarvis, M. E.}, 
         year={2020}, 
         pages={203–211}
}


@article{Scholtz2020.492MNRAS,
    author = {Scholtz, J and Harrison, C M and Rosario, D J and Alexander, D M and Chen, C-C and Kakkad, D and Mainieri, V and Tiley, A L and Turner, O and Cirasuolo, M and Sharples, R M and Stach, S},
    title = "{KASHz: No evidence for ionised outflows instantaneously suppressing star formation in moderate luminosity AGN at z ∼ 1.4–2.6}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {492},
    number = {3},
    pages = {3194-3216},
    year = {2020},
    month = {01},
    abstract = "{As part of our KMOS AGN Survey at High-redshift (KASHz), we present spatially resolved VLT/KMOS and VLT/SINFONI spectroscopic data and ALMA 870 μm continuum imaging of eight z = 1.4–2.6 moderate AGN (\\$L\_\\{\\rm 2-10 \\, \\rm kev\\}\\$ = 1042–1045 ergs s−1). We map [O iii], H α and rest-frame FIR emission to search for any spatial anticorrelation between ionised outflows (traced by the [O  iii] line) and star formation (SF; traced by H α and FIR), that has previously been claimed for some high-z AGN and used as evidence for negative and/or positive AGN feedback. First, we conclude that H α is unreliable to map SF inside our AGN host galaxies based on: (i) SF rates inferred from attenuation-corrected H α can lie below those inferred from FIR; (ii) the FIR continuum is more compact than the H α emission by a factor of ∼2 on average; (iii) in half of our sample, we observe significant spatial offsets between the FIR and H α emission, with an average offset of 1.4 ± 0.6 kpc. Secondly, for the five targets with outflows we find no evidence for a spatial anticorrelation between outflows and SF using either H α or FIR as a tracer. This holds for our re-analysis of a famous z = 1.6 X-ray AGN (‘XID 2028’) where positive and negative feedback has been previously claimed. Based on our results, any impact on SF by ionised outflows must be subtle, either occurring on scales below our resolution, or on long time-scales.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/staa030},
    url = {https://doi.org/10.1093/mnras/staa030},
    eprint = {https://academic.oup.com/mnras/article-pdf/492/3/3194/31922519/staa030.pdf},
}


@article{Wagner_2012,
	doi = {10.1088/0004-637x/757/2/136},
	url = {https://doi.org/10.1088/0004-637x/757/2/136},
	year = 2012,
	month = {sep},
	publisher = {American Astronomical Society},
	volume = {757},
	number = {2},
	pages = {136},
	author = {A. Y. Wagner and G. V. Bicknell and M. Umemura},
	title = {{DRIVING} {OUTFLOWS} {WITH} {RELATIVISTIC} {JETS} {AND} {THE} {DEPENDENCE} {OF} {ACTIVE} {GALACTIC} {NUCLEUS} {FEEDBACK} {EFFICIENCY} {ON} {INTERSTELLAR} {MEDIUM} {INHOMOGENEITY}},
	journal = {The Astrophysical Journal},
	abstract = {We examine the detailed physics of the feedback mechanism by relativistic active galactic nucleus (AGN) jets interacting with a two-phase fractal interstellar medium (ISM) in the kpc-scale core of galaxies using 29 three-dimensional grid-based hydrodynamical simulations. The feedback efficiency, as measured by the amount of cloud dispersal generated by the jet–ISM interactions, is sensitive to the maximum size of clouds in the fractal cloud distribution but not to their volume filling factor. Feedback ceases to be efficient for Eddington ratios Pjet/Ledd ≲ 10−4, although systems with large cloud complexes ≳ 50 pc require jets of Eddington ratio in excess of 10−2 to disperse the clouds appreciably. Based on measurements of the bubble expansion rates in our simulations, we argue that sub-grid AGN prescriptions resulting in negative feedback in cosmological simulations without a multi-phase treatment of the ISM are good approximations if the volume filling factor of warm-phase material is less than 0.1 and the cloud complexes are smaller than ∼25 pc. We find that the acceleration of the dense embedded clouds is provided by the ram pressure of the high-velocity flow through the porous channels of the warm phase, flow that has fully entrained the shocked hot-phase gas it has swept up, and is additionally mass loaded by ablated cloud material. This mechanism transfers 10$\%$ to 40$\%$ of the jet energy to the cold and warm gas, accelerating it within a few 10 to 100  Myr to velocities that match those observed in a range of high- and low-redshift radio galaxies hosting powerful radio jets.}
}

@ARTICLE{Dasyra&Combes2016A&A...595L...7D,
       author = {{Dasyra}, K.~M. and {Combes}, F. and {Oosterloo}, T. and {Oonk}, J.~B.~R. and {Morganti}, R. and {Salom{\'e}}, P. and {Vlahakis}, N.},
        title = "{ALMA reveals optically thin, highly excited CO gas in the jet-driven winds of the galaxy IC 5063}",
      journal = {\aap},
     keywords = {ISM: jets and outflows, ISM: kinematics and dynamics, ISM: molecules, submillimeter: ISM, galaxies: active, galaxies: nuclei, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = nov,
       volume = {595},
          eid = {L7},
        pages = {L7},
          doi = {10.1051/0004-6361/201629689},
archivePrefix = {arXiv},
       eprint = {1609.03421},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...595L...7D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Maccagni2018...614...A42,
	author = {{Maccagni, F. M.} and {Morganti, R.} and {Oosterloo, T. A.} and {Oonk, J. B. R.} and {Emonts, B. H. C.}},
	title = {ALMA observations of AGN fuelling - The case of PKS B1718-649},
	DOI= "10.1051/0004-6361/201732269",
	url= "https://doi.org/10.1051/0004-6361/201732269",
	journal = {A\&A},
	year = 2018,
	volume = 614,
	pages = "A42",
}


@article{Murthy2019...629...A58,
	author = {{Murthy, Suma} and {Morganti, Raffaella} and {Oosterloo, Tom} and {Schulz, Robert} and {Mukherjee, Dipanjan} and {Wagner, Alexander Y.} and {Bicknell, Geoffrey} and {Prandoni, Isabella} and {Shulevski, Aleksandar}},
	title = {Feedback from low-luminosity radio galaxies: B2 0258+35},
	DOI= "10.1051/0004-6361/201935931",
	url= "https://doi.org/10.1051/0004-6361/201935931",
	journal = {A\&A},
	year = 2019,
	volume = 629,
	pages = "A58",
}

@article{Oosterloo2017...608...A38,
	author = {{Oosterloo, Tom} and {Raymond Oonk, J. B.} and {Morganti, Raffaella} and {Combes, Fran\c{c}oise} and {Dasyra, Kalliopi} and {Salom\'e, Philippe} and {Vlahakis, Nektarios} and {Tadhunter, Clive}},
	title = {Properties of the molecular gas in the fast outflow  in the Seyfert galaxy IC 5063},
	DOI= "10.1051/0004-6361/201731781",
	url= "https://doi.org/10.1051/0004-6361/201731781",
	journal = {A\&A},
	year = 2017,
	volume = 608,
	pages = "A38",
}


@article{Schulz2018...617...A38,
	author = {{Schulz, R.} and {Morganti, R.} and {Nyland, K.} and {Paragi, Z.} and {Mahony, E. K.} and {Oosterloo, T.}},
	title = {Mapping the neutral atomic hydrogen gas outflow in the restarted radio galaxy 3C 236		},
	DOI= "10.1051/0004-6361/201833108",
	url= "https://doi.org/10.1051/0004-6361/201833108",
	journal = {A\&A},
	year = 2018,
	volume = 617,
	pages = "A38",
}


@article{Schulz2021...647...A63,
	author = {{Schulz, R.} and {Morganti, R.} and {Nyland, K.} and {Paragi, Z.} and {Mahony, E. K.} and {Oosterloo, T.}},
	title = {Parsec-scale HI outflows in powerful radio galaxies},
	DOI= "10.1051/0004-6361/202037677",
	url= "https://doi.org/10.1051/0004-6361/202037677",
	journal = {A\&A},
	year = 2021,
	volume = 647,
	pages = "A63",
}



@article{DeGouveiaDalPino2018proc,
     title={AGN and Star Formation Feedback in Galaxy Outflows}, 
     volume={14}, 
     DOI={10.1017/S174392131800604X}, 
     number={S342}, 
     journal={Proceedings of the International Astronomical Union}, 
     publisher={Cambridge University Press}, 
     author={de Gouveia Dal Pino, Elisabete M. and Clavijo-Bohórquez, William and Melioli, Claudio},
     year={2018}, 
     pages={229–233}
}



@article{Holt2008,
    author = {Holt, J. and Tadhunter, C. N. and Morganti, R.},
    title = "{Fast outflows in compact radio sources: evidence for AGN-induced feedback in the early stages of radio source evolution}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {387},
    number = {2},
    pages = {639-659},
    year = {2008},
    month = {05},
    abstract = "{We present intermediate-resolution, wide-wavelength coverage spectra for a complete sample of 14 compact radio sources taken with the aim of investigating the impact of the nuclear activity on the circumnuclear interstellar medium (ISM) in the early stages of radio source evolution. We observe spatially extended line emission (up to ∼20 kpc) in the majority of sources which is consistent with a quiescent halo. In the nuclear apertures we observe broad, highly complex emission-line profiles. Multiple Gaussian modelling of the [O iii]λ5007 line reveals between two and four components which can have velocity widths [full width at half-maximum (FWHM)] and blueshifts relative to the halo of up to ∼2000 km s−1. We interpret these broad, blueshifted components as material in outflow and discuss the kinematical evidence for jet-driven outflows as previously proposed for PKS 1549−79 and PKS 1345+12. Comparisons with samples in the literature show that compact radio sources harbour more extreme nuclear kinematics than their extended counterparts, a trend seen within our sample with larger velocities in the smaller sources. The observed velocities are also likely to be influenced by source orientation with respect to the observer's line of sight. Nine sources have associated H i absorption. In common with the optical emission-line gas, the H i profiles are often highly complex with the majority of the detected components significantly blueshifted, tracing outflows in the neutral gas. The sample has been tested for stratification in the ISM (FWHM/ionization potential/critical density) as suggested by Holt, Tadhunter \\&amp; Morganti for PKS 1345+12 but we find no significant trends within the sample using a Spearman rank analysis. This study supports the idea that compact radio sources are young radio-loud active galactic nuclei observed during the early stages of their evolution and currently shedding their natal cocoons through extreme circumnuclear outflows.}",
    issn = {0035-8711},
    doi = {10.1111/j.1365-2966.2008.13089.x},
    url = {https://doi.org/10.1111/j.1365-2966.2008.13089.x},
    eprint = {https://academic.oup.com/mnras/article-pdf/387/2/639/3371112/mnras0387-0639.pdf},
}

@article{Rose2017....474...128-156,
    author = {Rose, Marvin and Tadhunter, Clive and Ramos Almeida, Cristina and Rodríguez Zaurín, Javier and Santoro, Francesco and Spence, Robert},
    title = "{Quantifying the AGN-driven outflows in ULIRGs (QUADROS) – I: VLT/Xshooter observations of nine nearby objects}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {474},
    number = {1},
    pages = {128-156},
    year = {2017},
    month = {10},
    abstract = "{Although now routinely incorporated into hydrodynamic simulations of galaxy evolution, the true importance of the feedback effect of the outflows driven by active galactic nuclei (AGNs) remains uncertain from an observational perspective. This is due to a lack of accurate information on the densities, radial scales and level of dust extinction of the outflow regions. Here we use the unique capabilities of VLT/Xshooter to investigate the warm outflows in a representative sample of nine local (0.06 \\&lt; z \\&lt; 0.15) Ultraluminous Infrared Galaxies (ULIRGs) with AGNs and, for the first time, accurately quantify the key outflow properties. We find that the outflows are compact (0.06 \\&lt; \\$R\_\\{\\rm [O\\, \\small \\{III\\}]\\}\\$ \\&lt; 1.2 kpc), significantly reddened (median E(B − V) ∼ 0.5 magnitudes), and have relatively high electron densities (3.4 \\&lt; log10ne (cm−3) \\&lt; 4.8). It is notable that the latter densities – obtained using trans-auroral [S ii] and [O ii] emission-line ratios – exceed those typically assumed for the warm, emission-line outflows in active galaxies, but are similar to those estimated for broad and narrow absorption line outflow systems detected in some type 1 AGN. Even if we make the most optimistic assumptions about the true (deprojected) outflow velocities, we find relatively modest mass outflow rates (\\$0.07 \\&lt; \\dot\\{M\\} \\&lt; 14\\$ M⊙ yr−1) and kinetic powers measured as a fraction of the AGN bolometric luminosities (\\$4\\times 10^\\{-4\\} \\&lt; \\dot\\{E\\}/L\_\\{\\{\\rm BOL\\}\\} \\&lt; 0.8\\$ per cent). Therefore, although warm, AGN-driven outflows have the potential to strongly affect the star formation histories in the inner bulge regions (r ∼ 1 kpc) of nearby ULIRGs, we lack evidence that they have a significant impact on the evolution of these rapidly evolving systems on larger scales.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/stx2590},
    url = {https://doi.org/10.1093/mnras/stx2590},
    eprint = {https://academic.oup.com/mnras/article-pdf/474/1/128/22141778/stx2590.pdf},
}



@article{Bischetti2019...628...A118,
	author = {{Bischetti, M.} and {Piconcelli, E.} and {Feruglio, C.} and {Fiore, F.} and {Carniani, S.} and {Brusa, M.} and {Cicone, C.} and {Vignali, C.} and {Bongiorno, A.} and {Cresci, G.} and {Mainieri, V.} and {Maiolino, R.} and {Marconi, A.} and {Nardini, E.} and {Zappacosta, L.}},
	title = {The gentle monster PDS 456 - Kiloparsec-scale molecular outflow and its implications for QSO feedback},
	DOI= "10.1051/0004-6361/201935524",
	url= "https://doi.org/10.1051/0004-6361/201935524",
	journal = {A\&A},
	year = 2019,
	volume = 628,
	pages = "A118",
}

@article{Santoro2018...617...A139,
	author = {{Santoro, F.} and {Rose, M.} and {Morganti, R.} and {Tadhunter, C.} and {Oosterloo, T. A.} and {Holt, J.}},
	title = {Probing multi-phase outflows and AGN feedback in compact radio galaxies: the case of PKS B1934-63},
	DOI= "10.1051/0004-6361/201833248",
	url= "https://doi.org/10.1051/0004-6361/201833248",
	journal = {A\&A},
	year = 2018,
	volume = 617,
	pages = "A139",
}

@misc{Barai2019.arxiv.1903.04632,
  doi = {10.48550/ARXIV.1903.04632},
  url = {https://arxiv.org/abs/1903.04632},
  author = {Barai, Paramita and de Gouveia Dal Pino, Elisabete M.},
  keywords = {Astrophysics of Galaxies (astro-ph.GA), Cosmology and Nongalactic Astrophysics (astro-ph.CO), High Energy Astrophysical Phenomena (astro-ph.HE), FOS: Physical sciences, FOS: Physical sciences},
  title = {Supermassive and Intermediate-Mass Black Hole Growth at Galaxy Centers and Resulting Feedback using Cosmological Simulations},
  publisher = {arXiv},
  year = {2019},
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@article{Forbes&Norris1998MNRAS.300..757F,
       author = {{Forbes}, Duncan A. and {Norris}, R.~P.},
        title = "{Star formation in southern Seyfert galaxies}",
      journal = {\mnras},
     keywords = {STARS: FORMATION, GALAXIES: NUCLEI, GALAXIES: SEYFERT, RADIO CONTINUUM: GALAXIES, Astrophysics},
         year = 1998,
        month = nov,
       volume = {300},
       number = {3},
        pages = {757-766},
          doi = {10.1046/j.1365-8711.1998.01940.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/9804298},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998MNRAS.300..757F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Rodenbeck2016,
abstract = {Galaxy mergers are expected to play a central role for the evolution of galaxies and may have a strong effect on their magnetic fields. We present the first grid-based 3D magnetohydrodynamical simulations investigating the evolution of magnetic fields during merger events. For this purpose, we employed a simplified model considering the merger event of magnetized gaseous disks in the absence of stellar feedback and without a stellar or dark matter component. We show that our model naturally leads to the production of two peaks in the evolution of the average magnetic field strength within 5 kpc, within 25 kpc, and on scales in between 5 and 25 kpc. The latter is consistent with the peak in the magnetic field strength previously reported in a merger sequence of observed galaxies. We show that the peak on the galactic scale and in the outer regions is most likely due to geometrical effects, as the core of one galaxy enters the outskirts of the other one. In addition, the magnetic field within the central ∼5 kpc is physically enhanced, which reflects the enhancement in density that is due to efficient angular momentum transport. We conclude that high-resolution observations of the central regions will be particularly relevant for probing the evolution of magnetic field structures during merger events.},
author = {Rodenbeck, Kai and Schleicher, Dominik R.G.},
doi = {10.1051/0004-6361/201527393},
file = {:home/william/Documents/Papers/aa27393-15.pdf:pdf},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Galaxies: interactions,Galaxies: magnetic fields,Galaxy: evolution,Methods: numerical},
pages = {1--12},
title = {{Magnetic fields during galaxy mergers}},
volume = {593},
year = {2016}
}


@article{Ntormousi2018,
abstract = {Context. Magnetic fields play a very important role in the evolution of galaxies through their direct impact on star formation and stellar feedback-induced turbulence. However, their co-evolution with these processes has still not been thoroughly investigated, and the possible effect of the initial conditions is largely unknown. Aims. This Letter presents the first results from a series of high-resolution numerical models, aimed at deciphering the effect of the initial conditions and of stellar feedback on the evolution of the galactic magnetic field in isolated Milky Way-like galaxies. Methods. The models start with an ordered magnetic field of varying strength, either poloidal or toroidal, and are evolved with and without supernova feedback. They include a dark matter halo, a stellar and a gaseous disk, as well as the appropriate cooling and heating processes for the interstellar medium. Results. Independently of the initial conditions, the galaxies develop a turbulent velocity field and a random magnetic field component in under 15 Myr. Supernova feedback is extremely efficient in building a random magnetic field component up to large galactic heights. However, a random magnetic field emerges even in runs without feedback, which points to an inherent instability of the ordered component. Conclusions. Supernova feedback greatly affects the velocity field of the galaxy up to large galactic heights, and helps restructure the magnetic field up to 10 kpc above the disk, independently of the initial magnetic field morphology. On the other hand, the initial morphology of the magnetic field can accelerate the development of a random component at large heights. These effects have important implications for the study of the magnetic field evolution in galaxy simulations.},
archivePrefix = {arXiv},
arxivId = {1810.08450},
author = {Ntormousi, Evangelia},
doi = {10.1051/0004-6361/201834153},
eprint = {1810.08450},
file = {:home/william/Documents/Papers/aa34153-18.pdf:pdf},
issn = {14320746},
journal = {Astron. Astrophys.},
keywords = {Galaxies: Magnetic fields,ISM: Magnetic fields,Magnetic fields},
pages = {1--4},
title = {{Magnetic fields in massive spirals: The role of feedback and initial conditions}},
volume = {619},
year = {2018}
}



@article{Haring.Rix,
abstract = {We have re-examined the relation between the mass of the central black holes in nearby galaxies, M{\_}bh, and the stellar mass of the surrounding spheroid or bulge, M{\_}bulge. For a total of 30 galaxies bulge masses were derived through Jeans equation modeling or adopted from dynamical models in the literature. In stellar mass-to-light ratios the spheroids and bulges span a range of a factor of eight. The bulge masses were related to well-determined black hole masses taken from the literature. With these improved values for M{\_}bh, compared to Magorrian et al. (1998), and our redetermination of M{\_}bulge, we find the M{\_}bh-M{\_}bulge relation becomes very tight. We find M{\_}bh {\~{}} M{\_}bulge{\^{}}(1.12+/-0.06) with an observed scatter of {\textless} 0.30 dex, a fraction of which can be attributed to measurement errors. The scatter in this relation is therefore comparable to the scatter in the relations of M{\_}bh with sigma and the stellar concentration. These results confirm and refine the work of Marconi and Hunt (2003). For M{\_}bulge{\~{}}5x10{\^{}}10 M{\_}sun the median black hole mass is 0.14{\%} +/- 0.04{\%} of the bulge mass.},
archivePrefix = {arXiv},
arxivId = {astro-ph/0402376},
author = {H{\"{a}}ring, Nadine and Rix, Hans-Walter},
doi = {10.1086/383567},
eprint = {0402376},
file = {:home/william/Documents/Papers/H{\"{a}}ring{\_}2004{\_}ApJ{\_}604{\_}L89.pdf:pdf},
issn = {0004-637X},
journal = {Astrophys. J.},
number = {2},
pages = {L89--L92},
primaryClass = {astro-ph},
title = {{On the Black Hole Mass-Bulge Mass Relation}},
volume = {604},
year = {2004}
}

@ARTICLE{Oosterloo2019A&A...632A..66O,
       author = {{Oosterloo}, Tom and {Morganti}, Raffaella and {Tadhunter}, Clive and {Raymond Oonk}, J.~B. and {Bignall}, Hayley E. and {Tzioumis}, Tasso and {Reynolds}, Cormac},
        title = "{ALMA observations of PKS 1549-79: a case of feeding and feedback in a young radio quasar}",
      journal = {\aap},
     keywords = {galaxies: active, galaxies: individual: PKS 1549-79, ISM: jets and outflows, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = dec,
       volume = {632},
          eid = {A66},
        pages = {A66},
          doi = {10.1051/0004-6361/201936248},
archivePrefix = {arXiv},
       eprint = {1910.07865},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...632A..66O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Murthy2022NatAs...6..488M,
       author = {{Murthy}, Suma and {Morganti}, Raffaella and {Wagner}, Alexander Y. and {Oosterloo}, Tom and {Guillard}, Pierre and {Mukherjee}, Dipanjan and {Bicknell}, Geoffrey},
        title = "{Cold gas removal from the centre of a galaxy by a low-luminosity jet}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = feb,
       volume = {6},
        pages = {488-495},
          doi = {10.1038/s41550-021-01596-6},
archivePrefix = {arXiv},
       eprint = {2202.05222},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022NatAs...6..488M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pain1996ApJ...473..356P,
       author = {{Pain}, R. and {Hook}, I.~M. and {Deustua}, S. and {Gabi}, S. and {Goldhaber}, G. and {Groom}, D. and {Kim}, A.~G. and {Kim}, M.~Y. and {Lee}, J.~C. and {Pennypacker}, C.~R. and {Perlmutter}, S. and {Small}, I.~A. and {Goobar}, A. and {Ellis}, R.~S. and {McMahon}, R.~G. and {Glazebrook}, K. and {Boyle}, B.~J. and {Bunclark}, P.~S. and {Carter}, D. and {Irwin}, M.~J.},
        title = "{The Type IA Supernova Rate at Z approximately 0.4}",
      journal = {\apj},
     keywords = {STARS: STATISTICS, STARS: SUPERNOVAE: GENERAL, SURVEYS, Astrophysics},
         year = 1996,
        month = dec,
       volume = {473},
        pages = {356},
          doi = {10.1086/178150},
archivePrefix = {arXiv},
       eprint = {astro-ph/9607034},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...473..356P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zubovas2012ApJ...745L..34Z,
       author = {{Zubovas}, Kastytis and {King}, Andrew},
        title = "{Clearing Out a Galaxy}",
      journal = {\apjl},
     keywords = {accretion, accretion disks, black hole physics, galaxies: evolution, quasars: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2012,
        month = feb,
       volume = {745},
       number = {2},
          eid = {L34},
        pages = {L34},
          doi = {10.1088/2041-8205/745/2/L34},
archivePrefix = {arXiv},
       eprint = {1201.0866},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...745L..34Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Thompson2006,
doi = {10.1086/504035},
url = {https://dx.doi.org/10.1086/504035},
year = {2006},
month = {jul},
publisher = {},
volume = {645},
number = {1},
pages = {186},
author = {Todd A. Thompson and Eliot Quataert and Eli Waxman and Norman Murray and Crystal L. Martin},
title = {Magnetic Fields in Starburst Galaxies and the Origin of the FIR-Radio Correlation},
journal = {The Astrophysical Journal},
abstract = {We estimate minimum energy magnetic fields (Bmin) for a sample of galaxies with measured gas surface densities, spanning more than four orders of magnitude in surface density, from normal spirals to luminous starbursts. We show that the ratio of the minimum energy magnetic pressure to the total pressure in the ISM decreases substantially with increasing surface density. For the ultraluminous infrared galaxy Arp 220, this ratio is ~10-4. Therefore, if the minimum energy estimate is applicable, magnetic fields in starbursts are dynamically weak compared to gravity, in contrast to normal star-forming spiral galaxies. We argue, however, that rapid cooling of relativistic electrons in starbursts invalidates the minimum energy estimate. We assess a number of independent constraints on the magnetic field strength in starburst galaxies. In particular, we argue that the existence of the FIR-radio correlation implies that the synchrotron cooling timescale for cosmic-ray electrons is much shorter than their escape time from the galactic disk; this in turn implies that the true magnetic field in starbursts is significantly larger than Bmin. The strongest argument against such large fields is that one might expect starbursts to have steep radio spectra indicative of strong synchrotron cooling, which is not observed. However, we show that ionization and bremsstrahlung losses can flatten the nonthermal spectra of starburst galaxies even in the presence of rapid cooling, providing much better agreement with observed spectra. We further demonstrate that ionization and bremsstrahlung losses are likely to be important in shaping the radio spectra of most starbursts at GHz frequencies, thereby preserving the linearity of the FIR-radio correlation. We thus conclude that magnetic fields in starbursts are significantly larger than Bmin. We highlight several observations that can test this conclusion.}
}



@article{Tanner_2022,
doi = {10.3847/1538-3881/ac4d23},
url = {https://dx.doi.org/10.3847/1538-3881/ac4d23},
year = {2022},
month = {feb},
publisher = {The American Astronomical Society},
volume = {163},
number = {3},
pages = {134},
author = {Ryan Tanner and Kimberly A. Weaver},
title = {Simulations of AGN-driven Galactic Outflow Morphology and Content},
journal = {The Astronomical Journal},
abstract = {Using a series of 3D relativistic hydrodynamical simulations of active galactic nuclei (AGN) we investigate how AGN power, a clumpy interstellar medium (ISM) structure, and AGN jet angle with respect to the galactic disk affect the morphology and content of the resulting galactic outflow. For low-power AGN across three orders of magnitude of AGN luminosities (1041–1043 erg s−1) our simulations did not show significant changes to either the morphology or total mass of the outflow. Changing the angle of the AGN jet with respect to the galaxy did show small changes in the total outflow mass of a factor of 2–3. Jets perpendicular to the galactic disk created hot single-phase outflows, while jets close to parallel with the disk created multiphase outflows with equal parts warm and hot, and significant cold gas. Overall the final morphology of low-power AGN outflows depends primarily on how the jet impacts and interacts with large, dense clouds in the clumpy ISM. These clouds can disrupt, deflect, split, or suppress the jet, preventing it from leaving the galactic disk as a coherent structure. But for simulations with AGN luminosities &gt; 1044 erg s−1 the ISM played a minor role in determining the morphology of the outflow with an undisrupted jet leaving the disk. The final morphology of AGN outflows is different for low-power AGNs versus high-power AGNs with the final morphology of low-power AGN outflows dependent on the ISM structure within the first kiloparsec surrounding the AGN.}
}



@ARTICLE{Barreto-Mota2021.503.5425B,
       author = {{Barreto-Mota}, L. and {de Gouveia Dal Pino}, E.~M. and {Burkhart}, B. and {Melioli}, C. and {Santos-Lima}, R. and {Kadowaki}, L.~H.~S.},
        title = "{Magnetic field orientation in self-gravitating turbulent molecular clouds}",
      journal = {\mnras},
     keywords = {turbulence, stars: formation, ISM: kinematics and dynamics, galaxies: ISM, galaxies: star formation, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = jun,
       volume = {503},
       number = {4},
        pages = {5425-5447},
          doi = {10.1093/mnras/stab798},
archivePrefix = {arXiv},
       eprint = {2101.03246},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.503.5425B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Thompson2015,
    author = {Thompson, Todd A. and Fabian, Andrew C. and Quataert, Eliot and Murray, Norman},
    title = "{Dynamics of dusty radiation-pressure-driven shells and clouds: fast outflows from galaxies, star clusters, massive stars, and AGN}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {449},
    number = {1},
    pages = {147-161},
    year = {2015},
    month = {03},
    abstract = "{It is typically assumed that radiation-pressure-driven winds are accelerated to an asymptotic velocity of v∞ ≃ vesc, where vesc is the escape velocity from the central source. We note that this is not the case for dusty shells and clouds. Instead, if the shell or cloud is initially optically thick to the UV emission from the source of luminosity L, then there is a significant boost in v∞ that reflects the integral of the momentum absorbed as it is accelerated. For shells reaching a generalized Eddington limit, we show that v∞ ≃ (4RUVL/Mshc)1/2, in both point-mass and isothermal-sphere potentials, where RUV is the radius where the shell becomes optically thin to UV photons, and Msh is the mass of the shell. The asymptotic velocity significantly exceeds vesc for typical parameters, and can explain the ∼1000–2000 km s−1 outflows observed from rapidly star-forming galaxies and active galactic nuclei (AGN) if the surrounding halo has low gas density. Similarly fast outflows from massive stars can be accelerated on ∼few–103 yr time-scales. These results carry over to clouds that subtend only a small fraction of the solid angle from the source of radiation and that expand as a consequence of their internal sound speed. We further consider the dynamics of shells that sweep up a dense circumstellar or circumgalactic medium. We calculate the ‘momentum ratio’ \\$\\dot\\{M\\} v/(L/c)\\$ in the shell limit and show that it can only significantly exceed ∼2 if the effective optical depth of the shell to re-radiated far-infrared photons is much larger than unity. We discuss simple prescriptions for the properties of galactic outflows for use in large-scale cosmological simulations. We also briefly discuss applications to the dusty ejection episodes of massive stars, the disruption of giant molecular clouds, and AGN.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/stv246},
    url = {https://doi.org/10.1093/mnras/stv246},
    eprint = {https://academic.oup.com/mnras/article-pdf/449/1/147/4130198/stv246.pdf},
}

@article{Sharma_2013,
doi = {10.1088/0004-637X/763/1/17},
url = {https://dx.doi.org/10.1088/0004-637X/763/1/17},
year = {2012},
month = {dec},
publisher = {The American Astronomical Society},
volume = {763},
number = {1},
pages = {17},
author = {Mahavir Sharma and Biman B. Nath},
title = {SUPERNOVAE AND AGN DRIVEN GALACTIC OUTFLOWS},
journal = {The Astrophysical Journal},
abstract = {We present analytical solutions for winds from galaxies with a Navarro–Frank–White (NFW) dark matter halo. We consider winds driven by energy and mass injection from multiple supernovae (SNe), as well as momentum injection due to radiation from a central black hole. We find that the wind dynamics depends on three velocity scales: (1)  describes the effect of starburst activity, with  as energy and mass injection rate in a central region of radius R; (2) v• ∼ (GM•/2R)1/2 for the effect of a central black hole of mass M• on gas at distance R; and (3) , which is closely related to the circular speed (vc) for an NFW halo, where rs is the halo scale radius and  is a function of the halo concentration parameter. Our generalized formalism, in which we treat both energy and momentum injection from starbursts and radiation from the central active galactic nucleus (AGN), allows us to estimate the wind terminal speed to be (4v2⋆ + 6(Γ − 1)v•2 − 4v2s)1/2, where Γ is the ratio of force due to radiation pressure to gravity of the central black hole. Our dynamical model also predicts the following: (1) winds from quiescent star-forming galaxies cannot escape from 1011.5 M☉ ⩽ Mh ⩽ 1012.5 M☉ galaxies; (2) circumgalactic gas at large distances from galaxies should be present for galaxies in this mass range; (3) for an escaping wind, the wind speed in low- to intermediate-mass galaxies is ∼400–1000 km s−1, consistent with observed X-ray temperatures; and (4) winds from massive galaxies with AGNs at Eddington limit have speeds ≳ 1000 km s−1. We also find that the ratio [2v2⋆ − (1 − Γ)v•2]/v2c dictates the amount of gas lost through winds. Used in conjunction with an appropriate relation between M• and Mh and an appropriate opacity of dust grains in infrared (K band), this ratio has the attractive property of being minimum at a certain halo mass scale (Mh ∼ 1012–1012.5 M☉) that signifies the crossover of AGN domination in outflow properties from starburst activity at lower masses. We find that stellar mass for massive galaxies scales as M⋆∝M0.26h, and for low-mass galaxies, M⋆∝M5/3h.}
}

@article{Yu2020,
    author = {Yu, B P Brian and Owen, Ellis R and Wu, Kinwah and Ferreras, Ignacio},
    title = "{A hydrodynamical study of outflows in starburst galaxies with different driving mechanisms}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {492},
    number = {3},
    pages = {3179-3193},
    year = {2020},
    month = {01},
    abstract = "{Outflows from starburst galaxies can be driven by thermal pressure, radiation, and cosmic rays. We present an analytic phenomenological model that accounts for these contributions simultaneously to investigate their effects on the hydrodynamical properties of outflows. We assess the impact of energy injection, wind opacity, magnetic field strength, and the mass of the host galaxy on flow velocity, temperature, density, and pressure profiles. For an M82-like wind, a thermally dominated driving mechanism is found to deliver the fastest and hottest wind. Radiation-driven winds in typical starburst-galaxy configurations are unable to attain the higher flow velocities and temperatures associated with thermal and cosmic ray-driven systems, leading to higher wind densities which would be more susceptible to cooling and fragmentation at lower altitudes. High opacity winds are more sensitive to radiative driving, but terminal flow velocities are still lower than those achieved by other driving mechanisms at realistic opacities. We demonstrate that variations in the outflow magnetic field can influence its coupling with cosmic rays, where stronger fields enable greater streaming but less driving near the base of the flow, instead with cosmic rays redirecting their driving impact to higher altitudes. The gravitational potential is less important in M82-like wind configurations, and substantial variations in the flow profiles only emerge at high altitude in massive haloes. This model offers a more generalized approach to examine the large-scale hydrodynamical properties for a wide variety of starburst galaxies.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/staa021},
    url = {https://doi.org/10.1093/mnras/staa021},
    eprint = {https://academic.oup.com/mnras/article-pdf/492/3/3179/31922475/staa021.pdf},
}

@ARTICLE{Viegas1992,
       author = {{Viegas}, S.~M. and {de Gouveia dal Pino}, E.~M.},
        title = "{The Origin of the Optical Emission Lines Associated with Extragalactic Radio Sources}",
      journal = {\apj},
     keywords = {Emission Spectra, Extragalactic Radio Sources, Line Spectra, Radio Jets (Astronomy), Star Formation, Abundance, Astronomical Models, Photoionization, Radio Astronomy, Astrophysics, GALAXIES: JETS, LINE: FORMATION, RADIO CONTINUUM: GALAXIES, STARS: FORMATION},
         year = 1992,
        month = jan,
       volume = {384},
        pages = {467},
          doi = {10.1086/170888},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992ApJ...384..467V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lopez-Rodriguez2021NatAs...5..604L,
       author = {{Lopez-Rodriguez}, Enrique},
        title = "{The magnetic field across the molecular warped disk of Centaurus A}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = jun,
       volume = {5},
        pages = {604-614},
          doi = {10.1038/s41550-021-01329-9},
archivePrefix = {arXiv},
       eprint = {2104.00688},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021NatAs...5..604L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Leitherer1999ApJS..123....3L,
       author = {{Leitherer}, Claus and {Schaerer}, Daniel and {Goldader}, Jeffrey D. and {Delgado}, Rosa M. Gonz{\'a}lez and {Robert}, Carmelle and {Kune}, Denis Foo and {de Mello}, Du{\'\i}lia F. and {Devost}, Daniel and {Heckman}, Timothy M.},
        title = "{Starburst99: Synthesis Models for Galaxies with Active Star Formation}",
      journal = {\apjs},
     keywords = {GALAXIES: EVOLUTION, GALAXIES: FUNDAMENTAL PARAMETERS, GALAXIES: STARBURST, GALAXIES: STELLAR CONTENT, METHODS: NUMERICAL, Galaxies: Evolution, Galaxies: Fundamental Parameters, Galaxies: Starburst, Galaxies: Stellar Content, Methods: Numerical, Astrophysics},
         year = 1999,
        month = jul,
       volume = {123},
       number = {1},
        pages = {3-40},
          doi = {10.1086/313233},
archivePrefix = {arXiv},
       eprint = {astro-ph/9902334},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJS..123....3L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Farber2022MNRAS.510..551F,
       author = {{Farber}, Ryan J. and {Gronke}, Max},
        title = "{The survival of multiphase dusty clouds in hot winds}",
      journal = {\mnras},
     keywords = {hydrodynamics, ISM: clouds, ISM: molecules, Galaxy: halo, galaxies: evolution, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = feb,
       volume = {510},
       number = {1},
        pages = {551-567},
          doi = {10.1093/mnras/stab3412},
archivePrefix = {arXiv},
       eprint = {2107.07991},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.510..551F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


